X-ray absorption lines in FUV-detected quasars: I. Sample and analysis of the XMM-Newton and Chandra data

This paper presents initial results of a systematic search for resonance X-ray absorption lines from H-like O VIII and He-like O VII caused by the intervening warm-hot intergalactic medium (WHIM). The search is based on far ultra-violet redshift priors from O VI and H I broad Lyman-alpha lines that were previously detected by HST and FUSE in a sample of 51 sources with either XMM-Newton or Chandra data, for a total X-ray redshift path of $\Delta z$ = 10.9. Of the 1,224 absorption-line systems with FUV priors that were analyzed, 33 systems feature an absorption-line feature detected with $\geq$99 % confidence at the same redshift of the FUV prior, some coincident with previously reported absorption line detections. The ultimate goal of this search is to test the hypothesis that X-ray absorbing WHIM gas is the repository of the missing baryons in the local universe. Further results and the cosmological implications of this analysis are presented in a companion paper.

==> ADAPTableEdited.tex <==
1 & 1ES1028+511 & 0.3604 & 4 & 3 & 5 & 312 & 1 & 149   \\
2 & 1ES1553+113 & 0.4140 & 7 & 4 & 22 & 1998 & 3 & 496   \\
3 & 3C249 & 0.3115 & 4 & 2 & 1 & 37 & 0 & 0 \\
4 & 3C273 & 0.1583 & 10 & 4 & 35 & 1282 & 2 & 70   \\
5 & 3C66A & 0.3347 & 2 & 1 & 2 & 27 & 0 & 0   \\
6 & H1821+643 & 0.2968 & 15 & 7 & 15 & 130 & 4 & 470   \\
7 & H2356-309 & 0.1651 & 2 & 4 & 9 & 704 & 11 & 587   \\
8 & HE0056-3622 & 0.1641 & 2 & 0 & 4 & 186 & 0 & 0   \\
9 & HE0226-4110 & 0.4934 & 61 & 3 & 1 & 33 & 0 & 0   \\
10 & IRASF22456-5125 & 0.1000 & 8 & 2 & 4 & 108 & 0 & 0   \\
11 & MR2251-178 & 0.0640 & 1 & 7 & 10 & 610 & 1 & 78   \\
12 & Mrk421 & 0.0300 & 1 & 0 & 102 & 2876 & 38 & 639  \\
13 & Mrk478 & 0.0791 & 0 & 3 & 5 & 252 & 1 & 80   \\
14 & Mrk876 & 0.1290 & 6 & 6 & 2 & 21 & 0 & 0   \\
15 & NGC7469 & 0.0163 & 3 & 1 & 11 & 857 & 0 & 0  \\
16 & PG0157+001 & 0.1631 & 1 & 0 & 1 & 15 & 0 & 0   \\
17 & PG0003+158 & 0.4509 & 17 & 5 & 1 & 26 & 0 & 0   \\
18 & PG0804+761 & 0.1000 & 4 & 3 & 3 & 103 & 0 & 0   \\
19 & PG0832+251 & 0.3298 & 5 & 8 & 1 & 23 & 0 & 0   \\
20 & PG0838+770 & 0.1310 & 0 & 3 & 1 & 24 & 0 & 0   \\
21 & PG0953+414 & 0.2341 & 11 & 2 & 1 & 16 & 0 & 0   \\
22 & PG1048+342 & 0.1671 & 0 & 2 & 1 & 33 & 0 & 0   \\
23 & PG1115+407 & 0.1546 & 5 & 3 & 1 & 21 & 0 & 0   \\
24 & PG1116+215 & 0.1763 & 9 & 9 & 6 & 395 & 11 & 356   \\
25 & PG1211+143 & 0.0809 & 4 & 2 & 12 & 883 & 3 & 134  \\
26 & PG1216+069 & 0.3313 & 8 & 8 & 1 & 17 & 0 & 0   \\
27 & PG1229+204 & 0.0630 & 0 & 1 & 1 & 26 & 0 & 0   \\
28 & PG1259+593 & 0.4778 & 14 & 10 & 1 & 34 & 0 & 0   \\
29 & PG1307+085 & 0.1550 & 2 & 1 & 1 & 14 & 0 & 0   \\
30 & PG1309+355 & 0.1829 & 11 & 5 & 1 & 30 & 0 & 0   \\
31 & PG1444+407 & 0.2673 & 6 & 1 & 1 & 22 & 0 & 0  \\
32 & PG1626+554 & 0.1330 & 1 & 1 & 1 & 11 & 0 & 0   \\
33 & PHL1811 & 0.1920 & 13 & 6 & 2 & 92 & 0 & 0   \\
34 & PKS0312-770 & 0.2230 & 2 & 1 & 4 & 153 & 0 & 0\\
35 & PKS0405-123 & 0.5740 & 26 & 13 & 2 & 170 & 4 & 376   \\
36 & PKS0558-504 & 0.1372 & 0 & 1 & 20 & 1096 & 0 & 0   \\
37 & PKS1302-102 & 0.2784 & 11 & 8 & 1 & 16 & 0 & 0   \\
38 & PKS2005-489 & 0.0710 & 1 & 0 & 3 & 62 & 4 & 282   \\
39 & PKS2155-304 & 0.1165 & 2 & 4 & 36 & 2191 & 15 & 319   \\
40 & PMNJ1103-2329 & 0.1860 & 5 & 0 & 2 & 27 & 0 & 0   \\
41 & PMNJ2345-1555 & 0.6210 & 12 & 5 & 1 & 32 & 0 & 0   \\
42 & Q1230+0115 & 0.1170 & 15 & 13 & 1 & 71 & 0 & 0   \\
43 & QSO0045+3926 & 0.1340 & 2 & 2 & 1 & 17 & 0 & 0   \\
44 & RBS1892 & 0.2000 & 3 & 6 & 1 & 22 & 0 & 0   \\
45 & RBS542 & 0.1040 & 2 & 2 & 11 & 369 & 0 & 0   \\
46 & RXJ0439.6-5311 & 0.2430 & 7 & 2 & 2 & 162 & 0 & 0   \\
47 & S50716+714 & 0.2315 & 1 & 4 & 5 & 180 & 0 & 0   \\
48 & TonS210 & 0.1160 & 0 & 2 & 1 & 9 & 0 & 0   \\
49 & Ton28 & 0.3297 & 7 & 1 & 3 & 108 & 0 & 0  \\
50 & Ton580 & 0.2902 & 2 & 0 & 2 & 48 & 0 & 0   \\
51 & TonS180 & 0.0620 & 3 & 1 & 4 & 223 & 1 & 77  \\


==> HI_DanforthTilton.tex <==
\begin{longtable}{lllccccc}
\# & Name & Redshift & $\log N$ (cm$^{-2}$) & $b$ (km~s$^{-1}$) & Source\\ 
\hline
1 & 1es1028 & 0.13714 & 13.3$\pm$0.1 & 91.60$\pm$24.00 & Danforth \\ 
2 & 1es1028 & 0.20383 & 13.2$\pm$0.1 & 63.60$\pm$14.20 & Danforth \\ 
3 & 1es1028 & 0.22121 & 13.4$\pm$0.8 & 68.60$\pm$71.40 & Danforth \\ 
\hline
4 & 1es1553 & 0.03466 & 13.1$\pm$0.0 & 72.00$\pm$9.40 & Danforth \\ 
5 & 1es1553 & 0.04273 & 13.4$\pm$0.0 & 63.00$\pm$4.50 & Danforth \\ 
6 & 1es1553 & 0.06364 & 13.0$\pm$0.2 & 76.30$\pm$19.90 & Danforth \\ 
7 & 1es1553 & 0.21869 & 12.7$\pm$0.1 & 62.60$\pm$21.80 & Danforth \\ 
\hline
8 & 3c249 & 0.13470 & 13.1$\pm$0.1 & 65.00$\pm$2.00 & Tilton \\ 
9 & 3c249 & 0.26664 & 13.3$\pm$0.1 & 67.00$\pm$19.00 & Tilton \\ 
\hline
10 & 3c263 & 0.06003 & 13.0$\pm$0.1 & 71.30$\pm$21.70 & Danforth \\ 
11 & 3c263 & 0.14073 & 13.5$\pm$0.1 & 83.70$\pm$11.70 & Danforth \\ 
12 & 3c263 & 0.26322 & 12.9$\pm$0.1 & 61.00$\pm$17.40 & Danforth \\ 
13 & 3c263 & 0.31025 & 13.1$\pm$0.1 & 81.90$\pm$19.80 & Danforth \\ 
14 & 3c263 & 0.37740 & 13.4$\pm$0.1 & 85.80$\pm$11.30 & Danforth \\ 
\hline
15 & 3c273 & 0.00758 & 13.0$\pm$0.0 & 74.40$\pm$8.60 & Danforth \\ 
16 & 3c273 & 0.06707 & 12.6$\pm$0.1 & 73.60$\pm$27.60 & Danforth \\ 
17 & 3c273 & 0.07359 & 12.8$\pm$0.1 & 99.70$\pm$18.00 & Danforth \\ 
18 & 3c273 & 0.13960 & 12.6$\pm$0.1 & 64.90$\pm$8.70 & Danforth \\ 
\hline
19 & 3c351 & 0.06008 & 13.2$\pm$0.1 & 67.00$\pm$8.00 & Tilton \\ 
20 & 3c351 & 0.06592 & 13.9$\pm$0.0 & 118.20$\pm$5.60 & Tilton \\ 
21 & 3c351 & 0.18191 & 13.4$\pm$0.1 & 106.00$\pm$4.00 & Tilton \\ 
\hline
22 & 3c57 & 0.19558 & 13.2$\pm$0.1 & 71.30$\pm$12.00 & Danforth \\ 
23 & 3c57 & 0.25994 & 13.3$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
24 & 3c57 & 0.37357 & 13.7$\pm$0.0 & 62.00$\pm$6.70 & Danforth \\ 
25 & 3c57 & 0.44937 & 13.6$\pm$0.1 & 64.90$\pm$13.90 & Danforth \\ 
\hline
26 & 3c66a & 0.08850 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
\hline
27 & b0117 & 0.14156 & 13.7$\pm$0.0 & 69.10$\pm$5.40 & Danforth \\ 
28 & b0117 & 0.16029 & 13.0$\pm$0.1 & 95.60$\pm$29.50 & Danforth \\ 
\hline
29 & f1010 & 0.01614 & 13.2$\pm$0.1 & 88.30$\pm$31.00 & Danforth \\ 
\hline
30 & h1821 & 0.00944 & 13.0$\pm$0.0 & 61.20$\pm$6.90 & Danforth \\ 
31 & h1821 & 0.06779 & 12.7$\pm$0.1 & 87.50$\pm$20.80 & Danforth \\ 
32 & h1821 & 0.08483 & 12.9$\pm$0.1 & 80.60$\pm$17.30 & Danforth \\ 
33 & h1821 & 0.12147 & 13.8$\pm$0.1 & 77.00$\pm$5.00 & Tilton \\ 
34 & h1821 & 0.19817 & 12.9$\pm$0.1 & 71.50$\pm$11.60 & Danforth \\ 
35 & h1821 & 0.21321 & 13.6$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
36 & h1821 & 0.24531 & 13.2$\pm$0.1 & 72.00$\pm$22.50 & Danforth \\ 
\hline
37 & h2356 & 0.03830 & 13.3$\pm$0.1 & 92.40$\pm$20.00 & Danforth \\ 
38 & h2356 & 0.07881 & 13.4$\pm$0.2 & 99.80$\pm$34.30 & Danforth \\ 
39 & h2356 & 0.10467 & 13.5$\pm$0.1 & 71.90$\pm$10.80 & Danforth \\ 
40 & h2356 & 0.15613 & 13.6$\pm$0.1 & 61.00$\pm$15.40 & Danforth \\ 
\hline
41 & he0153 & 0.11318 & 13.7$\pm$0.0 & 69.60$\pm$3.70 & Danforth \\ 
42 & he0153 & 0.17060 & 13.7$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
\hline
43 & he0226 & 0.14274 & 12.8$\pm$0.1 & 63.50$\pm$13.20 & Danforth \\ 
44 & he0226 & 0.39890 & 13.6$\pm$0.1 & 84.00$\pm$27.00 & Tilton \\ 
45 & he0226 & 0.41024 & 13.3$\pm$0.1 & 69.40$\pm$12.10 & Danforth \\ 
\hline
46 & he0238 & 0.10641 & 13.3$\pm$0.1 & 60.50$\pm$6.20 & Danforth \\ 
47 & he0238 & 0.14922 & 13.1$\pm$0.1 & 75.20$\pm$22.00 & Danforth \\ 
48 & he0238 & 0.18747 & 13.1$\pm$0.0 & 62.60$\pm$7.90 & Danforth \\ 
49 & he0238 & 0.27913 & 13.4$\pm$0.0 & 62.10$\pm$7.30 & Danforth \\ 
50 & he0238 & 0.33435 & 13.7$\pm$0.0 & 61.30$\pm$4.20 & Danforth \\ 
\hline
51 & he0435 & 0.00549 & 14.0$\pm$0.1 & 67.50$\pm$15.90 & Danforth \\ 
52 & he0435 & 0.09037 & 13.4$\pm$0.2 & 98.20$\pm$21.50 & Danforth \\ 
53 & he0435 & 0.15328 & 13.3$\pm$0.1 & 71.50$\pm$18.50 & Danforth \\ 
54 & he0435 & 0.16107 & 13.5$\pm$0.1 & 66.10$\pm$9.50 & Danforth \\ 
55 & he0435 & 0.39044 & 13.9$\pm$0.1 & 62.70$\pm$7.90 & Danforth \\ 
56 & he0435 & 0.40988 & 13.6$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
57 & he0435 & 0.42218 & 13.7$\pm$0.0 & 71.80$\pm$6.70 & Danforth \\ 
\hline
58 & hs0624 & 0.05515 & 13.7$\pm$0.2 & 84.00$\pm$30.70 & Tilton \\ 
59 & hs0624 & 0.09005 & 13.5$\pm$0.0 & 122.00$\pm$3.00 & Tilton \\ 
60 & hs0624 & 0.31045 & 13.4$\pm$0.3 & 62.00$\pm$40.30 & Tilton \\ 
\hline
61 & hs1102 & 0.09533 & 13.2$\pm$0.1 & 76.50$\pm$23.20 & Danforth \\ 
62 & hs1102 & 0.18746 & 13.0$\pm$0.2 & 67.70$\pm$29.20 & Danforth \\ 
63 & hs1102 & 0.21101 & 13.6$\pm$0.1 & 130.80$\pm$28.00 & Danforth \\ 
64 & hs1102 & 0.21762 & 13.7$\pm$0.0 & 114.80$\pm$9.40 & Danforth \\ 
65 & hs1102 & 0.25125 & 13.6$\pm$0.1 & 108.40$\pm$23.40 & Danforth \\ 
66 & hs1102 & 0.25365 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
67 & hs1102 & 0.25794 & 13.5$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
68 & hs1102 & 0.25867 & 13.8$\pm$0.2 & 84.10$\pm$27.20 & Danforth \\ 
69 & hs1102 & 0.28713 & 13.2$\pm$0.1 & 63.00$\pm$17.30 & Danforth \\ 
70 & hs1102 & 0.40856 & 13.5$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
71 & hs1102 & 0.40970 & 13.7$\pm$0.2 & 100.00$\pm$0.00 & Danforth \\ 
72 & hs1102 & 0.41874 & 13.7$\pm$0.7 & 130.60$\pm$54.40 & Danforth \\ 
73 & hs1102 & 0.42280 & 14.2$\pm$0.0 & 65.90$\pm$4.00 & Danforth \\ 
74 & hs1102 & 0.46827 & 13.8$\pm$0.0 & 81.10$\pm$2.00 & Danforth \\ 
\hline
75 & i06229 & 0.01218 & 13.1$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
76 & i06229 & 0.05260 & 13.3$\pm$0.1 & 76.00$\pm$17.50 & Danforth \\ 
\hline
77 & i22456 & 0.00443 & 12.8$\pm$0.1 & 75.70$\pm$15.40 & Danforth \\ 
78 & i22456 & 0.09941 & 14.6$\pm$0.0 & 62.80$\pm$0.60 & Danforth \\ 
\hline
79 & mr2251 & 0.01068 & 14.6$\pm$0.7 & 69.00$\pm$4.00 & Tilton \\ 
80 & mr2251 & 0.01449 & 12.9$\pm$0.1 & 78.90$\pm$18.20 & Danforth \\ 
81 & mr2251 & 0.06131 & 13.2$\pm$0.0 & 64.50$\pm$2.90 & Danforth \\ 
82 & mr2251 & 0.06190 & 14.0$\pm$0.0 & 79.20$\pm$0.90 & Danforth \\ 
83 & mr2251 & 0.06276 & 14.3$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
84 & mr2251 & 0.06327 & 14.2$\pm$0.0 & 98.90$\pm$3.40 & Danforth \\ 
85 & mr2251 & 0.06381 & 13.8$\pm$0.0 & 69.70$\pm$2.20 & Danforth \\ 
\hline
86 & mrk106 & 0.06330 & 13.0$\pm$0.1 & 64.70$\pm$18.70 & Danforth \\ 
87 & mrk106 & 0.07672 & 13.2$\pm$0.1 & 72.50$\pm$19.80 & Danforth \\ 
\hline
88 & mrk478 & 0.06166 & 13.2$\pm$0.1 & 97.00$\pm$19.70 & Danforth \\ 
89 & mrk478 & 0.06578 & 13.0$\pm$0.1 & 64.20$\pm$22.30 & Danforth \\ 
90 & mrk478 & 0.07213 & 13.3$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
\hline
91 & mrk876 & 0.01159 & 13.2$\pm$0.1 & 84.90$\pm$10.10 & Danforth \\ 
92 & mrk876 & 0.05598 & 12.8$\pm$0.1 & 79.60$\pm$18.90 & Danforth \\ 
93 & mrk876 & 0.08709 & 12.3$\pm$0.2 & 68.20$\pm$35.10 & Danforth \\ 
94 & mrk876 & 0.08858 & 13.6$\pm$0.0 & 70.30$\pm$2.70 & Danforth \\ 
95 & mrk876 & 0.08917 & 12.9$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
96 & mrk876 & 0.11487 & 13.2$\pm$0.1 & 74.00$\pm$6.00 & Tilton \\ 
\hline
97 & ngc7469 & 0.00981 & 13.5$\pm$0.1 & 132.70$\pm$27.60 & Tilton \\ 
\hline
98 & pg0003 & 0.08299 & 13.8$\pm$0.0 & 64.40$\pm$6.40 & Danforth \\ 
99 & pg0003 & 0.17139 & 12.9$\pm$0.1 & 102.90$\pm$29.10 & Danforth \\ 
100 & pg0003 & 0.22541 & 13.1$\pm$0.1 & 92.80$\pm$18.60 & Danforth \\ 
101 & pg0003 & 0.38633 & 13.5$\pm$0.2 & 86.70$\pm$32.30 & Danforth \\ 
102 & pg0003 & 0.42051 & 13.4$\pm$0.1 & 63.90$\pm$9.30 & Danforth \\ 
\hline
103 & pg0804 & 0.05015 & 12.8$\pm$0.1 & 69.80$\pm$14.60 & Danforth \\ 
104 & pg0804 & 0.05576 & 12.8$\pm$10.0 & 64.20$\pm$99.90 & Danforth \\ 
105 & pg0804 & 0.36379 & 12.5$\pm$0.3 & 63.20$\pm$8.20 & Danforth \\ 
\hline
106 & pg0832 & 0.01753 & 15.6$\pm$0.2 & 87.30$\pm$5.40 & Danforth \\ 
107 & pg0832 & 0.02793 & 13.6$\pm$0.2 & 65.90$\pm$18.50 & Danforth \\ 
108 & pg0832 & 0.08748 & 13.4$\pm$0.1 & 116.70$\pm$31.70 & Danforth \\ 
109 & pg0832 & 0.10171 & 13.9$\pm$0.1 & 60.90$\pm$8.00 & Danforth \\ 
110 & pg0832 & 0.18391 & 13.3$\pm$0.1 & 130.50$\pm$38.30 & Danforth \\ 
111 & pg0832 & 0.27503 & 13.6$\pm$0.1 & 60.60$\pm$12.50 & Danforth \\ 
112 & pg0832 & 0.27694 & 13.6$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
113 & pg0832 & 0.32572 & 13.3$\pm$0.1 & 60.20$\pm$11.10 & Danforth \\ 
\hline
114 & pg0838 & 0.06583 & 13.3$\pm$0.1 & 81.20$\pm$14.30 & Danforth \\ 
115 & pg0838 & 0.08628 & 13.1$\pm$0.2 & 148.80$\pm$42.90 & Danforth \\ 
116 & pg0838 & 0.12676 & 13.1$\pm$0.1 & 91.90$\pm$13.20 & Danforth \\ 
\hline
117 & pg0953 & 0.16319 & 13.0$\pm$0.1 & 74.90$\pm$10.00 & Danforth \\ 
118 & pg0953 & 0.19221 & 13.3$\pm$0.1 & 63.80$\pm$14.60 & Tilton \\ 
\hline
119 & pg1001 & 0.00165 & 13.9$\pm$1.3 & 60.60$\pm$51.80 & Danforth \\ 
120 & pg1001 & 0.21343 & 13.9$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
\hline
121 & pg1048 & 0.00642 & 14.0$\pm$0.1 & 86.90$\pm$8.90 & Danforth \\ 
122 & pg1048 & 0.02414 & 13.2$\pm$0.1 & 66.70$\pm$13.00 & Danforth \\ 
\hline
123 & pg1049 & 0.03015 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
124 & pg1049 & 0.06313 & 13.6$\pm$0.1 & 86.30$\pm$13.20 & Danforth \\ 
125 & pg1049 & 0.12706 & 13.6$\pm$0.1 & 63.30$\pm$9.70 & Danforth \\ 
126 & pg1049 & 0.14980 & 13.3$\pm$0.1 & 72.00$\pm$10.50 & Danforth \\ 
127 & pg1049 & 0.16322 & 13.2$\pm$0.2 & 100.00$\pm$0.00 & Danforth \\ 
128 & pg1049 & 0.32523 & 13.3$\pm$0.1 & 105.90$\pm$32.00 & Danforth \\ 
129 & pg1049 & 0.34016 & 13.5$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
130 & pg1049 & 0.34187 & 14.1$\pm$0.0 & 64.30$\pm$4.00 & Danforth \\ 
\hline
131 & pg1115 & 0.09511 & 13.2$\pm$0.1 & 68.30$\pm$12.50 & Danforth \\ 
132 & pg1115 & 0.12059 & 13.0$\pm$0.1 & 73.50$\pm$20.20 & Danforth \\ 
133 & pg1115 & 0.12741 & 13.2$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
\hline
134 & pg1116 & 0.04114 & 13.2$\pm$0.0 & 69.50$\pm$8.40 & Danforth^{*} \\ 
135 & pg1116 & 0.06251 & 13.1$\pm$0.0 & 71.20$\pm$5.70 & Tilton \\ 
136 & pg1116 & 0.08382 & 13.2$\pm$0.1 & 63.80$\pm$13.80 & Danforth \\ 
137 & pg1116 & 0.09210 & 12.8$\pm$0.1 & 68.80$\pm$22.30 & Danforth \\ 
138 & pg1116 & 0.09281 & 13.1$\pm$0.1 & 77.40$\pm$11.90 & Danforth^{*} \\ 
139 & pg1116 & 0.13373 & 13.2$\pm$0.0 & 81.30$\pm$6.00 & Tilton \\ 
140 & pg1116 & 0.13851 & 13.5$\pm$0.2 & 80.80$\pm$16.20 & Danforth \\ 
\hline
141 & pg1121 & 0.00791 & 13.3$\pm$0.1 & 99.00$\pm$25.00 & Danforth \\ 
142 & pg1121 & 0.07727 & 13.5$\pm$0.1 & 60.90$\pm$13.30 & Danforth \\ 
143 & pg1121 & 0.18078 & 13.5$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
144 & pg1121 & 0.18869 & 13.1$\pm$0.1 & 70.40$\pm$20.40 & Danforth \\ 
145 & pg1121 & 0.21814 & 12.9$\pm$0.1 & 69.50$\pm$22.70 & Danforth \\ 
146 & pg1121 & 0.21992 & 13.9$\pm$0.0 & 80.70$\pm$2.20 & Danforth \\ 
\hline
147 & pg1211 & 0.02586 & 13.5$\pm$0.0 & 70.00$\pm$2.00 & Tilton \\ 
148 & pg1211 & 0.05443 & 13.2$\pm$0.0 & 98.00$\pm$1.00 & Tilton \\ 
\hline
149 & pg1216 & 0.00842 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
150 & pg1216 & 0.07969 & 13.2$\pm$0.1 & 66.80$\pm$14.50 & Danforth \\ 
151 & pg1216 & 0.12372 & 14.8$\pm$0.1 & 70.80$\pm$3.40 & Tilton \\ 
152 & pg1216 & 0.12473 & 14.7$\pm$0.1 & 73.60$\pm$3.50 & Tilton \\ 
153 & pg1216 & 0.17950 & 13.2$\pm$0.1 & 64.80$\pm$11.10 & Danforth \\ 
154 & pg1216 & 0.20014 & 13.6$\pm$0.0 & 60.60$\pm$6.90 & Danforth \\ 
155 & pg1216 & 0.21258 & 13.0$\pm$0.1 & 60.50$\pm$19.80 & Danforth \\ 
156 & pg1216 & 0.28204 & 13.9$\pm$1.2 & 78.60$\pm$22.50 & Danforth \\ 
\hline
157 & pg1222 & 0.15554 & 13.9$\pm$0.0 & 64.70$\pm$3.00 & Danforth \\ 
158 & pg1222 & 0.24198 & 13.6$\pm$0.1 & 91.40$\pm$12.50 & Danforth \\ 
159 & pg1222 & 0.26075 & 12.9$\pm$0.1 & 60.20$\pm$17.70 & Danforth \\ 
160 & pg1222 & 0.32786 & 13.2$\pm$0.1 & 84.70$\pm$28.00 & Danforth \\ 
161 & pg1222 & 0.36749 & 13.7$\pm$0.0 & 96.20$\pm$10.60 & Danforth \\ 
162 & pg1222 & 0.37471 & 13.8$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
163 & pg1222 & 0.37721 & 13.6$\pm$0.1 & 72.80$\pm$17.20 & Danforth \\ 
164 & pg1222 & 0.37840 & 13.5$\pm$1.4 & 61.40$\pm$67.10 & Danforth \\ 
\hline
165 & pg1229 & 0.05018 & 12.9$\pm$0.1 & 61.90$\pm$19.80 & Danforth \\ 
\hline
166 & pg1259 & 0.05563 & 13.4$\pm$0.0 & 70.70$\pm$5.90 & Danforth \\ 
167 & pg1259 & 0.15136 & 13.3$\pm$0.1 & 62.20$\pm$3.70 & Tilton \\ 
168 & pg1259 & 0.16647 & 13.3$\pm$0.1 & 93.30$\pm$8.90 & Tilton \\ 
169 & pg1259 & 0.17893 & 13.1$\pm$0.1 & 83.70$\pm$11.90 & Tilton \\ 
170 & pg1259 & 0.22376 & 13.0$\pm$0.1 & 76.50$\pm$17.90 & Danforth \\ 
171 & pg1259 & 0.24126 & 13.4$\pm$0.1 & 89.10$\pm$6.90 & Tilton \\ 
172 & pg1259 & 0.31974 & 14.0$\pm$0.0 & 70.30$\pm$3.10 & Tilton \\ 
173 & pg1259 & 0.36212 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
174 & pg1259 & 0.38254 & 13.5$\pm$0.0 & 82.20$\pm$8.90 & Danforth \\ 
175 & pg1259 & 0.38266 & 13.7$\pm$0.1 & 137.00$\pm$19.00 & Tilton \\ 
\hline
176 & pg1307 & 0.08345 & 13.4$\pm$0.1 & 84.60$\pm$7.10 & Danforth \\ 
\hline
177 & pg1309 & 0.03861 & 13.4$\pm$0.1 & 62.70$\pm$12.10 & Danforth \\ 
178 & pg1309 & 0.17740 & 13.9$\pm$0.0 & 65.10$\pm$5.30 & Danforth \\ 
179 & pg1309 & 0.17852 & 14.5$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
180 & pg1309 & 0.17918 & 14.4$\pm$0.0 & 128.90$\pm$8.10 & Danforth \\ 
181 & pg1309 & 0.18143 & 13.9$\pm$0.0 & 94.90$\pm$9.90 & Danforth \\ 
\hline
182 & pg1424 & 0.01908 & 13.5$\pm$0.1 & 96.00$\pm$14.30 & Danforth \\ 
183 & pg1424 & 0.25044 & 13.0$\pm$0.1 & 74.40$\pm$22.10 & Danforth \\ 
184 & pg1424 & 0.36260 & 13.2$\pm$0.1 & 82.40$\pm$23.40 & Danforth \\ 
\hline
185 & pg1444 & 0.22031 & 13.5$\pm$0.0 & 76.00$\pm$7.60 & Tilton \\ 
\hline
186 & pg1626 & 0.06137 & 13.6$\pm$0.0 & 60.50$\pm$6.60 & Danforth \\ 
\hline
187 & phl1811 & 0.05143 & 13.7$\pm$0.0 & 72.80$\pm$5.10 & Danforth \\ 
188 & phl1811 & 0.05813 & 13.2$\pm$0.1 & 89.50$\pm$16.80 & Danforth \\ 
189 & phl1811 & 0.08085 & 13.9$\pm$0.1 & 91.80$\pm$11.60 & Danforth \\ 
190 & phl1811 & 0.08163 & 13.2$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
191 & phl1811 & 0.12003 & 13.0$\pm$0.1 & 77.40$\pm$16.90 & Danforth \\ 
192 & phl1811 & 0.15787 & 13.2$\pm$0.1 & 70.40$\pm$9.90 & Danforth \\ 
\hline
193 & phl2525 & 0.06548 & 13.2$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
194 & phl2525 & 0.06682 & 13.4$\pm$0.1 & 64.80$\pm$14.20 & Danforth \\ 
195 & phl2525 & 0.08351 & 13.4$\pm$0.1 & 66.70$\pm$16.90 & Danforth \\ 
196 & phl2525 & 0.14869 & 13.1$\pm$0.1 & 65.20$\pm$16.20 & Danforth \\ 
197 & phl2525 & 0.17002 & 13.3$\pm$0.1 & 116.00$\pm$42.10 & Danforth \\ 
\hline
198 & pks0312 & 0.11454 & 14.0$\pm$0.0 & 79.00$\pm$4.00 & Tilton \\ 
\hline
199 & pks0405 & 0.02510 & 13.2$\pm$0.1 & 144.30$\pm$26.50 & Danforth \\ 
200 & pks0405 & 0.05902 & 13.3$\pm$0.1 & 62.30$\pm$11.10 & Tilton \\ 
201 & pks0405 & 0.09719 & 13.6$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
202 & pks0405 & 0.10152 & 13.2$\pm$0.1 & 67.90$\pm$11.30 & Tilton \\ 
203 & pks0405 & 0.10298 & 13.4$\pm$0.1 & 73.70$\pm$12.00 & Tilton \\ 
204 & pks0405 & 0.19456 & 12.8$\pm$0.1 & 63.60$\pm$8.10 & Danforth^{*} \\ 
205 & pks0405 & 0.21976 & 12.7$\pm$0.1 & 70.20$\pm$18.80 & Danforth \\ 
206 & pks0405 & 0.24564 & 13.1$\pm$0.1 & 77.40$\pm$14.80 & Danforth \\ 
207 & pks0405 & 0.29748 & 13.2$\pm$0.1 & 66.00$\pm$11.70 & Danforth \\ 
208 & pks0405 & 0.31016 & 12.9$\pm$0.1 & 76.70$\pm$20.20 & Danforth \\ 
209 & pks0405 & 0.32502 & 13.7$\pm$0.0 & 85.50$\pm$6.10 & Tilton \\ 
210 & pks0405 & 0.49508 & 14.3$\pm$0.0 & 64.90$\pm$7.70 & Tilton \\ 
\hline
211 & pks0552 & 0.26916 & 13.2$\pm$0.1 & 68.40$\pm$13.10 & Danforth \\ 
212 & pks0552 & 0.35661 & 13.3$\pm$0.1 & 64.70$\pm$9.50 & Danforth \\ 
\hline
213 & pks0558 & 0.10472 & 13.0$\pm$0.1 & 79.50$\pm$35.00 & Danforth \\ 
\hline
214 & pks0637 & 0.14272 & 13.1$\pm$0.1 & 77.90$\pm$13.80 & Danforth \\ 
215 & pks0637 & 0.16082 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
216 & pks0637 & 0.17428 & 13.0$\pm$0.1 & 72.20$\pm$16.30 & Danforth \\ 
217 & pks0637 & 0.36408 & 13.5$\pm$0.1 & 86.70$\pm$13.00 & Danforth \\ 
218 & pks0637 & 0.41784 & 13.7$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
\hline
219 & pks1302 & 0.01956 & 13.3$\pm$0.1 & 66.20$\pm$9.50 & Danforth \\ 
220 & pks1302 & 0.03281 & 13.1$\pm$0.1 & 62.80$\pm$14.60 & Danforth \\ 
221 & pks1302 & 0.14531 & 15.4$\pm$0.1 & 61.80$\pm$3.90 & Tilton \\ 
222 & pks1302 & 0.19281 & 13.6$\pm$0.1 & 68.90$\pm$14.10 & Tilton \\ 
223 & pks1302 & 0.23679 & 13.4$\pm$0.0 & 69.70$\pm$6.90 & Danforth \\ 
224 & pks1302 & 0.23752 & 13.0$\pm$0.1 & 74.70$\pm$26.90 & Danforth \\ 
225 & pks1302 & 0.24885 & 13.4$\pm$0.1 & 77.00$\pm$19.00 & Tilton \\ 
226 & pks1302 & 0.25120 & 13.7$\pm$0.0 & 71.40$\pm$4.10 & Danforth \\ 
\hline
227 & pks2155 & 0.05708 & 14.1$\pm$0.0 & 67.90$\pm$1.70 & Danforth^{*} \\ 
228 & pks2155 & 0.06236 & 12.8$\pm$0.1 & 69.10$\pm$22.20 & Danforth \\ 
229 & pks2155 & 0.10586 & 13.5$\pm$0.0 & 66.00$\pm$4.00 & Tilton \\ 
\hline
230 & pmn2345 & 0.28405 & 13.5$\pm$0.1 & 81.80$\pm$13.80 & Danforth \\ 
231 & pmn2345 & 0.31540 & 13.7$\pm$0.0 & 60.10$\pm$7.30 & Danforth \\ 
232 & pmn2345 & 0.37828 & 14.3$\pm$0.0 & 65.70$\pm$2.90 & Danforth \\ 
233 & pmn2345 & 0.43000 & 13.5$\pm$0.1 & 63.00$\pm$18.10 & Danforth \\ 
234 & pmn2345 & 0.47074 & 13.6$\pm$0.0 & 87.10$\pm$3.10 & Danforth \\ 
\hline
235 & q0045 & 0.05590 & 13.2$\pm$0.1 & 66.80$\pm$12.80 & Danforth \\ 
236 & q0045 & 0.06377 & 13.0$\pm$0.1 & 70.60$\pm$23.20 & Danforth \\ 
\hline
237 & q1230 & 0.08344 & 13.3$\pm$0.0 & 65.00$\pm$6.00 & Tilton \\ 
238 & q1230 & 0.08540 & 12.8$\pm$0.1 & 94.60$\pm$26.80 & Danforth \\ 
239 & q1230 & 0.09444 & 13.0$\pm$0.1 & 69.70$\pm$10.10 & Danforth \\ 
240 & q1230 & 0.10000 & 13.2$\pm$0.1 & 61.00$\pm$8.00 & Tilton \\ 
241 & q1230 & 0.10525 & 14.0$\pm$0.1 & 75.00$\pm$4.00 & Tilton \\ 
242 & q1230 & 0.10549 & 14.1$\pm$0.0 & 87.30$\pm$3.30 & Danforth \\ 
243 & q1230 & 0.10566 & 14.0$\pm$0.1 & 121.70$\pm$28.60 & Tilton \\ 
244 & q1230 & 0.10612 & 13.4$\pm$0.1 & 76.40$\pm$15.40 & Danforth \\ 
245 & q1230 & 0.10639 & 13.8$\pm$0.0 & 64.30$\pm$3.40 & Tilton \\ 
246 & q1230 & 0.10660 & 13.5$\pm$0.1 & 61.90$\pm$4.00 & Danforth \\ 
247 & q1230 & 0.10853 & 12.8$\pm$0.1 & 92.60$\pm$21.50 & Danforth \\ 
248 & q1230 & 0.10940 & 13.8$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
249 & q1230 & 0.12103 & 13.5$\pm$0.0 & 69.40$\pm$3.60 & Tilton \\ 
\hline
250 & rbs144 & 0.04528 & 13.1$\pm$0.1 & 62.30$\pm$12.70 & Danforth \\ 
\hline
251 & rbs1892 & 0.15567 & 13.3$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
252 & rbs1892 & 0.15633 & 13.4$\pm$0.0 & 150.00$\pm$0.00 & Danforth \\ 
253 & rbs1892 & 0.16343 & 13.8$\pm$0.0 & 67.60$\pm$2.70 & Danforth \\ 
254 & rbs1892 & 0.17001 & 13.2$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
255 & rbs1892 & 0.17155 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
256 & rbs1892 & 0.17185 & 13.2$\pm$0.1 & 84.70$\pm$14.20 & Danforth \\ 
\hline
257 & rbs542 & 0.04455 & 12.9$\pm$0.0 & 70.80$\pm$7.80 & Danforth \\ 
258 & rbs542 & 0.04992 & 12.8$\pm$0.1 & 62.10$\pm$13.30 & Danforth \\ 
\hline
259 & rxj0439 & 0.00550 & 13.7$\pm$0.2 & 67.90$\pm$15.90 & Danforth \\ 
260 & rxj0439 & 0.17680 & 13.5$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
\hline
261 & rxj0956 & 0.03471 & 13.8$\pm$0.0 & 64.80$\pm$5.90 & Danforth \\ 
262 & rxj0956 & 0.06924 & 13.2$\pm$0.1 & 67.30$\pm$18.50 & Danforth \\ 
263 & rxj0956 & 0.10858 & 13.3$\pm$0.1 & 74.30$\pm$21.00 & Danforth \\ 
264 & rxj0956 & 0.12796 & 13.6$\pm$0.1 & 89.60$\pm$11.00 & Danforth \\ 
265 & rxj0956 & 0.14704 & 13.2$\pm$0.1 & 88.40$\pm$25.40 & Danforth \\ 
266 & rxj0956 & 0.15101 & 13.0$\pm$0.1 & 81.80$\pm$22.40 & Danforth \\ 
\hline
267 & rxj2154 & 0.23009 & 13.1$\pm$0.1 & 68.20$\pm$17.40 & Danforth \\ 
\hline
268 & s080908 & 0.05775 & 13.5$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
269 & s080908 & 0.06391 & 13.6$\pm$0.2 & 149.00$\pm$46.10 & Danforth \\ 
270 & s080908 & 0.14214 & 13.4$\pm$0.1 & 94.80$\pm$15.00 & Danforth \\ 
271 & s080908 & 0.16001 & 13.4$\pm$0.1 & 76.00$\pm$9.70 & Danforth \\ 
272 & s080908 & 0.38700 & 13.4$\pm$0.2 & 100.00$\pm$0.00 & Danforth \\ 
\hline
273 & s09255b & 0.13118 & 13.4$\pm$0.1 & 86.70$\pm$12.00 & Danforth \\ 
\hline
274 & s092909 & 0.16491 & 13.8$\pm$0.0 & 63.60$\pm$5.70 & Danforth \\ 
275 & s092909 & 0.23508 & 13.5$\pm$0.0 & 83.10$\pm$8.20 & Danforth \\ 
\hline
276 & s094952 & 0.06581 & 13.4$\pm$0.1 & 90.00$\pm$28.60 & Danforth \\ 
277 & s094952 & 0.16442 & 13.4$\pm$1.0 & 63.40$\pm$55.70 & Danforth \\ 
\hline
278 & s135712 & 0.14702 & 14.0$\pm$0.0 & 79.90$\pm$1.90 & Danforth \\ 
\hline
279 & s50716 & 0.00989 & 13.1$\pm$0.1 & 61.90$\pm$12.90 & Danforth \\ 
280 & s50716 & 0.01766 & 13.1$\pm$0.1 & 89.50$\pm$13.60 & Danforth \\ 
281 & s50716 & 0.08834 & 13.1$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
282 & s50716 & 0.14936 & 12.9$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
\hline
283 & sbs1108 & 0.02497 & 13.8$\pm$0.0 & 79.40$\pm$3.10 & Danforth \\ 
284 & sbs1108 & 0.25715 & 13.7$\pm$0.0 & 61.40$\pm$6.50 & Danforth \\ 
285 & sbs1108 & 0.41402 & 13.6$\pm$0.1 & 81.20$\pm$18.30 & Danforth \\ 
\hline
286 & sbs1122 & 0.04709 & 13.3$\pm$0.1 & 62.00$\pm$13.00 & Danforth \\ 
287 & sbs1122 & 0.13699 & 13.3$\pm$0.2 & 77.60$\pm$32.70 & Danforth \\ 
288 & sbs1122 & 0.13812 & 13.6$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
289 & sbs1122 & 0.13865 & 13.8$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
290 & sbs1122 & 0.15271 & 13.5$\pm$0.2 & 74.50$\pm$23.30 & Danforth \\ 
291 & sbs1122 & 0.36707 & 13.7$\pm$0.1 & 82.90$\pm$13.80 & Danforth \\ 
\hline
292 & ton1187 & 0.01504 & 13.7$\pm$0.1 & 96.20$\pm$14.60 & Danforth \\ 
293 & ton1187 & 0.05216 & 13.5$\pm$0.2 & 61.20$\pm$9.80 & Danforth \\ 
294 & ton1187 & 0.07687 & 13.1$\pm$0.1 & 83.70$\pm$20.30 & Danforth \\ 
\hline
295 & ton28 & 0.03357 & 13.4$\pm$0.1 & 75.00$\pm$7.00 & Tilton \\ 
\hline
296 & tons180 & 0.04304 & 13.8$\pm$0.4 & 81.00$\pm$15.00 & Tilton \\ 
\hline
297 & tons210 & 0.06763 & 13.0$\pm$0.1 & 61.10$\pm$21.80 & Danforth \\ 
298 & tons210 & 0.08558 & 13.1$\pm$0.1 & 73.00$\pm$12.60 & Danforth \\ 
\hline
\caption{A '*' indicates a duplicate redshift in both Danforth and Tilton. The corresponding Tilton duplicates are omitted from the table}
\end{longtable}

==> OVI_Priors.tex <==
\begin{longtable}{lllccccc}
\# & Name & Redshift & $\log N$ (cm$^{-2}$) & $b$ (km~s$^{-1}$) & Source\\ 
\hline
1 & 1es1028 & 0.12314 & 14.3$\pm$0.1 & 41.37$\pm$5.57 & Danforth$^{M}$ \\ 
2 & 1es1028 & 0.13706 & 13.6$\pm$0.1 & 14.50$\pm$6.30 & Danforth$^{1032}$ \\ 
3 & 1es1028 & 0.33735 & 13.9$\pm$0.1 & 72.87$\pm$15.73 & Danforth$^{M}$ \\ 
\hline
4 & 1es1553 & 0.18759 & 13.8$\pm$0.1 & 12.10$\pm$3.00 & Danforth$^{M}$ \\ 
5 & 1es1553 & 0.18775 & 13.9$\pm$0.1 & 23.40$\pm$4.50 & Danforth$^{M}$ \\ 
6 & 1es1553 & 0.18984 & 13.4$\pm$1.5 & 23.37$\pm$6.57 & Danforth$^{M}$ \\ 
7 & 1es1553 & 0.21631 & 13.3$\pm$0.1 & 19.80$\pm$5.80 & Danforth$^{1032}$ \\ 
8 & 1es1553 & 0.31130 & 13.4$\pm$0.1 & 31.90$\pm$7.50 & Danforth$^{1032}$ \\ 
9 & 1es1553 & 0.37868 & 12.9$\pm$0.2 & 17.30$\pm$3.70 & Danforth$^{1032}$ \\ 
10 & 1es1553 & 0.39497 & 13.9$\pm$0.1 & 44.07$\pm$3.33 & Danforth$^{M}$ \\ 
\hline
11 & 1sj1032 & 0.17007 & 14.3$\pm$0.0 & 42.00$\pm$3.80 & Danforth$^{1032}$ \\ 
\hline
12 & 3c249 & 0.24676 & 13.8$\pm$0.1 & 24.70$\pm$2.50 & Tilton \\ 
13 & 3c249 & 0.30788 & 13.9$\pm$0.2 & 23.30$\pm$6.10 & Tilton \\ 
14 & 3c249 & 0.30809 & 14.5$\pm$0.0 & 20.00$\pm$1.00 & Tilton \\ 
15 & 3c249 & 0.31364 & 13.8$\pm$0.1 & 13.30$\pm$1.00 & Tilton \\ 
\hline
16 & 3c263 & 0.11388 & 13.7$\pm$0.1 & 33.10$\pm$8.20 & Danforth$^{1032}$ \\ 
17 & 3c263 & 0.14078 & 13.7$\pm$0.1 & 45.10$\pm$6.97 & Danforth$^{M}$ \\ 
18 & 3c263 & 0.29204 & 13.0$\pm$0.2 & 21.40$\pm$9.60 & Danforth$^{1032}$ \\ 
19 & 3c263 & 0.32566 & 14.0$\pm$0.0 & 32.57$\pm$2.47 & Danforth$^{M}$ \\ 
20 & 3c263 & 0.44677 & 13.9$\pm$0.1 & 64.10$\pm$10.70 & Danforth$^{1038}$ \\ 
21 & 3c263 & 0.52690 & 13.9$\pm$0.1 & 38.47$\pm$7.00 & Danforth$^{M}$ \\ 
22 & 3c263 & 0.52801 & 13.5$\pm$0.1 & 48.00$\pm$14.40 & Danforth$^{1032}$ \\ 
\hline
23 & 3c273 & 0.00337 & 13.4$\pm$0.1 & 28.00$\pm$1.00 & Tilton \\ 
24 & 3c273 & 0.00533 & 13.0$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
25 & 3c273 & 0.00764 & 13.1$\pm$0.2 & 25.00$\pm$9.00 & Tilton \\ 
26 & 3c273 & 0.02947 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
27 & 3c273 & 0.04898 & 14.0$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
28 & 3c273 & 0.06655 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
29 & 3c273 & 0.09018 & 13.3$\pm$0.1 & 22.20$\pm$10.80 & Tilton \\ 
30 & 3c273 & 0.12007 & 13.4$\pm$0.1 & 20.03$\pm$3.23 & Danforth$^{M,*}$ \\ 
31 & 3c273 & 0.14660 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
32 & 3c273 & 0.15784 & 13.1$\pm$0.1 & 30.30$\pm$4.90 & Danforth$^{1032*}$ \\ 
\hline
33 & 3c351 & 0.21789 & 14.0$\pm$0.0 & 74.40$\pm$8.60 & Tilton \\ 
34 & 3c351 & 0.22093 & 14.3$\pm$0.0 & 48.50$\pm$3.50 & Tilton \\ 
35 & 3c351 & 0.31635 & 13.7$\pm$0.1 & 22.70$\pm$3.30 & Tilton \\ 
36 & 3c351 & 0.31657 & 14.0$\pm$0.1 & 23.40$\pm$2.40 & Tilton \\ 
37 & 3c351 & 0.31687 & 14.0$\pm$0.1 & 31.80$\pm$2.90 & Tilton \\ 
38 & 3c351 & 0.32086 & 12.9$\pm$0.2 & 30.00$\pm$0.00 & Tilton \\ 
\hline
39 & 3c57 & 0.17002 & 13.6$\pm$0.1 & 43.50$\pm$12.40 & Danforth$^{1032}$ \\ 
40 & 3c57 & 0.24987 & 13.6$\pm$0.1 & 10.40$\pm$3.80 & Danforth$^{1032}$ \\ 
41 & 3c57 & 0.25022 & 13.8$\pm$0.1 & 60.00$\pm$12.20 & Danforth$^{1032}$ \\ 
42 & 3c57 & 0.27821 & 13.8$\pm$0.1 & 28.40$\pm$5.37 & Danforth$^{M}$ \\ 
43 & 3c57 & 0.28669 & 13.6$\pm$0.2 & 40.30$\pm$8.80 & Danforth$^{1032}$ \\ 
44 & 3c57 & 0.29238 & 14.3$\pm$0.0 & 41.53$\pm$2.50 & Danforth$^{M}$ \\ 
45 & 3c57 & 0.32010 & 13.8$\pm$0.1 & 26.60$\pm$9.30 & Danforth$^{1038}$ \\ 
46 & 3c57 & 0.32301 & 13.4$\pm$0.1 & 19.63$\pm$7.43 & Danforth$^{M}$ \\ 
47 & 3c57 & 0.32368 & 13.7$\pm$0.2 & 34.90$\pm$16.90 & Danforth$^{1038}$ \\ 
48 & 3c57 & 0.32405 & 14.1$\pm$0.1 & 74.33$\pm$25.17 & Danforth$^{M}$ \\ 
49 & 3c57 & 0.32460 & 14.1$\pm$0.1 & 39.93$\pm$6.17 & Danforth$^{M}$ \\ 
50 & 3c57 & 0.32780 & 13.7$\pm$0.1 & 40.80$\pm$15.13 & Danforth$^{M}$ \\ 
51 & 3c57 & 0.32820 & 14.5$\pm$0.0 & 38.83$\pm$2.00 & Danforth$^{M}$ \\ 
52 & 3c57 & 0.32902 & 13.9$\pm$0.0 & 29.03$\pm$3.97 & Danforth$^{M}$ \\ 
53 & 3c57 & 0.33332 & 13.7$\pm$0.1 & 29.97$\pm$7.40 & Danforth$^{M}$ \\ 
54 & 3c57 & 0.38342 & 14.0$\pm$0.0 & 23.03$\pm$2.43 & Danforth$^{M}$ \\ 
55 & 3c57 & 0.40187 & 13.2$\pm$0.1 & 5.20$\pm$5.20 & Danforth$^{1032}$ \\ 
56 & 3c57 & 0.40211 & 13.5$\pm$0.1 & 26.83$\pm$8.40 & Danforth$^{M}$ \\ 
57 & 3c57 & 0.43164 & 14.0$\pm$0.1 & 56.40$\pm$7.00 & Danforth$^{1032}$ \\ 
58 & 3c57 & 0.53325 & 13.9$\pm$0.1 & 12.33$\pm$2.67 & Danforth$^{M}$ \\ 
59 & 3c57 & 0.57997 & 14.1$\pm$0.1 & 21.53$\pm$4.27 & Danforth$^{M}$ \\ 
60 & 3c57 & 0.66914 & 13.9$\pm$0.1 & 13.23$\pm$3.87 & Danforth$^{M}$ \\ 
61 & 3c57 & 0.66948 & 13.9$\pm$0.1 & 14.97$\pm$4.53 & Danforth$^{M}$ \\ 
62 & 3c57 & 0.66976 & 14.2$\pm$0.1 & 15.80$\pm$2.63 & Danforth$^{M}$ \\ 
\hline
63 & 3c66a & 0.24258 & 14.2$\pm$0.0 & 25.63$\pm$2.10 & Danforth$^{M}$ \\ 
64 & 3c66a & 0.32824 & 13.4$\pm$0.1 & 35.30$\pm$12.70 & Danforth$^{1032}$ \\ 
\hline
65 & b0117 & 0.14191 & 13.3$\pm$0.1 & 13.60$\pm$8.60 & Danforth$^{1032}$ \\ 
66 & b0117 & 0.19073 & 13.6$\pm$0.1 & 15.10$\pm$2.70 & Danforth$^{M}$ \\ 
67 & b0117 & 0.34848 & 13.9$\pm$0.1 & 47.80$\pm$8.23 & Danforth$^{M}$ \\ 
68 & b0117 & 0.34861 & 13.8$\pm$0.1 & 17.63$\pm$3.83 & Danforth$^{M}$ \\ 
\hline
69 & f1010 & 0.11326 & 14.0$\pm$0.2 & 52.10$\pm$15.90 & Danforth$^{1032}$ \\ 
70 & f1010 & 0.19113 & 13.3$\pm$0.2 & 19.30$\pm$12.10 & Danforth$^{1032}$ \\ 
71 & f1010 & 0.19319 & 13.7$\pm$0.1 & 9.07$\pm$2.33 & Danforth$^{M}$ \\ 
72 & f1010 & 0.25473 & 18.0$\pm$0.3 & 30.10$\pm$0.50 & Danforth$^{1032}$ \\ 
\hline
73 & h1821 & 0.02438 & 13.4$\pm$0.1 & 21.00$\pm$7.50 & Tilton \\ 
74 & h1821 & 0.10817 & 13.2$\pm$0.1 & 10.00$\pm$0.00 & Tilton \\ 
75 & h1821 & 0.12133 & 14.0$\pm$0.0 & 76.00$\pm$12.00 & Tilton \\ 
76 & h1821 & 0.12147 & 13.7$\pm$0.1 & 50.30$\pm$8.60 & Danforth$^{1032}$ \\ 
77 & h1821 & 0.16992 & 13.8$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
78 & h1821 & 0.17043 & 13.6$\pm$0.0 & 57.60$\pm$7.50 & Danforth$^{1032}$ \\ 
79 & h1821 & 0.21326 & 13.6$\pm$0.0 & 23.77$\pm$2.83 & Danforth$^{M,*}$ \\ 
80 & h1821 & 0.22497 & 14.3$\pm$0.0 & 45.17$\pm$1.43 & Danforth$^{M,*}$ \\ 
81 & h1821 & 0.22522 & 13.1$\pm$0.1 & 5.00$\pm$0.00 & Danforth$^{M,*}$ \\ 
82 & h1821 & 0.22639 & 13.5$\pm$0.0 & 17.43$\pm$2.37 & Danforth$^{M,*}$ \\ 
83 & h1821 & 0.24531 & 13.7$\pm$0.0 & 26.90$\pm$2.43 & Danforth$^{M,*}$ \\ 
84 & h1821 & 0.26657 & 13.7$\pm$0.1 & 33.00$\pm$4.47 & Danforth$^{M,*}$ \\ 
85 & h1821 & 0.28800 & 13.4$\pm$0.1 & 29.87$\pm$4.40 & Danforth$^{M}$ \\ 
86 & h1821 & 0.29658 & 13.9$\pm$0.0 & 19.03$\pm$1.57 & Danforth$^{M,*}$ \\ 
87 & h1821 & 0.29680 & 14.0$\pm$0.0 & 36.40$\pm$2.47 & Danforth$^{M,*}$ \\ 
\hline
88 & h2356 & 0.11461 & 14.1$\pm$0.3 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
89 & h2356 & 0.16512 & 13.6$\pm$0.1 & 16.00$\pm$7.10 & Danforth$^{1032}$ \\ 
\hline
90 & he0056 & 0.16392 & 13.4$\pm$0.1 & 23.20$\pm$7.40 & Danforth$^{1032}$ \\ 
91 & he0056 & 0.16492 & 13.1$\pm$0.2 & 20.30$\pm$11.10 & Danforth$^{1032}$ \\ 
\hline
92 & he0153 & 0.13221 & 13.2$\pm$0.2 & 12.93$\pm$11.03 & Danforth$^{M}$ \\ 
93 & he0153 & 0.14844 & 13.9$\pm$0.1 & 54.10$\pm$9.43 & Danforth$^{M}$ \\ 
94 & he0153 & 0.14886 & 14.1$\pm$0.0 & 29.00$\pm$3.10 & Danforth$^{1032}$ \\ 
95 & he0153 & 0.17089 & 13.8$\pm$0.1 & 23.30$\pm$3.20 & Danforth$^{1032}$ \\ 
96 & he0153 & 0.19885 & 13.7$\pm$0.1 & 77.50$\pm$3.63 & Danforth$^{M}$ \\ 
97 & he0153 & 0.22202 & 13.6$\pm$0.1 & 18.60$\pm$7.80 & Danforth$^{1038}$ \\ 
98 & he0153 & 0.22600 & 14.2$\pm$0.0 & 33.00$\pm$2.33 & Danforth$^{M}$ \\ 
99 & he0153 & 0.29091 & 13.7$\pm$0.1 & 25.00$\pm$8.87 & Danforth$^{M}$ \\ 
100 & he0153 & 0.29115 & 13.9$\pm$0.1 & 21.77$\pm$4.43 & Danforth$^{M}$ \\ 
101 & he0153 & 0.39774 & 13.1$\pm$0.2 & 28.50$\pm$10.80 & Danforth$^{1032}$ \\ 
102 & he0153 & 0.40027 & 14.3$\pm$0.0 & 34.90$\pm$2.43 & Danforth$^{M}$ \\ 
103 & he0153 & 0.40058 & 13.4$\pm$0.2 & 20.93$\pm$8.87 & Danforth$^{M}$ \\ 
\hline
104 & he0226 & 0.01746 & 13.7$\pm$0.1 & 13.00$\pm$9.00 & Tilton \\ 
105 & he0226 & 0.02679 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
106 & he0226 & 0.04121 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
107 & he0226 & 0.04535 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
108 & he0226 & 0.04609 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
109 & he0226 & 0.06015 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
110 & he0226 & 0.06083 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
111 & he0226 & 0.07023 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
112 & he0226 & 0.08375 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
113 & he0226 & 0.08901 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
114 & he0226 & 0.08938 & 13.1$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
115 & he0226 & 0.08950 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
116 & he0226 & 0.09220 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
117 & he0226 & 0.10668 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
118 & he0226 & 0.11514 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
119 & he0226 & 0.11680 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
120 & he0226 & 0.11733 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
121 & he0226 & 0.12589 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
122 & he0226 & 0.13832 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
123 & he0226 & 0.15175 & 13.7$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
124 & he0226 & 0.15549 & 13.6$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
125 & he0226 & 0.16237 & 13.7$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
126 & he0226 & 0.16339 & 13.6$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
127 & he0226 & 0.16971 & 14.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
128 & he0226 & 0.18619 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
129 & he0226 & 0.18811 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
130 & he0226 & 0.18891 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
131 & he0226 & 0.19374 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
132 & he0226 & 0.19453 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
133 & he0226 & 0.19860 & 13.7$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
134 & he0226 & 0.20055 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
135 & he0226 & 0.20703 & 14.4$\pm$0.0 & 35.23$\pm$1.27 & Danforth$^{M,*}$ \\ 
136 & he0226 & 0.22009 & 13.0$\pm$0.1 & 11.20$\pm$6.80 & Danforth$^{1032*}$ \\ 
137 & he0226 & 0.22099 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
138 & he0226 & 0.23009 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
139 & he0226 & 0.23964 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
140 & he0226 & 0.24522 & 13.1$\pm$0.2 & 16.00$\pm$10.40 & Danforth$^{1032*}$ \\ 
141 & he0226 & 0.25099 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
142 & he0226 & 0.27155 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
143 & he0226 & 0.27956 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
144 & he0226 & 0.28041 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
145 & he0226 & 0.29134 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
146 & he0226 & 0.29213 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
147 & he0226 & 0.30939 & 13.4$\pm$0.1 & 45.90$\pm$12.00 & Danforth$^{1032*}$ \\ 
148 & he0226 & 0.31833 & 13.0$\pm$0.2 & 6.00$\pm$3.00 & Tilton \\ 
149 & he0226 & 0.33965 & 13.2$\pm$0.1 & 12.70$\pm$5.10 & Danforth$^{1032}$ \\ 
150 & he0226 & 0.34036 & 13.9$\pm$0.0 & 25.87$\pm$2.23 & Danforth$^{M,*}$ \\ 
151 & he0226 & 0.35493 & 12.9$\pm$0.3 & 13.00$\pm$9.00 & Tilton \\ 
152 & he0226 & 0.35528 & 13.7$\pm$0.1 & 34.80$\pm$4.47 & Danforth$^{M,*}$ \\ 
153 & he0226 & 0.37281 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
154 & he0226 & 0.38420 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
155 & he0226 & 0.38636 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
156 & he0226 & 0.39642 & 13.5$\pm$0.1 & 51.70$\pm$7.70 & Danforth$^{1032*}$ \\ 
157 & he0226 & 0.39692 & 13.3$\pm$0.1 & 21.80$\pm$4.50 & Danforth$^{1032}$ \\ 
158 & he0226 & 0.39890 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
159 & he0226 & 0.40034 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
160 & he0226 & 0.40274 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
161 & he0226 & 0.49225 & 14.4$\pm$0.1 & 34.93$\pm$3.37 & Danforth$^{M,*}$ \\ 
162 & he0226 & 0.49254 & 14.5$\pm$0.0 & 22.13$\pm$1.90 & Danforth$^{M,*}$ \\ 
163 & he0226 & 0.49280 & 14.0$\pm$0.2 & 27.90$\pm$22.60 & Danforth$^{M,*}$ \\ 
164 & he0226 & 0.49309 & 14.0$\pm$0.2 & 41.50$\pm$5.60 & Danforth$^{M,*}$ \\ 
\hline
165 & he0238 & 0.27918 & 13.3$\pm$0.2 & 30.20$\pm$11.20 & Danforth$^{1032}$ \\ 
166 & he0238 & 0.31404 & 13.4$\pm$0.1 & 24.10$\pm$2.80 & Danforth$^{M}$ \\ 
167 & he0238 & 0.40107 & 13.5$\pm$0.2 & 18.43$\pm$6.47 & Danforth$^{M}$ \\ 
168 & he0238 & 0.42387 & 14.4$\pm$0.0 & 52.03$\pm$3.33 & Danforth$^{M}$ \\ 
169 & he0238 & 0.42431 & 14.1$\pm$0.0 & 22.83$\pm$2.47 & Danforth$^{M}$ \\ 
170 & he0238 & 0.47203 & 14.1$\pm$0.0 & 20.47$\pm$2.27 & Danforth$^{M}$ \\ 
171 & he0238 & 0.47230 & 13.7$\pm$0.1 & 12.40$\pm$3.33 & Danforth$^{M}$ \\ 
172 & he0238 & 0.60294 & 14.2$\pm$0.1 & 66.80$\pm$13.10 & Danforth$^{1038}$ \\ 
173 & he0238 & 0.60334 & 14.1$\pm$0.0 & 80.80$\pm$9.90 & Danforth$^{1032}$ \\ 
174 & he0238 & 0.60364 & 13.7$\pm$0.3 & 33.40$\pm$18.50 & Danforth$^{1038}$ \\ 
175 & he0238 & 0.60431 & 14.5$\pm$0.2 & 87.40$\pm$28.37 & Danforth$^{M}$ \\ 
176 & he0238 & 0.60493 & 14.1$\pm$0.4 & 65.60$\pm$25.90 & Danforth$^{M}$ \\ 
177 & he0238 & 0.60912 & 14.5$\pm$0.1 & 89.80$\pm$7.20 & Danforth$^{1032}$ \\ 
178 & he0238 & 0.60938 & 14.7$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
179 & he0238 & 0.61015 & 14.3$\pm$0.1 & 79.00$\pm$9.90 & Danforth$^{1032}$ \\ 
180 & he0238 & 0.61091 & 13.8$\pm$0.1 & 29.33$\pm$6.20 & Danforth$^{M}$ \\ 
\hline
181 & he0435 & 0.24490 & 13.9$\pm$0.2 & 33.73$\pm$13.93 & Danforth$^{M}$ \\ 
182 & he0435 & 0.29849 & 13.8$\pm$0.2 & 37.40$\pm$9.40 & Danforth$^{1032}$ \\ 
183 & he0435 & 0.31319 & 14.0$\pm$0.1 & 10.97$\pm$3.67 & Danforth$^{M}$ \\ 
184 & he0435 & 0.39225 & 14.1$\pm$0.1 & 46.67$\pm$9.80 & Danforth$^{M}$ \\ 
185 & he0435 & 0.39266 & 14.0$\pm$0.1 & 33.97$\pm$7.67 & Danforth$^{M}$ \\ 
186 & he0435 & 0.40921 & 14.1$\pm$0.1 & 80.33$\pm$9.80 & Danforth$^{M}$ \\ 
187 & he0435 & 0.40997 & 14.5$\pm$0.0 & 58.83$\pm$4.13 & Danforth$^{M}$ \\ 
\hline
188 & hs0624 & 0.06342 & 14.2$\pm$0.2 & 57.10$\pm$21.60 & Tilton \\ 
189 & hs0624 & 0.07573 & 13.9$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
190 & hs0624 & 0.20482 & 13.4$\pm$0.2 & 28.00$\pm$12.00 & Tilton \\ 
191 & hs0624 & 0.20531 & 13.1$\pm$0.2 & 20.00$\pm$0.00 & Tilton \\ 
192 & hs0624 & 0.21134 & 13.1$\pm$0.2 & 20.00$\pm$0.00 & Tilton \\ 
193 & hs0624 & 0.22329 & 13.0$\pm$0.4 & 11.00$\pm$0.00 & Tilton \\ 
194 & hs0624 & 0.25230 & 13.2$\pm$0.1 & 27.00$\pm$8.80 & Tilton \\ 
195 & hs0624 & 0.29984 & 13.1$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
196 & hs0624 & 0.31794 & 13.7$\pm$0.1 & 29.00$\pm$1.60 & Tilton \\ 
197 & hs0624 & 0.33980 & 13.5$\pm$0.1 & 37.30$\pm$5.30 & Tilton \\ 
198 & hs0624 & 0.34863 & 13.1$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
199 & hs0624 & 0.37034 & 12.8$\pm$0.2 & 8.00$\pm$3.70 & Tilton \\ 
200 & hs0624 & 0.37058 & 13.6$\pm$0.0 & 19.90$\pm$2.40 & Tilton \\ 
201 & hs0624 & 0.37095 & 13.6$\pm$0.0 & 24.40$\pm$1.90 & Tilton \\ 
\hline
202 & hs1102 & 0.20136 & 13.2$\pm$0.2 & 22.10$\pm$6.40 & Danforth$^{1032}$ \\ 
203 & hs1102 & 0.20653 & 14.2$\pm$0.0 & 33.33$\pm$3.60 & Danforth$^{M}$ \\ 
204 & hs1102 & 0.23882 & 14.8$\pm$0.0 & 34.53$\pm$1.97 & Danforth$^{M}$ \\ 
205 & hs1102 & 0.26162 & 14.0$\pm$0.3 & 34.10$\pm$12.40 & Danforth$^{1038}$ \\ 
206 & hs1102 & 0.28902 & 13.8$\pm$0.1 & 56.10$\pm$13.20 & Danforth$^{1032}$ \\ 
207 & hs1102 & 0.28924 & 13.6$\pm$0.2 & 34.20$\pm$10.70 & Danforth$^{1032}$ \\ 
208 & hs1102 & 0.28974 & 14.2$\pm$0.1 & 38.27$\pm$5.27 & Danforth$^{M}$ \\ 
209 & hs1102 & 0.31046 & 14.3$\pm$0.0 & 28.27$\pm$2.40 & Danforth$^{M}$ \\ 
210 & hs1102 & 0.33619 & 13.5$\pm$0.3 & 43.20$\pm$19.60 & Danforth$^{1032}$ \\ 
211 & hs1102 & 0.38188 & 13.9$\pm$0.1 & 30.13$\pm$3.73 & Danforth$^{M}$ \\ 
212 & hs1102 & 0.40794 & 13.8$\pm$0.1 & 33.83$\pm$7.57 & Danforth$^{M}$ \\ 
213 & hs1102 & 0.40978 & 14.1$\pm$0.0 & 73.60$\pm$4.67 & Danforth$^{M}$ \\ 
214 & hs1102 & 0.43768 & 13.8$\pm$0.1 & 18.33$\pm$4.63 & Danforth$^{M}$ \\ 
215 & hs1102 & 0.43807 & 14.1$\pm$0.0 & 32.73$\pm$4.77 & Danforth$^{M}$ \\ 
216 & hs1102 & 0.48393 & 14.3$\pm$0.1 & 51.90$\pm$7.10 & Danforth$^{M}$ \\ 
217 & hs1102 & 0.48432 & 14.3$\pm$0.1 & 44.13$\pm$8.17 & Danforth$^{M}$ \\ 
218 & hs1102 & 0.48495 & 14.4$\pm$0.1 & 96.90$\pm$22.80 & Danforth$^{1032}$ \\ 
219 & hs1102 & 0.48525 & 14.3$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
220 & hs1102 & 0.48637 & 14.5$\pm$0.0 & 77.80$\pm$6.10 & Danforth$^{1038}$ \\ 
221 & hs1102 & 0.50606 & 13.8$\pm$0.1 & 61.60$\pm$8.90 & Danforth$^{1032}$ \\ 
\hline
222 & i22456 & 0.09858 & 14.7$\pm$0.0 & 48.70$\pm$2.10 & Danforth$^{M}$ \\ 
223 & i22456 & 0.09895 & 14.4$\pm$0.1 & 33.80$\pm$5.00 & Danforth$^{1032}$ \\ 
224 & i22456 & 0.09931 & 14.9$\pm$0.0 & 70.37$\pm$3.90 & Danforth$^{M}$ \\ 
225 & i22456 & 0.09959 & 14.0$\pm$0.0 & 9.60$\pm$2.30 & Danforth$^{1038}$ \\ 
226 & i22456 & 0.09989 & 14.8$\pm$0.0 & 34.57$\pm$1.37 & Danforth$^{M}$ \\ 
227 & i22456 & 0.10034 & 14.7$\pm$0.0 & 50.57$\pm$1.80 & Danforth$^{M}$ \\ 
228 & i22456 & 0.10101 & 15.4$\pm$0.0 & 55.57$\pm$1.30 & Danforth$^{M}$ \\ 
229 & i22456 & 0.10146 & 14.0$\pm$0.0 & 23.20$\pm$3.90 & Danforth$^{1032}$ \\ 
\hline
230 & mr2251 & 0.01070 & 13.4$\pm$0.2 & 14.00$\pm$0.00 & Tilton \\ 
\hline
231 & mrk421 & 0.01009 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
\hline
232 & mrk876 & 0.00311 & 13.6$\pm$0.1 & 25.00$\pm$6.00 & Tilton \\ 
233 & mrk876 & 0.06248 & 13.6$\pm$0.1 & 35.00$\pm$2.00 & Tilton \\ 
234 & mrk876 & 0.08579 & 14.1$\pm$0.1 & 51.00$\pm$5.20 & Tilton \\ 
235 & mrk876 & 0.11488 & 14.4$\pm$0.0 & 45.47$\pm$1.90 & Danforth$^{M,*}$ \\ 
236 & mrk876 & 0.11517 & 13.7$\pm$0.1 & 52.93$\pm$9.30 & Danforth$^{M}$ \\ 
237 & mrk876 & 0.11588 & 14.2$\pm$0.0 & 28.67$\pm$1.47 & Danforth$^{M,*}$ \\ 
\hline
238 & ngc7469 & 0.00962 & 14.1$\pm$0.1 & 28.60$\pm$6.00 & Tilton \\ 
239 & ngc7469 & 0.00994 & 14.7$\pm$0.0 & 41.60$\pm$3.00 & Tilton \\ 
240 & ngc7469 & 0.01153 & 13.4$\pm$0.2 & 19.00$\pm$10.00 & Tilton \\ 
\hline
241 & p1103 & 0.13556 & 13.8$\pm$0.2 & 83.50$\pm$26.10 & Danforth$^{1032}$ \\ 
242 & p1103 & 0.13937 & 13.7$\pm$0.2 & 20.60$\pm$11.00 & Danforth$^{M}$ \\ 
243 & p1103 & 0.14099 & 13.6$\pm$0.2 & 11.97$\pm$10.70 & Danforth$^{M}$ \\ 
244 & p1103 & 0.14126 & 14.2$\pm$0.1 & 55.50$\pm$13.50 & Danforth$^{M}$ \\ 
245 & p1103 & 0.17277 & 14.1$\pm$0.0 & 28.30$\pm$0.50 & Danforth$^{1032}$ \\ 
\hline
246 & pg0003 & 0.16521 & 13.8$\pm$0.2 & 61.03$\pm$13.67 & Danforth$^{M}$ \\ 
247 & pg0003 & 0.20907 & 13.7$\pm$0.1 & 34.10$\pm$5.70 & Danforth$^{1032}$ \\ 
248 & pg0003 & 0.29021 & 14.2$\pm$0.0 & 37.30$\pm$4.67 & Danforth$^{M}$ \\ 
249 & pg0003 & 0.30551 & 13.2$\pm$0.2 & 22.40$\pm$16.30 & Danforth$^{1032}$ \\ 
250 & pg0003 & 0.30569 & 13.3$\pm$0.2 & 19.00$\pm$13.73 & Danforth$^{M}$ \\ 
251 & pg0003 & 0.34757 & 14.3$\pm$0.0 & 29.47$\pm$2.60 & Danforth$^{M}$ \\ 
252 & pg0003 & 0.34788 & 13.9$\pm$0.1 & 15.47$\pm$2.70 & Danforth$^{M}$ \\ 
253 & pg0003 & 0.36452 & 14.3$\pm$0.0 & 40.43$\pm$2.30 & Danforth$^{M}$ \\ 
254 & pg0003 & 0.36508 & 14.5$\pm$0.0 & 27.60$\pm$1.40 & Danforth$^{1032}$ \\ 
255 & pg0003 & 0.36572 & 14.1$\pm$0.1 & 36.17$\pm$5.43 & Danforth$^{M}$ \\ 
256 & pg0003 & 0.36621 & 14.1$\pm$0.0 & 30.53$\pm$2.53 & Danforth$^{M}$ \\ 
257 & pg0003 & 0.37029 & 13.6$\pm$0.1 & 61.60$\pm$11.50 & Danforth$^{1032}$ \\ 
258 & pg0003 & 0.38608 & 13.8$\pm$0.1 & 23.83$\pm$4.10 & Danforth$^{M}$ \\ 
259 & pg0003 & 0.38639 & 13.9$\pm$0.1 & 36.77$\pm$5.90 & Danforth$^{M}$ \\ 
260 & pg0003 & 0.40138 & 14.3$\pm$0.0 & 32.80$\pm$1.87 & Danforth$^{M}$ \\ 
261 & pg0003 & 0.42192 & 14.3$\pm$0.0 & 27.67$\pm$1.97 & Danforth$^{M}$ \\ 
\hline
262 & pg0157 & 0.14621 & 13.4$\pm$0.2 & 13.10$\pm$9.40 & Danforth$^{1032}$ \\ 
\hline
263 & pg0804 & 0.00382 & 13.5$\pm$0.2 & 17.00$\pm$0.00 & Tilton \\ 
264 & pg0804 & 0.01851 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
265 & pg0804 & 0.10216 & 14.2$\pm$0.0 & 50.03$\pm$3.87 & Danforth$^{M}$ \\ 
266 & pg0804 & 0.10230 & 14.0$\pm$0.1 & 34.30$\pm$3.10 & Tilton \\ 
\hline
267 & pg0832 & 0.10772 & 13.5$\pm$0.0 & 17.80$\pm$1.00 & Danforth$^{1038}$ \\ 
268 & pg0832 & 0.13230 & 14.0$\pm$0.2 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
269 & pg0832 & 0.15276 & 13.8$\pm$0.2 & 52.20$\pm$20.10 & Danforth$^{1032}$ \\ 
270 & pg0832 & 0.23308 & 13.8$\pm$0.2 & 54.30$\pm$14.80 & Danforth$^{1032}$ \\ 
271 & pg0832 & 0.32567 & 14.1$\pm$0.1 & 60.83$\pm$7.80 & Danforth$^{M}$ \\ 
\hline
272 & pg0953 & 0.01560 & 13.7$\pm$0.2 & 11.00$\pm$0.00 & Tilton \\ 
273 & pg0953 & 0.05891 & 13.9$\pm$0.1 & 26.00$\pm$8.00 & Tilton \\ 
274 & pg0953 & 0.06807 & 14.3$\pm$0.1 & 13.50$\pm$1.80 & Tilton \\ 
275 & pg0953 & 0.11827 & 13.3$\pm$0.2 & 12.00$\pm$0.00 & Tilton \\ 
276 & pg0953 & 0.14236 & 14.0$\pm$0.0 & 20.63$\pm$2.37 & Danforth$^{M,*}$ \\ 
277 & pg0953 & 0.14263 & 13.6$\pm$0.1 & 27.17$\pm$5.87 & Danforth$^{M}$ \\ 
278 & pg0953 & 0.14307 & 13.3$\pm$0.1 & 36.43$\pm$4.63 & Danforth$^{M}$ \\ 
279 & pg0953 & 0.22967 & 13.9$\pm$0.0 & 33.97$\pm$2.37 & Danforth$^{M,*}$ \\ 
280 & pg0953 & 0.23251 & 13.4$\pm$0.1 & 19.20$\pm$2.80 & Danforth$^{1032}$ \\ 
281 & pg0953 & 0.23351 & 13.5$\pm$0.1 & 10.53$\pm$2.40 & Danforth$^{M,*}$ \\ 
\hline
282 & pg1001 & 0.13773 & 14.1$\pm$0.1 & 47.30$\pm$5.93 & Danforth$^{M}$ \\ 
283 & pg1001 & 0.21259 & 13.4$\pm$0.1 & 24.70$\pm$6.70 & Danforth$^{1032}$ \\ 
284 & pg1001 & 0.27333 & 13.3$\pm$0.2 & 20.07$\pm$10.07 & Danforth$^{M}$ \\ 
285 & pg1001 & 0.33018 & 14.2$\pm$0.1 & 10.67$\pm$1.20 & Danforth$^{M}$ \\ 
\hline
286 & pg1049 & 0.19406 & 13.7$\pm$0.2 & 27.60$\pm$11.37 & Danforth$^{M}$ \\ 
287 & pg1049 & 0.32490 & 13.7$\pm$0.3 & 51.80$\pm$15.80 & Danforth$^{M}$ \\ 
288 & pg1049 & 0.32545 & 13.7$\pm$0.1 & 54.40$\pm$20.30 & Danforth$^{1032}$ \\ 
289 & pg1049 & 0.32569 & 14.4$\pm$0.1 & 82.60$\pm$20.60 & Danforth$^{1038}$ \\ 
290 & pg1049 & 0.33481 & 14.4$\pm$0.1 & 90.00$\pm$13.50 & Danforth$^{1032}$ \\ 
291 & pg1049 & 0.33531 & 14.5$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
292 & pg1049 & 0.33904 & 14.1$\pm$0.1 & 51.63$\pm$8.57 & Danforth$^{M}$ \\ 
293 & pg1049 & 0.34006 & 15.1$\pm$0.0 & 80.77$\pm$4.07 & Danforth$^{M}$ \\ 
294 & pg1049 & 0.34096 & 14.9$\pm$0.0 & 80.10$\pm$7.43 & Danforth$^{M}$ \\ 
295 & pg1049 & 0.34181 & 15.1$\pm$0.0 & 68.97$\pm$4.83 & Danforth$^{M}$ \\ 
296 & pg1049 & 0.34260 & 14.6$\pm$0.0 & 76.90$\pm$10.43 & Danforth$^{M}$ \\ 
\hline
297 & pg1115 & 0.12285 & 13.6$\pm$0.2 & 28.67$\pm$12.13 & Danforth$^{M}$ \\ 
298 & pg1115 & 0.12313 & 13.8$\pm$0.1 & 29.87$\pm$11.33 & Danforth$^{M}$ \\ 
299 & pg1115 & 0.13104 & 14.0$\pm$0.1 & 39.40$\pm$6.13 & Danforth$^{M}$ \\ 
300 & pg1115 & 0.15456 & 14.3$\pm$0.1 & 27.37$\pm$3.57 & Danforth$^{M}$ \\ 
301 & pg1115 & 0.15467 & 14.7$\pm$0.0 & 26.50$\pm$2.00 & Danforth$^{1032}$ \\ 
\hline
302 & pg1116 & 0.05900 & 13.5$\pm$0.2 & 20.00$\pm$4.00 & Tilton \\ 
303 & pg1116 & 0.05927 & 13.5$\pm$0.2 & 12.30$\pm$5.70 & Tilton \\ 
304 & pg1116 & 0.11895 & 13.6$\pm$0.2 & 78.90$\pm$17.40 & Danforth$^{1032}$ \\ 
305 & pg1116 & 0.13852 & 13.8$\pm$0.1 & 33.87$\pm$4.00 & Danforth$^{M,*}$ \\ 
306 & pg1116 & 0.16539 & 13.7$\pm$0.3 & 35.07$\pm$16.97 & Danforth$^{M}$ \\ 
307 & pg1116 & 0.16554 & 13.9$\pm$0.1 & 20.70$\pm$3.20 & Danforth$^{M,*}$ \\ 
308 & pg1116 & 0.16610 & 13.6$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
309 & pg1116 & 0.16686 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
310 & pg1116 & 0.17343 & 13.3$\pm$0.1 & 40.90$\pm$8.80 & Danforth$^{1032*}$ \\ 
\hline
311 & pg1121 & 0.19245 & 13.4$\pm$0.1 & 17.10$\pm$7.70 & Danforth$^{1032}$ \\ 
312 & pg1121 & 0.21986 & 14.3$\pm$0.0 & 43.00$\pm$2.60 & Danforth$^{M}$ \\ 
\hline
313 & pg1211 & 0.00711 & 13.8$\pm$0.1 & 41.00$\pm$7.00 & Tilton \\ 
314 & pg1211 & 0.05117 & 14.3$\pm$0.1 & 53.00$\pm$9.50 & Tilton \\ 
315 & pg1211 & 0.06449 & 14.1$\pm$0.0 & 47.20$\pm$5.40 & Tilton \\ 
316 & pg1211 & 0.06491 & 13.7$\pm$0.1 & 26.60$\pm$5.10 & Tilton \\ 
\hline
317 & pg1216 & 0.12362 & 14.2$\pm$0.1 & 32.10$\pm$7.27 & Danforth$^{M,*}$ \\ 
318 & pg1216 & 0.12389 & 14.1$\pm$0.1 & 32.43$\pm$8.73 & Danforth$^{M,*}$ \\ 
319 & pg1216 & 0.12463 & 13.8$\pm$0.5 & 6.00$\pm$41.00 & Tilton \\ 
320 & pg1216 & 0.12485 & 14.2$\pm$0.1 & 60.00$\pm$9.03 & Danforth$^{M,*}$ \\ 
321 & pg1216 & 0.13499 & 13.8$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
322 & pg1216 & 0.26768 & 13.7$\pm$0.6 & 19.00$\pm$2.00 & Tilton \\ 
323 & pg1216 & 0.28199 & 13.8$\pm$0.2 & 47.17$\pm$11.20 & Danforth$^{M}$ \\ 
324 & pg1216 & 0.28237 & 13.6$\pm$0.1 & 14.43$\pm$5.40 & Danforth$^{M}$ \\ 
\hline
325 & pg1222 & 0.16715 & 13.5$\pm$0.2 & 5.00$\pm$0.00 & Danforth$^{M}$ \\ 
326 & pg1222 & 0.22263 & 13.9$\pm$0.1 & 30.47$\pm$5.77 & Danforth$^{M}$ \\ 
327 & pg1222 & 0.24184 & 14.2$\pm$0.2 & 30.10$\pm$7.80 & Danforth$^{M}$ \\ 
328 & pg1222 & 0.24454 & 14.1$\pm$0.1 & 25.13$\pm$4.17 & Danforth$^{M}$ \\ 
329 & pg1222 & 0.34686 & 13.6$\pm$0.2 & 30.17$\pm$10.03 & Danforth$^{M}$ \\ 
330 & pg1222 & 0.34941 & 13.8$\pm$0.1 & 42.37$\pm$6.20 & Danforth$^{M}$ \\ 
331 & pg1222 & 0.36375 & 13.6$\pm$0.1 & 32.13$\pm$6.67 & Danforth$^{M}$ \\ 
332 & pg1222 & 0.37616 & 13.5$\pm$0.1 & 31.60$\pm$5.70 & Danforth$^{1032}$ \\ 
333 & pg1222 & 0.37706 & 13.8$\pm$0.1 & 28.53$\pm$4.93 & Danforth$^{M}$ \\ 
334 & pg1222 & 0.37730 & 13.5$\pm$0.1 & 29.83$\pm$8.23 & Danforth$^{M}$ \\ 
335 & pg1222 & 0.37842 & 14.1$\pm$0.0 & 38.97$\pm$3.43 & Danforth$^{M}$ \\ 
336 & pg1222 & 0.37869 & 13.4$\pm$0.1 & 19.37$\pm$6.13 & Danforth$^{M}$ \\ 
337 & pg1222 & 0.39726 & 13.1$\pm$0.2 & 34.50$\pm$6.40 & Danforth$^{1032}$ \\ 
338 & pg1222 & 0.40828 & 13.1$\pm$0.2 & 30.50$\pm$12.70 & Danforth$^{1032}$ \\ 
339 & pg1222 & 0.42130 & 13.9$\pm$0.1 & 32.20$\pm$3.97 & Danforth$^{M}$ \\ 
340 & pg1222 & 0.42308 & 14.0$\pm$0.0 & 18.77$\pm$1.97 & Danforth$^{M}$ \\ 
\hline
341 & pg1259 & 0.00220 & 13.6$\pm$0.1 & 75.00$\pm$0.00 & Tilton \\ 
342 & pg1259 & 0.00762 & 13.3$\pm$0.1 & 24.00$\pm$16.00 & Tilton \\ 
343 & pg1259 & 0.02217 & 13.4$\pm$0.2 & 34.00$\pm$15.00 & Tilton \\ 
344 & pg1259 & 0.04606 & 13.9$\pm$0.1 & 39.00$\pm$12.00 & Tilton \\ 
345 & pg1259 & 0.04650 & 13.8$\pm$0.1 & 24.00$\pm$4.00 & Tilton \\ 
346 & pg1259 & 0.19576 & 13.7$\pm$0.1 & 21.90$\pm$3.57 & Danforth$^{M}$ \\ 
347 & pg1259 & 0.21940 & 14.1$\pm$0.0 & 38.30$\pm$2.60 & Danforth$^{M,*}$ \\ 
348 & pg1259 & 0.21953 & 13.6$\pm$0.1 & 14.20$\pm$2.00 & Tilton \\ 
349 & pg1259 & 0.22313 & 13.6$\pm$0.1 & 50.50$\pm$17.50 & Tilton \\ 
350 & pg1259 & 0.23284 & 13.5$\pm$0.1 & 17.00$\pm$8.00 & Tilton \\ 
351 & pg1259 & 0.23956 & 13.4$\pm$0.1 & 24.00$\pm$7.20 & Danforth$^{1032}$ \\ 
352 & pg1259 & 0.25973 & 13.8$\pm$0.1 & 52.70$\pm$7.60 & Danforth$^{1032*}$ \\ 
353 & pg1259 & 0.31979 & 13.3$\pm$0.1 & 17.67$\pm$6.13 & Danforth$^{M,*}$ \\ 
354 & pg1259 & 0.32472 & 13.3$\pm$0.1 & 14.00$\pm$8.00 & Tilton \\ 
\hline
355 & pg1307 & 0.14187 & 13.9$\pm$0.1 & 42.03$\pm$12.67 & Danforth$^{M}$ \\ 
356 & pg1307 & 0.14214 & 13.8$\pm$0.1 & 15.90$\pm$5.07 & Danforth$^{M}$ \\ 
\hline
357 & pg1309 & 0.17586 & 14.4$\pm$0.1 & 30.50$\pm$2.27 & Danforth$^{M}$ \\ 
358 & pg1309 & 0.17745 & 15.2$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
359 & pg1309 & 0.17866 & 15.9$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
360 & pg1309 & 0.17930 & 15.5$\pm$0.0 & 99.60$\pm$8.20 & Danforth$^{1038}$ \\ 
361 & pg1309 & 0.17979 & 15.2$\pm$0.0 & 73.60$\pm$7.20 & Danforth$^{1038}$ \\ 
362 & pg1309 & 0.18069 & 15.2$\pm$0.0 & 74.20$\pm$3.50 & Danforth$^{1038}$ \\ 
363 & pg1309 & 0.18117 & 15.1$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
364 & pg1309 & 0.18139 & 14.9$\pm$0.0 & 60.00$\pm$5.30 & Danforth$^{1038}$ \\ 
365 & pg1309 & 0.18145 & 14.8$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
366 & pg1309 & 0.18192 & 14.3$\pm$0.0 & 69.60$\pm$5.60 & Danforth$^{1032}$ \\ 
367 & pg1309 & 0.18698 & 14.0$\pm$2.5 & 28.00$\pm$9.90 & Danforth$^{1038}$ \\ 
\hline
368 & pg1424 & 0.12120 & 14.0$\pm$0.2 & 41.30$\pm$23.90 & Danforth$^{1032}$ \\ 
369 & pg1424 & 0.12152 & 14.4$\pm$0.1 & 32.17$\pm$4.43 & Danforth$^{M}$ \\ 
370 & pg1424 & 0.14689 & 13.9$\pm$0.2 & 48.13$\pm$19.27 & Danforth$^{M}$ \\ 
371 & pg1424 & 0.14712 & 13.7$\pm$0.2 & 16.20$\pm$9.30 & Danforth$^{1032}$ \\ 
372 & pg1424 & 0.33947 & 13.5$\pm$0.1 & 18.20$\pm$8.27 & Danforth$^{M}$ \\ 
373 & pg1424 & 0.33988 & 13.6$\pm$0.1 & 13.77$\pm$4.37 & Danforth$^{M}$ \\ 
374 & pg1424 & 0.38633 & 13.8$\pm$0.1 & 33.53$\pm$10.60 & Danforth$^{M}$ \\ 
375 & pg1424 & 0.38662 & 14.1$\pm$0.0 & 24.13$\pm$1.90 & Danforth$^{M}$ \\ 
376 & pg1424 & 0.42884 & 13.1$\pm$0.1 & 7.10$\pm$9.80 & Danforth$^{1032}$ \\ 
377 & pg1424 & 0.60369 & 13.4$\pm$0.1 & 10.10$\pm$5.60 & Danforth$^{1032}$ \\ 
\hline
378 & pg1444 & 0.22031 & 13.9$\pm$0.1 & 49.00$\pm$2.00 & Tilton \\ 
379 & pg1444 & 0.22676 & 13.3$\pm$0.1 & 27.00$\pm$5.00 & Tilton \\ 
380 & pg1444 & 0.26690 & 13.8$\pm$0.0 & 11.50$\pm$1.00 & Tilton \\ 
381 & pg1444 & 0.26728 & 13.5$\pm$0.1 & 14.90$\pm$3.80 & Tilton \\ 
382 & pg1444 & 0.26738 & 13.9$\pm$0.1 & 8.40$\pm$1.30 & Tilton \\ 
383 & pg1444 & 0.26747 & 13.5$\pm$0.1 & 11.90$\pm$2.90 & Tilton \\ 
\hline
384 & pg1626 & 0.13075 & 13.3$\pm$0.2 & 31.40$\pm$11.10 & Danforth$^{1032}$ \\ 
\hline
385 & phl1811 & 0.07344 & 13.0$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
386 & phl1811 & 0.07768 & 13.6$\pm$0.1 & 31.00$\pm$16.00 & Tilton \\ 
387 & phl1811 & 0.08131 & 13.9$\pm$0.2 & 7.90$\pm$5.20 & Tilton \\ 
388 & phl1811 & 0.13239 & 13.9$\pm$0.1 & 59.27$\pm$10.23 & Danforth$^{M,*}$ \\ 
389 & phl1811 & 0.13282 & 13.6$\pm$0.1 & 21.07$\pm$5.73 & Danforth$^{M,*}$ \\ 
390 & phl1811 & 0.13318 & 13.7$\pm$0.1 & 37.63$\pm$5.97 & Danforth$^{M,*}$ \\ 
391 & phl1811 & 0.13545 & 13.5$\pm$0.2 & 32.80$\pm$11.30 & Danforth$^{1038}$ \\ 
392 & phl1811 & 0.15752 & 13.5$\pm$0.1 & 37.03$\pm$10.37 & Danforth$^{M}$ \\ 
393 & phl1811 & 0.15786 & 13.6$\pm$0.1 & 29.03$\pm$5.83 & Danforth$^{M,*}$ \\ 
394 & phl1811 & 0.17652 & 14.1$\pm$0.0 & 18.10$\pm$2.20 & Danforth$^{1038*}$ \\ 
395 & phl1811 & 0.19157 & 13.5$\pm$0.1 & 23.37$\pm$5.17 & Danforth$^{M,*}$ \\ 
396 & phl1811 & 0.19194 & 14.7$\pm$0.0 & 34.87$\pm$1.70 & Danforth$^{M,*}$ \\ 
397 & phl1811 & 0.19220 & 13.6$\pm$0.2 & 30.30$\pm$17.47 & Danforth$^{M,*}$ \\ 
\hline
398 & phl2525 & 0.20154 & 14.1$\pm$0.0 & 19.40$\pm$2.13 & Danforth$^{M}$ \\ 
399 & phl2525 & 0.20207 & 13.6$\pm$0.1 & 19.13$\pm$4.60 & Danforth$^{M}$ \\ 
400 & phl2525 & 0.20605 & 14.0$\pm$0.1 & 39.73$\pm$6.70 & Danforth$^{M}$ \\ 
\hline
401 & pks0312 & 0.20188 & 13.8$\pm$0.1 & 40.00$\pm$0.00 & Tilton \\ 
402 & pks0312 & 0.20275 & 14.9$\pm$0.1 & 65.40$\pm$1.30 & Tilton \\ 
\hline
403 & pks0405 & 0.09192 & 13.8$\pm$0.0 & 25.00$\pm$10.00 & Tilton \\ 
404 & pks0405 & 0.09647 & 13.7$\pm$0.3 & 31.30$\pm$7.60 & Danforth$^{1038*}$ \\ 
405 & pks0405 & 0.14808 & 13.7$\pm$0.0 & 85.07$\pm$1.67 & Danforth$^{M}$ \\ 
406 & pks0405 & 0.16566 & 13.0$\pm$0.2 & 7.90$\pm$8.10 & Danforth$^{1038}$ \\ 
407 & pks0405 & 0.16606 & 14.1$\pm$0.0 & 74.20$\pm$3.20 & Danforth$^{1032*}$ \\ 
408 & pks0405 & 0.16659 & 13.9$\pm$0.1 & 31.20$\pm$4.70 & Danforth$^{M}$ \\ 
409 & pks0405 & 0.16688 & 14.2$\pm$0.1 & 40.33$\pm$8.93 & Danforth$^{M}$ \\ 
410 & pks0405 & 0.16712 & 14.4$\pm$0.1 & 36.90$\pm$3.03 & Danforth$^{M,*}$ \\ 
411 & pks0405 & 0.18257 & 13.7$\pm$2.0 & 34.70$\pm$4.97 & Danforth$^{M,*}$ \\ 
412 & pks0405 & 0.18289 & 13.8$\pm$0.6 & 18.53$\pm$1.47 & Danforth$^{M,*}$ \\ 
413 & pks0405 & 0.24052 & 13.5$\pm$0.1 & 33.60$\pm$4.30 & Danforth$^{M}$ \\ 
414 & pks0405 & 0.24094 & 13.0$\pm$0.1 & 26.00$\pm$7.80 & Danforth$^{1032}$ \\ 
415 & pks0405 & 0.24547 & 12.7$\pm$0.2 & 8.40$\pm$7.70 & Danforth$^{1032}$ \\ 
416 & pks0405 & 0.29762 & 13.6$\pm$0.1 & 66.87$\pm$6.50 & Danforth$^{M}$ \\ 
417 & pks0405 & 0.34188 & 13.5$\pm$0.0 & 37.30$\pm$3.50 & Danforth$^{1032}$ \\ 
418 & pks0405 & 0.34225 & 13.3$\pm$0.0 & 24.00$\pm$3.40 & Danforth$^{1032}$ \\ 
419 & pks0405 & 0.35092 & 13.3$\pm$0.2 & 35.00$\pm$7.00 & Tilton \\ 
420 & pks0405 & 0.36075 & 13.2$\pm$0.0 & 29.60$\pm$4.30 & Danforth$^{1032*}$ \\ 
421 & pks0405 & 0.36151 & 13.9$\pm$0.0 & 32.17$\pm$1.43 & Danforth$^{M,*}$ \\ 
422 & pks0405 & 0.36329 & 13.5$\pm$0.0 & 17.97$\pm$1.67 & Danforth$^{M,*}$ \\ 
423 & pks0405 & 0.40570 & 13.6$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
424 & pks0405 & 0.40890 & 13.2$\pm$0.1 & 36.93$\pm$6.70 & Danforth$^{M}$ \\ 
425 & pks0405 & 0.49505 & 14.3$\pm$0.0 & 32.50$\pm$2.53 & Danforth$^{M,*}$ \\ 
426 & pks0405 & 0.49530 & 13.8$\pm$0.1 & 15.97$\pm$2.63 & Danforth$^{M,*}$ \\ 
427 & pks0405 & 0.55506 & 14.0$\pm$0.1 & 27.90$\pm$3.13 & Danforth$^{M}$ \\ 
\hline
428 & pks0552 & 0.11067 & 13.9$\pm$0.1 & 33.60$\pm$12.30 & Danforth$^{1038}$ \\ 
429 & pks0552 & 0.14861 & 13.6$\pm$0.1 & 13.50$\pm$5.50 & Danforth$^{1032}$ \\ 
430 & pks0552 & 0.14893 & 13.8$\pm$0.1 & 45.80$\pm$11.50 & Danforth$^{1032}$ \\ 
431 & pks0552 & 0.18726 & 13.7$\pm$0.1 & 31.40$\pm$9.30 & Danforth$^{1032}$ \\ 
432 & pks0552 & 0.25380 & 13.5$\pm$1.6 & 25.17$\pm$7.50 & Danforth$^{M}$ \\ 
433 & pks0552 & 0.27850 & 13.7$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
434 & pks0552 & 0.28570 & 13.8$\pm$0.1 & 28.40$\pm$4.63 & Danforth$^{M}$ \\ 
435 & pks0552 & 0.34489 & 13.1$\pm$0.2 & 27.30$\pm$8.10 & Danforth$^{1032}$ \\ 
436 & pks0552 & 0.37621 & 13.6$\pm$0.1 & 43.90$\pm$10.17 & Danforth$^{M}$ \\ 
437 & pks0552 & 0.37655 & 13.6$\pm$0.1 & 25.20$\pm$4.93 & Danforth$^{M}$ \\ 
438 & pks0552 & 0.37974 & 13.1$\pm$0.1 & 24.50$\pm$8.30 & Danforth$^{1032}$ \\ 
439 & pks0552 & 0.39346 & 13.3$\pm$0.1 & 21.30$\pm$6.50 & Danforth$^{1032}$ \\ 
440 & pks0552 & 0.42511 & 13.2$\pm$0.2 & 25.40$\pm$12.60 & Danforth$^{1032}$ \\ 
441 & pks0552 & 0.44610 & 13.6$\pm$0.1 & 24.83$\pm$6.53 & Danforth$^{M}$ \\ 
442 & pks0552 & 0.59449 & 13.4$\pm$0.1 & 10.20$\pm$4.60 & Danforth$^{1032}$ \\ 
443 & pks0552 & 0.63163 & 13.8$\pm$0.1 & 8.83$\pm$3.73 & Danforth$^{M}$ \\ 
444 & pks0552 & 0.63186 & 13.9$\pm$0.1 & 14.10$\pm$3.10 & Danforth$^{M}$ \\ 
\hline
445 & pks0637 & 0.12291 & 14.1$\pm$0.1 & 43.87$\pm$5.67 & Danforth$^{M}$ \\ 
446 & pks0637 & 0.14420 & 13.8$\pm$0.1 & 29.30$\pm$10.30 & Danforth$^{1038}$ \\ 
447 & pks0637 & 0.16107 & 14.1$\pm$0.1 & 52.77$\pm$7.50 & Danforth$^{M}$ \\ 
448 & pks0637 & 0.20475 & 13.6$\pm$0.2 & 48.57$\pm$15.07 & Danforth$^{M}$ \\ 
449 & pks0637 & 0.24873 & 14.0$\pm$0.1 & 62.50$\pm$13.40 & Danforth$^{1038}$ \\ 
450 & pks0637 & 0.30079 & 13.8$\pm$0.1 & 25.77$\pm$7.70 & Danforth$^{M}$ \\ 
451 & pks0637 & 0.30107 & 14.0$\pm$0.0 & 26.20$\pm$2.80 & Danforth$^{1032}$ \\ 
452 & pks0637 & 0.38642 & 13.8$\pm$0.1 & 28.77$\pm$3.97 & Danforth$^{M}$ \\ 
453 & pks0637 & 0.40897 & 13.8$\pm$0.1 & 60.60$\pm$18.20 & Danforth$^{1038}$ \\ 
454 & pks0637 & 0.41753 & 14.2$\pm$0.0 & 45.33$\pm$4.60 & Danforth$^{M}$ \\ 
455 & pks0637 & 0.45294 & 13.7$\pm$0.1 & 36.10$\pm$11.60 & Danforth$^{M}$ \\ 
456 & pks0637 & 0.46848 & 13.9$\pm$0.1 & 55.10$\pm$11.30 & Danforth$^{M}$ \\ 
\hline
457 & pks1302 & 0.04225 & 14.4$\pm$0.1 & 54.00$\pm$3.00 & Tilton \\ 
458 & pks1302 & 0.06474 & 13.7$\pm$0.2 & 42.00$\pm$0.00 & Tilton \\ 
459 & pks1302 & 0.09486 & 13.9$\pm$0.2 & 61.60$\pm$17.80 & Tilton \\ 
460 & pks1302 & 0.09891 & 14.0$\pm$0.1 & 54.00$\pm$4.00 & Tilton \\ 
461 & pks1302 & 0.14518 & 13.8$\pm$0.1 & 31.67$\pm$6.33 & Danforth$^{M,*}$ \\ 
462 & pks1302 & 0.14552 & 13.4$\pm$0.1 & 23.10$\pm$8.80 & Danforth$^{1032*}$ \\ 
463 & pks1302 & 0.20438 & 13.6$\pm$0.1 & 38.00$\pm$3.80 & Tilton \\ 
464 & pks1302 & 0.22563 & 13.9$\pm$0.1 & 33.13$\pm$4.67 & Danforth$^{M,*}$ \\ 
465 & pks1302 & 0.22743 & 13.5$\pm$0.1 & 10.37$\pm$3.50 & Danforth$^{M,*}$ \\ 
466 & pks1302 & 0.25288 & 12.9$\pm$0.2 & 8.00$\pm$3.00 & Tilton \\ 
467 & pks1302 & 0.25299 & 13.4$\pm$0.3 & 30.90$\pm$10.80 & Danforth$^{1032}$ \\ 
\hline
468 & pks2005 & 0.06490 & 13.6$\pm$0.1 & 30.70$\pm$0.00 & Tilton \\ 
\hline
469 & pks2155 & 0.05405 & 13.6$\pm$0.1 & 14.00$\pm$6.00 & Tilton \\ 
470 & pks2155 & 0.05707 & 13.6$\pm$0.1 & 24.00$\pm$7.00 & Tilton \\ 
\hline
471 & pmn2345 & 0.19957 & 14.4$\pm$0.1 & 53.00$\pm$6.90 & Danforth$^{1038}$ \\ 
472 & pmn2345 & 0.37816 & 13.5$\pm$0.2 & 57.80$\pm$16.20 & Danforth$^{1032}$ \\ 
473 & pmn2345 & 0.39704 & 13.7$\pm$0.2 & 48.10$\pm$9.10 & Danforth$^{1032}$ \\ 
474 & pmn2345 & 0.42744 & 14.0$\pm$0.1 & 16.27$\pm$3.57 & Danforth$^{M}$ \\ 
475 & pmn2345 & 0.43053 & 13.8$\pm$0.1 & 23.73$\pm$6.77 & Danforth$^{M}$ \\ 
476 & pmn2345 & 0.43755 & 13.7$\pm$0.2 & 33.37$\pm$9.23 & Danforth$^{M}$ \\ 
477 & pmn2345 & 0.51360 & 14.0$\pm$0.1 & 22.90$\pm$5.37 & Danforth$^{M}$ \\ 
478 & pmn2345 & 0.53517 & 13.5$\pm$0.2 & 11.20$\pm$7.80 & Danforth$^{1032}$ \\ 
479 & pmn2345 & 0.59970 & 14.0$\pm$0.2 & 42.00$\pm$7.90 & Danforth$^{1032}$ \\ 
480 & pmn2345 & 0.61135 & 13.5$\pm$0.1 & 10.00$\pm$6.90 & Danforth$^{1032}$ \\ 
481 & pmn2345 & 0.61155 & 13.8$\pm$0.2 & 20.00$\pm$6.30 & Danforth$^{1038}$ \\ 
482 & pmn2345 & 0.61196 & 14.4$\pm$0.1 & 47.70$\pm$5.53 & Danforth$^{M}$ \\ 
\hline
483 & q0045 & 0.11052 & 13.8$\pm$0.2 & 45.47$\pm$9.40 & Danforth$^{M}$ \\ 
484 & q0045 & 0.13521 & 15.0$\pm$0.0 & 32.67$\pm$0.93 & Danforth$^{M}$ \\ 
\hline
485 & q1230 & 0.09518 & 14.5$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
486 & q1230 & 0.10318 & 13.4$\pm$0.2 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
487 & q1230 & 0.10445 & 13.4$\pm$0.1 & 15.30$\pm$5.50 & Danforth$^{1032}$ \\ 
488 & q1230 & 0.10530 & 15.1$\pm$0.0 & 89.83$\pm$2.30 & Danforth$^{M,*}$ \\ 
489 & q1230 & 0.10596 & 15.1$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{M,*}$ \\ 
490 & q1230 & 0.10666 & 15.0$\pm$0.0 & 76.87$\pm$2.30 & Danforth$^{M,*}$ \\ 
491 & q1230 & 0.10809 & 14.1$\pm$0.1 & 34.93$\pm$3.93 & Danforth$^{M}$ \\ 
492 & q1230 & 0.10820 & 14.6$\pm$0.1 & 78.10$\pm$10.90 & Danforth$^{1032}$ \\ 
493 & q1230 & 0.10861 & 14.6$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{M}$ \\ 
494 & q1230 & 0.10906 & 15.0$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
495 & q1230 & 0.10935 & 15.5$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
496 & q1230 & 0.10956 & 15.1$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
497 & q1230 & 0.11707 & 15.2$\pm$0.0 & 48.67$\pm$1.20 & Danforth$^{M}$ \\ 
498 & q1230 & 0.11743 & 14.8$\pm$0.0 & 22.70$\pm$1.37 & Danforth$^{M}$ \\ 
499 & q1230 & 0.11781 & 15.0$\pm$0.0 & 41.10$\pm$0.93 & Danforth$^{M}$ \\ 
\hline
500 & rbs1892 & 0.15752 & 14.3$\pm$0.0 & 46.13$\pm$4.50 & Danforth$^{M}$ \\ 
501 & rbs1892 & 0.17133 & 13.7$\pm$0.1 & 41.00$\pm$10.20 & Danforth$^{1032}$ \\ 
502 & rbs1892 & 0.19874 & 13.7$\pm$0.1 & 9.07$\pm$2.80 & Danforth$^{M}$ \\ 
\hline
503 & rbs542 & 0.10323 & 15.5$\pm$0.0 & 62.60$\pm$0.87 & Danforth$^{M}$ \\ 
504 & rbs542 & 0.10379 & 14.7$\pm$0.0 & 29.17$\pm$0.57 & Danforth$^{M}$ \\ 
\hline
505 & rxj0439 & 0.11547 & 14.1$\pm$0.1 & 35.87$\pm$8.73 & Danforth$^{M}$ \\ 
506 & rxj0439 & 0.21833 & 13.5$\pm$0.1 & 11.80$\pm$5.70 & Danforth$^{1032}$ \\ 
507 & rxj0439 & 0.24235 & 14.3$\pm$0.1 & 26.13$\pm$6.03 & Danforth$^{M}$ \\ 
508 & rxj0439 & 0.24258 & 14.3$\pm$0.1 & 15.23$\pm$3.70 & Danforth$^{M}$ \\ 
509 & rxj0439 & 0.24313 & 14.7$\pm$0.0 & 43.03$\pm$3.53 & Danforth$^{M}$ \\ 
510 & rxj0439 & 0.24387 & 13.9$\pm$0.1 & 40.00$\pm$8.93 & Danforth$^{M}$ \\ 
\hline
511 & rxj2154 & 0.15689 & 13.8$\pm$0.1 & 33.53$\pm$6.00 & Danforth$^{M}$ \\ 
512 & rxj2154 & 0.15862 & 13.6$\pm$0.1 & 33.13$\pm$10.50 & Danforth$^{M}$ \\ 
513 & rxj2154 & 0.15889 & 13.7$\pm$0.1 & 9.23$\pm$3.93 & Danforth$^{M}$ \\ 
\hline
514 & s080908 & 0.12865 & 14.1$\pm$0.1 & 90.60$\pm$8.87 & Danforth$^{M}$ \\ 
515 & s080908 & 0.30757 & 14.5$\pm$0.0 & 32.77$\pm$2.60 & Danforth$^{M}$ \\ 
516 & s080908 & 0.32236 & 14.3$\pm$0.5 & 7.30$\pm$3.30 & Danforth$^{1032}$ \\ 
517 & s080908 & 0.37184 & 13.9$\pm$0.1 & 23.27$\pm$4.77 & Danforth$^{M}$ \\ 
518 & s080908 & 0.40733 & 13.7$\pm$0.1 & 17.87$\pm$9.63 & Danforth$^{M}$ \\ 
519 & s080908 & 0.40764 & 14.0$\pm$0.1 & 30.40$\pm$9.97 & Danforth$^{M}$ \\ 
520 & s080908 & 0.41759 & 14.1$\pm$0.1 & 49.23$\pm$7.50 & Danforth$^{M}$ \\ 
521 & s080908 & 0.51541 & 13.8$\pm$0.1 & 48.00$\pm$18.40 & Danforth$^{1032}$ \\ 
522 & s080908 & 0.60328 & 13.8$\pm$0.2 & 18.80$\pm$5.07 & Danforth$^{M}$ \\ 
523 & s080908 & 0.61912 & 14.9$\pm$0.0 & 43.30$\pm$3.30 & Danforth$^{1038}$ \\ 
524 & s080908 & 0.65652 & 16.5$\pm$0.3 & 28.83$\pm$3.17 & Danforth$^{M}$ \\ 
525 & s080908 & 0.65727 & 14.4$\pm$0.2 & 13.30$\pm$3.10 & Danforth$^{1032}$ \\ 
526 & s080908 & 0.65745 & 14.2$\pm$0.1 & 23.90$\pm$6.10 & Danforth$^{1038}$ \\ 
527 & s080908 & 0.65761 & 16.4$\pm$9.6 & 6.50$\pm$13.70 & Danforth$^{1038}$ \\ 
\hline
528 & s09255b & 0.29645 & 14.5$\pm$0.0 & 34.17$\pm$2.73 & Danforth$^{M}$ \\ 
529 & s09255b & 0.30927 & 13.7$\pm$0.2 & 29.53$\pm$11.47 & Danforth$^{M}$ \\ 
\hline
530 & s092909 & 0.14489 & 13.9$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
531 & s092909 & 0.16671 & 14.2$\pm$0.1 & 49.83$\pm$7.47 & Danforth$^{M}$ \\ 
\hline
532 & s094952 & 0.16442 & 13.6$\pm$0.1 & 26.60$\pm$12.20 & Danforth$^{1032}$ \\ 
533 & s094952 & 0.35167 & 14.0$\pm$0.1 & 40.20$\pm$8.47 & Danforth$^{M}$ \\ 
534 & s094952 & 0.36551 & 14.3$\pm$0.1 & 41.07$\pm$6.13 & Danforth$^{M}$ \\ 
535 & s094952 & 0.36580 & 14.0$\pm$0.1 & 43.60$\pm$11.40 & Danforth$^{M}$ \\ 
\hline
536 & s135712 & 0.09753 & 14.5$\pm$0.1 & 61.20$\pm$13.50 & Danforth$^{1038}$ \\ 
537 & s135712 & 0.14701 & 14.5$\pm$0.0 & 65.90$\pm$3.60 & Danforth$^{1032}$ \\ 
\hline
538 & s50716 & 0.23145 & 13.8$\pm$0.0 & 14.00$\pm$2.03 & Danforth$^{M}$ \\ 
\hline
539 & sbs1108 & 0.16559 & 14.2$\pm$0.0 & 23.20$\pm$1.40 & Danforth$^{1032}$ \\ 
540 & sbs1108 & 0.32014 & 13.7$\pm$0.1 & 12.60$\pm$4.30 & Danforth$^{1032}$ \\ 
541 & sbs1108 & 0.33424 & 13.7$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
542 & sbs1108 & 0.33522 & 13.9$\pm$0.1 & 49.00$\pm$9.47 & Danforth$^{M}$ \\ 
543 & sbs1108 & 0.34523 & 13.8$\pm$0.1 & 23.97$\pm$4.70 & Danforth$^{M}$ \\ 
544 & sbs1108 & 0.43579 & 13.8$\pm$0.1 & 17.00$\pm$4.63 & Danforth$^{M}$ \\ 
545 & sbs1108 & 0.46320 & 13.8$\pm$0.2 & 45.80$\pm$13.80 & Danforth$^{M}$ \\ 
546 & sbs1108 & 0.46846 & 13.8$\pm$0.1 & 22.93$\pm$6.17 & Danforth$^{M}$ \\ 
547 & sbs1108 & 0.48712 & 13.8$\pm$0.1 & 27.17$\pm$4.63 & Danforth$^{M}$ \\ 
548 & sbs1108 & 0.61764 & 13.7$\pm$0.1 & 22.80$\pm$8.20 & Danforth$^{1032}$ \\ 
\hline
549 & sbs1122 & 0.15545 & 14.1$\pm$0.1 & 44.30$\pm$7.17 & Danforth$^{M}$ \\ 
550 & sbs1122 & 0.19439 & 13.9$\pm$0.1 & 27.40$\pm$7.17 & Danforth$^{M}$ \\ 
551 & sbs1122 & 0.21209 & 14.0$\pm$0.1 & 29.80$\pm$8.00 & Danforth$^{1032}$ \\ 
552 & sbs1122 & 0.25712 & 14.5$\pm$0.0 & 29.10$\pm$2.70 & Danforth$^{1032}$ \\ 
553 & sbs1122 & 0.31236 & 14.4$\pm$0.0 & 32.87$\pm$4.33 & Danforth$^{M}$ \\ 
554 & sbs1122 & 0.31274 & 14.0$\pm$0.1 & 25.33$\pm$6.07 & Danforth$^{M}$ \\ 
555 & sbs1122 & 0.42009 & 13.9$\pm$0.1 & 28.70$\pm$4.70 & Danforth$^{1032}$ \\ 
556 & sbs1122 & 0.57049 & 13.9$\pm$0.1 & 24.40$\pm$6.50 & Danforth$^{M}$ \\ 
\hline
557 & ton236 & 0.19452 & 14.1$\pm$0.1 & 69.13$\pm$4.07 & Danforth$^{M}$ \\ 
558 & ton236 & 0.21887 & 13.9$\pm$0.1 & 67.30$\pm$12.70 & Danforth$^{1032}$ \\ 
559 & ton236 & 0.21919 & 13.8$\pm$0.3 & 38.90$\pm$14.20 & Danforth$^{1038}$ \\ 
560 & ton236 & 0.25876 & 13.7$\pm$0.1 & 5.00$\pm$0.00 & Danforth$^{1032}$ \\ 
561 & ton236 & 0.25896 & 13.6$\pm$0.1 & 7.30$\pm$5.50 & Danforth$^{1032}$ \\ 
562 & ton236 & 0.39942 & 13.8$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
563 & ton236 & 0.43738 & 14.3$\pm$0.0 & 33.13$\pm$2.40 & Danforth$^{M}$ \\ 
564 & ton236 & 0.44804 & 13.2$\pm$0.1 & 16.60$\pm$7.80 & Danforth$^{1032}$ \\ 
\hline
565 & ton28 & 0.13746 & 14.2$\pm$0.3 & 18.20$\pm$7.90 & Tilton \\ 
566 & ton28 & 0.13781 & 13.8$\pm$0.2 & 13.60$\pm$7.50 & Tilton \\ 
567 & ton28 & 0.17251 & 13.7$\pm$0.1 & 26.00$\pm$8.00 & Tilton \\ 
568 & ton28 & 0.24292 & 13.2$\pm$0.2 & 11.00$\pm$5.00 & Tilton \\ 
569 & ton28 & 0.24859 & 13.1$\pm$0.2 & 13.00$\pm$5.00 & Tilton \\ 
570 & ton28 & 0.27338 & 13.3$\pm$0.1 & 20.00$\pm$3.70 & Tilton \\ 
571 & ton28 & 0.33021 & 14.2$\pm$0.0 & 9.90$\pm$0.70 & Tilton \\ 
\hline
572 & ton580 & 0.20258 & 13.4$\pm$0.1 & 20.90$\pm$8.30 & Danforth$^{1032}$ \\ 
573 & ton580 & 0.29171 & 13.2$\pm$0.1 & 12.00$\pm$6.40 & Danforth$^{1032}$ \\ 
\hline
574 & tons180 & 0.02340 & 13.5$\pm$0.1 & 30.00$\pm$0.00 & Tilton \\ 
575 & tons180 & 0.04360 & 13.4$\pm$0.0 & 40.00$\pm$0.00 & Tilton \\ 
576 & tons180 & 0.04560 & 13.7$\pm$0.1 & 33.30$\pm$0.00 & Tilton \\ 
\hline



\caption[\ovi\ Prior Detections]{A '$^M$' indicates that there was an OVI 1032 and 1038 doublet present. These 1032 and 1038 doublet values were averaged into one value on a weighted system of 2:1 respectively. A '*' indicates a duplicate redshift in both Danforth and Tilton. The corresponding Tilton duplicates are omitted from the table}
\end{longtable}

==> Omegas-ALL.tex <==
XMM OVII/OVI & 4.51 & 8.11 & 17.79 &  $\leq$ 7.94  \\
Chandra OVII/OVI & 4.00 & 2.53 & 16.87 &  $\leq$ 3.11  \\
XMM OVIII/OVI & 4.50 & 8.01 & 17.58 &  $\leq$ 49.95  \\
Chandra OVIII/OVI & 4.00 & 2.56 & 16.86 &  $\leq$ 29.50  \\
XMM OVII/HI & 4.52 & 8.36 & 16.63 &  $\leq$ 0.52  \\
Chandra OVII/HI & 4.00 & 2.52 & 16.12 &  $\leq$ 0.55  \\
XMM OVIII/HI & 4.53 & 8.41 & 16.65 &  $\leq$ 5.55  \\
Chandra OVIII/HI & 4.01 & 2.56 & 16.17 &  $\leq$ 6.12  \\


==> Tables/Chandra/Latex/chandra_o7_hi_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\footnotesize
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllll|l}
\caption[\chandra\ Data, \ovii\ With \hi\ Priors Results (Full)]{\ovii\ measurements with \chandra\ data, at the prior redshift from the \hi\ lines from Table~\ref{tab:hiPriorsTable}.}
\label{tab:chandrahiovii}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & \multicolumn{2}{c}{RGS1} & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \% $\frac{B}{D+B}$ & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.13714$ (\#1)  & 35.38(39) & 148933 & 24 & 1831$\pm^{ 64 }_{ 63 }$ & $1$ & 24.5622 & $ 1.34\pm^{ 2.73 }_{ 1.32 }$ & $ 15.58\pm^{ 0.28 }_{ 1.74 }$ & 1.14\\ 
1es1028 & $0.20383$ (\#2)  & 38.65(38) & 148933 & 24 & 1963$\pm^{ 69 }_{ 68 }$ & $1$ & 26.0027 & $ 1.18\pm^{ 2.92 }_{ 1.29 }$ & $ 15.52\pm^{ 0.31 }_{ nan }$ & 0.87\\ 
1es1028 & $0.22121$ (\#3)  & 35.87(38) & 148933 & 23 & 2058$\pm^{ 71 }_{ 70 }$ & $1$ & 26.3781 & $ 0.80\pm^{ 2.27 }_{ 1.13 }$ & $ 15.39\pm^{ 0.38 }_{ nan }$ & 0.48\\ 
1es1553 & $0.03466$ (\#4)  & 38.20(38) & 495645 & 25 & 2408$\pm^{ 40 }_{ 39 }$ & $1$ & 22.3487 & $ -0.03\pm^{ 0.50 }_{ 0.43 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
1es1553 & $0.04273$ (\#5)  & 54.53(38) & 495645 & 25 & 2461$\pm^{ 41 }_{ 41 }$ & $1$ & 22.5230 & $ 0.31\pm^{ 0.61 }_{ 0.49 }$ & $ 15.03\pm^{ 0.41 }_{ nan }$ & 0.42\\ 
1es1553 & $0.06364$ (\#6)  & 48.63(38) & 495645 & 24 & 2557$\pm^{ 43 }_{ 42 }$ & $1$ & 22.9746 & $ -1.05\pm^{ 0.36 }_{ 0.32 }$ & $ nan\pm^{ nan }_{ nan }$ & 7.56\\ 
1es1553 & $0.21869$ (\#7)  & 44.59(38) & 495645 & 23 & 3121$\pm^{ 49 }_{ 48 }$ & $1$ & 26.3237 & $ -0.47\pm^{ 0.39 }_{ 0.35 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.52\\ 
3c273 & $0.00758$ (\#8)  & 31.25(31) & 69608 & 8 & 5771$\pm^{ 159 }_{ 155 }$ & $1$ & 21.7637 & $ 0.01\pm^{ 0.82 }_{ 0.62 }$ & $ 13.58\pm^{ 1.83 }_{ nan }$ & 0.00\\ 
3c273 & $0.06707$ (\#9)  & 47.38(38) & 69608 & 9 & 6182$\pm^{ 155 }_{ 152 }$ & $1$ & 23.0487 & $ -0.98\pm^{ 0.55 }_{ 0.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.03\\ 
3c273 & $0.07359$ (\#10)  & 46.82(39) & 69608 & 8 & 6324$\pm^{ 156 }_{ 154 }$ & $1$ & 23.1895 & $ 2.44\pm^{ 3.08 }_{ 1.40 }$ & $ 15.74\pm^{ 0.15 }_{ 0.25 }$ & 5.26\\ 
3c273 & $0.13960$ (\#11)  & 35.63(39) & 69608 & 7 & 7537$\pm^{ 171 }_{ 168 }$ & $1$ & 24.6154 & $ 0.62\pm^{ 1.06 }_{ 0.73 }$ & $ 15.29\pm^{ 0.33 }_{ nan }$ & 0.77\\ 
h1821 & $0.00944$ (\#12)  & 21.13(18) & 470152 & 2 & 900$\pm^{ 29 }_{ 28 }$ & $1$ & 21.8039 & $ -0.36\pm^{ 0.52 }_{ 0.42 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.63\\ 
h1821 & $0.06779$ (\#13)  & 35.37(36) & 470152 & 2 & 970$\pm^{ 23 }_{ 22 }$ & $1$ & 23.0643 & $ -0.12\pm^{ 0.68 }_{ 0.56 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
h1821 & $0.08483$ (\#14)  & 41.18(32) & 470152 & 2 & 1048$\pm^{ 24 }_{ 23 }$ & $1$ & 23.4323 & $ -0.01\pm^{ 0.53 }_{ 0.42 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
h1821 & $0.12147$ (\#15)  & 46.13(38) & 470152 & 1 & 1203$\pm^{ 22 }_{ 22 }$ & $1$ & 24.2238 & $ 0.32\pm^{ 0.57 }_{ 0.49 }$ & $ 15.04\pm^{ 0.39 }_{ nan }$ & 0.44\\ 
h1821 & $0.19817$ (\#16)  & 30.74(38) & 470152 & 2 & 1134$\pm^{ 25 }_{ 25 }$ & $1$ & 25.8805 & $ 2.58\pm^{ 2.94 }_{ 1.42 }$ & $ 15.70\pm^{ 0.13 }_{ 0.21 }$ & 6.87\\ 
h1821 & $0.21321$ (\#17)  & 33.49(38) & 470152 & 2 & 1090$\pm^{ 25 }_{ 25 }$ & $1$ & 26.2053 & $ -0.81\pm^{ 0.40 }_{ 0.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.57\\ 
h1821 & $0.24531$ (\#18)  & 28.82(38) & 470152 & 2 & 1103$\pm^{ 27 }_{ 27 }$ & $1$ & 26.8987 & $ 1.09\pm^{ 1.14 }_{ 0.81 }$ & $ 15.51\pm^{ 0.22 }_{ 0.52 }$ & 2.16\\ 
h2356 & $0.03830$ (\#19)  & 36.54(38) & 586697 & 29 & 2132$\pm^{ 35 }_{ 35 }$ & $1$ & 22.4273 & $ -0.09\pm^{ 0.48 }_{ 0.42 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.06\\ 
h2356 & $0.07881$ (\#20)  & 54.01(38) & 586697 & 30 & 2125$\pm^{ 35 }_{ 35 }$ & $1$ & 23.3023 & $ -0.02\pm^{ 0.44 }_{ 0.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
h2356 & $0.10467$ (\#21)  & 36.31(39) & 586697 & 29 & 2213$\pm^{ 37 }_{ 36 }$ & $1$ & 23.8609 & $ -0.54\pm^{ 0.41 }_{ 0.35 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.85\\ 
h2356 & $0.15613$ (\#22)  & 33.28(38) & 586697 & 29 & 2378$\pm^{ 39 }_{ 39 }$ & $1$ & 24.9724 & $ -0.08\pm^{ 0.50 }_{ 0.41 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
mr2251 & $0.01068$ (\#23)  & 33.00(30) & 78434 & 15 & 3031$\pm^{ 114 }_{ 110 }$ & $1$ & 21.8307 & $ 0.05\pm^{ 1.37 }_{ 0.78 }$ & $ 14.25\pm^{ 1.29 }_{ nan }$ & 0.00\\ 
mr2251 & $0.01449$ (\#24)  & 29.99(31) & 78434 & 15 & 3080$\pm^{ 115 }_{ 112 }$ & $1$ & 21.9130 & $ -0.44\pm^{ 0.93 }_{ 0.71 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.30\\ 
mr2251 & $0.06131$ (\#25)  & 45.89(38) & 78434 & 16 & 3079$\pm^{ 107 }_{ 105 }$ & $1$ & 22.9243 & $ -0.40\pm^{ 1.04 }_{ 0.77 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.20\\ 
mr2251 & $0.06190$ (\#26)  & 47.80(39) & 78434 & 16 & 3092$\pm^{ 108 }_{ 106 }$ & $1$ & 22.9370 & $ 0.36\pm^{ 1.54 }_{ 1.00 }$ & $ 15.09\pm^{ 0.59 }_{ nan }$ & 0.11\\ 
mr2251 & $0.06276$ (\#27)  & 43.10(38) & 78434 & 17 & 3142$\pm^{ 109 }_{ 106 }$ & $1$ & 22.9556 & $ 4.57\pm^{ 12.54 }_{ 3.52 }$ & $ 15.80\pm^{ 0.19 }_{ 0.34 }$ & 3.42\\ 
mr2251 & $0.06327$ (\#28)  & 50.52(39) & 78434 & 16 & 3223$\pm^{ 118 }_{ 110 }$ & $1$ & 22.9666 & $ 14.07\pm^{ 1.71E+03 }_{ 11.29 }$ & $ 15.96\pm^{ 0.16 }_{ 0.23 }$ & 6.82\\ 
mr2251 & $0.06381$ (\#29)  & 48.05(38) & 78434 & 16 & 3234$\pm^{ 109 }_{ 107 }$ & $1$ & 22.9783 & $ 16.70\pm^{ 89.76 }_{ 13.12 }$ & $ 15.97\pm^{ 0.11 }_{ 0.18 }$ & 7.99\\ 
mrk478 & $0.06166$ (\#30)  & 28.21(39) & 80466 & 23 & 1423$\pm^{ 75 }_{ 73 }$ & $1$ & 22.9319 & $ -1.81\pm^{ 0.63 }_{ 0.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 5.15\\ 
mrk478 & $0.06578$ (\#31)  & 39.37(38) & 80466 & 23 & 1469$\pm^{ 76 }_{ 74 }$ & $1$ & 23.0208 & $ -1.02\pm^{ 1.08 }_{ 0.70 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.01\\ 
mrk478 & $0.07213$ (\#32)  & 37.11(39) & 80466 & 22 & 1556$\pm^{ 77 }_{ 75 }$ & $1$ & 23.1580 & $ 11.51\pm^{ 56.54 }_{ 9.70 }$ & $ 15.94\pm^{ 0.15 }_{ 0.32 }$ & 3.39\\ 
pg1116 & $0.04114$ (\#33)  & 35.29(39) & 355485 & 53 & 772$\pm^{ 36 }_{ 35 }$ & $1$ & 22.4886 & $ -0.16\pm^{ 1.61 }_{ 0.98 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
pg1116 & $0.06251$ (\#34)  & 38.29(38) & 355485 & 54 & 760$\pm^{ 36 }_{ 36 }$ & $1$ & 22.9502 & $ -0.65\pm^{ 1.45 }_{ 0.94 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.30\\ 
pg1116 & $0.08382$ (\#35)  & 35.87(39) & 355485 & 54 & 756$\pm^{ 36 }_{ 35 }$ & $1$ & 23.4105 & $ 1.23\pm^{ 4.23 }_{ 1.53 }$ & $ 15.54\pm^{ 0.34 }_{ nan }$ & 0.61\\ 
pg1116 & $0.09210$ (\#36)  & 43.67(38) & 355485 & 54 & 772$\pm^{ 36 }_{ 36 }$ & $1$ & 23.5894 & $ 3.27\pm^{ 159.72 }_{ 2.74 }$ & $ 15.80\pm^{ 0.26 }_{ 0.57 }$ & 2.02\\ 
pg1116 & $0.09281$ (\#37)  & 35.22(37) & 355485 & 54 & 759$\pm^{ 37 }_{ 36 }$ & $1$ & 23.6047 & $ 4.29\pm^{ 26.23 }_{ 3.78 }$ & $ 15.80\pm^{ 0.24 }_{ 0.59 }$ & 1.92\\ 
pg1116 & $0.13373$ (\#38)  & 41.71(34) & 355485 & 49 & 1001$\pm^{ 43 }_{ 41 }$ & $1$ & 24.4886 & $ 20.93\pm^{ 519.78 }_{ 18.48 }$ & $ 15.96\pm^{ 0.17 }_{ 0.21 }$ & 6.99\\ 
pg1116 & $0.13851$ (\#39)  & 47.35(34) & 355485 & 49 & 947$\pm^{ 42 }_{ 41 }$ & $1$ & 24.5918 & $ -1.45\pm^{ 0.60 }_{ 0.46 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.33\\ 
pg1211 & $0.02586$ (\#40)  & 27.92(37) & 133595 & 1 & 1286$\pm^{ 58 }_{ 56 }$ & $1$ & 22.1586 & $ -1.38\pm^{ 0.66 }_{ 0.51 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.58\\ 
pg1211 & $0.05443$ (\#41)  & 46.97(38) & 133595 & 1 & 1522$\pm^{ 67 }_{ 66 }$ & $1$ & 22.7757 & $ 2.08\pm^{ 7.09 }_{ 1.80 }$ & $ 15.71\pm^{ 0.23 }_{ 0.72 }$ & 1.60\\ 
pks0405 & $0.02510$ (\#42)  & 29.08(36) & 376096 & 68 & 481$\pm^{ 35 }_{ 34 }$ & $1$ & 22.1422 & $ -0.35\pm^{ 3.48 }_{ 1.14 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
pks0405 & $0.05902$ (\#43)  & 38.62(38) & 376096 & 68 & 512$\pm^{ 36 }_{ 35 }$ & $1$ & 22.8748 & $ -1.07\pm^{ 1.88 }_{ 1.11 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.47\\ 
pks0405 & $0.09719$ (\#44)  & 40.81(38) & 376096 & 67 & 550$\pm^{ 36 }_{ 36 }$ & $1$ & 23.6993 & $ 3.12E+03\pm^{ 2.80E+08 }_{ 3.10E+03 }$ & $ 16.23\pm^{ 0.09 }_{ 0.28 }$ & 6.32\\ 
pks0405 & $0.10152$ (\#45)  & 37.76(39) & 376096 & 68 & 505$\pm^{ 36 }_{ 35 }$ & $1$ & 23.7928 & $ -1.12\pm^{ 1.48 }_{ 0.79 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.76\\ 
pks0405 & $0.10298$ (\#46)  & 38.10(38) & 376096 & 68 & 505$\pm^{ 36 }_{ 35 }$ & $1$ & 23.8244 & $ -1.31\pm^{ 1.57 }_{ 0.99 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.84\\ 
pks0405 & $0.19456$ (\#47)  & 25.03(38) & 376096 & 69 & 528$\pm^{ 39 }_{ 38 }$ & $1$ & 25.8025 & $ -1.54\pm^{ 1.28 }_{ 0.82 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.43\\ 
pks0405 & $0.21976$ (\#48)  & 38.16(38) & 376096 & 70 & 555$\pm^{ 41 }_{ 40 }$ & $1$ & 26.3468 & $ 0.83\pm^{ 29.27 }_{ 1.99 }$ & $ 15.39\pm^{ 0.61 }_{ nan }$ & 0.10\\ 
pks0405 & $0.24564$ (\#49)  & 44.65(38) & 376096 & 68 & 596$\pm^{ 42 }_{ 41 }$ & $1$ & 26.9058 & $ -1.04\pm^{ 1.62 }_{ 0.81 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.61\\ 
pks0405 & $0.29748$ (\#50)  & 35.20(38) & 376096 & 69 & 612$\pm^{ 45 }_{ 44 }$ & $1$ & 28.0256 & $ -0.97\pm^{ 2.04 }_{ 1.15 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.36\\ 
pks0405 & $0.31016$ (\#51)  & 42.41(38) & 376096 & 72 & 565$\pm^{ 45 }_{ 44 }$ & $1$ & 28.2995 & $ 1.34\pm^{ 340.45 }_{ 2.33 }$ & $ 15.58\pm^{ 0.50 }_{ nan }$ & 0.24\\ 
pks0405 & $0.32502$ (\#52)  & 32.33(38) & 376096 & 74 & 548$\pm^{ 50 }_{ 44 }$ & $1$ & 28.6204 & $ 237.19\pm^{ 4.49E+10 }_{ 217.51 }$ & $ 16.12\pm^{ 0.23 }_{ 0.11 }$ & 3.20\\ 
pks0405 & $0.49508$ (\#53)  & 37.52(38) & 376096 & 78 & 489$\pm^{ 56 }_{ 55 }$ & $1$ & 32.2937 & $ -1.99\pm^{ 1.32 }_{ 0.74 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.80\\ 
pks2155 & $0.05708$ (\#54)  & 13.67(23) & 319334 & 4 & 16704$\pm^{ 152 }_{ 151 }$ & $1$ & 22.8329 & $ 0.50\pm^{ 0.28 }_{ 0.25 }$ & $ 15.20\pm^{ 0.16 }_{ 0.27 }$ & 5.40\\ 
pks2155 & $0.06236$ (\#55)  & 30.32(25) & 319334 & 5 & 16439$\pm^{ 143 }_{ 142 }$ & $1$ & 22.9470 & $ -0.38\pm^{ 0.19 }_{ 0.17 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.35\\ 
pks2155 & $0.10586$ (\#56)  & 38.15(34) & 319334 & 4 & 18205$\pm^{ 129 }_{ 129 }$ & $1$ & 23.8866 & $ -0.12\pm^{ 0.19 }_{ 0.18 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.52\\ 
tons180 & $0.04304$ (\#57)  & 28.54(38) & 76753 & 2 & 1841$\pm^{ 117 }_{ 112 }$ & $1$ & 22.5297 & $ -0.54\pm^{ 1.43 }_{ 0.84 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.24\\


\hline
\hline
 \end{longtable}
 \end{landscape}

==> Tables/Chandra/Latex/chandra_o7_hi_uppers_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\footnotesize
\begin{landscape}
\begin{longtable}{cc|lllllll|l}
\caption[\chandra\ Data, \ovii\ Upper Limits With \hi\ Priors Results (Full)]{\ovii\ upper limit measurements with \chandra\ data, at the prior redshift from the \hi\ lines from Table~\ref{tab:hiPriorsTable}.}
\label{tab:chandrahioviiuppers}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & RGS1 & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N + (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.13714$ (\#1)  & 35.38(39) & 148933 & 1831$\pm^{ 64 }_{ 63 }$ & $1$ & 24.5622 & 2.02 & 15.70 & 1.14\\ 
1es1028 & $0.20383$ (\#2)  & 38.65(38) & 148933 & 1963$\pm^{ 69 }_{ 68 }$ & $1$ & 26.0027 & 2.11 & 15.69 & 0.87\\ 
1es1028 & $0.22121$ (\#3)  & 35.87(38) & 148933 & 2058$\pm^{ 71 }_{ 70 }$ & $1$ & 26.3781 & 1.70 & 15.62 & 0.48\\ 
1es1553 & $0.03466$ (\#4)  & 38.20(38) & 495645 & 2408$\pm^{ 40 }_{ 39 }$ & $1$ & 22.3487 & 0.47 & 15.19 & 0.00\\ 
1es1553 & $0.04273$ (\#5)  & 54.53(38) & 495645 & 2461$\pm^{ 41 }_{ 41 }$ & $1$ & 22.5230 & 0.55 & 15.25 & 0.42\\ 
1es1553 & $0.06364$ (\#6)  & 48.63(38) & 495645 & 2557$\pm^{ 43 }_{ 42 }$ & $1$ & 22.9746 & 0.34 & 15.07 & 7.56\\ 
1es1553 & $0.21869$ (\#7)  & 44.59(38) & 495645 & 3121$\pm^{ 49 }_{ 48 }$ & $1$ & 26.3237 & 0.37 & 15.10 & 1.52\\ 
3c273 & $0.00758$ (\#8)  & 31.25(31) & 69608 & 5771$\pm^{ 159 }_{ 155 }$ & $1$ & 21.7637 & 0.72 & 15.36 & 0.00\\ 
3c273 & $0.06707$ (\#9)  & 47.38(38) & 69608 & 6182$\pm^{ 155 }_{ 152 }$ & $1$ & 23.0487 & 0.51 & 15.23 & 3.03\\ 
3c273 & $0.07359$ (\#10)  & 46.82(39) & 69608 & 6324$\pm^{ 156 }_{ 154 }$ & $1$ & 23.1895 & 2.24 & 15.72 & 5.26\\ 
3c273 & $0.13960$ (\#11)  & 35.63(39) & 69608 & 7537$\pm^{ 171 }_{ 168 }$ & $1$ & 24.6154 & 0.89 & 15.43 & 0.77\\ 
h1821 & $0.00944$ (\#12)  & 21.13(18) & 470152 & 900$\pm^{ 29 }_{ 28 }$ & $1$ & 21.8039 & 0.47 & 15.18 & 0.63\\ 
h1821 & $0.06779$ (\#13)  & 35.37(36) & 470152 & 970$\pm^{ 23 }_{ 22 }$ & $1$ & 23.0643 & 0.62 & 15.30 & 0.04\\ 
h1821 & $0.08483$ (\#14)  & 41.18(32) & 470152 & 1048$\pm^{ 24 }_{ 23 }$ & $1$ & 23.4323 & 0.48 & 15.18 & 0.00\\ 
h1821 & $0.12147$ (\#15)  & 46.13(38) & 470152 & 1203$\pm^{ 22 }_{ 22 }$ & $1$ & 24.2238 & 0.53 & 15.24 & 0.44\\ 
h1821 & $0.19817$ (\#16)  & 30.74(38) & 470152 & 1134$\pm^{ 25 }_{ 25 }$ & $1$ & 25.8805 & 2.18 & 15.66 & 6.87\\ 
h1821 & $0.21321$ (\#17)  & 33.49(38) & 470152 & 1090$\pm^{ 25 }_{ 25 }$ & $1$ & 26.2053 & 0.37 & 15.09 & 3.57\\ 
h1821 & $0.24531$ (\#18)  & 28.82(38) & 470152 & 1103$\pm^{ 27 }_{ 27 }$ & $1$ & 26.8987 & 0.97 & 15.47 & 2.16\\ 
h2356 & $0.03830$ (\#19)  & 36.54(38) & 586697 & 2132$\pm^{ 35 }_{ 35 }$ & $1$ & 22.4273 & 0.45 & 15.18 & 0.06\\ 
h2356 & $0.07881$ (\#20)  & 54.01(38) & 586697 & 2125$\pm^{ 35 }_{ 35 }$ & $1$ & 23.3023 & 0.46 & 15.19 & 0.01\\ 
h2356 & $0.10467$ (\#21)  & 36.31(39) & 586697 & 2213$\pm^{ 37 }_{ 36 }$ & $1$ & 23.8609 & 0.38 & 15.11 & 1.85\\ 
h2356 & $0.15613$ (\#22)  & 33.28(38) & 586697 & 2378$\pm^{ 39 }_{ 39 }$ & $1$ & 24.9724 & 0.45 & 15.18 & 0.03\\ 
mr2251 & $0.01068$ (\#23)  & 33.00(30) & 78434 & 3031$\pm^{ 114 }_{ 110 }$ & $1$ & 21.8307 & 1.08 & 15.47 & 0.00\\ 
mr2251 & $0.01449$ (\#24)  & 29.99(31) & 78434 & 3080$\pm^{ 115 }_{ 112 }$ & $1$ & 21.9130 & 0.82 & 15.41 & 0.30\\ 
mr2251 & $0.06131$ (\#25)  & 45.89(38) & 78434 & 3079$\pm^{ 107 }_{ 105 }$ & $1$ & 22.9243 & 0.90 & 15.44 & 0.20\\ 
mr2251 & $0.06190$ (\#26)  & 47.80(39) & 78434 & 3092$\pm^{ 108 }_{ 106 }$ & $1$ & 22.9370 & 1.27 & 15.56 & 0.11\\ 
mr2251 & $0.06276$ (\#27)  & 43.10(38) & 78434 & 3142$\pm^{ 109 }_{ 106 }$ & $1$ & 22.9556 & 8.03 & 15.89 & 3.42\\ 
mr2251 & $0.06327$ (\#28)  & 50.52(39) & 78434 & 3223$\pm^{ 118 }_{ 110 }$ & $1$ & 22.9666 & 861.22 & 16.12 & 6.82\\ 
mr2251 & $0.06381$ (\#29)  & 48.05(38) & 78434 & 3234$\pm^{ 109 }_{ 107 }$ & $1$ & 22.9783 & 51.44 & 16.03 & 7.99\\ 
mrk478 & $0.06166$ (\#30)  & 28.21(39) & 80466 & 1423$\pm^{ 75 }_{ 73 }$ & $1$ & 22.9319 & 0.55 & 15.24 & 5.15\\ 
mrk478 & $0.06578$ (\#31)  & 39.37(38) & 80466 & 1469$\pm^{ 76 }_{ 74 }$ & $1$ & 23.0208 & 0.89 & 15.41 & 1.01\\ 
mrk478 & $0.07213$ (\#32)  & 37.11(39) & 80466 & 1556$\pm^{ 77 }_{ 75 }$ & $1$ & 23.1580 & 33.12 & 16.05 & 3.39\\ 
pg1116 & $0.04114$ (\#33)  & 35.29(39) & 355485 & 772$\pm^{ 36 }_{ 35 }$ & $1$ & 22.4886 & 1.30 & 15.57 & 0.02\\ 
pg1116 & $0.06251$ (\#34)  & 38.29(38) & 355485 & 760$\pm^{ 36 }_{ 36 }$ & $1$ & 22.9502 & 1.20 & 15.54 & 0.30\\ 
pg1116 & $0.08382$ (\#35)  & 35.87(39) & 355485 & 756$\pm^{ 36 }_{ 35 }$ & $1$ & 23.4105 & 2.88 & 15.77 & 0.61\\ 
pg1116 & $0.09210$ (\#36)  & 43.67(38) & 355485 & 772$\pm^{ 36 }_{ 36 }$ & $1$ & 23.5894 & 81.23 & 16.01 & 2.02\\ 
pg1116 & $0.09281$ (\#37)  & 35.22(37) & 355485 & 759$\pm^{ 37 }_{ 36 }$ & $1$ & 23.6047 & 15.00 & 15.97 & 1.92\\ 
pg1116 & $0.13373$ (\#38)  & 41.71(34) & 355485 & 1001$\pm^{ 43 }_{ 41 }$ & $1$ & 24.4886 & 269.13 & 16.07 & 6.99\\ 
pg1116 & $0.13851$ (\#39)  & 47.35(34) & 355485 & 947$\pm^{ 42 }_{ 41 }$ & $1$ & 24.5918 & 0.53 & 15.23 & 4.33\\ 
pg1211 & $0.02586$ (\#40)  & 27.92(37) & 133595 & 1286$\pm^{ 58 }_{ 56 }$ & $1$ & 22.1586 & 0.59 & 15.27 & 3.58\\ 
pg1211 & $0.05443$ (\#41)  & 46.97(38) & 133595 & 1522$\pm^{ 67 }_{ 66 }$ & $1$ & 22.7757 & 4.45 & 15.87 & 1.60\\ 
pks0405 & $0.02510$ (\#42)  & 29.08(36) & 376096 & 481$\pm^{ 35 }_{ 34 }$ & $1$ & 22.1422 & 2.31 & 15.68 & 0.04\\ 
pks0405 & $0.05902$ (\#43)  & 38.62(38) & 376096 & 512$\pm^{ 36 }_{ 35 }$ & $1$ & 22.8748 & 1.49 & 15.61 & 0.47\\ 
pks0405 & $0.09719$ (\#44)  & 40.81(38) & 376096 & 550$\pm^{ 36 }_{ 36 }$ & $1$ & 23.6993 & 1.40E+08 & 16.30 & 6.32\\ 
pks0405 & $0.10152$ (\#45)  & 37.76(39) & 376096 & 505$\pm^{ 36 }_{ 35 }$ & $1$ & 23.7928 & 1.14 & 15.48 & 0.76\\ 
pks0405 & $0.10298$ (\#46)  & 38.10(38) & 376096 & 505$\pm^{ 36 }_{ 35 }$ & $1$ & 23.8244 & 1.28 & 15.56 & 0.84\\ 
pks0405 & $0.19456$ (\#47)  & 25.03(38) & 376096 & 528$\pm^{ 39 }_{ 38 }$ & $1$ & 25.8025 & 1.05 & 15.48 & 1.43\\ 
pks0405 & $0.21976$ (\#48)  & 38.16(38) & 376096 & 555$\pm^{ 41 }_{ 40 }$ & $1$ & 26.3468 & 15.63 & 15.97 & 0.10\\ 
pks0405 & $0.24564$ (\#49)  & 44.65(38) & 376096 & 596$\pm^{ 42 }_{ 41 }$ & $1$ & 26.9058 & 1.22 & 15.50 & 0.61\\ 
pks0405 & $0.29748$ (\#50)  & 35.20(38) & 376096 & 612$\pm^{ 45 }_{ 44 }$ & $1$ & 28.0256 & 1.59 & 15.63 & 0.36\\ 
pks0405 & $0.31016$ (\#51)  & 42.41(38) & 376096 & 565$\pm^{ 45 }_{ 44 }$ & $1$ & 28.2995 & 171.39 & 16.03 & 0.24\\ 
pks0405 & $0.32502$ (\#52)  & 32.33(38) & 376096 & 548$\pm^{ 50 }_{ 44 }$ & $1$ & 28.6204 & 2.24E+10 & 16.34 & 3.20\\ 
pks0405 & $0.49508$ (\#53)  & 37.52(38) & 376096 & 489$\pm^{ 56 }_{ 55 }$ & $1$ & 32.2937 & 1.03 & 15.45 & 1.80\\ 
pks2155 & $0.05708$ (\#54)  & 13.67(23) & 319334 & 16704$\pm^{ 152 }_{ 151 }$ & $1$ & 22.8329 & 0.26 & 14.96 & 5.40\\ 
pks2155 & $0.06236$ (\#55)  & 30.32(25) & 319334 & 16439$\pm^{ 143 }_{ 142 }$ & $1$ & 22.9470 & 0.18 & 14.80 & 4.35\\ 
pks2155 & $0.10586$ (\#56)  & 38.15(34) & 319334 & 18205$\pm^{ 129 }_{ 129 }$ & $1$ & 23.8866 & 0.18 & 14.81 & 0.52\\ 
tons180 & $0.04304$ (\#57)  & 28.54(38) & 76753 & 1841$\pm^{ 117 }_{ 112 }$ & $1$ & 22.5297 & 1.14 & 15.49 & 0.24\\ 


\hline
\hline
\end{longtable}
\end{landscape}

==> Tables/Chandra/Latex/chandra_o7_o6_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\footnotesize
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllll|l}
\caption[\chandra\ Data, \ovii\ With \ovi\ Priors Results (Full)]{\ovii\ measurements with \chandra\ data, at the prior redshift from the \ovi\ lines from Table~\ref{tab:oviPriorsTable}.}
\label{tab:chandraoviovii}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & \multicolumn{2}{c}{RGS1} & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \% $\frac{B}{D+B}$ & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.12314$ (\#1)  & 32.34(39) & 148933 & 24 & 1757$\pm^{ 63 }_{ 62 }$ & $1$ & 24.2598 & $ -0.56\pm^{ 0.97 }_{ 0.68 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.44\\ 
1es1028 & $0.13706$ (\#2)  & 35.52(39) & 148933 & 24 & 1830$\pm^{ 64 }_{ 63 }$ & $1$ & 24.5605 & $ 1.29\pm^{ 3.09 }_{ 1.34 }$ & $ 15.56\pm^{ 0.30 }_{ nan }$ & 0.99\\ 
1es1028 & $0.33735$ (\#3)  & 37.26(39) & 148933 & 25 & 2138$\pm^{ 81 }_{ 79 }$ & $1$ & 28.8868 & $ -0.66\pm^{ 0.98 }_{ 0.74 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.56\\ 
1es1553 & $0.18759$ (\#4)  & 44.14(38) & 495645 & 22 & 3135$\pm^{ 48 }_{ 48 }$ & $1$ & 25.6519 & $ 0.34\pm^{ 0.57 }_{ 0.46 }$ & $ 15.06\pm^{ 0.37 }_{ nan }$ & 0.58\\ 
1es1553 & $0.18775$ (\#5)  & 44.13(38) & 495645 & 22 & 3135$\pm^{ 48 }_{ 48 }$ & $1$ & 25.6554 & $ 0.35\pm^{ 0.62 }_{ 0.47 }$ & $ 15.07\pm^{ 0.37 }_{ nan }$ & 0.58\\ 
1es1553 & $0.18984$ (\#6)  & 42.53(38) & 495645 & 22 & 3106$\pm^{ 48 }_{ 48 }$ & $1$ & 25.7005 & $ -0.38\pm^{ 0.40 }_{ 0.36 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.00\\ 
1es1553 & $0.21631$ (\#7)  & 51.98(38) & 495645 & 23 & 3137$\pm^{ 49 }_{ 49 }$ & $1$ & 26.2723 & $ 0.29\pm^{ 0.58 }_{ 0.46 }$ & $ 15.00\pm^{ 0.42 }_{ nan }$ & 0.42\\ 
1es1553 & $0.31130$ (\#8)  & 36.35(38) & 495645 & 25 & 3202$\pm^{ 53 }_{ 54 }$ & $1$ & 28.3241 & $ -0.04\pm^{ 0.53 }_{ 0.44 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
1es1553 & $0.37868$ (\#9)  & 48.60(38) & 495645 & 28 & 3322$\pm^{ 62 }_{ 61 }$ & $1$ & 29.7795 & $ -0.69\pm^{ 0.39 }_{ 0.33 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.89\\ 
1es1553 & $0.39497$ (\#10)  & 39.90(38) & 495645 & 28 & 3374$\pm^{ 65 }_{ 64 }$ & $1$ & 30.1314 & $ -0.48\pm^{ 0.47 }_{ 0.37 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.16\\ 
h1821 & $0.02438$ (\#11)  & 44.15(32) & 470152 & 2 & 888$\pm^{ 22 }_{ 21 }$ & $1$ & 22.1266 & $ 0.33\pm^{ 0.73 }_{ 0.58 }$ & $ 15.05\pm^{ 0.44 }_{ nan }$ & 0.32\\ 
h1821 & $0.10817$ (\#12)  & 50.75(39) & 470152 & 1 & 1103$\pm^{ 21 }_{ 21 }$ & $1$ & 23.9365 & $ -1.08\pm^{ 0.34 }_{ 0.31 }$ & $ nan\pm^{ nan }_{ nan }$ & 8.78\\ 
h1821 & $0.12133$ (\#13)  & 46.33(38) & 470152 & 1 & 1202$\pm^{ 22 }_{ 22 }$ & $1$ & 24.2207 & $ 0.22\pm^{ 0.59 }_{ 0.46 }$ & $ 14.89\pm^{ 0.49 }_{ nan }$ & 0.22\\ 
h1821 & $0.12147$ (\#14)  & 46.13(38) & 470152 & 1 & 1203$\pm^{ 22 }_{ 22 }$ & $1$ & 24.2238 & $ 0.32\pm^{ 0.57 }_{ 0.49 }$ & $ 15.04\pm^{ 0.39 }_{ nan }$ & 0.44\\ 
h1821 & $0.16992$ (\#15)  & 37.35(38) & 470152 & 1 & 1107$\pm^{ 23 }_{ 23 }$ & $1$ & 25.2703 & $ -0.07\pm^{ 0.57 }_{ 0.45 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
h1821 & $0.17043$ (\#16)  & 37.01(38) & 470152 & 1 & 1104$\pm^{ 23 }_{ 23 }$ & $1$ & 25.2813 & $ -0.29\pm^{ 0.50 }_{ 0.40 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.39\\ 
h1821 & $0.21326$ (\#17)  & 33.42(38) & 470152 & 2 & 1090$\pm^{ 25 }_{ 25 }$ & $1$ & 26.2064 & $ -0.81\pm^{ 0.40 }_{ 0.33 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.65\\ 
h1821 & $0.22497$ (\#18)  & 31.24(39) & 470152 & 2 & 1097$\pm^{ 26 }_{ 25 }$ & $1$ & 26.4594 & $ 0.54\pm^{ 0.84 }_{ 0.63 }$ & $ 15.24\pm^{ 0.32 }_{ nan }$ & 0.74\\ 
h1821 & $0.22522$ (\#19)  & 31.59(39) & 470152 & 2 & 1095$\pm^{ 26 }_{ 25 }$ & $1$ & 26.4648 & $ 0.37\pm^{ 0.78 }_{ 0.60 }$ & $ 15.10\pm^{ 0.42 }_{ nan }$ & 0.37\\ 
h1821 & $0.22639$ (\#20)  & 32.44(39) & 470152 & 2 & 1098$\pm^{ 26 }_{ 25 }$ & $1$ & 26.4900 & $ 0.28\pm^{ 0.73 }_{ 0.57 }$ & $ 14.99\pm^{ 0.48 }_{ nan }$ & 0.23\\ 
h1821 & $0.24531$ (\#21)  & 28.82(38) & 470152 & 2 & 1103$\pm^{ 27 }_{ 27 }$ & $1$ & 26.8987 & $ 1.09\pm^{ 1.14 }_{ 0.81 }$ & $ 15.51\pm^{ 0.22 }_{ 0.52 }$ & 2.16\\ 
h1821 & $0.26657$ (\#22)  & 39.22(39) & 470152 & 2 & 1157$\pm^{ 29 }_{ 29 }$ & $1$ & 27.3579 & $ -0.17\pm^{ 0.65 }_{ 0.50 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.09\\ 
h1821 & $0.28800$ (\#23)  & 48.59(33) & 470152 & 1 & 1265$\pm^{ 37 }_{ 37 }$ & $1$ & 27.8208 & $ -0.77\pm^{ 0.52 }_{ 0.42 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.16\\ 
h1821 & $0.29658$ (\#24)  & 45.10(33) & 470152 & 2 & 1326$\pm^{ 41 }_{ 40 }$ & $1$ & 28.0061 & $ -1.47\pm^{ 0.70 }_{ 0.51 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.22\\ 
h1821 & $0.29680$ (\#25)  & 45.72(34) & 470152 & 2 & 1338$\pm^{ 42 }_{ 41 }$ & $1$ & 28.0109 & $ -1.81\pm^{ 0.92 }_{ 0.68 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.92\\ 
h2356 & $0.11461$ (\#26)  & 26.64(38) & 586697 & 29 & 2314$\pm^{ 37 }_{ 37 }$ & $1$ & 24.0756 & $ 1.22\pm^{ 0.88 }_{ 0.64 }$ & $ 15.55\pm^{ 0.16 }_{ 0.27 }$ & 4.89\\ 
h2356 & $0.16512$ (\#27)  & 34.18(39) & 586697 & 29 & 2408$\pm^{ 39 }_{ 39 }$ & $1$ & 25.1666 & $ 1.14\pm^{ 1.03 }_{ 0.70 }$ & $ 15.49\pm^{ 0.18 }_{ 0.33 }$ & 3.76\\ 
mr2251 & $0.01070$ (\#28)  & 33.00(30) & 78434 & 15 & 3031$\pm^{ 114 }_{ 110 }$ & $1$ & 21.8311 & $ 0.03\pm^{ 1.37 }_{ 0.76 }$ & $ 13.99\pm^{ 1.55 }_{ nan }$ & 0.00\\ 
pg1116 & $0.05900$ (\#29)  & 33.16(38) & 355485 & 54 & 756$\pm^{ 36 }_{ 36 }$ & $1$ & 22.8744 & $ -1.74\pm^{ 0.82 }_{ 0.64 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.69\\ 
pg1116 & $0.05927$ (\#30)  & 32.42(38) & 355485 & 54 & 755$\pm^{ 36 }_{ 35 }$ & $1$ & 22.8802 & $ -1.62\pm^{ 0.62 }_{ 0.46 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.50\\ 
pg1116 & $0.11895$ (\#31)  & 40.85(38) & 355485 & 51 & 878$\pm^{ 38 }_{ 37 }$ & $1$ & 24.1693 & $ 11.94\pm^{ 6.77E+03 }_{ 9.95 }$ & $ 15.94\pm^{ 0.18 }_{ 0.31 }$ & 4.27\\ 
pg1116 & $0.13852$ (\#32)  & 41.11(33) & 355485 & 50 & 886$\pm^{ 42 }_{ 41 }$ & $1$ & 24.5920 & $ -1.72\pm^{ 0.53 }_{ 0.42 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.79\\ 
pg1116 & $0.16539$ (\#33)  & 28.52(32) & 355485 & 50 & 949$\pm^{ 44 }_{ 43 }$ & $1$ & 25.1724 & $ 0.32\pm^{ 2.20 }_{ 1.10 }$ & $ 15.03\pm^{ 0.70 }_{ nan }$ & 0.06\\ 
pg1116 & $0.16554$ (\#34)  & 28.43(32) & 355485 & 50 & 952$\pm^{ 44 }_{ 43 }$ & $1$ & 25.1757 & $ 0.51\pm^{ 2.08 }_{ 1.17 }$ & $ 15.23\pm^{ 0.53 }_{ nan }$ & 0.16\\ 
pg1116 & $0.16610$ (\#35)  & 30.58(33) & 355485 & 50 & 948$\pm^{ 44 }_{ 43 }$ & $1$ & 25.1878 & $ 0.99\pm^{ 2.90 }_{ 1.35 }$ & $ 15.47\pm^{ 0.37 }_{ nan }$ & 0.51\\ 
pg1116 & $0.16686$ (\#36)  & 30.77(32) & 355485 & 50 & 944$\pm^{ 44 }_{ 43 }$ & $1$ & 25.2042 & $ 1.23\pm^{ 5.36 }_{ 1.51 }$ & $ 15.52\pm^{ 0.36 }_{ nan }$ & 0.64\\ 
pg1116 & $0.17343$ (\#37)  & 30.83(36) & 355485 & 50 & 941$\pm^{ 41 }_{ 41 }$ & $1$ & 25.3461 & $ -0.67\pm^{ 1.12 }_{ 0.71 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.50\\ 
pg1211 & $0.00711$ (\#38)  & 28.35(30) & 133595 & 1 & 1244$\pm^{ 60 }_{ 58 }$ & $1$ & 21.7536 & $ 0.27\pm^{ 1.59 }_{ 0.95 }$ & $ 14.97\pm^{ 0.67 }_{ nan }$ & 0.07\\ 
pg1211 & $0.05117$ (\#39)  & 48.13(38) & 133595 & 1 & 1465$\pm^{ 67 }_{ 65 }$ & $1$ & 22.7053 & $ 0.99\pm^{ 3.42 }_{ 1.33 }$ & $ 15.44\pm^{ 0.36 }_{ nan }$ & 0.50\\ 
pg1211 & $0.06449$ (\#40)  & 49.38(39) & 133595 & 1 & 1592$\pm^{ 67 }_{ 65 }$ & $1$ & 22.9930 & $ -0.20\pm^{ 1.65 }_{ 0.88 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
pg1211 & $0.06491$ (\#41)  & 51.45(38) & 133595 & 1 & 1586$\pm^{ 67 }_{ 65 }$ & $1$ & 23.0021 & $ -0.05\pm^{ 1.64 }_{ 1.03 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pks0405 & $0.09192$ (\#42)  & 36.05(39) & 376096 & 69 & 494$\pm^{ 35 }_{ 35 }$ & $1$ & 23.5855 & $ 0.49\pm^{ 6.13 }_{ 1.64 }$ & $ 15.21\pm^{ 0.69 }_{ nan }$ & 0.06\\ 
pks0405 & $0.09647$ (\#43)  & 44.38(39) & 376096 & 68 & 538$\pm^{ 35 }_{ 35 }$ & $1$ & 23.6838 & $ 24.63\pm^{ 4.19E+06 }_{ 21.48 }$ & $ 16.00\pm^{ 0.30 }_{ 0.24 }$ & 3.85\\ 
pks0405 & $0.14808$ (\#44)  & 51.46(38) & 376096 & 68 & 537$\pm^{ 38 }_{ 37 }$ & $1$ & 24.7985 & $ -1.29\pm^{ 1.53 }_{ 0.95 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.86\\ 
pks0405 & $0.16566$ (\#45)  & 45.81(38) & 376096 & 68 & 569$\pm^{ 40 }_{ 37 }$ & $1$ & 25.1783 & $ 1.30E+05\pm^{ 1.00E+20 }_{ 6.50E+04 }$ & $ 16.24\pm^{ 0.24 }_{ 0.00 }$ & 7.23\\ 
pks0405 & $0.16606$ (\#46)  & 53.91(39) & 376096 & 68 & 577$\pm^{ 38 }_{ 37 }$ & $1$ & 25.1869 & $ 1.87E+03\pm^{ 1.00E+20 }_{ 1.64E+03 }$ & $ 16.22\pm^{ 0.20 }_{ 0.17 }$ & 6.26\\ 
pks0405 & $0.16659$ (\#47)  & 47.68(38) & 376096 & 68 & 566$\pm^{ 39 }_{ 38 }$ & $1$ & 25.1983 & $ 5.16E+03\pm^{ 1.00E+20 }_{ 5.04E+03 }$ & $ 16.22\pm^{ 0.19 }_{ 0.19 }$ & 5.02\\ 
pks0405 & $0.16688$ (\#48)  & 47.52(38) & 376096 & 68 & 569$\pm^{ 39 }_{ 38 }$ & $1$ & 25.2046 & $ 1.42E+06\pm^{ 1.00E+20 }_{ 1.38E+06 }$ & $ 16.30\pm^{ 0.18 }_{ 0.10 }$ & 5.35\\ 
pks0405 & $0.16712$ (\#49)  & 49.50(39) & 376096 & 69 & 549$\pm^{ 38 }_{ 38 }$ & $1$ & 25.2098 & $ 1.50E+04\pm^{ 1.00E+20 }_{ 1.42E+04 }$ & $ 16.23\pm^{ 0.26 }_{ 0.10 }$ & 4.34\\ 
pks0405 & $0.18257$ (\#50)  & 42.98(38) & 376096 & 69 & 543$\pm^{ 38 }_{ 38 }$ & $1$ & 25.5435 & $ 4.90\pm^{ 1.21E+04 }_{ 5.02 }$ & $ 15.81\pm^{ 0.32 }_{ nan }$ & 0.95\\ 
pks0405 & $0.18289$ (\#51)  & 42.87(38) & 376096 & 69 & 545$\pm^{ 39 }_{ 38 }$ & $1$ & 25.5504 & $ 4.75\pm^{ 516.69 }_{ 4.79 }$ & $ 15.88\pm^{ 0.24 }_{ nan }$ & 1.09\\ 
pks0405 & $0.24052$ (\#52)  & 44.44(38) & 376096 & 68 & 610$\pm^{ 42 }_{ 41 }$ & $1$ & 26.7952 & $ -0.84\pm^{ 1.97 }_{ 0.90 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.36\\ 
pks0405 & $0.24094$ (\#53)  & 44.76(38) & 376096 & 68 & 618$\pm^{ 40 }_{ 41 }$ & $1$ & 26.8043 & $ -0.00\pm^{ 4.81 }_{ 1.21 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.00\\ 
pks0405 & $0.24547$ (\#54)  & 44.46(38) & 376096 & 68 & 595$\pm^{ 42 }_{ 41 }$ & $1$ & 26.9022 & $ -1.24\pm^{ 1.52 }_{ 0.92 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.81\\ 
pks0405 & $0.29762$ (\#55)  & 35.29(38) & 376096 & 69 & 613$\pm^{ 44 }_{ 44 }$ & $1$ & 28.0286 & $ -0.78\pm^{ 2.21 }_{ 1.02 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.26\\ 
pks0405 & $0.34188$ (\#56)  & 38.18(39) & 376096 & 73 & 566$\pm^{ 48 }_{ 46 }$ & $1$ & 28.9846 & $ 44.15\pm^{ 4.03E+06 }_{ 41.46 }$ & $ 16.01\pm^{ 0.26 }_{ 0.27 }$ & 2.12\\ 
pks0405 & $0.34225$ (\#57)  & 38.30(39) & 376096 & 73 & 567$\pm^{ 47 }_{ 46 }$ & $1$ & 28.9926 & $ 24.34\pm^{ 3.79E+05 }_{ 23.38 }$ & $ 16.03\pm^{ 0.25 }_{ 0.60 }$ & 2.00\\ 
pks0405 & $0.35092$ (\#58)  & 32.95(38) & 376096 & 71 & 622$\pm^{ 48 }_{ 48 }$ & $1$ & 29.1799 & $ 37.67\pm^{ 4.43E+06 }_{ 36.03 }$ & $ 16.07\pm^{ 0.27 }_{ 0.47 }$ & 2.62\\ 
pks0405 & $0.36075$ (\#59)  & 38.91(39) & 376096 & 74 & 537$\pm^{ 49 }_{ 48 }$ & $1$ & 29.3922 & $ -1.01\pm^{ 2.61 }_{ 1.02 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.34\\ 
pks0405 & $0.36151$ (\#60)  & 37.68(39) & 376096 & 74 & 542$\pm^{ 49 }_{ 48 }$ & $1$ & 29.4086 & $ -0.85\pm^{ 3.28 }_{ 1.10 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.21\\ 
pks0405 & $0.36329$ (\#61)  & 33.65(38) & 376096 & 74 & 517$\pm^{ 49 }_{ 48 }$ & $1$ & 29.4471 & $ -2.22\pm^{ 1.09 }_{ 0.73 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.88\\ 
pks0405 & $0.40570$ (\#62)  & 52.38(39) & 376096 & 76 & 564$\pm^{ 55 }_{ 54 }$ & $1$ & 30.3631 & $ 2.21\pm^{ 2.29E+03 }_{ 3.42 }$ & $ 15.73\pm^{ 0.50 }_{ nan }$ & 0.26\\ 
pks0405 & $0.40890$ (\#63)  & 47.45(39) & 376096 & 77 & 529$\pm^{ 56 }_{ 54 }$ & $1$ & 30.4322 & $ -0.06\pm^{ 58.07 }_{ 1.62 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.00\\ 
pks0405 & $0.49505$ (\#64)  & 37.44(39) & 376096 & 77 & 501$\pm^{ 56 }_{ 55 }$ & $1$ & 32.2931 & $ -1.91\pm^{ 1.38 }_{ 0.76 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.61\\ 
pks0405 & $0.49530$ (\#65)  & 37.74(38) & 376096 & 78 & 490$\pm^{ 56 }_{ 55 }$ & $1$ & 32.2985 & $ -2.23\pm^{ 1.72 }_{ 1.03 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.56\\ 
pks0405 & $0.55506$ (\#66)  & 35.55(39) & 376096 & 75 & 662$\pm^{ 62 }_{ 60 }$ & $1$ & 33.5893 & $ 1.34E+03\pm^{ 1.00E+20 }_{ 1.29E+03 }$ & $ 16.16\pm^{ 0.25 }_{ 0.18 }$ & 3.09\\ 
pks2005 & $0.06490$ (\#67)  & 35.79(38) & 282191 & 1 & 1954$\pm^{ 63 }_{ 62 }$ & $1$ & 23.0018 & $ -0.67\pm^{ 0.89 }_{ 0.68 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.65\\ 
tons180 & $0.02340$ (\#68)  & 36.68(34) & 76753 & 2 & 1801$\pm^{ 112 }_{ 107 }$ & $1$ & 22.1054 & $ -0.76\pm^{ 1.51 }_{ 0.85 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.38\\ 
tons180 & $0.04360$ (\#69)  & 28.48(39) & 76753 & 2 & 1826$\pm^{ 117 }_{ 112 }$ & $1$ & 22.5418 & $ -0.90\pm^{ 1.15 }_{ 0.75 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.77\\ 
tons180 & $0.04560$ (\#70)  & 25.72(39) & 76753 & 3 & 1796$\pm^{ 118 }_{ 113 }$ & $1$ & 22.5850 & $ -1.39\pm^{ 0.95 }_{ 0.71 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.08\\ 
3c273 & $0.00337$ (\#71)  & -- & -- & -- &  -- & -- & 21.6728 & -- & -- & --\\ 
3c273 & $0.00533$ (\#72)  & 34.47(31) & 69608 & 8 & 5635$\pm^{ 153 }_{ 150 }$ & $1$ & 21.7151 & $ -0.95\pm^{ 0.54 }_{ 0.44 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.87\\ 
3c273 & $0.00764$ (\#73)  & 31.25(31) & 69608 & 8 & 5772$\pm^{ 159 }_{ 155 }$ & $1$ & 21.7650 & $ 0.02\pm^{ 0.83 }_{ 0.61 }$ & $ 13.86\pm^{ 1.56 }_{ nan }$ & 0.00\\ 
3c273 & $0.02947$ (\#74)  & 32.45(39) & 69608 & 8 & 5842$\pm^{ 144 }_{ 141 }$ & $1$ & 22.2366 & $ 0.77\pm^{ 1.10 }_{ 0.78 }$ & $ 15.38\pm^{ 0.29 }_{ nan }$ & 1.06\\ 
3c273 & $0.04898$ (\#75)  & 44.84(39) & 69608 & 8 & 6048$\pm^{ 150 }_{ 147 }$ & $1$ & 22.6580 & $ -0.66\pm^{ 0.56 }_{ 0.43 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.48\\ 
3c273 & $0.06655$ (\#76)  & 50.06(39) & 69608 & 9 & 6143$\pm^{ 154 }_{ 152 }$ & $1$ & 23.0375 & $ -1.09\pm^{ 0.54 }_{ 0.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.80\\ 
3c273 & $0.09018$ (\#77)  & 44.86(38) & 69608 & 8 & 6487$\pm^{ 155 }_{ 153 }$ & $1$ & 23.5479 & $ 1.79\pm^{ 1.92 }_{ 1.09 }$ & $ 15.65\pm^{ 0.17 }_{ 0.31 }$ & 3.91\\ 
3c273 & $0.12007$ (\#78)  & 35.19(38) & 69608 & 7 & 7164$\pm^{ 163 }_{ 163 }$ & $1$ & 24.1935 & $ 0.07\pm^{ 0.81 }_{ 0.59 }$ & $ 14.39\pm^{ 1.01 }_{ nan }$ & 0.01\\ 
3c273 & $0.14660$ (\#79)  & 47.68(39) & 69608 & 7 & 7544$\pm^{ 172 }_{ 169 }$ & $1$ & 24.7666 & $ -0.45\pm^{ 0.60 }_{ 0.46 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.68\\ 
3c273 & $0.15784$ (\#80)  & 40.68(39) & 69608 & 7 & 7512$\pm^{ 172 }_{ 170 }$ & $1$ & 25.0093 & $ 0.46\pm^{ 0.99 }_{ 0.70 }$ & $ 15.18\pm^{ 0.40 }_{ nan }$ & 0.42\\ 
mrk421 & $0.01009$ (\#81)  & 26.88(21) & 638847 & 1 & 73974$\pm^{ 239 }_{ 230 }$ & $1$ & 21.8179 & $ -0.18\pm^{ 0.06 }_{ 0.06 }$ & $ nan\pm^{ nan }_{ nan }$ & 9.92\\ 
pks2155 & $0.05405$ (\#82)  & 20.69(25) & 319334 & 5 & 16258$\pm^{ 147 }_{ 139 }$ & $1$ & 22.7675 & $ 0.32\pm^{ 0.28 }_{ 0.21 }$ & $ 15.03\pm^{ 0.24 }_{ 0.46 }$ & 2.54\\ 
pks2155 & $0.05707$ (\#83)  & 17.03(22) & 319334 & 5 & 16350$\pm^{ 156 }_{ 151 }$ & $1$ & 22.8327 & $ 0.29\pm^{ 0.26 }_{ 0.22 }$ & $ 14.99\pm^{ 0.25 }_{ 0.62 }$ & 2.00\\ 


\hline
\hline
 \end{longtable}
 \end{landscape}

==> Tables/Chandra/Latex/chandra_o7_o6_uppers_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\footnotesize
\begin{landscape}
\begin{longtable}{cc|lllllll|l}
\caption[\chandra\ Data, \ovii\ Upper Limits With \ovi\ Priors Results (Full)]{\ovii\ upper limit measurements with \chandra\ data, at the prior redshift from the \ovi\ lines from Table~\ref{tab:oviPriorsTable}.}
\label{tab:chandraovioviiuppers}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & RGS1 & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N + (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.12314$ (\#1)  & 32.34(39) & 148933 & 1757$\pm^{ 63 }_{ 62 }$ & $1$ & 24.2598 & 0.83 & 15.40 & 0.44\\ 
1es1028 & $0.13706$ (\#2)  & 35.52(39) & 148933 & 1830$\pm^{ 64 }_{ 63 }$ & $1$ & 24.5605 & 2.22 & 15.71 & 0.99\\ 
1es1028 & $0.33735$ (\#3)  & 37.26(39) & 148933 & 2138$\pm^{ 81 }_{ 79 }$ & $1$ & 28.8868 & 0.86 & 15.43 & 0.56\\ 
1es1553 & $0.18759$ (\#4)  & 44.14(38) & 495645 & 3135$\pm^{ 48 }_{ 48 }$ & $1$ & 25.6519 & 0.51 & 15.23 & 0.58\\ 
1es1553 & $0.18775$ (\#5)  & 44.13(38) & 495645 & 3135$\pm^{ 48 }_{ 48 }$ & $1$ & 25.6554 & 0.55 & 15.24 & 0.58\\ 
1es1553 & $0.18984$ (\#6)  & 42.53(38) & 495645 & 3106$\pm^{ 48 }_{ 48 }$ & $1$ & 25.7005 & 0.38 & 15.11 & 1.00\\ 
1es1553 & $0.21631$ (\#7)  & 51.98(38) & 495645 & 3137$\pm^{ 49 }_{ 49 }$ & $1$ & 26.2723 & 0.52 & 15.23 & 0.42\\ 
1es1553 & $0.31130$ (\#8)  & 36.35(38) & 495645 & 3202$\pm^{ 53 }_{ 54 }$ & $1$ & 28.3241 & 0.48 & 15.21 & 0.01\\ 
1es1553 & $0.37868$ (\#9)  & 48.60(38) & 495645 & 3322$\pm^{ 62 }_{ 61 }$ & $1$ & 29.7795 & 0.36 & 15.08 & 2.89\\ 
1es1553 & $0.39497$ (\#10)  & 39.90(38) & 495645 & 3374$\pm^{ 65 }_{ 64 }$ & $1$ & 30.1314 & 0.42 & 15.13 & 1.16\\ 
h1821 & $0.02438$ (\#11)  & 44.15(32) & 470152 & 888$\pm^{ 22 }_{ 21 }$ & $1$ & 22.1266 & 0.66 & 15.32 & 0.32\\ 
h1821 & $0.10817$ (\#12)  & 50.75(39) & 470152 & 1103$\pm^{ 21 }_{ 21 }$ & $1$ & 23.9365 & 0.33 & 15.05 & 8.78\\ 
h1821 & $0.12133$ (\#13)  & 46.33(38) & 470152 & 1202$\pm^{ 22 }_{ 22 }$ & $1$ & 24.2207 & 0.53 & 15.23 & 0.22\\ 
h1821 & $0.12147$ (\#14)  & 46.13(38) & 470152 & 1203$\pm^{ 22 }_{ 22 }$ & $1$ & 24.2238 & 0.53 & 15.24 & 0.44\\ 
h1821 & $0.16992$ (\#15)  & 37.35(38) & 470152 & 1107$\pm^{ 23 }_{ 23 }$ & $1$ & 25.2703 & 0.51 & 15.21 & 0.02\\ 
h1821 & $0.17043$ (\#16)  & 37.01(38) & 470152 & 1104$\pm^{ 23 }_{ 23 }$ & $1$ & 25.2813 & 0.45 & 15.16 & 0.39\\ 
h1821 & $0.21326$ (\#17)  & 33.42(38) & 470152 & 1090$\pm^{ 25 }_{ 25 }$ & $1$ & 26.2064 & 0.36 & 15.08 & 3.65\\ 
h1821 & $0.22497$ (\#18)  & 31.24(39) & 470152 & 1097$\pm^{ 26 }_{ 25 }$ & $1$ & 26.4594 & 0.74 & 15.36 & 0.74\\ 
h1821 & $0.22522$ (\#19)  & 31.59(39) & 470152 & 1095$\pm^{ 26 }_{ 25 }$ & $1$ & 26.4648 & 0.69 & 15.34 & 0.37\\ 
h1821 & $0.22639$ (\#20)  & 32.44(39) & 470152 & 1098$\pm^{ 26 }_{ 25 }$ & $1$ & 26.4900 & 0.65 & 15.32 & 0.23\\ 
h1821 & $0.24531$ (\#21)  & 28.82(38) & 470152 & 1103$\pm^{ 27 }_{ 27 }$ & $1$ & 26.8987 & 0.97 & 15.47 & 2.16\\ 
h1821 & $0.26657$ (\#22)  & 39.22(39) & 470152 & 1157$\pm^{ 29 }_{ 29 }$ & $1$ & 27.3579 & 0.57 & 15.26 & 0.09\\ 
h1821 & $0.28800$ (\#23)  & 48.59(33) & 470152 & 1265$\pm^{ 37 }_{ 37 }$ & $1$ & 27.8208 & 0.47 & 15.18 & 2.16\\ 
h1821 & $0.29658$ (\#24)  & 45.10(33) & 470152 & 1326$\pm^{ 41 }_{ 40 }$ & $1$ & 28.0061 & 0.60 & 15.27 & 3.22\\ 
h1821 & $0.29680$ (\#25)  & 45.72(34) & 470152 & 1338$\pm^{ 42 }_{ 41 }$ & $1$ & 28.0109 & 0.80 & 15.40 & 2.92\\ 
h2356 & $0.11461$ (\#26)  & 26.64(38) & 586697 & 2314$\pm^{ 37 }_{ 37 }$ & $1$ & 24.0756 & 0.76 & 15.38 & 4.89\\ 
h2356 & $0.16512$ (\#27)  & 34.18(39) & 586697 & 2408$\pm^{ 39 }_{ 39 }$ & $1$ & 25.1666 & 0.87 & 15.40 & 3.76\\ 
mr2251 & $0.01070$ (\#28)  & 33.00(30) & 78434 & 3031$\pm^{ 114 }_{ 110 }$ & $1$ & 21.8311 & 1.07 & 15.46 & 0.00\\ 
pg1116 & $0.05900$ (\#29)  & 33.16(38) & 355485 & 756$\pm^{ 36 }_{ 36 }$ & $1$ & 22.8744 & 0.73 & 15.37 & 3.69\\ 
pg1116 & $0.05927$ (\#30)  & 32.42(38) & 355485 & 755$\pm^{ 36 }_{ 35 }$ & $1$ & 22.8802 & 0.54 & 15.23 & 4.50\\ 
pg1116 & $0.11895$ (\#31)  & 40.85(38) & 355485 & 878$\pm^{ 38 }_{ 37 }$ & $1$ & 24.1693 & 3.39E+03 & 16.12 & 4.27\\ 
pg1116 & $0.13852$ (\#32)  & 41.11(33) & 355485 & 886$\pm^{ 42 }_{ 41 }$ & $1$ & 24.5920 & 0.47 & 15.18 & 6.79\\ 
pg1116 & $0.16539$ (\#33)  & 28.52(32) & 355485 & 949$\pm^{ 44 }_{ 43 }$ & $1$ & 25.1724 & 1.65 & 15.62 & 0.06\\ 
pg1116 & $0.16554$ (\#34)  & 28.43(32) & 355485 & 952$\pm^{ 44 }_{ 43 }$ & $1$ & 25.1757 & 1.63 & 15.64 & 0.16\\ 
pg1116 & $0.16610$ (\#35)  & 30.58(33) & 355485 & 948$\pm^{ 44 }_{ 43 }$ & $1$ & 25.1878 & 2.12 & 15.71 & 0.51\\ 
pg1116 & $0.16686$ (\#36)  & 30.77(32) & 355485 & 944$\pm^{ 44 }_{ 43 }$ & $1$ & 25.2042 & 3.44 & 15.77 & 0.64\\ 
pg1116 & $0.17343$ (\#37)  & 30.83(36) & 355485 & 941$\pm^{ 41 }_{ 41 }$ & $1$ & 25.3461 & 0.91 & 15.42 & 0.50\\ 
pg1211 & $0.00711$ (\#38)  & 28.35(30) & 133595 & 1244$\pm^{ 60 }_{ 58 }$ & $1$ & 21.7536 & 1.27 & 15.53 & 0.07\\ 
pg1211 & $0.05117$ (\#39)  & 48.13(38) & 133595 & 1465$\pm^{ 67 }_{ 65 }$ & $1$ & 22.7053 & 2.38 & 15.68 & 0.50\\ 
pg1211 & $0.06449$ (\#40)  & 49.38(39) & 133595 & 1592$\pm^{ 67 }_{ 65 }$ & $1$ & 22.9930 & 1.27 & 15.52 & 0.03\\ 
pg1211 & $0.06491$ (\#41)  & 51.45(38) & 133595 & 1586$\pm^{ 67 }_{ 65 }$ & $1$ & 23.0021 & 1.33 & 15.56 & 0.00\\ 
pks0405 & $0.09192$ (\#42)  & 36.05(39) & 376096 & 494$\pm^{ 35 }_{ 35 }$ & $1$ & 23.5855 & 3.89 & 15.83 & 0.06\\ 
pks0405 & $0.09647$ (\#43)  & 44.38(39) & 376096 & 538$\pm^{ 35 }_{ 35 }$ & $1$ & 23.6838 & 2.09E+06 & 16.28 & 3.85\\ 
pks0405 & $0.14808$ (\#44)  & 51.46(38) & 376096 & 537$\pm^{ 38 }_{ 37 }$ & $1$ & 24.7985 & 1.24 & 15.55 & 0.86\\ 
pks0405 & $0.16566$ (\#45)  & 45.81(38) & 376096 & 569$\pm^{ 40 }_{ 37 }$ & $1$ & 25.1783 & 5.00E+19 & 16.48 & 7.23\\ 
pks0405 & $0.16606$ (\#46)  & 53.91(39) & 376096 & 577$\pm^{ 38 }_{ 37 }$ & $1$ & 25.1869 & 5.00E+19 & 16.42 & 6.26\\ 
pks0405 & $0.16659$ (\#47)  & 47.68(38) & 376096 & 566$\pm^{ 39 }_{ 38 }$ & $1$ & 25.1983 & 5.00E+19 & 16.42 & 5.02\\ 
pks0405 & $0.16688$ (\#48)  & 47.52(38) & 376096 & 569$\pm^{ 39 }_{ 38 }$ & $1$ & 25.2046 & 5.00E+19 & 16.48 & 5.35\\ 
pks0405 & $0.16712$ (\#49)  & 49.50(39) & 376096 & 549$\pm^{ 38 }_{ 38 }$ & $1$ & 25.2098 & 5.00E+19 & 16.48 & 4.34\\ 
pks0405 & $0.18257$ (\#50)  & 42.98(38) & 376096 & 543$\pm^{ 38 }_{ 38 }$ & $1$ & 25.5435 & 6.03E+03 & 16.12 & 0.95\\ 
pks0405 & $0.18289$ (\#51)  & 42.87(38) & 376096 & 545$\pm^{ 39 }_{ 38 }$ & $1$ & 25.5504 & 260.74 & 16.06 & 1.09\\ 
pks0405 & $0.24052$ (\#52)  & 44.44(38) & 376096 & 610$\pm^{ 42 }_{ 41 }$ & $1$ & 26.7952 & 1.43 & 15.56 & 0.36\\ 
pks0405 & $0.24094$ (\#53)  & 44.76(38) & 376096 & 618$\pm^{ 40 }_{ 41 }$ & $1$ & 26.8043 & 3.01 & 15.74 & -0.00\\ 
pks0405 & $0.24547$ (\#54)  & 44.46(38) & 376096 & 595$\pm^{ 42 }_{ 41 }$ & $1$ & 26.9022 & 1.22 & 15.54 & 0.81\\ 
pks0405 & $0.29762$ (\#55)  & 35.29(38) & 376096 & 613$\pm^{ 44 }_{ 44 }$ & $1$ & 28.0286 & 1.62 & 15.60 & 0.26\\ 
pks0405 & $0.34188$ (\#56)  & 38.18(39) & 376096 & 566$\pm^{ 48 }_{ 46 }$ & $1$ & 28.9846 & 2.02E+06 & 16.26 & 2.12\\ 
pks0405 & $0.34225$ (\#57)  & 38.30(39) & 376096 & 567$\pm^{ 47 }_{ 46 }$ & $1$ & 28.9926 & 1.89E+05 & 16.26 & 2.00\\ 
pks0405 & $0.35092$ (\#58)  & 32.95(38) & 376096 & 622$\pm^{ 48 }_{ 48 }$ & $1$ & 29.1799 & 2.21E+06 & 16.33 & 2.62\\ 
pks0405 & $0.36075$ (\#59)  & 38.91(39) & 376096 & 537$\pm^{ 49 }_{ 48 }$ & $1$ & 29.3922 & 1.82 & 15.62 & 0.34\\ 
pks0405 & $0.36151$ (\#60)  & 37.68(39) & 376096 & 542$\pm^{ 49 }_{ 48 }$ & $1$ & 29.4086 & 2.19 & 15.67 & 0.21\\ 
pks0405 & $0.36329$ (\#61)  & 33.65(38) & 376096 & 517$\pm^{ 49 }_{ 48 }$ & $1$ & 29.4471 & 0.91 & 15.43 & 2.88\\ 
pks0405 & $0.40570$ (\#62)  & 52.38(39) & 376096 & 564$\pm^{ 55 }_{ 54 }$ & $1$ & 30.3631 & 1.15E+03 & 16.19 & 0.26\\ 
pks0405 & $0.40890$ (\#63)  & 47.45(39) & 376096 & 529$\pm^{ 56 }_{ 54 }$ & $1$ & 30.4322 & 29.84 & 16.06 & -0.00\\ 
pks0405 & $0.49505$ (\#64)  & 37.44(39) & 376096 & 501$\pm^{ 56 }_{ 55 }$ & $1$ & 32.2931 & 1.07 & 15.46 & 1.61\\ 
pks0405 & $0.49530$ (\#65)  & 37.74(38) & 376096 & 490$\pm^{ 56 }_{ 55 }$ & $1$ & 32.2985 & 1.37 & 15.58 & 1.56\\ 
pks0405 & $0.55506$ (\#66)  & 35.55(39) & 376096 & 662$\pm^{ 62 }_{ 60 }$ & $1$ & 33.5893 & 5.00E+19 & 16.42 & 3.09\\ 
pks2005 & $0.06490$ (\#67)  & 35.79(38) & 282191 & 1954$\pm^{ 63 }_{ 62 }$ & $1$ & 23.0018 & 0.78 & 15.39 & 0.65\\ 
tons180 & $0.02340$ (\#68)  & 36.68(34) & 76753 & 1801$\pm^{ 112 }_{ 107 }$ & $1$ & 22.1054 & 1.18 & 15.49 & 0.38\\ 
tons180 & $0.04360$ (\#69)  & 28.48(39) & 76753 & 1826$\pm^{ 117 }_{ 112 }$ & $1$ & 22.5418 & 0.95 & 15.43 & 0.77\\ 
tons180 & $0.04560$ (\#70)  & 25.72(39) & 76753 & 1796$\pm^{ 118 }_{ 113 }$ & $1$ & 22.5850 & 0.83 & 15.40 & 2.08\\ 
3c273 & $0.00337$ (\#71)  & -- & -- & -- & -- & 21.6728 & -- & -- & --\\ 
3c273 & $0.00533$ (\#72)  & 34.47(31) & 69608 & 5635$\pm^{ 153 }_{ 150 }$ & $1$ & 21.7151 & 0.49 & 15.21 & 2.87\\ 
3c273 & $0.00764$ (\#73)  & 31.25(31) & 69608 & 5772$\pm^{ 159 }_{ 155 }$ & $1$ & 21.7650 & 0.72 & 15.35 & 0.00\\ 
3c273 & $0.02947$ (\#74)  & 32.45(39) & 69608 & 5842$\pm^{ 144 }_{ 141 }$ & $1$ & 22.2366 & 0.94 & 15.46 & 1.06\\ 
3c273 & $0.04898$ (\#75)  & 44.84(39) & 69608 & 6048$\pm^{ 150 }_{ 147 }$ & $1$ & 22.6580 & 0.50 & 15.20 & 1.48\\ 
3c273 & $0.06655$ (\#76)  & 50.06(39) & 69608 & 6143$\pm^{ 154 }_{ 152 }$ & $1$ & 23.0375 & 0.51 & 15.23 & 3.80\\ 
3c273 & $0.09018$ (\#77)  & 44.86(38) & 69608 & 6487$\pm^{ 155 }_{ 153 }$ & $1$ & 23.5479 & 1.51 & 15.60 & 3.91\\ 
3c273 & $0.12007$ (\#78)  & 35.19(38) & 69608 & 7164$\pm^{ 163 }_{ 163 }$ & $1$ & 24.1935 & 0.70 & 15.32 & 0.01\\ 
3c273 & $0.14660$ (\#79)  & 47.68(39) & 69608 & 7544$\pm^{ 172 }_{ 169 }$ & $1$ & 24.7666 & 0.53 & 15.23 & 0.68\\ 
3c273 & $0.15784$ (\#80)  & 40.68(39) & 69608 & 7512$\pm^{ 172 }_{ 170 }$ & $1$ & 25.0093 & 0.84 & 15.40 & 0.42\\ 
mrk421 & $0.01009$ (\#81)  & 26.88(21) & 638847 & 73974$\pm^{ 239 }_{ 230 }$ & $1$ & 21.8179 & 0.06 & 14.34 & 9.92\\ 
pks2155 & $0.05405$ (\#82)  & 20.69(25) & 319334 & 16258$\pm^{ 147 }_{ 139 }$ & $1$ & 22.7675 & 0.25 & 14.93 & 2.54\\ 
pks2155 & $0.05707$ (\#83)  & 17.03(22) & 319334 & 16350$\pm^{ 156 }_{ 151 }$ & $1$ & 22.8327 & 0.24 & 14.92 & 2.00\\ 


\hline
\hline
\end{longtable}
\end{landscape}

==> Tables/Chandra/Latex/chandra_o8_hi_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
%\footnotesize
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllll|l}
\caption[\chandra\ Data, \oviii\ With \hi\ Priors Results (Full)]{\oviii\ measurements with \chandra\ data, at the prior redshift from the \hi\ lines from Table~\ref{tab:hiPriorsTable}.}
\label{tab:chandrahioviii}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & \multicolumn{2}{c}{RGS1} & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \% $\frac{B}{D+B}$ & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.20383$ (\#2)  & 24.47(38) & 148933 & 25 & 1653$\pm^{ 61 }_{ 59 }$ & $1$ & 22.8246 & $ -1.22\pm^{ 0.69 }_{ 0.52 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.76\\ 
1es1028 & $0.22121$ (\#3)  & 26.80(38) & 148933 & 25 & 1757$\pm^{ 63 }_{ 61 }$ & $1$ & 23.1541 & $ 3.82\pm^{ 13.01 }_{ 2.75 }$ & $ 16.13\pm^{ 0.19 }_{ 0.32 }$ & 3.68\\ 
1es1553 & $0.03466$ (\#4)  & 51.93(39) & 495645 & 21 & 2174$\pm^{ 31 }_{ 31 }$ & $1$ & 19.6172 & $ 0.21\pm^{ 0.53 }_{ 0.42 }$ & $ 15.19\pm^{ 0.49 }_{ nan }$ & 0.23\\ 
1es1553 & $0.04273$ (\#5)  & 42.22(38) & 495645 & 22 & 2213$\pm^{ 32 }_{ 32 }$ & $1$ & 19.7702 & $ 0.00\pm^{ 0.58 }_{ 0.35 }$ & $ 13.57\pm^{ 2.03 }_{ nan }$ & 0.00\\ 
1es1553 & $0.06364$ (\#6)  & 42.31(39) & 495645 & 23 & 2255$\pm^{ 35 }_{ 35 }$ & $1$ & 20.1666 & $ 0.86\pm^{ 0.85 }_{ 0.59 }$ & $ 15.74\pm^{ 0.21 }_{ 0.44 }$ & 2.66\\ 
1es1553 & $0.21869$ (\#7)  & 36.69(30) & 495645 & 24 & 2585$\pm^{ 49 }_{ 48 }$ & $1$ & 23.1064 & $ -0.35\pm^{ 0.43 }_{ 0.35 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.78\\ 
3c273 & $0.00758$ (\#8)  & 49.20(38) & 69608 & 6 & 5103$\pm^{ 101 }_{ 99 }$ & $1$ & 19.1037 & $ 1.21\pm^{ 1.27 }_{ 0.81 }$ & $ 15.85\pm^{ 0.19 }_{ 0.39 }$ & 3.07\\ 
3c273 & $0.06707$ (\#9)  & 46.91(39) & 69608 & 8 & 5560$\pm^{ 124 }_{ 134 }$ & $1$ & 20.2316 & $ 0.02\pm^{ 0.67 }_{ 0.65 }$ & $ 14.14\pm^{ 1.51 }_{ nan }$ & -0.01\\ 
3c273 & $0.07359$ (\#10)  & 43.29(38) & 69608 & 8 & 5652$\pm^{ 130 }_{ 128 }$ & $1$ & 20.3553 & $ 1.00\pm^{ 1.61 }_{ 0.87 }$ & $ 15.78\pm^{ 0.25 }_{ 0.79 }$ & 1.54\\ 
3c273 & $0.13960$ (\#11)  & -- & -- & -- &  -- & -- & 21.6068 & -- & -- & --\\ 
h1821 & $0.00944$ (\#12)  & 38.66(39) & 470152 & 2 & 824$\pm^{ 14 }_{ 14 }$ & $1$ & 19.1390 & $ -0.32\pm^{ 0.39 }_{ 0.35 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.75\\ 
h1821 & $0.06779$ (\#13)  & 39.35(38) & 470152 & 2 & 852$\pm^{ 16 }_{ 15 }$ & $1$ & 20.2453 & $ 2.02\pm^{ 1.67 }_{ 0.98 }$ & $ 15.98\pm^{ 0.13 }_{ 0.19 }$ & 7.79\\ 
h1821 & $0.08483$ (\#14)  & 44.68(39) & 470152 & 2 & 843$\pm^{ 16 }_{ 16 }$ & $1$ & 20.5684 & $ -0.26\pm^{ 0.45 }_{ 0.37 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.39\\ 
h1821 & $0.12147$ (\#15)  & 42.69(31) & 470152 & 2 & 880$\pm^{ 20 }_{ 20 }$ & $1$ & 21.2631 & $ -0.03\pm^{ 0.54 }_{ 0.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
h1821 & $0.19817$ (\#16)  & 49.67(39) & 470152 & 2 & 931$\pm^{ 22 }_{ 22 }$ & $1$ & 22.7173 & $ 1.16\pm^{ 1.47 }_{ 0.86 }$ & $ 15.83\pm^{ 0.21 }_{ 0.49 }$ & 2.27\\ 
h1821 & $0.21321$ (\#17)  & 35.27(35) & 470152 & 2 & 948$\pm^{ 23 }_{ 23 }$ & $1$ & 23.0025 & $ -0.55\pm^{ 0.60 }_{ 0.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.93\\ 
h1821 & $0.24531$ (\#18)  & 32.59(30) & 470152 & 1 & 1130$\pm^{ 25 }_{ 24 }$ & $1$ & 23.6111 & $ 0.85\pm^{ 0.73 }_{ 0.58 }$ & $ 15.76\pm^{ 0.20 }_{ 0.44 }$ & 2.67\\ 
h2356 & $0.03830$ (\#19)  & 39.37(39) & 586697 & 25 & 2067$\pm^{ 29 }_{ 29 }$ & $1$ & 19.6862 & $ -0.53\pm^{ 0.35 }_{ 0.31 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.38\\ 
h2356 & $0.07881$ (\#20)  & 40.55(38) & 586697 & 27 & 2087$\pm^{ 32 }_{ 32 }$ & $1$ & 20.4542 & $ -0.51\pm^{ 0.35 }_{ 0.30 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.15\\ 
h2356 & $0.10467$ (\#21)  & 41.21(38) & 586697 & 28 & 2108$\pm^{ 31 }_{ 31 }$ & $1$ & 20.9445 & $ 0.01\pm^{ 0.52 }_{ 0.38 }$ & $ 13.73\pm^{ 1.83 }_{ nan }$ & 0.00\\ 
h2356 & $0.15613$ (\#22)  & 28.52(30) & 586697 & 28 & 2138$\pm^{ 39 }_{ 39 }$ & $1$ & 21.9202 & $ -0.08\pm^{ 0.48 }_{ 0.40 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.05\\ 
mr2251 & $0.01068$ (\#23)  & 31.54(39) & 78434 & 12 & 2573$\pm^{ 72 }_{ 70 }$ & $1$ & 19.1625 & $ 1.17\pm^{ 1.54 }_{ 0.99 }$ & $ 15.87\pm^{ 0.24 }_{ 0.73 }$ & 1.66\\ 
mr2251 & $0.01449$ (\#24)  & 25.42(39) & 78434 & 12 & 2473$\pm^{ 71 }_{ 70 }$ & $1$ & 19.2347 & $ -1.12\pm^{ 0.54 }_{ 0.44 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.77\\ 
mr2251 & $0.06131$ (\#25)  & 43.48(38) & 78434 & 15 & 2702$\pm^{ 88 }_{ 86 }$ & $1$ & 20.1224 & $ 3.21\pm^{ 12.08 }_{ 2.17 }$ & $ 16.12\pm^{ 0.17 }_{ 0.31 }$ & 3.98\\ 
mr2251 & $0.06190$ (\#26)  & 43.84(39) & 78434 & 15 & 2700$\pm^{ 88 }_{ 86 }$ & $1$ & 20.1336 & $ 3.41\pm^{ 9.45 }_{ 2.46 }$ & $ 16.11\pm^{ 0.18 }_{ 0.34 }$ & 3.61\\ 
mr2251 & $0.06276$ (\#27)  & 43.50(38) & 78434 & 15 & 2697$\pm^{ 88 }_{ 86 }$ & $1$ & 20.1499 & $ 2.98\pm^{ 54.62 }_{ 1.92 }$ & $ 16.13\pm^{ 0.17 }_{ 0.30 }$ & 4.11\\ 
mr2251 & $0.06327$ (\#28)  & 43.55(39) & 78434 & 15 & 2707$\pm^{ 88 }_{ 87 }$ & $1$ & 20.1596 & $ 5.13\pm^{ 32.32 }_{ 3.54 }$ & $ 16.20\pm^{ 0.14 }_{ 0.25 }$ & 5.17\\ 
mr2251 & $0.06381$ (\#29)  & 41.59(38) & 78434 & 15 & 2714$\pm^{ 89 }_{ 87 }$ & $1$ & 20.1698 & $ 7.99\pm^{ 14.98 }_{ 5.86 }$ & $ 16.22\pm^{ 0.14 }_{ 0.23 }$ & 5.94\\ 
mrk478 & $0.06166$ (\#30)  & 37.08(38) & 80466 & 20 & 1284$\pm^{ 61 }_{ 60 }$ & $1$ & 20.1291 & $ -1.60\pm^{ 0.68 }_{ 0.51 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.08\\ 
mrk478 & $0.06578$ (\#31)  & 38.24(39) & 80466 & 20 & 1328$\pm^{ 63 }_{ 61 }$ & $1$ & 20.2072 & $ 0.96\pm^{ 5.56 }_{ 1.48 }$ & $ 15.77\pm^{ 0.43 }_{ nan }$ & 0.35\\ 
mrk478 & $0.07213$ (\#32)  & 34.86(38) & 80466 & 20 & 1330$\pm^{ 62 }_{ 60 }$ & $1$ & 20.3276 & $ 21.99\pm^{ 1.46E+03 }_{ 18.85 }$ & $ 16.30\pm^{ 0.16 }_{ 0.19 }$ & 4.58\\ 
pg1116 & $0.04114$ (\#33)  & 38.61(39) & 355485 & 52 & 635$\pm^{ 27 }_{ 27 }$ & $1$ & 19.7400 & $ 0.85\pm^{ 3.32 }_{ 1.35 }$ & $ 15.75\pm^{ 0.43 }_{ nan }$ & 0.34\\ 
pg1116 & $0.06251$ (\#34)  & 31.45(38) & 355485 & 54 & 631$\pm^{ 29 }_{ 28 }$ & $1$ & 20.1452 & $ -0.69\pm^{ 1.20 }_{ 0.71 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.48\\ 
pg1116 & $0.08382$ (\#35)  & 36.50(38) & 355485 & 55 & 618$\pm^{ 30 }_{ 29 }$ & $1$ & 20.5492 & $ -0.65\pm^{ 1.33 }_{ 0.89 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.34\\ 
pg1116 & $0.09210$ (\#36)  & 33.90(38) & 355485 & 55 & 632$\pm^{ 30 }_{ 30 }$ & $1$ & 20.7062 & $ 1.27\pm^{ 7.97 }_{ 1.66 }$ & $ 15.85\pm^{ 0.39 }_{ nan }$ & 0.50\\ 
pg1116 & $0.09281$ (\#37)  & 33.80(38) & 355485 & 55 & 633$\pm^{ 30 }_{ 30 }$ & $1$ & 20.7197 & $ 1.43\pm^{ 8.70 }_{ 1.75 }$ & $ 15.89\pm^{ 0.37 }_{ nan }$ & 0.61\\ 
pg1116 & $0.13373$ (\#38)  & 21.48(30) & 355485 & 52 & 757$\pm^{ 36 }_{ 36 }$ & $1$ & 21.4955 & $ 0.31\pm^{ 4.31 }_{ 1.24 }$ & $ 15.35\pm^{ 0.80 }_{ nan }$ & 0.04\\ 
pg1116 & $0.13851$ (\#39)  & -- & -- & -- &  -- & -- & 21.5861 & -- & -- & --\\ 
pg1211 & $0.02586$ (\#40)  & 33.54(38) & 133595 & 1 & 1070$\pm^{ 37 }_{ 36 }$ & $1$ & 19.4503 & $ 1.44\pm^{ 2.02 }_{ 1.18 }$ & $ 15.94\pm^{ 0.23 }_{ 0.65 }$ & 1.73\\ 
pg1211 & $0.05443$ (\#41)  & 30.17(39) & 133595 & 1 & 1124$\pm^{ 41 }_{ 40 }$ & $1$ & 19.9920 & $ -0.98\pm^{ 0.63 }_{ 0.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.25\\ 
pks0405 & $0.02510$ (\#42)  & 32.93(39) & 376096 & 63 & 432$\pm^{ 24 }_{ 23 }$ & $1$ & 19.4359 & $ 0.83\pm^{ 5.37 }_{ 1.61 }$ & $ 15.75\pm^{ 0.49 }_{ nan }$ & 0.21\\ 
pks0405 & $0.05902$ (\#43)  & 31.53(38) & 376096 & 68 & 431$\pm^{ 29 }_{ 28 }$ & $1$ & 20.0790 & $ 1.75\pm^{ 35.93 }_{ 2.44 }$ & $ 15.96\pm^{ 0.42 }_{ nan }$ & 0.37\\ 
pks0405 & $0.09719$ (\#44)  & 37.54(38) & 376096 & 68 & 470$\pm^{ 30 }_{ 30 }$ & $1$ & 20.8027 & $ 719.82\pm^{ 8.55E+03 }_{ 727.42 }$ & $ 16.45\pm^{ 0.10 }_{ nan }$ & 3.80\\ 
pks0405 & $0.10152$ (\#45)  & 39.29(39) & 376096 & 67 & 462$\pm^{ 31 }_{ 30 }$ & $1$ & 20.8848 & $ -0.97\pm^{ 1.70 }_{ 0.93 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.49\\ 
pks0405 & $0.10298$ (\#46)  & 33.14(39) & 376096 & 67 & 466$\pm^{ 31 }_{ 30 }$ & $1$ & 20.9125 & $ 1.46\pm^{ 175.16 }_{ 2.15 }$ & $ 15.94\pm^{ 0.42 }_{ nan }$ & 0.38\\ 
pks0405 & $0.19456$ (\#47)  & 32.55(38) & 376096 & 68 & 514$\pm^{ 35 }_{ 35 }$ & $1$ & 22.6489 & $ -0.83\pm^{ 1.97 }_{ 1.11 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.30\\ 
pks0405 & $0.21976$ (\#48)  & 37.95(38) & 376096 & 68 & 537$\pm^{ 36 }_{ 36 }$ & $1$ & 23.1266 & $ 1.69\pm^{ 199.14 }_{ 2.35 }$ & $ 15.98\pm^{ 0.42 }_{ nan }$ & 0.41\\ 
pks0405 & $0.24564$ (\#49)  & 39.21(39) & 376096 & 69 & 487$\pm^{ 35 }_{ 35 }$ & $1$ & 23.6173 & $ -0.78\pm^{ 2.16 }_{ 0.93 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.29\\ 
pks0405 & $0.29748$ (\#50)  & 42.61(38) & 376096 & 66 & 595$\pm^{ 38 }_{ 37 }$ & $1$ & 24.6002 & $ 1.31\pm^{ 153.91 }_{ 1.98 }$ & $ 15.91\pm^{ 0.44 }_{ nan }$ & 0.37\\ 
pks0405 & $0.31016$ (\#51)  & 50.26(39) & 376096 & 68 & 547$\pm^{ 37 }_{ 37 }$ & $1$ & 24.8406 & $ 3.28\pm^{ 6.44E+03 }_{ 3.32 }$ & $ 16.12\pm^{ 0.40 }_{ nan }$ & 1.07\\ 
pks0405 & $0.32502$ (\#52)  & 53.39(38) & 376096 & 68 & 543$\pm^{ 39 }_{ 37 }$ & $1$ & 25.1224 & $ -0.25\pm^{ 6.77 }_{ 1.30 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pks0405 & $0.49508$ (\#53)  & 40.12(38) & 376096 & 71 & 570$\pm^{ 45 }_{ 44 }$ & $1$ & 28.3467 & $ -1.07\pm^{ 2.07 }_{ 0.99 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.46\\ 
pks2155 & $0.05708$ (\#54)  & 42.87(39) & 319334 & 4 & 13878$\pm^{ 90 }_{ 95 }$ & $1$ & 20.0422 & $ 0.08\pm^{ 0.18 }_{ 0.21 }$ & $ 14.81\pm^{ 0.49 }_{ nan }$ & 0.09\\ 
pks2155 & $0.06236$ (\#55)  & 43.07(39) & 319334 & 4 & 13944$\pm^{ 92 }_{ 93 }$ & $1$ & 20.1423 & $ -0.07\pm^{ 0.19 }_{ 0.18 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.14\\ 
pks2155 & $0.10586$ (\#56)  & 36.85(39) & 319334 & 4 & 14826$\pm^{ 95 }_{ 94 }$ & $1$ & 20.9671 & $ -0.01\pm^{ 0.31 }_{ 0.12 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.04\\ 
tons180 & $0.04304$ (\#57)  & 24.70(38) & 76753 & 1 & 1560$\pm^{ 44 }_{ 43 }$ & $1$ & 19.7760 & $ -0.78\pm^{ 0.60 }_{ 0.51 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.75\\

\hline
\hline
 \end{longtable}
 \end{landscape}

==> Tables/Chandra/Latex/chandra_o8_hi_uppers_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\footnotesize
\begin{landscape}
\begin{longtable}{cc|lllllll|l}
\caption[\chandra\ Data, \oviii\ Upper Limits With \hi\ Priors Results (Full)]{\oviii\ upper limit measurements with \chandra\ data, at the prior redshift from the \hi\ lines from Table~\ref{tab:hiPriorsTable}.}
\label{tab:chandrahioviiiuppers}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & RGS1 & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N + (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.13714$ (\#1)  & -- & -- & -- & -- & 21.5602 & -- & -- & --\\ 
1es1028 & $0.20383$ (\#2)  & 24.47(38) & 148933 & 1653$\pm^{ 61 }_{ 59 }$ & $1$ & 22.8246 & 0.61 & 15.63 & 2.76\\ 
1es1028 & $0.22121$ (\#3)  & 26.80(38) & 148933 & 1757$\pm^{ 63 }_{ 61 }$ & $1$ & 23.1541 & 7.88 & 16.23 & 3.68\\ 
1es1553 & $0.03466$ (\#4)  & 51.93(39) & 495645 & 2174$\pm^{ 31 }_{ 31 }$ & $1$ & 19.6172 & 0.48 & 15.52 & 0.23\\ 
1es1553 & $0.04273$ (\#5)  & 42.22(38) & 495645 & 2213$\pm^{ 32 }_{ 32 }$ & $1$ & 19.7702 & 0.46 & 15.51 & 0.00\\ 
1es1553 & $0.06364$ (\#6)  & 42.31(39) & 495645 & 2255$\pm^{ 35 }_{ 35 }$ & $1$ & 20.1666 & 0.72 & 15.68 & 2.66\\ 
1es1553 & $0.21869$ (\#7)  & 36.69(30) & 495645 & 2585$\pm^{ 49 }_{ 48 }$ & $1$ & 23.1064 & 0.39 & 15.44 & 0.78\\ 
3c273 & $0.00758$ (\#8)  & 49.20(38) & 69608 & 5103$\pm^{ 101 }_{ 99 }$ & $1$ & 19.1037 & 1.04 & 15.81 & 3.07\\ 
3c273 & $0.06707$ (\#9)  & 46.91(39) & 69608 & 5560$\pm^{ 124 }_{ 134 }$ & $1$ & 20.2316 & 0.66 & 15.64 & -0.01\\ 
3c273 & $0.07359$ (\#10)  & 43.29(38) & 69608 & 5652$\pm^{ 130 }_{ 128 }$ & $1$ & 20.3553 & 1.24 & 15.85 & 1.54\\ 
3c273 & $0.13960$ (\#11)  & -- & -- & -- & -- & 21.6068 & -- & -- & --\\ 
h1821 & $0.00944$ (\#12)  & 38.66(39) & 470152 & 824$\pm^{ 14 }_{ 14 }$ & $1$ & 19.1390 & 0.37 & 15.44 & 0.75\\ 
h1821 & $0.06779$ (\#13)  & 39.35(38) & 470152 & 852$\pm^{ 16 }_{ 15 }$ & $1$ & 20.2453 & 1.33 & 15.87 & 7.79\\ 
h1821 & $0.08483$ (\#14)  & 44.68(39) & 470152 & 843$\pm^{ 16 }_{ 16 }$ & $1$ & 20.5684 & 0.41 & 15.46 & 0.39\\ 
h1821 & $0.12147$ (\#15)  & 42.69(31) & 470152 & 880$\pm^{ 20 }_{ 20 }$ & $1$ & 21.2631 & 0.51 & 15.56 & 0.00\\ 
h1821 & $0.19817$ (\#16)  & 49.67(39) & 470152 & 931$\pm^{ 22 }_{ 22 }$ & $1$ & 22.7173 & 1.17 & 15.83 & 2.27\\ 
h1821 & $0.21321$ (\#17)  & 35.27(35) & 470152 & 948$\pm^{ 23 }_{ 23 }$ & $1$ & 23.0025 & 0.54 & 15.58 & 0.93\\ 
h1821 & $0.24531$ (\#18)  & 32.59(30) & 470152 & 1130$\pm^{ 25 }_{ 24 }$ & $1$ & 23.6111 & 0.65 & 15.66 & 2.67\\ 
h2356 & $0.03830$ (\#19)  & 39.37(39) & 586697 & 2067$\pm^{ 29 }_{ 29 }$ & $1$ & 19.6862 & 0.33 & 15.39 & 2.38\\ 
h2356 & $0.07881$ (\#20)  & 40.55(38) & 586697 & 2087$\pm^{ 32 }_{ 32 }$ & $1$ & 20.4542 & 0.33 & 15.38 & 2.15\\ 
h2356 & $0.10467$ (\#21)  & 41.21(38) & 586697 & 2108$\pm^{ 31 }_{ 31 }$ & $1$ & 20.9445 & 0.45 & 15.50 & 0.00\\ 
h2356 & $0.15613$ (\#22)  & 28.52(30) & 586697 & 2138$\pm^{ 39 }_{ 39 }$ & $1$ & 21.9202 & 0.44 & 15.49 & 0.05\\ 
mr2251 & $0.01068$ (\#23)  & 31.54(39) & 78434 & 2573$\pm^{ 72 }_{ 70 }$ & $1$ & 19.1625 & 1.27 & 15.90 & 1.66\\ 
mr2251 & $0.01449$ (\#24)  & 25.42(39) & 78434 & 2473$\pm^{ 71 }_{ 70 }$ & $1$ & 19.2347 & 0.49 & 15.54 & 3.77\\ 
mr2251 & $0.06131$ (\#25)  & 43.48(38) & 78434 & 2702$\pm^{ 88 }_{ 86 }$ & $1$ & 20.1224 & 7.12 & 16.24 & 3.98\\ 
mr2251 & $0.06190$ (\#26)  & 43.84(39) & 78434 & 2700$\pm^{ 88 }_{ 86 }$ & $1$ & 20.1336 & 5.95 & 16.20 & 3.61\\ 
mr2251 & $0.06276$ (\#27)  & 43.50(38) & 78434 & 2697$\pm^{ 88 }_{ 86 }$ & $1$ & 20.1499 & 28.27 & 16.29 & 4.11\\ 
mr2251 & $0.06327$ (\#28)  & 43.55(39) & 78434 & 2707$\pm^{ 88 }_{ 87 }$ & $1$ & 20.1596 & 17.93 & 16.31 & 5.17\\ 
mr2251 & $0.06381$ (\#29)  & 41.59(38) & 78434 & 2714$\pm^{ 89 }_{ 87 }$ & $1$ & 20.1698 & 10.42 & 16.26 & 5.94\\ 
mrk478 & $0.06166$ (\#30)  & 37.08(38) & 80466 & 1284$\pm^{ 61 }_{ 60 }$ & $1$ & 20.1291 & 0.59 & 15.61 & 4.08\\ 
mrk478 & $0.06578$ (\#31)  & 38.24(39) & 80466 & 1328$\pm^{ 63 }_{ 61 }$ & $1$ & 20.2072 & 3.52 & 16.10 & 0.35\\ 
mrk478 & $0.07213$ (\#32)  & 34.86(38) & 80466 & 1330$\pm^{ 62 }_{ 60 }$ & $1$ & 20.3276 & 740.13 & 16.42 & 4.58\\ 
pg1116 & $0.04114$ (\#33)  & 38.61(39) & 355485 & 635$\pm^{ 27 }_{ 27 }$ & $1$ & 19.7400 & 2.34 & 16.05 & 0.34\\ 
pg1116 & $0.06251$ (\#34)  & 31.45(38) & 355485 & 631$\pm^{ 29 }_{ 28 }$ & $1$ & 20.1452 & 0.95 & 15.77 & 0.48\\ 
pg1116 & $0.08382$ (\#35)  & 36.50(38) & 355485 & 618$\pm^{ 30 }_{ 29 }$ & $1$ & 20.5492 & 1.11 & 15.85 & 0.34\\ 
pg1116 & $0.09210$ (\#36)  & 33.90(38) & 355485 & 632$\pm^{ 30 }_{ 30 }$ & $1$ & 20.7062 & 4.82 & 16.14 & 0.50\\ 
pg1116 & $0.09281$ (\#37)  & 33.80(38) & 355485 & 633$\pm^{ 30 }_{ 30 }$ & $1$ & 20.7197 & 5.23 & 16.16 & 0.61\\ 
pg1116 & $0.13373$ (\#38)  & 21.48(30) & 355485 & 757$\pm^{ 36 }_{ 36 }$ & $1$ & 21.4955 & 2.78 & 16.06 & 0.04\\ 
pg1116 & $0.13851$ (\#39)  & -- & -- & -- & -- & 21.5861 & -- & -- & --\\ 
pg1211 & $0.02586$ (\#40)  & 33.54(38) & 133595 & 1070$\pm^{ 37 }_{ 36 }$ & $1$ & 19.4503 & 1.60 & 15.97 & 1.73\\ 
pg1211 & $0.05443$ (\#41)  & 30.17(39) & 133595 & 1124$\pm^{ 41 }_{ 40 }$ & $1$ & 19.9920 & 0.56 & 15.58 & 2.25\\ 
pks0405 & $0.02510$ (\#42)  & 32.93(39) & 376096 & 432$\pm^{ 24 }_{ 23 }$ & $1$ & 19.4359 & 3.49 & 16.15 & 0.21\\ 
pks0405 & $0.05902$ (\#43)  & 31.53(38) & 376096 & 431$\pm^{ 29 }_{ 28 }$ & $1$ & 20.0790 & 19.18 & 16.33 & 0.37\\ 
pks0405 & $0.09719$ (\#44)  & 37.54(38) & 376096 & 470$\pm^{ 30 }_{ 30 }$ & $1$ & 20.8027 & 4.64E+03 & 16.52 & 3.80\\ 
pks0405 & $0.10152$ (\#45)  & 39.29(39) & 376096 & 462$\pm^{ 31 }_{ 30 }$ & $1$ & 20.8848 & 1.32 & 15.89 & 0.49\\ 
pks0405 & $0.10298$ (\#46)  & 33.14(39) & 376096 & 466$\pm^{ 31 }_{ 30 }$ & $1$ & 20.9125 & 88.66 & 16.32 & 0.38\\ 
pks0405 & $0.19456$ (\#47)  & 32.55(38) & 376096 & 514$\pm^{ 35 }_{ 35 }$ & $1$ & 22.6489 & 1.54 & 15.96 & 0.30\\ 
pks0405 & $0.21976$ (\#48)  & 37.95(38) & 376096 & 537$\pm^{ 36 }_{ 36 }$ & $1$ & 23.1266 & 100.75 & 16.35 & 0.41\\ 
pks0405 & $0.24564$ (\#49)  & 39.21(39) & 376096 & 487$\pm^{ 35 }_{ 35 }$ & $1$ & 23.6173 & 1.55 & 15.91 & 0.29\\ 
pks0405 & $0.29748$ (\#50)  & 42.61(38) & 376096 & 595$\pm^{ 38 }_{ 37 }$ & $1$ & 24.6002 & 77.94 & 16.32 & 0.37\\ 
pks0405 & $0.31016$ (\#51)  & 50.26(39) & 376096 & 547$\pm^{ 37 }_{ 37 }$ & $1$ & 24.8406 & 3.22E+03 & 16.49 & 1.07\\ 
pks0405 & $0.32502$ (\#52)  & 53.39(38) & 376096 & 543$\pm^{ 39 }_{ 37 }$ & $1$ & 25.1224 & 4.04 & 16.17 & 0.01\\ 
pks0405 & $0.49508$ (\#53)  & 40.12(38) & 376096 & 570$\pm^{ 45 }_{ 44 }$ & $1$ & 28.3467 & 1.53 & 15.93 & 0.46\\ 
pks2155 & $0.05708$ (\#54)  & 42.87(39) & 319334 & 13878$\pm^{ 90 }_{ 95 }$ & $1$ & 20.0422 & 0.20 & 15.18 & 0.09\\ 
pks2155 & $0.06236$ (\#55)  & 43.07(39) & 319334 & 13944$\pm^{ 92 }_{ 93 }$ & $1$ & 20.1423 & 0.18 & 15.15 & 0.14\\ 
pks2155 & $0.10586$ (\#56)  & 36.85(39) & 319334 & 14826$\pm^{ 95 }_{ 94 }$ & $1$ & 20.9671 & 0.22 & 15.21 & -0.04\\ 
tons180 & $0.04304$ (\#57)  & 24.70(38) & 76753 & 1560$\pm^{ 44 }_{ 43 }$ & $1$ & 19.7760 & 0.55 & 15.60 & 1.75\\ 





\hline
\hline
\end{longtable}
\end{landscape}

==> Tables/Chandra/Latex/chandra_o8_o6_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
%\footnotesize
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllll|l}
\caption[\chandra\ Data, \oviii\ With \ovi\ Priors Results (Full)]{\oviii\ measurements with \chandra\ data, at the prior redshift from the \ovi\ lines from Table~\ref{tab:oviPriorsTable}.}
\label{tab:chandraovioviii}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & \multicolumn{2}{c}{RGS1} & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \% $\frac{B}{D+B}$ & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.12314$ (\#1)  & 35.82(30) & 148933 & 23 & 1585$\pm^{ 62 }_{ 61 }$ & $1$ & 21.2947 & $ -0.79\pm^{ 0.77 }_{ 0.55 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.19\\ 
1es1028 & $0.13706$ (\#2)  & -- & -- & -- &  -- & -- & 21.5587 & -- & -- & --\\ 
1es1028 & $0.33735$ (\#3)  & 34.59(38) & 148933 & 24 & 1851$\pm^{ 66 }_{ 65 }$ & $1$ & 25.3562 & $ -0.24\pm^{ 1.24 }_{ 0.72 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.07\\ 
1es1553 & $0.18759$ (\#4)  & 43.76(33) & 495645 & 25 & 2462$\pm^{ 44 }_{ 44 }$ & $1$ & 22.5167 & $ 0.23\pm^{ 0.63 }_{ 0.47 }$ & $ 15.23\pm^{ 0.50 }_{ nan }$ & 0.23\\ 
1es1553 & $0.18775$ (\#5)  & 43.78(32) & 495645 & 25 & 2464$\pm^{ 44 }_{ 44 }$ & $1$ & 22.5197 & $ 0.24\pm^{ 0.63 }_{ 0.48 }$ & $ 15.25\pm^{ 0.48 }_{ nan }$ & 0.23\\ 
1es1553 & $0.18984$ (\#6)  & 40.55(33) & 495645 & 25 & 2490$\pm^{ 43 }_{ 43 }$ & $1$ & 22.5594 & $ 0.20\pm^{ 1.23 }_{ 0.76 }$ & $ 15.18\pm^{ 0.73 }_{ nan }$ & 0.06\\ 
1es1553 & $0.21631$ (\#7)  & 30.16(26) & 495645 & 24 & 2584$\pm^{ 53 }_{ 52 }$ & $1$ & 23.0612 & $ -0.45\pm^{ 0.44 }_{ 0.38 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.20\\ 
1es1553 & $0.31130$ (\#8)  & 50.56(39) & 495645 & 22 & 2998$\pm^{ 46 }_{ 44 }$ & $1$ & 24.8622 & $ -0.05\pm^{ 0.58 }_{ 0.33 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.03\\ 
1es1553 & $0.37868$ (\#9)  & 48.06(39) & 495645 & 23 & 3124$\pm^{ 49 }_{ 48 }$ & $1$ & 26.1398 & $ -0.37\pm^{ 0.41 }_{ 0.35 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.89\\ 
1es1553 & $0.39497$ (\#10)  & 41.84(38) & 495645 & 23 & 3095$\pm^{ 49 }_{ 49 }$ & $1$ & 26.4486 & $ -0.63\pm^{ 0.38 }_{ 0.33 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.79\\ 
h1821 & $0.02438$ (\#11)  & 37.76(38) & 470152 & 2 & 858$\pm^{ 15 }_{ 14 }$ & $1$ & 19.4222 & $ 0.63\pm^{ 0.63 }_{ 0.50 }$ & $ 15.63\pm^{ 0.24 }_{ 0.63 }$ & 1.80\\ 
h1821 & $0.10817$ (\#12)  & 44.34(38) & 470152 & 2 & 854$\pm^{ 17 }_{ 17 }$ & $1$ & 21.0109 & $ -0.90\pm^{ 0.39 }_{ 0.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.97\\ 
h1821 & $0.12133$ (\#13)  & 42.59(31) & 470152 & 2 & 879$\pm^{ 20 }_{ 20 }$ & $1$ & 21.2604 & $ -0.16\pm^{ 0.53 }_{ 0.45 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.12\\ 
h1821 & $0.12147$ (\#14)  & 42.69(31) & 470152 & 2 & 880$\pm^{ 20 }_{ 20 }$ & $1$ & 21.2631 & $ -0.03\pm^{ 0.54 }_{ 0.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
h1821 & $0.16992$ (\#15)  & 54.02(38) & 470152 & 2 & 895$\pm^{ 20 }_{ 20 }$ & $1$ & 22.1817 & $ 0.27\pm^{ 0.78 }_{ 0.56 }$ & $ 15.29\pm^{ 0.50 }_{ nan }$ & 0.20\\ 
h1821 & $0.17043$ (\#16)  & 53.61(38) & 470152 & 2 & 897$\pm^{ 20 }_{ 20 }$ & $1$ & 22.1914 & $ 0.48\pm^{ 0.83 }_{ 0.61 }$ & $ 15.53\pm^{ 0.34 }_{ nan }$ & 0.64\\ 
h1821 & $0.21326$ (\#17)  & 33.98(34) & 470152 & 2 & 944$\pm^{ 23 }_{ 23 }$ & $1$ & 23.0034 & $ -0.56\pm^{ 0.58 }_{ 0.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.99\\ 
h1821 & $0.22497$ (\#18)  & 38.17(32) & 470152 & 2 & 997$\pm^{ 24 }_{ 24 }$ & $1$ & 23.2254 & $ -0.67\pm^{ 0.43 }_{ 0.38 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.59\\ 
h1821 & $0.22522$ (\#19)  & 38.06(32) & 470152 & 2 & 997$\pm^{ 24 }_{ 24 }$ & $1$ & 23.2302 & $ -0.63\pm^{ 0.38 }_{ 0.32 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.71\\ 
h1821 & $0.22639$ (\#20)  & 38.11(32) & 470152 & 2 & 1000$\pm^{ 24 }_{ 24 }$ & $1$ & 23.2524 & $ -0.54\pm^{ 0.42 }_{ 0.36 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.78\\ 
h1821 & $0.24531$ (\#21)  & 38.80(33) & 470152 & 1 & 1114$\pm^{ 23 }_{ 23 }$ & $1$ & 23.6111 & $ 0.73\pm^{ 0.69 }_{ 0.56 }$ & $ 15.70\pm^{ 0.23 }_{ 0.58 }$ & 2.00\\ 
h1821 & $0.26657$ (\#22)  & 38.28(37) & 470152 & 1 & 1161$\pm^{ 22 }_{ 22 }$ & $1$ & 24.0142 & $ -0.26\pm^{ 0.46 }_{ 0.40 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.36\\ 
h1821 & $0.28800$ (\#23)  & 41.01(38) & 470152 & 1 & 1232$\pm^{ 23 }_{ 23 }$ & $1$ & 24.4205 & $ 0.65\pm^{ 0.75 }_{ 0.55 }$ & $ 15.64\pm^{ 0.25 }_{ 0.76 }$ & 1.56\\ 
h1821 & $0.29658$ (\#24)  & 36.87(39) & 470152 & 1 & 1194$\pm^{ 23 }_{ 22 }$ & $1$ & 24.5832 & $ -1.05\pm^{ 0.30 }_{ 0.26 }$ & $ nan\pm^{ nan }_{ nan }$ & 9.64\\ 
h1821 & $0.29680$ (\#25)  & 37.18(39) & 470152 & 1 & 1194$\pm^{ 23 }_{ 23 }$ & $1$ & 24.5873 & $ -1.13\pm^{ 0.35 }_{ 0.32 }$ & $ nan\pm^{ nan }_{ nan }$ & 9.31\\ 
h2356 & $0.11461$ (\#26)  & 31.02(33) & 586697 & 28 & 2121$\pm^{ 36 }_{ 35 }$ & $1$ & 21.1330 & $ 0.09\pm^{ 0.55 }_{ 0.42 }$ & $ 14.82\pm^{ 0.80 }_{ nan }$ & 0.04\\ 
h2356 & $0.16512$ (\#27)  & 28.36(34) & 586697 & 29 & 2145$\pm^{ 37 }_{ 37 }$ & $1$ & 22.0907 & $ 0.16\pm^{ 0.58 }_{ 0.45 }$ & $ 15.10\pm^{ 0.60 }_{ nan }$ & 0.13\\ 
mr2251 & $0.01070$ (\#28)  & 31.58(39) & 78434 & 12 & 2572$\pm^{ 71 }_{ 70 }$ & $1$ & 19.1629 & $ 1.15\pm^{ 1.55 }_{ 0.99 }$ & $ 15.86\pm^{ 0.25 }_{ 0.76 }$ & 1.61\\ 
pg1116 & $0.05900$ (\#29)  & 33.05(38) & 355485 & 54 & 617$\pm^{ 29 }_{ 28 }$ & $1$ & 20.0786 & $ 0.41\pm^{ 3.40 }_{ 1.22 }$ & $ 15.47\pm^{ 0.67 }_{ nan }$ & 0.08\\ 
pg1116 & $0.05927$ (\#30)  & 31.93(39) & 355485 & 54 & 629$\pm^{ 29 }_{ 28 }$ & $1$ & 20.0838 & $ 0.46\pm^{ 3.09 }_{ 1.21 }$ & $ 15.51\pm^{ 0.61 }_{ nan }$ & 0.11\\ 
pg1116 & $0.11895$ (\#31)  & 26.57(31) & 355485 & 55 & 654$\pm^{ 34 }_{ 35 }$ & $1$ & 21.2153 & $ 0.06\pm^{ 2.25 }_{ 1.09 }$ & $ 14.71\pm^{ 1.34 }_{ nan }$ & 0.00\\ 
pg1116 & $0.13852$ (\#32)  & -- & -- & -- &  -- & -- & 21.5863 & -- & -- & --\\ 
pg1116 & $0.16539$ (\#33)  & 31.16(34) & 355485 & 52 & 773$\pm^{ 36 }_{ 35 }$ & $1$ & 22.0958 & $ -0.80\pm^{ 1.05 }_{ 0.66 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.73\\ 
pg1116 & $0.16554$ (\#34)  & 31.18(34) & 355485 & 52 & 774$\pm^{ 36 }_{ 36 }$ & $1$ & 22.0986 & $ -0.83\pm^{ 1.08 }_{ 0.77 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.72\\ 
pg1116 & $0.16610$ (\#35)  & 31.39(35) & 355485 & 52 & 775$\pm^{ 36 }_{ 35 }$ & $1$ & 22.1093 & $ -0.68\pm^{ 1.15 }_{ 0.73 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.49\\ 
pg1116 & $0.16686$ (\#36)  & 31.82(35) & 355485 & 52 & 782$\pm^{ 36 }_{ 35 }$ & $1$ & 22.1237 & $ -0.09\pm^{ 1.64 }_{ 1.00 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pg1116 & $0.17343$ (\#37)  & 35.93(38) & 355485 & 53 & 762$\pm^{ 34 }_{ 34 }$ & $1$ & 22.2482 & $ -0.25\pm^{ 1.49 }_{ 0.93 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.05\\ 
pg1211 & $0.00711$ (\#38)  & 42.02(38) & 133595 & 1 & 998$\pm^{ 34 }_{ 33 }$ & $1$ & 19.0948 & $ 0.63\pm^{ 1.71 }_{ 0.91 }$ & $ 15.62\pm^{ 0.39 }_{ nan }$ & 0.44\\ 
pg1211 & $0.05117$ (\#39)  & 30.00(38) & 133595 & 1 & 1107$\pm^{ 40 }_{ 39 }$ & $1$ & 19.9302 & $ -0.28\pm^{ 0.99 }_{ 0.65 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.12\\ 
pg1211 & $0.06449$ (\#40)  & 33.49(39) & 133595 & 1 & 1148$\pm^{ 42 }_{ 41 }$ & $1$ & 20.1827 & $ -0.36\pm^{ 0.92 }_{ 0.63 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.21\\ 
pg1211 & $0.06491$ (\#41)  & 33.15(39) & 133595 & 1 & 1145$\pm^{ 42 }_{ 41 }$ & $1$ & 20.1907 & $ -0.58\pm^{ 0.83 }_{ 0.62 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.58\\ 
pks0405 & $0.09192$ (\#42)  & 40.79(38) & 376096 & 68 & 455$\pm^{ 31 }_{ 30 }$ & $1$ & 20.7028 & $ 0.68\pm^{ 15.16 }_{ 1.73 }$ & $ 15.66\pm^{ 0.63 }_{ nan }$ & 0.10\\ 
pks0405 & $0.09647$ (\#43)  & 39.78(39) & 376096 & 68 & 467$\pm^{ 30 }_{ 30 }$ & $1$ & 20.7891 & $ 3.79\pm^{ 2.39E+03 }_{ 3.59 }$ & $ 16.17\pm^{ 0.36 }_{ 0.98 }$ & 1.33\\ 
pks0405 & $0.14808$ (\#44)  & 25.19(31) & 376096 & 69 & 472$\pm^{ 37 }_{ 37 }$ & $1$ & 21.7676 & $ 3.60\pm^{ 41.40 }_{ 4.08 }$ & $ 16.10\pm^{ 0.32 }_{ nan }$ & 0.66\\ 
pks0405 & $0.16566$ (\#45)  & 27.87(34) & 376096 & 68 & 471$\pm^{ 35 }_{ 34 }$ & $1$ & 22.1009 & $ -1.37\pm^{ 1.55 }_{ 0.99 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.92\\ 
pks0405 & $0.16606$ (\#46)  & 28.23(35) & 376096 & 68 & 474$\pm^{ 35 }_{ 34 }$ & $1$ & 22.1085 & $ -1.06\pm^{ 1.74 }_{ 0.89 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.57\\ 
pks0405 & $0.16659$ (\#47)  & 28.80(35) & 376096 & 68 & 479$\pm^{ 34 }_{ 34 }$ & $1$ & 22.1185 & $ -0.71\pm^{ 2.38 }_{ 0.96 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.23\\ 
pks0405 & $0.16688$ (\#48)  & 28.85(35) & 376096 & 68 & 480$\pm^{ 35 }_{ 35 }$ & $1$ & 22.1240 & $ -0.65\pm^{ 2.34 }_{ 1.23 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.16\\ 
pks0405 & $0.16712$ (\#49)  & 28.91(35) & 376096 & 68 & 481$\pm^{ 35 }_{ 34 }$ & $1$ & 22.1286 & $ -0.53\pm^{ 2.71 }_{ 1.10 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.10\\ 
pks0405 & $0.18257$ (\#50)  & 32.17(38) & 376096 & 68 & 522$\pm^{ 34 }_{ 34 }$ & $1$ & 22.4215 & $ 22.05\pm^{ 1.84E+06 }_{ 20.83 }$ & $ 16.33\pm^{ 0.28 }_{ 0.47 }$ & 2.54\\ 
pks0405 & $0.18289$ (\#51)  & 31.77(38) & 376096 & 68 & 525$\pm^{ 35 }_{ 34 }$ & $1$ & 22.4276 & $ 202.85\pm^{ 1.38E+07 }_{ 200.07 }$ & $ 16.43\pm^{ 0.20 }_{ 0.34 }$ & 3.03\\ 
pks0405 & $0.24052$ (\#52)  & 33.13(38) & 376096 & 68 & 525$\pm^{ 36 }_{ 35 }$ & $1$ & 23.5203 & $ 37.40\pm^{ 1.39E+06 }_{ 34.36 }$ & $ 16.40\pm^{ 0.25 }_{ 0.32 }$ & 3.46\\ 
pks0405 & $0.24094$ (\#53)  & 32.74(38) & 376096 & 68 & 527$\pm^{ 36 }_{ 35 }$ & $1$ & 23.5282 & $ 318.70\pm^{ 1.41E+07 }_{ 310.60 }$ & $ 16.45\pm^{ 0.21 }_{ 0.20 }$ & 3.93\\ 
pks0405 & $0.24547$ (\#54)  & 39.22(39) & 376096 & 69 & 487$\pm^{ 36 }_{ 35 }$ & $1$ & 23.6141 & $ -0.83\pm^{ 2.07 }_{ 1.10 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.28\\ 
pks0405 & $0.29762$ (\#55)  & 42.66(38) & 376096 & 66 & 595$\pm^{ 38 }_{ 38 }$ & $1$ & 24.6029 & $ 1.38\pm^{ 34.30 }_{ 2.09 }$ & $ 15.90\pm^{ 0.44 }_{ nan }$ & 0.32\\ 
pks0405 & $0.34188$ (\#56)  & 40.28(39) & 376096 & 68 & 552$\pm^{ 39 }_{ 38 }$ & $1$ & 25.4420 & $ 2.15\pm^{ 36.43 }_{ 2.78 }$ & $ 16.00\pm^{ 0.39 }_{ nan }$ & 0.45\\ 
pks0405 & $0.34225$ (\#57)  & 41.57(38) & 376096 & 68 & 540$\pm^{ 38 }_{ 38 }$ & $1$ & 25.4491 & $ 1.27\pm^{ 157.44 }_{ 2.16 }$ & $ 15.90\pm^{ 0.47 }_{ nan }$ & 0.26\\ 
pks0405 & $0.35092$ (\#58)  & 43.57(39) & 376096 & 70 & 504$\pm^{ 38 }_{ 38 }$ & $1$ & 25.6134 & $ -1.24\pm^{ 1.65 }_{ 0.91 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.75\\ 
pks0405 & $0.36075$ (\#59)  & 24.67(38) & 376096 & 69 & 526$\pm^{ 39 }_{ 38 }$ & $1$ & 25.7998 & $ -1.81\pm^{ 1.29 }_{ 0.90 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.84\\ 
pks0405 & $0.36151$ (\#60)  & 25.83(39) & 376096 & 68 & 534$\pm^{ 39 }_{ 38 }$ & $1$ & 25.8142 & $ -1.10\pm^{ 1.80 }_{ 1.03 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.53\\ 
pks0405 & $0.36329$ (\#61)  & 31.24(38) & 376096 & 69 & 545$\pm^{ 39 }_{ 38 }$ & $1$ & 25.8480 & $ -0.25\pm^{ 3.44 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
pks0405 & $0.40570$ (\#62)  & 41.81(38) & 376096 & 68 & 614$\pm^{ 42 }_{ 41 }$ & $1$ & 26.6521 & $ 1.10\pm^{ 85.63 }_{ 1.96 }$ & $ 15.84\pm^{ 0.52 }_{ nan }$ & 0.23\\ 
pks0405 & $0.40890$ (\#63)  & 39.69(39) & 376096 & 68 & 624$\pm^{ 45 }_{ 40 }$ & $1$ & 26.7127 & $ 26.09\pm^{ 3.07E+07 }_{ 23.51 }$ & $ 16.29\pm^{ 0.30 }_{ 0.19 }$ & 2.91\\ 
pks0405 & $0.49505$ (\#64)  & 40.12(38) & 376096 & 71 & 570$\pm^{ 45 }_{ 44 }$ & $1$ & 28.3461 & $ -1.06\pm^{ 2.05 }_{ 0.96 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.47\\ 
pks0405 & $0.49530$ (\#65)  & 40.23(38) & 376096 & 71 & 571$\pm^{ 45 }_{ 44 }$ & $1$ & 28.3509 & $ -1.00\pm^{ 2.23 }_{ 1.19 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.34\\ 
pks0405 & $0.55506$ (\#66)  & 33.01(39) & 376096 & 74 & 545$\pm^{ 50 }_{ 49 }$ & $1$ & 29.4839 & $ -0.77\pm^{ 4.84 }_{ 1.25 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.14\\ 
pks2005 & $0.06490$ (\#67)  & 35.04(39) & 282191 & 1 & 1757$\pm^{ 42 }_{ 41 }$ & $1$ & 20.1905 & $ -0.44\pm^{ 0.55 }_{ 0.45 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.71\\ 
tons180 & $0.02340$ (\#68)  & 38.98(38) & 76753 & 1 & 1528$\pm^{ 42 }_{ 41 }$ & $1$ & 19.4037 & $ -0.36\pm^{ 0.66 }_{ 0.52 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.36\\ 
tons180 & $0.04360$ (\#69)  & 26.47(39) & 76753 & 1 & 1554$\pm^{ 44 }_{ 43 }$ & $1$ & 19.7867 & $ -0.81\pm^{ 0.59 }_{ 0.51 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.91\\ 
tons180 & $0.04560$ (\#70)  & 28.12(38) & 76753 & 1 & 1572$\pm^{ 44 }_{ 44 }$ & $1$ & 19.8246 & $ -0.06\pm^{ 0.81 }_{ 0.64 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
3c273 & $0.00337$ (\#71)  & 46.56(38) & 69608 & 6 & 5095$\pm^{ 100 }_{ 98 }$ & $1$ & 19.0239 & $ 1.31\pm^{ 1.06 }_{ 0.75 }$ & $ 15.91\pm^{ 0.17 }_{ 0.30 }$ & 4.12\\ 
3c273 & $0.00533$ (\#72)  & 48.67(39) & 69608 & 6 & 5091$\pm^{ 100 }_{ 99 }$ & $1$ & 19.0611 & $ 1.27\pm^{ 1.07 }_{ 0.75 }$ & $ 15.89\pm^{ 0.18 }_{ 0.32 }$ & 3.85\\ 
3c273 & $0.00764$ (\#73)  & 49.34(38) & 69608 & 6 & 5102$\pm^{ 102 }_{ 100 }$ & $1$ & 19.1049 & $ 1.21\pm^{ 1.39 }_{ 0.83 }$ & $ 15.84\pm^{ 0.20 }_{ 0.41 }$ & 2.91\\ 
3c273 & $0.02947$ (\#74)  & 26.95(24) & 69608 & 7 & 5335$\pm^{ 146 }_{ 144 }$ & $1$ & 19.5188 & $ -0.28\pm^{ 0.64 }_{ 0.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.27\\ 
3c273 & $0.04898$ (\#75)  & 40.99(39) & 69608 & 7 & 5480$\pm^{ 125 }_{ 122 }$ & $1$ & 19.8887 & $ -1.55\pm^{ 0.39 }_{ 0.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 12.07\\ 
3c273 & $0.06655$ (\#76)  & 44.57(38) & 69608 & 8 & 5539$\pm^{ 132 }_{ 124 }$ & $1$ & 20.2218 & $ -0.04\pm^{ 0.84 }_{ 0.53 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.01\\ 
3c273 & $0.09018$ (\#77)  & 29.87(38) & 69608 & 8 & 5748$\pm^{ 134 }_{ 131 }$ & $1$ & 20.6698 & $ 3.34\pm^{ 4.82 }_{ 2.01 }$ & $ 16.09\pm^{ 0.14 }_{ 0.22 }$ & 6.58\\ 
3c273 & $0.12007$ (\#78)  & 34.40(31) & 69608 & 7 & 5957$\pm^{ 156 }_{ 154 }$ & $1$ & 21.2365 & $ 1.69\pm^{ 1.76 }_{ 1.05 }$ & $ 15.98\pm^{ 0.18 }_{ 0.33 }$ & 3.75\\ 
3c273 & $0.14660$ (\#79)  & 31.78(31) & 69608 & 8 & 5708$\pm^{ 157 }_{ 153 }$ & $1$ & 21.7395 & $ -0.36\pm^{ 0.69 }_{ 0.55 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.34\\ 
3c273 & $0.15784$ (\#80)  & 26.34(30) & 69608 & 8 & 5883$\pm^{ 161 }_{ 158 }$ & $1$ & 21.9526 & $ 1.60\pm^{ 1.95 }_{ 1.09 }$ & $ 15.95\pm^{ 0.19 }_{ 0.40 }$ & 3.00\\ 
mrk421 & $0.01009$ (\#81)  & 28.92(9) & 638847 & 1 & 1273$\pm^{ 5 }_{ 5 }$ & $1$ & 19.1513 & $ 0.09\pm^{ 0.08 }_{ 0.05 }$ & $ 14.84\pm^{ 0.26 }_{ 0.36 }$ & 3.66\\ 
pks2155 & $0.05405$ (\#82)  & 50.63(39) & 319334 & 4 & 13905$\pm^{ 93 }_{ 91 }$ & $1$ & 19.9848 & $ 0.15\pm^{ 0.22 }_{ 0.19 }$ & $ 15.08\pm^{ 0.36 }_{ nan }$ & 0.73\\ 
pks2155 & $0.05707$ (\#83)  & 42.86(39) & 319334 & 4 & 13877$\pm^{ 90 }_{ 91 }$ & $1$ & 20.0420 & $ 0.07\pm^{ 0.20 }_{ 0.20 }$ & $ 14.75\pm^{ 0.55 }_{ nan }$ & 0.10\\ 


\hline
\hline
 \end{longtable}
%\end{small}
\end{landscape}

==> Tables/Chandra/Latex/chandra_o8_o6_uppers_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\footnotesize
\begin{landscape}
\begin{longtable}{cc|lllllll|l}
\caption[\chandra\ Data, \oviii\ Upper Limits With \ovi\ Priors Results (Full)]{\oviii\ upper limit measurements with \chandra\ data, at the prior redshift from the \ovi\ lines from Table~\ref{tab:oviPriorsTable}.}
\label{tab:chandraovioviiiuppers}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & RGS1 & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N + (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.12314$ (\#1)  & 35.82(30) & 148933 & 1585$\pm^{ 62 }_{ 61 }$ & $1$ & 21.2947 & 0.66 & 15.64 & 1.19\\ 
1es1028 & $0.13706$ (\#2)  & -- & -- & -- & -- & 21.5587 & -- & -- & --\\ 
1es1028 & $0.33735$ (\#3)  & 34.59(38) & 148933 & 1851$\pm^{ 66 }_{ 65 }$ & $1$ & 25.3562 & 0.98 & 15.77 & 0.07\\ 
1es1553 & $0.18759$ (\#4)  & 43.76(33) & 495645 & 2462$\pm^{ 44 }_{ 44 }$ & $1$ & 22.5167 & 0.55 & 15.58 & 0.23\\ 
1es1553 & $0.18775$ (\#5)  & 43.78(32) & 495645 & 2464$\pm^{ 44 }_{ 44 }$ & $1$ & 22.5197 & 0.56 & 15.58 & 0.23\\ 
1es1553 & $0.18984$ (\#6)  & 40.55(33) & 495645 & 2490$\pm^{ 43 }_{ 43 }$ & $1$ & 22.5594 & 0.99 & 15.80 & 0.06\\ 
1es1553 & $0.21631$ (\#7)  & 30.16(26) & 495645 & 2584$\pm^{ 53 }_{ 52 }$ & $1$ & 23.0612 & 0.41 & 15.48 & 1.20\\ 
1es1553 & $0.31130$ (\#8)  & 50.56(39) & 495645 & 2998$\pm^{ 46 }_{ 44 }$ & $1$ & 24.8622 & 0.45 & 15.52 & -0.03\\ 
1es1553 & $0.37868$ (\#9)  & 48.06(39) & 495645 & 3124$\pm^{ 49 }_{ 48 }$ & $1$ & 26.1398 & 0.38 & 15.45 & 0.89\\ 
1es1553 & $0.39497$ (\#10)  & 41.84(38) & 495645 & 3095$\pm^{ 49 }_{ 49 }$ & $1$ & 26.4486 & 0.35 & 15.42 & 2.79\\ 
h1821 & $0.02438$ (\#11)  & 37.76(38) & 470152 & 858$\pm^{ 15 }_{ 14 }$ & $1$ & 19.4222 & 0.56 & 15.59 & 1.80\\ 
h1821 & $0.10817$ (\#12)  & 44.34(38) & 470152 & 854$\pm^{ 17 }_{ 17 }$ & $1$ & 21.0109 & 0.37 & 15.43 & 4.97\\ 
h1821 & $0.12133$ (\#13)  & 42.59(31) & 470152 & 879$\pm^{ 20 }_{ 20 }$ & $1$ & 21.2604 & 0.49 & 15.55 & 0.12\\ 
h1821 & $0.12147$ (\#14)  & 42.69(31) & 470152 & 880$\pm^{ 20 }_{ 20 }$ & $1$ & 21.2631 & 0.51 & 15.56 & 0.00\\ 
h1821 & $0.16992$ (\#15)  & 54.02(38) & 470152 & 895$\pm^{ 20 }_{ 20 }$ & $1$ & 22.1817 & 0.67 & 15.65 & 0.20\\ 
h1821 & $0.17043$ (\#16)  & 53.61(38) & 470152 & 897$\pm^{ 20 }_{ 20 }$ & $1$ & 22.1914 & 0.72 & 15.68 & 0.64\\ 
h1821 & $0.21326$ (\#17)  & 33.98(34) & 470152 & 944$\pm^{ 23 }_{ 23 }$ & $1$ & 23.0034 & 0.52 & 15.57 & 0.99\\ 
h1821 & $0.22497$ (\#18)  & 38.17(32) & 470152 & 997$\pm^{ 24 }_{ 24 }$ & $1$ & 23.2254 & 0.40 & 15.47 & 2.59\\ 
h1821 & $0.22522$ (\#19)  & 38.06(32) & 470152 & 997$\pm^{ 24 }_{ 24 }$ & $1$ & 23.2302 & 0.35 & 15.41 & 2.71\\ 
h1821 & $0.22639$ (\#20)  & 38.11(32) & 470152 & 1000$\pm^{ 24 }_{ 24 }$ & $1$ & 23.2524 & 0.39 & 15.46 & 1.78\\ 
h1821 & $0.24531$ (\#21)  & 38.80(33) & 470152 & 1114$\pm^{ 23 }_{ 23 }$ & $1$ & 23.6111 & 0.63 & 15.64 & 2.00\\ 
h1821 & $0.26657$ (\#22)  & 38.28(37) & 470152 & 1161$\pm^{ 22 }_{ 22 }$ & $1$ & 24.0142 & 0.43 & 15.49 & 0.36\\ 
h1821 & $0.28800$ (\#23)  & 41.01(38) & 470152 & 1232$\pm^{ 23 }_{ 23 }$ & $1$ & 24.4205 & 0.65 & 15.64 & 1.56\\ 
h1821 & $0.29658$ (\#24)  & 36.87(39) & 470152 & 1194$\pm^{ 23 }_{ 22 }$ & $1$ & 24.5832 & 0.28 & 15.32 & 9.64\\ 
h1821 & $0.29680$ (\#25)  & 37.18(39) & 470152 & 1194$\pm^{ 23 }_{ 23 }$ & $1$ & 24.5873 & 0.33 & 15.40 & 9.31\\ 
h2356 & $0.11461$ (\#26)  & 31.02(33) & 586697 & 2121$\pm^{ 36 }_{ 35 }$ & $1$ & 21.1330 & 0.48 & 15.53 & 0.04\\ 
h2356 & $0.16512$ (\#27)  & 28.36(34) & 586697 & 2145$\pm^{ 37 }_{ 37 }$ & $1$ & 22.0907 & 0.52 & 15.56 & 0.13\\ 
mr2251 & $0.01070$ (\#28)  & 31.58(39) & 78434 & 2572$\pm^{ 71 }_{ 70 }$ & $1$ & 19.1629 & 1.27 & 15.90 & 1.61\\ 
pg1116 & $0.05900$ (\#29)  & 33.05(38) & 355485 & 617$\pm^{ 29 }_{ 28 }$ & $1$ & 20.0786 & 2.31 & 16.03 & 0.08\\ 
pg1116 & $0.05927$ (\#30)  & 31.93(39) & 355485 & 629$\pm^{ 29 }_{ 28 }$ & $1$ & 20.0838 & 2.15 & 16.01 & 0.11\\ 
pg1116 & $0.11895$ (\#31)  & 26.57(31) & 355485 & 654$\pm^{ 34 }_{ 35 }$ & $1$ & 21.2153 & 1.67 & 15.96 & 0.00\\ 
pg1116 & $0.13852$ (\#32)  & -- & -- & -- & -- & 21.5863 & -- & -- & --\\ 
pg1116 & $0.16539$ (\#33)  & 31.16(34) & 355485 & 773$\pm^{ 36 }_{ 35 }$ & $1$ & 22.0958 & 0.86 & 15.74 & 0.73\\ 
pg1116 & $0.16554$ (\#34)  & 31.18(34) & 355485 & 774$\pm^{ 36 }_{ 36 }$ & $1$ & 22.0986 & 0.93 & 15.79 & 0.72\\ 
pg1116 & $0.16610$ (\#35)  & 31.39(35) & 355485 & 775$\pm^{ 36 }_{ 35 }$ & $1$ & 22.1093 & 0.94 & 15.78 & 0.49\\ 
pg1116 & $0.16686$ (\#36)  & 31.82(35) & 355485 & 782$\pm^{ 36 }_{ 35 }$ & $1$ & 22.1237 & 1.32 & 15.91 & 0.01\\ 
pg1116 & $0.17343$ (\#37)  & 35.93(38) & 355485 & 762$\pm^{ 34 }_{ 34 }$ & $1$ & 22.2482 & 1.21 & 15.87 & 0.05\\ 
pg1211 & $0.00711$ (\#38)  & 42.02(38) & 133595 & 998$\pm^{ 34 }_{ 33 }$ & $1$ & 19.0948 & 1.31 & 15.86 & 0.44\\ 
pg1211 & $0.05117$ (\#39)  & 30.00(38) & 133595 & 1107$\pm^{ 40 }_{ 39 }$ & $1$ & 19.9302 & 0.82 & 15.72 & 0.12\\ 
pg1211 & $0.06449$ (\#40)  & 33.49(39) & 133595 & 1148$\pm^{ 42 }_{ 41 }$ & $1$ & 20.1827 & 0.78 & 15.70 & 0.21\\ 
pg1211 & $0.06491$ (\#41)  & 33.15(39) & 133595 & 1145$\pm^{ 42 }_{ 41 }$ & $1$ & 20.1907 & 0.72 & 15.68 & 0.58\\ 
pks0405 & $0.09192$ (\#42)  & 40.79(38) & 376096 & 455$\pm^{ 31 }_{ 30 }$ & $1$ & 20.7028 & 8.45 & 16.26 & 0.10\\ 
pks0405 & $0.09647$ (\#43)  & 39.78(39) & 376096 & 467$\pm^{ 30 }_{ 30 }$ & $1$ & 20.7891 & 1.20E+03 & 16.50 & 1.33\\ 
pks0405 & $0.14808$ (\#44)  & 25.19(31) & 376096 & 472$\pm^{ 37 }_{ 37 }$ & $1$ & 21.7676 & 22.74 & 16.36 & 0.66\\ 
pks0405 & $0.16566$ (\#45)  & 27.87(34) & 376096 & 471$\pm^{ 35 }_{ 34 }$ & $1$ & 22.1009 & 1.27 & 15.90 & 0.92\\ 
pks0405 & $0.16606$ (\#46)  & 28.23(35) & 376096 & 474$\pm^{ 35 }_{ 34 }$ & $1$ & 22.1085 & 1.31 & 15.87 & 0.57\\ 
pks0405 & $0.16659$ (\#47)  & 28.80(35) & 376096 & 479$\pm^{ 34 }_{ 34 }$ & $1$ & 22.1185 & 1.67 & 15.93 & 0.23\\ 
pks0405 & $0.16688$ (\#48)  & 28.85(35) & 376096 & 480$\pm^{ 35 }_{ 35 }$ & $1$ & 22.1240 & 1.79 & 16.00 & 0.16\\ 
pks0405 & $0.16712$ (\#49)  & 28.91(35) & 376096 & 481$\pm^{ 35 }_{ 34 }$ & $1$ & 22.1286 & 1.90 & 15.98 & 0.10\\ 
pks0405 & $0.18257$ (\#50)  & 32.17(38) & 376096 & 522$\pm^{ 34 }_{ 34 }$ & $1$ & 22.4215 & 9.18E+05 & 16.59 & 2.54\\ 
pks0405 & $0.18289$ (\#51)  & 31.77(38) & 376096 & 525$\pm^{ 35 }_{ 34 }$ & $1$ & 22.4276 & 6.92E+06 & 16.61 & 3.03\\ 
pks0405 & $0.24052$ (\#52)  & 33.13(38) & 376096 & 525$\pm^{ 36 }_{ 35 }$ & $1$ & 23.5203 & 6.97E+05 & 16.62 & 3.46\\ 
pks0405 & $0.24094$ (\#53)  & 32.74(38) & 376096 & 527$\pm^{ 36 }_{ 35 }$ & $1$ & 23.5282 & 7.03E+06 & 16.64 & 3.93\\ 
pks0405 & $0.24547$ (\#54)  & 39.22(39) & 376096 & 487$\pm^{ 36 }_{ 35 }$ & $1$ & 23.6141 & 1.59 & 15.96 & 0.28\\ 
pks0405 & $0.29762$ (\#55)  & 42.66(38) & 376096 & 595$\pm^{ 38 }_{ 38 }$ & $1$ & 24.6029 & 18.19 & 16.31 & 0.32\\ 
pks0405 & $0.34188$ (\#56)  & 40.28(39) & 376096 & 552$\pm^{ 39 }_{ 38 }$ & $1$ & 25.4420 & 19.60 & 16.34 & 0.45\\ 
pks0405 & $0.34225$ (\#57)  & 41.57(38) & 376096 & 540$\pm^{ 38 }_{ 38 }$ & $1$ & 25.4491 & 79.80 & 16.33 & 0.26\\ 
pks0405 & $0.35092$ (\#58)  & 43.57(39) & 376096 & 504$\pm^{ 38 }_{ 38 }$ & $1$ & 25.6134 & 1.28 & 15.87 & 0.75\\ 
pks0405 & $0.36075$ (\#59)  & 24.67(38) & 376096 & 526$\pm^{ 39 }_{ 38 }$ & $1$ & 25.7998 & 1.10 & 15.85 & 1.84\\ 
pks0405 & $0.36151$ (\#60)  & 25.83(39) & 376096 & 534$\pm^{ 39 }_{ 38 }$ & $1$ & 25.8142 & 1.42 & 15.92 & 0.53\\ 
pks0405 & $0.36329$ (\#61)  & 31.24(38) & 376096 & 545$\pm^{ 39 }_{ 38 }$ & $1$ & 25.8480 & 2.39 & 16.07 & 0.02\\ 
pks0405 & $0.40570$ (\#62)  & 41.81(38) & 376096 & 614$\pm^{ 42 }_{ 41 }$ & $1$ & 26.6521 & 43.80 & 16.33 & 0.23\\ 
pks0405 & $0.40890$ (\#63)  & 39.69(39) & 376096 & 624$\pm^{ 45 }_{ 40 }$ & $1$ & 26.7127 & 1.54E+07 & 16.58 & 2.91\\ 
pks0405 & $0.49505$ (\#64)  & 40.12(38) & 376096 & 570$\pm^{ 45 }_{ 44 }$ & $1$ & 28.3461 & 1.50 & 15.92 & 0.47\\ 
pks0405 & $0.49530$ (\#65)  & 40.23(38) & 376096 & 571$\pm^{ 45 }_{ 44 }$ & $1$ & 28.3509 & 1.71 & 15.99 & 0.34\\ 
pks0405 & $0.55506$ (\#66)  & 33.01(39) & 376096 & 545$\pm^{ 50 }_{ 49 }$ & $1$ & 29.4839 & 3.04 & 16.09 & 0.14\\ 
pks2005 & $0.06490$ (\#67)  & 35.04(39) & 282191 & 1757$\pm^{ 42 }_{ 41 }$ & $1$ & 20.1905 & 0.50 & 15.55 & 0.71\\ 
tons180 & $0.02340$ (\#68)  & 38.98(38) & 76753 & 1528$\pm^{ 42 }_{ 41 }$ & $1$ & 19.4037 & 0.59 & 15.61 & 0.36\\ 
tons180 & $0.04360$ (\#69)  & 26.47(39) & 76753 & 1554$\pm^{ 44 }_{ 43 }$ & $1$ & 19.7867 & 0.55 & 15.59 & 1.91\\ 
tons180 & $0.04560$ (\#70)  & 28.12(38) & 76753 & 1572$\pm^{ 44 }_{ 44 }$ & $1$ & 19.8246 & 0.73 & 15.70 & 0.01\\ 
3c273 & $0.00337$ (\#71)  & 46.56(38) & 69608 & 5095$\pm^{ 100 }_{ 98 }$ & $1$ & 19.0239 & 0.91 & 15.78 & 4.12\\ 
3c273 & $0.00533$ (\#72)  & 48.67(39) & 69608 & 5091$\pm^{ 100 }_{ 99 }$ & $1$ & 19.0611 & 0.91 & 15.78 & 3.85\\ 
3c273 & $0.00764$ (\#73)  & 49.34(38) & 69608 & 5102$\pm^{ 102 }_{ 100 }$ & $1$ & 19.1049 & 1.11 & 15.82 & 2.91\\ 
3c273 & $0.02947$ (\#74)  & 26.95(24) & 69608 & 5335$\pm^{ 146 }_{ 144 }$ & $1$ & 19.5188 & 0.55 & 15.58 & 0.27\\ 
3c273 & $0.04898$ (\#75)  & 40.99(39) & 69608 & 5480$\pm^{ 125 }_{ 122 }$ & $1$ & 19.8887 & 0.37 & 15.43 & 12.07\\ 
3c273 & $0.06655$ (\#76)  & 44.57(38) & 69608 & 5539$\pm^{ 132 }_{ 124 }$ & $1$ & 20.2218 & 0.68 & 15.66 & -0.01\\ 
3c273 & $0.09018$ (\#77)  & 29.87(38) & 69608 & 5748$\pm^{ 134 }_{ 131 }$ & $1$ & 20.6698 & 3.41 & 16.09 & 6.58\\ 
3c273 & $0.12007$ (\#78)  & 34.40(31) & 69608 & 5957$\pm^{ 156 }_{ 154 }$ & $1$ & 21.2365 & 1.40 & 15.93 & 3.75\\ 
3c273 & $0.14660$ (\#79)  & 31.78(31) & 69608 & 5708$\pm^{ 157 }_{ 153 }$ & $1$ & 21.7395 & 0.62 & 15.63 & 0.34\\ 
3c273 & $0.15784$ (\#80)  & 26.34(30) & 69608 & 5883$\pm^{ 161 }_{ 158 }$ & $1$ & 21.9526 & 1.52 & 15.94 & 3.00\\ 
mrk421 & $0.01009$ (\#81)  & 28.92(9) & 638847 & 1273$\pm^{ 5 }_{ 5 }$ & $1$ & 19.1513 & 0.06 & 14.70 & 3.66\\ 
pks2155 & $0.05405$ (\#82)  & 50.63(39) & 319334 & 13905$\pm^{ 93 }_{ 91 }$ & $1$ & 19.9848 & 0.21 & 15.20 & 0.73\\ 
pks2155 & $0.05707$ (\#83)  & 42.86(39) & 319334 & 13877$\pm^{ 90 }_{ 91 }$ & $1$ & 20.0420 & 0.20 & 15.18 & 0.10\\ 

\hline
\hline
\end{longtable}
\end{landscape}

==> Tables/Priors/hipriors_full.tex <==
\renewcommand{\arraystretch}{.6}
\setlength\LTleft{1cm}
\begin{longtable}{lllccccc}
\caption[\hi\ \bla\ Prior Detections (Full)]{\hi\ \bla\ FUV prior detections table, adapted from the results of \cite{Danforth2016} ("Danforth") and \cite{Tilton2012} ("Tilton"). A '*' indicates a duplicate redshift in both Danforth and Tilton. The corresponding Tilton duplicates are omitted from the table.}
\label{tab:hiPriorsTable}
\hline
\# & Name & Redshift & $\log N$ (cm$^{-2}$) & $b$ (km~s$^{-1}$) & Source\\ 
\hline
1 & 1es1028 & 0.13714 & 13.3$\pm$0.1 & 91.60$\pm$24.00 & Danforth \\ 
2 & 1es1028 & 0.20383 & 13.2$\pm$0.1 & 63.60$\pm$14.20 & Danforth \\ 
3 & 1es1028 & 0.22121 & 13.4$\pm$0.8 & 68.60$\pm$71.40 & Danforth \\ 
\hline
4 & 1es1553 & 0.03466 & 13.1$\pm$0.0 & 72.00$\pm$9.40 & Danforth \\ 
5 & 1es1553 & 0.04273 & 13.4$\pm$0.0 & 63.00$\pm$4.50 & Danforth \\ 
6 & 1es1553 & 0.06364 & 13.0$\pm$0.2 & 76.30$\pm$19.90 & Danforth \\ 
7 & 1es1553 & 0.21869 & 12.7$\pm$0.1 & 62.60$\pm$21.80 & Danforth \\ 
\hline
8 & 3c249 & 0.13470 & 13.1$\pm$0.1 & 65.00$\pm$2.00 & Tilton \\ 
9 & 3c249 & 0.26664 & 13.3$\pm$0.1 & 67.00$\pm$19.00 & Tilton \\ 
\hline
10 & 3c263 & 0.06003 & 13.0$\pm$0.1 & 71.30$\pm$21.70 & Danforth \\ 
11 & 3c263 & 0.14073 & 13.5$\pm$0.1 & 83.70$\pm$11.70 & Danforth \\ 
12 & 3c263 & 0.26322 & 12.9$\pm$0.1 & 61.00$\pm$17.40 & Danforth \\ 
13 & 3c263 & 0.31025 & 13.1$\pm$0.1 & 81.90$\pm$19.80 & Danforth \\ 
14 & 3c263 & 0.37740 & 13.4$\pm$0.1 & 85.80$\pm$11.30 & Danforth \\ 
\hline
15 & 3c273 & 0.00758 & 13.0$\pm$0.0 & 74.40$\pm$8.60 & Danforth \\ 
16 & 3c273 & 0.06707 & 12.6$\pm$0.1 & 73.60$\pm$27.60 & Danforth \\ 
17 & 3c273 & 0.07359 & 12.8$\pm$0.1 & 99.70$\pm$18.00 & Danforth \\ 
18 & 3c273 & 0.13960 & 12.6$\pm$0.1 & 64.90$\pm$8.70 & Danforth \\ 
\hline
19 & 3c351 & 0.06008 & 13.2$\pm$0.1 & 67.00$\pm$8.00 & Tilton \\ 
20 & 3c351 & 0.06592 & 13.9$\pm$0.0 & 118.20$\pm$5.60 & Tilton \\ 
21 & 3c351 & 0.18191 & 13.4$\pm$0.1 & 106.00$\pm$4.00 & Tilton \\ 
\hline
22 & 3c57 & 0.19558 & 13.2$\pm$0.1 & 71.30$\pm$12.00 & Danforth \\ 
23 & 3c57 & 0.25994 & 13.3$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
24 & 3c57 & 0.37357 & 13.7$\pm$0.0 & 62.00$\pm$6.70 & Danforth \\ 
25 & 3c57 & 0.44937 & 13.6$\pm$0.1 & 64.90$\pm$13.90 & Danforth \\ 
\hline
26 & 3c66a & 0.08850 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
\hline
27 & b0117 & 0.14156 & 13.7$\pm$0.0 & 69.10$\pm$5.40 & Danforth \\ 
28 & b0117 & 0.16029 & 13.0$\pm$0.1 & 95.60$\pm$29.50 & Danforth \\ 
\hline
29 & f1010 & 0.01614 & 13.2$\pm$0.1 & 88.30$\pm$31.00 & Danforth \\ 
\hline
30 & h1821 & 0.00944 & 13.0$\pm$0.0 & 61.20$\pm$6.90 & Danforth \\ 
31 & h1821 & 0.06779 & 12.7$\pm$0.1 & 87.50$\pm$20.80 & Danforth \\ 
32 & h1821 & 0.08483 & 12.9$\pm$0.1 & 80.60$\pm$17.30 & Danforth \\ 
33 & h1821 & 0.12147 & 13.8$\pm$0.1 & 77.00$\pm$5.00 & Tilton \\ 
34 & h1821 & 0.19817 & 12.9$\pm$0.1 & 71.50$\pm$11.60 & Danforth \\ 
35 & h1821 & 0.21321 & 13.6$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
36 & h1821 & 0.24531 & 13.2$\pm$0.1 & 72.00$\pm$22.50 & Danforth \\ 
\hline
37 & h2356 & 0.03830 & 13.3$\pm$0.1 & 92.40$\pm$20.00 & Danforth \\ 
38 & h2356 & 0.07881 & 13.4$\pm$0.2 & 99.80$\pm$34.30 & Danforth \\ 
39 & h2356 & 0.10467 & 13.5$\pm$0.1 & 71.90$\pm$10.80 & Danforth \\ 
40 & h2356 & 0.15613 & 13.6$\pm$0.1 & 61.00$\pm$15.40 & Danforth \\ 
\hline
41 & he0153 & 0.11318 & 13.7$\pm$0.0 & 69.60$\pm$3.70 & Danforth \\ 
42 & he0153 & 0.17060 & 13.7$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
\hline
43 & he0226 & 0.14274 & 12.8$\pm$0.1 & 63.50$\pm$13.20 & Danforth \\ 
44 & he0226 & 0.39890 & 13.6$\pm$0.1 & 84.00$\pm$27.00 & Tilton \\ 
45 & he0226 & 0.41024 & 13.3$\pm$0.1 & 69.40$\pm$12.10 & Danforth \\ 
\hline
46 & he0238 & 0.10641 & 13.3$\pm$0.1 & 60.50$\pm$6.20 & Danforth \\ 
47 & he0238 & 0.14922 & 13.1$\pm$0.1 & 75.20$\pm$22.00 & Danforth \\ 
48 & he0238 & 0.18747 & 13.1$\pm$0.0 & 62.60$\pm$7.90 & Danforth \\ 
49 & he0238 & 0.27913 & 13.4$\pm$0.0 & 62.10$\pm$7.30 & Danforth \\ 
50 & he0238 & 0.33435 & 13.7$\pm$0.0 & 61.30$\pm$4.20 & Danforth \\ 
\hline
51 & he0435 & 0.00549 & 14.0$\pm$0.1 & 67.50$\pm$15.90 & Danforth \\ 
52 & he0435 & 0.09037 & 13.4$\pm$0.2 & 98.20$\pm$21.50 & Danforth \\ 
53 & he0435 & 0.15328 & 13.3$\pm$0.1 & 71.50$\pm$18.50 & Danforth \\ 
54 & he0435 & 0.16107 & 13.5$\pm$0.1 & 66.10$\pm$9.50 & Danforth \\ 
55 & he0435 & 0.39044 & 13.9$\pm$0.1 & 62.70$\pm$7.90 & Danforth \\ 
56 & he0435 & 0.40988 & 13.6$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
57 & he0435 & 0.42218 & 13.7$\pm$0.0 & 71.80$\pm$6.70 & Danforth \\ 
\hline
58 & hs0624 & 0.05515 & 13.7$\pm$0.2 & 84.00$\pm$30.70 & Tilton \\ 
59 & hs0624 & 0.09005 & 13.5$\pm$0.0 & 122.00$\pm$3.00 & Tilton \\ 
60 & hs0624 & 0.31045 & 13.4$\pm$0.3 & 62.00$\pm$40.30 & Tilton \\ 
\hline
61 & hs1102 & 0.09533 & 13.2$\pm$0.1 & 76.50$\pm$23.20 & Danforth \\ 
62 & hs1102 & 0.18746 & 13.0$\pm$0.2 & 67.70$\pm$29.20 & Danforth \\ 
63 & hs1102 & 0.21101 & 13.6$\pm$0.1 & 130.80$\pm$28.00 & Danforth \\ 
64 & hs1102 & 0.21762 & 13.7$\pm$0.0 & 114.80$\pm$9.40 & Danforth \\ 
65 & hs1102 & 0.25125 & 13.6$\pm$0.1 & 108.40$\pm$23.40 & Danforth \\ 
66 & hs1102 & 0.25365 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
67 & hs1102 & 0.25794 & 13.5$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
68 & hs1102 & 0.25867 & 13.8$\pm$0.2 & 84.10$\pm$27.20 & Danforth \\ 
69 & hs1102 & 0.28713 & 13.2$\pm$0.1 & 63.00$\pm$17.30 & Danforth \\ 
70 & hs1102 & 0.40856 & 13.5$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
71 & hs1102 & 0.40970 & 13.7$\pm$0.2 & 100.00$\pm$0.00 & Danforth \\ 
72 & hs1102 & 0.41874 & 13.7$\pm$0.7 & 130.60$\pm$54.40 & Danforth \\ 
73 & hs1102 & 0.42280 & 14.2$\pm$0.0 & 65.90$\pm$4.00 & Danforth \\ 
74 & hs1102 & 0.46827 & 13.8$\pm$0.0 & 81.10$\pm$2.00 & Danforth \\ 
\hline
75 & i06229 & 0.01218 & 13.1$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
76 & i06229 & 0.05260 & 13.3$\pm$0.1 & 76.00$\pm$17.50 & Danforth \\ 
\hline
77 & i22456 & 0.00443 & 12.8$\pm$0.1 & 75.70$\pm$15.40 & Danforth \\ 
78 & i22456 & 0.09941 & 14.6$\pm$0.0 & 62.80$\pm$0.60 & Danforth \\ 
\hline
79 & mr2251 & 0.01068 & 14.6$\pm$0.7 & 69.00$\pm$4.00 & Tilton \\ 
80 & mr2251 & 0.01449 & 12.9$\pm$0.1 & 78.90$\pm$18.20 & Danforth \\ 
81 & mr2251 & 0.06131 & 13.2$\pm$0.0 & 64.50$\pm$2.90 & Danforth \\ 
82 & mr2251 & 0.06190 & 14.0$\pm$0.0 & 79.20$\pm$0.90 & Danforth \\ 
83 & mr2251 & 0.06276 & 14.3$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
84 & mr2251 & 0.06327 & 14.2$\pm$0.0 & 98.90$\pm$3.40 & Danforth \\ 
85 & mr2251 & 0.06381 & 13.8$\pm$0.0 & 69.70$\pm$2.20 & Danforth \\ 
\hline
86 & mrk106 & 0.06330 & 13.0$\pm$0.1 & 64.70$\pm$18.70 & Danforth \\ 
87 & mrk106 & 0.07672 & 13.2$\pm$0.1 & 72.50$\pm$19.80 & Danforth \\ 
\hline
88 & mrk478 & 0.06166 & 13.2$\pm$0.1 & 97.00$\pm$19.70 & Danforth \\ 
89 & mrk478 & 0.06578 & 13.0$\pm$0.1 & 64.20$\pm$22.30 & Danforth \\ 
90 & mrk478 & 0.07213 & 13.3$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
\hline
91 & mrk876 & 0.01159 & 13.2$\pm$0.1 & 84.90$\pm$10.10 & Danforth \\ 
92 & mrk876 & 0.05598 & 12.8$\pm$0.1 & 79.60$\pm$18.90 & Danforth \\ 
93 & mrk876 & 0.08709 & 12.3$\pm$0.2 & 68.20$\pm$35.10 & Danforth \\ 
94 & mrk876 & 0.08858 & 13.6$\pm$0.0 & 70.30$\pm$2.70 & Danforth \\ 
95 & mrk876 & 0.08917 & 12.9$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
96 & mrk876 & 0.11487 & 13.2$\pm$0.1 & 74.00$\pm$6.00 & Tilton \\ 
\hline
97 & ngc7469 & 0.00981 & 13.5$\pm$0.1 & 132.70$\pm$27.60 & Tilton \\ 
\hline
98 & pg0003 & 0.08299 & 13.8$\pm$0.0 & 64.40$\pm$6.40 & Danforth \\ 
99 & pg0003 & 0.17139 & 12.9$\pm$0.1 & 102.90$\pm$29.10 & Danforth \\ 
100 & pg0003 & 0.22541 & 13.1$\pm$0.1 & 92.80$\pm$18.60 & Danforth \\ 
101 & pg0003 & 0.38633 & 13.5$\pm$0.2 & 86.70$\pm$32.30 & Danforth \\ 
102 & pg0003 & 0.42051 & 13.4$\pm$0.1 & 63.90$\pm$9.30 & Danforth \\ 
\hline
103 & pg0804 & 0.05015 & 12.8$\pm$0.1 & 69.80$\pm$14.60 & Danforth \\ 
104 & pg0804 & 0.05576 & 12.8$\pm$10.0 & 64.20$\pm$99.90 & Danforth \\ 
105 & pg0804 & 0.36379 & 12.5$\pm$0.3 & 63.20$\pm$8.20 & Danforth \\ 
\hline
106 & pg0832 & 0.01753 & 15.6$\pm$0.2 & 87.30$\pm$5.40 & Danforth \\ 
107 & pg0832 & 0.02793 & 13.6$\pm$0.2 & 65.90$\pm$18.50 & Danforth \\ 
108 & pg0832 & 0.08748 & 13.4$\pm$0.1 & 116.70$\pm$31.70 & Danforth \\ 
109 & pg0832 & 0.10171 & 13.9$\pm$0.1 & 60.90$\pm$8.00 & Danforth \\ 
110 & pg0832 & 0.18391 & 13.3$\pm$0.1 & 130.50$\pm$38.30 & Danforth \\ 
111 & pg0832 & 0.27503 & 13.6$\pm$0.1 & 60.60$\pm$12.50 & Danforth \\ 
112 & pg0832 & 0.27694 & 13.6$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
113 & pg0832 & 0.32572 & 13.3$\pm$0.1 & 60.20$\pm$11.10 & Danforth \\ 
\hline
114 & pg0838 & 0.06583 & 13.3$\pm$0.1 & 81.20$\pm$14.30 & Danforth \\ 
115 & pg0838 & 0.08628 & 13.1$\pm$0.2 & 148.80$\pm$42.90 & Danforth \\ 
116 & pg0838 & 0.12676 & 13.1$\pm$0.1 & 91.90$\pm$13.20 & Danforth \\ 
\hline
117 & pg0953 & 0.16319 & 13.0$\pm$0.1 & 74.90$\pm$10.00 & Danforth \\ 
118 & pg0953 & 0.19221 & 13.3$\pm$0.1 & 63.80$\pm$14.60 & Tilton \\ 
\hline
119 & pg1001 & 0.00165 & 13.9$\pm$1.3 & 60.60$\pm$51.80 & Danforth \\ 
120 & pg1001 & 0.21343 & 13.9$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
\hline
121 & pg1048 & 0.00642 & 14.0$\pm$0.1 & 86.90$\pm$8.90 & Danforth \\ 
122 & pg1048 & 0.02414 & 13.2$\pm$0.1 & 66.70$\pm$13.00 & Danforth \\ 
\hline
123 & pg1049 & 0.03015 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
124 & pg1049 & 0.06313 & 13.6$\pm$0.1 & 86.30$\pm$13.20 & Danforth \\ 
125 & pg1049 & 0.12706 & 13.6$\pm$0.1 & 63.30$\pm$9.70 & Danforth \\ 
126 & pg1049 & 0.14980 & 13.3$\pm$0.1 & 72.00$\pm$10.50 & Danforth \\ 
127 & pg1049 & 0.16322 & 13.2$\pm$0.2 & 100.00$\pm$0.00 & Danforth \\ 
128 & pg1049 & 0.32523 & 13.3$\pm$0.1 & 105.90$\pm$32.00 & Danforth \\ 
129 & pg1049 & 0.34016 & 13.5$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
130 & pg1049 & 0.34187 & 14.1$\pm$0.0 & 64.30$\pm$4.00 & Danforth \\ 
\hline
131 & pg1115 & 0.09511 & 13.2$\pm$0.1 & 68.30$\pm$12.50 & Danforth \\ 
132 & pg1115 & 0.12059 & 13.0$\pm$0.1 & 73.50$\pm$20.20 & Danforth \\ 
133 & pg1115 & 0.12741 & 13.2$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
\hline
134 & pg1116 & 0.04114 & 13.2$\pm$0.0 & 69.50$\pm$8.40 & Danforth^{*} \\ 
135 & pg1116 & 0.06251 & 13.1$\pm$0.0 & 71.20$\pm$5.70 & Tilton \\ 
136 & pg1116 & 0.08382 & 13.2$\pm$0.1 & 63.80$\pm$13.80 & Danforth \\ 
137 & pg1116 & 0.09210 & 12.8$\pm$0.1 & 68.80$\pm$22.30 & Danforth \\ 
138 & pg1116 & 0.09281 & 13.1$\pm$0.1 & 77.40$\pm$11.90 & Danforth^{*} \\ 
139 & pg1116 & 0.13373 & 13.2$\pm$0.0 & 81.30$\pm$6.00 & Tilton \\ 
140 & pg1116 & 0.13851 & 13.5$\pm$0.2 & 80.80$\pm$16.20 & Danforth \\ 
\hline
141 & pg1121 & 0.00791 & 13.3$\pm$0.1 & 99.00$\pm$25.00 & Danforth \\ 
142 & pg1121 & 0.07727 & 13.5$\pm$0.1 & 60.90$\pm$13.30 & Danforth \\ 
143 & pg1121 & 0.18078 & 13.5$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
144 & pg1121 & 0.18869 & 13.1$\pm$0.1 & 70.40$\pm$20.40 & Danforth \\ 
145 & pg1121 & 0.21814 & 12.9$\pm$0.1 & 69.50$\pm$22.70 & Danforth \\ 
146 & pg1121 & 0.21992 & 13.9$\pm$0.0 & 80.70$\pm$2.20 & Danforth \\ 
\hline
147 & pg1211 & 0.02586 & 13.5$\pm$0.0 & 70.00$\pm$2.00 & Tilton \\ 
148 & pg1211 & 0.05443 & 13.2$\pm$0.0 & 98.00$\pm$1.00 & Tilton \\ 
\hline
149 & pg1216 & 0.00842 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
150 & pg1216 & 0.07969 & 13.2$\pm$0.1 & 66.80$\pm$14.50 & Danforth \\ 
151 & pg1216 & 0.12372 & 14.8$\pm$0.1 & 70.80$\pm$3.40 & Tilton \\ 
152 & pg1216 & 0.12473 & 14.7$\pm$0.1 & 73.60$\pm$3.50 & Tilton \\ 
153 & pg1216 & 0.17950 & 13.2$\pm$0.1 & 64.80$\pm$11.10 & Danforth \\ 
154 & pg1216 & 0.20014 & 13.6$\pm$0.0 & 60.60$\pm$6.90 & Danforth \\ 
155 & pg1216 & 0.21258 & 13.0$\pm$0.1 & 60.50$\pm$19.80 & Danforth \\ 
156 & pg1216 & 0.28204 & 13.9$\pm$1.2 & 78.60$\pm$22.50 & Danforth \\ 
\hline
157 & pg1222 & 0.15554 & 13.9$\pm$0.0 & 64.70$\pm$3.00 & Danforth \\ 
158 & pg1222 & 0.24198 & 13.6$\pm$0.1 & 91.40$\pm$12.50 & Danforth \\ 
159 & pg1222 & 0.26075 & 12.9$\pm$0.1 & 60.20$\pm$17.70 & Danforth \\ 
160 & pg1222 & 0.32786 & 13.2$\pm$0.1 & 84.70$\pm$28.00 & Danforth \\ 
161 & pg1222 & 0.36749 & 13.7$\pm$0.0 & 96.20$\pm$10.60 & Danforth \\ 
162 & pg1222 & 0.37471 & 13.8$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
163 & pg1222 & 0.37721 & 13.6$\pm$0.1 & 72.80$\pm$17.20 & Danforth \\ 
164 & pg1222 & 0.37840 & 13.5$\pm$1.4 & 61.40$\pm$67.10 & Danforth \\ 
\hline
165 & pg1229 & 0.05018 & 12.9$\pm$0.1 & 61.90$\pm$19.80 & Danforth \\ 
\hline
166 & pg1259 & 0.05563 & 13.4$\pm$0.0 & 70.70$\pm$5.90 & Danforth \\ 
167 & pg1259 & 0.15136 & 13.3$\pm$0.1 & 62.20$\pm$3.70 & Tilton \\ 
168 & pg1259 & 0.16647 & 13.3$\pm$0.1 & 93.30$\pm$8.90 & Tilton \\ 
169 & pg1259 & 0.17893 & 13.1$\pm$0.1 & 83.70$\pm$11.90 & Tilton \\ 
170 & pg1259 & 0.22376 & 13.0$\pm$0.1 & 76.50$\pm$17.90 & Danforth \\ 
171 & pg1259 & 0.24126 & 13.4$\pm$0.1 & 89.10$\pm$6.90 & Tilton \\ 
172 & pg1259 & 0.31974 & 14.0$\pm$0.0 & 70.30$\pm$3.10 & Tilton \\ 
173 & pg1259 & 0.36212 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
174 & pg1259 & 0.38254 & 13.5$\pm$0.0 & 82.20$\pm$8.90 & Danforth \\ 
175 & pg1259 & 0.38266 & 13.7$\pm$0.1 & 137.00$\pm$19.00 & Tilton \\ 
\hline
176 & pg1307 & 0.08345 & 13.4$\pm$0.1 & 84.60$\pm$7.10 & Danforth \\ 
\hline
177 & pg1309 & 0.03861 & 13.4$\pm$0.1 & 62.70$\pm$12.10 & Danforth \\ 
178 & pg1309 & 0.17740 & 13.9$\pm$0.0 & 65.10$\pm$5.30 & Danforth \\ 
179 & pg1309 & 0.17852 & 14.5$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
180 & pg1309 & 0.17918 & 14.4$\pm$0.0 & 128.90$\pm$8.10 & Danforth \\ 
181 & pg1309 & 0.18143 & 13.9$\pm$0.0 & 94.90$\pm$9.90 & Danforth \\ 
\hline
182 & pg1424 & 0.01908 & 13.5$\pm$0.1 & 96.00$\pm$14.30 & Danforth \\ 
183 & pg1424 & 0.25044 & 13.0$\pm$0.1 & 74.40$\pm$22.10 & Danforth \\ 
184 & pg1424 & 0.36260 & 13.2$\pm$0.1 & 82.40$\pm$23.40 & Danforth \\ 
\hline
185 & pg1444 & 0.22031 & 13.5$\pm$0.0 & 76.00$\pm$7.60 & Tilton \\ 
\hline
186 & pg1626 & 0.06137 & 13.6$\pm$0.0 & 60.50$\pm$6.60 & Danforth \\ 
\hline
187 & phl1811 & 0.05143 & 13.7$\pm$0.0 & 72.80$\pm$5.10 & Danforth \\ 
188 & phl1811 & 0.05813 & 13.2$\pm$0.1 & 89.50$\pm$16.80 & Danforth \\ 
189 & phl1811 & 0.08085 & 13.9$\pm$0.1 & 91.80$\pm$11.60 & Danforth \\ 
190 & phl1811 & 0.08163 & 13.2$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
191 & phl1811 & 0.12003 & 13.0$\pm$0.1 & 77.40$\pm$16.90 & Danforth \\ 
192 & phl1811 & 0.15787 & 13.2$\pm$0.1 & 70.40$\pm$9.90 & Danforth \\ 
\hline
193 & phl2525 & 0.06548 & 13.2$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
194 & phl2525 & 0.06682 & 13.4$\pm$0.1 & 64.80$\pm$14.20 & Danforth \\ 
195 & phl2525 & 0.08351 & 13.4$\pm$0.1 & 66.70$\pm$16.90 & Danforth \\ 
196 & phl2525 & 0.14869 & 13.1$\pm$0.1 & 65.20$\pm$16.20 & Danforth \\ 
197 & phl2525 & 0.17002 & 13.3$\pm$0.1 & 116.00$\pm$42.10 & Danforth \\ 
\hline
198 & pks0312 & 0.11454 & 14.0$\pm$0.0 & 79.00$\pm$4.00 & Tilton \\ 
\hline
199 & pks0405 & 0.02510 & 13.2$\pm$0.1 & 144.30$\pm$26.50 & Danforth \\ 
200 & pks0405 & 0.05902 & 13.3$\pm$0.1 & 62.30$\pm$11.10 & Tilton \\ 
201 & pks0405 & 0.09719 & 13.6$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
202 & pks0405 & 0.10152 & 13.2$\pm$0.1 & 67.90$\pm$11.30 & Tilton \\ 
203 & pks0405 & 0.10298 & 13.4$\pm$0.1 & 73.70$\pm$12.00 & Tilton \\ 
204 & pks0405 & 0.19456 & 12.8$\pm$0.1 & 63.60$\pm$8.10 & Danforth^{*} \\ 
205 & pks0405 & 0.21976 & 12.7$\pm$0.1 & 70.20$\pm$18.80 & Danforth \\ 
206 & pks0405 & 0.24564 & 13.1$\pm$0.1 & 77.40$\pm$14.80 & Danforth \\ 
207 & pks0405 & 0.29748 & 13.2$\pm$0.1 & 66.00$\pm$11.70 & Danforth \\ 
208 & pks0405 & 0.31016 & 12.9$\pm$0.1 & 76.70$\pm$20.20 & Danforth \\ 
209 & pks0405 & 0.32502 & 13.7$\pm$0.0 & 85.50$\pm$6.10 & Tilton \\ 
210 & pks0405 & 0.49508 & 14.3$\pm$0.0 & 64.90$\pm$7.70 & Tilton \\ 
\hline
211 & pks0552 & 0.26916 & 13.2$\pm$0.1 & 68.40$\pm$13.10 & Danforth \\ 
212 & pks0552 & 0.35661 & 13.3$\pm$0.1 & 64.70$\pm$9.50 & Danforth \\ 
\hline
213 & pks0558 & 0.10472 & 13.0$\pm$0.1 & 79.50$\pm$35.00 & Danforth \\ 
\hline
214 & pks0637 & 0.14272 & 13.1$\pm$0.1 & 77.90$\pm$13.80 & Danforth \\ 
215 & pks0637 & 0.16082 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
216 & pks0637 & 0.17428 & 13.0$\pm$0.1 & 72.20$\pm$16.30 & Danforth \\ 
217 & pks0637 & 0.36408 & 13.5$\pm$0.1 & 86.70$\pm$13.00 & Danforth \\ 
218 & pks0637 & 0.41784 & 13.7$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
\hline
219 & pks1302 & 0.01956 & 13.3$\pm$0.1 & 66.20$\pm$9.50 & Danforth \\ 
220 & pks1302 & 0.03281 & 13.1$\pm$0.1 & 62.80$\pm$14.60 & Danforth \\ 
221 & pks1302 & 0.14531 & 15.4$\pm$0.1 & 61.80$\pm$3.90 & Tilton \\ 
222 & pks1302 & 0.19281 & 13.6$\pm$0.1 & 68.90$\pm$14.10 & Tilton \\ 
223 & pks1302 & 0.23679 & 13.4$\pm$0.0 & 69.70$\pm$6.90 & Danforth \\ 
224 & pks1302 & 0.23752 & 13.0$\pm$0.1 & 74.70$\pm$26.90 & Danforth \\ 
225 & pks1302 & 0.24885 & 13.4$\pm$0.1 & 77.00$\pm$19.00 & Tilton \\ 
226 & pks1302 & 0.25120 & 13.7$\pm$0.0 & 71.40$\pm$4.10 & Danforth \\ 
\hline
227 & pks2155 & 0.05708 & 14.1$\pm$0.0 & 67.90$\pm$1.70 & Danforth^{*} \\ 
228 & pks2155 & 0.06236 & 12.8$\pm$0.1 & 69.10$\pm$22.20 & Danforth \\ 
229 & pks2155 & 0.10586 & 13.5$\pm$0.0 & 66.00$\pm$4.00 & Tilton \\ 
\hline
230 & pmn2345 & 0.28405 & 13.5$\pm$0.1 & 81.80$\pm$13.80 & Danforth \\ 
231 & pmn2345 & 0.31540 & 13.7$\pm$0.0 & 60.10$\pm$7.30 & Danforth \\ 
232 & pmn2345 & 0.37828 & 14.3$\pm$0.0 & 65.70$\pm$2.90 & Danforth \\ 
233 & pmn2345 & 0.43000 & 13.5$\pm$0.1 & 63.00$\pm$18.10 & Danforth \\ 
234 & pmn2345 & 0.47074 & 13.6$\pm$0.0 & 87.10$\pm$3.10 & Danforth \\ 
\hline
235 & q0045 & 0.05590 & 13.2$\pm$0.1 & 66.80$\pm$12.80 & Danforth \\ 
236 & q0045 & 0.06377 & 13.0$\pm$0.1 & 70.60$\pm$23.20 & Danforth \\ 
\hline
237 & q1230 & 0.08344 & 13.3$\pm$0.0 & 65.00$\pm$6.00 & Tilton \\ 
238 & q1230 & 0.08540 & 12.8$\pm$0.1 & 94.60$\pm$26.80 & Danforth \\ 
239 & q1230 & 0.09444 & 13.0$\pm$0.1 & 69.70$\pm$10.10 & Danforth \\ 
240 & q1230 & 0.10000 & 13.2$\pm$0.1 & 61.00$\pm$8.00 & Tilton \\ 
241 & q1230 & 0.10525 & 14.0$\pm$0.1 & 75.00$\pm$4.00 & Tilton \\ 
242 & q1230 & 0.10549 & 14.1$\pm$0.0 & 87.30$\pm$3.30 & Danforth \\ 
243 & q1230 & 0.10566 & 14.0$\pm$0.1 & 121.70$\pm$28.60 & Tilton \\ 
244 & q1230 & 0.10612 & 13.4$\pm$0.1 & 76.40$\pm$15.40 & Danforth \\ 
245 & q1230 & 0.10639 & 13.8$\pm$0.0 & 64.30$\pm$3.40 & Tilton \\ 
246 & q1230 & 0.10660 & 13.5$\pm$0.1 & 61.90$\pm$4.00 & Danforth \\ 
247 & q1230 & 0.10853 & 12.8$\pm$0.1 & 92.60$\pm$21.50 & Danforth \\ 
248 & q1230 & 0.10940 & 13.8$\pm$0.0 & 100.00$\pm$0.00 & Danforth \\ 
249 & q1230 & 0.12103 & 13.5$\pm$0.0 & 69.40$\pm$3.60 & Tilton \\ 
\hline
250 & rbs144 & 0.04528 & 13.1$\pm$0.1 & 62.30$\pm$12.70 & Danforth \\ 
\hline
251 & rbs1892 & 0.15567 & 13.3$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
252 & rbs1892 & 0.15633 & 13.4$\pm$0.0 & 150.00$\pm$0.00 & Danforth \\ 
253 & rbs1892 & 0.16343 & 13.8$\pm$0.0 & 67.60$\pm$2.70 & Danforth \\ 
254 & rbs1892 & 0.17001 & 13.2$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
255 & rbs1892 & 0.17155 & 13.4$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
256 & rbs1892 & 0.17185 & 13.2$\pm$0.1 & 84.70$\pm$14.20 & Danforth \\ 
\hline
257 & rbs542 & 0.04455 & 12.9$\pm$0.0 & 70.80$\pm$7.80 & Danforth \\ 
258 & rbs542 & 0.04992 & 12.8$\pm$0.1 & 62.10$\pm$13.30 & Danforth \\ 
\hline
259 & rxj0439 & 0.00550 & 13.7$\pm$0.2 & 67.90$\pm$15.90 & Danforth \\ 
260 & rxj0439 & 0.17680 & 13.5$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
\hline
261 & rxj0956 & 0.03471 & 13.8$\pm$0.0 & 64.80$\pm$5.90 & Danforth \\ 
262 & rxj0956 & 0.06924 & 13.2$\pm$0.1 & 67.30$\pm$18.50 & Danforth \\ 
263 & rxj0956 & 0.10858 & 13.3$\pm$0.1 & 74.30$\pm$21.00 & Danforth \\ 
264 & rxj0956 & 0.12796 & 13.6$\pm$0.1 & 89.60$\pm$11.00 & Danforth \\ 
265 & rxj0956 & 0.14704 & 13.2$\pm$0.1 & 88.40$\pm$25.40 & Danforth \\ 
266 & rxj0956 & 0.15101 & 13.0$\pm$0.1 & 81.80$\pm$22.40 & Danforth \\ 
\hline
267 & rxj2154 & 0.23009 & 13.1$\pm$0.1 & 68.20$\pm$17.40 & Danforth \\ 
\hline
268 & s080908 & 0.05775 & 13.5$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
269 & s080908 & 0.06391 & 13.6$\pm$0.2 & 149.00$\pm$46.10 & Danforth \\ 
270 & s080908 & 0.14214 & 13.4$\pm$0.1 & 94.80$\pm$15.00 & Danforth \\ 
271 & s080908 & 0.16001 & 13.4$\pm$0.1 & 76.00$\pm$9.70 & Danforth \\ 
272 & s080908 & 0.38700 & 13.4$\pm$0.2 & 100.00$\pm$0.00 & Danforth \\ 
\hline
273 & s09255b & 0.13118 & 13.4$\pm$0.1 & 86.70$\pm$12.00 & Danforth \\ 
\hline
274 & s092909 & 0.16491 & 13.8$\pm$0.0 & 63.60$\pm$5.70 & Danforth \\ 
275 & s092909 & 0.23508 & 13.5$\pm$0.0 & 83.10$\pm$8.20 & Danforth \\ 
\hline
276 & s094952 & 0.06581 & 13.4$\pm$0.1 & 90.00$\pm$28.60 & Danforth \\ 
277 & s094952 & 0.16442 & 13.4$\pm$1.0 & 63.40$\pm$55.70 & Danforth \\ 
\hline
278 & s135712 & 0.14702 & 14.0$\pm$0.0 & 79.90$\pm$1.90 & Danforth \\ 
\hline
279 & s50716 & 0.00989 & 13.1$\pm$0.1 & 61.90$\pm$12.90 & Danforth \\ 
280 & s50716 & 0.01766 & 13.1$\pm$0.1 & 89.50$\pm$13.60 & Danforth \\ 
281 & s50716 & 0.08834 & 13.1$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
282 & s50716 & 0.14936 & 12.9$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
\hline
283 & sbs1108 & 0.02497 & 13.8$\pm$0.0 & 79.40$\pm$3.10 & Danforth \\ 
284 & sbs1108 & 0.25715 & 13.7$\pm$0.0 & 61.40$\pm$6.50 & Danforth \\ 
285 & sbs1108 & 0.41402 & 13.6$\pm$0.1 & 81.20$\pm$18.30 & Danforth \\ 
\hline
286 & sbs1122 & 0.04709 & 13.3$\pm$0.1 & 62.00$\pm$13.00 & Danforth \\ 
287 & sbs1122 & 0.13699 & 13.3$\pm$0.2 & 77.60$\pm$32.70 & Danforth \\ 
288 & sbs1122 & 0.13812 & 13.6$\pm$0.1 & 100.00$\pm$0.00 & Danforth \\ 
289 & sbs1122 & 0.13865 & 13.8$\pm$0.1 & 150.00$\pm$0.00 & Danforth \\ 
290 & sbs1122 & 0.15271 & 13.5$\pm$0.2 & 74.50$\pm$23.30 & Danforth \\ 
291 & sbs1122 & 0.36707 & 13.7$\pm$0.1 & 82.90$\pm$13.80 & Danforth \\ 
\hline
292 & ton1187 & 0.01504 & 13.7$\pm$0.1 & 96.20$\pm$14.60 & Danforth \\ 
293 & ton1187 & 0.05216 & 13.5$\pm$0.2 & 61.20$\pm$9.80 & Danforth \\ 
294 & ton1187 & 0.07687 & 13.1$\pm$0.1 & 83.70$\pm$20.30 & Danforth \\ 
\hline
295 & ton28 & 0.03357 & 13.4$\pm$0.1 & 75.00$\pm$7.00 & Tilton \\ 
\hline
296 & tons180 & 0.04304 & 13.8$\pm$0.4 & 81.00$\pm$15.00 & Tilton \\ 
\hline
297 & tons210 & 0.06763 & 13.0$\pm$0.1 & 61.10$\pm$21.80 & Danforth \\ 
298 & tons210 & 0.08558 & 13.1$\pm$0.1 & 73.00$\pm$12.60 & Danforth \\ 
\hline
\end{longtable}

==> Tables/Priors/o6priors_full.tex <==
\renewcommand{\arraystretch}{.6}
\setlength\LTleft{1cm}

\begin{longtable}{lllccccc}
\caption[\ovi\ Prior Detections (Full)]{\ovi\ FUV prior detections table, adapted from the results of \cite{Danforth2016} ("Danforth") and \cite{Tilton2012} ("Tilton"). A '$^M$' indicates that there was an OVI 1032 and 1038 doublet present. These 1032 and 1038 doublet values were averaged into one value on a weighted system of 2:1 respectively. A '*' indicates a duplicate redshift in both Danforth and Tilton. The corresponding Tilton duplicates are omitted from the table.}
\label{tab:oviPriorsTable}
\hline
\# & Name & Redshift & $\log N$ (cm$^{-2}$) & $b$ (km~s$^{-1}$) & Source\\ 
\hline
1 & 1es1028 & 0.12314 & 14.3$\pm$0.1 & 41.37$\pm$5.57 & Danforth$^{M}$ \\ 
2 & 1es1028 & 0.13706 & 13.6$\pm$0.1 & 14.50$\pm$6.30 & Danforth$^{1032}$ \\ 
3 & 1es1028 & 0.33735 & 13.9$\pm$0.1 & 72.87$\pm$15.73 & Danforth$^{M}$ \\ 
\hline
4 & 1es1553 & 0.18759 & 13.8$\pm$0.1 & 12.10$\pm$3.00 & Danforth$^{M}$ \\ 
5 & 1es1553 & 0.18775 & 13.9$\pm$0.1 & 23.40$\pm$4.50 & Danforth$^{M}$ \\ 
6 & 1es1553 & 0.18984 & 13.4$\pm$1.5 & 23.37$\pm$6.57 & Danforth$^{M}$ \\ 
7 & 1es1553 & 0.21631 & 13.3$\pm$0.1 & 19.80$\pm$5.80 & Danforth$^{1032}$ \\ 
8 & 1es1553 & 0.31130 & 13.4$\pm$0.1 & 31.90$\pm$7.50 & Danforth$^{1032}$ \\ 
9 & 1es1553 & 0.37868 & 12.9$\pm$0.2 & 17.30$\pm$3.70 & Danforth$^{1032}$ \\ 
10 & 1es1553 & 0.39497 & 13.9$\pm$0.1 & 44.07$\pm$3.33 & Danforth$^{M}$ \\ 
\hline
11 & 1sj1032 & 0.17007 & 14.3$\pm$0.0 & 42.00$\pm$3.80 & Danforth$^{1032}$ \\ 
\hline
12 & 3c249 & 0.24676 & 13.8$\pm$0.1 & 24.70$\pm$2.50 & Tilton \\ 
13 & 3c249 & 0.30788 & 13.9$\pm$0.2 & 23.30$\pm$6.10 & Tilton \\ 
14 & 3c249 & 0.30809 & 14.5$\pm$0.0 & 20.00$\pm$1.00 & Tilton \\ 
15 & 3c249 & 0.31364 & 13.8$\pm$0.1 & 13.30$\pm$1.00 & Tilton \\ 
\hline
16 & 3c263 & 0.11388 & 13.7$\pm$0.1 & 33.10$\pm$8.20 & Danforth$^{1032}$ \\ 
17 & 3c263 & 0.14078 & 13.7$\pm$0.1 & 45.10$\pm$6.97 & Danforth$^{M}$ \\ 
18 & 3c263 & 0.29204 & 13.0$\pm$0.2 & 21.40$\pm$9.60 & Danforth$^{1032}$ \\ 
19 & 3c263 & 0.32566 & 14.0$\pm$0.0 & 32.57$\pm$2.47 & Danforth$^{M}$ \\ 
20 & 3c263 & 0.44677 & 13.9$\pm$0.1 & 64.10$\pm$10.70 & Danforth$^{1038}$ \\ 
21 & 3c263 & 0.52690 & 13.9$\pm$0.1 & 38.47$\pm$7.00 & Danforth$^{M}$ \\ 
22 & 3c263 & 0.52801 & 13.5$\pm$0.1 & 48.00$\pm$14.40 & Danforth$^{1032}$ \\ 
\hline
23 & 3c273 & 0.00337 & 13.4$\pm$0.1 & 28.00$\pm$1.00 & Tilton \\ 
24 & 3c273 & 0.00533 & 13.0$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
25 & 3c273 & 0.00764 & 13.1$\pm$0.2 & 25.00$\pm$9.00 & Tilton \\ 
26 & 3c273 & 0.02947 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
27 & 3c273 & 0.04898 & 14.0$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
28 & 3c273 & 0.06655 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
29 & 3c273 & 0.09018 & 13.3$\pm$0.1 & 22.20$\pm$10.80 & Tilton \\ 
30 & 3c273 & 0.12007 & 13.4$\pm$0.1 & 20.03$\pm$3.23 & Danforth$^{M,*}$ \\ 
31 & 3c273 & 0.14660 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
32 & 3c273 & 0.15784 & 13.1$\pm$0.1 & 30.30$\pm$4.90 & Danforth$^{1032*}$ \\ 
\hline
33 & 3c351 & 0.21789 & 14.0$\pm$0.0 & 74.40$\pm$8.60 & Tilton \\ 
34 & 3c351 & 0.22093 & 14.3$\pm$0.0 & 48.50$\pm$3.50 & Tilton \\ 
35 & 3c351 & 0.31635 & 13.7$\pm$0.1 & 22.70$\pm$3.30 & Tilton \\ 
36 & 3c351 & 0.31657 & 14.0$\pm$0.1 & 23.40$\pm$2.40 & Tilton \\ 
37 & 3c351 & 0.31687 & 14.0$\pm$0.1 & 31.80$\pm$2.90 & Tilton \\ 
38 & 3c351 & 0.32086 & 12.9$\pm$0.2 & 30.00$\pm$0.00 & Tilton \\ 
\hline
39 & 3c57 & 0.17002 & 13.6$\pm$0.1 & 43.50$\pm$12.40 & Danforth$^{1032}$ \\ 
40 & 3c57 & 0.24987 & 13.6$\pm$0.1 & 10.40$\pm$3.80 & Danforth$^{1032}$ \\ 
41 & 3c57 & 0.25022 & 13.8$\pm$0.1 & 60.00$\pm$12.20 & Danforth$^{1032}$ \\ 
42 & 3c57 & 0.27821 & 13.8$\pm$0.1 & 28.40$\pm$5.37 & Danforth$^{M}$ \\ 
43 & 3c57 & 0.28669 & 13.6$\pm$0.2 & 40.30$\pm$8.80 & Danforth$^{1032}$ \\ 
44 & 3c57 & 0.29238 & 14.3$\pm$0.0 & 41.53$\pm$2.50 & Danforth$^{M}$ \\ 
45 & 3c57 & 0.32010 & 13.8$\pm$0.1 & 26.60$\pm$9.30 & Danforth$^{1038}$ \\ 
46 & 3c57 & 0.32301 & 13.4$\pm$0.1 & 19.63$\pm$7.43 & Danforth$^{M}$ \\ 
47 & 3c57 & 0.32368 & 13.7$\pm$0.2 & 34.90$\pm$16.90 & Danforth$^{1038}$ \\ 
48 & 3c57 & 0.32405 & 14.1$\pm$0.1 & 74.33$\pm$25.17 & Danforth$^{M}$ \\ 
49 & 3c57 & 0.32460 & 14.1$\pm$0.1 & 39.93$\pm$6.17 & Danforth$^{M}$ \\ 
50 & 3c57 & 0.32780 & 13.7$\pm$0.1 & 40.80$\pm$15.13 & Danforth$^{M}$ \\ 
51 & 3c57 & 0.32820 & 14.5$\pm$0.0 & 38.83$\pm$2.00 & Danforth$^{M}$ \\ 
52 & 3c57 & 0.32902 & 13.9$\pm$0.0 & 29.03$\pm$3.97 & Danforth$^{M}$ \\ 
53 & 3c57 & 0.33332 & 13.7$\pm$0.1 & 29.97$\pm$7.40 & Danforth$^{M}$ \\ 
54 & 3c57 & 0.38342 & 14.0$\pm$0.0 & 23.03$\pm$2.43 & Danforth$^{M}$ \\ 
55 & 3c57 & 0.40187 & 13.2$\pm$0.1 & 5.20$\pm$5.20 & Danforth$^{1032}$ \\ 
56 & 3c57 & 0.40211 & 13.5$\pm$0.1 & 26.83$\pm$8.40 & Danforth$^{M}$ \\ 
57 & 3c57 & 0.43164 & 14.0$\pm$0.1 & 56.40$\pm$7.00 & Danforth$^{1032}$ \\ 
58 & 3c57 & 0.53325 & 13.9$\pm$0.1 & 12.33$\pm$2.67 & Danforth$^{M}$ \\ 
59 & 3c57 & 0.57997 & 14.1$\pm$0.1 & 21.53$\pm$4.27 & Danforth$^{M}$ \\ 
60 & 3c57 & 0.66914 & 13.9$\pm$0.1 & 13.23$\pm$3.87 & Danforth$^{M}$ \\ 
61 & 3c57 & 0.66948 & 13.9$\pm$0.1 & 14.97$\pm$4.53 & Danforth$^{M}$ \\ 
62 & 3c57 & 0.66976 & 14.2$\pm$0.1 & 15.80$\pm$2.63 & Danforth$^{M}$ \\ 
\hline
63 & 3c66a & 0.24258 & 14.2$\pm$0.0 & 25.63$\pm$2.10 & Danforth$^{M}$ \\ 
64 & 3c66a & 0.32824 & 13.4$\pm$0.1 & 35.30$\pm$12.70 & Danforth$^{1032}$ \\ 
\hline
65 & b0117 & 0.14191 & 13.3$\pm$0.1 & 13.60$\pm$8.60 & Danforth$^{1032}$ \\ 
66 & b0117 & 0.19073 & 13.6$\pm$0.1 & 15.10$\pm$2.70 & Danforth$^{M}$ \\ 
67 & b0117 & 0.34848 & 13.9$\pm$0.1 & 47.80$\pm$8.23 & Danforth$^{M}$ \\ 
68 & b0117 & 0.34861 & 13.8$\pm$0.1 & 17.63$\pm$3.83 & Danforth$^{M}$ \\ 
\hline
69 & f1010 & 0.11326 & 14.0$\pm$0.2 & 52.10$\pm$15.90 & Danforth$^{1032}$ \\ 
70 & f1010 & 0.19113 & 13.3$\pm$0.2 & 19.30$\pm$12.10 & Danforth$^{1032}$ \\ 
71 & f1010 & 0.19319 & 13.7$\pm$0.1 & 9.07$\pm$2.33 & Danforth$^{M}$ \\ 
72 & f1010 & 0.25473 & 18.0$\pm$0.3 & 30.10$\pm$0.50 & Danforth$^{1032}$ \\ 
\hline
73 & h1821 & 0.02438 & 13.4$\pm$0.1 & 21.00$\pm$7.50 & Tilton \\ 
74 & h1821 & 0.10817 & 13.2$\pm$0.1 & 10.00$\pm$0.00 & Tilton \\ 
75 & h1821 & 0.12133 & 14.0$\pm$0.0 & 76.00$\pm$12.00 & Tilton \\ 
76 & h1821 & 0.12147 & 13.7$\pm$0.1 & 50.30$\pm$8.60 & Danforth$^{1032}$ \\ 
77 & h1821 & 0.16992 & 13.8$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
78 & h1821 & 0.17043 & 13.6$\pm$0.0 & 57.60$\pm$7.50 & Danforth$^{1032}$ \\ 
79 & h1821 & 0.21326 & 13.6$\pm$0.0 & 23.77$\pm$2.83 & Danforth$^{M,*}$ \\ 
80 & h1821 & 0.22497 & 14.3$\pm$0.0 & 45.17$\pm$1.43 & Danforth$^{M,*}$ \\ 
81 & h1821 & 0.22522 & 13.1$\pm$0.1 & 5.00$\pm$0.00 & Danforth$^{M,*}$ \\ 
82 & h1821 & 0.22639 & 13.5$\pm$0.0 & 17.43$\pm$2.37 & Danforth$^{M,*}$ \\ 
83 & h1821 & 0.24531 & 13.7$\pm$0.0 & 26.90$\pm$2.43 & Danforth$^{M,*}$ \\ 
84 & h1821 & 0.26657 & 13.7$\pm$0.1 & 33.00$\pm$4.47 & Danforth$^{M,*}$ \\ 
85 & h1821 & 0.28800 & 13.4$\pm$0.1 & 29.87$\pm$4.40 & Danforth$^{M}$ \\ 
86 & h1821 & 0.29658 & 13.9$\pm$0.0 & 19.03$\pm$1.57 & Danforth$^{M,*}$ \\ 
87 & h1821 & 0.29680 & 14.0$\pm$0.0 & 36.40$\pm$2.47 & Danforth$^{M,*}$ \\ 
\hline
88 & h2356 & 0.11461 & 14.1$\pm$0.3 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
89 & h2356 & 0.16512 & 13.6$\pm$0.1 & 16.00$\pm$7.10 & Danforth$^{1032}$ \\ 
\hline
90 & he0056 & 0.16392 & 13.4$\pm$0.1 & 23.20$\pm$7.40 & Danforth$^{1032}$ \\ 
91 & he0056 & 0.16492 & 13.1$\pm$0.2 & 20.30$\pm$11.10 & Danforth$^{1032}$ \\ 
\hline
92 & he0153 & 0.13221 & 13.2$\pm$0.2 & 12.93$\pm$11.03 & Danforth$^{M}$ \\ 
93 & he0153 & 0.14844 & 13.9$\pm$0.1 & 54.10$\pm$9.43 & Danforth$^{M}$ \\ 
94 & he0153 & 0.14886 & 14.1$\pm$0.0 & 29.00$\pm$3.10 & Danforth$^{1032}$ \\ 
95 & he0153 & 0.17089 & 13.8$\pm$0.1 & 23.30$\pm$3.20 & Danforth$^{1032}$ \\ 
96 & he0153 & 0.19885 & 13.7$\pm$0.1 & 77.50$\pm$3.63 & Danforth$^{M}$ \\ 
97 & he0153 & 0.22202 & 13.6$\pm$0.1 & 18.60$\pm$7.80 & Danforth$^{1038}$ \\ 
98 & he0153 & 0.22600 & 14.2$\pm$0.0 & 33.00$\pm$2.33 & Danforth$^{M}$ \\ 
99 & he0153 & 0.29091 & 13.7$\pm$0.1 & 25.00$\pm$8.87 & Danforth$^{M}$ \\ 
100 & he0153 & 0.29115 & 13.9$\pm$0.1 & 21.77$\pm$4.43 & Danforth$^{M}$ \\ 
101 & he0153 & 0.39774 & 13.1$\pm$0.2 & 28.50$\pm$10.80 & Danforth$^{1032}$ \\ 
102 & he0153 & 0.40027 & 14.3$\pm$0.0 & 34.90$\pm$2.43 & Danforth$^{M}$ \\ 
103 & he0153 & 0.40058 & 13.4$\pm$0.2 & 20.93$\pm$8.87 & Danforth$^{M}$ \\ 
\hline
104 & he0226 & 0.01746 & 13.7$\pm$0.1 & 13.00$\pm$9.00 & Tilton \\ 
105 & he0226 & 0.02679 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
106 & he0226 & 0.04121 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
107 & he0226 & 0.04535 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
108 & he0226 & 0.04609 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
109 & he0226 & 0.06015 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
110 & he0226 & 0.06083 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
111 & he0226 & 0.07023 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
112 & he0226 & 0.08375 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
113 & he0226 & 0.08901 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
114 & he0226 & 0.08938 & 13.1$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
115 & he0226 & 0.08950 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
116 & he0226 & 0.09220 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
117 & he0226 & 0.10668 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
118 & he0226 & 0.11514 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
119 & he0226 & 0.11680 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
120 & he0226 & 0.11733 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
121 & he0226 & 0.12589 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
122 & he0226 & 0.13832 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
123 & he0226 & 0.15175 & 13.7$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
124 & he0226 & 0.15549 & 13.6$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
125 & he0226 & 0.16237 & 13.7$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
126 & he0226 & 0.16339 & 13.6$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
127 & he0226 & 0.16971 & 14.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
128 & he0226 & 0.18619 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
129 & he0226 & 0.18811 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
130 & he0226 & 0.18891 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
131 & he0226 & 0.19374 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
132 & he0226 & 0.19453 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
133 & he0226 & 0.19860 & 13.7$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
134 & he0226 & 0.20055 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
135 & he0226 & 0.20703 & 14.4$\pm$0.0 & 35.23$\pm$1.27 & Danforth$^{M,*}$ \\ 
136 & he0226 & 0.22009 & 13.0$\pm$0.1 & 11.20$\pm$6.80 & Danforth$^{1032*}$ \\ 
137 & he0226 & 0.22099 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
138 & he0226 & 0.23009 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
139 & he0226 & 0.23964 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
140 & he0226 & 0.24522 & 13.1$\pm$0.2 & 16.00$\pm$10.40 & Danforth$^{1032*}$ \\ 
141 & he0226 & 0.25099 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
142 & he0226 & 0.27155 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
143 & he0226 & 0.27956 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
144 & he0226 & 0.28041 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
145 & he0226 & 0.29134 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
146 & he0226 & 0.29213 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
147 & he0226 & 0.30939 & 13.4$\pm$0.1 & 45.90$\pm$12.00 & Danforth$^{1032*}$ \\ 
148 & he0226 & 0.31833 & 13.0$\pm$0.2 & 6.00$\pm$3.00 & Tilton \\ 
149 & he0226 & 0.33965 & 13.2$\pm$0.1 & 12.70$\pm$5.10 & Danforth$^{1032}$ \\ 
150 & he0226 & 0.34036 & 13.9$\pm$0.0 & 25.87$\pm$2.23 & Danforth$^{M,*}$ \\ 
151 & he0226 & 0.35493 & 12.9$\pm$0.3 & 13.00$\pm$9.00 & Tilton \\ 
152 & he0226 & 0.35528 & 13.7$\pm$0.1 & 34.80$\pm$4.47 & Danforth$^{M,*}$ \\ 
153 & he0226 & 0.37281 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
154 & he0226 & 0.38420 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
155 & he0226 & 0.38636 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
156 & he0226 & 0.39642 & 13.5$\pm$0.1 & 51.70$\pm$7.70 & Danforth$^{1032*}$ \\ 
157 & he0226 & 0.39692 & 13.3$\pm$0.1 & 21.80$\pm$4.50 & Danforth$^{1032}$ \\ 
158 & he0226 & 0.39890 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
159 & he0226 & 0.40034 & 13.4$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
160 & he0226 & 0.40274 & 13.3$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
161 & he0226 & 0.49225 & 14.4$\pm$0.1 & 34.93$\pm$3.37 & Danforth$^{M,*}$ \\ 
162 & he0226 & 0.49254 & 14.5$\pm$0.0 & 22.13$\pm$1.90 & Danforth$^{M,*}$ \\ 
163 & he0226 & 0.49280 & 14.0$\pm$0.2 & 27.90$\pm$22.60 & Danforth$^{M,*}$ \\ 
164 & he0226 & 0.49309 & 14.0$\pm$0.2 & 41.50$\pm$5.60 & Danforth$^{M,*}$ \\ 
\hline
165 & he0238 & 0.27918 & 13.3$\pm$0.2 & 30.20$\pm$11.20 & Danforth$^{1032}$ \\ 
166 & he0238 & 0.31404 & 13.4$\pm$0.1 & 24.10$\pm$2.80 & Danforth$^{M}$ \\ 
167 & he0238 & 0.40107 & 13.5$\pm$0.2 & 18.43$\pm$6.47 & Danforth$^{M}$ \\ 
168 & he0238 & 0.42387 & 14.4$\pm$0.0 & 52.03$\pm$3.33 & Danforth$^{M}$ \\ 
169 & he0238 & 0.42431 & 14.1$\pm$0.0 & 22.83$\pm$2.47 & Danforth$^{M}$ \\ 
170 & he0238 & 0.47203 & 14.1$\pm$0.0 & 20.47$\pm$2.27 & Danforth$^{M}$ \\ 
171 & he0238 & 0.47230 & 13.7$\pm$0.1 & 12.40$\pm$3.33 & Danforth$^{M}$ \\ 
172 & he0238 & 0.60294 & 14.2$\pm$0.1 & 66.80$\pm$13.10 & Danforth$^{1038}$ \\ 
173 & he0238 & 0.60334 & 14.1$\pm$0.0 & 80.80$\pm$9.90 & Danforth$^{1032}$ \\ 
174 & he0238 & 0.60364 & 13.7$\pm$0.3 & 33.40$\pm$18.50 & Danforth$^{1038}$ \\ 
175 & he0238 & 0.60431 & 14.5$\pm$0.2 & 87.40$\pm$28.37 & Danforth$^{M}$ \\ 
176 & he0238 & 0.60493 & 14.1$\pm$0.4 & 65.60$\pm$25.90 & Danforth$^{M}$ \\ 
177 & he0238 & 0.60912 & 14.5$\pm$0.1 & 89.80$\pm$7.20 & Danforth$^{1032}$ \\ 
178 & he0238 & 0.60938 & 14.7$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
179 & he0238 & 0.61015 & 14.3$\pm$0.1 & 79.00$\pm$9.90 & Danforth$^{1032}$ \\ 
180 & he0238 & 0.61091 & 13.8$\pm$0.1 & 29.33$\pm$6.20 & Danforth$^{M}$ \\ 
\hline
181 & he0435 & 0.24490 & 13.9$\pm$0.2 & 33.73$\pm$13.93 & Danforth$^{M}$ \\ 
182 & he0435 & 0.29849 & 13.8$\pm$0.2 & 37.40$\pm$9.40 & Danforth$^{1032}$ \\ 
183 & he0435 & 0.31319 & 14.0$\pm$0.1 & 10.97$\pm$3.67 & Danforth$^{M}$ \\ 
184 & he0435 & 0.39225 & 14.1$\pm$0.1 & 46.67$\pm$9.80 & Danforth$^{M}$ \\ 
185 & he0435 & 0.39266 & 14.0$\pm$0.1 & 33.97$\pm$7.67 & Danforth$^{M}$ \\ 
186 & he0435 & 0.40921 & 14.1$\pm$0.1 & 80.33$\pm$9.80 & Danforth$^{M}$ \\ 
187 & he0435 & 0.40997 & 14.5$\pm$0.0 & 58.83$\pm$4.13 & Danforth$^{M}$ \\ 
\hline
188 & hs0624 & 0.06342 & 14.2$\pm$0.2 & 57.10$\pm$21.60 & Tilton \\ 
189 & hs0624 & 0.07573 & 13.9$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
190 & hs0624 & 0.20482 & 13.4$\pm$0.2 & 28.00$\pm$12.00 & Tilton \\ 
191 & hs0624 & 0.20531 & 13.1$\pm$0.2 & 20.00$\pm$0.00 & Tilton \\ 
192 & hs0624 & 0.21134 & 13.1$\pm$0.2 & 20.00$\pm$0.00 & Tilton \\ 
193 & hs0624 & 0.22329 & 13.0$\pm$0.4 & 11.00$\pm$0.00 & Tilton \\ 
194 & hs0624 & 0.25230 & 13.2$\pm$0.1 & 27.00$\pm$8.80 & Tilton \\ 
195 & hs0624 & 0.29984 & 13.1$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
196 & hs0624 & 0.31794 & 13.7$\pm$0.1 & 29.00$\pm$1.60 & Tilton \\ 
197 & hs0624 & 0.33980 & 13.5$\pm$0.1 & 37.30$\pm$5.30 & Tilton \\ 
198 & hs0624 & 0.34863 & 13.1$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
199 & hs0624 & 0.37034 & 12.8$\pm$0.2 & 8.00$\pm$3.70 & Tilton \\ 
200 & hs0624 & 0.37058 & 13.6$\pm$0.0 & 19.90$\pm$2.40 & Tilton \\ 
201 & hs0624 & 0.37095 & 13.6$\pm$0.0 & 24.40$\pm$1.90 & Tilton \\ 
\hline
202 & hs1102 & 0.20136 & 13.2$\pm$0.2 & 22.10$\pm$6.40 & Danforth$^{1032}$ \\ 
203 & hs1102 & 0.20653 & 14.2$\pm$0.0 & 33.33$\pm$3.60 & Danforth$^{M}$ \\ 
204 & hs1102 & 0.23882 & 14.8$\pm$0.0 & 34.53$\pm$1.97 & Danforth$^{M}$ \\ 
205 & hs1102 & 0.26162 & 14.0$\pm$0.3 & 34.10$\pm$12.40 & Danforth$^{1038}$ \\ 
206 & hs1102 & 0.28902 & 13.8$\pm$0.1 & 56.10$\pm$13.20 & Danforth$^{1032}$ \\ 
207 & hs1102 & 0.28924 & 13.6$\pm$0.2 & 34.20$\pm$10.70 & Danforth$^{1032}$ \\ 
208 & hs1102 & 0.28974 & 14.2$\pm$0.1 & 38.27$\pm$5.27 & Danforth$^{M}$ \\ 
209 & hs1102 & 0.31046 & 14.3$\pm$0.0 & 28.27$\pm$2.40 & Danforth$^{M}$ \\ 
210 & hs1102 & 0.33619 & 13.5$\pm$0.3 & 43.20$\pm$19.60 & Danforth$^{1032}$ \\ 
211 & hs1102 & 0.38188 & 13.9$\pm$0.1 & 30.13$\pm$3.73 & Danforth$^{M}$ \\ 
212 & hs1102 & 0.40794 & 13.8$\pm$0.1 & 33.83$\pm$7.57 & Danforth$^{M}$ \\ 
213 & hs1102 & 0.40978 & 14.1$\pm$0.0 & 73.60$\pm$4.67 & Danforth$^{M}$ \\ 
214 & hs1102 & 0.43768 & 13.8$\pm$0.1 & 18.33$\pm$4.63 & Danforth$^{M}$ \\ 
215 & hs1102 & 0.43807 & 14.1$\pm$0.0 & 32.73$\pm$4.77 & Danforth$^{M}$ \\ 
216 & hs1102 & 0.48393 & 14.3$\pm$0.1 & 51.90$\pm$7.10 & Danforth$^{M}$ \\ 
217 & hs1102 & 0.48432 & 14.3$\pm$0.1 & 44.13$\pm$8.17 & Danforth$^{M}$ \\ 
218 & hs1102 & 0.48495 & 14.4$\pm$0.1 & 96.90$\pm$22.80 & Danforth$^{1032}$ \\ 
219 & hs1102 & 0.48525 & 14.3$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
220 & hs1102 & 0.48637 & 14.5$\pm$0.0 & 77.80$\pm$6.10 & Danforth$^{1038}$ \\ 
221 & hs1102 & 0.50606 & 13.8$\pm$0.1 & 61.60$\pm$8.90 & Danforth$^{1032}$ \\ 
\hline
222 & i22456 & 0.09858 & 14.7$\pm$0.0 & 48.70$\pm$2.10 & Danforth$^{M}$ \\ 
223 & i22456 & 0.09895 & 14.4$\pm$0.1 & 33.80$\pm$5.00 & Danforth$^{1032}$ \\ 
224 & i22456 & 0.09931 & 14.9$\pm$0.0 & 70.37$\pm$3.90 & Danforth$^{M}$ \\ 
225 & i22456 & 0.09959 & 14.0$\pm$0.0 & 9.60$\pm$2.30 & Danforth$^{1038}$ \\ 
226 & i22456 & 0.09989 & 14.8$\pm$0.0 & 34.57$\pm$1.37 & Danforth$^{M}$ \\ 
227 & i22456 & 0.10034 & 14.7$\pm$0.0 & 50.57$\pm$1.80 & Danforth$^{M}$ \\ 
228 & i22456 & 0.10101 & 15.4$\pm$0.0 & 55.57$\pm$1.30 & Danforth$^{M}$ \\ 
229 & i22456 & 0.10146 & 14.0$\pm$0.0 & 23.20$\pm$3.90 & Danforth$^{1032}$ \\ 
\hline
230 & mr2251 & 0.01070 & 13.4$\pm$0.2 & 14.00$\pm$0.00 & Tilton \\ 
\hline
231 & mrk421 & 0.01009 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
\hline
232 & mrk876 & 0.00311 & 13.6$\pm$0.1 & 25.00$\pm$6.00 & Tilton \\ 
233 & mrk876 & 0.06248 & 13.6$\pm$0.1 & 35.00$\pm$2.00 & Tilton \\ 
234 & mrk876 & 0.08579 & 14.1$\pm$0.1 & 51.00$\pm$5.20 & Tilton \\ 
235 & mrk876 & 0.11488 & 14.4$\pm$0.0 & 45.47$\pm$1.90 & Danforth$^{M,*}$ \\ 
236 & mrk876 & 0.11517 & 13.7$\pm$0.1 & 52.93$\pm$9.30 & Danforth$^{M}$ \\ 
237 & mrk876 & 0.11588 & 14.2$\pm$0.0 & 28.67$\pm$1.47 & Danforth$^{M,*}$ \\ 
\hline
238 & ngc7469 & 0.00962 & 14.1$\pm$0.1 & 28.60$\pm$6.00 & Tilton \\ 
239 & ngc7469 & 0.00994 & 14.7$\pm$0.0 & 41.60$\pm$3.00 & Tilton \\ 
240 & ngc7469 & 0.01153 & 13.4$\pm$0.2 & 19.00$\pm$10.00 & Tilton \\ 
\hline
241 & p1103 & 0.13556 & 13.8$\pm$0.2 & 83.50$\pm$26.10 & Danforth$^{1032}$ \\ 
242 & p1103 & 0.13937 & 13.7$\pm$0.2 & 20.60$\pm$11.00 & Danforth$^{M}$ \\ 
243 & p1103 & 0.14099 & 13.6$\pm$0.2 & 11.97$\pm$10.70 & Danforth$^{M}$ \\ 
244 & p1103 & 0.14126 & 14.2$\pm$0.1 & 55.50$\pm$13.50 & Danforth$^{M}$ \\ 
245 & p1103 & 0.17277 & 14.1$\pm$0.0 & 28.30$\pm$0.50 & Danforth$^{1032}$ \\ 
\hline
246 & pg0003 & 0.16521 & 13.8$\pm$0.2 & 61.03$\pm$13.67 & Danforth$^{M}$ \\ 
247 & pg0003 & 0.20907 & 13.7$\pm$0.1 & 34.10$\pm$5.70 & Danforth$^{1032}$ \\ 
248 & pg0003 & 0.29021 & 14.2$\pm$0.0 & 37.30$\pm$4.67 & Danforth$^{M}$ \\ 
249 & pg0003 & 0.30551 & 13.2$\pm$0.2 & 22.40$\pm$16.30 & Danforth$^{1032}$ \\ 
250 & pg0003 & 0.30569 & 13.3$\pm$0.2 & 19.00$\pm$13.73 & Danforth$^{M}$ \\ 
251 & pg0003 & 0.34757 & 14.3$\pm$0.0 & 29.47$\pm$2.60 & Danforth$^{M}$ \\ 
252 & pg0003 & 0.34788 & 13.9$\pm$0.1 & 15.47$\pm$2.70 & Danforth$^{M}$ \\ 
253 & pg0003 & 0.36452 & 14.3$\pm$0.0 & 40.43$\pm$2.30 & Danforth$^{M}$ \\ 
254 & pg0003 & 0.36508 & 14.5$\pm$0.0 & 27.60$\pm$1.40 & Danforth$^{1032}$ \\ 
255 & pg0003 & 0.36572 & 14.1$\pm$0.1 & 36.17$\pm$5.43 & Danforth$^{M}$ \\ 
256 & pg0003 & 0.36621 & 14.1$\pm$0.0 & 30.53$\pm$2.53 & Danforth$^{M}$ \\ 
257 & pg0003 & 0.37029 & 13.6$\pm$0.1 & 61.60$\pm$11.50 & Danforth$^{1032}$ \\ 
258 & pg0003 & 0.38608 & 13.8$\pm$0.1 & 23.83$\pm$4.10 & Danforth$^{M}$ \\ 
259 & pg0003 & 0.38639 & 13.9$\pm$0.1 & 36.77$\pm$5.90 & Danforth$^{M}$ \\ 
260 & pg0003 & 0.40138 & 14.3$\pm$0.0 & 32.80$\pm$1.87 & Danforth$^{M}$ \\ 
261 & pg0003 & 0.42192 & 14.3$\pm$0.0 & 27.67$\pm$1.97 & Danforth$^{M}$ \\ 
\hline
262 & pg0157 & 0.14621 & 13.4$\pm$0.2 & 13.10$\pm$9.40 & Danforth$^{1032}$ \\ 
\hline
263 & pg0804 & 0.00382 & 13.5$\pm$0.2 & 17.00$\pm$0.00 & Tilton \\ 
264 & pg0804 & 0.01851 & 13.2$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
265 & pg0804 & 0.10216 & 14.2$\pm$0.0 & 50.03$\pm$3.87 & Danforth$^{M}$ \\ 
266 & pg0804 & 0.10230 & 14.0$\pm$0.1 & 34.30$\pm$3.10 & Tilton \\ 
\hline
267 & pg0832 & 0.10772 & 13.5$\pm$0.0 & 17.80$\pm$1.00 & Danforth$^{1038}$ \\ 
268 & pg0832 & 0.13230 & 14.0$\pm$0.2 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
269 & pg0832 & 0.15276 & 13.8$\pm$0.2 & 52.20$\pm$20.10 & Danforth$^{1032}$ \\ 
270 & pg0832 & 0.23308 & 13.8$\pm$0.2 & 54.30$\pm$14.80 & Danforth$^{1032}$ \\ 
271 & pg0832 & 0.32567 & 14.1$\pm$0.1 & 60.83$\pm$7.80 & Danforth$^{M}$ \\ 
\hline
272 & pg0953 & 0.01560 & 13.7$\pm$0.2 & 11.00$\pm$0.00 & Tilton \\ 
273 & pg0953 & 0.05891 & 13.9$\pm$0.1 & 26.00$\pm$8.00 & Tilton \\ 
274 & pg0953 & 0.06807 & 14.3$\pm$0.1 & 13.50$\pm$1.80 & Tilton \\ 
275 & pg0953 & 0.11827 & 13.3$\pm$0.2 & 12.00$\pm$0.00 & Tilton \\ 
276 & pg0953 & 0.14236 & 14.0$\pm$0.0 & 20.63$\pm$2.37 & Danforth$^{M,*}$ \\ 
277 & pg0953 & 0.14263 & 13.6$\pm$0.1 & 27.17$\pm$5.87 & Danforth$^{M}$ \\ 
278 & pg0953 & 0.14307 & 13.3$\pm$0.1 & 36.43$\pm$4.63 & Danforth$^{M}$ \\ 
279 & pg0953 & 0.22967 & 13.9$\pm$0.0 & 33.97$\pm$2.37 & Danforth$^{M,*}$ \\ 
280 & pg0953 & 0.23251 & 13.4$\pm$0.1 & 19.20$\pm$2.80 & Danforth$^{1032}$ \\ 
281 & pg0953 & 0.23351 & 13.5$\pm$0.1 & 10.53$\pm$2.40 & Danforth$^{M,*}$ \\ 
\hline
282 & pg1001 & 0.13773 & 14.1$\pm$0.1 & 47.30$\pm$5.93 & Danforth$^{M}$ \\ 
283 & pg1001 & 0.21259 & 13.4$\pm$0.1 & 24.70$\pm$6.70 & Danforth$^{1032}$ \\ 
284 & pg1001 & 0.27333 & 13.3$\pm$0.2 & 20.07$\pm$10.07 & Danforth$^{M}$ \\ 
285 & pg1001 & 0.33018 & 14.2$\pm$0.1 & 10.67$\pm$1.20 & Danforth$^{M}$ \\ 
\hline
286 & pg1049 & 0.19406 & 13.7$\pm$0.2 & 27.60$\pm$11.37 & Danforth$^{M}$ \\ 
287 & pg1049 & 0.32490 & 13.7$\pm$0.3 & 51.80$\pm$15.80 & Danforth$^{M}$ \\ 
288 & pg1049 & 0.32545 & 13.7$\pm$0.1 & 54.40$\pm$20.30 & Danforth$^{1032}$ \\ 
289 & pg1049 & 0.32569 & 14.4$\pm$0.1 & 82.60$\pm$20.60 & Danforth$^{1038}$ \\ 
290 & pg1049 & 0.33481 & 14.4$\pm$0.1 & 90.00$\pm$13.50 & Danforth$^{1032}$ \\ 
291 & pg1049 & 0.33531 & 14.5$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
292 & pg1049 & 0.33904 & 14.1$\pm$0.1 & 51.63$\pm$8.57 & Danforth$^{M}$ \\ 
293 & pg1049 & 0.34006 & 15.1$\pm$0.0 & 80.77$\pm$4.07 & Danforth$^{M}$ \\ 
294 & pg1049 & 0.34096 & 14.9$\pm$0.0 & 80.10$\pm$7.43 & Danforth$^{M}$ \\ 
295 & pg1049 & 0.34181 & 15.1$\pm$0.0 & 68.97$\pm$4.83 & Danforth$^{M}$ \\ 
296 & pg1049 & 0.34260 & 14.6$\pm$0.0 & 76.90$\pm$10.43 & Danforth$^{M}$ \\ 
\hline
297 & pg1115 & 0.12285 & 13.6$\pm$0.2 & 28.67$\pm$12.13 & Danforth$^{M}$ \\ 
298 & pg1115 & 0.12313 & 13.8$\pm$0.1 & 29.87$\pm$11.33 & Danforth$^{M}$ \\ 
299 & pg1115 & 0.13104 & 14.0$\pm$0.1 & 39.40$\pm$6.13 & Danforth$^{M}$ \\ 
300 & pg1115 & 0.15456 & 14.3$\pm$0.1 & 27.37$\pm$3.57 & Danforth$^{M}$ \\ 
301 & pg1115 & 0.15467 & 14.7$\pm$0.0 & 26.50$\pm$2.00 & Danforth$^{1032}$ \\ 
\hline
302 & pg1116 & 0.05900 & 13.5$\pm$0.2 & 20.00$\pm$4.00 & Tilton \\ 
303 & pg1116 & 0.05927 & 13.5$\pm$0.2 & 12.30$\pm$5.70 & Tilton \\ 
304 & pg1116 & 0.11895 & 13.6$\pm$0.2 & 78.90$\pm$17.40 & Danforth$^{1032}$ \\ 
305 & pg1116 & 0.13852 & 13.8$\pm$0.1 & 33.87$\pm$4.00 & Danforth$^{M,*}$ \\ 
306 & pg1116 & 0.16539 & 13.7$\pm$0.3 & 35.07$\pm$16.97 & Danforth$^{M}$ \\ 
307 & pg1116 & 0.16554 & 13.9$\pm$0.1 & 20.70$\pm$3.20 & Danforth$^{M,*}$ \\ 
308 & pg1116 & 0.16610 & 13.6$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
309 & pg1116 & 0.16686 & 13.5$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
310 & pg1116 & 0.17343 & 13.3$\pm$0.1 & 40.90$\pm$8.80 & Danforth$^{1032*}$ \\ 
\hline
311 & pg1121 & 0.19245 & 13.4$\pm$0.1 & 17.10$\pm$7.70 & Danforth$^{1032}$ \\ 
312 & pg1121 & 0.21986 & 14.3$\pm$0.0 & 43.00$\pm$2.60 & Danforth$^{M}$ \\ 
\hline
313 & pg1211 & 0.00711 & 13.8$\pm$0.1 & 41.00$\pm$7.00 & Tilton \\ 
314 & pg1211 & 0.05117 & 14.3$\pm$0.1 & 53.00$\pm$9.50 & Tilton \\ 
315 & pg1211 & 0.06449 & 14.1$\pm$0.0 & 47.20$\pm$5.40 & Tilton \\ 
316 & pg1211 & 0.06491 & 13.7$\pm$0.1 & 26.60$\pm$5.10 & Tilton \\ 
\hline
317 & pg1216 & 0.12362 & 14.2$\pm$0.1 & 32.10$\pm$7.27 & Danforth$^{M,*}$ \\ 
318 & pg1216 & 0.12389 & 14.1$\pm$0.1 & 32.43$\pm$8.73 & Danforth$^{M,*}$ \\ 
319 & pg1216 & 0.12463 & 13.8$\pm$0.5 & 6.00$\pm$41.00 & Tilton \\ 
320 & pg1216 & 0.12485 & 14.2$\pm$0.1 & 60.00$\pm$9.03 & Danforth$^{M,*}$ \\ 
321 & pg1216 & 0.13499 & 13.8$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
322 & pg1216 & 0.26768 & 13.7$\pm$0.6 & 19.00$\pm$2.00 & Tilton \\ 
323 & pg1216 & 0.28199 & 13.8$\pm$0.2 & 47.17$\pm$11.20 & Danforth$^{M}$ \\ 
324 & pg1216 & 0.28237 & 13.6$\pm$0.1 & 14.43$\pm$5.40 & Danforth$^{M}$ \\ 
\hline
325 & pg1222 & 0.16715 & 13.5$\pm$0.2 & 5.00$\pm$0.00 & Danforth$^{M}$ \\ 
326 & pg1222 & 0.22263 & 13.9$\pm$0.1 & 30.47$\pm$5.77 & Danforth$^{M}$ \\ 
327 & pg1222 & 0.24184 & 14.2$\pm$0.2 & 30.10$\pm$7.80 & Danforth$^{M}$ \\ 
328 & pg1222 & 0.24454 & 14.1$\pm$0.1 & 25.13$\pm$4.17 & Danforth$^{M}$ \\ 
329 & pg1222 & 0.34686 & 13.6$\pm$0.2 & 30.17$\pm$10.03 & Danforth$^{M}$ \\ 
330 & pg1222 & 0.34941 & 13.8$\pm$0.1 & 42.37$\pm$6.20 & Danforth$^{M}$ \\ 
331 & pg1222 & 0.36375 & 13.6$\pm$0.1 & 32.13$\pm$6.67 & Danforth$^{M}$ \\ 
332 & pg1222 & 0.37616 & 13.5$\pm$0.1 & 31.60$\pm$5.70 & Danforth$^{1032}$ \\ 
333 & pg1222 & 0.37706 & 13.8$\pm$0.1 & 28.53$\pm$4.93 & Danforth$^{M}$ \\ 
334 & pg1222 & 0.37730 & 13.5$\pm$0.1 & 29.83$\pm$8.23 & Danforth$^{M}$ \\ 
335 & pg1222 & 0.37842 & 14.1$\pm$0.0 & 38.97$\pm$3.43 & Danforth$^{M}$ \\ 
336 & pg1222 & 0.37869 & 13.4$\pm$0.1 & 19.37$\pm$6.13 & Danforth$^{M}$ \\ 
337 & pg1222 & 0.39726 & 13.1$\pm$0.2 & 34.50$\pm$6.40 & Danforth$^{1032}$ \\ 
338 & pg1222 & 0.40828 & 13.1$\pm$0.2 & 30.50$\pm$12.70 & Danforth$^{1032}$ \\ 
339 & pg1222 & 0.42130 & 13.9$\pm$0.1 & 32.20$\pm$3.97 & Danforth$^{M}$ \\ 
340 & pg1222 & 0.42308 & 14.0$\pm$0.0 & 18.77$\pm$1.97 & Danforth$^{M}$ \\ 
\hline
341 & pg1259 & 0.00220 & 13.6$\pm$0.1 & 75.00$\pm$0.00 & Tilton \\ 
342 & pg1259 & 0.00762 & 13.3$\pm$0.1 & 24.00$\pm$16.00 & Tilton \\ 
343 & pg1259 & 0.02217 & 13.4$\pm$0.2 & 34.00$\pm$15.00 & Tilton \\ 
344 & pg1259 & 0.04606 & 13.9$\pm$0.1 & 39.00$\pm$12.00 & Tilton \\ 
345 & pg1259 & 0.04650 & 13.8$\pm$0.1 & 24.00$\pm$4.00 & Tilton \\ 
346 & pg1259 & 0.19576 & 13.7$\pm$0.1 & 21.90$\pm$3.57 & Danforth$^{M}$ \\ 
347 & pg1259 & 0.21940 & 14.1$\pm$0.0 & 38.30$\pm$2.60 & Danforth$^{M,*}$ \\ 
348 & pg1259 & 0.21953 & 13.6$\pm$0.1 & 14.20$\pm$2.00 & Tilton \\ 
349 & pg1259 & 0.22313 & 13.6$\pm$0.1 & 50.50$\pm$17.50 & Tilton \\ 
350 & pg1259 & 0.23284 & 13.5$\pm$0.1 & 17.00$\pm$8.00 & Tilton \\ 
351 & pg1259 & 0.23956 & 13.4$\pm$0.1 & 24.00$\pm$7.20 & Danforth$^{1032}$ \\ 
352 & pg1259 & 0.25973 & 13.8$\pm$0.1 & 52.70$\pm$7.60 & Danforth$^{1032*}$ \\ 
353 & pg1259 & 0.31979 & 13.3$\pm$0.1 & 17.67$\pm$6.13 & Danforth$^{M,*}$ \\ 
354 & pg1259 & 0.32472 & 13.3$\pm$0.1 & 14.00$\pm$8.00 & Tilton \\ 
\hline
355 & pg1307 & 0.14187 & 13.9$\pm$0.1 & 42.03$\pm$12.67 & Danforth$^{M}$ \\ 
356 & pg1307 & 0.14214 & 13.8$\pm$0.1 & 15.90$\pm$5.07 & Danforth$^{M}$ \\ 
\hline
357 & pg1309 & 0.17586 & 14.4$\pm$0.1 & 30.50$\pm$2.27 & Danforth$^{M}$ \\ 
358 & pg1309 & 0.17745 & 15.2$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
359 & pg1309 & 0.17866 & 15.9$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
360 & pg1309 & 0.17930 & 15.5$\pm$0.0 & 99.60$\pm$8.20 & Danforth$^{1038}$ \\ 
361 & pg1309 & 0.17979 & 15.2$\pm$0.0 & 73.60$\pm$7.20 & Danforth$^{1038}$ \\ 
362 & pg1309 & 0.18069 & 15.2$\pm$0.0 & 74.20$\pm$3.50 & Danforth$^{1038}$ \\ 
363 & pg1309 & 0.18117 & 15.1$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
364 & pg1309 & 0.18139 & 14.9$\pm$0.0 & 60.00$\pm$5.30 & Danforth$^{1038}$ \\ 
365 & pg1309 & 0.18145 & 14.8$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
366 & pg1309 & 0.18192 & 14.3$\pm$0.0 & 69.60$\pm$5.60 & Danforth$^{1032}$ \\ 
367 & pg1309 & 0.18698 & 14.0$\pm$2.5 & 28.00$\pm$9.90 & Danforth$^{1038}$ \\ 
\hline
368 & pg1424 & 0.12120 & 14.0$\pm$0.2 & 41.30$\pm$23.90 & Danforth$^{1032}$ \\ 
369 & pg1424 & 0.12152 & 14.4$\pm$0.1 & 32.17$\pm$4.43 & Danforth$^{M}$ \\ 
370 & pg1424 & 0.14689 & 13.9$\pm$0.2 & 48.13$\pm$19.27 & Danforth$^{M}$ \\ 
371 & pg1424 & 0.14712 & 13.7$\pm$0.2 & 16.20$\pm$9.30 & Danforth$^{1032}$ \\ 
372 & pg1424 & 0.33947 & 13.5$\pm$0.1 & 18.20$\pm$8.27 & Danforth$^{M}$ \\ 
373 & pg1424 & 0.33988 & 13.6$\pm$0.1 & 13.77$\pm$4.37 & Danforth$^{M}$ \\ 
374 & pg1424 & 0.38633 & 13.8$\pm$0.1 & 33.53$\pm$10.60 & Danforth$^{M}$ \\ 
375 & pg1424 & 0.38662 & 14.1$\pm$0.0 & 24.13$\pm$1.90 & Danforth$^{M}$ \\ 
376 & pg1424 & 0.42884 & 13.1$\pm$0.1 & 7.10$\pm$9.80 & Danforth$^{1032}$ \\ 
377 & pg1424 & 0.60369 & 13.4$\pm$0.1 & 10.10$\pm$5.60 & Danforth$^{1032}$ \\ 
\hline
378 & pg1444 & 0.22031 & 13.9$\pm$0.1 & 49.00$\pm$2.00 & Tilton \\ 
379 & pg1444 & 0.22676 & 13.3$\pm$0.1 & 27.00$\pm$5.00 & Tilton \\ 
380 & pg1444 & 0.26690 & 13.8$\pm$0.0 & 11.50$\pm$1.00 & Tilton \\ 
381 & pg1444 & 0.26728 & 13.5$\pm$0.1 & 14.90$\pm$3.80 & Tilton \\ 
382 & pg1444 & 0.26738 & 13.9$\pm$0.1 & 8.40$\pm$1.30 & Tilton \\ 
383 & pg1444 & 0.26747 & 13.5$\pm$0.1 & 11.90$\pm$2.90 & Tilton \\ 
\hline
384 & pg1626 & 0.13075 & 13.3$\pm$0.2 & 31.40$\pm$11.10 & Danforth$^{1032}$ \\ 
\hline
385 & phl1811 & 0.07344 & 13.0$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
386 & phl1811 & 0.07768 & 13.6$\pm$0.1 & 31.00$\pm$16.00 & Tilton \\ 
387 & phl1811 & 0.08131 & 13.9$\pm$0.2 & 7.90$\pm$5.20 & Tilton \\ 
388 & phl1811 & 0.13239 & 13.9$\pm$0.1 & 59.27$\pm$10.23 & Danforth$^{M,*}$ \\ 
389 & phl1811 & 0.13282 & 13.6$\pm$0.1 & 21.07$\pm$5.73 & Danforth$^{M,*}$ \\ 
390 & phl1811 & 0.13318 & 13.7$\pm$0.1 & 37.63$\pm$5.97 & Danforth$^{M,*}$ \\ 
391 & phl1811 & 0.13545 & 13.5$\pm$0.2 & 32.80$\pm$11.30 & Danforth$^{1038}$ \\ 
392 & phl1811 & 0.15752 & 13.5$\pm$0.1 & 37.03$\pm$10.37 & Danforth$^{M}$ \\ 
393 & phl1811 & 0.15786 & 13.6$\pm$0.1 & 29.03$\pm$5.83 & Danforth$^{M,*}$ \\ 
394 & phl1811 & 0.17652 & 14.1$\pm$0.0 & 18.10$\pm$2.20 & Danforth$^{1038*}$ \\ 
395 & phl1811 & 0.19157 & 13.5$\pm$0.1 & 23.37$\pm$5.17 & Danforth$^{M,*}$ \\ 
396 & phl1811 & 0.19194 & 14.7$\pm$0.0 & 34.87$\pm$1.70 & Danforth$^{M,*}$ \\ 
397 & phl1811 & 0.19220 & 13.6$\pm$0.2 & 30.30$\pm$17.47 & Danforth$^{M,*}$ \\ 
\hline
398 & phl2525 & 0.20154 & 14.1$\pm$0.0 & 19.40$\pm$2.13 & Danforth$^{M}$ \\ 
399 & phl2525 & 0.20207 & 13.6$\pm$0.1 & 19.13$\pm$4.60 & Danforth$^{M}$ \\ 
400 & phl2525 & 0.20605 & 14.0$\pm$0.1 & 39.73$\pm$6.70 & Danforth$^{M}$ \\ 
\hline
401 & pks0312 & 0.20188 & 13.8$\pm$0.1 & 40.00$\pm$0.00 & Tilton \\ 
402 & pks0312 & 0.20275 & 14.9$\pm$0.1 & 65.40$\pm$1.30 & Tilton \\ 
\hline
403 & pks0405 & 0.09192 & 13.8$\pm$0.0 & 25.00$\pm$10.00 & Tilton \\ 
404 & pks0405 & 0.09647 & 13.7$\pm$0.3 & 31.30$\pm$7.60 & Danforth$^{1038*}$ \\ 
405 & pks0405 & 0.14808 & 13.7$\pm$0.0 & 85.07$\pm$1.67 & Danforth$^{M}$ \\ 
406 & pks0405 & 0.16566 & 13.0$\pm$0.2 & 7.90$\pm$8.10 & Danforth$^{1038}$ \\ 
407 & pks0405 & 0.16606 & 14.1$\pm$0.0 & 74.20$\pm$3.20 & Danforth$^{1032*}$ \\ 
408 & pks0405 & 0.16659 & 13.9$\pm$0.1 & 31.20$\pm$4.70 & Danforth$^{M}$ \\ 
409 & pks0405 & 0.16688 & 14.2$\pm$0.1 & 40.33$\pm$8.93 & Danforth$^{M}$ \\ 
410 & pks0405 & 0.16712 & 14.4$\pm$0.1 & 36.90$\pm$3.03 & Danforth$^{M,*}$ \\ 
411 & pks0405 & 0.18257 & 13.7$\pm$2.0 & 34.70$\pm$4.97 & Danforth$^{M,*}$ \\ 
412 & pks0405 & 0.18289 & 13.8$\pm$0.6 & 18.53$\pm$1.47 & Danforth$^{M,*}$ \\ 
413 & pks0405 & 0.24052 & 13.5$\pm$0.1 & 33.60$\pm$4.30 & Danforth$^{M}$ \\ 
414 & pks0405 & 0.24094 & 13.0$\pm$0.1 & 26.00$\pm$7.80 & Danforth$^{1032}$ \\ 
415 & pks0405 & 0.24547 & 12.7$\pm$0.2 & 8.40$\pm$7.70 & Danforth$^{1032}$ \\ 
416 & pks0405 & 0.29762 & 13.6$\pm$0.1 & 66.87$\pm$6.50 & Danforth$^{M}$ \\ 
417 & pks0405 & 0.34188 & 13.5$\pm$0.0 & 37.30$\pm$3.50 & Danforth$^{1032}$ \\ 
418 & pks0405 & 0.34225 & 13.3$\pm$0.0 & 24.00$\pm$3.40 & Danforth$^{1032}$ \\ 
419 & pks0405 & 0.35092 & 13.3$\pm$0.2 & 35.00$\pm$7.00 & Tilton \\ 
420 & pks0405 & 0.36075 & 13.2$\pm$0.0 & 29.60$\pm$4.30 & Danforth$^{1032*}$ \\ 
421 & pks0405 & 0.36151 & 13.9$\pm$0.0 & 32.17$\pm$1.43 & Danforth$^{M,*}$ \\ 
422 & pks0405 & 0.36329 & 13.5$\pm$0.0 & 17.97$\pm$1.67 & Danforth$^{M,*}$ \\ 
423 & pks0405 & 0.40570 & 13.6$\pm$0.0 & 0.00$\pm$0.00 & Tilton \\ 
424 & pks0405 & 0.40890 & 13.2$\pm$0.1 & 36.93$\pm$6.70 & Danforth$^{M}$ \\ 
425 & pks0405 & 0.49505 & 14.3$\pm$0.0 & 32.50$\pm$2.53 & Danforth$^{M,*}$ \\ 
426 & pks0405 & 0.49530 & 13.8$\pm$0.1 & 15.97$\pm$2.63 & Danforth$^{M,*}$ \\ 
427 & pks0405 & 0.55506 & 14.0$\pm$0.1 & 27.90$\pm$3.13 & Danforth$^{M}$ \\ 
\hline
428 & pks0552 & 0.11067 & 13.9$\pm$0.1 & 33.60$\pm$12.30 & Danforth$^{1038}$ \\ 
429 & pks0552 & 0.14861 & 13.6$\pm$0.1 & 13.50$\pm$5.50 & Danforth$^{1032}$ \\ 
430 & pks0552 & 0.14893 & 13.8$\pm$0.1 & 45.80$\pm$11.50 & Danforth$^{1032}$ \\ 
431 & pks0552 & 0.18726 & 13.7$\pm$0.1 & 31.40$\pm$9.30 & Danforth$^{1032}$ \\ 
432 & pks0552 & 0.25380 & 13.5$\pm$1.6 & 25.17$\pm$7.50 & Danforth$^{M}$ \\ 
433 & pks0552 & 0.27850 & 13.7$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
434 & pks0552 & 0.28570 & 13.8$\pm$0.1 & 28.40$\pm$4.63 & Danforth$^{M}$ \\ 
435 & pks0552 & 0.34489 & 13.1$\pm$0.2 & 27.30$\pm$8.10 & Danforth$^{1032}$ \\ 
436 & pks0552 & 0.37621 & 13.6$\pm$0.1 & 43.90$\pm$10.17 & Danforth$^{M}$ \\ 
437 & pks0552 & 0.37655 & 13.6$\pm$0.1 & 25.20$\pm$4.93 & Danforth$^{M}$ \\ 
438 & pks0552 & 0.37974 & 13.1$\pm$0.1 & 24.50$\pm$8.30 & Danforth$^{1032}$ \\ 
439 & pks0552 & 0.39346 & 13.3$\pm$0.1 & 21.30$\pm$6.50 & Danforth$^{1032}$ \\ 
440 & pks0552 & 0.42511 & 13.2$\pm$0.2 & 25.40$\pm$12.60 & Danforth$^{1032}$ \\ 
441 & pks0552 & 0.44610 & 13.6$\pm$0.1 & 24.83$\pm$6.53 & Danforth$^{M}$ \\ 
442 & pks0552 & 0.59449 & 13.4$\pm$0.1 & 10.20$\pm$4.60 & Danforth$^{1032}$ \\ 
443 & pks0552 & 0.63163 & 13.8$\pm$0.1 & 8.83$\pm$3.73 & Danforth$^{M}$ \\ 
444 & pks0552 & 0.63186 & 13.9$\pm$0.1 & 14.10$\pm$3.10 & Danforth$^{M}$ \\ 
\hline
445 & pks0637 & 0.12291 & 14.1$\pm$0.1 & 43.87$\pm$5.67 & Danforth$^{M}$ \\ 
446 & pks0637 & 0.14420 & 13.8$\pm$0.1 & 29.30$\pm$10.30 & Danforth$^{1038}$ \\ 
447 & pks0637 & 0.16107 & 14.1$\pm$0.1 & 52.77$\pm$7.50 & Danforth$^{M}$ \\ 
448 & pks0637 & 0.20475 & 13.6$\pm$0.2 & 48.57$\pm$15.07 & Danforth$^{M}$ \\ 
449 & pks0637 & 0.24873 & 14.0$\pm$0.1 & 62.50$\pm$13.40 & Danforth$^{1038}$ \\ 
450 & pks0637 & 0.30079 & 13.8$\pm$0.1 & 25.77$\pm$7.70 & Danforth$^{M}$ \\ 
451 & pks0637 & 0.30107 & 14.0$\pm$0.0 & 26.20$\pm$2.80 & Danforth$^{1032}$ \\ 
452 & pks0637 & 0.38642 & 13.8$\pm$0.1 & 28.77$\pm$3.97 & Danforth$^{M}$ \\ 
453 & pks0637 & 0.40897 & 13.8$\pm$0.1 & 60.60$\pm$18.20 & Danforth$^{1038}$ \\ 
454 & pks0637 & 0.41753 & 14.2$\pm$0.0 & 45.33$\pm$4.60 & Danforth$^{M}$ \\ 
455 & pks0637 & 0.45294 & 13.7$\pm$0.1 & 36.10$\pm$11.60 & Danforth$^{M}$ \\ 
456 & pks0637 & 0.46848 & 13.9$\pm$0.1 & 55.10$\pm$11.30 & Danforth$^{M}$ \\ 
\hline
457 & pks1302 & 0.04225 & 14.4$\pm$0.1 & 54.00$\pm$3.00 & Tilton \\ 
458 & pks1302 & 0.06474 & 13.7$\pm$0.2 & 42.00$\pm$0.00 & Tilton \\ 
459 & pks1302 & 0.09486 & 13.9$\pm$0.2 & 61.60$\pm$17.80 & Tilton \\ 
460 & pks1302 & 0.09891 & 14.0$\pm$0.1 & 54.00$\pm$4.00 & Tilton \\ 
461 & pks1302 & 0.14518 & 13.8$\pm$0.1 & 31.67$\pm$6.33 & Danforth$^{M,*}$ \\ 
462 & pks1302 & 0.14552 & 13.4$\pm$0.1 & 23.10$\pm$8.80 & Danforth$^{1032*}$ \\ 
463 & pks1302 & 0.20438 & 13.6$\pm$0.1 & 38.00$\pm$3.80 & Tilton \\ 
464 & pks1302 & 0.22563 & 13.9$\pm$0.1 & 33.13$\pm$4.67 & Danforth$^{M,*}$ \\ 
465 & pks1302 & 0.22743 & 13.5$\pm$0.1 & 10.37$\pm$3.50 & Danforth$^{M,*}$ \\ 
466 & pks1302 & 0.25288 & 12.9$\pm$0.2 & 8.00$\pm$3.00 & Tilton \\ 
467 & pks1302 & 0.25299 & 13.4$\pm$0.3 & 30.90$\pm$10.80 & Danforth$^{1032}$ \\ 
\hline
468 & pks2005 & 0.06490 & 13.6$\pm$0.1 & 30.70$\pm$0.00 & Tilton \\ 
\hline
469 & pks2155 & 0.05405 & 13.6$\pm$0.1 & 14.00$\pm$6.00 & Tilton \\ 
470 & pks2155 & 0.05707 & 13.6$\pm$0.1 & 24.00$\pm$7.00 & Tilton \\ 
\hline
471 & pmn2345 & 0.19957 & 14.4$\pm$0.1 & 53.00$\pm$6.90 & Danforth$^{1038}$ \\ 
472 & pmn2345 & 0.37816 & 13.5$\pm$0.2 & 57.80$\pm$16.20 & Danforth$^{1032}$ \\ 
473 & pmn2345 & 0.39704 & 13.7$\pm$0.2 & 48.10$\pm$9.10 & Danforth$^{1032}$ \\ 
474 & pmn2345 & 0.42744 & 14.0$\pm$0.1 & 16.27$\pm$3.57 & Danforth$^{M}$ \\ 
475 & pmn2345 & 0.43053 & 13.8$\pm$0.1 & 23.73$\pm$6.77 & Danforth$^{M}$ \\ 
476 & pmn2345 & 0.43755 & 13.7$\pm$0.2 & 33.37$\pm$9.23 & Danforth$^{M}$ \\ 
477 & pmn2345 & 0.51360 & 14.0$\pm$0.1 & 22.90$\pm$5.37 & Danforth$^{M}$ \\ 
478 & pmn2345 & 0.53517 & 13.5$\pm$0.2 & 11.20$\pm$7.80 & Danforth$^{1032}$ \\ 
479 & pmn2345 & 0.59970 & 14.0$\pm$0.2 & 42.00$\pm$7.90 & Danforth$^{1032}$ \\ 
480 & pmn2345 & 0.61135 & 13.5$\pm$0.1 & 10.00$\pm$6.90 & Danforth$^{1032}$ \\ 
481 & pmn2345 & 0.61155 & 13.8$\pm$0.2 & 20.00$\pm$6.30 & Danforth$^{1038}$ \\ 
482 & pmn2345 & 0.61196 & 14.4$\pm$0.1 & 47.70$\pm$5.53 & Danforth$^{M}$ \\ 
\hline
483 & q0045 & 0.11052 & 13.8$\pm$0.2 & 45.47$\pm$9.40 & Danforth$^{M}$ \\ 
484 & q0045 & 0.13521 & 15.0$\pm$0.0 & 32.67$\pm$0.93 & Danforth$^{M}$ \\ 
\hline
485 & q1230 & 0.09518 & 14.5$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
486 & q1230 & 0.10318 & 13.4$\pm$0.2 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
487 & q1230 & 0.10445 & 13.4$\pm$0.1 & 15.30$\pm$5.50 & Danforth$^{1032}$ \\ 
488 & q1230 & 0.10530 & 15.1$\pm$0.0 & 89.83$\pm$2.30 & Danforth$^{M,*}$ \\ 
489 & q1230 & 0.10596 & 15.1$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{M,*}$ \\ 
490 & q1230 & 0.10666 & 15.0$\pm$0.0 & 76.87$\pm$2.30 & Danforth$^{M,*}$ \\ 
491 & q1230 & 0.10809 & 14.1$\pm$0.1 & 34.93$\pm$3.93 & Danforth$^{M}$ \\ 
492 & q1230 & 0.10820 & 14.6$\pm$0.1 & 78.10$\pm$10.90 & Danforth$^{1032}$ \\ 
493 & q1230 & 0.10861 & 14.6$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{M}$ \\ 
494 & q1230 & 0.10906 & 15.0$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
495 & q1230 & 0.10935 & 15.5$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1038}$ \\ 
496 & q1230 & 0.10956 & 15.1$\pm$0.0 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
497 & q1230 & 0.11707 & 15.2$\pm$0.0 & 48.67$\pm$1.20 & Danforth$^{M}$ \\ 
498 & q1230 & 0.11743 & 14.8$\pm$0.0 & 22.70$\pm$1.37 & Danforth$^{M}$ \\ 
499 & q1230 & 0.11781 & 15.0$\pm$0.0 & 41.10$\pm$0.93 & Danforth$^{M}$ \\ 
\hline
500 & rbs1892 & 0.15752 & 14.3$\pm$0.0 & 46.13$\pm$4.50 & Danforth$^{M}$ \\ 
501 & rbs1892 & 0.17133 & 13.7$\pm$0.1 & 41.00$\pm$10.20 & Danforth$^{1032}$ \\ 
502 & rbs1892 & 0.19874 & 13.7$\pm$0.1 & 9.07$\pm$2.80 & Danforth$^{M}$ \\ 
\hline
503 & rbs542 & 0.10323 & 15.5$\pm$0.0 & 62.60$\pm$0.87 & Danforth$^{M}$ \\ 
504 & rbs542 & 0.10379 & 14.7$\pm$0.0 & 29.17$\pm$0.57 & Danforth$^{M}$ \\ 
\hline
505 & rxj0439 & 0.11547 & 14.1$\pm$0.1 & 35.87$\pm$8.73 & Danforth$^{M}$ \\ 
506 & rxj0439 & 0.21833 & 13.5$\pm$0.1 & 11.80$\pm$5.70 & Danforth$^{1032}$ \\ 
507 & rxj0439 & 0.24235 & 14.3$\pm$0.1 & 26.13$\pm$6.03 & Danforth$^{M}$ \\ 
508 & rxj0439 & 0.24258 & 14.3$\pm$0.1 & 15.23$\pm$3.70 & Danforth$^{M}$ \\ 
509 & rxj0439 & 0.24313 & 14.7$\pm$0.0 & 43.03$\pm$3.53 & Danforth$^{M}$ \\ 
510 & rxj0439 & 0.24387 & 13.9$\pm$0.1 & 40.00$\pm$8.93 & Danforth$^{M}$ \\ 
\hline
511 & rxj2154 & 0.15689 & 13.8$\pm$0.1 & 33.53$\pm$6.00 & Danforth$^{M}$ \\ 
512 & rxj2154 & 0.15862 & 13.6$\pm$0.1 & 33.13$\pm$10.50 & Danforth$^{M}$ \\ 
513 & rxj2154 & 0.15889 & 13.7$\pm$0.1 & 9.23$\pm$3.93 & Danforth$^{M}$ \\ 
\hline
514 & s080908 & 0.12865 & 14.1$\pm$0.1 & 90.60$\pm$8.87 & Danforth$^{M}$ \\ 
515 & s080908 & 0.30757 & 14.5$\pm$0.0 & 32.77$\pm$2.60 & Danforth$^{M}$ \\ 
516 & s080908 & 0.32236 & 14.3$\pm$0.5 & 7.30$\pm$3.30 & Danforth$^{1032}$ \\ 
517 & s080908 & 0.37184 & 13.9$\pm$0.1 & 23.27$\pm$4.77 & Danforth$^{M}$ \\ 
518 & s080908 & 0.40733 & 13.7$\pm$0.1 & 17.87$\pm$9.63 & Danforth$^{M}$ \\ 
519 & s080908 & 0.40764 & 14.0$\pm$0.1 & 30.40$\pm$9.97 & Danforth$^{M}$ \\ 
520 & s080908 & 0.41759 & 14.1$\pm$0.1 & 49.23$\pm$7.50 & Danforth$^{M}$ \\ 
521 & s080908 & 0.51541 & 13.8$\pm$0.1 & 48.00$\pm$18.40 & Danforth$^{1032}$ \\ 
522 & s080908 & 0.60328 & 13.8$\pm$0.2 & 18.80$\pm$5.07 & Danforth$^{M}$ \\ 
523 & s080908 & 0.61912 & 14.9$\pm$0.0 & 43.30$\pm$3.30 & Danforth$^{1038}$ \\ 
524 & s080908 & 0.65652 & 16.5$\pm$0.3 & 28.83$\pm$3.17 & Danforth$^{M}$ \\ 
525 & s080908 & 0.65727 & 14.4$\pm$0.2 & 13.30$\pm$3.10 & Danforth$^{1032}$ \\ 
526 & s080908 & 0.65745 & 14.2$\pm$0.1 & 23.90$\pm$6.10 & Danforth$^{1038}$ \\ 
527 & s080908 & 0.65761 & 16.4$\pm$9.6 & 6.50$\pm$13.70 & Danforth$^{1038}$ \\ 
\hline
528 & s09255b & 0.29645 & 14.5$\pm$0.0 & 34.17$\pm$2.73 & Danforth$^{M}$ \\ 
529 & s09255b & 0.30927 & 13.7$\pm$0.2 & 29.53$\pm$11.47 & Danforth$^{M}$ \\ 
\hline
530 & s092909 & 0.14489 & 13.9$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
531 & s092909 & 0.16671 & 14.2$\pm$0.1 & 49.83$\pm$7.47 & Danforth$^{M}$ \\ 
\hline
532 & s094952 & 0.16442 & 13.6$\pm$0.1 & 26.60$\pm$12.20 & Danforth$^{1032}$ \\ 
533 & s094952 & 0.35167 & 14.0$\pm$0.1 & 40.20$\pm$8.47 & Danforth$^{M}$ \\ 
534 & s094952 & 0.36551 & 14.3$\pm$0.1 & 41.07$\pm$6.13 & Danforth$^{M}$ \\ 
535 & s094952 & 0.36580 & 14.0$\pm$0.1 & 43.60$\pm$11.40 & Danforth$^{M}$ \\ 
\hline
536 & s135712 & 0.09753 & 14.5$\pm$0.1 & 61.20$\pm$13.50 & Danforth$^{1038}$ \\ 
537 & s135712 & 0.14701 & 14.5$\pm$0.0 & 65.90$\pm$3.60 & Danforth$^{1032}$ \\ 
\hline
538 & s50716 & 0.23145 & 13.8$\pm$0.0 & 14.00$\pm$2.03 & Danforth$^{M}$ \\ 
\hline
539 & sbs1108 & 0.16559 & 14.2$\pm$0.0 & 23.20$\pm$1.40 & Danforth$^{1032}$ \\ 
540 & sbs1108 & 0.32014 & 13.7$\pm$0.1 & 12.60$\pm$4.30 & Danforth$^{1032}$ \\ 
541 & sbs1108 & 0.33424 & 13.7$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
542 & sbs1108 & 0.33522 & 13.9$\pm$0.1 & 49.00$\pm$9.47 & Danforth$^{M}$ \\ 
543 & sbs1108 & 0.34523 & 13.8$\pm$0.1 & 23.97$\pm$4.70 & Danforth$^{M}$ \\ 
544 & sbs1108 & 0.43579 & 13.8$\pm$0.1 & 17.00$\pm$4.63 & Danforth$^{M}$ \\ 
545 & sbs1108 & 0.46320 & 13.8$\pm$0.2 & 45.80$\pm$13.80 & Danforth$^{M}$ \\ 
546 & sbs1108 & 0.46846 & 13.8$\pm$0.1 & 22.93$\pm$6.17 & Danforth$^{M}$ \\ 
547 & sbs1108 & 0.48712 & 13.8$\pm$0.1 & 27.17$\pm$4.63 & Danforth$^{M}$ \\ 
548 & sbs1108 & 0.61764 & 13.7$\pm$0.1 & 22.80$\pm$8.20 & Danforth$^{1032}$ \\ 
\hline
549 & sbs1122 & 0.15545 & 14.1$\pm$0.1 & 44.30$\pm$7.17 & Danforth$^{M}$ \\ 
550 & sbs1122 & 0.19439 & 13.9$\pm$0.1 & 27.40$\pm$7.17 & Danforth$^{M}$ \\ 
551 & sbs1122 & 0.21209 & 14.0$\pm$0.1 & 29.80$\pm$8.00 & Danforth$^{1032}$ \\ 
552 & sbs1122 & 0.25712 & 14.5$\pm$0.0 & 29.10$\pm$2.70 & Danforth$^{1032}$ \\ 
553 & sbs1122 & 0.31236 & 14.4$\pm$0.0 & 32.87$\pm$4.33 & Danforth$^{M}$ \\ 
554 & sbs1122 & 0.31274 & 14.0$\pm$0.1 & 25.33$\pm$6.07 & Danforth$^{M}$ \\ 
555 & sbs1122 & 0.42009 & 13.9$\pm$0.1 & 28.70$\pm$4.70 & Danforth$^{1032}$ \\ 
556 & sbs1122 & 0.57049 & 13.9$\pm$0.1 & 24.40$\pm$6.50 & Danforth$^{M}$ \\ 
\hline
557 & ton236 & 0.19452 & 14.1$\pm$0.1 & 69.13$\pm$4.07 & Danforth$^{M}$ \\ 
558 & ton236 & 0.21887 & 13.9$\pm$0.1 & 67.30$\pm$12.70 & Danforth$^{1032}$ \\ 
559 & ton236 & 0.21919 & 13.8$\pm$0.3 & 38.90$\pm$14.20 & Danforth$^{1038}$ \\ 
560 & ton236 & 0.25876 & 13.7$\pm$0.1 & 5.00$\pm$0.00 & Danforth$^{1032}$ \\ 
561 & ton236 & 0.25896 & 13.6$\pm$0.1 & 7.30$\pm$5.50 & Danforth$^{1032}$ \\ 
562 & ton236 & 0.39942 & 13.8$\pm$0.1 & 100.00$\pm$0.00 & Danforth$^{1032}$ \\ 
563 & ton236 & 0.43738 & 14.3$\pm$0.0 & 33.13$\pm$2.40 & Danforth$^{M}$ \\ 
564 & ton236 & 0.44804 & 13.2$\pm$0.1 & 16.60$\pm$7.80 & Danforth$^{1032}$ \\ 
\hline
565 & ton28 & 0.13746 & 14.2$\pm$0.3 & 18.20$\pm$7.90 & Tilton \\ 
566 & ton28 & 0.13781 & 13.8$\pm$0.2 & 13.60$\pm$7.50 & Tilton \\ 
567 & ton28 & 0.17251 & 13.7$\pm$0.1 & 26.00$\pm$8.00 & Tilton \\ 
568 & ton28 & 0.24292 & 13.2$\pm$0.2 & 11.00$\pm$5.00 & Tilton \\ 
569 & ton28 & 0.24859 & 13.1$\pm$0.2 & 13.00$\pm$5.00 & Tilton \\ 
570 & ton28 & 0.27338 & 13.3$\pm$0.1 & 20.00$\pm$3.70 & Tilton \\ 
571 & ton28 & 0.33021 & 14.2$\pm$0.0 & 9.90$\pm$0.70 & Tilton \\ 
\hline
572 & ton580 & 0.20258 & 13.4$\pm$0.1 & 20.90$\pm$8.30 & Danforth$^{1032}$ \\ 
573 & ton580 & 0.29171 & 13.2$\pm$0.1 & 12.00$\pm$6.40 & Danforth$^{1032}$ \\ 
\hline
574 & tons180 & 0.02340 & 13.5$\pm$0.1 & 30.00$\pm$0.00 & Tilton \\ 
575 & tons180 & 0.04360 & 13.4$\pm$0.0 & 40.00$\pm$0.00 & Tilton \\ 
576 & tons180 & 0.04560 & 13.7$\pm$0.1 & 33.30$\pm$0.00 & Tilton \\ 
\hline
\end{longtable}


==> Tables/XMM/Latex/xmm_o7_hi_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllllll|l}
\caption[\xmm\ Data, \hi\ With \ovi\ Priors Results (Full)]{\ovii\ measurements with \xmm\ data, at the prior redshift from the \hi\ lines from Table~\ref{tab:hiPriorsTable}.}
\label{tab:xmmhiovii}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & \multicolumn{2}{c}{RGS1} & \multicolumn{2}{c}{RGS2} & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \% & avg exp (s) & \%  & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.13714$ (\#1)  & 92.78(90) & 143804 & 9 & 146370 & 7 & 1121$\pm^{ 32 }_{ 32 }$ & $1.00$ & 24.5622 & $ -0.33\pm^{ 0.82 }_{ 0.55 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.27\\ 
1es1028 & $0.20383$ (\#2)  & 114.22(94) & 146421 & 9 & 145107 & 9 & 1207$\pm^{ 32 }_{ 35 }$ & $1.00$ & 26.0027 & $ 0.03\pm^{ 0.97 }_{ 0.83 }$ & $ 14.01\pm^{ 1.43 }_{ nan }$ & -0.01\\ 
1es1028 & $0.22121$ (\#3)  & 101.58(92) & 144278 & 9 & 146704 & 9 & 1198$\pm^{ 35 }_{ 35 }$ & $1.00$ & 26.3781 & $ -0.70\pm^{ 0.67 }_{ 0.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.33\\ 
1es1553 & $0.03466$ (\#4)  & 38.25(27) & 1791095 & 9 & nan & nan & 747$\pm^{ 397 }_{ 326 }$ & $1.97$ & 22.3487 & $ -0.18\pm^{ 0.33 }_{ 0.25 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.53\\ 
1es1553 & $0.04273$ (\#5)  & 30.79(21) & 1784759 & 9 & nan & nan & 489$\pm^{ 628 }_{ 294 }$ & $2.72$ & 22.5230 & $ 0.51\pm^{ 0.64 }_{ 0.44 }$ & $ 15.21\pm^{ 0.28 }_{ 0.85 }$ & 2.85\\ 
1es1553 & $0.06364$ (\#6*)  & 64.48(28) & 1661330 & 9 & nan & nan & 27$\pm^{ 12 }_{ 9 }$ & $7.49$ & 22.9746 & $ 0.53\pm^{ 0.63 }_{ 0.44 }$ & $ 15.22\pm^{ 0.27 }_{ 0.73 }$ & 1.84\\ 
1es1553 & $0.21869$ (\#7)  & 108.81(87) & 1691684 & 7 & 1788288 & 8 & 1010$\pm^{ 415 }_{ 304 }$ & $1.74$ & 26.3237 & $ -0.01\pm^{ 0.65 }_{ 0.08 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.07\\ 
3c249 & $0.13470$ (\#8)  & 67.71(86) & 2642 & 7 & 2524 & 10 & 336$\pm^{ 146 }_{ 105 }$ & $1.00$ & 24.5095 & $ 9.67E+04\pm^{ 1.00E+20 }_{ 9.68E+04 }$ & $ 16.21\pm^{ 0.25 }_{ nan }$ & 0.52\\ 
3c249 & $0.26664$ (\#9)  & 79.78(93) & 2639 & 31 & 2524 & 59 & 306$\pm^{ 146 }_{ 111 }$ & $1.00$ & 27.3594 & $ 0.17\pm^{ 1.00E+20 }_{ 30.17 }$ & $ 14.78\pm^{ 1.68 }_{ nan }$ & -0.00\\ 
3c273 & $0.00758$ (\#10)  & -- & -- & -- & -- & -- & -- & -- & 21.7637 & -- & -- & --\\ 
3c273 & $0.06707$ (\#11*)  & 35.22(22) & 897879 & 5 & nan & nan & 4641$\pm^{ 37 }_{ 41 }$ & $1.00$ & 23.0487 & $ 0.24\pm^{ 0.31 }_{ 0.30 }$ & $ 14.91\pm^{ 0.32 }_{ nan }$ & 0.86\\ 
3c273 & $0.07359$ (\#12*)  & 45.49(29) & 930374 & 5 & nan & nan & 4656$\pm^{ 32 }_{ 34 }$ & $1.00$ & 23.1895 & $ -0.10\pm^{ 0.21 }_{ 0.19 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.39\\ 
3c273 & $0.13960$ (\#13)  & 68.74(61) & 892303 & 4 & 1027847 & 3 & 5246$\pm^{ 31 }_{ 31 }$ & $1.00$ & 24.6154 & $ -0.39\pm^{ 0.12 }_{ 0.11 }$ & $ nan\pm^{ nan }_{ nan }$ & 12.82\\ 
h1821 & $0.00944$ (\#14)  & -- & -- & -- & -- & -- & -- & -- & 21.8039 & -- & -- & --\\ 
h1821 & $0.06779$ (\#15)  & 48.43(43) & 28966 & 55 & nan & nan & 1081$\pm^{ 99 }_{ 91 }$ & $1.00$ & 23.0643 & $ 8.21E+04\pm^{ 1.00E+20 }_{ 5.68E+04 }$ & $ 16.18\pm^{ 0.28 }_{ 0.02 }$ & 1.16\\ 
h1821 & $0.08483$ (\#16)  & 62.62(44) & 31062 & 57 & nan & nan & 1008$\pm^{ 91 }_{ 87 }$ & $1.00$ & 23.4323 & $ 13.36\pm^{ 1.80E+08 }_{ 14.39 }$ & $ 15.89\pm^{ 0.40 }_{ nan }$ & 0.54\\ 
h1821 & $0.12147$ (\#17)  & 96.56(82) & 30593 & 48 & 43368 & 41 & 1284$\pm^{ 89 }_{ 85 }$ & $1.00$ & 24.2238 & $ 10.07\pm^{ 2.49E+04 }_{ 9.53 }$ & $ 15.88\pm^{ 0.29 }_{ 0.65 }$ & 1.85\\ 
h1821 & $0.19817$ (\#18)  & 79.32(81) & 32357 & 53 & 41356 & 43 & 1363$\pm^{ 112 }_{ 109 }$ & $1.00$ & 25.8805 & $ -1.36\pm^{ 1.36 }_{ 0.72 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.30\\ 
h1821 & $0.21321$ (\#19)  & 110.19(98) & 31737 & 48 & 41863 & 43 & 1644$\pm^{ 133 }_{ 107 }$ & $1.00$ & 26.2053 & $ 18.57\pm^{ 4.34E+07 }_{ 17.25 }$ & $ 15.96\pm^{ 0.34 }_{ 0.44 }$ & 2.38\\ 
h1821 & $0.24531$ (\#20)  & 119.80(98) & 31065 & 49 & 44448 & 47 & 1591$\pm^{ 120 }_{ 113 }$ & $1.00$ & 26.8987 & $ 0.44\pm^{ 17.76 }_{ 1.60 }$ & $ 15.15\pm^{ 0.78 }_{ nan }$ & 0.06\\ 
h2356 & $0.03830$ (\#21)  & 60.56(47) & 466679 & 7 & nan & nan & 1093$\pm^{ 15 }_{ 15 }$ & $1.00$ & 22.4273 & $ 0.02\pm^{ 0.48 }_{ 0.70 }$ & $ 13.78\pm^{ 1.43 }_{ nan }$ & -0.02\\ 
h2356 & $0.07881$ (\#22)  & 44.92(38) & 468683 & 8 & nan & nan & 1173$\pm^{ 21 }_{ 20 }$ & $1.00$ & 23.3023 & $ -0.79\pm^{ 0.59 }_{ 0.46 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.04\\ 
h2356 & $0.10467$ (\#23)  & 52.51(56) & 471489 & 8 & 510756 & 5 & 1280$\pm^{ 22 }_{ 21 }$ & $1.00$ & 23.8609 & $ 0.71\pm^{ 1.17 }_{ 0.68 }$ & $ 15.33\pm^{ 0.30 }_{ 1.43 }$ & 1.39\\ 
h2356 & $0.15613$ (\#24)  & 105.03(97) & 482157 & 6 & 504552 & 6 & 1323$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.9724 & $ 0.62\pm^{ 0.66 }_{ 0.49 }$ & $ 15.29\pm^{ 0.24 }_{ 0.62 }$ & 2.10\\ 
he0226 & $0.14274$ (\#25)  & 83.16(89) & 31710 & 21 & 31705 & 24 & 257$\pm^{ 34 }_{ 31 }$ & $1.00$ & 24.6832 & $ -1.95\pm^{ 2.49 }_{ 0.98 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.97\\ 
he0226 & $0.39890$ (\#26)  & 85.66(67) & 31717 & 39 & 31717 & 70 & 409$\pm^{ 80 }_{ 73 }$ & $1.00$ & 30.2162 & $ 0.54\pm^{ 7.93E+07 }_{ 30.54 }$ & $ 15.23\pm^{ 1.08 }_{ nan }$ & 0.01\\ 
he0226 & $0.41024$ (\#27)  & 81.69(56) & 31717 & 38 & 31717 & 67 & 421$\pm^{ 91 }_{ 82 }$ & $1.00$ & 30.4612 & $ 0.21\pm^{ 4.66E+08 }_{ 2.98 }$ & $ 14.87\pm^{ 1.42 }_{ nan }$ & 0.00\\ 
i22456 & $0.00443$ (\#28)  & -- & -- & -- & -- & -- & -- & -- & 21.6957 & -- & -- & --\\ 
i22456 & $0.09941$ (\#29)  & 74.98(61) & 79883 & 51 & 73453 & 44 & 671$\pm^{ 38 }_{ 37 }$ & $1.00$ & 23.7473 & $ 0.18\pm^{ 15.96 }_{ 1.63 }$ & $ 14.80\pm^{ 1.12 }_{ nan }$ & 0.00\\ 
mr2251 & $0.01068$ (\#30)  & -- & -- & -- & -- & -- & -- & -- & 21.8307 & -- & -- & --\\ 
mr2251 & $0.01449$ (\#31)  & 37.36(27) & 446548 & 6 & nan & nan & 2964$\pm^{ 3361 }_{ 1081 }$ & $0.01$ & 21.9130 & $ -0.65\pm^{ 0.43 }_{ 0.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.50\\ 
mr2251 & $0.06131$ (\#32)  & 32.34(25) & 452767 & 7 & nan & nan & 117$\pm^{ 170 }_{ 69 }$ & $5.55$ & 22.9243 & $ 2.49\pm^{ 13.28 }_{ 1.77 }$ & $ 15.71\pm^{ 0.19 }_{ 0.36 }$ & 4.17\\ 
mr2251 & $0.06190$ (\#33)  & 29.54(24) & 452283 & 7 & nan & nan & 59$\pm^{ 91 }_{ 37 }$ & $6.67$ & 22.9370 & $ 6.43\pm^{ 162.24 }_{ 4.90 }$ & $ 15.86\pm^{ 0.16 }_{ 0.29 }$ & 5.95\\ 
mr2251 & $0.06276$ (\#34)  & 30.33(22) & 451202 & 7 & nan & nan & 57$\pm^{ 104 }_{ 37 }$ & $6.71$ & 22.9556 & $ 3.48\pm^{ 9.04 }_{ 2.61 }$ & $ 15.76\pm^{ 0.17 }_{ 0.36 }$ & 4.37\\ 
mr2251 & $0.06327$ (\#35*)  & 31.04(20) & 449939 & 7 & nan & nan & 30$\pm^{ 81 }_{ 20 }$ & $7.77$ & 22.9666 & $ 1.82\pm^{ 4.06 }_{ 1.51 }$ & $ 15.62\pm^{ 0.23 }_{ 0.60 }$ & 2.99\\ 
mr2251 & $0.06381$ (\#36*)  & 33.43(22) & 451202 & 7 & nan & nan & 148$\pm^{ 162 }_{ 116 }$ & $5.14$ & 22.9783 & $ 0.01\pm^{ 0.93 }_{ 0.65 }$ & $ 13.43\pm^{ 2.00 }_{ nan }$ & -0.00\\ 
mrk478 & $0.06166$ (\#37)  & 61.33(42) & 192118 & 15 & nan & nan & 253$\pm^{ 786 }_{ 195 }$ & $2.48$ & 22.9319 & $ -0.49\pm^{ 5.63 }_{ 1.27 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.07\\ 
mrk478 & $0.06578$ (\#38)  & 54.57(42) & 192119 & 15 & nan & nan & 606$\pm^{ 1058 }_{ 523 }$ & $1.09$ & 23.0208 & $ 44.37\pm^{ 1.45E+06 }_{ 45.85 }$ & $ 15.99\pm^{ 0.22 }_{ nan }$ & 3.82\\ 
mrk478 & $0.07213$ (\#39)  & 54.93(42) & 192121 & 15 & nan & nan & 640$\pm^{ 1985 }_{ 489 }$ & $1.00$ & 23.1580 & $ 0.48\pm^{ 4.43 }_{ 1.30 }$ & $ 15.19\pm^{ 0.63 }_{ nan }$ & 0.10\\ 
mrk876 & $0.01159$ (\#40)  & -- & -- & -- & -- & -- & -- & -- & 21.8503 & -- & -- & --\\ 
mrk876 & $0.05598$ (\#41)  & 44.97(46) & 2714 & 12 & nan & nan & 477$\pm^{ 142 }_{ 112 }$ & $1.00$ & 22.8092 & $ 9.00E+03\pm^{ 1.00E+20 }_{ 9.03E+03 }$ & $ 16.20\pm^{ 0.26 }_{ nan }$ & 0.21\\ 
mrk876 & $0.08709$ (\#42)  & 37.14(46) & 2802 & 11 & nan & nan & 345$\pm^{ 146 }_{ 103 }$ & $1.00$ & 23.4811 & $ 2.64E+09\pm^{ 1.00E+20 }_{ 2.64E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 1.36\\ 
mrk876 & $0.08858$ (\#43)  & 37.69(46) & 2802 & 10 & nan & nan & 378$\pm^{ 139 }_{ 105 }$ & $1.00$ & 23.5133 & $ 3.17E+12\pm^{ 1.00E+20 }_{ 3.17E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 1.70\\ 
mrk876 & $0.08917$ (\#44)  & 37.84(47) & 2802 & 10 & 996 & nan & 377$\pm^{ 134 }_{ 98 }$ & $1.00$ & 23.5261 & $ 1.28E+13\pm^{ 1.00E+20 }_{ 1.28E+13 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 1.65\\ 
mrk876 & $0.11487$ (\#45)  & 73.35(75) & 2743 & 19 & 2633 & 28 & 529$\pm^{ 144 }_{ 121 }$ & $1.00$ & 24.0812 & $ 0.22\pm^{ 1.00E+20 }_{ 30.22 }$ & $ 14.87\pm^{ 1.59 }_{ nan }$ & 0.00\\ 
ngc7469 & $0.00981$ (\#46)  & -- & -- & -- & -- & -- & -- & -- & 21.8119 & -- & -- & --\\ 
pg0003 & $0.08299$ (\#47)  & 59.05(43) & 13037 & 19 & nan & nan & 234$\pm^{ 52 }_{ 46 }$ & $1.00$ & 23.3926 & $ -3.31\pm^{ 3.02E+06 }_{ 1.67 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.47\\ 
pg0003 & $0.17139$ (\#48)  & 111.61(94) & 13033 & 24 & 12941 & 16 & 332$\pm^{ 65 }_{ 54 }$ & $1.00$ & 25.3020 & $ 14.29\pm^{ 1.08E+15 }_{ 44.29 }$ & $ 15.93\pm^{ 0.50 }_{ nan }$ & 0.31\\ 
pg0003 & $0.22541$ (\#49)  & 114.13(94) & 13034 & 39 & 12838 & 28 & 231$\pm^{ 58 }_{ 50 }$ & $1.00$ & 26.4689 & $ 0.46\pm^{ 3.20E+09 }_{ 30.46 }$ & $ 15.17\pm^{ 1.17 }_{ nan }$ & 0.00\\ 
pg0003 & $0.38633$ (\#50)  & 104.20(85) & 13041 & 125 & 12919 & 49 & 115$\pm^{ 65 }_{ 47 }$ & $1.00$ & 29.9447 & $ -5.97\pm^{ 1.21 }_{ 1.08 }$ & $ nan\pm^{ nan }_{ nan }$ & 12.63\\ 
pg0003 & $0.42051$ (\#51)  & 114.71(91) & 13041 & 92 & 12843 & 45 & 362$\pm^{ 115 }_{ 95 }$ & $1.00$ & 30.6830 & $ -1.35\pm^{ 9.66E+09 }_{ 2.59 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.06\\ 
pg0804 & $0.05015$ (\#52)  & 46.31(37) & 27851 & 8 & nan & nan & 1439$\pm^{ 93 }_{ 87 }$ & $1.00$ & 22.6832 & $ 3.75E+05\pm^{ 1.00E+20 }_{ 3.75E+05 }$ & $ 16.25\pm^{ 0.16 }_{ nan }$ & 7.42\\ 
pg0804 & $0.05576$ (\#53)  & 53.92(41) & 28550 & 8 & nan & nan & 1333$\pm^{ 83 }_{ 80 }$ & $1.00$ & 22.8044 & $ 2.94\pm^{ 6.29E+04 }_{ 32.94 }$ & $ 15.74\pm^{ 0.45 }_{ nan }$ & 0.29\\ 
pg0804 & $0.36379$ (\#54)  & 127.43(96) & 29665 & 20 & 30901 & 12 & 2024$\pm^{ 141 }_{ 134 }$ & $1.00$ & 29.4579 & $ -0.91\pm^{ 1.96 }_{ 0.95 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.42\\ 
pg0832 & $0.01753$ (\#55)  & -- & -- & -- & -- & -- & -- & -- & 21.9786 & -- & -- & --\\ 
pg0832 & $0.02793$ (\#56)  & 52.15(36) & 20654 & 133 & nan & nan & 26$\pm^{ 18 }_{ 14 }$ & $1.00$ & 22.2033 & $ -6.69\pm^{ 1.61 }_{ 1.73 }$ & $ nan\pm^{ nan }_{ nan }$ & 9.82\\ 
pg0832 & $0.08748$ (\#57)  & 53.03(45) & 20655 & 77 & nan & nan & 71$\pm^{ 25 }_{ 19 }$ & $1.00$ & 23.4896 & $ 1.15E+13\pm^{ 1.00E+20 }_{ 1.15E+13 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 1.13\\ 
pg0832 & $0.10171$ (\#58)  & 73.57(56) & 20655 & 68 & 20637 & 75 & 84$\pm^{ 30 }_{ 22 }$ & $1.00$ & 23.7969 & $ 3.93E+04\pm^{ 1.00E+20 }_{ 3.94E+04 }$ & $ 16.21\pm^{ 0.25 }_{ nan }$ & 0.91\\ 
pg0832 & $0.18391$ (\#59)  & 60.33(41) & 20654 & 143 & 20637 & 67 & 70$\pm^{ 54 }_{ 32 }$ & $1.00$ & 25.5725 & $ 1.66E+06\pm^{ 1.00E+20 }_{ 1.66E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 1.25\\ 
pg0832 & $0.27503$ (\#60)  & 124.41(86) & 20656 & 150 & 20637 & 94 & 58$\pm^{ 29 }_{ 21 }$ & $1.00$ & 27.5406 & $ -0.97\pm^{ 1.00E+20 }_{ 29.03 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pg0832 & $0.27694$ (\#61)  & 119.21(86) & 20656 & 135 & 20637 & 95 & 60$\pm^{ 28 }_{ 22 }$ & $1.00$ & 27.5819 & $ 2.50\pm^{ 1.00E+20 }_{ 32.50 }$ & $ 15.70\pm^{ 0.76 }_{ nan }$ & 0.02\\ 
pg0832 & $0.32572$ (\#62*)  & 136.80(85) & 20656 & 238 & 20645 & 93 & 51$\pm^{ 28 }_{ 20 }$ & $1.00$ & 28.6356 & $ -2.54\pm^{ 1.08E+05 }_{ 2.21 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.31\\ 
pg0838 & $0.06583$ (\#63)  & 1.34(41) & 1609 & inf & nan & nan & 0$\pm^{ 36 }_{ -0 }$ & $1.00$ & 23.0219 & $ 2.00\pm^{ 1.00E+20 }_{ 32.00 }$ & $ 15.64\pm^{ 0.82 }_{ nan }$ & 0.00\\ 
pg0838 & $0.08628$ (\#64)  & 16.24(44) & 1609 & 90 & nan & nan & 130$\pm^{ 124 }_{ 72 }$ & $1.00$ & 23.4636 & $ 1.51E+04\pm^{ 1.00E+20 }_{ 1.51E+04 }$ & $ 16.21\pm^{ 0.26 }_{ nan }$ & 0.17\\ 
pg0838 & $0.12676$ (\#65)  & 32.38(79) & 1609 & 198 & 1519 & 38 & 75$\pm^{ 109 }_{ 75 }$ & $1.00$ & 24.3380 & $ 8.43E+12\pm^{ 1.00E+20 }_{ 8.43E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 0.75\\ 
pg0953 & $0.16319$ (\#66)  & 129.94(91) & 12778 & 16 & 12309 & 8 & 593$\pm^{ 77 }_{ 71 }$ & $1.00$ & 25.1249 & $ 1.31\pm^{ 5.35E+03 }_{ 2.85 }$ & $ 15.53\pm^{ 0.67 }_{ nan }$ & 0.09\\ 
pg0953 & $0.19221$ (\#67)  & 122.56(92) & 12777 & 11 & 12309 & 10 & 612$\pm^{ 78 }_{ 71 }$ & $1.00$ & 25.7517 & $ -0.51\pm^{ 475.06 }_{ 1.65 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
pg1048 & $0.00642$ (\#68)  & -- & -- & -- & -- & -- & -- & -- & 21.7387 & -- & -- & --\\ 
pg1048 & $0.02414$ (\#69)  & 32.85(32) & 18864 & 38 & nan & nan & 156$\pm^{ 38 }_{ 33 }$ & $1.00$ & 22.1214 & $ 61.26\pm^{ 1.00E+20 }_{ 91.26 }$ & $ 16.02\pm^{ 0.38 }_{ nan }$ & 0.12\\ 
pg1115 & $0.09511$ (\#70)  & 47.02(50) & 17510 & 31 & 16953 & 21 & 325$\pm^{ 54 }_{ 46 }$ & $1.00$ & 23.6544 & $ 7.12\pm^{ 1.00E+20 }_{ 37.12 }$ & $ 15.85\pm^{ 0.56 }_{ nan }$ & 0.20\\ 
pg1115 & $0.12059$ (\#71)  & 98.56(73) & 17510 & 33 & 16953 & 13 & 310$\pm^{ 48 }_{ 44 }$ & $1.00$ & 24.2047 & $ 1.36E+03\pm^{ 1.00E+20 }_{ 1.39E+03 }$ & $ 16.12\pm^{ 0.34 }_{ nan }$ & 2.50\\ 
pg1115 & $0.12741$ (\#72)  & 107.59(76) & 17513 & 30 & 16953 & 11 & 311$\pm^{ 51 }_{ 47 }$ & $1.00$ & 24.3521 & $ 0.00\pm^{ 8.23E+03 }_{ 1.93 }$ & $ 13.12\pm^{ 3.04 }_{ nan }$ & 0.00\\ 
pg1116 & $0.04114$ (\#73)  & 41.06(39) & 284047 & 15 & nan & nan & 540$\pm^{ 17 }_{ 17 }$ & $1.00$ & 22.4886 & $ -0.84\pm^{ 0.90 }_{ 0.61 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.16\\ 
pg1116 & $0.06251$ (\#74)  & 40.85(30) & 283934 & 17 & nan & nan & 549$\pm^{ 22 }_{ 21 }$ & $1.00$ & 22.9502 & $ 1.33\pm^{ 140.93 }_{ 2.32 }$ & $ 15.54\pm^{ 0.51 }_{ nan }$ & 0.23\\ 
pg1116 & $0.08382$ (\#75)  & 46.62(32) & 284638 & 17 & nan & nan & 588$\pm^{ 22 }_{ 18 }$ & $1.00$ & 23.4105 & $ 2.02E+07\pm^{ 1.00E+20 }_{ 1.99E+07 }$ & $ 16.29\pm^{ 0.17 }_{ 0.08 }$ & 8.15\\ 
pg1116 & $0.09210$ (\#76)  & 51.16(38) & 292136 & 17 & 222826 & 11 & 576$\pm^{ 20 }_{ 19 }$ & $1.00$ & 23.5894 & $ 0.28\pm^{ 2.14 }_{ 1.00 }$ & $ 14.98\pm^{ 0.72 }_{ nan }$ & 0.07\\ 
pg1116 & $0.09281$ (\#77)  & 50.89(38) & 292136 & 17 & 222826 & 10 & 579$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.6047 & $ 0.59\pm^{ 2.86 }_{ 1.14 }$ & $ 15.26\pm^{ 0.50 }_{ nan }$ & 0.25\\ 
pg1116 & $0.13373$ (\#78)  & 89.85(89) & 277711 & 16 & 284726 & 12 & 680$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.4886 & $ 3.28\pm^{ 6.08 }_{ 2.17 }$ & $ 15.75\pm^{ 0.16 }_{ 0.28 }$ & 5.37\\ 
pg1116 & $0.13851$ (\#79)  & 94.60(91) & 277702 & 15 & 291047 & 12 & 693$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.5918 & $ 1.55\pm^{ 2.89 }_{ 1.21 }$ & $ 15.58\pm^{ 0.23 }_{ 0.53 }$ & 2.45\\ 
pg1211 & $0.02586$ (\#80)  & 33.66(32) & 769591 & 13 & nan & nan & 575$\pm^{ 12 }_{ 12 }$ & $1.00$ & 22.1586 & $ -0.39\pm^{ 1.04 }_{ 0.68 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.25\\ 
pg1211 & $0.05443$ (\#81)  & 49.81(35) & 745965 & 14 & nan & nan & 634$\pm^{ 12 }_{ 12 }$ & $1.00$ & 22.7757 & $ 0.25\pm^{ 1.61 }_{ 0.89 }$ & $ 14.94\pm^{ 0.70 }_{ nan }$ & 0.06\\ 
pg1216 & $0.00842$ (\#82)  & -- & -- & -- & -- & -- & -- & -- & 21.7819 & -- & -- & --\\ 
pg1216 & $0.07969$ (\#83)  & 53.17(43) & 11245 & 40 & nan & nan & 185$\pm^{ 50 }_{ 39 }$ & $1.00$ & 23.3213 & $ 583.85\pm^{ 1.00E+20 }_{ 613.85 }$ & $ 16.11\pm^{ 0.30 }_{ nan }$ & 0.44\\ 
pg1216 & $0.12372$ (\#84)  & 107.60(78) & 11245 & 36 & 11258 & 15 & 182$\pm^{ 51 }_{ 48 }$ & $1.00$ & 24.2724 & $ 4.72E+06\pm^{ 1.00E+20 }_{ 4.72E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 3.27\\ 
pg1216 & $0.12473$ (\#85)  & 107.90(78) & 11245 & 36 & 11258 & 15 & 186$\pm^{ 59 }_{ 40 }$ & $1.00$ & 24.2942 & $ 1.11E+04\pm^{ 1.00E+20 }_{ 1.12E+04 }$ & $ 16.21\pm^{ 0.26 }_{ nan }$ & 1.76\\ 
pg1216 & $0.17950$ (\#86)  & 106.70(95) & 11257 & 23 & 11258 & 31 & 243$\pm^{ 51 }_{ 45 }$ & $1.00$ & 25.4772 & $ 3.13E+09\pm^{ 1.00E+20 }_{ 3.13E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 2.17\\ 
pg1216 & $0.20014$ (\#87)  & 86.38(92) & 11257 & 29 & 11258 & 46 & 179$\pm^{ 53 }_{ 39 }$ & $1.00$ & 25.9230 & $ 9.58E+05\pm^{ 1.00E+20 }_{ 9.58E+05 }$ & $ 16.28\pm^{ 0.13 }_{ nan }$ & 1.23\\ 
pg1216 & $0.21258$ (\#88)  & 84.99(93) & 11257 & 19 & 11258 & 27 & 191$\pm^{ 48 }_{ 41 }$ & $1.00$ & 26.1917 & $ 679.96\pm^{ 1.00E+20 }_{ 709.96 }$ & $ 16.11\pm^{ 0.35 }_{ nan }$ & 0.49\\ 
pg1216 & $0.28204$ (\#89)  & 112.71(89) & 11258 & 41 & 11258 & 68 & 237$\pm^{ 66 }_{ 56 }$ & $1.00$ & 27.6921 & $ -2.70\pm^{ 5.32 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.83\\ 
pg1229 & $0.05018$ (\#90)  & 55.71(43) & 24016 & 20 & nan & nan & 521$\pm^{ 63 }_{ 49 }$ & $1.00$ & 22.6839 & $ 2.38E+06\pm^{ 1.00E+20 }_{ 2.38E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 3.04\\ 
pg1259 & $0.05563$ (\#91)  & 50.01(43) & 11485 & 47 & nan & nan & 165$\pm^{ 50 }_{ 38 }$ & $1.00$ & 22.8016 & $ 3.07E+09\pm^{ 1.00E+20 }_{ 3.07E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 0.63\\ 
pg1259 & $0.15136$ (\#92)  & 99.16(90) & 11483 & 47 & 11479 & 39 & 130$\pm^{ 43 }_{ 35 }$ & $1.00$ & 24.8694 & $ 6.07\pm^{ 6.78E+16 }_{ 36.07 }$ & $ 15.84\pm^{ 0.62 }_{ nan }$ & 0.08\\ 
pg1259 & $0.16647$ (\#93)  & 105.90(92) & 11483 & 34 & 11479 & 49 & 145$\pm^{ 43 }_{ 36 }$ & $1.00$ & 25.1958 & $ -2.40\pm^{ 9.65 }_{ 1.49 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.61\\ 
pg1259 & $0.17893$ (\#94)  & 108.49(96) & 11483 & 38 & 11479 & 42 & 180$\pm^{ 52 }_{ 40 }$ & $1.00$ & 25.4649 & $ 3.20E+04\pm^{ 1.00E+20 }_{ 3.20E+04 }$ & $ 16.21\pm^{ 0.25 }_{ nan }$ & 0.92\\ 
pg1259 & $0.22376$ (\#95)  & 105.77(93) & 11483 & 32 & 11479 & 49 & 277$\pm^{ 65 }_{ 56 }$ & $1.00$ & 26.4332 & $ 0.49\pm^{ 5.50E+12 }_{ 30.49 }$ & $ 15.20\pm^{ 1.20 }_{ nan }$ & 0.01\\ 
pg1259 & $0.24126$ (\#96)  & 121.27(95) & 11483 & 71 & 11479 & 62 & 149$\pm^{ 49 }_{ 40 }$ & $1.00$ & 26.8112 & $ -2.43\pm^{ 2.39E+03 }_{ 1.39 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.44\\ 
pg1259 & $0.31974$ (\#97)  & 80.23(82) & 11483 & 42 & 11480 & 55 & 293$\pm^{ 92 }_{ 69 }$ & $1.00$ & 28.5064 & $ 819.38\pm^{ 1.00E+20 }_{ 849.38 }$ & $ 16.11\pm^{ 0.30 }_{ nan }$ & 0.53\\ 
pg1259 & $0.36212$ (\#98)  & 114.78(79) & 11487 & 85 & 11480 & 57 & 291$\pm^{ 96 }_{ 78 }$ & $1.00$ & 29.4218 & $ 5.74E+09\pm^{ 1.00E+20 }_{ 5.74E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 1.38\\ 
pg1259 & $0.38254$ (\#99)  & 134.54(94) & 11487 & 66 & 11480 & 43 & 351$\pm^{ 94 }_{ 79 }$ & $1.00$ & 29.8629 & $ -1.02\pm^{ 2.79E+05 }_{ 2.46 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
pg1259 & $0.38266$ (\#100)  & 134.54(94) & 11487 & 66 & 11480 & 43 & 351$\pm^{ 93 }_{ 79 }$ & $1.00$ & 29.8655 & $ -0.93\pm^{ 5.36E+06 }_{ 2.11 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
pg1307 & $0.08345$ (\#101)  & 53.56(43) & 9827 & 33 & nan & nan & 196$\pm^{ 53 }_{ 46 }$ & $1.00$ & 23.4025 & $ -4.57\pm^{ 1.90 }_{ 1.20 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.97\\ 
pg1309 & $0.03861$ (\#102)  & 52.72(41) & 27263 & 80 & nan & nan & 74$\pm^{ 24 }_{ 17 }$ & $1.00$ & 22.4340 & $ 5.94E+06\pm^{ 1.00E+20 }_{ 5.94E+06 }$ & $ 16.28\pm^{ 0.18 }_{ nan }$ & 0.98\\ 
pg1309 & $0.17740$ (\#103)  & 116.75(95) & 27265 & 32 & 26163 & 73 & 153$\pm^{ 33 }_{ 25 }$ & $1.00$ & 25.4318 & $ 7.33E+12\pm^{ 1.00E+20 }_{ 7.33E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 2.31\\ 
pg1309 & $0.17852$ (\#104)  & 121.37(94) & 27265 & 33 & 26163 & 75 & 155$\pm^{ 35 }_{ 26 }$ & $1.00$ & 25.4560 & $ 9.71E+08\pm^{ 1.00E+20 }_{ 9.71E+08 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 2.13\\ 
pg1309 & $0.17918$ (\#105)  & 120.71(95) & 27265 & 33 & 26163 & 75 & 154$\pm^{ 28 }_{ 26 }$ & $1.00$ & 25.4703 & $ 2.60E+06\pm^{ 1.00E+20 }_{ 2.60E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 1.80\\ 
pg1309 & $0.18143$ (\#106)  & 116.88(93) & 27265 & 33 & 26163 & 75 & 141$\pm^{ 28 }_{ 25 }$ & $1.00$ & 25.5189 & $ 7.45\pm^{ 1.00E+20 }_{ 37.45 }$ & $ 15.86\pm^{ 0.60 }_{ nan }$ & 0.09\\ 
pg1444 & $0.22031$ (\#107)  & 113.67(93) & 17674 & 27 & 17137 & 35 & 183$\pm^{ 40 }_{ 35 }$ & $1.00$ & 26.3587 & $ -2.51\pm^{ 2.34 }_{ 1.07 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.34\\ 
pg1626 & $0.06137$ (\#108)  & -- & -- & -- & -- & -- & -- & -- & 22.9256 & -- & -- & --\\ 
phl1811 & $0.05143$ (\#109)  & -- & -- & -- & -- & -- & -- & -- & 22.7109 & -- & -- & --\\ 
phl1811 & $0.05813$ (\#110)  & -- & -- & -- & -- & -- & -- & -- & 22.8556 & -- & -- & --\\ 
phl1811 & $0.08085$ (\#111)  & -- & -- & -- & -- & -- & -- & -- & 23.3464 & -- & -- & --\\ 
phl1811 & $0.08163$ (\#112)  & -- & -- & -- & -- & -- & -- & -- & 23.3632 & -- & -- & --\\ 
phl1811 & $0.12003$ (\#113)  & 77.84(58) & 74729 & 91 & 79201 & 70 & 33$\pm^{ 15 }_{ 14 }$ & $1.00$ & 24.1926 & $ 6.97E+07\pm^{ 1.00E+20 }_{ 6.97E+07 }$ & $ 16.33\pm^{ 0.13 }_{ -0.13 }$ & 1.01\\ 
phl1811 & $0.15787$ (\#114)  & -- & -- & -- & -- & -- & -- & -- & 25.0100 & -- & -- & --\\ 
pks0312 & $0.11454$ (\#115)  & 64.38(70) & 23887 & 39 & 22982 & 29 & 266$\pm^{ 37 }_{ 35 }$ & $1.00$ & 24.0741 & $ 4.42E+04\pm^{ 1.00E+20 }_{ 4.42E+04 }$ & $ 16.21\pm^{ 0.25 }_{ nan }$ & 2.67\\ 
pks0405 & $0.02510$ (\#116)  & 41.67(34) & 137701 & 23 & nan & nan & 304$\pm^{ 19 }_{ 17 }$ & $1.00$ & 22.1422 & $ -0.00\pm^{ 67.52 }_{ 1.38 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.00\\ 
pks0405 & $0.05902$ (\#117)  & 53.75(40) & 134613 & 23 & nan & nan & 316$\pm^{ 20 }_{ 19 }$ & $1.00$ & 22.8748 & $ -1.86\pm^{ 1.00 }_{ 0.63 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.69\\ 
pks0405 & $0.09719$ (\#118)  & 64.86(45) & 135771 & 21 & nan & nan & 354$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.6993 & $ -1.55\pm^{ 1.30 }_{ 0.83 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.60\\ 
pks0405 & $0.10152$ (\#119)  & 65.13(49) & 134959 & 21 & 138649 & 18 & 355$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.7928 & $ -2.00\pm^{ 0.89 }_{ 0.64 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.98\\ 
pks0405 & $0.10298$ (\#120)  & 68.35(50) & 134879 & 21 & 138649 & 16 & 368$\pm^{ 20 }_{ 20 }$ & $1.00$ & 23.8244 & $ -1.08\pm^{ 1.74 }_{ 0.83 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.70\\ 
pks0405 & $0.19456$ (\#121)  & 116.94(93) & 137986 & 20 & 134948 & 21 & 405$\pm^{ 21 }_{ 21 }$ & $1.00$ & 25.8025 & $ 18.91\pm^{ 3.63E+04 }_{ 18.08 }$ & $ 15.92\pm^{ 0.25 }_{ 0.52 }$ & 1.98\\ 
pks0405 & $0.21976$ (\#122)  & 126.59(92) & 137232 & 19 & 135759 & 24 & 408$\pm^{ 22 }_{ 22 }$ & $1.00$ & 26.3468 & $ -1.02\pm^{ 1.30 }_{ 0.80 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.87\\ 
pks0405 & $0.24564$ (\#123)  & 98.79(93) & 136439 & 23 & 138647 & 30 & 383$\pm^{ 23 }_{ 23 }$ & $1.00$ & 26.9058 & $ -1.04\pm^{ 1.25 }_{ 0.70 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.95\\ 
pks0405 & $0.29748$ (\#124)  & 98.21(89) & 135766 & 33 & 137130 & 34 & 382$\pm^{ 27 }_{ 25 }$ & $1.00$ & 28.0256 & $ -0.20\pm^{ 3.89 }_{ 1.16 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pks0405 & $0.31016$ (\#125)  & 96.82(90) & 137275 & 34 & 137114 & 39 & 378$\pm^{ 26 }_{ 25 }$ & $1.00$ & 28.2995 & $ -2.30\pm^{ 0.65 }_{ 0.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.68\\ 
pks0405 & $0.32502$ (\#126)  & 92.49(84) & 135467 & 36 & 137166 & 41 & 414$\pm^{ 31 }_{ 30 }$ & $1.00$ & 28.6204 & $ 3.81\pm^{ 1.66E+03 }_{ 4.17 }$ & $ 15.78\pm^{ 0.36 }_{ nan }$ & 0.79\\ 
pks0405 & $0.49508$ (\#127)  & 112.25(94) & 138729 & 51 & 137202 & 58 & 536$\pm^{ 45 }_{ 43 }$ & $1.00$ & 32.2937 & $ -2.11\pm^{ 0.90 }_{ 0.58 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.47\\ 
pks0558 & $0.10472$ (\#128)  & 82.71(58) & 705422 & 22 & 787021 & 25 & 2580$\pm^{ 30 }_{ 21 }$ & $1.00$ & 23.8620 & $ 0.07\pm^{ 0.62 }_{ 0.22 }$ & $ 14.41\pm^{ 0.91 }_{ nan }$ & 0.22\\ 
pks2155 & $0.05708$ (\#129)  & 42.12(39) & 1687774 & 3 & nan & nan & 641$\pm^{ 88 }_{ 82 }$ & $4.94$ & 22.8329 & $ -0.29\pm^{ 0.12 }_{ 0.11 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.22\\ 
pks2155 & $0.06236$ (\#130)  & -- & -- & -- & -- & -- & -- & -- & 22.9470 & -- & -- & --\\ 
pks2155 & $0.10586$ (\#131)  & 60.97(48) & 1694875 & 3 & 1691927 & 3 & 1743$\pm^{ 77 }_{ 762 }$ & $3.33$ & 23.8866 & $ -0.02\pm^{ 0.35 }_{ 0.10 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.23\\ 
q0045 & $0.05590$ (\#132)  & 48.77(38) & 13827 & 153 & nan & nan & 59$\pm^{ 32 }_{ 22 }$ & $1.00$ & 22.8074 & $ 81.83\pm^{ 1.00E+20 }_{ 111.83 }$ & $ 16.01\pm^{ 0.45 }_{ nan }$ & 0.14\\ 
q0045 & $0.06377$ (\#133)  & -- & -- & -- & -- & -- & -- & -- & 22.9774 & -- & -- & --\\ 
q1230 & $0.08344$ (\#134)  & 49.74(34) & 39335 & 66 & nan & nan & 83$\pm^{ 24 }_{ 21 }$ & $1.00$ & 23.4023 & $ -3.52\pm^{ 5.75 }_{ 1.49 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.96\\ 
q1230 & $0.08540$ (\#135)  & 49.18(36) & 39335 & 61 & nan & nan & 99$\pm^{ 24 }_{ 23 }$ & $1.00$ & 23.4446 & $ 33.06\pm^{ 1.00E+20 }_{ 63.06 }$ & $ 15.99\pm^{ 0.47 }_{ nan }$ & 0.11\\ 
q1230 & $0.09444$ (\#136)  & 57.34(47) & 39335 & 61 & 39139 & 97 & 98$\pm^{ 26 }_{ 19 }$ & $1.00$ & 23.6399 & $ 4.50E+04\pm^{ 1.00E+20 }_{ 4.50E+04 }$ & $ 16.21\pm^{ 0.26 }_{ nan }$ & 1.01\\ 
q1230 & $0.10000$ (\#137)  & 69.52(51) & 39335 & 69 & 39139 & 87 & 67$\pm^{ 22 }_{ 19 }$ & $1.00$ & 23.7600 & $ -4.12\pm^{ 1.28 }_{ 0.90 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.46\\ 
q1230 & $0.10525$ (\#138)  & 71.15(53) & 39335 & 67 & 39139 & 75 & 95$\pm^{ 23 }_{ 20 }$ & $1.00$ & 23.8734 & $ 214.72\pm^{ 1.00E+20 }_{ 244.72 }$ & $ 16.09\pm^{ 0.32 }_{ nan }$ & 0.19\\ 
q1230 & $0.10549$ (\#139)  & 74.01(55) & 39335 & 67 & 39139 & 80 & 93$\pm^{ 22 }_{ 20 }$ & $1.00$ & 23.8786 & $ 1.38E+03\pm^{ 1.00E+20 }_{ 1.41E+03 }$ & $ 16.12\pm^{ 0.34 }_{ nan }$ & 0.15\\ 
q1230 & $0.10566$ (\#140)  & 74.03(55) & 39335 & 67 & 39139 & 80 & 93$\pm^{ 23 }_{ 20 }$ & $1.00$ & 23.8823 & $ 74.47\pm^{ 1.00E+20 }_{ 104.47 }$ & $ 16.02\pm^{ 0.44 }_{ nan }$ & 0.12\\ 
q1230 & $0.10612$ (\#141)  & 75.39(55) & 39335 & 67 & 39139 & 80 & 90$\pm^{ 22 }_{ 20 }$ & $1.00$ & 23.8922 & $ 4.67\pm^{ 1.00E+20 }_{ 34.67 }$ & $ 15.79\pm^{ 0.62 }_{ nan }$ & 0.03\\ 
q1230 & $0.10639$ (\#142)  & 76.90(57) & 39335 & 68 & 39139 & 75 & 89$\pm^{ 23 }_{ 20 }$ & $1.00$ & 23.8980 & $ 1.30\pm^{ 1.00E+20 }_{ 31.30 }$ & $ 15.52\pm^{ 0.94 }_{ nan }$ & 0.01\\ 
q1230 & $0.10660$ (\#143)  & 76.91(57) & 39335 & 68 & 39139 & 75 & 89$\pm^{ 22 }_{ 20 }$ & $1.00$ & 23.9026 & $ 0.41\pm^{ 1.00E+20 }_{ 30.41 }$ & $ 15.12\pm^{ 1.29 }_{ nan }$ & 0.00\\ 
q1230 & $0.10853$ (\#144)  & 76.74(55) & 39335 & 73 & 39139 & 71 & 74$\pm^{ 22 }_{ 19 }$ & $1.00$ & 23.9442 & $ -2.92\pm^{ 2.29E+03 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.57\\ 
q1230 & $0.10940$ (\#145)  & 74.41(56) & 39335 & 72 & 39139 & 71 & 72$\pm^{ 22 }_{ 19 }$ & $1.00$ & 23.9630 & $ -3.09\pm^{ 21.88 }_{ 1.26 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.77\\ 
q1230 & $0.12103$ (\#146)  & 95.35(67) & 39335 & 75 & 39139 & 80 & 87$\pm^{ 26 }_{ 20 }$ & $1.00$ & 24.2142 & $ 1.63E+03\pm^{ 1.00E+20 }_{ 1.66E+03 }$ & $ 16.12\pm^{ 0.32 }_{ nan }$ & 0.52\\ 
rbs1892 & $0.15567$ (\#147)  & 94.13(91) & 4935 & 48 & 4865 & 18 & 242$\pm^{ 87 }_{ 69 }$ & $1.00$ & 24.9625 & $ -2.82\pm^{ 4.80 }_{ 1.52 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.82\\ 
rbs1892 & $0.15633$ (\#148)  & 86.99(91) & 4935 & 52 & 4865 & 20 & 214$\pm^{ 82 }_{ 65 }$ & $1.00$ & 24.9767 & $ -2.83\pm^{ 2.62 }_{ 1.07 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.32\\ 
rbs1892 & $0.16343$ (\#149)  & 79.53(90) & 4936 & 61 & 4865 & 21 & 181$\pm^{ 82 }_{ 63 }$ & $1.00$ & 25.1301 & $ 2.74E+05\pm^{ 1.00E+20 }_{ 2.74E+05 }$ & $ 16.26\pm^{ 0.15 }_{ nan }$ & 0.91\\ 
rbs1892 & $0.17001$ (\#150)  & 90.53(95) & 4937 & 50 & 4865 & 26 & 293$\pm^{ 132 }_{ 93 }$ & $1.00$ & 25.2722 & $ 1.99E+04\pm^{ 1.00E+20 }_{ 1.99E+04 }$ & $ 16.21\pm^{ 0.26 }_{ nan }$ & 1.63\\ 
rbs1892 & $0.17155$ (\#151)  & 87.14(94) & 4937 & 48 & 4865 & 27 & 306$\pm^{ 140 }_{ 98 }$ & $1.00$ & 25.3055 & $ 2.95E+06\pm^{ 1.00E+20 }_{ 2.95E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 2.29\\ 
rbs1892 & $0.17185$ (\#152)  & 86.42(95) & 4937 & 48 & 4865 & 27 & 313$\pm^{ 126 }_{ 95 }$ & $1.00$ & 25.3120 & $ 6.31E+12\pm^{ 1.00E+20 }_{ 6.31E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 2.91\\ 
rbs542 & $0.04455$ (\#153)  & 57.17(47) & 190972 & 9 & nan & nan & 1168$\pm^{ 28 }_{ 29 }$ & $1.00$ & 22.5623 & $ -0.04\pm^{ 1.10 }_{ 0.77 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
rbs542 & $0.04992$ (\#154)  & 55.96(47) & 193118 & 10 & nan & nan & 1213$\pm^{ 28 }_{ 28 }$ & $1.00$ & 22.6783 & $ 3.30\pm^{ 12.51 }_{ 2.52 }$ & $ 15.75\pm^{ 0.19 }_{ 0.39 }$ & 3.36\\ 
rxj0439 & $0.00550$ (\#155)  & -- & -- & -- & -- & -- & -- & -- & 21.7188 & -- & -- & --\\ 
rxj0439 & $0.17680$ (\#156)  & 120.22(96) & 151878 & 14 & 151926 & 16 & 592$\pm^{ 24 }_{ 24 }$ & $1.00$ & 25.4189 & $ 1.65\pm^{ 7.84 }_{ 1.84 }$ & $ 15.59\pm^{ 0.32 }_{ nan }$ & 0.88\\ 
s50716 & $0.00989$ (\#157)  & -- & -- & -- & -- & -- & -- & -- & 21.8136 & -- & -- & --\\ 
s50716 & $0.01766$ (\#158)  & 25.23(27) & 76296 & 14 & nan & nan & 651$\pm^{ 42 }_{ 41 }$ & $1.00$ & 21.9815 & $ 1.72\pm^{ 69.52 }_{ 2.48 }$ & $ 15.61\pm^{ 0.41 }_{ nan }$ & 0.41\\ 
s50716 & $0.08834$ (\#159)  & 48.91(39) & 77059 & 12 & nan & nan & 813$\pm^{ 36 }_{ 37 }$ & $1.00$ & 23.5081 & $ 4.84E+04\pm^{ 5.27E+07 }_{ 4.84E+04 }$ & $ 16.21\pm^{ 0.08 }_{ nan }$ & 7.95\\ 
s50716 & $0.14936$ (\#160)  & 100.74(92) & 76556 & 10 & 76514 & 10 & 894$\pm^{ 39 }_{ 38 }$ & $1.00$ & 24.8262 & $ -0.74\pm^{ 1.12 }_{ 0.72 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.64\\ 
ton28 & $0.03357$ (\#161)  & 53.66(39) & 81822 & 38 & nan & nan & 137$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.3251 & $ -1.47\pm^{ 40.45 }_{ 1.65 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.25\\ 
tons180 & $0.04304$ (\#162)  & 45.92(46) & 181158 & 8 & nan & nan & 1136$\pm^{ 27 }_{ 28 }$ & $1.00$ & 22.5297 & $ -0.34\pm^{ 0.92 }_{ 0.66 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.24\\ 
tons210 & $0.06763$ (\#163)  & 48.59(41) & 6728 & 10 & nan & nan & 664$\pm^{ 122 }_{ 97 }$ & $1.00$ & 23.0608 & $ 3.88E+06\pm^{ 1.00E+20 }_{ 3.89E+06 }$ & $ 16.26\pm^{ 0.20 }_{ nan }$ & 0.73\\ 
tons210 & $0.08558$ (\#164)  & 51.90(45) & 6728 & 8 & nan & nan & 706$\pm^{ 112 }_{ 102 }$ & $1.00$ & 23.4485 & $ -2.10\pm^{ 4.91 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.63\\ 



\hline
\hline
 \end{longtable}
 \end{landscape}

==> Tables/XMM/Latex/xmm_o7_hi_uppers_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllll|l}
\caption[\xmm\ Data, \ovii\ Upper Limits With \hi\ Priors Results (Full)]{\ovii\ upper limit measurements with \xmm\ data, at the prior redshift from the \hi\ lines from Table~\ref{tab:hiPriorsTable}.}
\label{tab:xmmhioviiuppers}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & RGS1 & RGS2 & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & avg exp (s) & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N + (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.13714$ (\#1)  & 92.78(90) & 143804 & 146370 & 1121$\pm^{ 32 }_{ 32 }$ & $1.00$ & 24.5622 & 0.68 & 15.31 & 0.27\\ 
1es1028 & $0.20383$ (\#2)  & 114.22(94) & 146421 & 145107 & 1207$\pm^{ 32 }_{ 35 }$ & $1.00$ & 26.0027 & 0.90 & 15.41 & -0.01\\ 
1es1028 & $0.22121$ (\#3)  & 101.58(92) & 144278 & 146704 & 1198$\pm^{ 35 }_{ 35 }$ & $1.00$ & 26.3781 & 0.58 & 15.26 & 1.33\\ 
1es1553 & $0.03466$ (\#4)  & 38.25(27) & 1791095 & nan & 747$\pm^{ 397 }_{ 326 }$ & $1.97$ & 22.3487 & 0.29 & 14.99 & 0.53\\ 
1es1553 & $0.04273$ (\#5)  & 30.79(21) & 1784759 & nan & 489$\pm^{ 628 }_{ 294 }$ & $2.72$ & 22.5230 & 0.54 & 15.23 & 2.85\\ 
1es1553 & $0.06364$ (\#6*)  & 64.48(28) & 1661330 & nan & 27$\pm^{ 12 }_{ 9 }$ & $7.49$ & 22.9746 & 0.53 & 15.23 & 1.84\\ 
1es1553 & $0.21869$ (\#7)  & 108.81(87) & 1691684 & 1788288 & 1010$\pm^{ 415 }_{ 304 }$ & $1.74$ & 26.3237 & 0.36 & 15.08 & -0.07\\ 
3c249 & $0.13470$ (\#8)  & 67.71(86) & 2642 & 2524 & 336$\pm^{ 146 }_{ 105 }$ & $1.00$ & 24.5095 & 5.00E+19 & 16.46 & 0.52\\ 
3c249 & $0.26664$ (\#9)  & 79.78(93) & 2639 & 2524 & 306$\pm^{ 146 }_{ 111 }$ & $1.00$ & 27.3594 & 5.00E+19 & 16.46 & -0.00\\ 
3c273 & $0.00758$ (\#10)  & -- & -- & -- & -- & -- & 21.7637 & -- & -- & --\\ 
3c273 & $0.06707$ (\#11*)  & 35.22(22) & 897879 & nan & 4641$\pm^{ 37 }_{ 41 }$ & $1.00$ & 23.0487 & 0.30 & 15.01 & 0.86\\ 
3c273 & $0.07359$ (\#12*)  & 45.49(29) & 930374 & nan & 4656$\pm^{ 32 }_{ 34 }$ & $1.00$ & 23.1895 & 0.20 & 14.84 & 0.39\\ 
3c273 & $0.13960$ (\#13)  & 68.74(61) & 892303 & 1027847 & 5246$\pm^{ 31 }_{ 31 }$ & $1.00$ & 24.6154 & 0.12 & 14.62 & 12.82\\ 
h1821 & $0.00944$ (\#14)  & -- & -- & -- & -- & -- & 21.8039 & -- & -- & --\\ 
h1821 & $0.06779$ (\#15)  & 48.43(43) & 28966 & nan & 1081$\pm^{ 99 }_{ 91 }$ & $1.00$ & 23.0643 & 5.00E+19 & 16.46 & 1.16\\ 
h1821 & $0.08483$ (\#16)  & 62.62(44) & 31062 & nan & 1008$\pm^{ 91 }_{ 87 }$ & $1.00$ & 23.4323 & 9.01E+07 & 16.29 & 0.54\\ 
h1821 & $0.12147$ (\#17)  & 96.56(82) & 30593 & 43368 & 1284$\pm^{ 89 }_{ 85 }$ & $1.00$ & 24.2238 & 1.24E+04 & 16.15 & 1.85\\ 
h1821 & $0.19817$ (\#18)  & 79.32(81) & 32357 & 41356 & 1363$\pm^{ 112 }_{ 109 }$ & $1.00$ & 25.8805 & 1.04 & 15.46 & 1.30\\ 
h1821 & $0.21321$ (\#19)  & 110.19(98) & 31737 & 41863 & 1644$\pm^{ 133 }_{ 107 }$ & $1.00$ & 26.2053 & 2.17E+07 & 16.29 & 2.38\\ 
h1821 & $0.24531$ (\#20)  & 119.80(98) & 31065 & 44448 & 1591$\pm^{ 120 }_{ 113 }$ & $1.00$ & 26.8987 & 9.68 & 15.89 & 0.06\\ 
h2356 & $0.03830$ (\#21)  & 60.56(47) & 466679 & nan & 1093$\pm^{ 15 }_{ 15 }$ & $1.00$ & 22.4273 & 0.59 & 15.27 & -0.02\\ 
h2356 & $0.07881$ (\#22)  & 44.92(38) & 468683 & nan & 1173$\pm^{ 21 }_{ 20 }$ & $1.00$ & 23.3023 & 0.52 & 15.23 & 2.04\\ 
h2356 & $0.10467$ (\#23)  & 52.51(56) & 471489 & 510756 & 1280$\pm^{ 22 }_{ 21 }$ & $1.00$ & 23.8609 & 0.93 & 15.42 & 1.39\\ 
h2356 & $0.15613$ (\#24)  & 105.03(97) & 482157 & 504552 & 1323$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.9724 & 0.57 & 15.26 & 2.10\\ 
he0226 & $0.14274$ (\#25)  & 83.16(89) & 31710 & 31705 & 257$\pm^{ 34 }_{ 31 }$ & $1.00$ & 24.6832 & 1.74 & 15.61 & 0.97\\ 
he0226 & $0.39890$ (\#26)  & 85.66(67) & 31717 & 31717 & 409$\pm^{ 80 }_{ 73 }$ & $1.00$ & 30.2162 & 3.96E+07 & 16.30 & 0.01\\ 
he0226 & $0.41024$ (\#27)  & 81.69(56) & 31717 & 31717 & 421$\pm^{ 91 }_{ 82 }$ & $1.00$ & 30.4612 & 2.33E+08 & 16.29 & 0.00\\ 
i22456 & $0.00443$ (\#28)  & -- & -- & -- & -- & -- & 21.6957 & -- & -- & --\\ 
i22456 & $0.09941$ (\#29)  & 74.98(61) & 79883 & 73453 & 671$\pm^{ 38 }_{ 37 }$ & $1.00$ & 23.7473 & 8.80 & 15.88 & 0.00\\ 
mr2251 & $0.01068$ (\#30)  & -- & -- & -- & -- & -- & 21.8307 & -- & -- & --\\ 
mr2251 & $0.01449$ (\#31)  & 37.36(27) & 446548 & nan & 2964$\pm^{ 3361 }_{ 1081 }$ & $0.01$ & 21.9130 & 0.39 & 15.10 & 2.50\\ 
mr2251 & $0.06131$ (\#32)  & 32.34(25) & 452767 & nan & 117$\pm^{ 170 }_{ 69 }$ & $5.55$ & 22.9243 & 7.53 & 15.85 & 4.17\\ 
mr2251 & $0.06190$ (\#33)  & 29.54(24) & 452283 & nan & 59$\pm^{ 91 }_{ 37 }$ & $6.67$ & 22.9370 & 83.57 & 16.01 & 5.95\\ 
mr2251 & $0.06276$ (\#34)  & 30.33(22) & 451202 & nan & 57$\pm^{ 104 }_{ 37 }$ & $6.71$ & 22.9556 & 5.82 & 15.85 & 4.37\\ 
mr2251 & $0.06327$ (\#35*)  & 31.04(20) & 449939 & nan & 30$\pm^{ 81 }_{ 20 }$ & $7.77$ & 22.9666 & 2.78 & 15.72 & 2.99\\ 
mr2251 & $0.06381$ (\#36*)  & 33.43(22) & 451202 & nan & 148$\pm^{ 162 }_{ 116 }$ & $5.14$ & 22.9783 & 0.79 & 15.37 & -0.00\\ 
mrk478 & $0.06166$ (\#37)  & 61.33(42) & 192118 & nan & 253$\pm^{ 786 }_{ 195 }$ & $2.48$ & 22.9319 & 3.45 & 15.77 & 0.07\\ 
mrk478 & $0.06578$ (\#38)  & 54.57(42) & 192119 & nan & 606$\pm^{ 1058 }_{ 523 }$ & $1.09$ & 23.0208 & 7.26E+05 & 16.21 & 3.82\\ 
mrk478 & $0.07213$ (\#39)  & 54.93(42) & 192121 & nan & 640$\pm^{ 1985 }_{ 489 }$ & $1.00$ & 23.1580 & 2.87 & 15.73 & 0.10\\ 
mrk876 & $0.01159$ (\#40)  & -- & -- & -- & -- & -- & 21.8503 & -- & -- & --\\ 
mrk876 & $0.05598$ (\#41)  & 44.97(46) & 2714 & nan & 477$\pm^{ 142 }_{ 112 }$ & $1.00$ & 22.8092 & 5.00E+19 & 16.46 & 0.21\\ 
mrk876 & $0.08709$ (\#42)  & 37.14(46) & 2802 & nan & 345$\pm^{ 146 }_{ 103 }$ & $1.00$ & 23.4811 & 5.00E+19 & 16.46 & 1.36\\ 
mrk876 & $0.08858$ (\#43)  & 37.69(46) & 2802 & nan & 378$\pm^{ 139 }_{ 105 }$ & $1.00$ & 23.5133 & 5.00E+19 & 16.46 & 1.70\\ 
mrk876 & $0.08917$ (\#44)  & 37.84(47) & 2802 & 996 & 377$\pm^{ 134 }_{ 98 }$ & $1.00$ & 23.5261 & 5.00E+19 & 16.46 & 1.65\\ 
mrk876 & $0.11487$ (\#45)  & 73.35(75) & 2743 & 2633 & 529$\pm^{ 144 }_{ 121 }$ & $1.00$ & 24.0812 & 5.00E+19 & 16.46 & 0.00\\ 
ngc7469 & $0.00981$ (\#46)  & -- & -- & -- & -- & -- & 21.8119 & -- & -- & --\\ 
pg0003 & $0.08299$ (\#47)  & 59.05(43) & 13037 & nan & 234$\pm^{ 52 }_{ 46 }$ & $1.00$ & 23.3926 & 1.51E+06 & 16.25 & 0.47\\ 
pg0003 & $0.17139$ (\#48)  & 111.61(94) & 13033 & 12941 & 332$\pm^{ 65 }_{ 54 }$ & $1.00$ & 25.3020 & 5.41E+14 & 16.42 & 0.31\\ 
pg0003 & $0.22541$ (\#49)  & 114.13(94) & 13034 & 12838 & 231$\pm^{ 58 }_{ 50 }$ & $1.00$ & 26.4689 & 1.60E+09 & 16.33 & 0.00\\ 
pg0003 & $0.38633$ (\#50)  & 104.20(85) & 13041 & 12919 & 115$\pm^{ 65 }_{ 47 }$ & $1.00$ & 29.9447 & 1.14 & 15.50 & 12.63\\ 
pg0003 & $0.42051$ (\#51)  & 114.71(91) & 13041 & 12843 & 362$\pm^{ 115 }_{ 95 }$ & $1.00$ & 30.6830 & 4.83E+09 & 16.31 & 0.06\\ 
pg0804 & $0.05015$ (\#52)  & 46.31(37) & 27851 & nan & 1439$\pm^{ 93 }_{ 87 }$ & $1.00$ & 22.6832 & 5.00E+19 & 16.41 & 7.42\\ 
pg0804 & $0.05576$ (\#53)  & 53.92(41) & 28550 & nan & 1333$\pm^{ 83 }_{ 80 }$ & $1.00$ & 22.8044 & 3.15E+04 & 16.15 & 0.29\\ 
pg0804 & $0.36379$ (\#54)  & 127.43(96) & 29665 & 30901 & 2024$\pm^{ 141 }_{ 134 }$ & $1.00$ & 29.4579 & 1.46 & 15.57 & 0.42\\ 
pg0832 & $0.01753$ (\#55)  & -- & -- & -- & -- & -- & 21.9786 & -- & -- & --\\ 
pg0832 & $0.02793$ (\#56)  & 52.15(36) & 20654 & nan & 26$\pm^{ 18 }_{ 14 }$ & $1.00$ & 22.2033 & 1.67 & 15.61 & 9.82\\ 
pg0832 & $0.08748$ (\#57)  & 53.03(45) & 20655 & nan & 71$\pm^{ 25 }_{ 19 }$ & $1.00$ & 23.4896 & 5.00E+19 & 16.46 & 1.13\\ 
pg0832 & $0.10171$ (\#58)  & 73.57(56) & 20655 & 20637 & 84$\pm^{ 30 }_{ 22 }$ & $1.00$ & 23.7969 & 5.00E+19 & 16.46 & 0.91\\ 
pg0832 & $0.18391$ (\#59)  & 60.33(41) & 20654 & 20637 & 70$\pm^{ 54 }_{ 32 }$ & $1.00$ & 25.5725 & 5.00E+19 & 16.41 & 1.25\\ 
pg0832 & $0.27503$ (\#60)  & 124.41(86) & 20656 & 20637 & 58$\pm^{ 29 }_{ 21 }$ & $1.00$ & 27.5406 & 5.00E+19 & 16.46 & 0.01\\ 
pg0832 & $0.27694$ (\#61)  & 119.21(86) & 20656 & 20637 & 60$\pm^{ 28 }_{ 22 }$ & $1.00$ & 27.5819 & 5.00E+19 & 16.46 & 0.02\\ 
pg0832 & $0.32572$ (\#62*)  & 136.80(85) & 20656 & 20645 & 51$\pm^{ 28 }_{ 20 }$ & $1.00$ & 28.6356 & 5.40E+04 & 16.18 & 0.31\\ 
pg0838 & $0.06583$ (\#63)  & 1.34(41) & 1609 & nan & 0$\pm^{ 36 }_{ -0 }$ & $1.00$ & 23.0219 & 5.00E+19 & 16.46 & 0.00\\ 
pg0838 & $0.08628$ (\#64)  & 16.24(44) & 1609 & nan & 130$\pm^{ 124 }_{ 72 }$ & $1.00$ & 23.4636 & 5.00E+19 & 16.46 & 0.17\\ 
pg0838 & $0.12676$ (\#65)  & 32.38(79) & 1609 & 1519 & 75$\pm^{ 109 }_{ 75 }$ & $1.00$ & 24.3380 & 5.00E+19 & 16.46 & 0.75\\ 
pg0953 & $0.16319$ (\#66)  & 129.94(91) & 12778 & 12309 & 593$\pm^{ 77 }_{ 71 }$ & $1.00$ & 25.1249 & 2.68E+03 & 16.17 & 0.09\\ 
pg0953 & $0.19221$ (\#67)  & 122.56(92) & 12777 & 12309 & 612$\pm^{ 78 }_{ 71 }$ & $1.00$ & 25.7517 & 238.36 & 16.02 & 0.03\\ 
pg1048 & $0.00642$ (\#68)  & -- & -- & -- & -- & -- & 21.7387 & -- & -- & --\\ 
pg1048 & $0.02414$ (\#69)  & 32.85(32) & 18864 & nan & 156$\pm^{ 38 }_{ 33 }$ & $1.00$ & 22.1214 & 5.00E+19 & 16.41 & 0.12\\ 
pg1115 & $0.09511$ (\#70)  & 47.02(50) & 17510 & 16953 & 325$\pm^{ 54 }_{ 46 }$ & $1.00$ & 23.6544 & 5.00E+19 & 16.41 & 0.20\\ 
pg1115 & $0.12059$ (\#71)  & 98.56(73) & 17510 & 16953 & 310$\pm^{ 48 }_{ 44 }$ & $1.00$ & 24.2047 & 5.00E+19 & 16.46 & 2.50\\ 
pg1115 & $0.12741$ (\#72)  & 107.59(76) & 17513 & 16953 & 311$\pm^{ 51 }_{ 47 }$ & $1.00$ & 24.3521 & 4.12E+03 & 16.14 & 0.00\\ 
pg1116 & $0.04114$ (\#73)  & 41.06(39) & 284047 & nan & 540$\pm^{ 17 }_{ 17 }$ & $1.00$ & 22.4886 & 0.75 & 15.35 & 1.16\\ 
pg1116 & $0.06251$ (\#74)  & 40.85(30) & 283934 & nan & 549$\pm^{ 22 }_{ 21 }$ & $1.00$ & 22.9502 & 71.62 & 16.02 & 0.23\\ 
pg1116 & $0.08382$ (\#75)  & 46.62(32) & 284638 & nan & 588$\pm^{ 22 }_{ 18 }$ & $1.00$ & 23.4105 & 5.00E+19 & 16.46 & 8.15\\ 
pg1116 & $0.09210$ (\#76)  & 51.16(38) & 292136 & 222826 & 576$\pm^{ 20 }_{ 19 }$ & $1.00$ & 23.5894 & 1.57 & 15.59 & 0.07\\ 
pg1116 & $0.09281$ (\#77)  & 50.89(38) & 292136 & 222826 & 579$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.6047 & 2.00 & 15.65 & 0.25\\ 
pg1116 & $0.13373$ (\#78)  & 89.85(89) & 277711 & 284726 & 680$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.4886 & 4.13 & 15.79 & 5.37\\ 
pg1116 & $0.13851$ (\#79)  & 94.60(91) & 277702 & 291047 & 693$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.5918 & 2.05 & 15.65 & 2.45\\ 
pg1211 & $0.02586$ (\#80)  & 33.66(32) & 769591 & nan & 575$\pm^{ 12 }_{ 12 }$ & $1.00$ & 22.1586 & 0.86 & 15.41 & 0.25\\ 
pg1211 & $0.05443$ (\#81)  & 49.81(35) & 745965 & nan & 634$\pm^{ 12 }_{ 12 }$ & $1.00$ & 22.7757 & 1.25 & 15.53 & 0.06\\ 
pg1216 & $0.00842$ (\#82)  & -- & -- & -- & -- & -- & 21.7819 & -- & -- & --\\ 
pg1216 & $0.07969$ (\#83)  & 53.17(43) & 11245 & nan & 185$\pm^{ 50 }_{ 39 }$ & $1.00$ & 23.3213 & 5.00E+19 & 16.41 & 0.44\\ 
pg1216 & $0.12372$ (\#84)  & 107.60(78) & 11245 & 11258 & 182$\pm^{ 51 }_{ 48 }$ & $1.00$ & 24.2724 & 5.00E+19 & 16.41 & 3.27\\ 
pg1216 & $0.12473$ (\#85)  & 107.90(78) & 11245 & 11258 & 186$\pm^{ 59 }_{ 40 }$ & $1.00$ & 24.2942 & 5.00E+19 & 16.46 & 1.76\\ 
pg1216 & $0.17950$ (\#86)  & 106.70(95) & 11257 & 11258 & 243$\pm^{ 51 }_{ 45 }$ & $1.00$ & 25.4772 & 5.00E+19 & 16.46 & 2.17\\ 
pg1216 & $0.20014$ (\#87)  & 86.38(92) & 11257 & 11258 & 179$\pm^{ 53 }_{ 39 }$ & $1.00$ & 25.9230 & 5.00E+19 & 16.41 & 1.23\\ 
pg1216 & $0.21258$ (\#88)  & 84.99(93) & 11257 & 11258 & 191$\pm^{ 48 }_{ 41 }$ & $1.00$ & 26.1917 & 5.00E+19 & 16.46 & 0.49\\ 
pg1216 & $0.28204$ (\#89)  & 112.71(89) & 11258 & 11258 & 237$\pm^{ 66 }_{ 56 }$ & $1.00$ & 27.6921 & 3.33 & 15.76 & 0.83\\ 
pg1229 & $0.05018$ (\#90)  & 55.71(43) & 24016 & nan & 521$\pm^{ 63 }_{ 49 }$ & $1.00$ & 22.6839 & 5.00E+19 & 16.41 & 3.04\\ 
pg1259 & $0.05563$ (\#91)  & 50.01(43) & 11485 & nan & 165$\pm^{ 50 }_{ 38 }$ & $1.00$ & 22.8016 & 5.00E+19 & 16.46 & 0.63\\ 
pg1259 & $0.15136$ (\#92)  & 99.16(90) & 11483 & 11479 & 130$\pm^{ 43 }_{ 35 }$ & $1.00$ & 24.8694 & 3.39E+16 & 16.46 & 0.08\\ 
pg1259 & $0.16647$ (\#93)  & 105.90(92) & 11483 & 11479 & 145$\pm^{ 43 }_{ 36 }$ & $1.00$ & 25.1958 & 5.57 & 15.83 & 0.61\\ 
pg1259 & $0.17893$ (\#94)  & 108.49(96) & 11483 & 11479 & 180$\pm^{ 52 }_{ 40 }$ & $1.00$ & 25.4649 & 5.00E+19 & 16.46 & 0.92\\ 
pg1259 & $0.22376$ (\#95)  & 105.77(93) & 11483 & 11479 & 277$\pm^{ 65 }_{ 56 }$ & $1.00$ & 26.4332 & 2.75E+12 & 16.39 & 0.01\\ 
pg1259 & $0.24126$ (\#96)  & 121.27(95) & 11483 & 11479 & 149$\pm^{ 49 }_{ 40 }$ & $1.00$ & 26.8112 & 1.20E+03 & 16.12 & 0.44\\ 
pg1259 & $0.31974$ (\#97)  & 80.23(82) & 11483 & 11480 & 293$\pm^{ 92 }_{ 69 }$ & $1.00$ & 28.5064 & 5.00E+19 & 16.41 & 0.53\\ 
pg1259 & $0.36212$ (\#98)  & 114.78(79) & 11487 & 11480 & 291$\pm^{ 96 }_{ 78 }$ & $1.00$ & 29.4218 & 5.00E+19 & 16.46 & 1.38\\ 
pg1259 & $0.38254$ (\#99)  & 134.54(94) & 11487 & 11480 & 351$\pm^{ 94 }_{ 79 }$ & $1.00$ & 29.8629 & 1.40E+05 & 16.23 & 0.04\\ 
pg1259 & $0.38266$ (\#100)  & 134.54(94) & 11487 & 11480 & 351$\pm^{ 93 }_{ 79 }$ & $1.00$ & 29.8655 & 2.68E+06 & 16.24 & 0.04\\ 
pg1307 & $0.08345$ (\#101)  & 53.56(43) & 9827 & nan & 196$\pm^{ 53 }_{ 46 }$ & $1.00$ & 23.4025 & 1.55 & 15.59 & 2.97\\ 
pg1309 & $0.03861$ (\#102)  & 52.72(41) & 27263 & nan & 74$\pm^{ 24 }_{ 17 }$ & $1.00$ & 22.4340 & 5.00E+19 & 16.46 & 0.98\\ 
pg1309 & $0.17740$ (\#103)  & 116.75(95) & 27265 & 26163 & 153$\pm^{ 33 }_{ 25 }$ & $1.00$ & 25.4318 & 5.00E+19 & 16.46 & 2.31\\ 
pg1309 & $0.17852$ (\#104)  & 121.37(94) & 27265 & 26163 & 155$\pm^{ 35 }_{ 26 }$ & $1.00$ & 25.4560 & 5.00E+19 & 16.46 & 2.13\\ 
pg1309 & $0.17918$ (\#105)  & 120.71(95) & 27265 & 26163 & 154$\pm^{ 28 }_{ 26 }$ & $1.00$ & 25.4703 & 5.00E+19 & 16.41 & 1.80\\ 
pg1309 & $0.18143$ (\#106)  & 116.88(93) & 27265 & 26163 & 141$\pm^{ 28 }_{ 25 }$ & $1.00$ & 25.5189 & 5.00E+19 & 16.46 & 0.09\\ 
pg1444 & $0.22031$ (\#107)  & 113.67(93) & 17674 & 17137 & 183$\pm^{ 40 }_{ 35 }$ & $1.00$ & 26.3587 & 1.70 & 15.61 & 1.34\\ 
pg1626 & $0.06137$ (\#108)  & -- & -- & -- & -- & -- & 22.9256 & -- & -- & --\\ 
phl1811 & $0.05143$ (\#109)  & -- & -- & -- & -- & -- & 22.7109 & -- & -- & --\\ 
phl1811 & $0.05813$ (\#110)  & -- & -- & -- & -- & -- & 22.8556 & -- & -- & --\\ 
phl1811 & $0.08085$ (\#111)  & -- & -- & -- & -- & -- & 23.3464 & -- & -- & --\\ 
phl1811 & $0.08163$ (\#112)  & -- & -- & -- & -- & -- & 23.3632 & -- & -- & --\\ 
phl1811 & $0.12003$ (\#113)  & 77.84(58) & 74729 & 79201 & 33$\pm^{ 15 }_{ 14 }$ & $1.00$ & 24.1926 & 5.00E+19 & 16.46 & 1.01\\ 
phl1811 & $0.15787$ (\#114)  & -- & -- & -- & -- & -- & 25.0100 & -- & -- & --\\ 
pks0312 & $0.11454$ (\#115)  & 64.38(70) & 23887 & 22982 & 266$\pm^{ 37 }_{ 35 }$ & $1.00$ & 24.0741 & 5.00E+19 & 16.46 & 2.67\\ 
pks0405 & $0.02510$ (\#116)  & 41.67(34) & 137701 & nan & 304$\pm^{ 19 }_{ 17 }$ & $1.00$ & 22.1422 & 34.45 & 15.98 & -0.00\\ 
pks0405 & $0.05902$ (\#117)  & 53.75(40) & 134613 & nan & 316$\pm^{ 20 }_{ 19 }$ & $1.00$ & 22.8748 & 0.81 & 15.38 & 2.69\\ 
pks0405 & $0.09719$ (\#118)  & 64.86(45) & 135771 & nan & 354$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.6993 & 1.07 & 15.48 & 1.60\\ 
pks0405 & $0.10152$ (\#119)  & 65.13(49) & 134959 & 138649 & 355$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.7928 & 0.77 & 15.36 & 3.98\\ 
pks0405 & $0.10298$ (\#120)  & 68.35(50) & 134879 & 138649 & 368$\pm^{ 20 }_{ 20 }$ & $1.00$ & 23.8244 & 1.29 & 15.52 & 0.70\\ 
pks0405 & $0.19456$ (\#121)  & 116.94(93) & 137986 & 134948 & 405$\pm^{ 21 }_{ 21 }$ & $1.00$ & 25.8025 & 1.82E+04 & 16.14 & 1.98\\ 
pks0405 & $0.21976$ (\#122)  & 126.59(92) & 137232 & 135759 & 408$\pm^{ 22 }_{ 22 }$ & $1.00$ & 26.3468 & 1.05 & 15.47 & 0.87\\ 
pks0405 & $0.24564$ (\#123)  & 98.79(93) & 136439 & 138647 & 383$\pm^{ 23 }_{ 23 }$ & $1.00$ & 26.9058 & 0.97 & 15.43 & 0.95\\ 
pks0405 & $0.29748$ (\#124)  & 98.21(89) & 135766 & 137130 & 382$\pm^{ 27 }_{ 25 }$ & $1.00$ & 28.0256 & 2.53 & 15.71 & 0.01\\ 
pks0405 & $0.31016$ (\#125)  & 96.82(90) & 137275 & 137114 & 378$\pm^{ 26 }_{ 25 }$ & $1.00$ & 28.2995 & 0.56 & 15.24 & 6.68\\ 
pks0405 & $0.32502$ (\#126)  & 92.49(84) & 135467 & 137166 & 414$\pm^{ 31 }_{ 30 }$ & $1.00$ & 28.6204 & 832.36 & 16.10 & 0.79\\ 
pks0405 & $0.49508$ (\#127)  & 112.25(94) & 138729 & 137202 & 536$\pm^{ 45 }_{ 43 }$ & $1.00$ & 32.2937 & 0.74 & 15.34 & 3.47\\ 
pks0558 & $0.10472$ (\#128)  & 82.71(58) & 705422 & 787021 & 2580$\pm^{ 30 }_{ 21 }$ & $1.00$ & 23.8620 & 0.42 & 15.14 & 0.22\\ 
pks2155 & $0.05708$ (\#129)  & 42.12(39) & 1687774 & nan & 641$\pm^{ 88 }_{ 82 }$ & $4.94$ & 22.8329 & 0.12 & 14.62 & 6.22\\ 
pks2155 & $0.06236$ (\#130)  & -- & -- & -- & -- & -- & 22.9470 & -- & -- & --\\ 
pks2155 & $0.10586$ (\#131)  & 60.97(48) & 1694875 & 1691927 & 1743$\pm^{ 77 }_{ 762 }$ & $3.33$ & 23.8866 & 0.22 & 14.89 & -0.23\\ 
q0045 & $0.05590$ (\#132)  & 48.77(38) & 13827 & nan & 59$\pm^{ 32 }_{ 22 }$ & $1.00$ & 22.8074 & 5.00E+19 & 16.46 & 0.14\\ 
q0045 & $0.06377$ (\#133)  & -- & -- & -- & -- & -- & 22.9774 & -- & -- & --\\ 
q1230 & $0.08344$ (\#134)  & 49.74(34) & 39335 & nan & 83$\pm^{ 24 }_{ 21 }$ & $1.00$ & 23.4023 & 3.62 & 15.77 & 0.96\\ 
q1230 & $0.08540$ (\#135)  & 49.18(36) & 39335 & nan & 99$\pm^{ 24 }_{ 23 }$ & $1.00$ & 23.4446 & 5.00E+19 & 16.46 & 0.11\\ 
q1230 & $0.09444$ (\#136)  & 57.34(47) & 39335 & 39139 & 98$\pm^{ 26 }_{ 19 }$ & $1.00$ & 23.6399 & 5.00E+19 & 16.46 & 1.01\\ 
q1230 & $0.10000$ (\#137)  & 69.52(51) & 39335 & 39139 & 67$\pm^{ 22 }_{ 19 }$ & $1.00$ & 23.7600 & 1.09 & 15.47 & 4.46\\ 
q1230 & $0.10525$ (\#138)  & 71.15(53) & 39335 & 39139 & 95$\pm^{ 23 }_{ 20 }$ & $1.00$ & 23.8734 & 5.00E+19 & 16.41 & 0.19\\ 
q1230 & $0.10549$ (\#139)  & 74.01(55) & 39335 & 39139 & 93$\pm^{ 22 }_{ 20 }$ & $1.00$ & 23.8786 & 5.00E+19 & 16.46 & 0.15\\ 
q1230 & $0.10566$ (\#140)  & 74.03(55) & 39335 & 39139 & 93$\pm^{ 23 }_{ 20 }$ & $1.00$ & 23.8823 & 5.00E+19 & 16.46 & 0.12\\ 
q1230 & $0.10612$ (\#141)  & 75.39(55) & 39335 & 39139 & 90$\pm^{ 22 }_{ 20 }$ & $1.00$ & 23.8922 & 5.00E+19 & 16.41 & 0.03\\ 
q1230 & $0.10639$ (\#142)  & 76.90(57) & 39335 & 39139 & 89$\pm^{ 23 }_{ 20 }$ & $1.00$ & 23.8980 & 5.00E+19 & 16.46 & 0.01\\ 
q1230 & $0.10660$ (\#143)  & 76.91(57) & 39335 & 39139 & 89$\pm^{ 22 }_{ 20 }$ & $1.00$ & 23.9026 & 5.00E+19 & 16.41 & 0.00\\ 
q1230 & $0.10853$ (\#144)  & 76.74(55) & 39335 & 39139 & 74$\pm^{ 22 }_{ 19 }$ & $1.00$ & 23.9442 & 1.15E+03 & 16.11 & 0.57\\ 
q1230 & $0.10940$ (\#145)  & 74.41(56) & 39335 & 39139 & 72$\pm^{ 22 }_{ 19 }$ & $1.00$ & 23.9630 & 11.57 & 15.93 & 0.77\\ 
q1230 & $0.12103$ (\#146)  & 95.35(67) & 39335 & 39139 & 87$\pm^{ 26 }_{ 20 }$ & $1.00$ & 24.2142 & 5.00E+19 & 16.43 & 0.52\\ 
rbs1892 & $0.15567$ (\#147)  & 94.13(91) & 4935 & 4865 & 242$\pm^{ 87 }_{ 69 }$ & $1.00$ & 24.9625 & 3.16 & 15.75 & 0.82\\ 
rbs1892 & $0.15633$ (\#148)  & 86.99(91) & 4935 & 4865 & 214$\pm^{ 82 }_{ 65 }$ & $1.00$ & 24.9767 & 1.85 & 15.62 & 1.32\\ 
rbs1892 & $0.16343$ (\#149)  & 79.53(90) & 4936 & 4865 & 181$\pm^{ 82 }_{ 63 }$ & $1.00$ & 25.1301 & 5.00E+19 & 16.41 & 0.91\\ 
rbs1892 & $0.17001$ (\#150)  & 90.53(95) & 4937 & 4865 & 293$\pm^{ 132 }_{ 93 }$ & $1.00$ & 25.2722 & 5.00E+19 & 16.46 & 1.63\\ 
rbs1892 & $0.17155$ (\#151)  & 87.14(94) & 4937 & 4865 & 306$\pm^{ 140 }_{ 98 }$ & $1.00$ & 25.3055 & 5.00E+19 & 16.41 & 2.29\\ 
rbs1892 & $0.17185$ (\#152)  & 86.42(95) & 4937 & 4865 & 313$\pm^{ 126 }_{ 95 }$ & $1.00$ & 25.3120 & 5.00E+19 & 16.46 & 2.91\\ 
rbs542 & $0.04455$ (\#153)  & 57.17(47) & 190972 & nan & 1168$\pm^{ 28 }_{ 29 }$ & $1.00$ & 22.5623 & 0.93 & 15.42 & 0.01\\ 
rbs542 & $0.04992$ (\#154)  & 55.96(47) & 193118 & nan & 1213$\pm^{ 28 }_{ 28 }$ & $1.00$ & 22.6783 & 7.51 & 15.88 & 3.36\\ 
rxj0439 & $0.00550$ (\#155)  & -- & -- & -- & -- & -- & 21.7188 & -- & -- & --\\ 
rxj0439 & $0.17680$ (\#156)  & 120.22(96) & 151878 & 151926 & 592$\pm^{ 24 }_{ 24 }$ & $1.00$ & 25.4189 & 4.84 & 15.82 & 0.88\\ 
s50716 & $0.00989$ (\#157)  & -- & -- & -- & -- & -- & 21.8136 & -- & -- & --\\ 
s50716 & $0.01766$ (\#158)  & 25.23(27) & 76296 & nan & 651$\pm^{ 42 }_{ 41 }$ & $1.00$ & 21.9815 & 36.00 & 15.98 & 0.41\\ 
s50716 & $0.08834$ (\#159)  & 48.91(39) & 77059 & nan & 813$\pm^{ 36 }_{ 37 }$ & $1.00$ & 23.5081 & 2.64E+07 & 16.29 & 7.95\\ 
s50716 & $0.14936$ (\#160)  & 100.74(92) & 76556 & 76514 & 894$\pm^{ 39 }_{ 38 }$ & $1.00$ & 24.8262 & 0.92 & 15.43 & 0.64\\ 
ton28 & $0.03357$ (\#161)  & 53.66(39) & 81822 & nan & 137$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.3251 & 21.05 & 15.92 & 0.25\\ 
tons180 & $0.04304$ (\#162)  & 45.92(46) & 181158 & nan & 1136$\pm^{ 27 }_{ 28 }$ & $1.00$ & 22.5297 & 0.79 & 15.37 & 0.24\\ 
tons210 & $0.06763$ (\#163)  & 48.59(41) & 6728 & nan & 664$\pm^{ 122 }_{ 97 }$ & $1.00$ & 23.0608 & 5.00E+19 & 16.46 & 0.73\\ 
tons210 & $0.08558$ (\#164)  & 51.90(45) & 6728 & nan & 706$\pm^{ 112 }_{ 102 }$ & $1.00$ & 23.4485 & 3.12 & 15.75 & 0.63\\ 

\hline
\hline
\end{longtable}
\end{landscape}

==> Tables/XMM/Latex/xmm_o7_o6_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllllll|l}
\caption[\xmm\ Data, \ovii\ With \ovi\ Priors Results (Full)]{\ovii\ measurements with \xmm\ data, at the prior redshift from the \ovi\ lines from Table~\ref{tab:oviPriorsTable}. Column "\%" reports the percent background level, ${B}/{S+B}$, where $B$ is the background count rate, and $S$ the source count rate. Entries with an asterisk sign indicate poor fits; entries that have a `$\nodata$' sign indicate lines that fall in a region of reduced efficiency, and therefore they could not be constrained (see Sec.~\ref{sec:ccdgapsexclusions}).}
\label{tab:XMMfirst}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & \multicolumn{2}{c}{RGS1} & \multicolumn{2}{c}{RGS2} & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \% & avg exp (s) & \%    & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.12314$ (\#1)  & 95.40(79) & 144787 & 10 & 147275 & 7 & 1102$\pm^{ 30 }_{ 30 }$ & $1.00$ & 24.2598 & $ 0.55\pm^{ 1.74 }_{ 0.88 }$ & $ 15.24\pm^{ 0.44 }_{ nan }$ & 0.40\\ 
1es1028 & $0.13706$ (\#2)  & 92.82(90) & 143804 & 9 & 146370 & 7 & 1121$\pm^{ 33 }_{ 32 }$ & $1.00$ & 24.5605 & $ -0.31\pm^{ 0.85 }_{ 0.56 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.22\\ 
1es1028 & $0.33735$ (\#3)  & 86.46(91) & 145450 & 17 & 146420 & 22 & 1324$\pm^{ 48 }_{ 46 }$ & $1.00$ & 28.8868 & $ -0.78\pm^{ 0.84 }_{ 0.57 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.08\\ 
1es1553 & $0.18759$ (\#4)  & 102.10(88) & 1793737 & 7 & 1757303 & 7 & 1796$\pm^{ 13 }_{ 12 }$ & $1.00$ & 25.6519 & $ 0.60\pm^{ 0.32 }_{ 0.26 }$ & $ 15.27\pm^{ 0.15 }_{ 0.21 }$ & 7.82\\ 
1es1553 & $0.18775$ (\#5)  & 102.34(88) & 1793737 & 7 & 1757303 & 7 & 1796$\pm^{ 13 }_{ 12 }$ & $1.00$ & 25.6554 & $ 0.57\pm^{ 0.30 }_{ 0.25 }$ & $ 15.26\pm^{ 0.15 }_{ 0.22 }$ & 7.53\\ 
1es1553 & $0.18984$ (\#6)  & 105.72(86) & 1794800 & 7 & 1753128 & 7 & 1778$\pm^{ 12 }_{ 12 }$ & $1.00$ & 25.7005 & $ -0.05\pm^{ 0.17 }_{ 0.23 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.16\\ 
1es1553 & $0.21631$ (\#7)  & 84.95(81) & 1756247 & 7 & 1757203 & 8 & 1778$\pm^{ 14 }_{ 14 }$ & $1.00$ & 26.2723 & $ 0.19\pm^{ 0.25 }_{ 0.22 }$ & $ 14.83\pm^{ 0.33 }_{ nan }$ & 0.95\\ 
1es1553 & $0.31130$ (\#8)  & 113.79(90) & 1740303 & 11 & 1677696 & 14 & 1807$\pm^{ 15 }_{ 15 }$ & $1.00$ & 28.3241 & $ -0.15\pm^{ 0.26 }_{ 0.23 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.45\\ 
1es1553 & $0.37868$ (\#9)  & 119.25(98) & 1809416 & 21 & 1817188 & 12 & 1834$\pm^{ 17 }_{ 17 }$ & $1.00$ & 29.7795 & $ 0.00\pm^{ 0.09 }_{ 0.80 }$ & $ 13.08\pm^{ 1.43 }_{ nan }$ & -0.04\\ 
1es1553 & $0.39497$ (\#10)  & 90.13(98) & 1751580 & 21 & 1813451 & 12 & 1810$\pm^{ 18 }_{ 18 }$ & $1.00$ & 30.1314 & $ 0.02\pm^{ 0.38 }_{ 0.24 }$ & $ 13.80\pm^{ 1.32 }_{ nan }$ & 0.02\\ 
3c249 & $0.24676$ (\#11)  & 78.14(93) & 2639 & 31 & 2524 & 34 & 282$\pm^{ 141 }_{ 104 }$ & $1.00$ & 26.9300 & $ -1.24\pm^{ 1.07E+12 }_{ 28.76 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
3c249 & $0.30788$ (\#12)  & 81.25(88) & 2639 & 20 & 2535 & 85 & 697$\pm^{ 234 }_{ 175 }$ & $1.00$ & 28.2502 & $ 9.81E+04\pm^{ 1.00E+20 }_{ 9.82E+04 }$ & $ 16.21\pm^{ 0.25 }_{ nan }$ & 0.35\\ 
3c249 & $0.30809$ (\#13)  & 81.15(88) & 2639 & 20 & 2535 & 85 & 701$\pm^{ 236 }_{ 177 }$ & $1.00$ & 28.2547 & $ 1.45E+07\pm^{ 1.00E+20 }_{ 1.45E+07 }$ & $ 16.29\pm^{ 0.17 }_{ nan }$ & 0.47\\ 
3c249 & $0.31364$ (\#14)  & 78.36(88) & 2639 & 20 & 2538 & 62 & 758$\pm^{ 250 }_{ 193 }$ & $1.00$ & 28.3746 & $ 9.44E+12\pm^{ 1.00E+20 }_{ 9.44E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 1.72\\ 
3c273 & $0.00337$ (\#15)  & -- & -- & -- & -- & -- & -- & -- & 21.6728 & -- & -- & --\\ 
3c273 & $0.00533$ (\#16)  & -- & -- & -- & -- & -- & -- & -- & 21.7151 & -- & -- & --\\ 
3c273 & $0.00764$ (\#17)  & -- & -- & -- & -- & -- & -- & -- & 21.7650 & -- & -- & --\\ 
3c273 & $0.02947$ (\#18*)  & 61.61(38) & 995937 & 4 & nan & nan & 4600$\pm^{ 1762 }_{ 886 }$ & $0.84$ & 22.2366 & $ -0.05\pm^{ 0.26 }_{ 0.16 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.00\\ 
3c273 & $0.04898$ (\#19)  & 63.63(45) & 936604 & 4 & nan & nan & 1268$\pm^{ 345 }_{ 291 }$ & $3.02$ & 22.6580 & $ 0.14\pm^{ 0.30 }_{ 0.17 }$ & $ 14.69\pm^{ 0.47 }_{ nan }$ & 0.84\\ 
3c273 & $0.06655$ (\#20*)  & 153.93(46) & 912160 & 5 & nan & nan & 1021$\pm^{ 260 }_{ 212 }$ & $3.36$ & 23.0375 & $ -0.60\pm^{ 0.18 }_{ 0.17 }$ & $ nan\pm^{ nan }_{ nan }$ & 10.40\\ 
3c273 & $0.09018$ (\#21*)  & 100.60(47) & 996642 & 4 & nan & nan & 931$\pm^{ 250 }_{ 186 }$ & $3.57$ & 23.5479 & $ 2.95\pm^{ 0.87 }_{ 0.66 }$ & $ 15.73\pm^{ 0.05 }_{ 0.06 }$ & 78.29\\ 
3c273 & $0.12007$ (\#22)  & 53.39(62) & 1024121 & 4 & 1027398 & 3 & 1102$\pm^{ 252 }_{ 235 }$ & $3.32$ & 24.1935 & $ 0.23\pm^{ 0.14 }_{ 0.18 }$ & $ 14.90\pm^{ 0.19 }_{ 0.59 }$ & 2.79\\ 
3c273 & $0.14660$ (\#23)  & 91.01(79) & 921050 & 4 & 1030884 & 3 & 2069$\pm^{ 402 }_{ 386 }$ & $2.37$ & 24.7666 & $ 0.81\pm^{ 0.31 }_{ 0.24 }$ & $ 15.38\pm^{ 0.10 }_{ 0.13 }$ & 17.90\\ 
3c273 & $0.15784$ (\#24)  & 115.64(86) & 931929 & 3 & 1033805 & 3 & 1143$\pm^{ 230 }_{ 202 }$ & $3.21$ & 25.0093 & $ 0.17\pm^{ 0.12 }_{ 0.18 }$ & $ 14.77\pm^{ 0.22 }_{ nan }$ & 1.10\\ 
h1821 & $0.02438$ (\#25)  & -- & -- & -- & -- & -- & -- & -- & 22.1266 & -- & -- & --\\ 
h1821 & $0.10817$ (\#26)  & 95.28(70) & 31345 & 52 & 42458 & 43 & 1133$\pm^{ 91 }_{ 88 }$ & $1.00$ & 23.9365 & $ 1.53\pm^{ 793.68 }_{ 2.95 }$ & $ 15.57\pm^{ 0.53 }_{ nan }$ & 0.11\\ 
h1821 & $0.12133$ (\#27)  & 100.65(84) & 29451 & 50 & 43368 & 41 & 1293$\pm^{ 89 }_{ 87 }$ & $1.00$ & 24.2207 & $ 8.45\pm^{ 2.57E+03 }_{ 8.13 }$ & $ 15.90\pm^{ 0.27 }_{ 0.88 }$ & 1.69\\ 
h1821 & $0.12147$ (\#28)  & 100.41(84) & 29451 & 50 & 43368 & 41 & 1292$\pm^{ 89 }_{ 85 }$ & $1.00$ & 24.2238 & $ 10.15\pm^{ 2.65E+04 }_{ 9.34 }$ & $ 15.88\pm^{ 0.29 }_{ 0.50 }$ & 1.90\\ 
h1821 & $0.16992$ (\#29)  & 141.11(98) & 32964 & 48 & 42688 & 43 & 1380$\pm^{ 94 }_{ 90 }$ & $1.00$ & 25.2703 & $ -1.12\pm^{ 1.44 }_{ 0.78 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.88\\ 
h1821 & $0.17043$ (\#30)  & 142.88(98) & 32977 & 48 & 42408 & 42 & 1382$\pm^{ 93 }_{ 90 }$ & $1.00$ & 25.2813 & $ -1.34\pm^{ 1.11 }_{ 0.64 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.58\\ 
h1821 & $0.21326$ (\#31)  & 109.00(98) & 31699 & 49 & 41854 & 43 & 1642$\pm^{ 109 }_{ 108 }$ & $1.00$ & 26.2064 & $ 707.25\pm^{ 3.46E+07 }_{ 694.75 }$ & $ 16.11\pm^{ 0.18 }_{ 0.19 }$ & 2.96\\ 
h1821 & $0.22497$ (\#32)  & 122.07(98) & 32383 & 49 & 43022 & 44 & 1546$\pm^{ 108 }_{ 106 }$ & $1.00$ & 26.4594 & $ -0.26\pm^{ 3.67 }_{ 1.19 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
h1821 & $0.22522$ (\#33)  & 122.01(98) & 32383 & 49 & 43022 & 44 & 1543$\pm^{ 109 }_{ 106 }$ & $1.00$ & 26.4648 & $ -0.46\pm^{ 2.70 }_{ 1.05 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.10\\ 
h1821 & $0.22639$ (\#34)  & 119.71(98) & 32358 & 49 & 43044 & 44 & 1535$\pm^{ 108 }_{ 104 }$ & $1.00$ & 26.4900 & $ -1.12\pm^{ 1.36 }_{ 0.72 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.95\\ 
h1821 & $0.24531$ (\#35)  & 119.80(98) & 31065 & 49 & 44448 & 47 & 1591$\pm^{ 120 }_{ 113 }$ & $1.00$ & 26.8987 & $ 0.44\pm^{ 17.76 }_{ 1.60 }$ & $ 15.15\pm^{ 0.78 }_{ nan }$ & 0.06\\ 
h1821 & $0.26657$ (\#36)  & 111.36(98) & 30604 & 55 & 44448 & 47 & 1501$\pm^{ 135 }_{ 123 }$ & $1.00$ & 27.3579 & $ 707.89\pm^{ 2.35E+07 }_{ 715.63 }$ & $ 16.08\pm^{ 0.21 }_{ nan }$ & 3.28\\ 
h1821 & $0.28800$ (\#37)  & 134.30(98) & 30054 & 55 & 39392 & 45 & 1661$\pm^{ 136 }_{ 133 }$ & $1.00$ & 27.8208 & $ 22.47\pm^{ 2.85E+05 }_{ 22.44 }$ & $ 15.96\pm^{ 0.25 }_{ 1.97 }$ & 1.58\\ 
h1821 & $0.29658$ (\#38)  & 134.83(98) & 31075 & 56 & 39131 & 45 & 1569$\pm^{ 132 }_{ 127 }$ & $1.00$ & 28.0061 & $ -2.37\pm^{ 0.69 }_{ 0.52 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.80\\ 
h1821 & $0.29680$ (\#39)  & 135.23(98) & 31075 & 56 & 39131 & 45 & 1574$\pm^{ 131 }_{ 127 }$ & $1.00$ & 28.0109 & $ -2.21\pm^{ 0.66 }_{ 0.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.28\\ 
h2356 & $0.11461$ (\#40)  & 85.19(77) & 491451 & 7 & 516214 & 6 & 1312$\pm^{ 17 }_{ 17 }$ & $1.00$ & 24.0756 & $ 0.55\pm^{ 0.70 }_{ 0.51 }$ & $ 15.24\pm^{ 0.28 }_{ 1.07 }$ & 1.54\\ 
h2356 & $0.16512$ (\#41)  & 111.39(97) & 497056 & 6 & 504552 & 6 & 1325$\pm^{ 18 }_{ 18 }$ & $1.00$ & 25.1666 & $ 0.04\pm^{ 0.66 }_{ 0.29 }$ & $ 14.13\pm^{ 1.20 }_{ nan }$ & 0.06\\ 
he0056 & $0.16392$ (\#42)  & 96.42(92) & 162630 & 15 & 161955 & 14 & 479$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.1407 & $ 0.03\pm^{ 1.70 }_{ 0.98 }$ & $ 14.08\pm^{ 1.54 }_{ nan }$ & -0.00\\ 
he0056 & $0.16492$ (\#43)  & 99.30(92) & 162629 & 15 & 161955 & 14 & 478$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.1623 & $ -0.18\pm^{ 1.66 }_{ 0.79 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
he0226 & $0.01746$ (\#44)  & 23.70(19) & 31712 & 30 & nan & nan & 123$\pm^{ 40 }_{ 35 }$ & $1.00$ & 21.9771 & $ -2.31\pm^{ 5.19 }_{ 1.35 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.85\\ 
he0226 & $0.02679$ (\#45)  & 39.57(27) & 31712 & 41 & nan & nan & 114$\pm^{ 31 }_{ 27 }$ & $1.00$ & 22.1787 & $ -3.11\pm^{ 2.38E+04 }_{ 1.79 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.51\\ 
he0226 & $0.04121$ (\#46)  & 45.84(33) & 31712 & 36 & nan & nan & 158$\pm^{ 38 }_{ 27 }$ & $1.00$ & 22.4901 & $ 168.50\pm^{ 1.00E+20 }_{ 198.50 }$ & $ 16.09\pm^{ 0.32 }_{ nan }$ & 0.70\\ 
he0226 & $0.04535$ (\#47)  & 43.77(36) & 31712 & 36 & nan & nan & 177$\pm^{ 31 }_{ 29 }$ & $1.00$ & 22.5796 & $ 1.29E+09\pm^{ 1.00E+20 }_{ 1.29E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 3.25\\ 
he0226 & $0.04609$ (\#48)  & 44.36(37) & 31712 & 35 & nan & nan & 176$\pm^{ 42 }_{ 29 }$ & $1.00$ & 22.5955 & $ 2.47E+09\pm^{ 1.00E+20 }_{ 2.47E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 3.70\\ 
he0226 & $0.06015$ (\#49)  & 53.36(41) & 31712 & 44 & nan & nan & 149$\pm^{ 30 }_{ 27 }$ & $1.00$ & 22.8992 & $ -2.25\pm^{ 244.16 }_{ 1.55 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.40\\ 
he0226 & $0.06083$ (\#50)  & 51.97(41) & 31712 & 45 & nan & nan & 141$\pm^{ 29 }_{ 26 }$ & $1.00$ & 22.9139 & $ -3.28\pm^{ 2.88 }_{ 1.36 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.36\\ 
he0226 & $0.07023$ (\#51)  & 37.36(40) & 31713 & 38 & nan & nan & 187$\pm^{ 31 }_{ 30 }$ & $1.00$ & 23.1170 & $ 32.55\pm^{ 1.00E+20 }_{ 62.55 }$ & $ 15.97\pm^{ 0.44 }_{ nan }$ & 0.11\\ 
he0226 & $0.08375$ (\#52)  & 44.35(43) & 31713 & 37 & nan & nan & 188$\pm^{ 31 }_{ 29 }$ & $1.00$ & 23.4090 & $ -2.59\pm^{ 301.77 }_{ 1.31 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.56\\ 
he0226 & $0.08901$ (\#53)  & 43.41(45) & 31713 & 43 & nan & nan & 177$\pm^{ 31 }_{ 27 }$ & $1.00$ & 23.5226 & $ 8.73\pm^{ 1.02E+17 }_{ 38.73 }$ & $ 15.87\pm^{ 0.59 }_{ nan }$ & 0.17\\ 
he0226 & $0.08938$ (\#54)  & 43.45(45) & 31713 & 44 & nan & nan & 177$\pm^{ 28 }_{ 26 }$ & $1.00$ & 23.5306 & $ 1.19E+03\pm^{ 1.00E+20 }_{ 1.22E+03 }$ & $ 16.12\pm^{ 0.34 }_{ nan }$ & 0.44\\ 
he0226 & $0.08950$ (\#55)  & 43.43(45) & 31713 & 44 & nan & nan & 177$\pm^{ 30 }_{ 25 }$ & $1.00$ & 23.5332 & $ 630.24\pm^{ 1.00E+20 }_{ 660.24 }$ & $ 16.11\pm^{ 0.30 }_{ nan }$ & 0.45\\ 
he0226 & $0.09220$ (\#56)  & 50.37(48) & 31713 & 46 & 31705 & 38 & 158$\pm^{ 28 }_{ 27 }$ & $1.00$ & 23.5915 & $ 0.55\pm^{ 3.02E+14 }_{ 30.55 }$ & $ 15.24\pm^{ 1.18 }_{ nan }$ & 0.00\\ 
he0226 & $0.10668$ (\#57)  & 72.04(63) & 31713 & 37 & 31705 & 20 & 193$\pm^{ 37 }_{ 27 }$ & $1.00$ & 23.9043 & $ 6.36E+10\pm^{ 1.00E+20 }_{ 6.36E+10 }$ & $ 16.36\pm^{ 0.10 }_{ inf }$ & 2.49\\ 
he0226 & $0.11514$ (\#58)  & 76.88(72) & 31713 & 32 & 31705 & 20 & 222$\pm^{ 39 }_{ 30 }$ & $1.00$ & 24.0870 & $ 1.55E+06\pm^{ 1.00E+20 }_{ 1.55E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 2.99\\ 
he0226 & $0.11680$ (\#59)  & 80.69(74) & 31713 & 30 & 31705 & 22 & 229$\pm^{ 34 }_{ 28 }$ & $1.00$ & 24.1229 & $ 119.13\pm^{ 1.00E+20 }_{ 149.13 }$ & $ 16.07\pm^{ 0.34 }_{ nan }$ & 0.56\\ 
he0226 & $0.11733$ (\#60)  & 85.55(74) & 31713 & 29 & 31705 & 23 & 230$\pm^{ 32 }_{ 28 }$ & $1.00$ & 24.1343 & $ 19.10\pm^{ 1.00E+20 }_{ 49.10 }$ & $ 15.93\pm^{ 0.48 }_{ nan }$ & 0.27\\ 
he0226 & $0.12589$ (\#61)  & 80.14(78) & 31713 & 27 & 31705 & 22 & 242$\pm^{ 34 }_{ 31 }$ & $1.00$ & 24.3192 & $ -1.16\pm^{ 58.93 }_{ 1.64 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.16\\ 
he0226 & $0.13832$ (\#62)  & 83.89(87) & 31710 & 20 & 31705 & 24 & 263$\pm^{ 36 }_{ 33 }$ & $1.00$ & 24.5877 & $ -1.75\pm^{ 3.60 }_{ 1.11 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.65\\ 
he0226 & $0.15175$ (\#63)  & 89.30(91) & 31708 & 21 & 31705 & 27 & 251$\pm^{ 34 }_{ 31 }$ & $1.00$ & 24.8778 & $ 0.23\pm^{ 1.12E+04 }_{ 2.27 }$ & $ 14.89\pm^{ 1.28 }_{ nan }$ & 0.00\\ 
he0226 & $0.15549$ (\#64)  & 93.36(91) & 31708 & 24 & 31705 & 27 & 240$\pm^{ 34 }_{ 31 }$ & $1.00$ & 24.9586 & $ 3.72\pm^{ 5.71E+07 }_{ 33.72 }$ & $ 15.77\pm^{ 0.56 }_{ nan }$ & 0.18\\ 
he0226 & $0.16237$ (\#65)  & 100.56(90) & 31707 & 25 & 31705 & 26 & 223$\pm^{ 34 }_{ 30 }$ & $1.00$ & 25.1072 & $ 5.77\pm^{ 3.14E+08 }_{ 35.77 }$ & $ 15.85\pm^{ 0.50 }_{ nan }$ & 0.28\\ 
he0226 & $0.16339$ (\#66)  & 99.03(90) & 31706 & 25 & 31705 & 25 & 228$\pm^{ 34 }_{ 29 }$ & $1.00$ & 25.1292 & $ 612.65\pm^{ 1.00E+20 }_{ 642.65 }$ & $ 16.11\pm^{ 0.30 }_{ nan }$ & 1.02\\ 
he0226 & $0.16971$ (\#67)  & 101.88(94) & 31706 & 22 & 31705 & 30 & 234$\pm^{ 33 }_{ 30 }$ & $1.00$ & 25.2657 & $ -1.03\pm^{ 61.71 }_{ 1.53 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.13\\ 
he0226 & $0.18619$ (\#68)  & 124.06(95) & 31706 & 22 & 31705 & 21 & 245$\pm^{ 33 }_{ 30 }$ & $1.00$ & 25.6217 & $ -1.65\pm^{ 3.25 }_{ 1.07 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.65\\ 
he0226 & $0.18811$ (\#69)  & 120.64(94) & 31706 & 21 & 31704 & 21 & 254$\pm^{ 34 }_{ 31 }$ & $1.00$ & 25.6632 & $ -1.84\pm^{ 3.24 }_{ 1.22 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.71\\ 
he0226 & $0.18891$ (\#70)  & 118.10(94) & 31706 & 22 & 31704 & 20 & 247$\pm^{ 33 }_{ 31 }$ & $1.00$ & 25.6805 & $ -2.01\pm^{ 2.34 }_{ 1.01 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.08\\ 
he0226 & $0.19374$ (\#71)  & 104.01(94) & 31706 & 23 & 31704 & 18 & 234$\pm^{ 33 }_{ 31 }$ & $1.00$ & 25.7848 & $ -3.59\pm^{ 1.12 }_{ 0.82 }$ & $ nan\pm^{ nan }_{ nan }$ & 5.57\\ 
he0226 & $0.19453$ (\#72)  & 106.55(94) & 31706 & 23 & 31704 & 20 & 233$\pm^{ 33 }_{ 31 }$ & $1.00$ & 25.8018 & $ -3.53\pm^{ 1.02 }_{ 0.75 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.18\\ 
he0226 & $0.19860$ (\#73)  & 120.02(93) & 31706 & 23 & 31704 & 24 & 266$\pm^{ 35 }_{ 32 }$ & $1.00$ & 25.8898 & $ -1.54\pm^{ 7.29 }_{ 1.22 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.39\\ 
he0226 & $0.20055$ (\#74)  & 120.40(93) & 31706 & 21 & 31704 & 25 & 280$\pm^{ 35 }_{ 33 }$ & $1.00$ & 25.9319 & $ 4.37\pm^{ 2.13E+05 }_{ 34.37 }$ & $ 15.80\pm^{ 0.46 }_{ nan }$ & 0.23\\ 
he0226 & $0.20703$ (\#75)  & 112.17(93) & 31706 & 18 & 31704 & 26 & 314$\pm^{ 36 }_{ 34 }$ & $1.00$ & 26.0718 & $ 765.45\pm^{ 4.05E+15 }_{ 795.45 }$ & $ 16.11\pm^{ 0.31 }_{ nan }$ & 1.31\\ 
he0226 & $0.22009$ (\#76)  & 120.76(87) & 31706 & 24 & 31704 & 26 & 255$\pm^{ 37 }_{ 34 }$ & $1.00$ & 26.3539 & $ -1.10\pm^{ 13.00 }_{ 1.41 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.19\\ 
he0226 & $0.22099$ (\#77)  & 119.34(87) & 31706 & 25 & 31704 & 26 & 260$\pm^{ 36 }_{ 34 }$ & $1.00$ & 26.3734 & $ 4.64\pm^{ 2.98E+05 }_{ 34.64 }$ & $ 15.81\pm^{ 0.43 }_{ nan }$ & 0.27\\ 
he0226 & $0.23009$ (\#78)  & 123.04(89) & 31707 & 24 & 31704 & 29 & 282$\pm^{ 39 }_{ 35 }$ & $1.00$ & 26.5699 & $ 0.13\pm^{ 2.30E+04 }_{ 2.35 }$ & $ 14.66\pm^{ 1.50 }_{ nan }$ & 0.00\\ 
he0226 & $0.23964$ (\#79)  & 122.92(92) & 31707 & 22 & 31704 & 37 & 314$\pm^{ 41 }_{ 38 }$ & $1.00$ & 26.7762 & $ 1.90E+03\pm^{ 2.14E+13 }_{ 1.93E+03 }$ & $ 16.15\pm^{ 0.23 }_{ nan }$ & 1.38\\ 
he0226 & $0.24522$ (\#80)  & 115.07(90) & 31708 & 23 & 31704 & 33 & 293$\pm^{ 42 }_{ 39 }$ & $1.00$ & 26.8968 & $ -0.17\pm^{ 1.60E+03 }_{ 2.00 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
he0226 & $0.25099$ (\#81)  & 119.85(90) & 31708 & 28 & 31704 & 34 & 270$\pm^{ 40 }_{ 37 }$ & $1.00$ & 27.0214 & $ -1.36\pm^{ 5.58 }_{ 1.41 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.34\\ 
he0226 & $0.27155$ (\#82)  & 120.66(94) & 31709 & 34 & 31704 & 39 & 262$\pm^{ 40 }_{ 37 }$ & $1.00$ & 27.4655 & $ 888.46\pm^{ 5.79E+09 }_{ 918.46 }$ & $ 16.11\pm^{ 0.24 }_{ nan }$ & 1.18\\ 
he0226 & $0.27956$ (\#83)  & 118.26(89) & 31709 & 31 & 31704 & 43 & 292$\pm^{ 43 }_{ 39 }$ & $1.00$ & 27.6385 & $ 1.19E+06\pm^{ 1.00E+20 }_{ 1.19E+06 }$ & $ 16.28\pm^{ 0.13 }_{ nan }$ & 2.01\\ 
he0226 & $0.28041$ (\#84)  & 121.45(88) & 31709 & 34 & 31704 & 43 & 281$\pm^{ 46 }_{ 39 }$ & $1.00$ & 27.6569 & $ 170.80\pm^{ 1.00E+20 }_{ 200.80 }$ & $ 16.10\pm^{ 0.31 }_{ nan }$ & 0.86\\ 
he0226 & $0.29134$ (\#85)  & 114.15(85) & 31709 & 29 & 31707 & 48 & 303$\pm^{ 45 }_{ 41 }$ & $1.00$ & 27.8929 & $ -0.65\pm^{ 752.83 }_{ 1.62 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
he0226 & $0.29213$ (\#86)  & 114.62(85) & 31709 & 28 & 31707 & 51 & 318$\pm^{ 47 }_{ 42 }$ & $1.00$ & 27.9100 & $ 1.25\pm^{ 4.71E+06 }_{ 31.25 }$ & $ 15.51\pm^{ 0.73 }_{ nan }$ & 0.06\\ 
he0226 & $0.30939$ (\#87)  & 100.48(87) & 31709 & 28 & 31713 & 53 & 363$\pm^{ 48 }_{ 46 }$ & $1.00$ & 28.2828 & $ -0.03\pm^{ 4.28E+05 }_{ 2.50 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
he0226 & $0.31833$ (\#88)  & 104.18(83) & 31709 & 30 & 31716 & 69 & 375$\pm^{ 58 }_{ 51 }$ & $1.00$ & 28.4759 & $ 1.78\pm^{ 2.86E+11 }_{ 31.78 }$ & $ 15.62\pm^{ 0.74 }_{ nan }$ & 0.06\\ 
he0226 & $0.33965$ (\#89)  & 125.18(89) & 31713 & 43 & 31717 & 52 & 336$\pm^{ 56 }_{ 52 }$ & $1.00$ & 28.9364 & $ 5.62E+04\pm^{ 1.00E+20 }_{ 5.62E+04 }$ & $ 16.21\pm^{ 0.25 }_{ nan }$ & 2.50\\ 
he0226 & $0.34036$ (\#90)  & 130.69(90) & 31713 & 45 & 31717 & 51 & 335$\pm^{ 56 }_{ 52 }$ & $1.00$ & 28.9518 & $ 1.66E+03\pm^{ 1.00E+20 }_{ 1.69E+03 }$ & $ 16.13\pm^{ 0.33 }_{ nan }$ & 1.44\\ 
he0226 & $0.35493$ (\#91)  & 120.67(92) & 31716 & 48 & 31717 & 58 & 281$\pm^{ 58 }_{ 52 }$ & $1.00$ & 29.2665 & $ -2.95\pm^{ 1.31 }_{ 0.76 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.03\\ 
he0226 & $0.35528$ (\#92)  & 120.85(92) & 31716 & 48 & 31717 & 58 & 282$\pm^{ 58 }_{ 53 }$ & $1.00$ & 29.2740 & $ -3.10\pm^{ 1.52 }_{ 0.87 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.77\\ 
he0226 & $0.37281$ (\#93)  & 111.76(99) & 31717 & 47 & 31717 & 48 & 352$\pm^{ 79 }_{ 56 }$ & $1.00$ & 29.6527 & $ 1.30E+06\pm^{ 1.00E+20 }_{ 1.30E+06 }$ & $ 16.24\pm^{ 0.22 }_{ nan }$ & 2.58\\ 
he0226 & $0.38420$ (\#94)  & 114.74(94) & 31717 & 46 & 31717 & 61 & 360$\pm^{ 63 }_{ 58 }$ & $1.00$ & 29.8987 & $ 0.97\pm^{ 7.80E+09 }_{ 30.97 }$ & $ 15.45\pm^{ 0.88 }_{ nan }$ & 0.03\\ 
he0226 & $0.38636$ (\#95)  & 107.14(90) & 31717 & 47 & 31717 & 64 & 355$\pm^{ 72 }_{ 57 }$ & $1.00$ & 29.9454 & $ 879.88\pm^{ 1.00E+20 }_{ 909.88 }$ & $ 16.11\pm^{ 0.30 }_{ nan }$ & 0.74\\ 
he0226 & $0.39642$ (\#96)  & 117.89(86) & 31717 & 52 & 31717 & 71 & 283$\pm^{ 60 }_{ 53 }$ & $1.00$ & 30.1627 & $ -1.85\pm^{ 10.21 }_{ 1.29 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.48\\ 
he0226 & $0.39692$ (\#97)  & 121.57(86) & 31717 & 54 & 31717 & 69 & 282$\pm^{ 62 }_{ 55 }$ & $1.00$ & 30.1735 & $ -0.90\pm^{ 1.84E+04 }_{ 2.15 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
he0226 & $0.39890$ (\#98)  & 118.58(86) & 31717 & 53 & 31717 & 70 & 289$\pm^{ 62 }_{ 55 }$ & $1.00$ & 30.2162 & $ -1.49\pm^{ 3.14E+03 }_{ 1.63 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.18\\ 
he0226 & $0.40034$ (\#99)  & 117.15(85) & 31717 & 51 & 31717 & 70 & 273$\pm^{ 59 }_{ 53 }$ & $1.00$ & 30.2473 & $ -2.89\pm^{ 1.59 }_{ 0.93 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.43\\ 
he0226 & $0.40274$ (\#100)  & 121.91(83) & 31717 & 49 & 31717 & 70 & 307$\pm^{ 63 }_{ 57 }$ & $1.00$ & 30.2992 & $ -0.82\pm^{ 4.88E+06 }_{ 2.14 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
he0226 & $0.49225$ (\#101)  & 130.27(93) & 31722 & 61 & 31717 & 60 & 423$\pm^{ 80 }_{ 73 }$ & $1.00$ & 32.2326 & $ -2.37\pm^{ 2.87 }_{ 1.13 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.03\\ 
he0226 & $0.49254$ (\#102)  & 123.54(92) & 31722 & 60 & 31717 & 59 & 434$\pm^{ 80 }_{ 74 }$ & $1.00$ & 32.2389 & $ -2.05\pm^{ 3.73 }_{ 1.06 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.77\\ 
he0226 & $0.49280$ (\#103)  & 123.59(92) & 31722 & 60 & 31717 & 59 & 435$\pm^{ 81 }_{ 74 }$ & $1.00$ & 32.2445 & $ -2.07\pm^{ 4.37 }_{ 1.19 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.70\\ 
he0226 & $0.49309$ (\#104)  & 129.01(93) & 31722 & 62 & 31717 & 59 & 423$\pm^{ 79 }_{ 73 }$ & $1.00$ & 32.2507 & $ -2.25\pm^{ 4.38 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.71\\ 
i22456 & $0.09858$ (\#105)  & 68.71(60) & 79883 & 52 & 72481 & 44 & 656$\pm^{ 39 }_{ 37 }$ & $1.00$ & 23.7293 & $ 0.29\pm^{ 30.11 }_{ 1.67 }$ & $ 15.00\pm^{ 0.98 }_{ nan }$ & 0.02\\ 
i22456 & $0.09895$ (\#106)  & 68.38(60) & 79752 & 52 & 73453 & 44 & 659$\pm^{ 38 }_{ 37 }$ & $1.00$ & 23.7373 & $ 0.26\pm^{ 27.35 }_{ 1.70 }$ & $ 14.95\pm^{ 1.00 }_{ nan }$ & 0.01\\ 
i22456 & $0.09931$ (\#107)  & 68.39(60) & 79752 & 52 & 73453 & 44 & 657$\pm^{ 37 }_{ 37 }$ & $1.00$ & 23.7451 & $ -0.10\pm^{ 14.31 }_{ 1.52 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
i22456 & $0.09959$ (\#108)  & 74.98(61) & 79883 & 51 & 73453 & 44 & 669$\pm^{ 37 }_{ 37 }$ & $1.00$ & 23.7511 & $ -0.12\pm^{ 7.55 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
i22456 & $0.09989$ (\#109)  & 68.68(61) & 79752 & 51 & 74286 & 44 & 651$\pm^{ 38 }_{ 37 }$ & $1.00$ & 23.7576 & $ -0.71\pm^{ 3.30 }_{ 1.08 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.18\\ 
i22456 & $0.10034$ (\#110)  & 69.76(62) & 79883 & 51 & 74286 & 44 & 656$\pm^{ 37 }_{ 37 }$ & $1.00$ & 23.7673 & $ -0.82\pm^{ 2.55 }_{ 1.00 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.30\\ 
i22456 & $0.10101$ (\#111)  & 73.32(62) & 79121 & 51 & 75007 & 45 & 657$\pm^{ 38 }_{ 37 }$ & $1.00$ & 23.7818 & $ -0.83\pm^{ 2.69 }_{ 1.11 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.26\\ 
i22456 & $0.10146$ (\#112)  & 75.43(63) & 77663 & 55 & 75007 & 45 & 665$\pm^{ 36 }_{ 42 }$ & $1.00$ & 23.7915 & $ -0.07\pm^{ 4.28 }_{ 1.75 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
mr2251 & $0.01070$ (\#113)  & -- & -- & -- & -- & -- & -- & -- & 21.8311 & -- & -- & --\\ 
mrk421 & $0.01009$ (\#114)  & -- & -- & -- & -- & -- & -- & -- & 21.8179 & -- & -- & --\\ 
mrk876 & $0.00311$ (\#115)  & -- & -- & -- & -- & -- & -- & -- & 21.6672 & -- & -- & --\\ 
mrk876 & $0.06248$ (\#116)  & 41.89(45) & 2651 & 13 & nan & nan & 495$\pm^{ 152 }_{ 120 }$ & $1.00$ & 22.9496 & $ 1.62E+13\pm^{ 1.00E+20 }_{ 1.62E+13 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 0.83\\ 
mrk876 & $0.08579$ (\#117)  & 36.44(46) & 2765 & 11 & nan & nan & 357$\pm^{ 118 }_{ 97 }$ & $1.00$ & 23.4531 & $ 2.06E+16\pm^{ 1.00E+20 }_{ 2.06E+16 }$ & $ 16.46\pm^{ 0.00 }_{ inf }$ & 1.63\\ 
mrk876 & $0.11488$ (\#118)  & 73.35(75) & 2743 & 19 & 2633 & 28 & 529$\pm^{ 144 }_{ 121 }$ & $1.00$ & 24.0814 & $ 0.21\pm^{ 1.00E+20 }_{ 30.21 }$ & $ 14.86\pm^{ 1.60 }_{ nan }$ & 0.00\\ 
mrk876 & $0.11517$ (\#119)  & 75.24(76) & 2746 & 18 & 2633 & 25 & 567$\pm^{ 149 }_{ 126 }$ & $1.00$ & 24.0877 & $ 4.09\pm^{ 1.00E+20 }_{ 34.09 }$ & $ 15.79\pm^{ 0.62 }_{ nan }$ & 0.05\\ 
mrk876 & $0.11588$ (\#120)  & 76.60(76) & 2743 & 17 & 2636 & 25 & 603$\pm^{ 153 }_{ 130 }$ & $1.00$ & 24.1030 & $ 44.70\pm^{ 1.00E+20 }_{ 74.70 }$ & $ 16.00\pm^{ 0.46 }_{ nan }$ & 0.14\\ 
ngc7469 & $0.00962$ (\#121)  & -- & -- & -- & -- & -- & -- & -- & 21.8078 & -- & -- & --\\ 
ngc7469 & $0.00994$ (\#122)  & -- & -- & -- & -- & -- & -- & -- & 21.8147 & -- & -- & --\\ 
ngc7469 & $0.01153$ (\#123)  & -- & -- & -- & -- & -- & -- & -- & 21.8490 & -- & -- & --\\ 
p1103 & $0.13556$ (\#124)  & 87.53(87) & 15673 & 4 & 15681 & 4 & 3494$\pm^{ 169 }_{ 164 }$ & $1.00$ & 24.5281 & $ -0.67\pm^{ 1.25 }_{ 0.75 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.47\\ 
p1103 & $0.13937$ (\#125)  & 91.46(88) & 15673 & 4 & 15681 & 4 & 3603$\pm^{ 170 }_{ 165 }$ & $1.00$ & 24.6104 & $ 1.92\pm^{ 16.76 }_{ 2.07 }$ & $ 15.64\pm^{ 0.31 }_{ nan }$ & 0.98\\ 
p1103 & $0.14099$ (\#126)  & 96.68(88) & 15673 & 4 & 15681 & 4 & 3562$\pm^{ 166 }_{ 161 }$ & $1.00$ & 24.6454 & $ -0.49\pm^{ 1.42 }_{ 0.75 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.24\\ 
p1103 & $0.14126$ (\#127)  & 97.21(89) & 15673 & 4 & 15681 & 4 & 3537$\pm^{ 166 }_{ 160 }$ & $1.00$ & 24.6512 & $ -0.76\pm^{ 1.17 }_{ 0.73 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.62\\ 
p1103 & $0.17277$ (\#128)  & 83.97(94) & 15671 & 3 & 15681 & 5 & 3424$\pm^{ 156 }_{ 152 }$ & $1.00$ & 25.3318 & $ -0.78\pm^{ 1.21 }_{ 0.77 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.61\\ 
pg0003 & $0.16521$ (\#129)  & 110.21(91) & 13034 & 29 & 12941 & 15 & 284$\pm^{ 60 }_{ 53 }$ & $1.00$ & 25.1685 & $ -1.83\pm^{ 9.33 }_{ 1.39 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.44\\ 
pg0003 & $0.20907$ (\#130)  & 119.20(94) & 13033 & 23 & 12875 & 32 & 302$\pm^{ 63 }_{ 55 }$ & $1.00$ & 26.1159 & $ -1.58\pm^{ 413.20 }_{ 1.88 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.18\\ 
pg0003 & $0.29021$ (\#131)  & 124.39(88) & 13035 & 43 & 12849 & 33 & 347$\pm^{ 85 }_{ 74 }$ & $1.00$ & 27.8685 & $ -0.71\pm^{ 4.65E+04 }_{ 2.41 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
pg0003 & $0.30551$ (\#132*)  & 138.04(89) & 13035 & 53 & 12885 & 39 & 291$\pm^{ 75 }_{ 64 }$ & $1.00$ & 28.1990 & $ -3.06\pm^{ 2.40 }_{ 1.08 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.53\\ 
pg0003 & $0.30569$ (\#133*)  & 137.89(89) & 13035 & 53 & 12885 & 39 & 292$\pm^{ 74 }_{ 64 }$ & $1.00$ & 28.2029 & $ -3.27\pm^{ 2.34 }_{ 1.18 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.68\\ 
pg0003 & $0.34757$ (\#134)  & 105.38(90) & 13039 & 75 & 12932 & 59 & 231$\pm^{ 86 }_{ 68 }$ & $1.00$ & 29.1075 & $ -4.17\pm^{ 1.46 }_{ 0.98 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.27\\ 
pg0003 & $0.34788$ (\#135)  & 105.00(90) & 13039 & 75 & 12932 & 59 & 229$\pm^{ 84 }_{ 68 }$ & $1.00$ & 29.1142 & $ -4.49\pm^{ 1.50 }_{ 1.07 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.76\\ 
pg0003 & $0.36452$ (\#136)  & 126.87(94) & 13041 & 78 & 12932 & 54 & 361$\pm^{ 143 }_{ 107 }$ & $1.00$ & 29.4736 & $ 4.88E+06\pm^{ 1.00E+20 }_{ 4.88E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 2.32\\ 
pg0003 & $0.36508$ (\#137)  & 128.24(95) & 13041 & 80 & 12932 & 54 & 358$\pm^{ 99 }_{ 86 }$ & $1.00$ & 29.4857 & $ 4.18E+12\pm^{ 1.00E+20 }_{ 4.18E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 3.18\\ 
pg0003 & $0.36572$ (\#138)  & 128.74(97) & 13041 & 80 & 12932 & 54 & 356$\pm^{ 99 }_{ 85 }$ & $1.00$ & 29.4996 & $ 2.12E+16\pm^{ 1.00E+20 }_{ 2.12E+16 }$ & $ 16.46\pm^{ 0.00 }_{ inf }$ & 3.55\\ 
pg0003 & $0.36621$ (\#139)  & 130.11(96) & 13041 & 80 & 12932 & 53 & 349$\pm^{ 116 }_{ 93 }$ & $1.00$ & 29.5101 & $ 2.61E+12\pm^{ 1.00E+20 }_{ 2.61E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 3.05\\ 
pg0003 & $0.37029$ (\#140)  & 139.10(98) & 13041 & 87 & 12932 & 56 & 313$\pm^{ 91 }_{ 78 }$ & $1.00$ & 29.5983 & $ 2.06E+03\pm^{ 1.00E+20 }_{ 2.09E+03 }$ & $ 16.15\pm^{ 0.31 }_{ nan }$ & 0.44\\ 
pg0003 & $0.38608$ (\#141)  & 106.39(88) & 13041 & 125 & 12920 & 51 & 115$\pm^{ 65 }_{ 46 }$ & $1.00$ & 29.9393 & $ -4.99\pm^{ 0.89 }_{ 0.78 }$ & $ nan\pm^{ nan }_{ nan }$ & 13.26\\ 
pg0003 & $0.38639$ (\#142)  & 114.18(87) & 13041 & 119 & 12920 & 57 & 151$\pm^{ 74 }_{ 56 }$ & $1.00$ & 29.9460 & $ -5.40\pm^{ 1.28 }_{ 1.06 }$ & $ nan\pm^{ nan }_{ nan }$ & 8.98\\ 
pg0003 & $0.40138$ (\#143)  & 124.56(86) & 13041 & 79 & 12886 & 53 & 432$\pm^{ 127 }_{ 117 }$ & $1.00$ & 30.2698 & $ 2.71E+12\pm^{ 1.00E+20 }_{ 2.71E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 2.95\\ 
pg0003 & $0.42192$ (\#144)  & 120.23(94) & 13041 & 89 & 12843 & 41 & 378$\pm^{ 116 }_{ 97 }$ & $1.00$ & 30.7135 & $ -2.22\pm^{ 2.71E+06 }_{ 1.75 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.26\\ 
pg0157 & $0.14621$ (\#145)  & 89.37(90) & 3707 & 30 & 3516 & 41 & 333$\pm^{ 101 }_{ 84 }$ & $1.00$ & 24.7581 & $ 1.21E+03\pm^{ 1.00E+20 }_{ 1.24E+03 }$ & $ 16.12\pm^{ 0.34 }_{ nan }$ & 0.32\\ 
pg0804 & $0.00382$ (\#146)  & -- & -- & -- & -- & -- & -- & -- & 21.6825 & -- & -- & --\\ 
pg0804 & $0.01851$ (\#147)  & 16.80(23) & 29128 & 12 & nan & nan & 945$\pm^{ 97 }_{ 92 }$ & $1.00$ & 21.9998 & $ -1.81\pm^{ 1.53 }_{ 0.87 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.89\\ 
pg0804 & $0.10216$ (\#148)  & 79.20(62) & 28053 & 6 & 28091 & 3 & 1727$\pm^{ 87 }_{ 84 }$ & $1.00$ & 23.8067 & $ -0.51\pm^{ 2.91 }_{ 1.02 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.11\\ 
pg0804 & $0.10230$ (\#149)  & 79.21(62) & 28053 & 6 & 28091 & 3 & 1728$\pm^{ 87 }_{ 84 }$ & $1.00$ & 23.8097 & $ -0.47\pm^{ 2.82 }_{ 1.16 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.10\\ 
pg0832 & $0.10772$ (\#150)  & 80.67(64) & 20655 & 63 & 20637 & 75 & 76$\pm^{ 24 }_{ 21 }$ & $1.00$ & 23.9268 & $ -3.20\pm^{ 2.96 }_{ 1.25 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.33\\ 
pg0832 & $0.13230$ (\#151)  & 108.67(84) & 20655 & 92 & 20637 & 151 & 61$\pm^{ 24 }_{ 19 }$ & $1.00$ & 24.4577 & $ -0.85\pm^{ 1.00E+20 }_{ 29.15 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pg0832 & $0.15276$ (\#152)  & 120.88(91) & 20654 & 102 & 20637 & 191 & 47$\pm^{ 21 }_{ 16 }$ & $1.00$ & 24.8996 & $ 2.53E+05\pm^{ 1.00E+20 }_{ 2.53E+05 }$ & $ 16.25\pm^{ 0.16 }_{ nan }$ & 0.35\\ 
pg0832 & $0.23308$ (\#153)  & 129.97(95) & 20655 & 89 & 20637 & 102 & 82$\pm^{ 28 }_{ 23 }$ & $1.00$ & 26.6345 & $ -3.17\pm^{ 1.00E+04 }_{ 1.79 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.58\\ 
pg0832 & $0.32567$ (\#154)  & 75.57(61) & 20656 & 168 & 20645 & 75 & 67$\pm^{ 36 }_{ 26 }$ & $1.00$ & 28.6345 & $ -1.01\pm^{ 1.00E+20 }_{ 28.99 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
pg0953 & $0.01560$ (\#155)  & 28.56(26) & 12792 & 15 & nan & nan & 420$\pm^{ 81 }_{ 73 }$ & $1.00$ & 21.9370 & $ -2.59\pm^{ 2.65 }_{ 1.33 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.29\\ 
pg0953 & $0.05891$ (\#156)  & 62.59(44) & 12792 & 17 & nan & nan & 452$\pm^{ 68 }_{ 62 }$ & $1.00$ & 22.8725 & $ -1.64\pm^{ 201.57 }_{ 1.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.26\\ 
pg0953 & $0.06807$ (\#157)  & 48.31(41) & 12792 & 16 & nan & nan & 546$\pm^{ 89 }_{ 74 }$ & $1.00$ & 23.0703 & $ 3.07E+12\pm^{ 1.00E+20 }_{ 3.07E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 3.12\\ 
pg0953 & $0.11827$ (\#158)  & 75.73(75) & 12792 & 18 & 12309 & 9 & 500$\pm^{ 67 }_{ 61 }$ & $1.00$ & 24.1546 & $ -0.43\pm^{ 90.04 }_{ 1.66 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
pg0953 & $0.14236$ (\#159)  & 105.46(88) & 12786 & 21 & 12309 & 8 & 548$\pm^{ 75 }_{ 68 }$ & $1.00$ & 24.6750 & $ -3.03\pm^{ 0.91 }_{ 0.63 }$ & $ nan\pm^{ nan }_{ nan }$ & 5.66\\ 
pg0953 & $0.14263$ (\#160)  & 109.34(89) & 12785 & 22 & 12309 & 8 & 547$\pm^{ 74 }_{ 69 }$ & $1.00$ & 24.6808 & $ -2.96\pm^{ 0.83 }_{ 0.58 }$ & $ nan\pm^{ nan }_{ nan }$ & 5.97\\ 
pg0953 & $0.14307$ (\#161)  & 107.64(88) & 12785 & 22 & 12309 & 8 & 540$\pm^{ 74 }_{ 68 }$ & $1.00$ & 24.6903 & $ -3.05\pm^{ 0.81 }_{ 0.57 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.36\\ 
pg0953 & $0.22967$ (\#162)  & 126.93(87) & 12777 & 8 & 12309 & 16 & 692$\pm^{ 88 }_{ 81 }$ & $1.00$ & 26.5609 & $ -2.57\pm^{ 1.33 }_{ 0.84 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.87\\ 
pg0953 & $0.23251$ (\#163)  & 116.37(87) & 12777 & 9 & 12309 & 16 & 645$\pm^{ 85 }_{ 78 }$ & $1.00$ & 26.6222 & $ -2.98\pm^{ 1.09 }_{ 0.74 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.37\\ 
pg0953 & $0.23351$ (\#164)  & 118.01(88) & 12777 & 9 & 12309 & 15 & 650$\pm^{ 85 }_{ 78 }$ & $1.00$ & 26.6438 & $ -2.92\pm^{ 1.42 }_{ 0.87 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.94\\ 
pg1115 & $0.12285$ (\#165)  & 111.34(78) & 17510 & 36 & 16953 & 10 & 307$\pm^{ 48 }_{ 44 }$ & $1.00$ & 24.2536 & $ 2.73E+06\pm^{ 1.00E+20 }_{ 2.73E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 3.46\\ 
pg1115 & $0.12313$ (\#166)  & 110.77(77) & 17510 & 37 & 16953 & 10 & 298$\pm^{ 64 }_{ 43 }$ & $1.00$ & 24.2596 & $ 154.01\pm^{ 1.00E+20 }_{ 184.01 }$ & $ 16.04\pm^{ 0.42 }_{ nan }$ & 1.57\\ 
pg1115 & $0.13104$ (\#167*)  & 126.82(83) & 17517 & 38 & 16953 & 13 & 303$\pm^{ 52 }_{ 47 }$ & $1.00$ & 24.4305 & $ 2.10\pm^{ 7.83E+05 }_{ 32.10 }$ & $ 15.66\pm^{ 0.57 }_{ nan }$ & 0.14\\ 
pg1115 & $0.15456$ (\#168*)  & 137.20(89) & 17538 & 26 & 16953 & 15 & 351$\pm^{ 52 }_{ 48 }$ & $1.00$ & 24.9385 & $ -1.25\pm^{ 14.84 }_{ 1.36 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.22\\ 
pg1115 & $0.15467$ (\#169*)  & 137.21(89) & 17538 & 26 & 16953 & 15 & 351$\pm^{ 53 }_{ 48 }$ & $1.00$ & 24.9409 & $ -1.19\pm^{ 13.28 }_{ 1.32 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.21\\ 
pg1116 & $0.05900$ (\#170)  & 49.53(36) & 281330 & 15 & nan & nan & 597$\pm^{ 19 }_{ 19 }$ & $1.00$ & 22.8744 & $ 3.08\pm^{ 18.52 }_{ 2.71 }$ & $ 15.74\pm^{ 0.24 }_{ 0.65 }$ & 2.02\\ 
pg1116 & $0.05927$ (\#171)  & 43.85(35) & 280940 & 15 & nan & nan & 590$\pm^{ 19 }_{ 19 }$ & $1.00$ & 22.8802 & $ 2.47\pm^{ 24.40 }_{ 2.27 }$ & $ 15.70\pm^{ 0.26 }_{ 0.85 }$ & 1.62\\ 
pg1116 & $0.11895$ (\#172)  & 95.95(79) & 285653 & 15 & 287248 & 12 & 652$\pm^{ 16 }_{ 16 }$ & $1.00$ & 24.1693 & $ -0.41\pm^{ 0.72 }_{ 0.52 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.50\\ 
pg1116 & $0.13852$ (\#173)  & 94.61(91) & 277702 & 15 & 291047 & 12 & 693$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.5920 & $ 1.53\pm^{ 2.90 }_{ 1.20 }$ & $ 15.58\pm^{ 0.23 }_{ 0.53 }$ & 2.43\\ 
pg1116 & $0.16539$ (\#174)  & 104.05(93) & 289660 & 12 & 291047 & 10 & 750$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.1724 & $ 1.15\pm^{ 2.07 }_{ 1.03 }$ & $ 15.49\pm^{ 0.26 }_{ 0.86 }$ & 1.66\\ 
pg1116 & $0.16554$ (\#175)  & 100.41(92) & 289658 & 12 & 290943 & 10 & 751$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.1757 & $ 1.29\pm^{ 2.32 }_{ 1.05 }$ & $ 15.54\pm^{ 0.24 }_{ 0.62 }$ & 2.12\\ 
pg1116 & $0.16610$ (\#176)  & 106.71(93) & 289658 & 11 & 291047 & 10 & 760$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.1878 & $ 1.79\pm^{ 3.14 }_{ 1.32 }$ & $ 15.62\pm^{ 0.21 }_{ 0.44 }$ & 3.04\\ 
pg1116 & $0.16686$ (\#177)  & 105.29(92) & 291239 & 11 & 290943 & 10 & 756$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.2042 & $ 1.73\pm^{ 3.60 }_{ 1.25 }$ & $ 15.62\pm^{ 0.21 }_{ 0.43 }$ & 3.07\\ 
pg1116 & $0.17343$ (\#178)  & 112.47(96) & 296094 & 11 & 285607 & 10 & 756$\pm^{ 18 }_{ 18 }$ & $1.00$ & 25.3461 & $ 0.82\pm^{ 1.68 }_{ 0.89 }$ & $ 15.38\pm^{ 0.32 }_{ nan }$ & 0.98\\ 
pg1211 & $0.00711$ (\#179)  & -- & -- & -- & -- & -- & -- & -- & 21.7536 & -- & -- & --\\ 
pg1211 & $0.05117$ (\#180)  & 45.23(34) & 736547 & 13 & nan & nan & 672$\pm^{ 13 }_{ 13 }$ & $1.00$ & 22.7053 & $ 201.73\pm^{ 3.78E+05 }_{ 184.38 }$ & $ 16.06\pm^{ 0.16 }_{ 0.12 }$ & 13.49\\ 
pg1211 & $0.06449$ (\#181)  & -- & -- & -- & -- & -- & -- & -- & 22.9930 & -- & -- & --\\ 
pg1211 & $0.06491$ (\#182)  & -- & -- & -- & -- & -- & -- & -- & 23.0021 & -- & -- & --\\ 
pg1216 & $0.12362$ (\#183)  & 106.86(78) & 11245 & 36 & 11258 & 15 & 185$\pm^{ 46 }_{ 40 }$ & $1.00$ & 24.2702 & $ 1.23E+12\pm^{ 1.00E+20 }_{ 1.23E+12 }$ & $ 16.41\pm^{ 0.00 }_{ inf }$ & 4.18\\ 
pg1216 & $0.12389$ (\#184)  & 105.56(77) & 11245 & 36 & 11258 & 15 & 183$\pm^{ 66 }_{ 49 }$ & $1.00$ & 24.2760 & $ 1.71E+04\pm^{ 1.00E+20 }_{ 1.72E+04 }$ & $ 16.21\pm^{ 0.26 }_{ nan }$ & 2.64\\ 
pg1216 & $0.12463$ (\#185)  & 107.31(78) & 11245 & 36 & 11258 & 15 & 187$\pm^{ 46 }_{ 40 }$ & $1.00$ & 24.2920 & $ 1.14E+07\pm^{ 1.00E+20 }_{ 1.14E+07 }$ & $ 16.29\pm^{ 0.18 }_{ nan }$ & 2.41\\ 
pg1216 & $0.12485$ (\#186)  & 106.17(77) & 11245 & 36 & 11258 & 15 & 186$\pm^{ 46 }_{ 40 }$ & $1.00$ & 24.2968 & $ 7.83E+04\pm^{ 1.00E+20 }_{ 7.83E+04 }$ & $ 16.21\pm^{ 0.25 }_{ nan }$ & 1.71\\ 
pg1216 & $0.13499$ (\#187)  & 116.72(86) & 11248 & 35 & 11258 & 16 & 192$\pm^{ 50 }_{ 43 }$ & $1.00$ & 24.5158 & $ 2.34\pm^{ 1.06E+13 }_{ 32.34 }$ & $ 15.68\pm^{ 0.69 }_{ nan }$ & 0.06\\ 
pg1216 & $0.26768$ (\#188)  & 113.01(93) & 11258 & 41 & 11258 & 73 & 223$\pm^{ 67 }_{ 53 }$ & $1.00$ & 27.3819 & $ 14.94\pm^{ 1.00E+20 }_{ 44.94 }$ & $ 15.91\pm^{ 0.55 }_{ nan }$ & 0.14\\ 
pg1216 & $0.28199$ (\#189)  & 112.68(89) & 11258 & 41 & 11258 & 68 & 237$\pm^{ 66 }_{ 56 }$ & $1.00$ & 27.6910 & $ -2.60\pm^{ 4.73 }_{ 1.22 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.87\\ 
pg1216 & $0.28237$ (\#190)  & 112.03(88) & 11258 & 41 & 11258 & 68 & 245$\pm^{ 68 }_{ 57 }$ & $1.00$ & 27.6992 & $ -2.15\pm^{ 330.94 }_{ 1.38 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.43\\ 
pg1259 & $0.00220$ (\#191)  & -- & -- & -- & -- & -- & -- & -- & 21.6475 & -- & -- & --\\ 
pg1259 & $0.00762$ (\#192)  & -- & -- & -- & -- & -- & -- & -- & 21.7646 & -- & -- & --\\ 
pg1259 & $0.02217$ (\#193)  & 31.57(30) & 11484 & 31 & nan & nan & 172$\pm^{ 52 }_{ 46 }$ & $1.00$ & 22.0789 & $ 37.76\pm^{ 1.00E+20 }_{ 67.76 }$ & $ 15.99\pm^{ 0.47 }_{ nan }$ & 0.12\\ 
pg1259 & $0.04606$ (\#194)  & 45.32(42) & 11485 & 41 & nan & nan & 178$\pm^{ 51 }_{ 39 }$ & $1.00$ & 22.5949 & $ 4.41E+09\pm^{ 1.00E+20 }_{ 4.41E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 1.04\\ 
pg1259 & $0.04650$ (\#195)  & 43.77(42) & 11485 & 37 & nan & nan & 188$\pm^{ 53 }_{ 41 }$ & $1.00$ & 22.6044 & $ 4.23E+09\pm^{ 1.00E+20 }_{ 4.23E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 1.02\\ 
pg1259 & $0.19576$ (\#196)  & 107.87(92) & 11483 & 28 & 11479 & 32 & 236$\pm^{ 54 }_{ 46 }$ & $1.00$ & 25.8284 & $ -2.09\pm^{ 25.68 }_{ 1.50 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.42\\ 
pg1259 & $0.21940$ (\#197)  & 110.09(92) & 11483 & 38 & 11479 & 41 & 267$\pm^{ 65 }_{ 56 }$ & $1.00$ & 26.3390 & $ -1.52\pm^{ 3.11E+05 }_{ 2.22 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.10\\ 
pg1259 & $0.21953$ (\#198)  & 110.10(92) & 11483 & 38 & 11479 & 41 & 267$\pm^{ 65 }_{ 56 }$ & $1.00$ & 26.3418 & $ -1.36\pm^{ 8.12E+06 }_{ 1.90 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.09\\ 
pg1259 & $0.22313$ (\#199)  & 105.90(93) & 11483 & 32 & 11479 & 49 & 275$\pm^{ 64 }_{ 56 }$ & $1.00$ & 26.4196 & $ -0.23\pm^{ 6.24E+09 }_{ 2.86 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pg1259 & $0.23284$ (\#200)  & 120.10(95) & 11483 & 44 & 11479 & 68 & 235$\pm^{ 60 }_{ 51 }$ & $1.00$ & 26.6293 & $ 6.49E+07\pm^{ 1.00E+20 }_{ 6.49E+07 }$ & $ 16.32\pm^{ 0.14 }_{ -0.14 }$ & 1.29\\ 
pg1259 & $0.23956$ (\#201)  & 123.67(95) & 11483 & 62 & 11479 & 61 & 179$\pm^{ 54 }_{ 45 }$ & $1.00$ & 26.7745 & $ 0.89\pm^{ 2.33E+14 }_{ 30.89 }$ & $ 15.41\pm^{ 1.01 }_{ nan }$ & 0.01\\ 
pg1259 & $0.25973$ (\#202)  & 111.65(93) & 11483 & 81 & 11479 & 66 & 126$\pm^{ 49 }_{ 39 }$ & $1.00$ & 27.2102 & $ 2.29E+04\pm^{ 1.00E+20 }_{ 2.29E+04 }$ & $ 16.21\pm^{ 0.26 }_{ nan }$ & 0.83\\ 
pg1259 & $0.31979$ (\#203)  & 80.12(82) & 11483 & 42 & 11480 & 55 & 296$\pm^{ 92 }_{ 70 }$ & $1.00$ & 28.5075 & $ 1.46E+05\pm^{ 1.00E+20 }_{ 1.46E+05 }$ & $ 16.22\pm^{ 0.24 }_{ nan }$ & 0.67\\ 
pg1259 & $0.32472$ (\#204)  & 90.97(82) & 11484 & 43 & 11480 & 66 & 337$\pm^{ 109 }_{ 77 }$ & $1.00$ & 28.6140 & $ 5.09E+09\pm^{ 1.00E+20 }_{ 5.09E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 2.56\\ 
pg1307 & $0.14187$ (\#205)  & 117.92(89) & 9837 & 52 & 9504 & 88 & 210$\pm^{ 60 }_{ 45 }$ & $1.00$ & 24.6644 & $ 2.26E+04\pm^{ 1.00E+20 }_{ 2.26E+04 }$ & $ 16.21\pm^{ 0.26 }_{ nan }$ & 0.58\\ 
pg1307 & $0.14214$ (\#206)  & 117.74(88) & 9837 & 52 & 9504 & 88 & 211$\pm^{ 60 }_{ 46 }$ & $1.00$ & 24.6702 & $ 5.01E+06\pm^{ 1.00E+20 }_{ 5.01E+06 }$ & $ 16.28\pm^{ 0.18 }_{ nan }$ & 0.69\\ 
pg1309 & $0.17586$ (\#207)  & 112.33(93) & 27265 & 31 & 26163 & 75 & 153$\pm^{ 28 }_{ 25 }$ & $1.00$ & 25.3986 & $ 3.69E+12\pm^{ 1.00E+20 }_{ 3.69E+12 }$ & $ 16.41\pm^{ 0.05 }_{ inf }$ & 3.00\\ 
pg1309 & $0.17745$ (\#208)  & 117.17(95) & 27265 & 32 & 26163 & 73 & 150$\pm^{ 36 }_{ 25 }$ & $1.00$ & 25.4329 & $ 2.70E+06\pm^{ 1.00E+20 }_{ 2.70E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 1.76\\ 
pg1309 & $0.17866$ (\#209)  & 121.37(94) & 27265 & 33 & 26163 & 75 & 155$\pm^{ 35 }_{ 25 }$ & $1.00$ & 25.4591 & $ 5.56E+09\pm^{ 1.00E+20 }_{ 5.56E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 2.13\\ 
pg1309 & $0.17930$ (\#210)  & 120.67(95) & 27265 & 33 & 26163 & 75 & 156$\pm^{ 33 }_{ 26 }$ & $1.00$ & 25.4729 & $ 4.80E+09\pm^{ 1.00E+20 }_{ 4.80E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 1.89\\ 
pg1309 & $0.17979$ (\#211)  & 121.42(94) & 27265 & 31 & 26163 & 75 & 157$\pm^{ 29 }_{ 25 }$ & $1.00$ & 25.4835 & $ 4.66E+07\pm^{ 1.00E+20 }_{ 4.66E+07 }$ & $ 16.31\pm^{ 0.16 }_{ nan }$ & 1.65\\ 
pg1309 & $0.18069$ (\#212)  & 121.63(94) & 27265 & 33 & 26163 & 73 & 147$\pm^{ 27 }_{ 25 }$ & $1.00$ & 25.5029 & $ 4.34E+03\pm^{ 1.00E+20 }_{ 4.37E+03 }$ & $ 16.19\pm^{ 0.27 }_{ nan }$ & 0.54\\ 
pg1309 & $0.18117$ (\#213)  & 119.61(95) & 27265 & 33 & 26163 & 75 & 144$\pm^{ 29 }_{ 25 }$ & $1.00$ & 25.5133 & $ 36.84\pm^{ 1.00E+20 }_{ 66.84 }$ & $ 15.99\pm^{ 0.47 }_{ nan }$ & 0.17\\ 
pg1309 & $0.18139$ (\#214)  & 116.87(93) & 27265 & 33 & 26163 & 75 & 141$\pm^{ 28 }_{ 24 }$ & $1.00$ & 25.5180 & $ 7.15\pm^{ 1.00E+20 }_{ 37.15 }$ & $ 15.85\pm^{ 0.56 }_{ nan }$ & 0.10\\ 
pg1309 & $0.18145$ (\#215)  & 116.88(93) & 27265 & 33 & 26163 & 75 & 141$\pm^{ 29 }_{ 25 }$ & $1.00$ & 25.5193 & $ 6.05\pm^{ 1.00E+20 }_{ 36.05 }$ & $ 15.85\pm^{ 0.61 }_{ nan }$ & 0.09\\ 
pg1309 & $0.18192$ (\#216)  & 114.96(94) & 27265 & 33 & 26163 & 78 & 145$\pm^{ 29 }_{ 25 }$ & $1.00$ & 25.5295 & $ 3.81\pm^{ 1.00E+20 }_{ 33.81 }$ & $ 15.78\pm^{ 0.68 }_{ nan }$ & 0.06\\ 
pg1309 & $0.18698$ (\#217)  & 107.23(91) & 27265 & 35 & 26163 & 78 & 158$\pm^{ 35 }_{ 26 }$ & $1.00$ & 25.6388 & $ 9.01E+09\pm^{ 1.00E+20 }_{ 9.01E+09 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 1.76\\ 
pg1444 & $0.22031$ (\#218)  & 113.67(93) & 17674 & 27 & 17137 & 35 & 183$\pm^{ 40 }_{ 35 }$ & $1.00$ & 26.3587 & $ -2.51\pm^{ 2.34 }_{ 1.07 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.34\\ 
pg1444 & $0.22676$ (\#219)  & 127.72(94) & 17674 & 34 & 17137 & 39 & 179$\pm^{ 40 }_{ 35 }$ & $1.00$ & 26.4980 & $ 1.03\pm^{ 9.66E+12 }_{ 31.03 }$ & $ 15.45\pm^{ 0.95 }_{ nan }$ & 0.03\\ 
pg1444 & $0.26690$ (\#220)  & 132.30(93) & 17674 & 56 & 17137 & 57 & 145$\pm^{ 39 }_{ 33 }$ & $1.00$ & 27.3650 & $ -3.50\pm^{ 1.38 }_{ 0.84 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.41\\ 
pg1444 & $0.26728$ (\#221)  & 132.11(94) & 17674 & 56 & 17137 & 57 & 146$\pm^{ 40 }_{ 34 }$ & $1.00$ & 27.3732 & $ -3.72\pm^{ 1.42 }_{ 0.90 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.67\\ 
pg1444 & $0.26738$ (\#222)  & 132.08(94) & 17674 & 56 & 17137 & 57 & 146$\pm^{ 40 }_{ 34 }$ & $1.00$ & 27.3754 & $ -3.39\pm^{ 1.24 }_{ 0.78 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.70\\ 
pg1444 & $0.26747$ (\#223)  & 127.49(93) & 17674 & 58 & 17137 & 61 & 143$\pm^{ 39 }_{ 33 }$ & $1.00$ & 27.3774 & $ -3.71\pm^{ 1.15 }_{ 0.78 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.74\\ 
pg1626 & $0.13075$ (\#224)  & 124.04(83) & 69157 & 66 & 68865 & 77 & 386$\pm^{ 48 }_{ 46 }$ & $1.00$ & 24.4242 & $ -2.57\pm^{ 0.92 }_{ 0.60 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.32\\ 
phl1811 & $0.07344$ (\#225)  & -- & -- & -- & -- & -- & -- & -- & 23.1863 & -- & -- & --\\ 
phl1811 & $0.07768$ (\#226)  & -- & -- & -- & -- & -- & -- & -- & 23.2779 & -- & -- & --\\ 
phl1811 & $0.08131$ (\#227)  & -- & -- & -- & -- & -- & -- & -- & 23.3563 & -- & -- & --\\ 
phl1811 & $0.13239$ (\#228)  & -- & -- & -- & -- & -- & -- & -- & 24.4596 & -- & -- & --\\ 
phl1811 & $0.13282$ (\#229)  & -- & -- & -- & -- & -- & -- & -- & 24.4689 & -- & -- & --\\ 
phl1811 & $0.13318$ (\#230)  & -- & -- & -- & -- & -- & -- & -- & 24.4767 & -- & -- & --\\ 
phl1811 & $0.13545$ (\#231)  & -- & -- & -- & -- & -- & -- & -- & 24.5257 & -- & -- & --\\ 
phl1811 & $0.15752$ (\#232)  & -- & -- & -- & -- & -- & -- & -- & 25.0024 & -- & -- & --\\ 
phl1811 & $0.15786$ (\#233)  & -- & -- & -- & -- & -- & -- & -- & 25.0098 & -- & -- & --\\ 
phl1811 & $0.17652$ (\#234)  & 118.26(84) & 79254 & 89 & 77556 & 75 & 35$\pm^{ 12 }_{ 11 }$ & $1.00$ & 25.4128 & $ 7.11E+04\pm^{ 1.00E+20 }_{ 7.11E+04 }$ & $ 16.21\pm^{ 0.25 }_{ nan }$ & 1.08\\ 
phl1811 & $0.19157$ (\#235*)  & 164.17(89) & 79254 & 101 & 76738 & 99 & 35$\pm^{ 13 }_{ 11 }$ & $1.00$ & 25.7379 & $ 141.21\pm^{ 1.00E+20 }_{ 171.21 }$ & $ 16.09\pm^{ 0.32 }_{ nan }$ & 0.13\\ 
phl1811 & $0.19194$ (\#236*)  & 167.21(88) & 79254 & 103 & 76682 & 100 & 34$\pm^{ 13 }_{ 11 }$ & $1.00$ & 25.7459 & $ 46.75\pm^{ 1.00E+20 }_{ 76.75 }$ & $ 16.00\pm^{ 0.46 }_{ nan }$ & 0.06\\ 
phl1811 & $0.19220$ (\#237*)  & 167.23(88) & 79254 & 103 & 76682 & 100 & 34$\pm^{ 12 }_{ 11 }$ & $1.00$ & 25.7515 & $ 8.42\pm^{ 1.00E+20 }_{ 38.42 }$ & $ 15.90\pm^{ 0.56 }_{ nan }$ & 0.03\\ 
pks0312 & $0.20188$ (\#238)  & 93.47(64) & 23858 & 44 & 22982 & 36 & 161$\pm^{ 40 }_{ 35 }$ & $1.00$ & 25.9606 & $ 3.90E+06\pm^{ 1.00E+20 }_{ 3.90E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 1.94\\ 
pks0312 & $0.20275$ (\#239*)  & 99.01(66) & 23858 & 48 & 22982 & 37 & 154$\pm^{ 39 }_{ 33 }$ & $1.00$ & 25.9794 & $ 4.48E+06\pm^{ 1.00E+20 }_{ 4.48E+06 }$ & $ 16.28\pm^{ 0.12 }_{ nan }$ & 1.41\\ 
pks0405 & $0.09192$ (\#240)  & 67.08(46) & 137245 & 21 & nan & nan & 358$\pm^{ 19 }_{ 18 }$ & $1.00$ & 23.5855 & $ -0.55\pm^{ 2.90 }_{ 1.06 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.13\\ 
pks0405 & $0.09647$ (\#241)  & 69.21(48) & 135771 & 21 & 138649 & 18 & 361$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.6838 & $ -1.25\pm^{ 1.51 }_{ 0.79 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.98\\ 
pks0405 & $0.14808$ (\#242)  & 88.65(90) & 136323 & 20 & 137234 & 20 & 373$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.7985 & $ -0.66\pm^{ 2.09 }_{ 0.99 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.23\\ 
pks0405 & $0.16566$ (\#243)  & 79.70(91) & 137140 & 18 & 137234 & 21 & 394$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.1783 & $ 4.27\pm^{ 309.84 }_{ 4.00 }$ & $ 15.80\pm^{ 0.27 }_{ 0.83 }$ & 1.67\\ 
pks0405 & $0.16606$ (\#244)  & 79.75(92) & 136407 & 17 & 137234 & 21 & 395$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.1869 & $ 4.75\pm^{ 228.47 }_{ 4.41 }$ & $ 15.81\pm^{ 0.25 }_{ 0.75 }$ & 1.78\\ 
pks0405 & $0.16659$ (\#245)  & 78.27(91) & 137924 & 18 & 137234 & 22 & 394$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.1983 & $ 5.60\pm^{ 767.40 }_{ 5.11 }$ & $ 15.84\pm^{ 0.24 }_{ 0.65 }$ & 2.01\\ 
pks0405 & $0.16688$ (\#246)  & 78.15(91) & 137924 & 18 & 137234 & 22 & 395$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.2046 & $ 8.37\pm^{ 265.42 }_{ 7.69 }$ & $ 15.87\pm^{ 0.23 }_{ 0.54 }$ & 2.16\\ 
pks0405 & $0.16712$ (\#247)  & 83.54(92) & 137941 & 18 & 137234 & 22 & 391$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.2098 & $ 6.94\pm^{ 643.47 }_{ 6.36 }$ & $ 15.86\pm^{ 0.24 }_{ 0.60 }$ & 2.15\\ 
pks0405 & $0.18257$ (\#248)  & 113.72(95) & 137986 & 22 & 136490 & 21 & 365$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.5435 & $ -0.51\pm^{ 1.96 }_{ 0.97 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.17\\ 
pks0405 & $0.18289$ (\#249)  & 114.40(96) & 138000 & 21 & 136490 & 21 & 365$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.5504 & $ -0.29\pm^{ 2.50 }_{ 1.00 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.05\\ 
pks0405 & $0.24052$ (\#250)  & 109.18(95) & 137976 & 21 & 138647 & 29 & 413$\pm^{ 23 }_{ 22 }$ & $1.00$ & 26.7952 & $ 3.89\pm^{ 1.05E+03 }_{ 3.98 }$ & $ 15.78\pm^{ 0.31 }_{ nan }$ & 1.03\\ 
pks0405 & $0.24094$ (\#251)  & 104.97(95) & 137961 & 21 & 138647 & 30 & 410$\pm^{ 23 }_{ 22 }$ & $1.00$ & 26.8043 & $ 5.51\pm^{ 1.53E+03 }_{ 5.63 }$ & $ 15.82\pm^{ 0.31 }_{ nan }$ & 1.15\\ 
pks0405 & $0.24547$ (\#252)  & 98.26(94) & 136439 & 23 & 138647 & 30 & 386$\pm^{ 23 }_{ 23 }$ & $1.00$ & 26.9022 & $ -0.96\pm^{ 1.43 }_{ 0.82 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.69\\ 
pks0405 & $0.29762$ (\#253)  & 98.20(89) & 135766 & 33 & 137130 & 34 & 382$\pm^{ 27 }_{ 26 }$ & $1.00$ & 28.0286 & $ -0.21\pm^{ 3.56 }_{ 1.16 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
pks0405 & $0.34188$ (\#254)  & 98.93(90) & 136321 & 40 & 138714 & 46 & 379$\pm^{ 29 }_{ 28 }$ & $1.00$ & 28.9846 & $ -1.69\pm^{ 2.22 }_{ 1.03 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.90\\ 
pks0405 & $0.34225$ (\#255)  & 98.19(90) & 136322 & 40 & 138714 & 47 & 381$\pm^{ 29 }_{ 28 }$ & $1.00$ & 28.9926 & $ -1.80\pm^{ 1.83 }_{ 0.88 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.22\\ 
pks0405 & $0.35092$ (\#256)  & 86.77(91) & 136325 & 43 & 138714 & 47 & 392$\pm^{ 32 }_{ 31 }$ & $1.00$ & 29.1799 & $ 118.44\pm^{ 1.95E+09 }_{ 117.08 }$ & $ 16.08\pm^{ 0.22 }_{ 0.52 }$ & 2.55\\ 
pks0405 & $0.36075$ (\#257)  & 90.38(93) & 137923 & 45 & 138714 & 45 & 385$\pm^{ 33 }_{ 32 }$ & $1.00$ & 29.3922 & $ 93.75\pm^{ 1.18E+09 }_{ 90.97 }$ & $ 16.06\pm^{ 0.24 }_{ 0.33 }$ & 2.11\\ 
pks0405 & $0.36151$ (\#258)  & 92.10(93) & 137923 & 46 & 138714 & 46 & 376$\pm^{ 32 }_{ 32 }$ & $1.00$ & 29.4086 & $ 23.36\pm^{ 1.43E+05 }_{ 24.12 }$ & $ 15.95\pm^{ 0.27 }_{ nan }$ & 1.10\\ 
pks0405 & $0.36329$ (\#259)  & 96.83(94) & 138708 & 47 & 138714 & 45 & 363$\pm^{ 32 }_{ 31 }$ & $1.00$ & 29.4471 & $ -0.68\pm^{ 3.27 }_{ 1.20 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.16\\ 
pks0405 & $0.40570$ (\#260)  & 120.73(84) & 137132 & 41 & 133905 & 45 & 452$\pm^{ 35 }_{ 34 }$ & $1.00$ & 30.3631 & $ 39.93\pm^{ 2.27E+06 }_{ 41.65 }$ & $ 15.99\pm^{ 0.26 }_{ nan }$ & 0.79\\ 
pks0405 & $0.40890$ (\#261)  & 110.16(86) & 137167 & 39 & 134014 & 47 & 491$\pm^{ 42 }_{ 35 }$ & $1.00$ & 30.4322 & $ 1.00E+07\pm^{ 1.00E+20 }_{ 9.95E+06 }$ & $ 16.29\pm^{ 0.18 }_{ 0.08 }$ & 6.95\\ 
pks0405 & $0.49505$ (\#262)  & 112.27(94) & 138729 & 51 & 137202 & 58 & 536$\pm^{ 45 }_{ 43 }$ & $1.00$ & 32.2931 & $ -2.10\pm^{ 0.90 }_{ 0.58 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.45\\ 
pks0405 & $0.49530$ (\#263)  & 108.35(92) & 138729 & 51 & 137169 & 58 & 528$\pm^{ 45 }_{ 43 }$ & $1.00$ & 32.2985 & $ -2.48\pm^{ 0.99 }_{ 0.69 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.18\\ 
pks0405 & $0.55506$ (\#264)  & 104.58(82) & 132269 & 59 & 134976 & 41 & 444$\pm^{ 57 }_{ 54 }$ & $1.00$ & 33.5893 & $ 2.18E+05\pm^{ 1.00E+20 }_{ 2.12E+05 }$ & $ 16.26\pm^{ 0.15 }_{ 0.14 }$ & 2.35\\ 
pks2005 & $0.06490$ (\#265)  & 59.89(42) & 53473 & 5 & nan & nan & 2202$\pm^{ 73 }_{ 71 }$ & $1.00$ & 23.0018 & $ -0.87\pm^{ 1.18 }_{ 0.68 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.74\\ 
pks2155 & $0.05405$ (\#266)  & -- & -- & -- & -- & -- & -- & -- & 22.7675 & -- & -- & --\\ 
pks2155 & $0.05707$ (\#267)  & 20.80(28) & 1697089 & 3 & nan & nan & 679$\pm^{ 108 }_{ 82 }$ & $4.85$ & 22.8327 & $ -0.26\pm^{ 0.11 }_{ 0.13 }$ & $ nan\pm^{ nan }_{ nan }$ & 5.24\\ 
q0045 & $0.11052$ (\#268)  & -- & -- & -- & -- & -- & -- & -- & 23.9872 & -- & -- & --\\ 
q0045 & $0.13521$ (\#269)  & -- & -- & -- & -- & -- & -- & -- & 24.5205 & -- & -- & --\\ 
q1230 & $0.09518$ (\#270)  & 63.84(48) & 39335 & 57 & 39139 & 83 & 112$\pm^{ 23 }_{ 20 }$ & $1.00$ & 23.6559 & $ 1.24E+03\pm^{ 1.00E+20 }_{ 1.27E+03 }$ & $ 16.12\pm^{ 0.34 }_{ nan }$ & 0.60\\ 
q1230 & $0.10318$ (\#271)  & 59.80(44) & 39335 & 55 & 39139 & 69 & 93$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.8287 & $ -3.93\pm^{ 2.04 }_{ 1.33 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.91\\ 
q1230 & $0.10445$ (\#272)  & 62.04(47) & 39335 & 57 & 39139 & 64 & 100$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.8561 & $ -3.24\pm^{ 3.05 }_{ 1.49 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.45\\ 
q1230 & $0.10530$ (\#273)  & 62.81(47) & 39335 & 57 & 39139 & 59 & 106$\pm^{ 27 }_{ 24 }$ & $1.00$ & 23.8745 & $ -2.31\pm^{ 1.93E+04 }_{ 2.00 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.34\\ 
q1230 & $0.10596$ (\#274)  & 63.04(47) & 39335 & 57 & 39139 & 59 & 111$\pm^{ 27 }_{ 24 }$ & $1.00$ & 23.8887 & $ -0.71\pm^{ 2.31E+08 }_{ 2.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
q1230 & $0.10666$ (\#275)  & 63.05(47) & 39335 & 57 & 39139 & 59 & 113$\pm^{ 26 }_{ 24 }$ & $1.00$ & 23.9039 & $ 0.65\pm^{ 3.29E+16 }_{ 30.65 }$ & $ 15.30\pm^{ 1.16 }_{ nan }$ & 0.00\\ 
q1230 & $0.10809$ (\#276)  & 59.85(45) & 39335 & 59 & 39139 & 59 & 103$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9347 & $ -1.44\pm^{ 1.00E+20 }_{ 2.10 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.06\\ 
q1230 & $0.10820$ (\#277)  & 62.54(45) & 39335 & 60 & 39139 & 59 & 103$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9371 & $ -1.59\pm^{ 1.00E+20 }_{ 2.24 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.08\\ 
q1230 & $0.10861$ (\#278)  & 59.64(45) & 39335 & 58 & 39139 & 55 & 105$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9460 & $ -1.69\pm^{ 1.00E+20 }_{ 2.08 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.10\\ 
q1230 & $0.10906$ (\#279)  & 61.31(47) & 39335 & 59 & 39139 & 55 & 101$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9557 & $ -2.14\pm^{ 2.35E+16 }_{ 1.90 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.20\\ 
q1230 & $0.10935$ (\#280)  & 61.34(47) & 39335 & 59 & 39139 & 55 & 102$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9620 & $ -1.88\pm^{ 1.00E+20 }_{ 1.72 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.16\\ 
q1230 & $0.10956$ (\#281)  & 61.25(46) & 39335 & 58 & 39139 & 55 & 107$\pm^{ 27 }_{ 24 }$ & $1.00$ & 23.9665 & $ -1.54\pm^{ 1.00E+20 }_{ 2.51 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.07\\ 
q1230 & $0.11707$ (\#282)  & 70.22(56) & 39335 & 56 & 39139 & 61 & 120$\pm^{ 31 }_{ 23 }$ & $1.00$ & 24.1287 & $ 1.72E+04\pm^{ 1.00E+20 }_{ 1.72E+04 }$ & $ 16.21\pm^{ 0.26 }_{ nan }$ & 1.38\\ 
q1230 & $0.11743$ (\#283)  & 71.60(58) & 39335 & 55 & 39139 & 59 & 121$\pm^{ 30 }_{ 24 }$ & $1.00$ & 24.1365 & $ 1.61E+04\pm^{ 1.00E+20 }_{ 1.61E+04 }$ & $ 16.20\pm^{ 0.23 }_{ nan }$ & 1.25\\ 
q1230 & $0.11781$ (\#284)  & 71.89(58) & 39335 & 55 & 39139 & 59 & 120$\pm^{ 26 }_{ 23 }$ & $1.00$ & 24.1447 & $ 1.50E+03\pm^{ 1.00E+20 }_{ 1.53E+03 }$ & $ 16.12\pm^{ 0.34 }_{ nan }$ & 0.91\\ 
rbs1892 & $0.15752$ (\#285)  & 86.45(91) & 4935 & 52 & 4865 & 20 & 220$\pm^{ 84 }_{ 67 }$ & $1.00$ & 25.0024 & $ -2.48\pm^{ 7.21 }_{ 1.42 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.66\\ 
rbs1892 & $0.17133$ (\#286)  & 86.80(94) & 4937 & 48 & 4865 & 27 & 309$\pm^{ 139 }_{ 95 }$ & $1.00$ & 25.3007 & $ 7.28E+08\pm^{ 1.00E+20 }_{ 7.28E+08 }$ & $ 16.35\pm^{ 0.11 }_{ inf }$ & 2.67\\ 
rbs1892 & $0.19874$ (\#287)  & 104.23(94) & 4937 & 29 & 4849 & 49 & 500$\pm^{ 129 }_{ 110 }$ & $1.00$ & 25.8928 & $ -1.31\pm^{ 1.34E+11 }_{ 2.25 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.06\\ 
rbs542 & $0.10323$ (\#288)  & 86.68(64) & 192553 & 9 & 181905 & 6 & 1543$\pm^{ 32 }_{ 31 }$ & $1.00$ & 23.8298 & $ 0.31\pm^{ 1.26 }_{ 0.76 }$ & $ 15.02\pm^{ 0.57 }_{ nan }$ & 0.16\\ 
rbs542 & $0.10379$ (\#289)  & 87.77(65) & 192488 & 8 & 181905 & 6 & 1551$\pm^{ 32 }_{ 32 }$ & $1.00$ & 23.8419 & $ 0.63\pm^{ 1.69 }_{ 0.90 }$ & $ 15.29\pm^{ 0.39 }_{ nan }$ & 0.52\\ 
rxj0439 & $0.11547$ (\#290)  & 95.23(74) & 148931 & 18 & 151265 & 13 & 506$\pm^{ 20 }_{ 20 }$ & $1.00$ & 24.0942 & $ -0.07\pm^{ 2.68 }_{ 1.03 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.00\\ 
rxj0439 & $0.21833$ (\#291)  & 118.05(95) & 147527 & 14 & 149811 & 17 & 588$\pm^{ 27 }_{ 26 }$ & $1.00$ & 26.3159 & $ 2.54\pm^{ 18.65 }_{ 2.52 }$ & $ 15.70\pm^{ 0.27 }_{ 1.77 }$ & 1.26\\ 
rxj0439 & $0.24235$ (\#292)  & 94.71(94) & 148524 & 17 & 152414 & 20 & 592$\pm^{ 28 }_{ 27 }$ & $1.00$ & 26.8348 & $ 2.06\pm^{ 42.43 }_{ 2.31 }$ & $ 15.66\pm^{ 0.33 }_{ nan }$ & 0.81\\ 
rxj0439 & $0.24258$ (\#293)  & 103.01(95) & 147411 & 16 & 152414 & 20 & 590$\pm^{ 28 }_{ 27 }$ & $1.00$ & 26.8397 & $ 2.33\pm^{ 27.65 }_{ 2.51 }$ & $ 15.68\pm^{ 0.31 }_{ nan }$ & 0.92\\ 
rxj0439 & $0.24313$ (\#294)  & 94.82(94) & 147411 & 16 & 152414 & 19 & 592$\pm^{ 28 }_{ 27 }$ & $1.00$ & 26.8516 & $ 1.25\pm^{ 10.07 }_{ 1.71 }$ & $ 15.52\pm^{ 0.40 }_{ nan }$ & 0.50\\ 
rxj0439 & $0.24387$ (\#295)  & 93.90(94) & 147412 & 16 & 152414 & 20 & 593$\pm^{ 29 }_{ 27 }$ & $1.00$ & 26.8676 & $ 0.20\pm^{ 3.28 }_{ 1.06 }$ & $ 14.84\pm^{ 0.92 }_{ nan }$ & 0.04\\ 
s50716 & $0.23145$ (\#296)  & 93.47(94) & 75297 & 11 & 76133 & 14 & 887$\pm^{ 42 }_{ 41 }$ & $1.00$ & 26.5993 & $ -0.22\pm^{ 2.24 }_{ 0.98 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
ton28 & $0.13746$ (\#297)  & 111.07(90) & 83595 & 34 & 86028 & 35 & 225$\pm^{ 23 }_{ 21 }$ & $1.00$ & 24.5691 & $ 1.60\pm^{ 3.50E+03 }_{ 2.97 }$ & $ 15.59\pm^{ 0.55 }_{ nan }$ & 0.16\\ 
ton28 & $0.13773$ (\#298)  & 110.95(90) & 83595 & 34 & 86028 & 35 & 227$\pm^{ 22 }_{ 22 }$ & $1.00$ & 24.5750 & $ 3.14\pm^{ 3.83E+04 }_{ 4.38 }$ & $ 15.75\pm^{ 0.42 }_{ nan }$ & 0.30\\ 
ton28 & $0.13781$ (\#299)  & 111.91(90) & 83595 & 34 & 86028 & 34 & 227$\pm^{ 23 }_{ 22 }$ & $1.00$ & 24.5767 & $ 3.47\pm^{ 7.02E+04 }_{ 4.65 }$ & $ 15.77\pm^{ 0.43 }_{ nan }$ & 0.35\\ 
ton28 & $0.17251$ (\#300)  & 98.29(95) & 86114 & 26 & 85104 & 36 & 203$\pm^{ 19 }_{ 18 }$ & $1.00$ & 25.3262 & $ -2.07\pm^{ 1.13 }_{ 0.69 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.67\\ 
ton28 & $0.21259$ (\#301)  & 116.22(89) & 84885 & 36 & 83740 & 41 & 193$\pm^{ 24 }_{ 22 }$ & $1.00$ & 26.1919 & $ 0.89\pm^{ 699.95 }_{ 2.51 }$ & $ 15.42\pm^{ 0.69 }_{ nan }$ & 0.06\\ 
ton28 & $0.24292$ (\#302)  & 105.70(82) & 83762 & 37 & 86136 & 41 & 178$\pm^{ 26 }_{ 24 }$ & $1.00$ & 26.8471 & $ -2.01\pm^{ 1.89 }_{ 0.96 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.35\\ 
ton28 & $0.24859$ (\#303*)  & 126.01(83) & 83842 & 34 & 86136 & 36 & 232$\pm^{ 28 }_{ 26 }$ & $1.00$ & 26.9695 & $ -1.05\pm^{ 3.86 }_{ 1.10 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.31\\ 
ton28 & $0.27338$ (\#304)  & 112.36(81) & 83758 & 31 & 86136 & 36 & 267$\pm^{ 32 }_{ 30 }$ & $1.00$ & 27.5050 & $ -1.96\pm^{ 1.29 }_{ 0.72 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.14\\ 
ton28 & $0.33021$ (\#305)  & 117.99(85) & 83660 & 49 & 84983 & 57 & 277$\pm^{ 37 }_{ 34 }$ & $1.00$ & 28.7325 & $ -0.78\pm^{ 170.49 }_{ 1.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.08\\ 
tons180 & $0.02340$ (\#306)  & 40.94(32) & 193565 & 8 & nan & nan & 1151$\pm^{ 32 }_{ 30 }$ & $1.00$ & 22.1054 & $ 0.86\pm^{ 2.71 }_{ 1.07 }$ & $ 15.40\pm^{ 0.37 }_{ nan }$ & 0.73\\ 
tons180 & $0.04360$ (\#307)  & 48.00(45) & 180786 & 8 & nan & nan & 1149$\pm^{ 28 }_{ 27 }$ & $1.00$ & 22.5418 & $ 0.29\pm^{ 1.61 }_{ 0.84 }$ & $ 14.99\pm^{ 0.64 }_{ nan }$ & 0.10\\ 
tons180 & $0.04560$ (\#308)  & 39.89(45) & 180786 & 8 & nan & nan & 1198$\pm^{ 28 }_{ 27 }$ & $1.00$ & 22.5850 & $ 69.38\pm^{ 4.72E+03 }_{ 56.06 }$ & $ 16.02\pm^{ 0.11 }_{ 0.11 }$ & 14.42\\ 
\hline
\hline
 \end{longtable}
 \end{landscape}

==> Tables/XMM/Latex/xmm_o7_o6_uppers_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllll|l}
\caption[\xmm\ Data, \ovii\ Upper Limits With \ovi\ Priors Results (Full)]{\ovii\ upper limit measurements with \xmm\ data, at the prior redshift from the \ovi\ lines from Table~\ref{tab:oviPriorsTable}. The $\tau_0$ in this table is calculated through the previous table's $\tau_0$ errors, given by Equation \ref{eq:tau0+}. The corresponding column density was calculated using this value.}
\label{tab:xmmovioviiuppers}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & RGS1 & RGS2 & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & avg exp (s) & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N + (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 

1es1028 & $0.12314$ (\#1)  & 95.40(79) & 144787 & 147275 & 1102$\pm^{ 30 }_{ 30 }$ & $1.00$ & 24.2598 & 1.31 & 15.53 & 0.40\\ 
1es1028 & $0.13706$ (\#2)  & 92.82(90) & 143804 & 146370 & 1121$\pm^{ 33 }_{ 32 }$ & $1.00$ & 24.5605 & 0.71 & 15.33 & 0.22\\ 
1es1028 & $0.33735$ (\#3)  & 86.46(91) & 145450 & 146420 & 1324$\pm^{ 48 }_{ 46 }$ & $1.00$ & 28.8868 & 0.70 & 15.33 & 1.08\\ 
1es1553 & $0.18759$ (\#4)  & 102.10(88) & 1793737 & 1757303 & 1796$\pm^{ 13 }_{ 12 }$ & $1.00$ & 25.6519 & 0.29 & 14.99 & 7.82\\ 
1es1553 & $0.18775$ (\#5)  & 102.34(88) & 1793737 & 1757303 & 1796$\pm^{ 13 }_{ 12 }$ & $1.00$ & 25.6554 & 0.27 & 14.97 & 7.53\\ 
1es1553 & $0.18984$ (\#6)  & 105.72(86) & 1794800 & 1753128 & 1778$\pm^{ 12 }_{ 12 }$ & $1.00$ & 25.7005 & 0.20 & 14.85 & 0.16\\ 
1es1553 & $0.21631$ (\#7)  & 84.95(81) & 1756247 & 1757203 & 1778$\pm^{ 14 }_{ 14 }$ & $1.00$ & 26.2723 & 0.24 & 14.91 & 0.95\\ 
1es1553 & $0.31130$ (\#8)  & 113.79(90) & 1740303 & 1677696 & 1807$\pm^{ 15 }_{ 15 }$ & $1.00$ & 28.3241 & 0.24 & 14.92 & 0.45\\ 
1es1553 & $0.37868$ (\#9)  & 119.25(98) & 1809416 & 1817188 & 1834$\pm^{ 17 }_{ 17 }$ & $1.00$ & 29.7795 & 0.44 & 15.16 & -0.04\\ 
1es1553 & $0.39497$ (\#10)  & 90.13(98) & 1751580 & 1813451 & 1810$\pm^{ 18 }_{ 18 }$ & $1.00$ & 30.1314 & 0.31 & 15.02 & 0.02\\ 
3c249 & $0.24676$ (\#11)  & 78.14(93) & 2639 & 2524 & 282$\pm^{ 141 }_{ 104 }$ & $1.00$ & 26.9300 & 5.33E+11 & 16.40 & 0.03\\ 
3c249 & $0.30788$ (\#12)  & 81.25(88) & 2639 & 2535 & 697$\pm^{ 234 }_{ 175 }$ & $1.00$ & 28.2502 & 5.00E+19 & 16.46 & 0.35\\ 
3c249 & $0.30809$ (\#13)  & 81.15(88) & 2639 & 2535 & 701$\pm^{ 236 }_{ 177 }$ & $1.00$ & 28.2547 & 5.00E+19 & 16.46 & 0.47\\ 
3c249 & $0.31364$ (\#14)  & 78.36(88) & 2639 & 2538 & 758$\pm^{ 250 }_{ 193 }$ & $1.00$ & 28.3746 & 5.00E+19 & 16.46 & 1.72\\ 
3c273 & $0.00337$ (\#15)  & -- & -- & -- & -- & -- & 21.6728 & -- & -- & --\\ 
3c273 & $0.00533$ (\#16)  & -- & -- & -- & -- & -- & 21.7151 & -- & -- & --\\ 
3c273 & $0.00764$ (\#17)  & -- & -- & -- & -- & -- & 21.7650 & -- & -- & --\\ 
3c273 & $0.02947$ (\#18*)  & 61.61(38) & 995937 & nan & 4600$\pm^{ 1762 }_{ 886 }$ & $0.84$ & 22.2366 & 0.21 & 14.86 & -0.00\\ 
3c273 & $0.04898$ (\#19)  & 63.63(45) & 936604 & nan & 1268$\pm^{ 345 }_{ 291 }$ & $3.02$ & 22.6580 & 0.23 & 14.91 & 0.84\\ 
3c273 & $0.06655$ (\#20*)  & 153.93(46) & 912160 & nan & 1021$\pm^{ 260 }_{ 212 }$ & $3.36$ & 23.0375 & 0.17 & 14.79 & 10.40\\ 
3c273 & $0.09018$ (\#21*)  & 100.60(47) & 996642 & nan & 931$\pm^{ 250 }_{ 186 }$ & $3.57$ & 23.5479 & 0.76 & 15.35 & 78.29\\ 
3c273 & $0.12007$ (\#22)  & 53.39(62) & 1024121 & 1027398 & 1102$\pm^{ 252 }_{ 235 }$ & $3.32$ & 24.1935 & 0.16 & 14.75 & 2.79\\ 
3c273 & $0.14660$ (\#23)  & 91.01(79) & 921050 & 1030884 & 2069$\pm^{ 402 }_{ 386 }$ & $2.37$ & 24.7666 & 0.27 & 14.97 & 17.90\\ 
3c273 & $0.15784$ (\#24)  & 115.64(86) & 931929 & 1033805 & 1143$\pm^{ 230 }_{ 202 }$ & $3.21$ & 25.0093 & 0.15 & 14.73 & 1.10\\ 
h1821 & $0.02438$ (\#25)  & -- & -- & -- & -- & -- & 22.1266 & -- & -- & --\\ 
h1821 & $0.10817$ (\#26)  & 95.28(70) & 31345 & 42458 & 1133$\pm^{ 91 }_{ 88 }$ & $1.00$ & 23.9365 & 398.31 & 16.08 & 0.11\\ 
h1821 & $0.12133$ (\#27)  & 100.65(84) & 29451 & 43368 & 1293$\pm^{ 89 }_{ 87 }$ & $1.00$ & 24.2207 & 1.29E+03 & 16.12 & 1.69\\ 
h1821 & $0.12147$ (\#28)  & 100.41(84) & 29451 & 43368 & 1292$\pm^{ 89 }_{ 85 }$ & $1.00$ & 24.2238 & 1.32E+04 & 16.15 & 1.90\\ 
h1821 & $0.16992$ (\#29)  & 141.11(98) & 32964 & 42688 & 1380$\pm^{ 94 }_{ 90 }$ & $1.00$ & 25.2703 & 1.11 & 15.48 & 0.88\\ 
h1821 & $0.17043$ (\#30)  & 142.88(98) & 32977 & 42408 & 1382$\pm^{ 93 }_{ 90 }$ & $1.00$ & 25.2813 & 0.87 & 15.40 & 1.58\\ 
h1821 & $0.21326$ (\#31)  & 109.00(98) & 31699 & 41854 & 1642$\pm^{ 109 }_{ 108 }$ & $1.00$ & 26.2064 & 1.73E+07 & 16.29 & 2.96\\ 
h1821 & $0.22497$ (\#32)  & 122.07(98) & 32383 & 43022 & 1546$\pm^{ 108 }_{ 106 }$ & $1.00$ & 26.4594 & 2.43 & 15.70 & 0.03\\ 
h1821 & $0.22522$ (\#33)  & 122.01(98) & 32383 & 43022 & 1543$\pm^{ 109 }_{ 106 }$ & $1.00$ & 26.4648 & 1.88 & 15.63 & 0.10\\ 
h1821 & $0.22639$ (\#34)  & 119.71(98) & 32358 & 43044 & 1535$\pm^{ 108 }_{ 104 }$ & $1.00$ & 26.4900 & 1.04 & 15.45 & 0.95\\ 
h1821 & $0.24531$ (\#35)  & 119.80(98) & 31065 & 44448 & 1591$\pm^{ 120 }_{ 113 }$ & $1.00$ & 26.8987 & 9.68 & 15.89 & 0.06\\ 
h1821 & $0.26657$ (\#36)  & 111.36(98) & 30604 & 44448 & 1501$\pm^{ 135 }_{ 123 }$ & $1.00$ & 27.3579 & 1.18E+07 & 16.26 & 3.28\\ 
h1821 & $0.28800$ (\#37)  & 134.30(98) & 30054 & 39392 & 1661$\pm^{ 136 }_{ 133 }$ & $1.00$ & 27.8208 & 1.42E+05 & 16.21 & 1.58\\ 
h1821 & $0.29658$ (\#38)  & 134.83(98) & 31075 & 39131 & 1569$\pm^{ 132 }_{ 127 }$ & $1.00$ & 28.0061 & 0.61 & 15.28 & 6.80\\ 
h1821 & $0.29680$ (\#39)  & 135.23(98) & 31075 & 39131 & 1574$\pm^{ 131 }_{ 127 }$ & $1.00$ & 28.0109 & 0.57 & 15.25 & 6.28\\ 
h2356 & $0.11461$ (\#40)  & 85.19(77) & 491451 & 516214 & 1312$\pm^{ 17 }_{ 17 }$ & $1.00$ & 24.0756 & 0.60 & 15.28 & 1.54\\ 
h2356 & $0.16512$ (\#41)  & 111.39(97) & 497056 & 504552 & 1325$\pm^{ 18 }_{ 18 }$ & $1.00$ & 25.1666 & 0.48 & 15.19 & 0.06\\ 
he0056 & $0.16392$ (\#42)  & 96.42(92) & 162630 & 161955 & 479$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.1407 & 1.34 & 15.54 & -0.00\\ 
he0056 & $0.16492$ (\#43)  & 99.30(92) & 162629 & 161955 & 478$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.1623 & 1.23 & 15.51 & 0.02\\ 
he0226 & $0.01746$ (\#44)  & 23.70(19) & 31712 & nan & 123$\pm^{ 40 }_{ 35 }$ & $1.00$ & 21.9771 & 3.27 & 15.75 & 0.85\\ 
he0226 & $0.02679$ (\#45)  & 39.57(27) & 31712 & nan & 114$\pm^{ 31 }_{ 27 }$ & $1.00$ & 22.1787 & 1.19E+04 & 16.15 & 0.51\\ 
he0226 & $0.04121$ (\#46)  & 45.84(33) & 31712 & nan & 158$\pm^{ 38 }_{ 27 }$ & $1.00$ & 22.4901 & 5.00E+19 & 16.41 & 0.70\\ 
he0226 & $0.04535$ (\#47)  & 43.77(36) & 31712 & nan & 177$\pm^{ 31 }_{ 29 }$ & $1.00$ & 22.5796 & 5.00E+19 & 16.46 & 3.25\\ 
he0226 & $0.04609$ (\#48)  & 44.36(37) & 31712 & nan & 176$\pm^{ 42 }_{ 29 }$ & $1.00$ & 22.5955 & 5.00E+19 & 16.46 & 3.70\\ 
he0226 & $0.06015$ (\#49)  & 53.36(41) & 31712 & nan & 149$\pm^{ 30 }_{ 27 }$ & $1.00$ & 22.8992 & 122.85 & 16.03 & 0.40\\ 
he0226 & $0.06083$ (\#50)  & 51.97(41) & 31712 & nan & 141$\pm^{ 29 }_{ 26 }$ & $1.00$ & 22.9139 & 2.12 & 15.67 & 1.36\\ 
he0226 & $0.07023$ (\#51)  & 37.36(40) & 31713 & nan & 187$\pm^{ 31 }_{ 30 }$ & $1.00$ & 23.1170 & 5.00E+19 & 16.41 & 0.11\\ 
he0226 & $0.08375$ (\#52)  & 44.35(43) & 31713 & nan & 188$\pm^{ 31 }_{ 29 }$ & $1.00$ & 23.4090 & 151.54 & 16.01 & 0.56\\ 
he0226 & $0.08901$ (\#53)  & 43.41(45) & 31713 & nan & 177$\pm^{ 31 }_{ 27 }$ & $1.00$ & 23.5226 & 5.10E+16 & 16.46 & 0.17\\ 
he0226 & $0.08938$ (\#54)  & 43.45(45) & 31713 & nan & 177$\pm^{ 28 }_{ 26 }$ & $1.00$ & 23.5306 & 5.00E+19 & 16.46 & 0.44\\ 
he0226 & $0.08950$ (\#55)  & 43.43(45) & 31713 & nan & 177$\pm^{ 30 }_{ 25 }$ & $1.00$ & 23.5332 & 5.00E+19 & 16.41 & 0.45\\ 
he0226 & $0.09220$ (\#56)  & 50.37(48) & 31713 & 31705 & 158$\pm^{ 28 }_{ 27 }$ & $1.00$ & 23.5915 & 1.51E+14 & 16.41 & 0.00\\ 
he0226 & $0.10668$ (\#57)  & 72.04(63) & 31713 & 31705 & 193$\pm^{ 37 }_{ 27 }$ & $1.00$ & 23.9043 & 5.00E+19 & 16.46 & 2.49\\ 
he0226 & $0.11514$ (\#58)  & 76.88(72) & 31713 & 31705 & 222$\pm^{ 39 }_{ 30 }$ & $1.00$ & 24.0870 & 5.00E+19 & 16.41 & 2.99\\ 
he0226 & $0.11680$ (\#59)  & 80.69(74) & 31713 & 31705 & 229$\pm^{ 34 }_{ 28 }$ & $1.00$ & 24.1229 & 5.00E+19 & 16.41 & 0.56\\ 
he0226 & $0.11733$ (\#60)  & 85.55(74) & 31713 & 31705 & 230$\pm^{ 32 }_{ 28 }$ & $1.00$ & 24.1343 & 5.00E+19 & 16.41 & 0.27\\ 
he0226 & $0.12589$ (\#61)  & 80.14(78) & 31713 & 31705 & 242$\pm^{ 34 }_{ 31 }$ & $1.00$ & 24.3192 & 30.29 & 15.97 & 0.16\\ 
he0226 & $0.13832$ (\#62)  & 83.89(87) & 31710 & 31705 & 263$\pm^{ 36 }_{ 33 }$ & $1.00$ & 24.5877 & 2.36 & 15.69 & 0.65\\ 
he0226 & $0.15175$ (\#63)  & 89.30(91) & 31708 & 31705 & 251$\pm^{ 34 }_{ 31 }$ & $1.00$ & 24.8778 & 5.58E+03 & 16.15 & 0.00\\ 
he0226 & $0.15549$ (\#64)  & 93.36(91) & 31708 & 31705 & 240$\pm^{ 34 }_{ 31 }$ & $1.00$ & 24.9586 & 2.86E+07 & 16.30 & 0.18\\ 
he0226 & $0.16237$ (\#65)  & 100.56(90) & 31707 & 31705 & 223$\pm^{ 34 }_{ 30 }$ & $1.00$ & 25.1072 & 1.57E+08 & 16.34 & 0.28\\ 
he0226 & $0.16339$ (\#66)  & 99.03(90) & 31706 & 31705 & 228$\pm^{ 34 }_{ 29 }$ & $1.00$ & 25.1292 & 5.00E+19 & 16.41 & 1.02\\ 
he0226 & $0.16971$ (\#67)  & 101.88(94) & 31706 & 31705 & 234$\pm^{ 33 }_{ 30 }$ & $1.00$ & 25.2657 & 31.62 & 15.98 & 0.13\\ 
he0226 & $0.18619$ (\#68)  & 124.06(95) & 31706 & 31705 & 245$\pm^{ 33 }_{ 30 }$ & $1.00$ & 25.6217 & 2.16 & 15.66 & 0.65\\ 
he0226 & $0.18811$ (\#69)  & 120.64(94) & 31706 & 31704 & 254$\pm^{ 34 }_{ 31 }$ & $1.00$ & 25.6632 & 2.23 & 15.68 & 0.71\\ 
he0226 & $0.18891$ (\#70)  & 118.10(94) & 31706 & 31704 & 247$\pm^{ 33 }_{ 31 }$ & $1.00$ & 25.6805 & 1.68 & 15.60 & 1.08\\ 
he0226 & $0.19374$ (\#71)  & 104.01(94) & 31706 & 31704 & 234$\pm^{ 33 }_{ 31 }$ & $1.00$ & 25.7848 & 0.97 & 15.45 & 5.57\\ 
he0226 & $0.19453$ (\#72)  & 106.55(94) & 31706 & 31704 & 233$\pm^{ 33 }_{ 31 }$ & $1.00$ & 25.8018 & 0.88 & 15.41 & 6.18\\ 
he0226 & $0.19860$ (\#73)  & 120.02(93) & 31706 & 31704 & 266$\pm^{ 35 }_{ 32 }$ & $1.00$ & 25.8898 & 4.25 & 15.80 & 0.39\\ 
he0226 & $0.20055$ (\#74)  & 120.40(93) & 31706 & 31704 & 280$\pm^{ 35 }_{ 33 }$ & $1.00$ & 25.9319 & 1.07E+05 & 16.22 & 0.23\\ 
he0226 & $0.20703$ (\#75)  & 112.17(93) & 31706 & 31704 & 314$\pm^{ 36 }_{ 34 }$ & $1.00$ & 26.0718 & 2.03E+15 & 16.42 & 1.31\\ 
he0226 & $0.22009$ (\#76)  & 120.76(87) & 31706 & 31704 & 255$\pm^{ 37 }_{ 34 }$ & $1.00$ & 26.3539 & 7.21 & 15.87 & 0.19\\ 
he0226 & $0.22099$ (\#77)  & 119.34(87) & 31706 & 31704 & 260$\pm^{ 36 }_{ 34 }$ & $1.00$ & 26.3734 & 1.49E+05 & 16.22 & 0.27\\ 
he0226 & $0.23009$ (\#78)  & 123.04(89) & 31707 & 31704 & 282$\pm^{ 39 }_{ 35 }$ & $1.00$ & 26.5699 & 1.15E+04 & 16.14 & 0.00\\ 
he0226 & $0.23964$ (\#79)  & 122.92(92) & 31707 & 31704 & 314$\pm^{ 41 }_{ 38 }$ & $1.00$ & 26.7762 & 1.07E+13 & 16.37 & 1.38\\ 
he0226 & $0.24522$ (\#80)  & 115.07(90) & 31708 & 31704 & 293$\pm^{ 42 }_{ 39 }$ & $1.00$ & 26.8968 & 800.78 & 16.09 & 0.00\\ 
he0226 & $0.25099$ (\#81)  & 119.85(90) & 31708 & 31704 & 270$\pm^{ 40 }_{ 37 }$ & $1.00$ & 27.0214 & 3.49 & 15.77 & 0.34\\ 
he0226 & $0.27155$ (\#82)  & 120.66(94) & 31709 & 31704 & 262$\pm^{ 40 }_{ 37 }$ & $1.00$ & 27.4655 & 2.90E+09 & 16.34 & 1.18\\ 
he0226 & $0.27956$ (\#83)  & 118.26(89) & 31709 & 31704 & 292$\pm^{ 43 }_{ 39 }$ & $1.00$ & 27.6385 & 5.00E+19 & 16.41 & 2.01\\ 
he0226 & $0.28041$ (\#84)  & 121.45(88) & 31709 & 31704 & 281$\pm^{ 46 }_{ 39 }$ & $1.00$ & 27.6569 & 5.00E+19 & 16.41 & 0.86\\ 
he0226 & $0.29134$ (\#85)  & 114.15(85) & 31709 & 31707 & 303$\pm^{ 45 }_{ 41 }$ & $1.00$ & 27.8929 & 377.22 & 16.04 & 0.04\\ 
he0226 & $0.29213$ (\#86)  & 114.62(85) & 31709 & 31707 & 318$\pm^{ 47 }_{ 42 }$ & $1.00$ & 27.9100 & 2.36E+06 & 16.23 & 0.06\\ 
he0226 & $0.30939$ (\#87)  & 100.48(87) & 31709 & 31713 & 363$\pm^{ 48 }_{ 46 }$ & $1.00$ & 28.2828 & 2.14E+05 & 16.22 & 0.00\\ 
he0226 & $0.31833$ (\#88)  & 104.18(83) & 31709 & 31716 & 375$\pm^{ 58 }_{ 51 }$ & $1.00$ & 28.4759 & 1.43E+11 & 16.36 & 0.06\\ 
he0226 & $0.33965$ (\#89)  & 125.18(89) & 31713 & 31717 & 336$\pm^{ 56 }_{ 52 }$ & $1.00$ & 28.9364 & 5.00E+19 & 16.46 & 2.50\\ 
he0226 & $0.34036$ (\#90)  & 130.69(90) & 31713 & 31717 & 335$\pm^{ 56 }_{ 52 }$ & $1.00$ & 28.9518 & 5.00E+19 & 16.46 & 1.44\\ 
he0226 & $0.35493$ (\#91)  & 120.67(92) & 31716 & 31717 & 281$\pm^{ 58 }_{ 52 }$ & $1.00$ & 29.2665 & 1.04 & 15.45 & 3.03\\ 
he0226 & $0.35528$ (\#92)  & 120.85(92) & 31716 & 31717 & 282$\pm^{ 58 }_{ 53 }$ & $1.00$ & 29.2740 & 1.19 & 15.51 & 2.77\\ 
he0226 & $0.37281$ (\#93)  & 111.76(99) & 31717 & 31717 & 352$\pm^{ 79 }_{ 56 }$ & $1.00$ & 29.6527 & 5.00E+19 & 16.46 & 2.58\\ 
he0226 & $0.38420$ (\#94)  & 114.74(94) & 31717 & 31717 & 360$\pm^{ 63 }_{ 58 }$ & $1.00$ & 29.8987 & 3.90E+09 & 16.31 & 0.03\\ 
he0226 & $0.38636$ (\#95)  & 107.14(90) & 31717 & 31717 & 355$\pm^{ 72 }_{ 57 }$ & $1.00$ & 29.9454 & 5.00E+19 & 16.41 & 0.74\\ 
he0226 & $0.39642$ (\#96)  & 117.89(86) & 31717 & 31717 & 283$\pm^{ 60 }_{ 53 }$ & $1.00$ & 30.1627 & 5.75 & 15.85 & 0.48\\ 
he0226 & $0.39692$ (\#97)  & 121.57(86) & 31717 & 31717 & 282$\pm^{ 62 }_{ 55 }$ & $1.00$ & 30.1735 & 9.22E+03 & 16.17 & 0.04\\ 
he0226 & $0.39890$ (\#98)  & 118.58(86) & 31717 & 31717 & 289$\pm^{ 62 }_{ 55 }$ & $1.00$ & 30.2162 & 1.57E+03 & 16.13 & 0.18\\ 
he0226 & $0.40034$ (\#99)  & 117.15(85) & 31717 & 31717 & 273$\pm^{ 59 }_{ 53 }$ & $1.00$ & 30.2473 & 1.26 & 15.52 & 2.43\\ 
he0226 & $0.40274$ (\#100)  & 121.91(83) & 31717 & 31717 & 307$\pm^{ 63 }_{ 57 }$ & $1.00$ & 30.2992 & 2.44E+06 & 16.23 & 0.03\\ 
he0226 & $0.49225$ (\#101)  & 130.27(93) & 31722 & 31717 & 423$\pm^{ 80 }_{ 73 }$ & $1.00$ & 32.2326 & 2.00 & 15.64 & 1.03\\ 
he0226 & $0.49254$ (\#102)  & 123.54(92) & 31722 & 31717 & 434$\pm^{ 80 }_{ 74 }$ & $1.00$ & 32.2389 & 2.39 & 15.68 & 0.77\\ 
he0226 & $0.49280$ (\#103)  & 123.59(92) & 31722 & 31717 & 435$\pm^{ 81 }_{ 74 }$ & $1.00$ & 32.2445 & 2.78 & 15.70 & 0.70\\ 
he0226 & $0.49309$ (\#104)  & 129.01(93) & 31722 & 31717 & 423$\pm^{ 79 }_{ 73 }$ & $1.00$ & 32.2507 & 2.86 & 15.73 & 0.71\\ 
i22456 & $0.09858$ (\#105)  & 68.71(60) & 79883 & 72481 & 656$\pm^{ 39 }_{ 37 }$ & $1.00$ & 23.7293 & 15.89 & 15.93 & 0.02\\ 
i22456 & $0.09895$ (\#106)  & 68.38(60) & 79752 & 73453 & 659$\pm^{ 38 }_{ 37 }$ & $1.00$ & 23.7373 & 14.53 & 15.90 & 0.01\\ 
i22456 & $0.09931$ (\#107)  & 68.39(60) & 79752 & 73453 & 657$\pm^{ 37 }_{ 37 }$ & $1.00$ & 23.7451 & 7.91 & 15.86 & 0.00\\ 
i22456 & $0.09959$ (\#108)  & 74.98(61) & 79883 & 73453 & 669$\pm^{ 37 }_{ 37 }$ & $1.00$ & 23.7511 & 4.44 & 15.81 & 0.00\\ 
i22456 & $0.09989$ (\#109)  & 68.68(61) & 79752 & 74286 & 651$\pm^{ 38 }_{ 37 }$ & $1.00$ & 23.7576 & 2.19 & 15.67 & 0.18\\ 
i22456 & $0.10034$ (\#110)  & 69.76(62) & 79883 & 74286 & 656$\pm^{ 37 }_{ 37 }$ & $1.00$ & 23.7673 & 1.77 & 15.61 & 0.30\\ 
i22456 & $0.10101$ (\#111)  & 73.32(62) & 79121 & 75007 & 657$\pm^{ 38 }_{ 37 }$ & $1.00$ & 23.7818 & 1.90 & 15.64 & 0.26\\ 
i22456 & $0.10146$ (\#112)  & 75.43(63) & 77663 & 75007 & 665$\pm^{ 36 }_{ 42 }$ & $1.00$ & 23.7915 & 3.02 & 15.74 & 0.02\\ 
mr2251 & $0.01070$ (\#113)  & -- & -- & -- & -- & -- & 21.8311 & -- & -- & --\\ 
mrk421 & $0.01009$ (\#114)  & -- & -- & -- & -- & -- & 21.8179 & -- & -- & --\\ 
mrk876 & $0.00311$ (\#115)  & -- & -- & -- & -- & -- & 21.6672 & -- & -- & --\\ 
mrk876 & $0.06248$ (\#116)  & 41.89(45) & 2651 & nan & 495$\pm^{ 152 }_{ 120 }$ & $1.00$ & 22.9496 & 5.00E+19 & 16.46 & 0.83\\ 
mrk876 & $0.08579$ (\#117)  & 36.44(46) & 2765 & nan & 357$\pm^{ 118 }_{ 97 }$ & $1.00$ & 23.4531 & 5.00E+19 & 16.46 & 1.63\\ 
mrk876 & $0.11488$ (\#118)  & 73.35(75) & 2743 & 2633 & 529$\pm^{ 144 }_{ 121 }$ & $1.00$ & 24.0814 & 5.00E+19 & 16.46 & 0.00\\ 
mrk876 & $0.11517$ (\#119)  & 75.24(76) & 2746 & 2633 & 567$\pm^{ 149 }_{ 126 }$ & $1.00$ & 24.0877 & 5.00E+19 & 16.41 & 0.05\\ 
mrk876 & $0.11588$ (\#120)  & 76.60(76) & 2743 & 2636 & 603$\pm^{ 153 }_{ 130 }$ & $1.00$ & 24.1030 & 5.00E+19 & 16.46 & 0.14\\ 
ngc7469 & $0.00962$ (\#121)  & -- & -- & -- & -- & -- & 21.8078 & -- & -- & --\\ 
ngc7469 & $0.00994$ (\#122)  & -- & -- & -- & -- & -- & 21.8147 & -- & -- & --\\ 
ngc7469 & $0.01153$ (\#123)  & -- & -- & -- & -- & -- & 21.8490 & -- & -- & --\\ 
p1103 & $0.13556$ (\#124)  & 87.53(87) & 15673 & 15681 & 3494$\pm^{ 169 }_{ 164 }$ & $1.00$ & 24.5281 & 1.00 & 15.45 & 0.47\\ 
p1103 & $0.13937$ (\#125)  & 91.46(88) & 15673 & 15681 & 3603$\pm^{ 170 }_{ 165 }$ & $1.00$ & 24.6104 & 9.42 & 15.89 & 0.98\\ 
p1103 & $0.14099$ (\#126)  & 96.68(88) & 15673 & 15681 & 3562$\pm^{ 166 }_{ 161 }$ & $1.00$ & 24.6454 & 1.08 & 15.47 & 0.24\\ 
p1103 & $0.14126$ (\#127)  & 97.21(89) & 15673 & 15681 & 3537$\pm^{ 166 }_{ 160 }$ & $1.00$ & 24.6512 & 0.95 & 15.43 & 0.62\\ 
p1103 & $0.17277$ (\#128)  & 83.97(94) & 15671 & 15681 & 3424$\pm^{ 156 }_{ 152 }$ & $1.00$ & 25.3318 & 0.99 & 15.45 & 0.61\\ 
pg0003 & $0.16521$ (\#129)  & 110.21(91) & 13034 & 12941 & 284$\pm^{ 60 }_{ 53 }$ & $1.00$ & 25.1685 & 5.36 & 15.83 & 0.44\\ 
pg0003 & $0.20907$ (\#130)  & 119.20(94) & 13033 & 12875 & 302$\pm^{ 63 }_{ 55 }$ & $1.00$ & 26.1159 & 207.54 & 16.10 & 0.18\\ 
pg0003 & $0.29021$ (\#131)  & 124.39(88) & 13035 & 12849 & 347$\pm^{ 85 }_{ 74 }$ & $1.00$ & 27.8685 & 2.33E+04 & 16.16 & 0.03\\ 
pg0003 & $0.30551$ (\#132*)  & 138.04(89) & 13035 & 12885 & 291$\pm^{ 75 }_{ 64 }$ & $1.00$ & 28.1990 & 1.74 & 15.61 & 1.53\\ 
pg0003 & $0.30569$ (\#133*)  & 137.89(89) & 13035 & 12885 & 292$\pm^{ 74 }_{ 64 }$ & $1.00$ & 28.2029 & 1.76 & 15.62 & 1.68\\ 
pg0003 & $0.34757$ (\#134)  & 105.38(90) & 13039 & 12932 & 231$\pm^{ 86 }_{ 68 }$ & $1.00$ & 29.1075 & 1.22 & 15.51 & 4.27\\ 
pg0003 & $0.34788$ (\#135)  & 105.00(90) & 13039 & 12932 & 229$\pm^{ 84 }_{ 68 }$ & $1.00$ & 29.1142 & 1.28 & 15.53 & 4.76\\ 
pg0003 & $0.36452$ (\#136)  & 126.87(94) & 13041 & 12932 & 361$\pm^{ 143 }_{ 107 }$ & $1.00$ & 29.4736 & 5.00E+19 & 16.41 & 2.32\\ 
pg0003 & $0.36508$ (\#137)  & 128.24(95) & 13041 & 12932 & 358$\pm^{ 99 }_{ 86 }$ & $1.00$ & 29.4857 & 5.00E+19 & 16.46 & 3.18\\ 
pg0003 & $0.36572$ (\#138)  & 128.74(97) & 13041 & 12932 & 356$\pm^{ 99 }_{ 85 }$ & $1.00$ & 29.4996 & 5.00E+19 & 16.46 & 3.55\\ 
pg0003 & $0.36621$ (\#139)  & 130.11(96) & 13041 & 12932 & 349$\pm^{ 116 }_{ 93 }$ & $1.00$ & 29.5101 & 5.00E+19 & 16.46 & 3.05\\ 
pg0003 & $0.37029$ (\#140)  & 139.10(98) & 13041 & 12932 & 313$\pm^{ 91 }_{ 78 }$ & $1.00$ & 29.5983 & 5.00E+19 & 16.46 & 0.44\\ 
pg0003 & $0.38608$ (\#141)  & 106.39(88) & 13041 & 12920 & 115$\pm^{ 65 }_{ 46 }$ & $1.00$ & 29.9393 & 0.83 & 15.39 & 13.26\\ 
pg0003 & $0.38639$ (\#142)  & 114.18(87) & 13041 & 12920 & 151$\pm^{ 74 }_{ 56 }$ & $1.00$ & 29.9460 & 1.17 & 15.51 & 8.98\\ 
pg0003 & $0.40138$ (\#143)  & 124.56(86) & 13041 & 12886 & 432$\pm^{ 127 }_{ 117 }$ & $1.00$ & 30.2698 & 5.00E+19 & 16.46 & 2.95\\ 
pg0003 & $0.42192$ (\#144)  & 120.23(94) & 13041 & 12843 & 378$\pm^{ 116 }_{ 97 }$ & $1.00$ & 30.7135 & 1.35E+06 & 16.25 & 0.26\\ 
pg0157 & $0.14621$ (\#145)  & 89.37(90) & 3707 & 3516 & 333$\pm^{ 101 }_{ 84 }$ & $1.00$ & 24.7581 & 5.00E+19 & 16.46 & 0.32\\ 
pg0804 & $0.00382$ (\#146)  & -- & -- & -- & -- & -- & 21.6825 & -- & -- & --\\ 
pg0804 & $0.01851$ (\#147)  & 16.80(23) & 29128 & nan & 945$\pm^{ 97 }_{ 92 }$ & $1.00$ & 21.9998 & 1.20 & 15.51 & 1.89\\ 
pg0804 & $0.10216$ (\#148)  & 79.20(62) & 28053 & 28091 & 1727$\pm^{ 87 }_{ 84 }$ & $1.00$ & 23.8067 & 1.96 & 15.64 & 0.11\\ 
pg0804 & $0.10230$ (\#149)  & 79.21(62) & 28053 & 28091 & 1728$\pm^{ 87 }_{ 84 }$ & $1.00$ & 23.8097 & 1.99 & 15.66 & 0.10\\ 
pg0832 & $0.10772$ (\#150)  & 80.67(64) & 20655 & 20637 & 76$\pm^{ 24 }_{ 21 }$ & $1.00$ & 23.9268 & 2.10 & 15.66 & 1.33\\ 
pg0832 & $0.13230$ (\#151)  & 108.67(84) & 20655 & 20637 & 61$\pm^{ 24 }_{ 19 }$ & $1.00$ & 24.4577 & 5.00E+19 & 16.46 & 0.01\\ 
pg0832 & $0.15276$ (\#152)  & 120.88(91) & 20654 & 20637 & 47$\pm^{ 21 }_{ 16 }$ & $1.00$ & 24.8996 & 5.00E+19 & 16.41 & 0.35\\ 
pg0832 & $0.23308$ (\#153)  & 129.97(95) & 20655 & 20637 & 82$\pm^{ 28 }_{ 23 }$ & $1.00$ & 26.6345 & 5.01E+03 & 16.12 & 0.58\\ 
pg0832 & $0.32567$ (\#154)  & 75.57(61) & 20656 & 20645 & 67$\pm^{ 36 }_{ 26 }$ & $1.00$ & 28.6345 & 5.00E+19 & 16.41 & 0.03\\ 
pg0953 & $0.01560$ (\#155)  & 28.56(26) & 12792 & nan & 420$\pm^{ 81 }_{ 73 }$ & $1.00$ & 21.9370 & 1.99 & 15.66 & 1.29\\ 
pg0953 & $0.05891$ (\#156)  & 62.59(44) & 12792 & nan & 452$\pm^{ 68 }_{ 62 }$ & $1.00$ & 22.8725 & 101.52 & 16.01 & 0.26\\ 
pg0953 & $0.06807$ (\#157)  & 48.31(41) & 12792 & nan & 546$\pm^{ 89 }_{ 74 }$ & $1.00$ & 23.0703 & 5.00E+19 & 16.46 & 3.12\\ 
pg0953 & $0.11827$ (\#158)  & 75.73(75) & 12792 & 12309 & 500$\pm^{ 67 }_{ 61 }$ & $1.00$ & 24.1546 & 45.85 & 16.00 & 0.02\\ 
pg0953 & $0.14236$ (\#159)  & 105.46(88) & 12786 & 12309 & 548$\pm^{ 75 }_{ 68 }$ & $1.00$ & 24.6750 & 0.77 & 15.36 & 5.66\\ 
pg0953 & $0.14263$ (\#160)  & 109.34(89) & 12785 & 12309 & 547$\pm^{ 74 }_{ 69 }$ & $1.00$ & 24.6808 & 0.70 & 15.33 & 5.97\\ 
pg0953 & $0.14307$ (\#161)  & 107.64(88) & 12785 & 12309 & 540$\pm^{ 74 }_{ 68 }$ & $1.00$ & 24.6903 & 0.69 & 15.32 & 6.36\\ 
pg0953 & $0.22967$ (\#162)  & 126.93(87) & 12777 & 12309 & 692$\pm^{ 88 }_{ 81 }$ & $1.00$ & 26.5609 & 1.09 & 15.48 & 2.87\\ 
pg0953 & $0.23251$ (\#163)  & 116.37(87) & 12777 & 12309 & 645$\pm^{ 85 }_{ 78 }$ & $1.00$ & 26.6222 & 0.91 & 15.42 & 4.37\\ 
pg0953 & $0.23351$ (\#164)  & 118.01(88) & 12777 & 12309 & 650$\pm^{ 85 }_{ 78 }$ & $1.00$ & 26.6438 & 1.15 & 15.50 & 2.94\\ 
pg1115 & $0.12285$ (\#165)  & 111.34(78) & 17510 & 16953 & 307$\pm^{ 48 }_{ 44 }$ & $1.00$ & 24.2536 & 5.00E+19 & 16.41 & 3.46\\ 
pg1115 & $0.12313$ (\#166)  & 110.77(77) & 17510 & 16953 & 298$\pm^{ 64 }_{ 43 }$ & $1.00$ & 24.2596 & 5.00E+19 & 16.46 & 1.57\\ 
pg1115 & $0.13104$ (\#167*)  & 126.82(83) & 17517 & 16953 & 303$\pm^{ 52 }_{ 47 }$ & $1.00$ & 24.4305 & 3.92E+05 & 16.21 & 0.14\\ 
pg1115 & $0.15456$ (\#168*)  & 137.20(89) & 17538 & 16953 & 351$\pm^{ 52 }_{ 48 }$ & $1.00$ & 24.9385 & 8.10 & 15.88 & 0.22\\ 
pg1115 & $0.15467$ (\#169*)  & 137.21(89) & 17538 & 16953 & 351$\pm^{ 53 }_{ 48 }$ & $1.00$ & 24.9409 & 7.30 & 15.88 & 0.21\\ 
pg1116 & $0.05900$ (\#170)  & 49.53(36) & 281330 & nan & 597$\pm^{ 19 }_{ 19 }$ & $1.00$ & 22.8744 & 10.62 & 15.93 & 2.02\\ 
pg1116 & $0.05927$ (\#171)  & 43.85(35) & 280940 & nan & 590$\pm^{ 19 }_{ 19 }$ & $1.00$ & 22.8802 & 13.33 & 15.91 & 1.62\\ 
pg1116 & $0.11895$ (\#172)  & 95.95(79) & 285653 & 287248 & 652$\pm^{ 16 }_{ 16 }$ & $1.00$ & 24.1693 & 0.62 & 15.28 & 0.50\\ 
pg1116 & $0.13852$ (\#173)  & 94.61(91) & 277702 & 291047 & 693$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.5920 & 2.05 & 15.65 & 2.43\\ 
pg1116 & $0.16539$ (\#174)  & 104.05(93) & 289660 & 291047 & 750$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.1724 & 1.55 & 15.58 & 1.66\\ 
pg1116 & $0.16554$ (\#175)  & 100.41(92) & 289658 & 290943 & 751$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.1757 & 1.69 & 15.61 & 2.12\\ 
pg1116 & $0.16610$ (\#176)  & 106.71(93) & 289658 & 291047 & 760$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.1878 & 2.23 & 15.67 & 3.04\\ 
pg1116 & $0.16686$ (\#177)  & 105.29(92) & 291239 & 290943 & 756$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.2042 & 2.43 & 15.70 & 3.07\\ 
pg1116 & $0.17343$ (\#178)  & 112.47(96) & 296094 & 285607 & 756$\pm^{ 18 }_{ 18 }$ & $1.00$ & 25.3461 & 1.29 & 15.52 & 0.98\\ 
pg1211 & $0.00711$ (\#179)  & -- & -- & -- & -- & -- & 21.7536 & -- & -- & --\\ 
pg1211 & $0.05117$ (\#180)  & 45.23(34) & 736547 & nan & 672$\pm^{ 13 }_{ 13 }$ & $1.00$ & 22.7053 & 1.89E+05 & 16.21 & 13.49\\ 
pg1211 & $0.06449$ (\#181)  & -- & -- & -- & -- & -- & 22.9930 & -- & -- & --\\ 
pg1211 & $0.06491$ (\#182)  & -- & -- & -- & -- & -- & 23.0021 & -- & -- & --\\ 
pg1216 & $0.12362$ (\#183)  & 106.86(78) & 11245 & 11258 & 185$\pm^{ 46 }_{ 40 }$ & $1.00$ & 24.2702 & 5.00E+19 & 16.41 & 4.18\\ 
pg1216 & $0.12389$ (\#184)  & 105.56(77) & 11245 & 11258 & 183$\pm^{ 66 }_{ 49 }$ & $1.00$ & 24.2760 & 5.00E+19 & 16.46 & 2.64\\ 
pg1216 & $0.12463$ (\#185)  & 107.31(78) & 11245 & 11258 & 187$\pm^{ 46 }_{ 40 }$ & $1.00$ & 24.2920 & 5.00E+19 & 16.46 & 2.41\\ 
pg1216 & $0.12485$ (\#186)  & 106.17(77) & 11245 & 11258 & 186$\pm^{ 46 }_{ 40 }$ & $1.00$ & 24.2968 & 5.00E+19 & 16.46 & 1.71\\ 
pg1216 & $0.13499$ (\#187)  & 116.72(86) & 11248 & 11258 & 192$\pm^{ 50 }_{ 43 }$ & $1.00$ & 24.5158 & 5.30E+12 & 16.36 & 0.06\\ 
pg1216 & $0.26768$ (\#188)  & 113.01(93) & 11258 & 11258 & 223$\pm^{ 67 }_{ 53 }$ & $1.00$ & 27.3819 & 5.00E+19 & 16.46 & 0.14\\ 
pg1216 & $0.28199$ (\#189)  & 112.68(89) & 11258 & 11258 & 237$\pm^{ 66 }_{ 56 }$ & $1.00$ & 27.6910 & 2.97 & 15.73 & 0.87\\ 
pg1216 & $0.28237$ (\#190)  & 112.03(88) & 11258 & 11258 & 245$\pm^{ 68 }_{ 57 }$ & $1.00$ & 27.6992 & 166.16 & 16.01 & 0.43\\ 
pg1259 & $0.00220$ (\#191)  & -- & -- & -- & -- & -- & 21.6475 & -- & -- & --\\ 
pg1259 & $0.00762$ (\#192)  & -- & -- & -- & -- & -- & 21.7646 & -- & -- & --\\ 
pg1259 & $0.02217$ (\#193)  & 31.57(30) & 11484 & nan & 172$\pm^{ 52 }_{ 46 }$ & $1.00$ & 22.0789 & 5.00E+19 & 16.46 & 0.12\\ 
pg1259 & $0.04606$ (\#194)  & 45.32(42) & 11485 & nan & 178$\pm^{ 51 }_{ 39 }$ & $1.00$ & 22.5949 & 5.00E+19 & 16.46 & 1.04\\ 
pg1259 & $0.04650$ (\#195)  & 43.77(42) & 11485 & nan & 188$\pm^{ 53 }_{ 41 }$ & $1.00$ & 22.6044 & 5.00E+19 & 16.46 & 1.02\\ 
pg1259 & $0.19576$ (\#196)  & 107.87(92) & 11483 & 11479 & 236$\pm^{ 54 }_{ 46 }$ & $1.00$ & 25.8284 & 13.59 & 15.92 & 0.42\\ 
pg1259 & $0.21940$ (\#197)  & 110.09(92) & 11483 & 11479 & 267$\pm^{ 65 }_{ 56 }$ & $1.00$ & 26.3390 & 1.56E+05 & 16.23 & 0.10\\ 
pg1259 & $0.21953$ (\#198)  & 110.10(92) & 11483 & 11479 & 267$\pm^{ 65 }_{ 56 }$ & $1.00$ & 26.3418 & 4.06E+06 & 16.24 & 0.09\\ 
pg1259 & $0.22313$ (\#199)  & 105.90(93) & 11483 & 11479 & 275$\pm^{ 64 }_{ 56 }$ & $1.00$ & 26.4196 & 3.12E+09 & 16.33 & 0.00\\ 
pg1259 & $0.23284$ (\#200)  & 120.10(95) & 11483 & 11479 & 235$\pm^{ 60 }_{ 51 }$ & $1.00$ & 26.6293 & 5.00E+19 & 16.46 & 1.29\\ 
pg1259 & $0.23956$ (\#201)  & 123.67(95) & 11483 & 11479 & 179$\pm^{ 54 }_{ 45 }$ & $1.00$ & 26.7745 & 1.17E+14 & 16.41 & 0.01\\ 
pg1259 & $0.25973$ (\#202)  & 111.65(93) & 11483 & 11479 & 126$\pm^{ 49 }_{ 39 }$ & $1.00$ & 27.2102 & 5.00E+19 & 16.46 & 0.83\\ 
pg1259 & $0.31979$ (\#203)  & 80.12(82) & 11483 & 11480 & 296$\pm^{ 92 }_{ 70 }$ & $1.00$ & 28.5075 & 5.00E+19 & 16.46 & 0.67\\ 
pg1259 & $0.32472$ (\#204)  & 90.97(82) & 11484 & 11480 & 337$\pm^{ 109 }_{ 77 }$ & $1.00$ & 28.6140 & 5.00E+19 & 16.46 & 2.56\\ 
pg1307 & $0.14187$ (\#205)  & 117.92(89) & 9837 & 9504 & 210$\pm^{ 60 }_{ 45 }$ & $1.00$ & 24.6644 & 5.00E+19 & 16.46 & 0.58\\ 
pg1307 & $0.14214$ (\#206)  & 117.74(88) & 9837 & 9504 & 211$\pm^{ 60 }_{ 46 }$ & $1.00$ & 24.6702 & 5.00E+19 & 16.46 & 0.69\\ 
pg1309 & $0.17586$ (\#207)  & 112.33(93) & 27265 & 26163 & 153$\pm^{ 28 }_{ 25 }$ & $1.00$ & 25.3986 & 5.00E+19 & 16.46 & 3.00\\ 
pg1309 & $0.17745$ (\#208)  & 117.17(95) & 27265 & 26163 & 150$\pm^{ 36 }_{ 25 }$ & $1.00$ & 25.4329 & 5.00E+19 & 16.41 & 1.76\\ 
pg1309 & $0.17866$ (\#209)  & 121.37(94) & 27265 & 26163 & 155$\pm^{ 35 }_{ 25 }$ & $1.00$ & 25.4591 & 5.00E+19 & 16.46 & 2.13\\ 
pg1309 & $0.17930$ (\#210)  & 120.67(95) & 27265 & 26163 & 156$\pm^{ 33 }_{ 26 }$ & $1.00$ & 25.4729 & 5.00E+19 & 16.46 & 1.89\\ 
pg1309 & $0.17979$ (\#211)  & 121.42(94) & 27265 & 26163 & 157$\pm^{ 29 }_{ 25 }$ & $1.00$ & 25.4835 & 5.00E+19 & 16.46 & 1.65\\ 
pg1309 & $0.18069$ (\#212)  & 121.63(94) & 27265 & 26163 & 147$\pm^{ 27 }_{ 25 }$ & $1.00$ & 25.5029 & 5.00E+19 & 16.46 & 0.54\\ 
pg1309 & $0.18117$ (\#213)  & 119.61(95) & 27265 & 26163 & 144$\pm^{ 29 }_{ 25 }$ & $1.00$ & 25.5133 & 5.00E+19 & 16.46 & 0.17\\ 
pg1309 & $0.18139$ (\#214)  & 116.87(93) & 27265 & 26163 & 141$\pm^{ 28 }_{ 24 }$ & $1.00$ & 25.5180 & 5.00E+19 & 16.41 & 0.10\\ 
pg1309 & $0.18145$ (\#215)  & 116.88(93) & 27265 & 26163 & 141$\pm^{ 29 }_{ 25 }$ & $1.00$ & 25.5193 & 5.00E+19 & 16.46 & 0.09\\ 
pg1309 & $0.18192$ (\#216)  & 114.96(94) & 27265 & 26163 & 145$\pm^{ 29 }_{ 25 }$ & $1.00$ & 25.5295 & 5.00E+19 & 16.46 & 0.06\\ 
pg1309 & $0.18698$ (\#217)  & 107.23(91) & 27265 & 26163 & 158$\pm^{ 35 }_{ 26 }$ & $1.00$ & 25.6388 & 5.00E+19 & 16.46 & 1.76\\ 
pg1444 & $0.22031$ (\#218)  & 113.67(93) & 17674 & 17137 & 183$\pm^{ 40 }_{ 35 }$ & $1.00$ & 26.3587 & 1.70 & 15.61 & 1.34\\ 
pg1444 & $0.22676$ (\#219)  & 127.72(94) & 17674 & 17137 & 179$\pm^{ 40 }_{ 35 }$ & $1.00$ & 26.4980 & 4.83E+12 & 16.39 & 0.03\\ 
pg1444 & $0.26690$ (\#220)  & 132.30(93) & 17674 & 17137 & 145$\pm^{ 39 }_{ 33 }$ & $1.00$ & 27.3650 & 1.11 & 15.48 & 3.41\\ 
pg1444 & $0.26728$ (\#221)  & 132.11(94) & 17674 & 17137 & 146$\pm^{ 40 }_{ 34 }$ & $1.00$ & 27.3732 & 1.16 & 15.50 & 3.67\\ 
pg1444 & $0.26738$ (\#222)  & 132.08(94) & 17674 & 17137 & 146$\pm^{ 40 }_{ 34 }$ & $1.00$ & 27.3754 & 1.01 & 15.44 & 3.70\\ 
pg1444 & $0.26747$ (\#223)  & 127.49(93) & 17674 & 17137 & 143$\pm^{ 39 }_{ 33 }$ & $1.00$ & 27.3774 & 0.97 & 15.43 & 4.74\\ 
pg1626 & $0.13075$ (\#224)  & 124.04(83) & 69157 & 68865 & 386$\pm^{ 48 }_{ 46 }$ & $1.00$ & 24.4242 & 0.76 & 15.35 & 4.32\\ 
phl1811 & $0.07344$ (\#225)  & -- & -- & -- & -- & -- & 23.1863 & -- & -- & --\\ 
phl1811 & $0.07768$ (\#226)  & -- & -- & -- & -- & -- & 23.2779 & -- & -- & --\\ 
phl1811 & $0.08131$ (\#227)  & -- & -- & -- & -- & -- & 23.3563 & -- & -- & --\\ 
phl1811 & $0.13239$ (\#228)  & -- & -- & -- & -- & -- & 24.4596 & -- & -- & --\\ 
phl1811 & $0.13282$ (\#229)  & -- & -- & -- & -- & -- & 24.4689 & -- & -- & --\\ 
phl1811 & $0.13318$ (\#230)  & -- & -- & -- & -- & -- & 24.4767 & -- & -- & --\\ 
phl1811 & $0.13545$ (\#231)  & -- & -- & -- & -- & -- & 24.5257 & -- & -- & --\\ 
phl1811 & $0.15752$ (\#232)  & -- & -- & -- & -- & -- & 25.0024 & -- & -- & --\\ 
phl1811 & $0.15786$ (\#233)  & -- & -- & -- & -- & -- & 25.0098 & -- & -- & --\\ 
phl1811 & $0.17652$ (\#234)  & 118.26(84) & 79254 & 77556 & 35$\pm^{ 12 }_{ 11 }$ & $1.00$ & 25.4128 & 5.00E+19 & 16.46 & 1.08\\ 
phl1811 & $0.19157$ (\#235*)  & 164.17(89) & 79254 & 76738 & 35$\pm^{ 13 }_{ 11 }$ & $1.00$ & 25.7379 & 5.00E+19 & 16.41 & 0.13\\ 
phl1811 & $0.19194$ (\#236*)  & 167.21(88) & 79254 & 76682 & 34$\pm^{ 13 }_{ 11 }$ & $1.00$ & 25.7459 & 5.00E+19 & 16.46 & 0.06\\ 
phl1811 & $0.19220$ (\#237*)  & 167.23(88) & 79254 & 76682 & 34$\pm^{ 12 }_{ 11 }$ & $1.00$ & 25.7515 & 5.00E+19 & 16.46 & 0.03\\ 
pks0312 & $0.20188$ (\#238)  & 93.47(64) & 23858 & 22982 & 161$\pm^{ 40 }_{ 35 }$ & $1.00$ & 25.9606 & 5.00E+19 & 16.41 & 1.94\\ 
pks0312 & $0.20275$ (\#239*)  & 99.01(66) & 23858 & 22982 & 154$\pm^{ 39 }_{ 33 }$ & $1.00$ & 25.9794 & 5.00E+19 & 16.41 & 1.41\\ 
pks0405 & $0.09192$ (\#240)  & 67.08(46) & 137245 & nan & 358$\pm^{ 19 }_{ 18 }$ & $1.00$ & 23.5855 & 1.98 & 15.64 & 0.13\\ 
pks0405 & $0.09647$ (\#241)  & 69.21(48) & 135771 & 138649 & 361$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.6838 & 1.15 & 15.49 & 0.98\\ 
pks0405 & $0.14808$ (\#242)  & 88.65(90) & 136323 & 137234 & 373$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.7985 & 1.54 & 15.59 & 0.23\\ 
pks0405 & $0.16566$ (\#243)  & 79.70(91) & 137140 & 137234 & 394$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.1783 & 156.92 & 16.03 & 1.67\\ 
pks0405 & $0.16606$ (\#244)  & 79.75(92) & 136407 & 137234 & 395$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.1869 & 116.44 & 16.04 & 1.78\\ 
pks0405 & $0.16659$ (\#245)  & 78.27(91) & 137924 & 137234 & 394$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.1983 & 386.26 & 16.04 & 2.01\\ 
pks0405 & $0.16688$ (\#246)  & 78.15(91) & 137924 & 137234 & 395$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.2046 & 136.55 & 16.07 & 2.16\\ 
pks0405 & $0.16712$ (\#247)  & 83.54(92) & 137941 & 137234 & 391$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.2098 & 324.91 & 16.07 & 2.15\\ 
pks0405 & $0.18257$ (\#248)  & 113.72(95) & 137986 & 136490 & 365$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.5435 & 1.46 & 15.57 & 0.17\\ 
pks0405 & $0.18289$ (\#249)  & 114.40(96) & 138000 & 136490 & 365$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.5504 & 1.75 & 15.61 & 0.05\\ 
pks0405 & $0.24052$ (\#250)  & 109.18(95) & 137976 & 138647 & 413$\pm^{ 23 }_{ 22 }$ & $1.00$ & 26.7952 & 527.04 & 16.06 & 1.03\\ 
pks0405 & $0.24094$ (\#251)  & 104.97(95) & 137961 & 138647 & 410$\pm^{ 23 }_{ 22 }$ & $1.00$ & 26.8043 & 769.41 & 16.09 & 1.15\\ 
pks0405 & $0.24547$ (\#252)  & 98.26(94) & 136439 & 138647 & 386$\pm^{ 23 }_{ 23 }$ & $1.00$ & 26.9022 & 1.12 & 15.49 & 0.69\\ 
pks0405 & $0.29762$ (\#253)  & 98.20(89) & 135766 & 137130 & 382$\pm^{ 27 }_{ 26 }$ & $1.00$ & 28.0286 & 2.36 & 15.69 & 0.02\\ 
pks0405 & $0.34188$ (\#254)  & 98.93(90) & 136321 & 138714 & 379$\pm^{ 29 }_{ 28 }$ & $1.00$ & 28.9846 & 1.62 & 15.60 & 0.90\\ 
pks0405 & $0.34225$ (\#255)  & 98.19(90) & 136322 & 138714 & 381$\pm^{ 29 }_{ 28 }$ & $1.00$ & 28.9926 & 1.36 & 15.54 & 1.22\\ 
pks0405 & $0.35092$ (\#256)  & 86.77(91) & 136325 & 138714 & 392$\pm^{ 32 }_{ 31 }$ & $1.00$ & 29.1799 & 9.75E+08 & 16.29 & 2.55\\ 
pks0405 & $0.36075$ (\#257)  & 90.38(93) & 137923 & 138714 & 385$\pm^{ 33 }_{ 32 }$ & $1.00$ & 29.3922 & 5.90E+08 & 16.29 & 2.11\\ 
pks0405 & $0.36151$ (\#258)  & 92.10(93) & 137923 & 138714 & 376$\pm^{ 32 }_{ 32 }$ & $1.00$ & 29.4086 & 7.14E+04 & 16.21 & 1.10\\ 
pks0405 & $0.36329$ (\#259)  & 96.83(94) & 138708 & 138714 & 363$\pm^{ 32 }_{ 31 }$ & $1.00$ & 29.4471 & 2.23 & 15.68 & 0.16\\ 
pks0405 & $0.40570$ (\#260)  & 120.73(84) & 137132 & 133905 & 452$\pm^{ 35 }_{ 34 }$ & $1.00$ & 30.3631 & 1.13E+06 & 16.24 & 0.79\\ 
pks0405 & $0.40890$ (\#261)  & 110.16(86) & 137167 & 134014 & 491$\pm^{ 42 }_{ 35 }$ & $1.00$ & 30.4322 & 5.00E+19 & 16.46 & 6.95\\ 
pks0405 & $0.49505$ (\#262)  & 112.27(94) & 138729 & 137202 & 536$\pm^{ 45 }_{ 43 }$ & $1.00$ & 32.2931 & 0.74 & 15.34 & 3.45\\ 
pks0405 & $0.49530$ (\#263)  & 108.35(92) & 138729 & 137169 & 528$\pm^{ 45 }_{ 43 }$ & $1.00$ & 32.2985 & 0.84 & 15.40 & 4.18\\ 
pks0405 & $0.55506$ (\#264)  & 104.58(82) & 132269 & 134976 & 444$\pm^{ 57 }_{ 54 }$ & $1.00$ & 33.5893 & 5.00E+19 & 16.41 & 2.35\\ 
pks2005 & $0.06490$ (\#265)  & 59.89(42) & 53473 & nan & 2202$\pm^{ 73 }_{ 71 }$ & $1.00$ & 23.0018 & 0.93 & 15.42 & 0.74\\ 
pks2155 & $0.05405$ (\#266)  & -- & -- & -- & -- & -- & 22.7675 & -- & -- & --\\ 
pks2155 & $0.05707$ (\#267)  & 20.80(28) & 1697089 & nan & 679$\pm^{ 108 }_{ 82 }$ & $4.85$ & 22.8327 & 0.12 & 14.64 & 5.24\\ 
q0045 & $0.11052$ (\#268)  & -- & -- & -- & -- & -- & 23.9872 & -- & -- & --\\ 
q0045 & $0.13521$ (\#269)  & -- & -- & -- & -- & -- & 24.5205 & -- & -- & --\\ 
q1230 & $0.09518$ (\#270)  & 63.84(48) & 39335 & 39139 & 112$\pm^{ 23 }_{ 20 }$ & $1.00$ & 23.6559 & 5.00E+19 & 16.46 & 0.60\\ 
q1230 & $0.10318$ (\#271)  & 59.80(44) & 39335 & 39139 & 93$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.8287 & 1.68 & 15.61 & 2.91\\ 
q1230 & $0.10445$ (\#272)  & 62.04(47) & 39335 & 39139 & 100$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.8561 & 2.27 & 15.69 & 1.45\\ 
q1230 & $0.10530$ (\#273)  & 62.81(47) & 39335 & 39139 & 106$\pm^{ 27 }_{ 24 }$ & $1.00$ & 23.8745 & 9.63E+03 & 16.12 & 0.34\\ 
q1230 & $0.10596$ (\#274)  & 63.04(47) & 39335 & 39139 & 111$\pm^{ 27 }_{ 24 }$ & $1.00$ & 23.8887 & 1.15E+08 & 16.35 & 0.01\\ 
q1230 & $0.10666$ (\#275)  & 63.05(47) & 39335 & 39139 & 113$\pm^{ 26 }_{ 24 }$ & $1.00$ & 23.9039 & 1.65E+16 & 16.45 & 0.00\\ 
q1230 & $0.10809$ (\#276)  & 59.85(45) & 39335 & 39139 & 103$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9347 & 5.00E+19 & 16.43 & 0.06\\ 
q1230 & $0.10820$ (\#277)  & 62.54(45) & 39335 & 39139 & 103$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9371 & 5.00E+19 & 16.43 & 0.08\\ 
q1230 & $0.10861$ (\#278)  & 59.64(45) & 39335 & 39139 & 105$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9460 & 5.00E+19 & 16.46 & 0.10\\ 
q1230 & $0.10906$ (\#279)  & 61.31(47) & 39335 & 39139 & 101$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9557 & 1.17E+16 & 16.45 & 0.20\\ 
q1230 & $0.10935$ (\#280)  & 61.34(47) & 39335 & 39139 & 102$\pm^{ 26 }_{ 23 }$ & $1.00$ & 23.9620 & 5.00E+19 & 16.46 & 0.16\\ 
q1230 & $0.10956$ (\#281)  & 61.25(46) & 39335 & 39139 & 107$\pm^{ 27 }_{ 24 }$ & $1.00$ & 23.9665 & 5.00E+19 & 16.41 & 0.07\\ 
q1230 & $0.11707$ (\#282)  & 70.22(56) & 39335 & 39139 & 120$\pm^{ 31 }_{ 23 }$ & $1.00$ & 24.1287 & 5.00E+19 & 16.46 & 1.38\\ 
q1230 & $0.11743$ (\#283)  & 71.60(58) & 39335 & 39139 & 121$\pm^{ 30 }_{ 24 }$ & $1.00$ & 24.1365 & 5.00E+19 & 16.44 & 1.25\\ 
q1230 & $0.11781$ (\#284)  & 71.89(58) & 39335 & 39139 & 120$\pm^{ 26 }_{ 23 }$ & $1.00$ & 24.1447 & 5.00E+19 & 16.46 & 0.91\\ 
rbs1892 & $0.15752$ (\#285)  & 86.45(91) & 4935 & 4865 & 220$\pm^{ 84 }_{ 67 }$ & $1.00$ & 25.0024 & 4.32 & 15.80 & 0.66\\ 
rbs1892 & $0.17133$ (\#286)  & 86.80(94) & 4937 & 4865 & 309$\pm^{ 139 }_{ 95 }$ & $1.00$ & 25.3007 & 5.00E+19 & 16.46 & 2.67\\ 
rbs1892 & $0.19874$ (\#287)  & 104.23(94) & 4937 & 4849 & 500$\pm^{ 129 }_{ 110 }$ & $1.00$ & 25.8928 & 6.72E+10 & 16.36 & 0.06\\ 
rbs542 & $0.10323$ (\#288)  & 86.68(64) & 192553 & 181905 & 1543$\pm^{ 32 }_{ 31 }$ & $1.00$ & 23.8298 & 1.01 & 15.46 & 0.16\\ 
rbs542 & $0.10379$ (\#289)  & 87.77(65) & 192488 & 181905 & 1551$\pm^{ 32 }_{ 32 }$ & $1.00$ & 23.8419 & 1.30 & 15.52 & 0.52\\ 
rxj0439 & $0.11547$ (\#290)  & 95.23(74) & 148931 & 151265 & 506$\pm^{ 20 }_{ 20 }$ & $1.00$ & 24.0942 & 1.86 & 15.63 & -0.00\\ 
rxj0439 & $0.21833$ (\#291)  & 118.05(95) & 147527 & 149811 & 588$\pm^{ 27 }_{ 26 }$ & $1.00$ & 26.3159 & 10.59 & 15.92 & 1.26\\ 
rxj0439 & $0.24235$ (\#292)  & 94.71(94) & 148524 & 152414 & 592$\pm^{ 28 }_{ 27 }$ & $1.00$ & 26.8348 & 22.37 & 15.94 & 0.81\\ 
rxj0439 & $0.24258$ (\#293)  & 103.01(95) & 147411 & 152414 & 590$\pm^{ 28 }_{ 27 }$ & $1.00$ & 26.8397 & 15.08 & 15.95 & 0.92\\ 
rxj0439 & $0.24313$ (\#294)  & 94.82(94) & 147411 & 152414 & 592$\pm^{ 28 }_{ 27 }$ & $1.00$ & 26.8516 & 5.89 & 15.85 & 0.50\\ 
rxj0439 & $0.24387$ (\#295)  & 93.90(94) & 147412 & 152414 & 593$\pm^{ 29 }_{ 27 }$ & $1.00$ & 26.8676 & 2.17 & 15.66 & 0.04\\ 
s50716 & $0.23145$ (\#296)  & 93.47(94) & 75297 & 76133 & 887$\pm^{ 42 }_{ 41 }$ & $1.00$ & 26.5993 & 1.61 & 15.59 & 0.03\\ 
ton28 & $0.13746$ (\#297)  & 111.07(90) & 83595 & 86028 & 225$\pm^{ 23 }_{ 21 }$ & $1.00$ & 24.5691 & 1.75E+03 & 16.13 & 0.16\\ 
ton28 & $0.13773$ (\#298)  & 110.95(90) & 83595 & 86028 & 227$\pm^{ 22 }_{ 22 }$ & $1.00$ & 24.5750 & 1.91E+04 & 16.15 & 0.30\\ 
ton28 & $0.13781$ (\#299)  & 111.91(90) & 83595 & 86028 & 227$\pm^{ 23 }_{ 22 }$ & $1.00$ & 24.5767 & 3.51E+04 & 16.17 & 0.35\\ 
ton28 & $0.17251$ (\#300)  & 98.29(95) & 86114 & 85104 & 203$\pm^{ 19 }_{ 18 }$ & $1.00$ & 25.3262 & 0.91 & 15.42 & 2.67\\ 
ton28 & $0.21259$ (\#301)  & 116.22(89) & 84885 & 83740 & 193$\pm^{ 24 }_{ 22 }$ & $1.00$ & 26.1919 & 351.23 & 16.09 & 0.06\\ 
ton28 & $0.24292$ (\#302)  & 105.70(82) & 83762 & 86136 & 178$\pm^{ 26 }_{ 24 }$ & $1.00$ & 26.8471 & 1.43 & 15.56 & 1.35\\ 
ton28 & $0.24859$ (\#303*)  & 126.01(83) & 83842 & 86136 & 232$\pm^{ 28 }_{ 26 }$ & $1.00$ & 26.9695 & 2.48 & 15.69 & 0.31\\ 
ton28 & $0.27338$ (\#304)  & 112.36(81) & 83758 & 86136 & 267$\pm^{ 32 }_{ 30 }$ & $1.00$ & 27.5050 & 1.00 & 15.44 & 2.14\\ 
ton28 & $0.33021$ (\#305)  & 117.99(85) & 83660 & 84983 & 277$\pm^{ 37 }_{ 34 }$ & $1.00$ & 28.7325 & 85.98 & 16.00 & 0.08\\ 
tons180 & $0.02340$ (\#306)  & 40.94(32) & 193565 & nan & 1151$\pm^{ 32 }_{ 30 }$ & $1.00$ & 22.1054 & 1.89 & 15.64 & 0.73\\ 
tons180 & $0.04360$ (\#307)  & 48.00(45) & 180786 & nan & 1149$\pm^{ 28 }_{ 27 }$ & $1.00$ & 22.5418 & 1.23 & 15.50 & 0.10\\ 
tons180 & $0.04560$ (\#308)  & 39.89(45) & 180786 & nan & 1198$\pm^{ 28 }_{ 27 }$ & $1.00$ & 22.5850 & 2.39E+03 & 16.12 & 14.42\\

\hline
\hline
\end{longtable}
\end{landscape}

==> Tables/XMM/Latex/xmm_o8_hi_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllllll|l}
\caption[\xmm\ Data, \oviii\ With \hi\ Priors Results (Full)]{\oviii\ measurements with \xmm\ data, at the prior redshift from the \hi\ lines from Table~\ref{tab:hiPriorsTable}.}
\label{tab:xmmhioviii}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & \multicolumn{2}{c}{RGS1} & \multicolumn{2}{c}{RGS2} & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \% & avg exp (s) & \%  & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.13714$ (\#1)  & -- & -- & -- & -- & -- & -- & -- & 21.5602 & -- & -- & --\\ 
1es1028 & $0.20383$ (\#2)  & 62.35(44) & 146640 & 9 & nan & nan & 1006$\pm^{ 29 }_{ 29 }$ & $1.00$ & 22.8246 & $ 0.05\pm^{ 2.21 }_{ 0.94 }$ & $ 14.58\pm^{ 1.44 }_{ nan }$ & 0.01\\ 
1es1028 & $0.22121$ (\#3)  & 57.62(42) & 144940 & 9 & nan & nan & 1031$\pm^{ 32 }_{ 31 }$ & $1.00$ & 23.1541 & $ -1.47\pm^{ 0.70 }_{ 0.53 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.89\\ 
1es1553 & $0.03466$ (\#4)  & 90.75(81) & 1722815 & 7 & 1780022 & 7 & 752$\pm^{ 116 }_{ 96 }$ & $2.09$ & 19.6172 & $ -0.03\pm^{ 0.65 }_{ 0.06 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.41\\ 
1es1553 & $0.04273$ (\#5)  & 89.06(72) & 1720386 & 8 & 1774803 & 7 & 776$\pm^{ 127 }_{ 108 }$ & $2.01$ & 19.7702 & $ 0.08\pm^{ 0.18 }_{ 0.21 }$ & $ 14.82\pm^{ 0.47 }_{ nan }$ & 0.14\\ 
1es1553 & $0.06364$ (\#6)  & 46.18(56) & 1785421 & 8 & 1740261 & 7 & 1161$\pm^{ 253 }_{ 220 }$ & $1.18$ & 20.1666 & $ 0.07\pm^{ 0.22 }_{ 0.32 }$ & $ 14.72\pm^{ 0.61 }_{ nan }$ & -0.04\\ 
1es1553 & $0.21869$ (\#7)  & 36.89(28) & 1666450 & 9 & nan & nan & 36$\pm^{ 20 }_{ 13 }$ & $7.01$ & 23.1064 & $ -0.43\pm^{ 0.30 }_{ 0.26 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.52\\ 
3c249 & $0.13470$ (\#8)  & -- & -- & -- & -- & -- & -- & -- & 21.5139 & -- & -- & --\\ 
3c249 & $0.26664$ (\#9)  & 53.79(69) & 2644 & 23 & 2524 & 18 & 320$\pm^{ 120 }_{ 95 }$ & $1.00$ & 24.0155 & $ 1.16E+13\pm^{ 1.00E+20 }_{ 1.16E+13 }$ & $ 16.75\pm^{ 0.05 }_{ inf }$ & 1.35\\ 
3c273 & $0.00758$ (\#10)  & 83.67(67) & 1048814 & 3 & 1012144 & 3 & 3696$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1037 & $ 0.04\pm^{ 0.42 }_{ 0.05 }$ & $ 14.45\pm^{ 1.06 }_{ nan }$ & 0.77\\ 
3c273 & $0.06707$ (\#11)  & 77.60(60) & 1015660 & 4 & 1019511 & 4 & 3919$\pm^{ 16 }_{ 16 }$ & $1.00$ & 20.2316 & $ -0.04\pm^{ 0.44 }_{ 0.08 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.35\\ 
3c273 & $0.07359$ (\#12)  & 63.12(54) & 922775 & 4 & 1018570 & 4 & 3920$\pm^{ 17 }_{ 16 }$ & $1.00$ & 20.3553 & $ -0.03\pm^{ 0.41 }_{ 0.09 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.21\\ 
3c273 & $0.13960$ (\#13)  & -- & -- & -- & -- & -- & -- & -- & 21.6068 & -- & -- & --\\ 
h1821 & $0.00944$ (\#14)  & 120.55(98) & 30556 & 35 & 43312 & 33 & 1002$\pm^{ 55 }_{ 53 }$ & $1.00$ & 19.1390 & $ -0.92\pm^{ 1.21 }_{ 0.70 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.86\\ 
h1821 & $0.06779$ (\#15)  & 81.53(61) & 31940 & 36 & 43282 & 34 & 1055$\pm^{ 61 }_{ 60 }$ & $1.00$ & 20.2453 & $ -0.65\pm^{ 3.61 }_{ 1.09 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.15\\ 
h1821 & $0.08483$ (\#16)  & 49.50(43) & 30565 & 41 & nan & nan & 1106$\pm^{ 71 }_{ 68 }$ & $1.00$ & 20.5684 & $ -1.02\pm^{ 2.54 }_{ 0.94 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.43\\ 
h1821 & $0.12147$ (\#17)  & 44.27(31) & 30928 & 49 & nan & nan & 1128$\pm^{ 97 }_{ 95 }$ & $1.00$ & 21.2631 & $ -0.74\pm^{ 6.44 }_{ 1.40 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.14\\ 
h1821 & $0.19817$ (\#18)  & 63.03(48) & 30824 & 55 & nan & nan & 974$\pm^{ 88 }_{ 85 }$ & $1.00$ & 22.7173 & $ -2.05\pm^{ 2.15 }_{ 0.88 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.17\\ 
h1821 & $0.21321$ (\#19)  & 58.22(45) & 29048 & 55 & nan & nan & 1010$\pm^{ 95 }_{ 92 }$ & $1.00$ & 23.0025 & $ -1.40\pm^{ 5.08 }_{ 1.10 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.40\\ 
h1821 & $0.24531$ (\#20)  & 69.92(50) & 31312 & 54 & 36214 & 40 & 1107$\pm^{ 101 }_{ 88 }$ & $1.00$ & 23.6111 & $ 9.21\pm^{ 7.55E+13 }_{ 10.06 }$ & $ 16.24\pm^{ 0.52 }_{ nan }$ & 0.61\\ 
h2356 & $0.03830$ (\#21)  & 97.28(88) & 479869 & 6 & 503477 & 6 & 1019$\pm^{ 12 }_{ 13 }$ & $1.00$ & 19.6862 & $ 0.40\pm^{ 0.47 }_{ 0.45 }$ & $ 15.47\pm^{ 0.28 }_{ nan }$ & 1.03\\ 
h2356 & $0.07881$ (\#22)  & 54.41(41) & 506719 & 6 & 263751 & 5 & 1072$\pm^{ 15 }_{ 15 }$ & $1.00$ & 20.4542 & $ -0.54\pm^{ 0.45 }_{ 0.35 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.77\\ 
h2356 & $0.10467$ (\#23)  & 43.81(39) & 507154 & 6 & nan & nan & 1072$\pm^{ 16 }_{ 15 }$ & $1.00$ & 20.9445 & $ -0.74\pm^{ 0.38 }_{ 0.31 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.88\\ 
h2356 & $0.15613$ (\#24)  & 37.69(29) & 503603 & 7 & nan & nan & 1088$\pm^{ 19 }_{ 18 }$ & $1.00$ & 21.9202 & $ 0.05\pm^{ 0.64 }_{ 0.62 }$ & $ 14.56\pm^{ 1.10 }_{ nan }$ & -0.01\\ 
he0226 & $0.14274$ (\#25)  & -- & -- & -- & -- & -- & -- & -- & 21.6664 & -- & -- & --\\ 
he0226 & $0.39890$ (\#26)  & 130.12(94) & 31707 & 25 & 31704 & 28 & 265$\pm^{ 37 }_{ 34 }$ & $1.00$ & 26.5231 & $ -1.60\pm^{ 3.61 }_{ 1.31 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.53\\ 
he0226 & $0.41024$ (\#27)  & 136.42(96) & 31707 & 25 & 31704 & 32 & 274$\pm^{ 38 }_{ 35 }$ & $1.00$ & 26.7382 & $ -1.81\pm^{ 2.41 }_{ 0.97 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.89\\ 
i22456 & $0.00443$ (\#28)  & 130.08(99) & 76706 & 53 & 81909 & 47 & 381$\pm^{ 22 }_{ 21 }$ & $1.00$ & 19.0440 & $ -2.01\pm^{ 0.61 }_{ 0.44 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.46\\ 
i22456 & $0.09941$ (\#29)  & 59.72(44) & 79900 & 60 & nan & nan & 501$\pm^{ 38 }_{ 27 }$ & $1.00$ & 20.8448 & $ 3.13E+04\pm^{ 1.00E+20 }_{ 3.13E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 4.43\\ 
mr2251 & $0.01068$ (\#30)  & 121.16(93) & 414226 & 5 & 451165 & 5 & 1243$\pm^{ 275 }_{ 224 }$ & $1.52$ & 19.1625 & $ -0.67\pm^{ 0.22 }_{ 0.20 }$ & $ nan\pm^{ nan }_{ nan }$ & 9.71\\ 
mr2251 & $0.01449$ (\#31)  & 122.62(90) & 428129 & 5 & 462131 & 5 & 1173$\pm^{ 252 }_{ 199 }$ & $1.69$ & 19.2347 & $ 0.07\pm^{ 0.39 }_{ 0.25 }$ & $ 14.74\pm^{ 0.78 }_{ nan }$ & 0.13\\ 
mr2251 & $0.06131$ (\#32)  & 68.20(47) & 466085 & 5 & 461291 & 5 & 2234$\pm^{ 1198 }_{ 730 }$ & $0.41$ & 20.1224 & $ 1.29\pm^{ 1.11 }_{ 0.72 }$ & $ 15.86\pm^{ 0.16 }_{ 0.28 }$ & 5.66\\ 
mr2251 & $0.06190$ (\#33)  & 62.95(47) & 466085 & 5 & 461291 & 5 & 2211$\pm^{ 1157 }_{ 717 }$ & $0.45$ & 20.1336 & $ 3.43\pm^{ 2.87 }_{ 1.58 }$ & $ 16.10\pm^{ 0.10 }_{ 0.14 }$ & 16.53\\ 
mr2251 & $0.06276$ (\#34)  & 50.87(49) & 466106 & 5 & 461162 & 4 & 2612$\pm^{ 1875 }_{ 645 }$ & $0.13$ & 20.1499 & $ 24.01\pm^{ 44.38 }_{ 15.19 }$ & $ 16.30\pm^{ 0.05 }_{ 0.08 }$ & 38.86\\ 
mr2251 & $0.06327$ (\#35)  & 44.88(49) & 466112 & 5 & 461008 & 4 & 2740$\pm^{ 1569 }_{ 769 }$ & $0.03$ & 20.1596 & $ 30.33\pm^{ 110.01 }_{ 19.55 }$ & $ 16.32\pm^{ 0.04 }_{ 0.07 }$ & 45.67\\ 
mr2251 & $0.06381$ (\#36)  & 45.72(49) & 466112 & 5 & 461008 & 4 & 2376$\pm^{ 1389 }_{ 647 }$ & $0.33$ & 20.1698 & $ 19.77\pm^{ 318.94 }_{ 11.43 }$ & $ 16.31\pm^{ 0.07 }_{ 0.07 }$ & 45.47\\ 
mrk478 & $0.06166$ (\#37)  & 76.63(64) & 202266 & 13 & 202111 & 12 & 465$\pm^{ 14 }_{ 14 }$ & $1.00$ & 20.1291 & $ -0.09\pm^{ 1.95 }_{ 0.94 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
mrk478 & $0.06578$ (\#38)  & 70.27(61) & 204255 & 14 & 201677 & 12 & 472$\pm^{ 14 }_{ 15 }$ & $1.00$ & 20.2072 & $ 0.13\pm^{ 2.23 }_{ 1.06 }$ & $ 15.00\pm^{ 1.02 }_{ nan }$ & -0.00\\ 
mrk478 & $0.07213$ (\#39)  & 54.18(51) & 200098 & 13 & 200301 & 12 & 492$\pm^{ 16 }_{ 15 }$ & $1.00$ & 20.3276 & $ 3.42\pm^{ 129.59 }_{ 3.09 }$ & $ 16.09\pm^{ 0.25 }_{ 0.71 }$ & 1.94\\ 
mrk876 & $0.01159$ (\#40)  & 84.83(96) & 2656 & 58 & 2600 & 11 & 174$\pm^{ 70 }_{ 54 }$ & $1.00$ & 19.1797 & $ 8.15E+07\pm^{ 1.00E+20 }_{ 8.15E+07 }$ & $ 16.62\pm^{ 0.12 }_{ -0.12 }$ & 0.81\\ 
mrk876 & $0.05598$ (\#41)  & 59.57(72) & 2736 & 34 & 2708 & 18 & 227$\pm^{ 89 }_{ 64 }$ & $1.00$ & 20.0214 & $ 4.30E+04\pm^{ 1.00E+20 }_{ 4.30E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 0.48\\ 
mrk876 & $0.08709$ (\#42)  & 42.06(43) & 2804 & 10 & nan & nan & 414$\pm^{ 119 }_{ 103 }$ & $1.00$ & 20.6112 & $ -4.18\pm^{ 1.43 }_{ 1.00 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.24\\ 
mrk876 & $0.08858$ (\#43)  & 42.31(44) & 2805 & 10 & nan & nan & 419$\pm^{ 123 }_{ 105 }$ & $1.00$ & 20.6395 & $ -4.01\pm^{ 1.48 }_{ 0.99 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.77\\ 
mrk876 & $0.08917$ (\#44)  & 42.90(43) & 2804 & 10 & nan & nan & 427$\pm^{ 125 }_{ 107 }$ & $1.00$ & 20.6507 & $ -3.76\pm^{ 1.65 }_{ 1.00 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.96\\ 
mrk876 & $0.11487$ (\#45)  & 52.10(37) & 2790 & 15 & nan & nan & 714$\pm^{ 237 }_{ 160 }$ & $1.00$ & 21.1379 & $ 5.33E+09\pm^{ 1.00E+20 }_{ 5.33E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 3.07\\ 
ngc7469 & $0.00981$ (\#46)  & 85.67(65) & 629599 & 4 & 665412 & 4 & 1934$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1460 & $ 2.83\pm^{ 1.01 }_{ 0.77 }$ & $ 16.06\pm^{ 0.06 }_{ 0.07 }$ & 51.59\\ 
pg0003 & $0.08299$ (\#47)  & 56.55(41) & 13036 & 36 & nan & nan & 169$\pm^{ 41 }_{ 36 }$ & $1.00$ & 20.5335 & $ -2.19\pm^{ 8.22E+03 }_{ 1.87 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.31\\ 
pg0003 & $0.17139$ (\#48)  & 45.45(37) & 13036 & 24 & nan & nan & 315$\pm^{ 63 }_{ 56 }$ & $1.00$ & 22.2096 & $ -0.59\pm^{ 1.00E+20 }_{ 2.38 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pg0003 & $0.22541$ (\#49)  & 47.36(42) & 13037 & 29 & nan & nan & 145$\pm^{ 50 }_{ 43 }$ & $1.00$ & 23.2338 & $ -4.47\pm^{ 1.05 }_{ 0.87 }$ & $ nan\pm^{ nan }_{ nan }$ & 8.09\\ 
pg0003 & $0.38633$ (\#50)  & 107.06(92) & 13033 & 32 & 12857 & 29 & 248$\pm^{ 69 }_{ 50 }$ & $1.00$ & 26.2848 & $ 1.54E+07\pm^{ 1.00E+20 }_{ 1.54E+07 }$ & $ 16.62\pm^{ 0.17 }_{ nan }$ & 1.31\\ 
pg0003 & $0.42051$ (\#51)  & 129.11(93) & 13034 & 47 & 12830 & 27 & 327$\pm^{ 75 }_{ 64 }$ & $1.00$ & 26.9329 & $ 1.24E+04\pm^{ 1.00E+20 }_{ 1.24E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 0.73\\ 
pg0804 & $0.05015$ (\#52)  & 80.99(78) & 28468 & 6 & 30600 & 4 & 1084$\pm^{ 53 }_{ 49 }$ & $1.00$ & 19.9108 & $ -0.03\pm^{ 3.38 }_{ 1.16 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pg0804 & $0.05576$ (\#53)  & 70.57(71) & 28779 & 6 & 30600 & 5 & 1101$\pm^{ 55 }_{ 53 }$ & $1.00$ & 20.0172 & $ 10.40\pm^{ 1.46E+04 }_{ 40.40 }$ & $ 16.22\pm^{ 0.26 }_{ nan }$ & 1.53\\ 
pg0804 & $0.36379$ (\#54)  & 131.95(97) & 30110 & 7 & 29227 & 6 & 1657$\pm^{ 86 }_{ 84 }$ & $1.00$ & 25.8575 & $ -1.38\pm^{ 1.07 }_{ 0.72 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.74\\ 
pg0832 & $0.01753$ (\#55)  & -- & -- & -- & -- & -- & -- & -- & 19.2924 & -- & -- & --\\ 
pg0832 & $0.02793$ (\#56)  & -- & -- & -- & -- & -- & -- & -- & 19.4896 & -- & -- & --\\ 
pg0832 & $0.08748$ (\#57)  & 59.08(42) & 20650 & 99 & nan & nan & 41$\pm^{ 16 }_{ 12 }$ & $1.00$ & 20.6186 & $ 2.35E+06\pm^{ 1.00E+20 }_{ 2.35E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 0.57\\ 
pg0832 & $0.10171$ (\#58)  & 53.76(42) & 20652 & 78 & nan & nan & 29$\pm^{ 15 }_{ 12 }$ & $1.00$ & 20.8884 & $ -4.03\pm^{ 2.72 }_{ 1.45 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.81\\ 
pg0832 & $0.18391$ (\#59)  & 40.73(29) & 20654 & 138 & nan & nan & 36$\pm^{ 22 }_{ 16 }$ & $1.00$ & 22.4469 & $ -4.07\pm^{ 3.66 }_{ 1.66 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.60\\ 
pg0832 & $0.27503$ (\#60)  & 100.19(76) & 20655 & 80 & 20637 & 113 & 76$\pm^{ 24 }_{ 20 }$ & $1.00$ & 24.1746 & $ -1.15\pm^{ 6.74E+13 }_{ 28.85 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
pg0832 & $0.27694$ (\#61)  & 100.69(77) & 20655 & 94 & 20637 & 103 & 63$\pm^{ 23 }_{ 18 }$ & $1.00$ & 24.2108 & $ 1.32\pm^{ 1.00E+20 }_{ 31.32 }$ & $ 15.86\pm^{ 0.91 }_{ nan }$ & 0.01\\ 
pg0832 & $0.32572$ (\#62)  & -- & -- & -- & -- & -- & -- & -- & 25.1357 & -- & -- & --\\ 
pg0838 & $0.06583$ (\#63)  & 34.64(61) & 1623 & 24 & 1514 & 75 & 244$\pm^{ 130 }_{ 88 }$ & $1.00$ & 20.2081 & $ 5.03E+04\pm^{ 1.00E+20 }_{ 5.03E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 0.40\\ 
pg0838 & $0.08628$ (\#64)  & 23.30(42) & 1619 & 54 & nan & nan & 186$\pm^{ 121 }_{ 78 }$ & $1.00$ & 20.5959 & $ 9.17E+08\pm^{ 1.00E+20 }_{ 9.17E+08 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 0.39\\ 
pg0838 & $0.12676$ (\#65)  & 8.14(29) & 1609 & 72 & nan & nan & 73$\pm^{ 103 }_{ 73 }$ & $1.00$ & 21.3634 & $ 5.09E+12\pm^{ 1.00E+20 }_{ 5.09E+12 }$ & $ 16.75\pm^{ 0.05 }_{ inf }$ & 0.20\\ 
pg0953 & $0.16319$ (\#66)  & 32.74(29) & 12792 & 13 & nan & nan & 419$\pm^{ 81 }_{ 73 }$ & $1.00$ & 22.0541 & $ -2.49\pm^{ 2.50 }_{ 1.06 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.46\\ 
pg0953 & $0.19221$ (\#67)  & 49.32(42) & 12792 & 21 & nan & nan & 417$\pm^{ 66 }_{ 61 }$ & $1.00$ & 22.6043 & $ -1.21\pm^{ 227.99 }_{ 1.61 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.15\\ 
pg1048 & $0.00642$ (\#68)  & 130.68(89) & 18905 & 22 & 18341 & 40 & 165$\pm^{ 26 }_{ 24 }$ & $1.00$ & 19.0817 & $ -0.28\pm^{ 9.29E+03 }_{ 2.10 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pg1048 & $0.02414$ (\#69)  & 121.85(91) & 18905 & 22 & 18341 & 48 & 157$\pm^{ 26 }_{ 23 }$ & $1.00$ & 19.4177 & $ -0.98\pm^{ 185.56 }_{ 1.83 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.09\\ 
pg1115 & $0.09511$ (\#70)  & 54.44(43) & 17542 & 15 & nan & nan & 312$\pm^{ 40 }_{ 40 }$ & $1.00$ & 20.7633 & $ 889.83\pm^{ 1.00E+20 }_{ 919.83 }$ & $ 16.45\pm^{ 0.35 }_{ nan }$ & 0.07\\ 
pg1115 & $0.12059$ (\#71)  & 43.07(32) & 17510 & 23 & nan & nan & 290$\pm^{ 49 }_{ 45 }$ & $1.00$ & 21.2464 & $ 5.39\pm^{ 1.65E+11 }_{ 35.39 }$ & $ 16.16\pm^{ 0.57 }_{ nan }$ & 0.14\\ 
pg1115 & $0.12741$ (\#72)  & 42.59(29) & 17510 & 25 & nan & nan & 274$\pm^{ 50 }_{ 45 }$ & $1.00$ & 21.3757 & $ -1.39\pm^{ 135.48 }_{ 1.81 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.18\\ 
pg1116 & $0.04114$ (\#73)  & 87.87(85) & 280360 & 13 & 294383 & 11 & 456$\pm^{ 11 }_{ 11 }$ & $1.00$ & 19.7400 & $ 2.58\pm^{ 6.98 }_{ 1.74 }$ & $ 16.05\pm^{ 0.17 }_{ 0.32 }$ & 4.54\\ 
pg1116 & $0.06251$ (\#74)  & 79.62(66) & 285035 & 13 & 294383 & 10 & 480$\pm^{ 13 }_{ 12 }$ & $1.00$ & 20.1452 & $ 4.15\pm^{ 51.81 }_{ 3.31 }$ & $ 16.13\pm^{ 0.21 }_{ 0.40 }$ & 3.41\\ 
pg1116 & $0.08382$ (\#75)  & 44.01(43) & 287898 & 13 & nan & nan & 470$\pm^{ 13 }_{ 13 }$ & $1.00$ & 20.5492 & $ -1.19\pm^{ 0.61 }_{ 0.44 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.46\\ 
pg1116 & $0.09210$ (\#76)  & 46.83(43) & 287898 & 12 & nan & nan & 499$\pm^{ 13 }_{ 13 }$ & $1.00$ & 20.7062 & $ 0.53\pm^{ 2.55 }_{ 1.08 }$ & $ 15.56\pm^{ 0.52 }_{ nan }$ & 0.19\\ 
pg1116 & $0.09281$ (\#77)  & 49.13(44) & 288074 & 12 & nan & nan & 497$\pm^{ 13 }_{ 13 }$ & $1.00$ & 20.7197 & $ 0.46\pm^{ 2.50 }_{ 1.13 }$ & $ 15.51\pm^{ 0.57 }_{ nan }$ & 0.12\\ 
pg1116 & $0.13373$ (\#78)  & 34.69(29) & 296156 & 14 & nan & nan & 516$\pm^{ 16 }_{ 17 }$ & $1.00$ & 21.4955 & $ 12.96\pm^{ 138.59 }_{ 12.14 }$ & $ 16.23\pm^{ 0.18 }_{ 0.51 }$ & 2.54\\ 
pg1116 & $0.13851$ (\#79)  & -- & -- & -- & -- & -- & -- & -- & 21.5861 & -- & -- & --\\ 
pg1211 & $0.02586$ (\#80)  & 108.44(86) & 736771 & 11 & 780487 & 11 & 490$\pm^{ 7 }_{ 7 }$ & $1.00$ & 19.4503 & $ -0.44\pm^{ 0.38 }_{ 0.31 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.62\\ 
pg1211 & $0.05443$ (\#81)  & 83.50(61) & 752151 & 10 & 777295 & 10 & 566$\pm^{ 8 }_{ 8 }$ & $1.00$ & 19.9920 & $ -0.58\pm^{ 0.39 }_{ 0.32 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.55\\ 
pg1216 & $0.00842$ (\#82)  & 112.05(92) & 11245 & 43 & 11250 & 41 & 100$\pm^{ 26 }_{ 22 }$ & $1.00$ & 19.1196 & $ -1.91\pm^{ 18.19 }_{ 1.36 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.42\\ 
pg1216 & $0.07969$ (\#83)  & 61.07(43) & 11245 & 40 & 11250 & 0 & 134$\pm^{ 37 }_{ 32 }$ & $1.00$ & 20.4709 & $ -4.17\pm^{ 2.47 }_{ 1.40 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.23\\ 
pg1216 & $0.12372$ (\#84*)  & 47.41(31) & 11245 & 31 & nan & nan & 212$\pm^{ 52 }_{ 42 }$ & $1.00$ & 21.3057 & $ 2.13E+04\pm^{ 1.00E+20 }_{ 2.14E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 0.88\\ 
pg1216 & $0.12473$ (\#85*)  & 47.65(31) & 11245 & 31 & nan & nan & 211$\pm^{ 55 }_{ 41 }$ & $1.00$ & 21.3249 & $ 3.48E+04\pm^{ 1.00E+20 }_{ 3.48E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 0.63\\ 
pg1216 & $0.17950$ (\#86)  & 55.47(38) & 11245 & 30 & nan & nan & 190$\pm^{ 49 }_{ 41 }$ & $1.00$ & 22.3633 & $ 0.54\pm^{ 1.00E+20 }_{ 30.54 }$ & $ 15.57\pm^{ 1.22 }_{ nan }$ & 0.00\\ 
pg1216 & $0.20014$ (\#87)  & 56.76(42) & 11245 & 69 & nan & nan & 145$\pm^{ 40 }_{ 33 }$ & $1.00$ & 22.7547 & $ 5.57E+07\pm^{ 1.00E+20 }_{ 5.57E+07 }$ & $ 16.65\pm^{ 0.15 }_{ -0.15 }$ & 0.44\\ 
pg1216 & $0.21258$ (\#88)  & 45.73(40) & 11245 & 53 & nan & nan & 138$\pm^{ 43 }_{ 36 }$ & $1.00$ & 22.9905 & $ -4.11\pm^{ 2.19 }_{ 1.29 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.17\\ 
pg1216 & $0.28204$ (\#89)  & 109.28(79) & 11245 & 36 & 11258 & 14 & 185$\pm^{ 46 }_{ 40 }$ & $1.00$ & 24.3075 & $ 107.15\pm^{ 1.00E+20 }_{ 137.15 }$ & $ 16.40\pm^{ 0.34 }_{ nan }$ & 0.67\\ 
pg1229 & $0.05018$ (\#90)  & 102.73(72) & 24011 & 21 & 24007 & 19 & 394$\pm^{ 38 }_{ 36 }$ & $1.00$ & 19.9114 & $ 1.82\pm^{ 2.89E+03 }_{ 31.82 }$ & $ 15.95\pm^{ 0.55 }_{ nan }$ & 0.17\\ 
pg1259 & $0.05563$ (\#91)  & 91.28(69) & 11479 & 52 & 11480 & 59 & 114$\pm^{ 32 }_{ 25 }$ & $1.00$ & 20.0147 & $ 3.04E+04\pm^{ 1.00E+20 }_{ 3.04E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 0.34\\ 
pg1259 & $0.15136$ (\#92)  & -- & -- & -- & -- & -- & -- & -- & 21.8298 & -- & -- & --\\ 
pg1259 & $0.16647$ (\#93)  & 32.56(32) & 11484 & 33 & nan & nan & 155$\pm^{ 50 }_{ 42 }$ & $1.00$ & 22.1163 & $ -1.42\pm^{ 1.26E+14 }_{ 2.24 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.07\\ 
pg1259 & $0.17893$ (\#94)  & 39.84(42) & 11484 & 36 & nan & nan & 163$\pm^{ 42 }_{ 36 }$ & $1.00$ & 22.3525 & $ 1.52E+06\pm^{ 1.00E+20 }_{ 1.52E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 1.00\\ 
pg1259 & $0.22376$ (\#95)  & 58.87(41) & 11485 & 46 & nan & nan & 216$\pm^{ 63 }_{ 46 }$ & $1.00$ & 23.2025 & $ 1.97E+06\pm^{ 1.00E+20 }_{ 1.97E+06 }$ & $ 16.62\pm^{ 0.13 }_{ nan }$ & 1.05\\ 
pg1259 & $0.24126$ (\#96)  & 61.99(46) & 11485 & 40 & 11479 & nan & 194$\pm^{ 48 }_{ 41 }$ & $1.00$ & 23.5343 & $ -0.93\pm^{ 1.00E+20 }_{ 2.70 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
pg1259 & $0.31974$ (\#97)  & 106.65(91) & 11483 & 41 & 11479 & 44 & 148$\pm^{ 44 }_{ 36 }$ & $1.00$ & 25.0223 & $ 0.54\pm^{ 1.00E+20 }_{ 30.54 }$ & $ 15.57\pm^{ 1.23 }_{ nan }$ & 0.00\\ 
pg1259 & $0.36212$ (\#98)  & 107.88(92) & 11483 & 28 & 11479 & 32 & 236$\pm^{ 54 }_{ 47 }$ & $1.00$ & 25.8258 & $ -1.97\pm^{ 19.74 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.41\\ 
pg1259 & $0.38254$ (\#99)  & 106.89(91) & 11483 & 29 & 11479 & 40 & 273$\pm^{ 64 }_{ 55 }$ & $1.00$ & 26.2130 & $ -0.95\pm^{ 1.28E+07 }_{ 2.00 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
pg1259 & $0.38266$ (\#100)  & 106.88(91) & 11483 & 29 & 11479 & 40 & 272$\pm^{ 64 }_{ 55 }$ & $1.00$ & 26.2152 & $ -1.00\pm^{ 2.39E+06 }_{ 2.09 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.05\\ 
pg1307 & $0.08345$ (\#101)  & 49.47(43) & 9851 & 11 & nan & nan & 199$\pm^{ 44 }_{ 39 }$ & $1.00$ & 20.5422 & $ -2.82\pm^{ 4.13 }_{ 1.36 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.96\\ 
pg1309 & $0.03861$ (\#102)  & 113.84(79) & 27332 & 89 & 26079 & 77 & 46$\pm^{ 15 }_{ 11 }$ & $1.00$ & 19.6920 & $ 1.21E+09\pm^{ 1.00E+20 }_{ 1.21E+09 }$ & $ 16.69\pm^{ 0.10 }_{ inf }$ & 1.82\\ 
pg1309 & $0.17740$ (\#103)  & 47.95(38) & 27263 & 86 & nan & nan & 59$\pm^{ 20 }_{ 17 }$ & $1.00$ & 22.3235 & $ -2.14\pm^{ 1.00E+20 }_{ 2.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.12\\ 
pg1309 & $0.17852$ (\#104)  & 48.79(39) & 27263 & 88 & nan & nan & 59$\pm^{ 20 }_{ 17 }$ & $1.00$ & 22.3447 & $ -1.22\pm^{ 1.00E+20 }_{ 28.78 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
pg1309 & $0.17918$ (\#105)  & 49.59(40) & 27263 & 88 & nan & nan & 58$\pm^{ 20 }_{ 17 }$ & $1.00$ & 22.3573 & $ -0.51\pm^{ 1.00E+20 }_{ 29.49 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pg1309 & $0.18143$ (\#106)  & 54.59(42) & 27263 & 81 & nan & nan & 70$\pm^{ 21 }_{ 17 }$ & $1.00$ & 22.3999 & $ 95.88\pm^{ 1.00E+20 }_{ 125.88 }$ & $ 16.38\pm^{ 0.41 }_{ nan }$ & 0.18\\ 
pg1444 & $0.22031$ (\#107)  & 50.77(40) & 17630 & 43 & nan & nan & 104$\pm^{ 38 }_{ 33 }$ & $1.00$ & 23.1371 & $ -6.35\pm^{ 1.09 }_{ 1.04 }$ & $ nan\pm^{ nan }_{ nan }$ & 17.52\\ 
pg1626 & $0.06137$ (\#108)  & 77.10(65) & 69300 & 62 & 67705 & 52 & 197$\pm^{ 24 }_{ 24 }$ & $1.00$ & 20.1236 & $ -1.17\pm^{ 389.37 }_{ 1.45 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.16\\ 
phl1811 & $0.05143$ (\#109*)  & 129.49(67) & 75753 & 86 & 78895 & 104 & 29$\pm^{ 9 }_{ 8 }$ & $1.00$ & 19.9351 & $ -1.81\pm^{ 4.24E+04 }_{ 2.05 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.22\\ 
phl1811 & $0.05813$ (\#110*)  & 121.07(62) & 77392 & 85 & 78895 & 100 & 28$\pm^{ 9 }_{ 8 }$ & $1.00$ & 20.0621 & $ -1.31\pm^{ 1.00E+20 }_{ 28.69 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
phl1811 & $0.08085$ (\#111)  & 54.95(37) & 78263 & 74 & 78895 & inf & 47$\pm^{ 11 }_{ 10 }$ & $1.00$ & 20.4929 & $ 2.01E+04\pm^{ 1.00E+20 }_{ 2.01E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 1.02\\ 
phl1811 & $0.08163$ (\#112)  & 53.36(36) & 78263 & 74 & nan & nan & 49$\pm^{ 11 }_{ 10 }$ & $1.00$ & 20.5077 & $ 2.85E+06\pm^{ 1.00E+20 }_{ 2.85E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 1.08\\ 
phl1811 & $0.12003$ (\#113)  & -- & -- & -- & -- & -- & -- & -- & 21.2358 & -- & -- & --\\ 
phl1811 & $0.15787$ (\#114)  & -- & -- & -- & -- & -- & -- & -- & 21.9532 & -- & -- & --\\ 
pks0312 & $0.11454$ (\#115)  & 27.80(20) & 23881 & 37 & nan & nan & 218$\pm^{ 42 }_{ 38 }$ & $1.00$ & 21.1317 & $ 1.37E+03\pm^{ 1.00E+20 }_{ 1.40E+03 }$ & $ 16.46\pm^{ 0.34 }_{ nan }$ & 0.86\\ 
pks0405 & $0.02510$ (\#116)  & 113.13(93) & 134903 & 16 & 138652 & 19 & 261$\pm^{ 13 }_{ 12 }$ & $1.00$ & 19.4359 & $ 4.17\pm^{ 126.34 }_{ 3.84 }$ & $ 16.13\pm^{ 0.25 }_{ 0.75 }$ & 1.85\\ 
pks0405 & $0.05902$ (\#117)  & 69.58(67) & 137242 & 19 & 138652 & 17 & 263$\pm^{ 13 }_{ 13 }$ & $1.00$ & 20.0790 & $ 3.25\pm^{ 1.29E+03 }_{ 3.79 }$ & $ 16.09\pm^{ 0.37 }_{ nan }$ & 0.63\\ 
pks0405 & $0.09719$ (\#118)  & 43.14(43) & 137149 & 20 & nan & nan & 305$\pm^{ 16 }_{ 14 }$ & $1.00$ & 20.8027 & $ -0.02\pm^{ 1.00E+20 }_{ 3.62 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pks0405 & $0.10152$ (\#119)  & 47.15(43) & 137149 & 20 & nan & nan & 319$\pm^{ 15 }_{ 15 }$ & $1.00$ & 20.8848 & $ 4.58\pm^{ 9.06E+03 }_{ 4.97 }$ & $ 16.14\pm^{ 0.32 }_{ nan }$ & 0.83\\ 
pks0405 & $0.10298$ (\#120)  & 43.50(43) & 137148 & 20 & nan & nan & 317$\pm^{ 16 }_{ 15 }$ & $1.00$ & 20.9125 & $ 0.36\pm^{ 22.57 }_{ 1.61 }$ & $ 15.42\pm^{ 0.85 }_{ nan }$ & 0.03\\ 
pks0405 & $0.19456$ (\#121)  & 47.40(42) & 134792 & 23 & nan & nan & 344$\pm^{ 29 }_{ 18 }$ & $1.00$ & 22.6489 & $ 6.59E+06\pm^{ 1.00E+20 }_{ 6.26E+06 }$ & $ 16.62\pm^{ 0.12 }_{ 0.04 }$ & 13.44\\ 
pks0405 & $0.21976$ (\#122)  & 58.71(41) & 133933 & 25 & nan & nan & 335$\pm^{ 20 }_{ 20 }$ & $1.00$ & 23.1266 & $ -0.95\pm^{ 3.38 }_{ 1.22 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.26\\ 
pks0405 & $0.24564$ (\#123)  & 62.85(45) & 136481 & 20 & nan & nan & 365$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.6173 & $ -0.87\pm^{ 2.01 }_{ 0.97 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.39\\ 
pks0405 & $0.29748$ (\#124)  & 79.55(87) & 133010 & 20 & 137174 & 19 & 392$\pm^{ 22 }_{ 21 }$ & $1.00$ & 24.6002 & $ 9.55\pm^{ 895.66 }_{ 8.54 }$ & $ 16.24\pm^{ 0.20 }_{ 0.46 }$ & 2.68\\ 
pks0405 & $0.31016$ (\#125)  & 83.17(91) & 137132 & 19 & 137234 & 21 & 382$\pm^{ 20 }_{ 19 }$ & $1.00$ & 24.8406 & $ -0.75\pm^{ 1.39 }_{ 0.76 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.48\\ 
pks0405 & $0.32502$ (\#126)  & 81.66(91) & 137139 & 18 & 137234 & 22 & 390$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.1224 & $ 1.21\pm^{ 16.95 }_{ 1.74 }$ & $ 15.85\pm^{ 0.43 }_{ nan }$ & 0.45\\ 
pks0405 & $0.49508$ (\#127)  & 96.67(89) & 136537 & 33 & 137118 & 41 & 387$\pm^{ 26 }_{ 25 }$ & $1.00$ & 28.3467 & $ -2.00\pm^{ 0.78 }_{ 0.54 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.48\\ 
pks0558 & $0.10472$ (\#128)  & 56.06(47) & 718011 & 24 & nan & nan & 1867$\pm^{ 16 }_{ 16 }$ & $1.00$ & 20.9455 & $ -0.74\pm^{ 0.23 }_{ 0.21 }$ & $ nan\pm^{ nan }_{ nan }$ & 9.26\\ 
pks2155 & $0.05708$ (\#129)  & 51.87(51) & 1703911 & 3 & 1685268 & 3 & 4633$\pm^{ 441 }_{ 413 }$ & $1.47$ & 20.0422 & $ 0.29\pm^{ 0.18 }_{ 0.11 }$ & $ 15.32\pm^{ 0.19 }_{ 0.21 }$ & 7.04\\
pks2155 & $0.06236$ (\#130)  & 47.13(42) & 1703863 & 3 & 1685268 & 3 & 3901$\pm^{ 490 }_{ 417 }$ & $1.82$ & 20.1423 & $ 0.14\pm^{ 0.14 }_{ 0.13 }$ & $ 15.04\pm^{ 0.28 }_{ 1.00 }$ & 1.63\\ 
pks2155 & $0.10586$ (\#131)  & 53.78(37) & 1701058 & 3 & nan & nan & 3620$\pm^{ 354 }_{ 403 }$ & $2.02$ & 20.9671 & $ 0.02\pm^{ 0.09 }_{ 0.16 }$ & $ 14.11\pm^{ 0.80 }_{ nan }$ & -0.07\\ 
q0045 & $0.05590$ (\#132)  & -- & -- & -- & -- & -- & -- & -- & 20.0199 & -- & -- & --\\ 
q0045 & $0.06377$ (\#133)  & -- & -- & -- & -- & -- & -- & -- & 20.1691 & -- & -- & --\\ 
q1230 & $0.08344$ (\#134)  & 47.77(33) & 39327 & 59 & nan & nan & 68$\pm^{ 18 }_{ 17 }$ & $1.00$ & 20.5420 & $ 2.51\pm^{ 2.29E+15 }_{ 32.51 }$ & $ 16.04\pm^{ 0.72 }_{ nan }$ & 0.03\\ 
q1230 & $0.08540$ (\#135)  & 48.90(35) & 39327 & 60 & nan & nan & 64$\pm^{ 15 }_{ 13 }$ & $1.00$ & 20.5792 & $ 0.00\pm^{ 9.25E+16 }_{ 30.00 }$ & $ 12.67\pm^{ 4.12 }_{ nan }$ & 0.00\\ 
q1230 & $0.09444$ (\#136)  & 42.77(29) & 39328 & 56 & nan & nan & 64$\pm^{ 19 }_{ 18 }$ & $1.00$ & 20.7506 & $ -2.79\pm^{ 1.00E+20 }_{ 27.21 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.09\\ 
q1230 & $0.10000$ (\#137)  & 42.86(29) & 39328 & 60 & nan & nan & 55$\pm^{ 18 }_{ 15 }$ & $1.00$ & 20.8560 & $ -3.67\pm^{ 2.82 }_{ 1.31 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.71\\ 
q1230 & $0.10525$ (\#138)  & 43.32(30) & 39329 & 65 & nan & nan & 73$\pm^{ 21 }_{ 16 }$ & $1.00$ & 20.9555 & $ 2.12E+04\pm^{ 1.00E+20 }_{ 2.13E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 0.78\\ 
q1230 & $0.10549$ (\#139)  & 43.13(30) & 39329 & 65 & nan & nan & 74$\pm^{ 22 }_{ 16 }$ & $1.00$ & 20.9601 & $ 2.02E+06\pm^{ 1.00E+20 }_{ 2.02E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 0.99\\ 
q1230 & $0.10566$ (\#140)  & 43.20(30) & 39329 & 65 & nan & nan & 73$\pm^{ 22 }_{ 16 }$ & $1.00$ & 20.9633 & $ 3.03E+04\pm^{ 1.00E+20 }_{ 3.04E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 0.90\\ 
q1230 & $0.10612$ (\#141)  & 39.76(29) & 39330 & 63 & nan & nan & 77$\pm^{ 23 }_{ 16 }$ & $1.00$ & 20.9720 & $ 1.38E+09\pm^{ 1.00E+20 }_{ 1.38E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.52\\ 
q1230 & $0.10639$ (\#142)  & 40.21(30) & 39330 & 65 & nan & nan & 72$\pm^{ 23 }_{ 17 }$ & $1.00$ & 20.9772 & $ 2.30E+06\pm^{ 1.00E+20 }_{ 2.30E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 1.23\\ 
q1230 & $0.10660$ (\#143)  & 39.93(30) & 39330 & 65 & nan & nan & 73$\pm^{ 23 }_{ 16 }$ & $1.00$ & 20.9811 & $ 1.95E+09\pm^{ 1.00E+20 }_{ 1.95E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.54\\ 
q1230 & $0.10853$ (\#144)  & 39.15(27) & 39331 & 86 & nan & nan & 50$\pm^{ 20 }_{ 15 }$ & $1.00$ & 21.0177 & $ 2.90E+09\pm^{ 1.00E+20 }_{ 2.90E+09 }$ & $ 16.69\pm^{ 0.08 }_{ inf }$ & 1.22\\ 
q1230 & $0.10940$ (\#145)  & 39.98(27) & 39331 & 96 & nan & nan & 49$\pm^{ 17 }_{ 14 }$ & $1.00$ & 21.0342 & $ 1.31E+12\pm^{ 1.00E+20 }_{ 1.31E+12 }$ & $ 16.75\pm^{ 0.00 }_{ inf }$ & 1.53\\ 
q1230 & $0.12103$ (\#146)  & -- & -- & -- & -- & -- & -- & -- & 21.2547 & -- & -- & --\\ 
rbs1892 & $0.15567$ (\#147)  & -- & -- & -- & -- & -- & -- & -- & 21.9115 & -- & -- & --\\ 
rbs1892 & $0.15633$ (\#148)  & -- & -- & -- & -- & -- & -- & -- & 21.9240 & -- & -- & --\\ 
rbs1892 & $0.16343$ (\#149)  & 33.64(29) & 4929 & 10 & nan & nan & 164$\pm^{ 103 }_{ 79 }$ & $1.00$ & 22.0586 & $ -6.14\pm^{ 1.50 }_{ 1.44 }$ & $ nan\pm^{ nan }_{ nan }$ & 11.71\\ 
rbs1892 & $0.17001$ (\#150)  & 45.15(35) & 4929 & 14 & nan & nan & 243$\pm^{ 126 }_{ 104 }$ & $1.00$ & 22.1834 & $ -4.41\pm^{ 1.56E+08 }_{ 1.80 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.30\\ 
rbs1892 & $0.17155$ (\#151)  & 46.20(37) & 4929 & 14 & nan & nan & 316$\pm^{ 102 }_{ 77 }$ & $1.00$ & 22.2126 & $ 4.74E+06\pm^{ 1.00E+20 }_{ 4.74E+06 }$ & $ 16.62\pm^{ 0.18 }_{ nan }$ & 0.59\\ 
rbs1892 & $0.17185$ (\#152)  & 46.34(37) & 4929 & 14 & nan & nan & 311$\pm^{ 104 }_{ 75 }$ & $1.00$ & 22.2183 & $ 2.09E+04\pm^{ 1.00E+20 }_{ 2.09E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 0.56\\ 
rbs542 & $0.04455$ (\#153)  & 100.05(84) & 197378 & 8 & 212046 & 8 & 956$\pm^{ 19 }_{ 19 }$ & $1.00$ & 19.8047 & $ -0.25\pm^{ 0.65 }_{ 0.47 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.23\\ 
rbs542 & $0.04992$ (\#154)  & 97.00(77) & 197040 & 8 & 212046 & 8 & 962$\pm^{ 18 }_{ 18 }$ & $1.00$ & 19.9065 & $ -0.04\pm^{ 0.97 }_{ 0.50 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.01\\ 
rxj0439 & $0.00550$ (\#155)  & 111.59(94) & 146061 & 18 & 150968 & 15 & 276$\pm^{ 12 }_{ 12 }$ & $1.00$ & 19.0643 & $ 2.72\pm^{ 19.78 }_{ 2.59 }$ & $ 16.05\pm^{ 0.26 }_{ 1.04 }$ & 1.50\\ 
rxj0439 & $0.17680$ (\#156)  & 56.53(41) & 146765 & 20 & nan & nan & 365$\pm^{ 22 }_{ 19 }$ & $1.00$ & 22.3121 & $ 14.37\pm^{ 8.72E+03 }_{ 13.75 }$ & $ 16.25\pm^{ 0.28 }_{ 0.64 }$ & 1.68\\ 
s50716 & $0.00989$ (\#157)  & 106.78(94) & 74106 & 11 & 75858 & 11 & 613$\pm^{ 25 }_{ 24 }$ & $1.00$ & 19.1475 & $ 1.40\pm^{ 6.33 }_{ 1.62 }$ & $ 15.88\pm^{ 0.34 }_{ nan }$ & 0.82\\ 
s50716 & $0.01766$ (\#158)  & 104.96(94) & 74441 & 11 & 76625 & 10 & 604$\pm^{ 25 }_{ 24 }$ & $1.00$ & 19.2948 & $ -0.48\pm^{ 1.26 }_{ 0.72 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.28\\ 
s50716 & $0.08834$ (\#159)  & 40.33(43) & 77052 & 11 & nan & nan & 620$\pm^{ 28 }_{ 27 }$ & $1.00$ & 20.6349 & $ -1.52\pm^{ 1.01 }_{ 0.68 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.22\\ 
s50716 & $0.14936$ (\#160)  & -- & -- & -- & -- & -- & -- & -- & 21.7919 & -- & -- & --\\ 
ton28 & $0.03357$ (\#161)  & 104.99(91) & 83993 & 29 & 86174 & 29 & 124$\pm^{ 12 }_{ 11 }$ & $1.00$ & 19.5965 & $ -1.25\pm^{ 2.69 }_{ 1.03 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.52\\ 
tons180 & $0.04304$ (\#162)  & 73.60(82) & 187350 & 6 & 195496 & 7 & 956$\pm^{ 19 }_{ 19 }$ & $1.00$ & 19.7760 & $ -0.08\pm^{ 0.71 }_{ 0.52 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
tons210 & $0.06763$ (\#163)  & 71.27(58) & 6723 & 15 & 6719 & 6 & 382$\pm^{ 71 }_{ 64 }$ & $1.00$ & 20.2423 & $ -2.67\pm^{ 3.16 }_{ 1.20 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.12\\ 
tons210 & $0.08558$ (\#164)  & 52.71(42) & 6725 & 18 & nan & nan & 460$\pm^{ 80 }_{ 73 }$ & $1.00$ & 20.5826 & $ -1.42\pm^{ 2.97E+04 }_{ 1.84 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.14\\ 



\hline
\hline
 \end{longtable}
 \end{landscape}

==> Tables/XMM/Latex/xmm_o8_hi_uppers_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllll|l}
\caption[\xmm\ Data, \oviii\ Upper Limits With \hi\ Priors Results (Full)]{\oviii\ upper limit measurements with \xmm\ data, at the prior redshift from the \hi\ lines from Table~\ref{tab:hiPriorsTable}.}
\label{tab:xmmhioviiiuppers}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & RGS1 & RGS2 & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & avg exp (s) & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N + (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.13714$ (\#1)  & -- & -- & -- & -- & -- & 21.5602 & -- & -- & --\\ 
1es1028 & $0.20383$ (\#2)  & 62.35(44) & 146640 & nan & 1006$\pm^{ 29 }_{ 29 }$ & $1.00$ & 22.8246 & 1.57 &  15.92 & 0.01\\ 
1es1028 & $0.22121$ (\#3)  & 57.62(42) & 144940 & nan & 1031$\pm^{ 32 }_{ 31 }$ & $1.00$ & 23.1541 & 0.62 &  15.62 & 3.89\\ 
1es1553 & $0.03466$ (\#4)  & 90.75(81) & 1722815 & 1780022 & 752$\pm^{ 116 }_{ 96 }$ & $2.09$ & 19.6172 & 0.35 &  15.41 & -0.41\\ 
1es1553 & $0.04273$ (\#5)  & 89.06(72) & 1720386 & 1774803 & 776$\pm^{ 127 }_{ 108 }$ & $2.01$ & 19.7702 & 0.19 &  15.17 & 0.14\\ 
1es1553 & $0.06364$ (\#6)  & 46.18(56) & 1785421 & 1740261 & 1161$\pm^{ 253 }_{ 220 }$ & $1.18$ & 20.1666 & 0.27 &  15.31 & -0.04\\ 
1es1553 & $0.21869$ (\#7)  & 36.89(28) & 1666450 & nan & 36$\pm^{ 20 }_{ 13 }$ & $7.01$ & 23.1064 & 0.28 &  15.32 & 2.52\\ 
3c249 & $0.13470$ (\#8)  & -- & -- & -- & -- & -- & 21.5139 & -- & -- & --\\ 
3c249 & $0.26664$ (\#9)  & 53.79(69) & 2644 & 2524 & 320$\pm^{ 120 }_{ 95 }$ & $1.00$ & 24.0155 & 5.00E+19 &  16.80 & 1.35\\ 
3c273 & $0.00758$ (\#10)  & 83.67(67) & 1048814 & 1012144 & 3696$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1037 & 0.23 &  15.24 & 0.77\\ 
3c273 & $0.06707$ (\#11)  & 77.60(60) & 1015660 & 1019511 & 3919$\pm^{ 16 }_{ 16 }$ & $1.00$ & 20.2316 & 0.26 &  15.29 & -0.35\\ 
3c273 & $0.07359$ (\#12)  & 63.12(54) & 922775 & 1018570 & 3920$\pm^{ 17 }_{ 16 }$ & $1.00$ & 20.3553 & 0.25 &  15.27 & -0.21\\ 
3c273 & $0.13960$ (\#13)  & -- & -- & -- & -- & -- & 21.6068 & -- & -- & --\\ 
h1821 & $0.00944$ (\#14)  & 120.55(98) & 30556 & 43312 & 1002$\pm^{ 55 }_{ 53 }$ & $1.00$ & 19.1390 & 0.95 &  15.77 & 0.86\\ 
h1821 & $0.06779$ (\#15)  & 81.53(61) & 31940 & 43282 & 1055$\pm^{ 61 }_{ 60 }$ & $1.00$ & 20.2453 & 2.35 &  16.02 & 0.15\\ 
h1821 & $0.08483$ (\#16)  & 49.50(43) & 30565 & nan & 1106$\pm^{ 71 }_{ 68 }$ & $1.00$ & 20.5684 & 1.74 &  15.93 & 0.43\\ 
h1821 & $0.12147$ (\#17)  & 44.27(31) & 30928 & nan & 1128$\pm^{ 97 }_{ 95 }$ & $1.00$ & 21.2631 & 3.92 &  16.12 & 0.14\\ 
h1821 & $0.19817$ (\#18)  & 63.03(48) & 30824 & nan & 974$\pm^{ 88 }_{ 85 }$ & $1.00$ & 22.7173 & 1.51 &  15.90 & 1.17\\ 
h1821 & $0.21321$ (\#19)  & 58.22(45) & 29048 & nan & 1010$\pm^{ 95 }_{ 92 }$ & $1.00$ & 23.0025 & 3.09 &  16.07 & 0.40\\ 
h1821 & $0.24531$ (\#20)  & 69.92(50) & 31312 & 36214 & 1107$\pm^{ 101 }_{ 88 }$ & $1.00$ & 23.6111 & 3.78E+13 &  16.75 & 0.61\\ 
h2356 & $0.03830$ (\#21)  & 97.28(88) & 479869 & 503477 & 1019$\pm^{ 12 }_{ 13 }$ & $1.00$ & 19.6862 & 0.46 &  15.52 & 1.03\\ 
h2356 & $0.07881$ (\#22)  & 54.41(41) & 506719 & 263751 & 1072$\pm^{ 15 }_{ 15 }$ & $1.00$ & 20.4542 & 0.40 &  15.46 & 1.77\\ 
h2356 & $0.10467$ (\#23)  & 43.81(39) & 507154 & nan & 1072$\pm^{ 16 }_{ 15 }$ & $1.00$ & 20.9445 & 0.35 &  15.40 & 3.88\\ 
h2356 & $0.15613$ (\#24)  & 37.69(29) & 503603 & nan & 1088$\pm^{ 19 }_{ 18 }$ & $1.00$ & 21.9202 & 0.63 &  15.63 & -0.01\\ 
he0226 & $0.14274$ (\#25)  & -- & -- & -- & -- & -- & 21.6664 & -- & -- & --\\ 
he0226 & $0.39890$ (\#26)  & 130.12(94) & 31707 & 31704 & 265$\pm^{ 37 }_{ 34 }$ & $1.00$ & 26.5231 & 2.46 &  16.04 & 0.53\\ 
he0226 & $0.41024$ (\#27)  & 136.42(96) & 31707 & 31704 & 274$\pm^{ 38 }_{ 35 }$ & $1.00$ & 26.7382 & 1.69 &  15.94 & 0.89\\ 
i22456 & $0.00443$ (\#28)  & 130.08(99) & 76706 & 81909 & 381$\pm^{ 22 }_{ 21 }$ & $1.00$ & 19.0440 & 0.53 &  15.56 & 6.46\\ 
i22456 & $0.09941$ (\#29)  & 59.72(44) & 79900 & nan & 501$\pm^{ 38 }_{ 27 }$ & $1.00$ & 20.8448 & 5.00E+19 &  16.80 & 4.43\\ 
mr2251 & $0.01068$ (\#30)  & 121.16(93) & 414226 & 451165 & 1243$\pm^{ 275 }_{ 224 }$ & $1.52$ & 19.1625 & 0.21 &  15.19 & 9.71\\ 
mr2251 & $0.01449$ (\#31)  & 122.62(90) & 428129 & 462131 & 1173$\pm^{ 252 }_{ 199 }$ & $1.69$ & 19.2347 & 0.32 &  15.38 & 0.13\\ 
mr2251 & $0.06131$ (\#32)  & 68.20(47) & 466085 & 461291 & 2234$\pm^{ 1198 }_{ 730 }$ & $0.41$ & 20.1224 & 0.92 &  15.76 & 5.66\\ 
mr2251 & $0.06190$ (\#33)  & 62.95(47) & 466085 & 461291 & 2211$\pm^{ 1157 }_{ 717 }$ & $0.45$ & 20.1336 & 2.23 &  16.00 & 16.53\\ 
mr2251 & $0.06276$ (\#34)  & 50.87(49) & 466106 & 461162 & 2612$\pm^{ 1875 }_{ 645 }$ & $0.13$ & 20.1499 & 29.78 &  16.31 & 38.86\\ 
mr2251 & $0.06327$ (\#35)  & 44.88(49) & 466112 & 461008 & 2740$\pm^{ 1569 }_{ 769 }$ & $0.03$ & 20.1596 & 64.78 &  16.34 & 45.67\\ 
mr2251 & $0.06381$ (\#36)  & 45.72(49) & 466112 & 461008 & 2376$\pm^{ 1389 }_{ 647 }$ & $0.33$ & 20.1698 & 165.19 &  16.35 & 45.47\\ 
mrk478 & $0.06166$ (\#37)  & 76.63(64) & 202266 & 202111 & 465$\pm^{ 14 }_{ 14 }$ & $1.00$ & 20.1291 & 1.45 &  15.91 & 0.00\\ 
mrk478 & $0.06578$ (\#38)  & 70.27(61) & 204255 & 201677 & 472$\pm^{ 14 }_{ 15 }$ & $1.00$ & 20.2072 & 1.65 &  15.93 & -0.00\\ 
mrk478 & $0.07213$ (\#39)  & 54.18(51) & 200098 & 200301 & 492$\pm^{ 16 }_{ 15 }$ & $1.00$ & 20.3276 & 66.34 &  16.33 & 1.94\\ 
mrk876 & $0.01159$ (\#40)  & 84.83(96) & 2656 & 2600 & 174$\pm^{ 70 }_{ 54 }$ & $1.00$ & 19.1797 & 5.00E+19 &  16.75 & 0.81\\ 
mrk876 & $0.05598$ (\#41)  & 59.57(72) & 2736 & 2708 & 227$\pm^{ 89 }_{ 64 }$ & $1.00$ & 20.0214 & 5.00E+19 &  16.80 & 0.48\\ 
mrk876 & $0.08709$ (\#42)  & 42.06(43) & 2804 & nan & 414$\pm^{ 119 }_{ 103 }$ & $1.00$ & 20.6112 & 1.22 &  15.85 & 4.24\\ 
mrk876 & $0.08858$ (\#43)  & 42.31(44) & 2805 & nan & 419$\pm^{ 123 }_{ 105 }$ & $1.00$ & 20.6395 & 1.23 &  15.85 & 3.77\\ 
mrk876 & $0.08917$ (\#44)  & 42.90(43) & 2804 & nan & 427$\pm^{ 125 }_{ 107 }$ & $1.00$ & 20.6507 & 1.32 &  15.86 & 2.96\\ 
mrk876 & $0.11487$ (\#45)  & 52.10(37) & 2790 & nan & 714$\pm^{ 237 }_{ 160 }$ & $1.00$ & 21.1379 & 5.00E+19 &  16.80 & 3.07\\ 
ngc7469 & $0.00981$ (\#46)  & 85.67(65) & 629599 & 665412 & 1934$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1460 & 0.89 &  15.74 & 51.59\\ 
pg0003 & $0.08299$ (\#47)  & 56.55(41) & 13036 & nan & 169$\pm^{ 41 }_{ 36 }$ & $1.00$ & 20.5335 & 4.11E+03 &  16.46 & 0.31\\ 
pg0003 & $0.17139$ (\#48)  & 45.45(37) & 13036 & nan & 315$\pm^{ 63 }_{ 56 }$ & $1.00$ & 22.2096 & 5.00E+19 &  16.80 & 0.01\\ 
pg0003 & $0.22541$ (\#49)  & 47.36(42) & 13037 & nan & 145$\pm^{ 50 }_{ 43 }$ & $1.00$ & 23.2338 & 0.96 &  15.76 & 8.09\\ 
pg0003 & $0.38633$ (\#50)  & 107.06(92) & 13033 & 12857 & 248$\pm^{ 69 }_{ 50 }$ & $1.00$ & 26.2848 & 5.00E+19 &  16.80 & 1.31\\ 
pg0003 & $0.42051$ (\#51)  & 129.11(93) & 13034 & 12830 & 327$\pm^{ 75 }_{ 64 }$ & $1.00$ & 26.9329 & 5.00E+19 &  16.80 & 0.73\\ 
pg0804 & $0.05015$ (\#52)  & 80.99(78) & 28468 & 30600 & 1084$\pm^{ 53 }_{ 49 }$ & $1.00$ & 19.9108 & 2.27 &  16.01 & 0.00\\ 
pg0804 & $0.05576$ (\#53)  & 70.57(71) & 28779 & 30600 & 1101$\pm^{ 55 }_{ 53 }$ & $1.00$ & 20.0172 & 7.34E+03 &  16.46 & 1.53\\ 
pg0804 & $0.36379$ (\#54)  & 131.95(97) & 30110 & 29227 & 1657$\pm^{ 86 }_{ 84 }$ & $1.00$ & 25.8575 & 0.90 &  15.76 & 1.74\\ 
pg0832 & $0.01753$ (\#55)  & -- & -- & -- & -- & -- & 19.2924 & -- & -- & --\\ 
pg0832 & $0.02793$ (\#56)  & -- & -- & -- & -- & -- & 19.4896 & -- & -- & --\\ 
pg0832 & $0.08748$ (\#57)  & 59.08(42) & 20650 & nan & 41$\pm^{ 16 }_{ 12 }$ & $1.00$ & 20.6186 & 5.00E+19 &  16.75 & 0.57\\ 
pg0832 & $0.10171$ (\#58)  & 53.76(42) & 20652 & nan & 29$\pm^{ 15 }_{ 12 }$ & $1.00$ & 20.8884 & 2.08 &  15.99 & 1.81\\ 
pg0832 & $0.18391$ (\#59)  & 40.73(29) & 20654 & nan & 36$\pm^{ 22 }_{ 16 }$ & $1.00$ & 22.4469 & 2.66 &  16.05 & 1.60\\ 
pg0832 & $0.27503$ (\#60)  & 100.19(76) & 20655 & 20637 & 76$\pm^{ 24 }_{ 20 }$ & $1.00$ & 24.1746 & 3.37E+13 &  16.74 & 0.04\\ 
pg0832 & $0.27694$ (\#61)  & 100.69(77) & 20655 & 20637 & 63$\pm^{ 23 }_{ 18 }$ & $1.00$ & 24.2108 & 5.00E+19 &  16.77 & 0.01\\ 
pg0832 & $0.32572$ (\#62)  & -- & -- & -- & -- & -- & 25.1357 & -- & -- & --\\ 
pg0838 & $0.06583$ (\#63)  & 34.64(61) & 1623 & 1514 & 244$\pm^{ 130 }_{ 88 }$ & $1.00$ & 20.2081 & 5.00E+19 &  16.80 & 0.40\\ 
pg0838 & $0.08628$ (\#64)  & 23.30(42) & 1619 & nan & 186$\pm^{ 121 }_{ 78 }$ & $1.00$ & 20.5959 & 5.00E+19 &  16.80 & 0.39\\ 
pg0838 & $0.12676$ (\#65)  & 8.14(29) & 1609 & nan & 73$\pm^{ 103 }_{ 73 }$ & $1.00$ & 21.3634 & 5.00E+19 &  16.80 & 0.20\\ 
pg0953 & $0.16319$ (\#66)  & 32.74(29) & 12792 & nan & 419$\pm^{ 81 }_{ 73 }$ & $1.00$ & 22.0541 & 1.78 &  15.95 & 1.46\\ 
pg0953 & $0.19221$ (\#67)  & 49.32(42) & 12792 & nan & 417$\pm^{ 66 }_{ 61 }$ & $1.00$ & 22.6043 & 114.80 &  16.36 & 0.15\\ 
pg1048 & $0.00642$ (\#68)  & 130.68(89) & 18905 & 18341 & 165$\pm^{ 26 }_{ 24 }$ & $1.00$ & 19.0817 & 4.65E+03 &  16.53 & 0.00\\ 
pg1048 & $0.02414$ (\#69)  & 121.85(91) & 18905 & 18341 & 157$\pm^{ 26 }_{ 23 }$ & $1.00$ & 19.4177 & 93.69 &  16.39 & 0.09\\ 
pg1115 & $0.09511$ (\#70)  & 54.44(43) & 17542 & nan & 312$\pm^{ 40 }_{ 40 }$ & $1.00$ & 20.7633 & 5.00E+19 &  16.80 & 0.07\\ 
pg1115 & $0.12059$ (\#71)  & 43.07(32) & 17510 & nan & 290$\pm^{ 49 }_{ 45 }$ & $1.00$ & 21.2464 & 8.25E+10 &  16.71 & 0.14\\ 
pg1115 & $0.12741$ (\#72)  & 42.59(29) & 17510 & nan & 274$\pm^{ 50 }_{ 45 }$ & $1.00$ & 21.3757 & 68.65 &  16.37 & 0.18\\ 
pg1116 & $0.04114$ (\#73)  & 87.87(85) & 280360 & 294383 & 456$\pm^{ 11 }_{ 11 }$ & $1.00$ & 19.7400 & 4.36 &  16.14 & 4.54\\ 
pg1116 & $0.06251$ (\#74)  & 79.62(66) & 285035 & 294383 & 480$\pm^{ 13 }_{ 12 }$ & $1.00$ & 20.1452 & 27.56 &  16.31 & 3.41\\ 
pg1116 & $0.08382$ (\#75)  & 44.01(43) & 287898 & nan & 470$\pm^{ 13 }_{ 13 }$ & $1.00$ & 20.5492 & 0.53 &  15.56 & 3.46\\ 
pg1116 & $0.09210$ (\#76)  & 46.83(43) & 287898 & nan & 499$\pm^{ 13 }_{ 13 }$ & $1.00$ & 20.7062 & 1.82 &  15.95 & 0.19\\ 
pg1116 & $0.09281$ (\#77)  & 49.13(44) & 288074 & nan & 497$\pm^{ 13 }_{ 13 }$ & $1.00$ & 20.7197 & 1.82 &  15.97 & 0.12\\ 
pg1116 & $0.13373$ (\#78)  & 34.69(29) & 296156 & nan & 516$\pm^{ 16 }_{ 17 }$ & $1.00$ & 21.4955 & 75.36 &  16.37 & 2.54\\ 
pg1116 & $0.13851$ (\#79)  & -- & -- & -- & -- & -- & 21.5861 & -- & -- & --\\ 
pg1211 & $0.02586$ (\#80)  & 108.44(86) & 736771 & 780487 & 490$\pm^{ 7 }_{ 7 }$ & $1.00$ & 19.4503 & 0.35 &  15.40 & 1.62\\ 
pg1211 & $0.05443$ (\#81)  & 83.50(61) & 752151 & 777295 & 566$\pm^{ 8 }_{ 8 }$ & $1.00$ & 19.9920 & 0.36 &  15.42 & 2.55\\ 
pg1216 & $0.00842$ (\#82)  & 112.05(92) & 11245 & 11250 & 100$\pm^{ 26 }_{ 22 }$ & $1.00$ & 19.1196 & 9.78 &  16.25 & 0.42\\ 
pg1216 & $0.07969$ (\#83)  & 61.07(43) & 11245 & 11250 & 134$\pm^{ 37 }_{ 32 }$ & $1.00$ & 20.4709 & 1.93 &  15.98 & 2.23\\ 
pg1216 & $0.12372$ (\#84*)  & 47.41(31) & 11245 & nan & 212$\pm^{ 52 }_{ 42 }$ & $1.00$ & 21.3057 & 5.00E+19 &  16.80 & 0.88\\ 
pg1216 & $0.12473$ (\#85*)  & 47.65(31) & 11245 & nan & 211$\pm^{ 55 }_{ 41 }$ & $1.00$ & 21.3249 & 5.00E+19 &  16.80 & 0.63\\ 
pg1216 & $0.17950$ (\#86)  & 55.47(38) & 11245 & nan & 190$\pm^{ 49 }_{ 41 }$ & $1.00$ & 22.3633 & 5.00E+19 &  16.80 & 0.00\\ 
pg1216 & $0.20014$ (\#87)  & 56.76(42) & 11245 & nan & 145$\pm^{ 40 }_{ 33 }$ & $1.00$ & 22.7547 & 5.00E+19 &  16.80 & 0.44\\ 
pg1216 & $0.21258$ (\#88)  & 45.73(40) & 11245 & nan & 138$\pm^{ 43 }_{ 36 }$ & $1.00$ & 22.9905 & 1.74 &  15.95 & 2.17\\ 
pg1216 & $0.28204$ (\#89)  & 109.28(79) & 11245 & 11258 & 185$\pm^{ 46 }_{ 40 }$ & $1.00$ & 24.3075 & 5.00E+19 &  16.75 & 0.67\\ 
pg1229 & $0.05018$ (\#90)  & 102.73(72) & 24011 & 24007 & 394$\pm^{ 38 }_{ 36 }$ & $1.00$ & 19.9114 & 1.46E+03 &  16.47 & 0.17\\ 
pg1259 & $0.05563$ (\#91)  & 91.28(69) & 11479 & 11480 & 114$\pm^{ 32 }_{ 25 }$ & $1.00$ & 20.0147 & 5.00E+19 &  16.80 & 0.34\\ 
pg1259 & $0.15136$ (\#92)  & -- & -- & -- & -- & -- & 21.8298 & -- & -- & --\\ 
pg1259 & $0.16647$ (\#93)  & 32.56(32) & 11484 & nan & 155$\pm^{ 50 }_{ 42 }$ & $1.00$ & 22.1163 & 6.28E+13 &  16.76 & 0.07\\ 
pg1259 & $0.17893$ (\#94)  & 39.84(42) & 11484 & nan & 163$\pm^{ 42 }_{ 36 }$ & $1.00$ & 22.3525 & 5.00E+19 &  16.75 & 1.00\\ 
pg1259 & $0.22376$ (\#95)  & 58.87(41) & 11485 & nan & 216$\pm^{ 63 }_{ 46 }$ & $1.00$ & 23.2025 & 5.00E+19 &  16.75 & 1.05\\ 
pg1259 & $0.24126$ (\#96)  & 61.99(46) & 11485 & 11479 & 194$\pm^{ 48 }_{ 41 }$ & $1.00$ & 23.5343 & 5.00E+19 &  16.75 & 0.03\\ 
pg1259 & $0.31974$ (\#97)  & 106.65(91) & 11483 & 11479 & 148$\pm^{ 44 }_{ 36 }$ & $1.00$ & 25.0223 & 5.00E+19 &  16.80 & 0.00\\ 
pg1259 & $0.36212$ (\#98)  & 107.88(92) & 11483 & 11479 & 236$\pm^{ 54 }_{ 47 }$ & $1.00$ & 25.8258 & 10.54 &  16.26 & 0.41\\ 
pg1259 & $0.38254$ (\#99)  & 106.89(91) & 11483 & 11479 & 273$\pm^{ 64 }_{ 55 }$ & $1.00$ & 26.2130 & 6.38E+06 &  16.58 & 0.04\\ 
pg1259 & $0.38266$ (\#100)  & 106.88(91) & 11483 & 11479 & 272$\pm^{ 64 }_{ 55 }$ & $1.00$ & 26.2152 & 1.20E+06 &  16.57 & 0.05\\ 
pg1307 & $0.08345$ (\#101)  & 49.47(43) & 9851 & nan & 199$\pm^{ 44 }_{ 39 }$ & $1.00$ & 20.5422 & 2.75 &  16.06 & 0.96\\ 
pg1309 & $0.03861$ (\#102)  & 113.84(79) & 27332 & 26079 & 46$\pm^{ 15 }_{ 11 }$ & $1.00$ & 19.6920 & 5.00E+19 &  16.79 & 1.82\\ 
pg1309 & $0.17740$ (\#103)  & 47.95(38) & 27263 & nan & 59$\pm^{ 20 }_{ 17 }$ & $1.00$ & 22.3235 & 5.00E+19 &  16.75 & 0.12\\ 
pg1309 & $0.17852$ (\#104)  & 48.79(39) & 27263 & nan & 59$\pm^{ 20 }_{ 17 }$ & $1.00$ & 22.3447 & 5.00E+19 &  16.80 & 0.02\\ 
pg1309 & $0.17918$ (\#105)  & 49.59(40) & 27263 & nan & 58$\pm^{ 20 }_{ 17 }$ & $1.00$ & 22.3573 & 5.00E+19 &  16.80 & 0.00\\ 
pg1309 & $0.18143$ (\#106)  & 54.59(42) & 27263 & nan & 70$\pm^{ 21 }_{ 17 }$ & $1.00$ & 22.3999 & 5.00E+19 &  16.80 & 0.18\\ 
pg1444 & $0.22031$ (\#107)  & 50.77(40) & 17630 & nan & 104$\pm^{ 38 }_{ 33 }$ & $1.00$ & 23.1371 & 1.07 &  15.81 & 17.52\\ 
pg1626 & $0.06137$ (\#108)  & 77.10(65) & 69300 & 67705 & 197$\pm^{ 24 }_{ 24 }$ & $1.00$ & 20.1236 & 195.41 &  16.35 & 0.16\\ 
phl1811 & $0.05143$ (\#109*)  & 129.49(67) & 75753 & 78895 & 29$\pm^{ 9 }_{ 8 }$ & $1.00$ & 19.9351 & 2.12E+04 &  16.48 & 0.22\\ 
phl1811 & $0.05813$ (\#110*)  & 121.07(62) & 77392 & 78895 & 28$\pm^{ 9 }_{ 8 }$ & $1.00$ & 20.0621 & 5.00E+19 &  16.80 & 0.03\\ 
phl1811 & $0.08085$ (\#111)  & 54.95(37) & 78263 & 78895 & 47$\pm^{ 11 }_{ 10 }$ & $1.00$ & 20.4929 & 5.00E+19 &  16.80 & 1.02\\ 
phl1811 & $0.08163$ (\#112)  & 53.36(36) & 78263 & nan & 49$\pm^{ 11 }_{ 10 }$ & $1.00$ & 20.5077 & 5.00E+19 &  16.75 & 1.08\\ 
phl1811 & $0.12003$ (\#113)  & -- & -- & -- & -- & -- & 21.2358 & -- & -- & --\\ 
phl1811 & $0.15787$ (\#114)  & -- & -- & -- & -- & -- & 21.9532 & -- & -- & --\\ 
pks0312 & $0.11454$ (\#115)  & 27.80(20) & 23881 & nan & 218$\pm^{ 42 }_{ 38 }$ & $1.00$ & 21.1317 & 5.00E+19 &  16.80 & 0.86\\ 
pks0405 & $0.02510$ (\#116)  & 113.13(93) & 134903 & 138652 & 261$\pm^{ 13 }_{ 12 }$ & $1.00$ & 19.4359 & 65.09 &  16.33 & 1.85\\ 
pks0405 & $0.05902$ (\#117)  & 69.58(67) & 137242 & 138652 & 263$\pm^{ 13 }_{ 13 }$ & $1.00$ & 20.0790 & 645.42 &  16.41 & 0.63\\ 
pks0405 & $0.09719$ (\#118)  & 43.14(43) & 137149 & nan & 305$\pm^{ 16 }_{ 14 }$ & $1.00$ & 20.8027 & 5.00E+19 &  16.75 & 0.00\\ 
pks0405 & $0.10152$ (\#119)  & 47.15(43) & 137149 & nan & 319$\pm^{ 15 }_{ 15 }$ & $1.00$ & 20.8848 & 4.53E+03 &  16.45 & 0.83\\ 
pks0405 & $0.10298$ (\#120)  & 43.50(43) & 137148 & nan & 317$\pm^{ 16 }_{ 15 }$ & $1.00$ & 20.9125 & 12.09 &  16.22 & 0.03\\ 
pks0405 & $0.19456$ (\#121)  & 47.40(42) & 134792 & nan & 344$\pm^{ 29 }_{ 18 }$ & $1.00$ & 22.6489 & 5.00E+19 &  16.75 & 13.44\\ 
pks0405 & $0.21976$ (\#122)  & 58.71(41) & 133933 & nan & 335$\pm^{ 20 }_{ 20 }$ & $1.00$ & 23.1266 & 2.30 &  16.02 & 0.26\\ 
pks0405 & $0.24564$ (\#123)  & 62.85(45) & 136481 & nan & 365$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.6173 & 1.49 &  15.91 & 0.39\\ 
pks0405 & $0.29748$ (\#124)  & 79.55(87) & 133010 & 137174 & 392$\pm^{ 22 }_{ 21 }$ & $1.00$ & 24.6002 & 452.10 &  16.40 & 2.68\\ 
pks0405 & $0.31016$ (\#125)  & 83.17(91) & 137132 & 137234 & 382$\pm^{ 20 }_{ 19 }$ & $1.00$ & 24.8406 & 1.08 &  15.81 & 0.48\\ 
pks0405 & $0.32502$ (\#126)  & 81.66(91) & 137139 & 137234 & 390$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.1224 & 9.34 &  16.22 & 0.45\\ 
pks0405 & $0.49508$ (\#127)  & 96.67(89) & 136537 & 137118 & 387$\pm^{ 26 }_{ 25 }$ & $1.00$ & 28.3467 & 0.66 &  15.64 & 4.48\\ 
pks0558 & $0.10472$ (\#128)  & 56.06(47) & 718011 & nan & 1867$\pm^{ 16 }_{ 16 }$ & $1.00$ & 20.9455 & 0.22 &  15.21 & 9.26\\ 
pks2155 & $0.05708$ (\#129)  & 51.87(51) & 1703911 & 1685268 & 4633$\pm^{ 441 }_{ 413 }$ & $1.47$ & 20.0422 & 0.15 &  15.05 & 7.04\\ 
pks2155 & $0.06236$ (\#130)  & 47.13(42) & 1703863 & 1685268 & 3901$\pm^{ 490 }_{ 417 }$ & $1.82$ & 20.1423 & 0.13 &  15.01 & 1.63\\ 
pks2155 & $0.10586$ (\#131)  & 53.78(37) & 1701058 & nan & 3620$\pm^{ 354 }_{ 403 }$ & $2.02$ & 20.9671 & 0.13 &  14.99 & -0.07\\ 
q0045 & $0.05590$ (\#132)  & -- & -- & -- & -- & -- & 20.0199 & -- & -- & --\\ 
q0045 & $0.06377$ (\#133)  & -- & -- & -- & -- & -- & 20.1691 & -- & -- & --\\ 
q1230 & $0.08344$ (\#134)  & 47.77(33) & 39327 & nan & 68$\pm^{ 18 }_{ 17 }$ & $1.00$ & 20.5420 & 1.15E+15 &  16.74 & 0.03\\ 
q1230 & $0.08540$ (\#135)  & 48.90(35) & 39327 & nan & 64$\pm^{ 15 }_{ 13 }$ & $1.00$ & 20.5792 & 4.63E+16 &  16.80 & 0.00\\ 
q1230 & $0.09444$ (\#136)  & 42.77(29) & 39328 & nan & 64$\pm^{ 19 }_{ 18 }$ & $1.00$ & 20.7506 & 5.00E+19 &  16.80 & 0.09\\ 
q1230 & $0.10000$ (\#137)  & 42.86(29) & 39328 & nan & 55$\pm^{ 18 }_{ 15 }$ & $1.00$ & 20.8560 & 2.06 &  16.00 & 1.71\\ 
q1230 & $0.10525$ (\#138)  & 43.32(30) & 39329 & nan & 73$\pm^{ 21 }_{ 16 }$ & $1.00$ & 20.9555 & 5.00E+19 &  16.80 & 0.78\\ 
q1230 & $0.10549$ (\#139)  & 43.13(30) & 39329 & nan & 74$\pm^{ 22 }_{ 16 }$ & $1.00$ & 20.9601 & 5.00E+19 &  16.75 & 0.99\\ 
q1230 & $0.10566$ (\#140)  & 43.20(30) & 39329 & nan & 73$\pm^{ 22 }_{ 16 }$ & $1.00$ & 20.9633 & 5.00E+19 &  16.80 & 0.90\\ 
q1230 & $0.10612$ (\#141)  & 39.76(29) & 39330 & nan & 77$\pm^{ 23 }_{ 16 }$ & $1.00$ & 20.9720 & 5.00E+19 &  16.80 & 1.52\\ 
q1230 & $0.10639$ (\#142)  & 40.21(30) & 39330 & nan & 72$\pm^{ 23 }_{ 17 }$ & $1.00$ & 20.9772 & 5.00E+19 &  16.75 & 1.23\\ 
q1230 & $0.10660$ (\#143)  & 39.93(30) & 39330 & nan & 73$\pm^{ 23 }_{ 16 }$ & $1.00$ & 20.9811 & 5.00E+19 &  16.80 & 1.54\\ 
q1230 & $0.10853$ (\#144)  & 39.15(27) & 39331 & nan & 50$\pm^{ 20 }_{ 15 }$ & $1.00$ & 21.0177 & 5.00E+19 &  16.77 & 1.22\\ 
q1230 & $0.10940$ (\#145)  & 39.98(27) & 39331 & nan & 49$\pm^{ 17 }_{ 14 }$ & $1.00$ & 21.0342 & 5.00E+19 &  16.75 & 1.53\\ 
q1230 & $0.12103$ (\#146)  & -- & -- & -- & -- & -- & 21.2547 & -- & -- & --\\ 
rbs1892 & $0.15567$ (\#147)  & -- & -- & -- & -- & -- & 21.9115 & -- & -- & --\\ 
rbs1892 & $0.15633$ (\#148)  & -- & -- & -- & -- & -- & 21.9240 & -- & -- & --\\ 
rbs1892 & $0.16343$ (\#149)  & 33.64(29) & 4929 & nan & 164$\pm^{ 103 }_{ 79 }$ & $1.00$ & 22.0586 & 1.47 &  15.91 & 11.71\\ 
rbs1892 & $0.17001$ (\#150)  & 45.15(35) & 4929 & nan & 243$\pm^{ 126 }_{ 104 }$ & $1.00$ & 22.1834 & 7.82E+07 &  16.64 & 1.30\\ 
rbs1892 & $0.17155$ (\#151)  & 46.20(37) & 4929 & nan & 316$\pm^{ 102 }_{ 77 }$ & $1.00$ & 22.2126 & 5.00E+19 &  16.80 & 0.59\\ 
rbs1892 & $0.17185$ (\#152)  & 46.34(37) & 4929 & nan & 311$\pm^{ 104 }_{ 75 }$ & $1.00$ & 22.2183 & 5.00E+19 &  16.80 & 0.56\\ 
rbs542 & $0.04455$ (\#153)  & 100.05(84) & 197378 & 212046 & 956$\pm^{ 19 }_{ 19 }$ & $1.00$ & 19.8047 & 0.56 &  15.59 & 0.23\\ 
rbs542 & $0.04992$ (\#154)  & 97.00(77) & 197040 & 212046 & 962$\pm^{ 18 }_{ 18 }$ & $1.00$ & 19.9065 & 0.74 &  15.69 & -0.01\\ 
rxj0439 & $0.00550$ (\#155)  & 111.59(94) & 146061 & 150968 & 276$\pm^{ 12 }_{ 12 }$ & $1.00$ & 19.0643 & 11.19 &  16.27 & 1.50\\ 
rxj0439 & $0.17680$ (\#156)  & 56.53(41) & 146765 & nan & 365$\pm^{ 22 }_{ 19 }$ & $1.00$ & 22.3121 & 4.37E+03 &  16.51 & 1.68\\ 
s50716 & $0.00989$ (\#157)  & 106.78(94) & 74106 & 75858 & 613$\pm^{ 25 }_{ 24 }$ & $1.00$ & 19.1475 & 3.97 &  16.12 & 0.82\\ 
s50716 & $0.01766$ (\#158)  & 104.96(94) & 74441 & 76625 & 604$\pm^{ 25 }_{ 24 }$ & $1.00$ & 19.2948 & 0.99 &  15.78 & 0.28\\ 
s50716 & $0.08834$ (\#159)  & 40.33(43) & 77052 & nan & 620$\pm^{ 28 }_{ 27 }$ & $1.00$ & 20.6349 & 0.84 &  15.73 & 2.22\\ 
s50716 & $0.14936$ (\#160)  & -- & -- & -- & -- & -- & 21.7919 & -- & -- & --\\ 
ton28 & $0.03357$ (\#161)  & 104.99(91) & 83993 & 86174 & 124$\pm^{ 12 }_{ 11 }$ & $1.00$ & 19.5965 & 1.86 &  15.97 & 0.52\\ 
tons180 & $0.04304$ (\#162)  & 73.60(82) & 187350 & 195496 & 956$\pm^{ 19 }_{ 19 }$ & $1.00$ & 19.7760 & 0.62 &  15.62 & 0.03\\ 
tons210 & $0.06763$ (\#163)  & 71.27(58) & 6723 & 6719 & 382$\pm^{ 71 }_{ 64 }$ & $1.00$ & 20.2423 & 2.18 &  16.00 & 1.12\\ 
tons210 & $0.08558$ (\#164)  & 52.71(42) & 6725 & nan & 460$\pm^{ 80 }_{ 73 }$ & $1.00$ & 20.5826 & 1.49E+04 &  16.49 & 0.14\\ 



\hline
\hline
\end{longtable}
\end{landscape}

==> Tables/XMM/Latex/xmm_o8_o6_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllllll|l}
\caption[\xmm\ Data, \oviii\ With \ovi\ Priors Results (Full)]{\oviii\ measurements with \xmm\ data, at the prior redshift from the \ovi\ lines from Table~\ref{tab:oviPriorsTable}.}
\label{tab:xmmovioviii}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & \multicolumn{2}{c}{RGS1} & \multicolumn{2}{c}{RGS2} & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \% & avg exp (s) & \%   & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.12314$ (\#1)  & 33.31(31) & 146792 & 8 & nan & nan & 963$\pm^{ 40 }_{ 26 }$ & $1.00$ & 21.2947 & $ 0.02\pm^{ 3.99 }_{ 0.61 }$ & $ 14.13\pm^{ 2.00 }_{ nan }$ & 0.01\\ 
1es1028 & $0.13706$ (\#2)  & -- & -- & -- & -- & -- & -- & -- & 21.5587 & -- & -- & --\\ 
1es1028 & $0.33735$ (\#3)  & 92.62(96) & 147900 & 8 & 144798 & 8 & 1196$\pm^{ 31 }_{ 31 }$ & $1.00$ & 25.3562 & $ 5.01\pm^{ 15.34 }_{ 3.36 }$ & $ 16.16\pm^{ 0.15 }_{ 0.24 }$ & 6.58\\ 
1es1553 & $0.18759$ (\#4)  & 29.26(27) & 1729540 & 9 & nan & nan & 540$\pm^{ 318 }_{ 194 }$ & $2.55$ & 22.5167 & $ 0.37\pm^{ 0.44 }_{ 0.33 }$ & $ 15.43\pm^{ 0.29 }_{ 0.90 }$ & 1.81\\ 
1es1553 & $0.18775$ (\#5)  & 28.91(27) & 1729540 & 9 & nan & nan & 550$\pm^{ 295 }_{ 211 }$ & $2.52$ & 22.5197 & $ 0.39\pm^{ 0.49 }_{ 0.31 }$ & $ 15.45\pm^{ 0.29 }_{ 0.62 }$ & 2.20\\ 
1es1553 & $0.18984$ (\#6)  & 25.62(27) & 1729542 & 9 & nan & nan & 406$\pm^{ 219 }_{ 140 }$ & $3.05$ & 22.5594 & $ 0.98\pm^{ 0.60 }_{ 0.48 }$ & $ 15.77\pm^{ 0.14 }_{ 0.23 }$ & 8.20\\ 
1es1553 & $0.21631$ (\#7)  & 33.20(25) & 1723969 & 9 & nan & nan & 60$\pm^{ 36 }_{ 21 }$ & $6.19$ & 23.0612 & $ -0.08\pm^{ 0.43 }_{ 0.30 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
1es1553 & $0.31130$ (\#8)  & 113.12(91) & 1744157 & 7 & 1748313 & 7 & 2268$\pm^{ 757 }_{ 440 }$ & $0.67$ & 24.8622 & $ 1.01\pm^{ 0.37 }_{ 0.33 }$ & $ 15.80\pm^{ 0.10 }_{ 0.14 }$ & 17.08\\ 
1es1553 & $0.37868$ (\#9)  & 113.07(88) & 1784762 & 7 & 1713272 & 8 & 1213$\pm^{ 467 }_{ 336 }$ & $1.52$ & 26.1398 & $ 1.03\pm^{ 0.44 }_{ 0.35 }$ & $ 15.79\pm^{ 0.11 }_{ 0.14 }$ & 15.34\\ 
1es1553 & $0.39497$ (\#10)  & 118.64(92) & 1704141 & 7 & 1756581 & 9 & 481$\pm^{ 192 }_{ 138 }$ & $2.74$ & 26.4486 & $ -0.20\pm^{ 0.19 }_{ 0.18 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.31\\ 
3c249 & $0.24676$ (\#11)  & 41.19(50) & 2644 & 37 & 2524 & inf & 373$\pm^{ 135 }_{ 107 }$ & $1.00$ & 23.6386 & $ 43.49\pm^{ 1.00E+20 }_{ 73.49 }$ & $ 16.33\pm^{ 0.47 }_{ nan }$ & 0.10\\ 
3c249 & $0.30788$ (\#12)  & 70.28(91) & 2641 & 15 & 2524 & 8 & 269$\pm^{ 119 }_{ 90 }$ & $1.00$ & 24.7974 & $ -1.35\pm^{ 1.00E+20 }_{ 2.77 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.05\\ 
3c249 & $0.30809$ (\#13)  & 70.31(91) & 2641 & 15 & 2524 & 8 & 271$\pm^{ 119 }_{ 91 }$ & $1.00$ & 24.8014 & $ -0.85\pm^{ 3.10E+14 }_{ 29.15 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
3c249 & $0.31364$ (\#14)  & 73.37(90) & 2640 & 17 & 2524 & 5 & 377$\pm^{ 139 }_{ 111 }$ & $1.00$ & 24.9066 & $ 4.71E+06\pm^{ 1.00E+20 }_{ 4.71E+06 }$ & $ 16.62\pm^{ 0.18 }_{ nan }$ & 1.07\\ 
3c273 & $0.00337$ (\#15)  & 122.62(82) & 1002935 & 3 & 1016589 & 3 & 2162$\pm^{ 179 }_{ 168 }$ & $2.23$ & 19.0239 & $ -0.01\pm^{ 0.61 }_{ 0.03 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.27\\ 
3c273 & $0.00533$ (\#16)  & 121.19(82) & 1000681 & 3 & 1016019 & 4 & 2034$\pm^{ 174 }_{ 166 }$ & $2.37$ & 19.0611 & $ 0.05\pm^{ 0.10 }_{ 0.17 }$ & $ 14.58\pm^{ 0.47 }_{ nan }$ & -0.06\\ 
3c273 & $0.00764$ (\#17)  & 119.15(82) & 1000362 & 3 & 1015449 & 4 & 1895$\pm^{ 175 }_{ 164 }$ & $2.53$ & 19.1049 & $ 0.13\pm^{ 0.11 }_{ 0.17 }$ & $ 14.99\pm^{ 0.26 }_{ nan }$ & 0.70\\ 
3c273 & $0.02947$ (\#18)  & 124.26(90) & 979671 & 3 & 1010400 & 4 & 2182$\pm^{ 194 }_{ 180 }$ & $2.22$ & 19.5188 & $ -0.00\pm^{ 0.16 }_{ 0.14 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
3c273 & $0.04898$ (\#19)  & 97.81(72) & 981682 & 3 & 1017674 & 4 & 2995$\pm^{ 379 }_{ 339 }$ & $1.54$ & 19.8887 & $ -0.02\pm^{ 0.09 }_{ 0.25 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.19\\ 
3c273 & $0.06655$ (\#20)  & 70.47(59) & 1020346 & 4 & 1015505 & 4 & 3584$\pm^{ 502 }_{ 559 }$ & $1.18$ & 20.2218 & $ -0.09\pm^{ 0.43 }_{ 0.08 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.58\\ 
3c273 & $0.09018$ (\#21)  & 39.08(47) & 949280 & 4 & nan & nan & 2360$\pm^{ 380 }_{ 338 }$ & $2.03$ & 20.6698 & $ 0.15\pm^{ 0.31 }_{ 0.14 }$ & $ 15.05\pm^{ 0.45 }_{ 1.84 }$ & 1.16\\ 
3c273 & $0.12007$ (\#22)  & 29.12(34) & 930918 & 4 & nan & nan & 2926$\pm^{ 1141 }_{ 776 }$ & $1.62$ & 21.2365 & $ 0.01\pm^{ 0.13 }_{ 0.30 }$ & $ 13.82\pm^{ 1.21 }_{ nan }$ & -0.04\\ 
3c273 & $0.14660$ (\#23)  & -- & -- & -- & -- & -- & -- & -- & 21.7395 & -- & -- & --\\ 
3c273 & $0.15784$ (\#24)  & 34.61(25) & 1047179 & 4 & nan & nan & 2310$\pm^{ 773 }_{ 593 }$ & $2.01$ & 21.9526 & $ -0.53\pm^{ 0.17 }_{ 0.15 }$ & $ nan\pm^{ nan }_{ nan }$ & 12.16\\ 
h1821 & $0.02438$ (\#25)  & 127.18(98) & 30082 & 34 & 44303 & 33 & 1073$\pm^{ 56 }_{ 55 }$ & $1.00$ & 19.4222 & $ -0.48\pm^{ 1.75 }_{ 0.82 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.18\\ 
h1821 & $0.10817$ (\#26)  & 50.54(39) & 33073 & 43 & nan & nan & 1206$\pm^{ 79 }_{ 77 }$ & $1.00$ & 21.0109 & $ -0.66\pm^{ 4.98 }_{ 1.17 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.13\\ 
h1821 & $0.12133$ (\#27)  & 38.85(28) & 33486 & 46 & nan & nan & 1220$\pm^{ 99 }_{ 97 }$ & $1.00$ & 21.2604 & $ 0.79\pm^{ 330.83 }_{ 2.13 }$ & $ 15.70\pm^{ 0.69 }_{ nan }$ & 0.08\\ 
h1821 & $0.12147$ (\#28)  & 38.90(28) & 33486 & 46 & nan & nan & 1214$\pm^{ 99 }_{ 97 }$ & $1.00$ & 21.2631 & $ 0.30\pm^{ 64.44 }_{ 1.91 }$ & $ 15.34\pm^{ 1.02 }_{ nan }$ & 0.01\\ 
h1821 & $0.16992$ (\#29)  & 47.55(34) & 32399 & 54 & nan & nan & 970$\pm^{ 94 }_{ 91 }$ & $1.00$ & 22.1817 & $ 0.21\pm^{ 8.43E+06 }_{ 2.24 }$ & $ 15.20\pm^{ 1.38 }_{ nan }$ & 0.00\\ 
h1821 & $0.17043$ (\#30)  & 47.37(34) & 32399 & 54 & nan & nan & 986$\pm^{ 100 }_{ 91 }$ & $1.00$ & 22.1914 & $ 4.63\pm^{ 6.81E+13 }_{ 6.06 }$ & $ 16.15\pm^{ 0.61 }_{ nan }$ & 0.23\\ 
h1821 & $0.21326$ (\#31)  & 58.03(45) & 29109 & 56 & nan & nan & 975$\pm^{ 94 }_{ 92 }$ & $1.00$ & 23.0034 & $ -1.61\pm^{ 3.48 }_{ 1.02 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.60\\ 
h1821 & $0.22497$ (\#32)  & 67.04(48) & 29437 & 57 & nan & nan & 945$\pm^{ 94 }_{ 91 }$ & $1.00$ & 23.2254 & $ -2.05\pm^{ 1.41 }_{ 0.76 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.95\\ 
h1821 & $0.22522$ (\#33)  & 66.78(47) & 29837 & 57 & nan & nan & 962$\pm^{ 94 }_{ 90 }$ & $1.00$ & 23.2302 & $ -2.04\pm^{ 1.72 }_{ 0.93 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.57\\ 
h1821 & $0.22639$ (\#34)  & 68.85(47) & 29881 & 57 & nan & nan & 947$\pm^{ 93 }_{ 89 }$ & $1.00$ & 23.2524 & $ -1.72\pm^{ 1.87 }_{ 0.84 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.14\\ 
h1821 & $0.24531$ (\#35)  & 72.51(51) & 31382 & 55 & 32028 & 39 & 1052$\pm^{ 92 }_{ 86 }$ & $1.00$ & 23.6111 & $ 3.97\pm^{ 6.56E+07 }_{ 5.11 }$ & $ 16.12\pm^{ 0.54 }_{ nan }$ & 0.31\\ 
h1821 & $0.26657$ (\#36)  & 79.55(72) & 31337 & 54 & 42756 & 42 & 1040$\pm^{ 83 }_{ 81 }$ & $1.00$ & 24.0142 & $ -1.77\pm^{ 1.37 }_{ 0.81 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.71\\ 
h1821 & $0.28800$ (\#37)  & 114.20(93) & 27766 & 49 & 42046 & 40 & 1294$\pm^{ 95 }_{ 91 }$ & $1.00$ & 24.4205 & $ 2.11\pm^{ 97.57 }_{ 2.56 }$ & $ 16.00\pm^{ 0.38 }_{ nan }$ & 0.65\\ 
h1821 & $0.29658$ (\#38)  & 111.33(97) & 27950 & 49 & 42972 & 39 & 1276$\pm^{ 93 }_{ 91 }$ & $1.00$ & 24.5832 & $ -1.34\pm^{ 1.14 }_{ 0.71 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.58\\ 
h1821 & $0.29680$ (\#39)  & 112.27(97) & 27836 & 49 & 43008 & 39 & 1282$\pm^{ 94 }_{ 91 }$ & $1.00$ & 24.5873 & $ -1.12\pm^{ 1.32 }_{ 0.75 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.00\\ 
h2356 & $0.11461$ (\#40)  & 57.52(40) & 476224 & 7 & nan & nan & 1072$\pm^{ 17 }_{ 14 }$ & $1.00$ & 21.1330 & $ 0.01\pm^{ 2.12 }_{ 0.23 }$ & $ 13.79\pm^{ 2.21 }_{ nan }$ & 0.03\\ 
h2356 & $0.16512$ (\#41)  & 37.80(32) & 505443 & 7 & nan & nan & 1093$\pm^{ 17 }_{ 20 }$ & $1.00$ & 22.0907 & $ -0.03\pm^{ 0.61 }_{ 0.63 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
he0056 & $0.16392$ (\#42)  & 27.81(24) & 160091 & 16 & nan & nan & 356$\pm^{ 24 }_{ 22 }$ & $1.00$ & 22.0679 & $ 31.45\pm^{ 5.71E+04 }_{ 29.99 }$ & $ 16.31\pm^{ 0.23 }_{ 0.40 }$ & 2.53\\ 
he0056 & $0.16492$ (\#43)  & 28.43(24) & 160091 & 16 & nan & nan & 353$\pm^{ 25 }_{ 21 }$ & $1.00$ & 22.0869 & $ 8.08\pm^{ 1.06E+04 }_{ 7.85 }$ & $ 16.21\pm^{ 0.29 }_{ 0.96 }$ & 1.64\\ 
he0226 & $0.01746$ (\#44)  & 124.17(84) & 31711 & 17 & 31707 & 30 & 157$\pm^{ 20 }_{ 19 }$ & $1.00$ & 19.2910 & $ -1.87\pm^{ 2.58 }_{ 1.13 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.93\\ 
he0226 & $0.02679$ (\#45)  & 131.34(93) & 31711 & 20 & 31707 & 31 & 154$\pm^{ 20 }_{ 18 }$ & $1.00$ & 19.4679 & $ -0.27\pm^{ 579.74 }_{ 1.88 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
he0226 & $0.04121$ (\#46)  & 120.74(81) & 31711 & 19 & 31707 & 33 & 166$\pm^{ 22 }_{ 20 }$ & $1.00$ & 19.7413 & $ -1.70\pm^{ 4.07 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.53\\ 
he0226 & $0.04535$ (\#47)  & 113.12(77) & 31711 & 22 & 31707 & 32 & 161$\pm^{ 22 }_{ 20 }$ & $1.00$ & 19.8198 & $ -1.30\pm^{ 8.63 }_{ 1.26 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.29\\ 
he0226 & $0.04609$ (\#48)  & 112.96(76) & 31711 & 24 & 31707 & 32 & 164$\pm^{ 22 }_{ 20 }$ & $1.00$ & 19.8339 & $ -0.63\pm^{ 109.55 }_{ 1.94 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
he0226 & $0.06015$ (\#49)  & 84.08(65) & 31711 & 30 & 31707 & 36 & 121$\pm^{ 22 }_{ 20 }$ & $1.00$ & 20.1004 & $ -4.04\pm^{ 0.97 }_{ 0.76 }$ & $ nan\pm^{ nan }_{ nan }$ & 8.15\\ 
he0226 & $0.06083$ (\#50)  & 83.15(64) & 31711 & 29 & 31707 & 36 & 129$\pm^{ 22 }_{ 20 }$ & $1.00$ & 20.1133 & $ -3.38\pm^{ 1.02 }_{ 0.73 }$ & $ nan\pm^{ nan }_{ nan }$ & 5.31\\ 
he0226 & $0.07023$ (\#51)  & 66.31(54) & 31711 & 29 & 31707 & 36 & 170$\pm^{ 24 }_{ 23 }$ & $1.00$ & 20.2916 & $ 0.37\pm^{ 1.57E+08 }_{ 2.69 }$ & $ 15.42\pm^{ 1.24 }_{ nan }$ & 0.01\\ 
he0226 & $0.08375$ (\#52)  & 52.16(42) & 31711 & 25 & nan & nan & 196$\pm^{ 28 }_{ 23 }$ & $1.00$ & 20.5479 & $ 4.04E+08\pm^{ 1.00E+20 }_{ 4.04E+08 }$ & $ 16.65\pm^{ 0.14 }_{ -0.14 }$ & 2.53\\ 
he0226 & $0.08901$ (\#53)  & 47.97(42) & 31711 & 24 & nan & nan & 183$\pm^{ 25 }_{ 23 }$ & $1.00$ & 20.6476 & $ -2.40\pm^{ 2.42 }_{ 1.09 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.23\\ 
he0226 & $0.08938$ (\#54)  & 47.78(42) & 31711 & 24 & nan & nan & 182$\pm^{ 25 }_{ 23 }$ & $1.00$ & 20.6546 & $ -2.67\pm^{ 2.28 }_{ 1.19 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.47\\ 
he0226 & $0.08950$ (\#55)  & 46.05(43) & 31711 & 23 & nan & nan & 182$\pm^{ 25 }_{ 23 }$ & $1.00$ & 20.6569 & $ -2.57\pm^{ 2.05 }_{ 1.02 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.57\\ 
he0226 & $0.09220$ (\#56)  & 46.95(42) & 31711 & 24 & nan & nan & 186$\pm^{ 25 }_{ 23 }$ & $1.00$ & 20.7081 & $ -2.29\pm^{ 3.14 }_{ 1.16 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.92\\ 
he0226 & $0.10668$ (\#57)  & 50.29(43) & 31711 & 18 & nan & nan & 175$\pm^{ 26 }_{ 24 }$ & $1.00$ & 20.9827 & $ -2.67\pm^{ 1.60 }_{ 0.85 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.23\\ 
he0226 & $0.11514$ (\#58)  & 39.66(36) & 31711 & 15 & nan & nan & 203$\pm^{ 30 }_{ 27 }$ & $1.00$ & 21.1431 & $ 3.88\pm^{ 5.21E+09 }_{ 33.88 }$ & $ 16.12\pm^{ 0.54 }_{ nan }$ & 0.15\\ 
he0226 & $0.11680$ (\#59)  & 37.43(34) & 31711 & 15 & nan & nan & 207$\pm^{ 37 }_{ 25 }$ & $1.00$ & 21.1745 & $ 5.70E+04\pm^{ 1.00E+20 }_{ 5.70E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 1.76\\ 
he0226 & $0.11733$ (\#60)  & 36.95(34) & 31711 & 15 & nan & nan & 202$\pm^{ 39 }_{ 25 }$ & $1.00$ & 21.1846 & $ 2.48E+04\pm^{ 1.00E+20 }_{ 2.48E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 2.01\\ 
he0226 & $0.12589$ (\#61)  & 35.52(30) & 31712 & 15 & nan & nan & 206$\pm^{ 36 }_{ 27 }$ & $1.00$ & 21.3469 & $ 1.54E+06\pm^{ 1.00E+20 }_{ 1.54E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 2.12\\ 
he0226 & $0.13832$ (\#62)  & -- & -- & -- & -- & -- & -- & -- & 21.5825 & -- & -- & --\\ 
he0226 & $0.15175$ (\#63)  & -- & -- & -- & -- & -- & -- & -- & 21.8372 & -- & -- & --\\ 
he0226 & $0.15549$ (\#64)  & -- & -- & -- & -- & -- & -- & -- & 21.9081 & -- & -- & --\\ 
he0226 & $0.16237$ (\#65)  & 33.50(25) & 31712 & 27 & nan & nan & 113$\pm^{ 37 }_{ 33 }$ & $1.00$ & 22.0385 & $ -5.22\pm^{ 1.12 }_{ 1.03 }$ & $ nan\pm^{ nan }_{ nan }$ & 15.81\\ 
he0226 & $0.16339$ (\#66)  & 33.20(26) & 31712 & 28 & nan & nan & 113$\pm^{ 36 }_{ 32 }$ & $1.00$ & 22.0579 & $ -5.22\pm^{ 1.07 }_{ 0.98 }$ & $ nan\pm^{ nan }_{ nan }$ & 16.22\\ 
he0226 & $0.16971$ (\#67)  & 40.73(28) & 31712 & 36 & nan & nan & 140$\pm^{ 34 }_{ 30 }$ & $1.00$ & 22.1777 & $ -2.91\pm^{ 9.88E+04 }_{ 2.04 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.43\\ 
he0226 & $0.18619$ (\#68)  & 50.47(36) & 31712 & 33 & nan & nan & 175$\pm^{ 30 }_{ 27 }$ & $1.00$ & 22.4902 & $ 2.41E+05\pm^{ 1.00E+20 }_{ 2.41E+05 }$ & $ 16.59\pm^{ 0.15 }_{ nan }$ & 1.41\\ 
he0226 & $0.18811$ (\#69)  & 48.87(35) & 31712 & 26 & nan & nan & 219$\pm^{ 37 }_{ 30 }$ & $1.00$ & 22.5266 & $ 5.13E+06\pm^{ 1.00E+20 }_{ 5.13E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 1.73\\ 
he0226 & $0.18891$ (\#70)  & 57.62(39) & 31712 & 31 & nan & nan & 196$\pm^{ 30 }_{ 28 }$ & $1.00$ & 22.5417 & $ 2.30E+08\pm^{ 1.00E+20 }_{ 2.30E+08 }$ & $ 16.69\pm^{ 0.11 }_{ -0.11 }$ & 2.21\\ 
he0226 & $0.19374$ (\#71)  & 46.89(38) & 31712 & 38 & nan & nan & 168$\pm^{ 30 }_{ 28 }$ & $1.00$ & 22.6333 & $ 5.60E+07\pm^{ 1.00E+20 }_{ 5.60E+07 }$ & $ 16.66\pm^{ 0.14 }_{ -0.14 }$ & 2.44\\ 
he0226 & $0.19453$ (\#72)  & 48.32(38) & 31712 & 40 & nan & nan & 157$\pm^{ 34 }_{ 26 }$ & $1.00$ & 22.6483 & $ 609.96\pm^{ 1.00E+20 }_{ 639.96 }$ & $ 16.45\pm^{ 0.30 }_{ nan }$ & 0.67\\ 
he0226 & $0.19860$ (\#73)  & 51.59(40) & 31712 & 38 & nan & nan & 161$\pm^{ 31 }_{ 28 }$ & $1.00$ & 22.7255 & $ 0.09\pm^{ 1.14E+13 }_{ 30.09 }$ & $ 14.85\pm^{ 1.87 }_{ nan }$ & 0.00\\ 
he0226 & $0.20055$ (\#74)  & 50.95(40) & 31712 & 38 & nan & nan & 166$\pm^{ 29 }_{ 27 }$ & $1.00$ & 22.7624 & $ 4.03E+03\pm^{ 1.00E+20 }_{ 4.06E+03 }$ & $ 16.52\pm^{ 0.27 }_{ nan }$ & 0.43\\ 
he0226 & $0.20703$ (\#75)  & 53.97(42) & 31712 & 43 & nan & nan & 158$\pm^{ 30 }_{ 27 }$ & $1.00$ & 22.8853 & $ -0.72\pm^{ 5.88E+08 }_{ 2.56 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
he0226 & $0.22009$ (\#76)  & 36.18(41) & 31713 & 38 & nan & nan & 188$\pm^{ 33 }_{ 30 }$ & $1.00$ & 23.1329 & $ 0.49\pm^{ 9.51E+12 }_{ 30.49 }$ & $ 15.53\pm^{ 1.19 }_{ nan }$ & 0.00\\ 
he0226 & $0.22099$ (\#77)  & 39.39(41) & 31713 & 36 & nan & nan & 197$\pm^{ 33 }_{ 30 }$ & $1.00$ & 23.1500 & $ -0.73\pm^{ 2.25E+07 }_{ 2.06 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
he0226 & $0.23009$ (\#78)  & 42.36(43) & 31713 & 38 & nan & nan & 209$\pm^{ 33 }_{ 28 }$ & $1.00$ & 23.3225 & $ 5.39E+06\pm^{ 1.00E+20 }_{ 5.39E+06 }$ & $ 16.62\pm^{ 0.18 }_{ nan }$ & 1.39\\ 
he0226 & $0.23964$ (\#79)  & 46.29(45) & 31713 & 43 & nan & nan & 171$\pm^{ 30 }_{ 27 }$ & $1.00$ & 23.5036 & $ -0.54\pm^{ 1.07E+08 }_{ 2.36 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
he0226 & $0.24522$ (\#80)  & 46.47(48) & 31713 & 44 & 31705 & 26 & 152$\pm^{ 29 }_{ 27 }$ & $1.00$ & 23.6094 & $ -2.46\pm^{ 14.39 }_{ 1.37 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.65\\ 
he0226 & $0.25099$ (\#81)  & 54.13(54) & 31713 & 42 & 31705 & 21 & 163$\pm^{ 30 }_{ 27 }$ & $1.00$ & 23.7188 & $ -0.31\pm^{ 8.20E+05 }_{ 2.71 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
he0226 & $0.27155$ (\#82)  & 78.85(73) & 31713 & 31 & 31705 & 21 & 224$\pm^{ 30 }_{ 28 }$ & $1.00$ & 24.1086 & $ 2.38E+03\pm^{ 1.00E+20 }_{ 2.41E+03 }$ & $ 16.48\pm^{ 0.31 }_{ nan }$ & 1.20\\ 
he0226 & $0.27956$ (\#83)  & 79.52(77) & 31713 & 30 & 31705 & 21 & 224$\pm^{ 32 }_{ 29 }$ & $1.00$ & 24.2605 & $ -1.80\pm^{ 4.37 }_{ 1.28 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.59\\ 
he0226 & $0.28041$ (\#84)  & 78.68(77) & 31713 & 30 & 31705 & 20 & 234$\pm^{ 33 }_{ 30 }$ & $1.00$ & 24.2766 & $ -1.37\pm^{ 16.51 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.27\\ 
he0226 & $0.29134$ (\#85)  & 83.52(84) & 31711 & 25 & 31705 & 20 & 238$\pm^{ 35 }_{ 32 }$ & $1.00$ & 24.4838 & $ -1.98\pm^{ 2.51 }_{ 1.19 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.00\\ 
he0226 & $0.29213$ (\#86)  & 86.12(85) & 31711 & 24 & 31705 & 21 & 240$\pm^{ 35 }_{ 32 }$ & $1.00$ & 24.4988 & $ -1.84\pm^{ 2.32 }_{ 0.97 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.02\\ 
he0226 & $0.30939$ (\#87)  & 97.61(90) & 31709 & 22 & 31705 & 26 & 246$\pm^{ 33 }_{ 30 }$ & $1.00$ & 24.8260 & $ 5.29\pm^{ 1.90E+06 }_{ 35.29 }$ & $ 16.16\pm^{ 0.46 }_{ nan }$ & 0.27\\ 
he0226 & $0.31833$ (\#88)  & 99.31(91) & 31708 & 25 & 31705 & 27 & 223$\pm^{ 33 }_{ 30 }$ & $1.00$ & 24.9955 & $ 15.13\pm^{ 8.43E+09 }_{ 45.13 }$ & $ 16.30\pm^{ 0.37 }_{ nan }$ & 0.49\\ 
he0226 & $0.33965$ (\#89)  & 102.15(94) & 31706 & 18 & 31705 & 30 & 273$\pm^{ 39 }_{ 31 }$ & $1.00$ & 25.3998 & $ 68.61\pm^{ 2.31E+15 }_{ 98.61 }$ & $ 16.34\pm^{ 0.44 }_{ nan }$ & 0.91\\ 
he0226 & $0.34036$ (\#90)  & 108.55(94) & 31706 & 19 & 31705 & 28 & 273$\pm^{ 40 }_{ 31 }$ & $1.00$ & 25.4132 & $ 5.55E+03\pm^{ 1.00E+20 }_{ 5.58E+03 }$ & $ 16.48\pm^{ 0.32 }_{ nan }$ & 1.70\\ 
he0226 & $0.35493$ (\#91)  & 115.28(93) & 31706 & 22 & 31704 & 20 & 247$\pm^{ 33 }_{ 30 }$ & $1.00$ & 25.6895 & $ -2.19\pm^{ 1.86 }_{ 0.91 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.51\\ 
he0226 & $0.35528$ (\#92)  & 116.14(94) & 31706 & 22 & 31704 & 20 & 242$\pm^{ 33 }_{ 30 }$ & $1.00$ & 25.6961 & $ -2.30\pm^{ 1.48 }_{ 0.79 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.04\\ 
he0226 & $0.37281$ (\#93)  & 117.30(93) & 31706 & 19 & 31704 & 25 & 305$\pm^{ 42 }_{ 33 }$ & $1.00$ & 26.0285 & $ 84.87\pm^{ 1.84E+13 }_{ 114.87 }$ & $ 16.34\pm^{ 0.39 }_{ nan }$ & 0.86\\ 
he0226 & $0.38420$ (\#94)  & 128.19(92) & 31706 & 23 & 31704 & 27 & 295$\pm^{ 38 }_{ 36 }$ & $1.00$ & 26.2444 & $ 3.95E+05\pm^{ 1.00E+20 }_{ 3.95E+05 }$ & $ 16.58\pm^{ 0.16 }_{ nan }$ & 2.16\\ 
he0226 & $0.38636$ (\#95)  & 130.09(92) & 31706 & 21 & 31704 & 29 & 281$\pm^{ 36 }_{ 34 }$ & $1.00$ & 26.2854 & $ 3.47\pm^{ 1.45E+07 }_{ 33.47 }$ & $ 16.10\pm^{ 0.52 }_{ nan }$ & 0.22\\ 
he0226 & $0.39642$ (\#96)  & 139.43(93) & 31706 & 26 & 31704 & 30 & 262$\pm^{ 37 }_{ 34 }$ & $1.00$ & 26.4761 & $ -1.35\pm^{ 5.03 }_{ 1.41 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.35\\ 
he0226 & $0.39692$ (\#97*)  & 137.43(91) & 31706 & 26 & 31704 & 30 & 261$\pm^{ 37 }_{ 34 }$ & $1.00$ & 26.4856 & $ -1.58\pm^{ 3.70 }_{ 1.34 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.52\\ 
he0226 & $0.39890$ (\#98)  & 135.24(93) & 31707 & 25 & 31704 & 31 & 270$\pm^{ 38 }_{ 35 }$ & $1.00$ & 26.5231 & $ -1.60\pm^{ 3.57 }_{ 1.31 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.54\\ 
he0226 & $0.40034$ (\#99)  & 134.81(92) & 31707 & 24 & 31704 & 30 & 276$\pm^{ 38 }_{ 35 }$ & $1.00$ & 26.5504 & $ -0.65\pm^{ 63.36 }_{ 1.81 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.05\\ 
he0226 & $0.40274$ (\#100)  & 137.73(93) & 31707 & 23 & 31704 & 32 & 295$\pm^{ 39 }_{ 36 }$ & $1.00$ & 26.5960 & $ 6.17\pm^{ 7.88E+08 }_{ 36.17 }$ & $ 16.17\pm^{ 0.45 }_{ nan }$ & 0.26\\ 
he0226 & $0.49225$ (\#101)  & 110.65(88) & 31709 & 28 & 31712 & 47 & 363$\pm^{ 50 }_{ 46 }$ & $1.00$ & 28.2931 & $ 0.19\pm^{ 1.35E+05 }_{ 2.56 }$ & $ 15.16\pm^{ 1.41 }_{ nan }$ & 0.00\\ 
he0226 & $0.49254$ (\#102)  & 110.33(88) & 31709 & 28 & 31712 & 49 & 359$\pm^{ 49 }_{ 46 }$ & $1.00$ & 28.2986 & $ -0.68\pm^{ 874.00 }_{ 1.68 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
he0226 & $0.49280$ (\#103)  & 110.26(88) & 31709 & 28 & 31712 & 49 & 357$\pm^{ 50 }_{ 46 }$ & $1.00$ & 28.3035 & $ -1.08\pm^{ 54.49 }_{ 1.75 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.12\\ 
he0226 & $0.49309$ (\#104)  & 109.11(87) & 31709 & 29 & 31713 & 49 & 348$\pm^{ 49 }_{ 46 }$ & $1.00$ & 28.3090 & $ -1.32\pm^{ 10.14 }_{ 1.32 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.27\\ 
i22456 & $0.09858$ (\#105)  & 56.99(44) & 79900 & 60 & nan & nan & 498$\pm^{ 28 }_{ 27 }$ & $1.00$ & 20.8291 & $ 2.67E+06\pm^{ 1.00E+20 }_{ 1.34E+06 }$ & $ 16.62\pm^{ 0.12 }_{ 0.00 }$ & 4.29\\ 
i22456 & $0.09895$ (\#106)  & 60.07(44) & 79900 & 60 & nan & nan & 499$\pm^{ 44 }_{ 27 }$ & $1.00$ & 20.8361 & $ 3.99E+04\pm^{ 1.00E+20 }_{ 3.99E+04 }$ & $ 16.52\pm^{ 0.28 }_{ nan }$ & 3.98\\ 
i22456 & $0.09931$ (\#107)  & 59.72(44) & 79900 & 60 & nan & nan & 501$\pm^{ 44 }_{ 27 }$ & $1.00$ & 20.8429 & $ 2.38E+04\pm^{ 1.00E+20 }_{ 1.19E+04 }$ & $ 16.54\pm^{ 0.26 }_{ 0.00 }$ & 4.43\\ 
i22456 & $0.09959$ (\#108)  & 54.85(44) & 79898 & 60 & nan & nan & 498$\pm^{ 28 }_{ 27 }$ & $1.00$ & 20.8482 & $ 1.73E+06\pm^{ 1.00E+20 }_{ 1.63E+06 }$ & $ 16.62\pm^{ 0.12 }_{ 0.07 }$ & 4.62\\ 
i22456 & $0.09989$ (\#109)  & 55.11(44) & 79898 & 60 & nan & nan & 496$\pm^{ 38 }_{ 27 }$ & $1.00$ & 20.8539 & $ 2.00E+04\pm^{ 1.00E+20 }_{ 2.00E+04 }$ & $ 16.54\pm^{ 0.24 }_{ nan }$ & 4.24\\ 
i22456 & $0.10034$ (\#110)  & 55.73(44) & 79898 & 60 & nan & nan & 500$\pm^{ 28 }_{ 27 }$ & $1.00$ & 20.8624 & $ 2.24E+04\pm^{ 1.00E+20 }_{ 2.24E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 4.33\\ 
i22456 & $0.10101$ (\#111)  & 55.60(44) & 79897 & 60 & nan & nan & 495$\pm^{ 38 }_{ 27 }$ & $1.00$ & 20.8751 & $ 716.19\pm^{ 1.00E+20 }_{ 606.50 }$ & $ 16.45\pm^{ 0.30 }_{ 0.05 }$ & 3.43\\ 
i22456 & $0.10146$ (\#112)  & 55.42(44) & 79897 & 60 & nan & nan & 499$\pm^{ 28 }_{ 28 }$ & $1.00$ & 20.8837 & $ 6.78E+04\pm^{ 3.72E+11 }_{ 6.07E+04 }$ & $ 16.55\pm^{ 0.18 }_{ 0.07 }$ & 3.55\\ 
mr2251 & $0.01070$ (\#113)  & 126.25(97) & 415723 & 5 & 451165 & 5 & 1562$\pm^{ 16 }_{ 16 }$ & $1.00$ & 19.1629 & $ -0.66\pm^{ 0.21 }_{ 0.19 }$ & $ nan\pm^{ nan }_{ nan }$ & 9.49\\ 
mrk421 & $0.01009$ (\#114*)  & 95.39(57) & 1385032 & 10 & 1437210 & 10 & 27095$\pm^{ 56 }_{ 49 }$ & $1.00$ & 19.1513 & $ 0.09\pm^{ 0.11 }_{ 0.02 }$ & $ 14.87\pm^{ 0.32 }_{ 0.11 }$ & 9.73\\
mrk876 & $0.00311$ (\#115)  & 98.25(96) & 2693 & 31 & 2600 & 9 & 283$\pm^{ 87 }_{ 69 }$ & $1.00$ & 19.0190 & $ 5.15E+04\pm^{ 1.00E+20 }_{ 5.16E+04 }$ & $ 16.54\pm^{ 0.21 }_{ nan }$ & 0.38\\ 
mrk876 & $0.06248$ (\#116)  & 59.48(66) & 2754 & 16 & 2708 & 21 & 362$\pm^{ 110 }_{ 83 }$ & $1.00$ & 20.1446 & $ 3.78E+09\pm^{ 1.00E+20 }_{ 3.78E+09 }$ & $ 16.69\pm^{ 0.07 }_{ inf }$ & 1.48\\ 
mrk876 & $0.08579$ (\#117)  & 44.05(43) & 2804 & 10 & nan & nan & 444$\pm^{ 126 }_{ 109 }$ & $1.00$ & 20.5866 & $ -3.42\pm^{ 2.47 }_{ 1.14 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.79\\ 
mrk876 & $0.11488$ (\#118)  & 52.10(37) & 2790 & 15 & nan & nan & 714$\pm^{ 157 }_{ 165 }$ & $1.00$ & 21.1381 & $ 1.66E+09\pm^{ 1.00E+20 }_{ 1.66E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 3.07\\ 
mrk876 & $0.11517$ (\#119)  & 52.51(37) & 2790 & 15 & nan & nan & 706$\pm^{ 235 }_{ 159 }$ & $1.00$ & 21.1436 & $ 1.69E+06\pm^{ 1.00E+20 }_{ 1.69E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 2.62\\ 
mrk876 & $0.11588$ (\#120)  & 50.65(36) & 2788 & 16 & nan & nan & 705$\pm^{ 157 }_{ 137 }$ & $1.00$ & 21.1571 & $ 7.43E+08\pm^{ 1.00E+20 }_{ 7.43E+08 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 2.97\\ 
ngc7469 & $0.00962$ (\#121)  & 84.33(74) & 631131 & 4 & 664074 & 4 & 1941$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1424 & $ 2.35\pm^{ 0.90 }_{ 0.64 }$ & $ 16.03\pm^{ 0.06 }_{ 0.08 }$ & 45.84\\ 
ngc7469 & $0.00994$ (\#122)  & 94.79(74) & 630829 & 4 & 663435 & 4 & 1942$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1485 & $ 2.92\pm^{ 1.08 }_{ 0.81 }$ & $ 16.07\pm^{ 0.06 }_{ 0.07 }$ & 53.76\\ 
ngc7469 & $0.01153$ (\#123)  & 85.80(74) & 622605 & 4 & 665535 & 4 & 1939$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1786 & $ 3.35\pm^{ 1.86 }_{ 1.00 }$ & $ 16.10\pm^{ 0.06 }_{ 0.07 }$ & 53.36\\ 
p1103 & $0.13556$ (\#124)  & -- & -- & -- & -- & -- & -- & -- & 21.5302 & -- & -- & --\\ 
p1103 & $0.13937$ (\#125)  & -- & -- & -- & -- & -- & -- & -- & 21.6025 & -- & -- & --\\ 
p1103 & $0.14099$ (\#126)  & -- & -- & -- & -- & -- & -- & -- & 21.6332 & -- & -- & --\\ 
p1103 & $0.14126$ (\#127)  & -- & -- & -- & -- & -- & -- & -- & 21.6383 & -- & -- & --\\ 
p1103 & $0.17277$ (\#128)  & 44.35(37) & 15674 & 4 & nan & nan & 2927$\pm^{ 142 }_{ 138 }$ & $1.00$ & 22.2357 & $ 3.46E+04\pm^{ 7.18E+11 }_{ 3.47E+04 }$ & $ 16.54\pm^{ 0.15 }_{ nan }$ & 6.11\\ 
pg0003 & $0.16521$ (\#129)  & 39.30(31) & 13036 & 24 & nan & nan & 287$\pm^{ 72 }_{ 63 }$ & $1.00$ & 22.0924 & $ -3.48\pm^{ 1.86 }_{ 1.12 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.77\\ 
pg0003 & $0.20907$ (\#130)  & 38.93(42) & 13036 & 22 & nan & nan & 282$\pm^{ 58 }_{ 51 }$ & $1.00$ & 22.9240 & $ 4.32E+05\pm^{ 1.00E+20 }_{ 4.32E+05 }$ & $ 16.61\pm^{ 0.13 }_{ nan }$ & 0.89\\ 
pg0003 & $0.29021$ (\#131)  & 98.06(84) & 13036 & 43 & 12941 & 11 & 230$\pm^{ 57 }_{ 49 }$ & $1.00$ & 24.4624 & $ -2.91\pm^{ 1.47 }_{ 0.87 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.68\\ 
pg0003 & $0.30551$ (\#132)  & 110.03(89) & 13035 & 41 & 12941 & 9 & 297$\pm^{ 62 }_{ 55 }$ & $1.00$ & 24.7525 & $ 1.49E+05\pm^{ 1.00E+20 }_{ 1.49E+05 }$ & $ 16.56\pm^{ 0.24 }_{ nan }$ & 1.06\\ 
pg0003 & $0.30569$ (\#133)  & 111.09(89) & 13035 & 43 & 12941 & 9 & 297$\pm^{ 71 }_{ 55 }$ & $1.00$ & 24.7559 & $ 8.96E+04\pm^{ 1.00E+20 }_{ 8.96E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 1.07\\ 
pg0003 & $0.34757$ (\#134)  & 112.83(95) & 13033 & 24 & 12938 & 19 & 306$\pm^{ 63 }_{ 54 }$ & $1.00$ & 25.5499 & $ 2.65\pm^{ 2.29E+13 }_{ 32.65 }$ & $ 16.04\pm^{ 0.69 }_{ nan }$ & 0.09\\ 
pg0003 & $0.34788$ (\#135)  & 112.95(95) & 13033 & 24 & 12938 & 20 & 297$\pm^{ 60 }_{ 53 }$ & $1.00$ & 25.5558 & $ 1.11\pm^{ 2.80E+09 }_{ 31.11 }$ & $ 15.82\pm^{ 0.86 }_{ nan }$ & 0.03\\ 
pg0003 & $0.36452$ (\#136)  & 111.56(93) & 13033 & 20 & 12904 & 26 & 311$\pm^{ 62 }_{ 55 }$ & $1.00$ & 25.8713 & $ 2.13\pm^{ 9.82E+12 }_{ 32.13 }$ & $ 15.99\pm^{ 0.72 }_{ nan }$ & 0.04\\ 
pg0003 & $0.36508$ (\#137)  & 109.85(94) & 13033 & 18 & 12903 & 28 & 308$\pm^{ 63 }_{ 55 }$ & $1.00$ & 25.8819 & $ -0.48\pm^{ 3.01E+07 }_{ 2.43 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pg0003 & $0.36572$ (\#138)  & 108.78(93) & 13033 & 16 & 12902 & 29 & 322$\pm^{ 64 }_{ 56 }$ & $1.00$ & 25.8941 & $ -0.80\pm^{ 5.19E+05 }_{ 2.38 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.03\\ 
pg0003 & $0.36621$ (\#139)  & 111.21(94) & 13033 & 18 & 12901 & 27 & 311$\pm^{ 62 }_{ 55 }$ & $1.00$ & 25.9033 & $ -1.12\pm^{ 5.70E+04 }_{ 2.04 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.08\\ 
pg0003 & $0.37029$ (\#140)  & 111.68(94) & 13033 & 20 & 12891 & 30 & 338$\pm^{ 67 }_{ 60 }$ & $1.00$ & 25.9807 & $ 8.09E+03\pm^{ 1.00E+20 }_{ 8.12E+03 }$ & $ 16.50\pm^{ 0.30 }_{ nan }$ & 0.59\\ 
pg0003 & $0.38608$ (\#141)  & 106.87(92) & 13033 & 32 & 12857 & 29 & 250$\pm^{ 69 }_{ 51 }$ & $1.00$ & 26.2801 & $ 3.31E+09\pm^{ 1.00E+20 }_{ 3.31E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.56\\ 
pg0003 & $0.38639$ (\#142)  & 106.91(93) & 13033 & 33 & 12857 & 29 & 237$\pm^{ 59 }_{ 49 }$ & $1.00$ & 26.2860 & $ 4.16E+07\pm^{ 1.00E+20 }_{ 4.16E+07 }$ & $ 16.64\pm^{ 0.16 }_{ -0.16 }$ & 1.19\\ 
pg0003 & $0.40138$ (\#143)  & 126.94(94) & 13034 & 33 & 12830 & 29 & 339$\pm^{ 76 }_{ 60 }$ & $1.00$ & 26.5702 & $ 6.72E+06\pm^{ 1.00E+20 }_{ 6.72E+06 }$ & $ 16.62\pm^{ 0.18 }_{ nan }$ & 1.59\\ 
pg0003 & $0.42192$ (\#144)  & 130.53(94) & 13034 & 47 & 12830 & 24 & 305$\pm^{ 79 }_{ 64 }$ & $1.00$ & 26.9596 & $ 11.39\pm^{ 1.48E+14 }_{ 41.39 }$ & $ 16.26\pm^{ 0.50 }_{ nan }$ & 0.25\\ 
pg0157 & $0.14621$ (\#145)  & -- & -- & -- & -- & -- & -- & -- & 21.7321 & -- & -- & --\\ 
pg0804 & $0.00382$ (\#146)  & 96.91(99) & 28317 & 7 & 30000 & 5 & 1025$\pm^{ 49 }_{ 47 }$ & $1.00$ & 19.0324 & $ -1.17\pm^{ 1.08 }_{ 0.70 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.42\\ 
pg0804 & $0.01851$ (\#147)  & 98.66(99) & 27987 & 6 & 30600 & 5 & 1068$\pm^{ 52 }_{ 50 }$ & $1.00$ & 19.3109 & $ 1.16\pm^{ 7.95 }_{ 1.65 }$ & $ 15.83\pm^{ 0.41 }_{ nan }$ & 0.46\\ 
pg0804 & $0.10216$ (\#148)  & 59.36(43) & 28660 & 8 & nan & nan & 1091$\pm^{ 61 }_{ 59 }$ & $1.00$ & 20.8970 & $ -0.30\pm^{ 9.75 }_{ 1.42 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
pg0804 & $0.10230$ (\#149)  & 59.37(43) & 28660 & 8 & nan & nan & 1094$\pm^{ 61 }_{ 59 }$ & $1.00$ & 20.8996 & $ -0.11\pm^{ 11.49 }_{ 1.46 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pg0832 & $0.10772$ (\#150)  & 51.86(42) & 20653 & 61 & nan & nan & 49$\pm^{ 17 }_{ 14 }$ & $1.00$ & 21.0024 & $ 1.39E+03\pm^{ 1.00E+20 }_{ 1.42E+03 }$ & $ 16.46\pm^{ 0.34 }_{ nan }$ & 0.18\\ 
pg0832 & $0.13230$ (\#151)  & 33.25(28) & 20654 & 53 & nan & nan & 37$\pm^{ 21 }_{ 16 }$ & $1.00$ & 21.4684 & $ -3.53\pm^{ 2.47E+04 }_{ 2.19 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.59\\ 
pg0832 & $0.15276$ (\#152)  & -- & -- & -- & -- & -- & -- & -- & 21.8563 & -- & -- & --\\ 
pg0832 & $0.23308$ (\#153)  & 50.44(43) & 20655 & 85 & nan & nan & 60$\pm^{ 24 }_{ 18 }$ & $1.00$ & 23.3792 & $ 4.51E+09\pm^{ 1.00E+20 }_{ 4.51E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 0.38\\ 
pg0832 & $0.32567$ (\#154)  & 127.93(90) & 20654 & 142 & 20637 & 171 & 49$\pm^{ 24 }_{ 16 }$ & $1.00$ & 25.1347 & $ 3.10E+04\pm^{ 1.00E+20 }_{ 3.10E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 0.65\\ 
pg0953 & $0.01560$ (\#155)  & 111.24(90) & 12824 & 14 & 12310 & 13 & 312$\pm^{ 42 }_{ 39 }$ & $1.00$ & 19.2558 & $ -1.55\pm^{ 2.98 }_{ 1.04 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.65\\ 
pg0953 & $0.05891$ (\#156)  & 84.64(66) & 12824 & 17 & 12310 & 22 & 428$\pm^{ 49 }_{ 46 }$ & $1.00$ & 20.0769 & $ 1.25E+03\pm^{ 1.37E+15 }_{ 1.28E+03 }$ & $ 16.46\pm^{ 0.33 }_{ nan }$ & 0.71\\ 
pg0953 & $0.06807$ (\#157)  & 69.63(58) & 12824 & 16 & 12310 & 21 & 398$\pm^{ 52 }_{ 49 }$ & $1.00$ & 20.2506 & $ -2.42\pm^{ 2.69 }_{ 1.17 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.18\\ 
pg0953 & $0.11827$ (\#158)  & 36.08(32) & 12794 & 14 & nan & nan & 444$\pm^{ 71 }_{ 65 }$ & $1.00$ & 21.2024 & $ -0.76\pm^{ 1.16E+04 }_{ 1.97 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.04\\ 
pg0953 & $0.14236$ (\#159)  & -- & -- & -- & -- & -- & -- & -- & 21.6591 & -- & -- & --\\ 
pg0953 & $0.14263$ (\#160)  & -- & -- & -- & -- & -- & -- & -- & 21.6643 & -- & -- & --\\ 
pg0953 & $0.14307$ (\#161)  & -- & -- & -- & -- & -- & -- & -- & 21.6726 & -- & -- & --\\ 
pg0953 & $0.22967$ (\#162)  & 53.43(43) & 12792 & 15 & nan & nan & 475$\pm^{ 71 }_{ 65 }$ & $1.00$ & 23.3145 & $ -2.40\pm^{ 2.85 }_{ 1.12 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.08\\ 
pg0953 & $0.23251$ (\#163)  & 49.94(43) & 12792 & 14 & nan & nan & 472$\pm^{ 70 }_{ 65 }$ & $1.00$ & 23.3684 & $ -3.04\pm^{ 27.69 }_{ 1.60 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.68\\ 
pg0953 & $0.23351$ (\#164)  & 51.78(43) & 12792 & 14 & nan & nan & 480$\pm^{ 72 }_{ 67 }$ & $1.00$ & 23.3873 & $ -3.48\pm^{ 15.11 }_{ 1.45 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.88\\ 
pg1115 & $0.12285$ (\#165)  & 41.88(32) & 17510 & 23 & nan & nan & 304$\pm^{ 54 }_{ 42 }$ & $1.00$ & 21.2892 & $ 1.29E+07\pm^{ 1.00E+20 }_{ 1.29E+07 }$ & $ 16.62\pm^{ 0.18 }_{ nan }$ & 1.56\\ 
pg1115 & $0.12313$ (\#166)  & 41.92(32) & 17510 & 23 & nan & nan & 300$\pm^{ 57 }_{ 41 }$ & $1.00$ & 21.2945 & $ 4.11E+04\pm^{ 1.00E+20 }_{ 4.11E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 1.44\\ 
pg1115 & $0.13104$ (\#167*)  & 46.21(29) & 17510 & 24 & nan & nan & 319$\pm^{ 61 }_{ 46 }$ & $1.00$ & 21.4445 & $ 3.29E+04\pm^{ 1.00E+20 }_{ 3.29E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 1.03\\ 
pg1115 & $0.15456$ (\#168)  & -- & -- & -- & -- & -- & -- & -- & 21.8905 & -- & -- & --\\ 
pg1115 & $0.15467$ (\#169)  & -- & -- & -- & -- & -- & -- & -- & 21.8925 & -- & -- & --\\ 
pg1116 & $0.05900$ (\#170)  & 85.18(69) & 285035 & 13 & 294383 & 10 & 469$\pm^{ 12 }_{ 12 }$ & $1.00$ & 20.0786 & $ -0.09\pm^{ 1.50 }_{ 0.76 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pg1116 & $0.05927$ (\#171)  & 85.16(69) & 285035 & 13 & 294383 & 10 & 470$\pm^{ 12 }_{ 12 }$ & $1.00$ & 20.0838 & $ 0.09\pm^{ 1.80 }_{ 0.80 }$ & $ 14.83\pm^{ 1.14 }_{ nan }$ & 0.03\\ 
pg1116 & $0.11895$ (\#172)  & 37.22(33) & 285607 & 13 & nan & nan & 509$\pm^{ 16 }_{ 16 }$ & $1.00$ & 21.2153 & $ 0.65\pm^{ 2.98 }_{ 1.16 }$ & $ 15.64\pm^{ 0.47 }_{ nan }$ & 0.31\\ 
pg1116 & $0.13852$ (\#173)  & -- & -- & -- & -- & -- & -- & -- & 21.5863 & -- & -- & --\\ 
pg1116 & $0.16539$ (\#174)  & 36.23(32) & 288889 & 14 & nan & nan & 549$\pm^{ 18 }_{ 18 }$ & $1.00$ & 22.0958 & $ 0.72\pm^{ 3.01 }_{ 1.18 }$ & $ 15.68\pm^{ 0.44 }_{ nan }$ & 0.38\\ 
pg1116 & $0.16554$ (\#175)  & 36.14(32) & 288889 & 14 & nan & nan & 549$\pm^{ 19 }_{ 18 }$ & $1.00$ & 22.0986 & $ 0.84\pm^{ 3.58 }_{ 1.23 }$ & $ 15.72\pm^{ 0.42 }_{ nan }$ & 0.48\\ 
pg1116 & $0.16610$ (\#176)  & 37.64(33) & 289091 & 14 & nan & nan & 548$\pm^{ 18 }_{ 18 }$ & $1.00$ & 22.1093 & $ 1.26\pm^{ 4.92 }_{ 1.50 }$ & $ 15.85\pm^{ 0.34 }_{ nan }$ & 0.80\\ 
pg1116 & $0.16686$ (\#177)  & 39.71(33) & 289091 & 14 & nan & nan & 545$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.1237 & $ 1.18\pm^{ 5.60 }_{ 1.46 }$ & $ 15.84\pm^{ 0.35 }_{ nan }$ & 0.73\\ 
pg1116 & $0.17343$ (\#178)  & 50.92(38) & 289065 & 14 & nan & nan & 531$\pm^{ 16 }_{ 16 }$ & $1.00$ & 22.2482 & $ -0.67\pm^{ 1.06 }_{ 0.66 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.61\\ 
pg1211 & $0.00711$ (\#179)  & 130.66(97) & 709355 & 11 & 767876 & 10 & 488$\pm^{ 7 }_{ 7 }$ & $1.00$ & 19.0948 & $ 0.42\pm^{ 0.61 }_{ 0.46 }$ & $ 15.48\pm^{ 0.32 }_{ nan }$ & 1.02\\ 
pg1211 & $0.05117$ (\#180)  & 79.82(69) & 726954 & 10 & 778637 & 10 & 541$\pm^{ 8 }_{ 8 }$ & $1.00$ & 19.9302 & $ 0.38\pm^{ 0.68 }_{ 0.47 }$ & $ 15.44\pm^{ 0.36 }_{ nan }$ & 0.82\\ 
pg1211 & $0.06449$ (\#181)  & 80.33(55) & 776352 & 11 & 776215 & 10 & 557$\pm^{ 9 }_{ 9 }$ & $1.00$ & 20.1827 & $ -0.57\pm^{ 0.51 }_{ 0.40 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.52\\ 
pg1211 & $0.06491$ (\#182)  & 77.87(55) & 776352 & 11 & 776215 & 10 & 560$\pm^{ 9 }_{ 9 }$ & $1.00$ & 20.1907 & $ -0.50\pm^{ 0.52 }_{ 0.40 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.19\\ 
pg1216 & $0.12362$ (\#183)  & 42.81(30) & 11245 & 26 & nan & nan & 225$\pm^{ 51 }_{ 44 }$ & $1.00$ & 21.3038 & $ 1.85E+09\pm^{ 1.00E+20 }_{ 1.85E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.17\\ 
pg1216 & $0.12389$ (\#184)  & 42.84(30) & 11245 & 26 & nan & nan & 222$\pm^{ 50 }_{ 44 }$ & $1.00$ & 21.3090 & $ 2.64E+06\pm^{ 1.00E+20 }_{ 2.64E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 1.09\\ 
pg1216 & $0.12463$ (\#185)  & 43.15(30) & 11245 & 26 & nan & nan & 218$\pm^{ 58 }_{ 44 }$ & $1.00$ & 21.3230 & $ 4.36E+03\pm^{ 1.00E+20 }_{ 4.39E+03 }$ & $ 16.52\pm^{ 0.28 }_{ nan }$ & 0.72\\ 
pg1216 & $0.12485$ (\#186)  & 43.34(30) & 11245 & 26 & nan & nan & 216$\pm^{ 58 }_{ 43 }$ & $1.00$ & 21.3272 & $ 203.43\pm^{ 1.00E+20 }_{ 233.43 }$ & $ 16.43\pm^{ 0.32 }_{ nan }$ & 0.50\\ 
pg1216 & $0.13499$ (\#187)  & -- & -- & -- & -- & -- & -- & -- & 21.5194 & -- & -- & --\\ 
pg1216 & $0.26768$ (\#188)  & 88.48(70) & 11245 & 33 & 11258 & 21 & 157$\pm^{ 56 }_{ 41 }$ & $1.00$ & 24.0352 & $ 1.14E+09\pm^{ 1.00E+20 }_{ 1.14E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 3.23\\ 
pg1216 & $0.28199$ (\#189)  & 109.24(79) & 11245 & 36 & 11258 & 14 & 184$\pm^{ 46 }_{ 39 }$ & $1.00$ & 24.3065 & $ 80.21\pm^{ 1.00E+20 }_{ 110.21 }$ & $ 16.37\pm^{ 0.43 }_{ nan }$ & 0.71\\ 
pg1216 & $0.28237$ (\#190)  & 109.62(79) & 11245 & 36 & 11258 & 14 & 184$\pm^{ 46 }_{ 39 }$ & $1.00$ & 24.3137 & $ 41.22\pm^{ 1.00E+20 }_{ 71.22 }$ & $ 16.33\pm^{ 0.47 }_{ nan }$ & 0.31\\ 
pg1259 & $0.00220$ (\#191)  & 124.99(93) & 11480 & 60 & 11480 & 42 & 106$\pm^{ 26 }_{ 24 }$ & $1.00$ & 19.0017 & $ 809.18\pm^{ 1.00E+20 }_{ 839.18 }$ & $ 16.45\pm^{ 0.35 }_{ nan }$ & 0.30\\ 
pg1259 & $0.00762$ (\#192)  & 122.32(92) & 11480 & 63 & 11480 & 38 & 112$\pm^{ 30 }_{ 24 }$ & $1.00$ & 19.1045 & $ 6.51E+05\pm^{ 1.00E+20 }_{ 6.51E+05 }$ & $ 16.62\pm^{ 0.13 }_{ nan }$ & 1.94\\ 
pg1259 & $0.02217$ (\#193)  & 129.87(93) & 11480 & 52 & 11480 & 42 & 99$\pm^{ 27 }_{ 23 }$ & $1.00$ & 19.3803 & $ -1.76\pm^{ 196.56 }_{ 1.80 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.24\\ 
pg1259 & $0.04606$ (\#194)  & 94.97(77) & 11479 & 35 & 11480 & 53 & 122$\pm^{ 32 }_{ 26 }$ & $1.00$ & 19.8333 & $ 663.51\pm^{ 1.00E+20 }_{ 693.51 }$ & $ 16.45\pm^{ 0.30 }_{ nan }$ & 0.40\\ 
pg1259 & $0.04650$ (\#195)  & 92.99(76) & 11479 & 33 & 11480 & 52 & 123$\pm^{ 30 }_{ 26 }$ & $1.00$ & 19.8416 & $ 933.16\pm^{ 1.00E+20 }_{ 963.16 }$ & $ 16.45\pm^{ 0.34 }_{ nan }$ & 0.84\\ 
pg1259 & $0.19576$ (\#196)  & 53.02(43) & 11485 & 37 & nan & nan & 196$\pm^{ 49 }_{ 42 }$ & $1.00$ & 22.6716 & $ -0.32\pm^{ 1.00E+20 }_{ 29.68 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pg1259 & $0.21940$ (\#197)  & 47.70(41) & 11485 & 46 & nan & nan & 141$\pm^{ 49 }_{ 41 }$ & $1.00$ & 23.1198 & $ -5.05\pm^{ 1.34 }_{ 1.05 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.35\\ 
pg1259 & $0.21953$ (\#198)  & 47.70(41) & 11485 & 46 & nan & nan & 141$\pm^{ 48 }_{ 41 }$ & $1.00$ & 23.1223 & $ -4.44\pm^{ 1.10 }_{ 0.87 }$ & $ nan\pm^{ nan }_{ nan }$ & 6.32\\ 
pg1259 & $0.22313$ (\#199)  & 51.02(41) & 11485 & 51 & nan & nan & 179$\pm^{ 48 }_{ 41 }$ & $1.00$ & 23.1905 & $ 813.26\pm^{ 1.00E+20 }_{ 843.26 }$ & $ 16.45\pm^{ 0.35 }_{ nan }$ & 0.27\\ 
pg1259 & $0.23284$ (\#200)  & 57.87(43) & 11485 & 35 & nan & nan & 221$\pm^{ 53 }_{ 47 }$ & $1.00$ & 23.3746 & $ -2.24\pm^{ 1.00E+20 }_{ 27.76 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.06\\ 
pg1259 & $0.23956$ (\#201)  & 64.61(45) & 11485 & 40 & nan & nan & 204$\pm^{ 49 }_{ 45 }$ & $1.00$ & 23.5021 & $ 33.63\pm^{ 1.00E+20 }_{ 63.63 }$ & $ 16.32\pm^{ 0.47 }_{ nan }$ & 0.07\\ 
pg1259 & $0.25973$ (\#202)  & 74.33(62) & 11485 & 44 & 11479 & 43 & 204$\pm^{ 59 }_{ 41 }$ & $1.00$ & 23.8845 & $ 1.57E+06\pm^{ 1.00E+20 }_{ 1.57E+06 }$ & $ 16.62\pm^{ 0.13 }_{ nan }$ & 1.08\\ 
pg1259 & $0.31979$ (\#203)  & 106.65(91) & 11483 & 41 & 11479 & 44 & 148$\pm^{ 44 }_{ 36 }$ & $1.00$ & 25.0232 & $ 0.35\pm^{ 1.00E+20 }_{ 30.35 }$ & $ 15.41\pm^{ 1.39 }_{ nan }$ & 0.00\\ 
pg1259 & $0.32472$ (\#204)  & 104.67(91) & 11483 & 40 & 11479 & 44 & 156$\pm^{ 49 }_{ 38 }$ & $1.00$ & 25.1167 & $ 8.44E+08\pm^{ 1.00E+20 }_{ 8.44E+08 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.52\\ 
pg1307 & $0.14187$ (\#205)  & -- & -- & -- & -- & -- & -- & -- & 21.6499 & -- & -- & --\\ 
pg1307 & $0.14214$ (\#206)  & -- & -- & -- & -- & -- & -- & -- & 21.6550 & -- & -- & --\\ 
pg1309 & $0.17586$ (\#207)  & 38.46(33) & 27263 & 75 & nan & nan & 69$\pm^{ 22 }_{ 21 }$ & $1.00$ & 22.2943 & $ -0.02\pm^{ 1.00E+20 }_{ 29.98 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.00\\ 
pg1309 & $0.17745$ (\#208)  & 38.48(35) & 27263 & 74 & nan & nan & 68$\pm^{ 23 }_{ 19 }$ & $1.00$ & 22.3245 & $ -1.02\pm^{ 1.00E+20 }_{ 28.98 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pg1309 & $0.17866$ (\#209)  & 39.78(36) & 27263 & 76 & nan & nan & 66$\pm^{ 22 }_{ 19 }$ & $1.00$ & 22.3474 & $ 1.78\pm^{ 1.00E+20 }_{ 31.78 }$ & $ 15.95\pm^{ 0.85 }_{ nan }$ & 0.01\\ 
pg1309 & $0.17930$ (\#210)  & 40.20(37) & 27263 & 76 & nan & nan & 66$\pm^{ 22 }_{ 19 }$ & $1.00$ & 22.3595 & $ 7.63\pm^{ 1.00E+20 }_{ 37.63 }$ & $ 16.21\pm^{ 0.59 }_{ nan }$ & 0.03\\ 
pg1309 & $0.17979$ (\#211)  & 40.62(37) & 27263 & 76 & nan & nan & 65$\pm^{ 21 }_{ 18 }$ & $1.00$ & 22.3688 & $ 7.28\pm^{ 1.00E+20 }_{ 37.28 }$ & $ 16.20\pm^{ 0.60 }_{ nan }$ & 0.03\\ 
pg1309 & $0.18069$ (\#212)  & 43.43(38) & 27263 & 72 & nan & nan & 74$\pm^{ 22 }_{ 19 }$ & $1.00$ & 22.3859 & $ 1.91E+03\pm^{ 1.00E+20 }_{ 1.94E+03 }$ & $ 16.48\pm^{ 0.32 }_{ nan }$ & 0.18\\ 
pg1309 & $0.18117$ (\#213)  & 43.39(38) & 27263 & 72 & nan & nan & 74$\pm^{ 23 }_{ 19 }$ & $1.00$ & 22.3950 & $ 2.24E+03\pm^{ 1.00E+20 }_{ 2.27E+03 }$ & $ 16.49\pm^{ 0.31 }_{ nan }$ & 0.23\\ 
pg1309 & $0.18139$ (\#214)  & 44.59(39) & 27263 & 70 & nan & nan & 79$\pm^{ 21 }_{ 18 }$ & $1.00$ & 22.3992 & $ 2.25E+05\pm^{ 1.00E+20 }_{ 2.25E+05 }$ & $ 16.59\pm^{ 0.16 }_{ nan }$ & 0.42\\ 
pg1309 & $0.18145$ (\#215)  & 44.58(39) & 27263 & 70 & nan & nan & 78$\pm^{ 24 }_{ 18 }$ & $1.00$ & 22.4003 & $ 1.24E+05\pm^{ 1.00E+20 }_{ 1.24E+05 }$ & $ 16.55\pm^{ 0.24 }_{ nan }$ & 0.42\\ 
pg1309 & $0.18192$ (\#216)  & 43.04(39) & 27263 & 70 & nan & nan & 78$\pm^{ 25 }_{ 18 }$ & $1.00$ & 22.4092 & $ 1.58E+05\pm^{ 1.00E+20 }_{ 1.58E+05 }$ & $ 16.56\pm^{ 0.24 }_{ nan }$ & 0.58\\ 
pg1309 & $0.18698$ (\#217)  & 43.52(37) & 27263 & 77 & nan & nan & 79$\pm^{ 24 }_{ 19 }$ & $1.00$ & 22.5051 & $ 2.31E+04\pm^{ 1.00E+20 }_{ 2.31E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 0.52\\ 
pg1444 & $0.22031$ (\#218)  & 50.77(40) & 17630 & 43 & nan & nan & 104$\pm^{ 38 }_{ 33 }$ & $1.00$ & 23.1371 & $ -6.35\pm^{ 1.09 }_{ 1.04 }$ & $ nan\pm^{ nan }_{ nan }$ & 17.52\\ 
pg1444 & $0.22676$ (\#219)  & 57.73(42) & 17630 & 44 & nan & nan & 197$\pm^{ 39 }_{ 35 }$ & $1.00$ & 23.2594 & $ 5.11E+04\pm^{ 1.00E+20 }_{ 5.12E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 0.81\\ 
pg1444 & $0.26690$ (\#220)  & 91.99(69) & 17630 & 54 & 17137 & 37 & 162$\pm^{ 36 }_{ 32 }$ & $1.00$ & 24.0204 & $ 2.17\pm^{ 2.40E+16 }_{ 32.17 }$ & $ 16.01\pm^{ 0.78 }_{ nan }$ & 0.06\\ 
pg1444 & $0.26728$ (\#221)  & 94.03(70) & 17630 & 52 & 17137 & 37 & 166$\pm^{ 36 }_{ 32 }$ & $1.00$ & 24.0276 & $ 3.60\pm^{ 9.89E+14 }_{ 33.60 }$ & $ 16.11\pm^{ 0.69 }_{ nan }$ & 0.09\\ 
pg1444 & $0.26738$ (\#222)  & 94.02(70) & 17630 & 52 & 17137 & 37 & 166$\pm^{ 36 }_{ 32 }$ & $1.00$ & 24.0295 & $ 4.30\pm^{ 2.79E+16 }_{ 34.30 }$ & $ 16.14\pm^{ 0.66 }_{ nan }$ & 0.10\\ 
pg1444 & $0.26747$ (\#223)  & 94.01(70) & 17630 & 52 & 17137 & 37 & 166$\pm^{ 36 }_{ 32 }$ & $1.00$ & 24.0312 & $ 4.80\pm^{ 1.00E+20 }_{ 34.80 }$ & $ 16.15\pm^{ 0.60 }_{ nan }$ & 0.11\\ 
pg1626 & $0.13075$ (\#224)  & 28.51(25) & 69285 & 70 & nan & nan & 214$\pm^{ 44 }_{ 42 }$ & $1.00$ & 21.4390 & $ -3.65\pm^{ 1.35 }_{ 0.97 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.65\\ 
phl1811 & $0.07344$ (\#225)  & 64.36(45) & 77298 & 71 & 78895 & 116 & 51$\pm^{ 0 }_{ 0 }$ & $1.00$ & 20.3524 & $ 9.66E+06\pm^{ 1.00 }_{ 1.00 }$ & $ 16.62\pm^{ 0.00 }_{ -0.00 }$ & 1.51\\ 
phl1811 & $0.07768$ (\#226)  & 59.44(40) & 78263 & 67 & 78895 & 188 & 51$\pm^{ 12 }_{ 11 }$ & $1.00$ & 20.4328 & $ 71.63\pm^{ 1.00E+20 }_{ 101.63 }$ & $ 16.37\pm^{ 0.37 }_{ nan }$ & 0.08\\ 
phl1811 & $0.08131$ (\#227)  & 49.10(33) & 78178 & 68 & nan & nan & 56$\pm^{ 14 }_{ 11 }$ & $1.00$ & 20.5016 & $ 1.19E+09\pm^{ 1.00E+20 }_{ 1.19E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.80\\ 
phl1811 & $0.13239$ (\#228)  & -- & -- & -- & -- & -- & -- & -- & 21.4701 & -- & -- & --\\ 
phl1811 & $0.13282$ (\#229)  & -- & -- & -- & -- & -- & -- & -- & 21.4783 & -- & -- & --\\ 
phl1811 & $0.13318$ (\#230)  & -- & -- & -- & -- & -- & -- & -- & 21.4851 & -- & -- & --\\ 
phl1811 & $0.13545$ (\#231)  & -- & -- & -- & -- & -- & -- & -- & 21.5281 & -- & -- & --\\ 
phl1811 & $0.15752$ (\#232)  & -- & -- & -- & -- & -- & -- & -- & 21.9466 & -- & -- & --\\ 
phl1811 & $0.15786$ (\#233)  & -- & -- & -- & -- & -- & -- & -- & 21.9530 & -- & -- & --\\ 
phl1811 & $0.17652$ (\#234)  & -- & -- & -- & -- & -- & -- & -- & 22.3068 & -- & -- & --\\ 
phl1811 & $0.19157$ (\#235)  & -- & -- & -- & -- & -- & -- & -- & 22.5922 & -- & -- & --\\ 
phl1811 & $0.19194$ (\#236)  & -- & -- & -- & -- & -- & -- & -- & 22.5992 & -- & -- & --\\ 
phl1811 & $0.19220$ (\#237)  & -- & -- & -- & -- & -- & -- & -- & 22.6041 & -- & -- & --\\ 
pks0312 & $0.20188$ (\#238)  & 58.64(41) & 23887 & 48 & nan & nan & 194$\pm^{ 38 }_{ 35 }$ & $1.00$ & 22.7876 & $ -0.88\pm^{ 6.61E+16 }_{ 29.12 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.01\\ 
pks0312 & $0.20275$ (\#239)  & 59.87(41) & 23887 & 49 & nan & nan & 181$\pm^{ 37 }_{ 34 }$ & $1.00$ & 22.8041 & $ -2.34\pm^{ 3.89E+10 }_{ 2.36 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.14\\ 
pks0405 & $0.09192$ (\#240)  & 40.76(43) & 137149 & 20 & nan & nan & 285$\pm^{ 15 }_{ 14 }$ & $1.00$ & 20.7028 & $ -1.82\pm^{ 0.98 }_{ 0.66 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.85\\ 
pks0405 & $0.09647$ (\#241)  & 44.12(43) & 137149 & 20 & nan & nan & 305$\pm^{ 17 }_{ 20 }$ & $1.00$ & 20.7891 & $ 0.09\pm^{ 3.40E+14 }_{ 3.47 }$ & $ 14.83\pm^{ 1.96 }_{ nan }$ & -0.00\\ 
pks0405 & $0.14808$ (\#242)  & -- & -- & -- & -- & -- & -- & -- & 21.7676 & -- & -- & --\\ 
pks0405 & $0.16566$ (\#243)  & 34.33(32) & 137647 & 22 & nan & nan & 322$\pm^{ 21 }_{ 20 }$ & $1.00$ & 22.1009 & $ 6.62\pm^{ 1.04E+04 }_{ 6.85 }$ & $ 16.19\pm^{ 0.31 }_{ nan }$ & 1.05\\ 
pks0405 & $0.16606$ (\#244)  & 35.08(32) & 137647 & 22 & nan & nan & 320$\pm^{ 20 }_{ 20 }$ & $1.00$ & 22.1085 & $ 8.30\pm^{ 3.94E+03 }_{ 8.43 }$ & $ 16.24\pm^{ 0.29 }_{ nan }$ & 1.17\\ 
pks0405 & $0.16659$ (\#245)  & 37.18(33) & 137675 & 22 & nan & nan & 317$\pm^{ 20 }_{ 20 }$ & $1.00$ & 22.1185 & $ 7.71\pm^{ 5.09E+03 }_{ 7.93 }$ & $ 16.22\pm^{ 0.29 }_{ nan }$ & 0.98\\ 
pks0405 & $0.16688$ (\#246)  & 37.31(33) & 137675 & 22 & nan & nan & 316$\pm^{ 19 }_{ 19 }$ & $1.00$ & 22.1240 & $ 5.33\pm^{ 9.17E+03 }_{ 5.83 }$ & $ 16.17\pm^{ 0.33 }_{ nan }$ & 0.80\\ 
pks0405 & $0.16712$ (\#247)  & 37.91(33) & 137675 & 22 & nan & nan & 313$\pm^{ 21 }_{ 19 }$ & $1.00$ & 22.1286 & $ 3.07\pm^{ 1.50E+03 }_{ 3.80 }$ & $ 16.08\pm^{ 0.38 }_{ nan }$ & 0.51\\ 
pks0405 & $0.18257$ (\#248)  & 59.45(44) & 136430 & 23 & nan & nan & 304$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.4215 & $ -1.68\pm^{ 1.03 }_{ 0.62 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.41\\ 
pks0405 & $0.18289$ (\#249)  & 63.38(44) & 136430 & 23 & nan & nan & 307$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.4276 & $ -1.49\pm^{ 1.39 }_{ 0.83 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.39\\ 
pks0405 & $0.24052$ (\#250)  & 57.03(46) & 137245 & 22 & nan & nan & 367$\pm^{ 20 }_{ 19 }$ & $1.00$ & 23.5203 & $ 8.95\pm^{ 8.33E+03 }_{ 8.77 }$ & $ 16.24\pm^{ 0.29 }_{ 1.11 }$ & 1.43\\ 
pks0405 & $0.24094$ (\#251)  & 61.56(45) & 137216 & 21 & nan & nan & 377$\pm^{ 21 }_{ 19 }$ & $1.00$ & 23.5282 & $ 13.92\pm^{ 4.89E+06 }_{ 13.26 }$ & $ 16.29\pm^{ 0.28 }_{ 0.65 }$ & 1.85\\ 
pks0405 & $0.24547$ (\#252)  & 66.61(47) & 136481 & 21 & 138649 & 28 & 361$\pm^{ 19 }_{ 18 }$ & $1.00$ & 23.6141 & $ -0.97\pm^{ 1.84 }_{ 0.90 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.52\\ 
pks0405 & $0.29762$ (\#253)  & 85.15(89) & 133010 & 20 & 137234 & 19 & 392$\pm^{ 21 }_{ 21 }$ & $1.00$ & 24.6029 & $ 16.09\pm^{ 266.81 }_{ 15.18 }$ & $ 16.24\pm^{ 0.20 }_{ 0.48 }$ & 2.58\\ 
pks0405 & $0.34188$ (\#254)  & 114.95(95) & 137986 & 22 & 137234 & 21 & 365$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.4420 & $ -0.18\pm^{ 2.58 }_{ 1.09 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.02\\ 
pks0405 & $0.34225$ (\#255)  & 120.66(97) & 138000 & 22 & 137943 & 21 & 367$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.4491 & $ -0.30\pm^{ 2.31 }_{ 0.98 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.05\\ 
pks0405 & $0.35092$ (\#256)  & 113.60(95) & 138000 & 22 & 136470 & 22 & 368$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.6134 & $ -0.58\pm^{ 1.90 }_{ 0.85 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.23\\ 
pks0405 & $0.36075$ (\#257)  & 117.15(93) & 137986 & 20 & 134948 & 21 & 404$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.7998 & $ 6.47\pm^{ 3.81E+03 }_{ 6.09 }$ & $ 16.20\pm^{ 0.30 }_{ 0.76 }$ & 1.70\\ 
pks0405 & $0.36151$ (\#258)  & 115.63(94) & 138000 & 20 & 134948 & 21 & 404$\pm^{ 20 }_{ 20 }$ & $1.00$ & 25.8142 & $ 54.17\pm^{ 5.50E+05 }_{ 51.50 }$ & $ 16.34\pm^{ 0.23 }_{ 0.29 }$ & 3.70\\ 
pks0405 & $0.36329$ (\#259)  & 110.13(94) & 138000 & 20 & 134948 & 21 & 408$\pm^{ 22 }_{ 20 }$ & $1.00$ & 25.8480 & $ 2.92E+04\pm^{ 4.34E+09 }_{ 2.88E+04 }$ & $ 16.50\pm^{ 0.16 }_{ 0.06 }$ & 8.04\\ 
pks0405 & $0.40570$ (\#260)  & 109.37(95) & 137975 & 19 & 138647 & 28 & 415$\pm^{ 23 }_{ 21 }$ & $1.00$ & 26.6521 & $ 0.37\pm^{ 20.34 }_{ 1.50 }$ & $ 15.43\pm^{ 0.83 }_{ nan }$ & 0.05\\ 
pks0405 & $0.40890$ (\#261)  & 111.06(95) & 137975 & 20 & 138647 & 29 & 432$\pm^{ 24 }_{ 23 }$ & $1.00$ & 26.7127 & $ 9.18\pm^{ 1.07E+03 }_{ 8.55 }$ & $ 16.24\pm^{ 0.21 }_{ 0.62 }$ & 2.02\\ 
pks0405 & $0.49505$ (\#262)  & 96.58(89) & 136537 & 33 & 137118 & 41 & 387$\pm^{ 26 }_{ 25 }$ & $1.00$ & 28.3461 & $ -1.97\pm^{ 0.74 }_{ 0.52 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.59\\ 
pks0405 & $0.49530$ (\#263)  & 97.66(89) & 136537 & 33 & 137118 & 41 & 389$\pm^{ 27 }_{ 26 }$ & $1.00$ & 28.3509 & $ -1.86\pm^{ 0.92 }_{ 0.64 }$ & $ nan\pm^{ nan }_{ nan }$ & 3.23\\ 
pks0405 & $0.55506$ (\#264)  & 98.30(94) & 138708 & 47 & 138714 & 45 & 363$\pm^{ 31 }_{ 30 }$ & $1.00$ & 29.4839 & $ -0.91\pm^{ 2.72 }_{ 1.13 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.30\\ 
pks2005 & $0.06490$ (\#265)  & 60.15(62) & 54472 & 6 & 54641 & 7 & 1896$\pm^{ 53 }_{ 53 }$ & $1.00$ & 20.1905 & $ -1.05\pm^{ 0.79 }_{ 0.54 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.94\\ 
pks2155 & $0.05405$ (\#266)  & 83.01(59) & 1701313 & 3 & 1685268 & 3 & 4444$\pm^{ 444 }_{ 409 }$ & $1.55$ & 19.9848 & $ 0.00\pm^{ 0.13 }_{ 0.11 }$ & $ 13.43\pm^{ 1.59 }_{ nan }$ & 0.01\\
pks2155 & $0.05707$ (\#267)  & 76.79(59) & 1701521 & 3 & 1685268 & 3 & 4316$\pm^{ 448 }_{ 438 }$ & $1.62$ & 20.0420 & $ 0.25\pm^{ 0.26 }_{ 0.08 }$ & $ 15.27\pm^{ 0.28 }_{ 0.14 }$ & 7.35\\
q0045 & $0.11052$ (\#268)  & -- & -- & -- & -- & -- & -- & -- & 21.0555 & -- & -- & --\\ 
q0045 & $0.13521$ (\#269)  & -- & -- & -- & -- & -- & -- & -- & 21.5236 & -- & -- & --\\ 
q1230 & $0.09518$ (\#270)  & 44.14(33) & 39329 & 61 & nan & nan & 48$\pm^{ 19 }_{ 18 }$ & $1.00$ & 20.7646 & $ -5.80\pm^{ 1.00E+20 }_{ 2.21 }$ & $ nan\pm^{ nan }_{ nan }$ & 1.10\\ 
q1230 & $0.10318$ (\#271)  & 48.14(34) & 39330 & 67 & nan & nan & 56$\pm^{ 17 }_{ 15 }$ & $1.00$ & 20.9163 & $ -2.54\pm^{ 76.95 }_{ 1.48 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.59\\ 
q1230 & $0.10445$ (\#272)  & 48.96(34) & 39330 & 69 & nan & nan & 66$\pm^{ 18 }_{ 14 }$ & $1.00$ & 20.9404 & $ 510.19\pm^{ 1.00E+20 }_{ 540.19 }$ & $ 16.45\pm^{ 0.30 }_{ nan }$ & 0.28\\ 
q1230 & $0.10530$ (\#273)  & 49.30(34) & 39331 & 72 & nan & nan & 68$\pm^{ 17 }_{ 15 }$ & $1.00$ & 20.9565 & $ 1.86E+07\pm^{ 1.00E+20 }_{ 1.86E+07 }$ & $ 16.62\pm^{ 0.17 }_{ nan }$ & 0.84\\ 
q1230 & $0.10596$ (\#274)  & 46.27(33) & 39331 & 70 & nan & nan & 70$\pm^{ 17 }_{ 15 }$ & $1.00$ & 20.9690 & $ 2.20E+06\pm^{ 1.00E+20 }_{ 2.20E+06 }$ & $ 16.62\pm^{ 0.12 }_{ nan }$ & 1.07\\ 
q1230 & $0.10666$ (\#275)  & 46.39(34) & 39331 & 72 & nan & nan & 65$\pm^{ 21 }_{ 15 }$ & $1.00$ & 20.9823 & $ 1.92E+04\pm^{ 1.00E+20 }_{ 1.93E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 0.96\\ 
q1230 & $0.10809$ (\#276)  & 45.09(33) & 39331 & 83 & nan & nan & 53$\pm^{ 20 }_{ 14 }$ & $1.00$ & 21.0094 & $ 7.62E+08\pm^{ 1.00E+20 }_{ 7.62E+08 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.29\\ 
q1230 & $0.10820$ (\#277)  & 45.09(33) & 39331 & 83 & nan & nan & 53$\pm^{ 20 }_{ 14 }$ & $1.00$ & 21.0115 & $ 2.11E+09\pm^{ 1.00E+20 }_{ 2.11E+09 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.29\\ 
q1230 & $0.10861$ (\#278)  & 48.14(33) & 39331 & 85 & nan & nan & 52$\pm^{ 20 }_{ 14 }$ & $1.00$ & 21.0192 & $ 1.52E+04\pm^{ 1.00E+20 }_{ 1.53E+04 }$ & $ 16.54\pm^{ 0.23 }_{ nan }$ & 1.02\\ 
q1230 & $0.10906$ (\#279)  & 44.60(32) & 39332 & 82 & nan & nan & 53$\pm^{ 25 }_{ 15 }$ & $1.00$ & 21.0278 & $ 3.02E+04\pm^{ 1.00E+20 }_{ 3.02E+04 }$ & $ 16.54\pm^{ 0.26 }_{ nan }$ & 1.08\\ 
q1230 & $0.10935$ (\#280)  & 44.06(32) & 39332 & 82 & nan & nan & 55$\pm^{ 17 }_{ 14 }$ & $1.00$ & 21.0333 & $ 3.16E+11\pm^{ 1.00E+20 }_{ 3.16E+11 }$ & $ 16.75\pm^{ 0.00 }_{ inf }$ & 1.71\\ 
q1230 & $0.10956$ (\#281)  & 43.57(32) & 39332 & 82 & nan & nan & 56$\pm^{ 21 }_{ 15 }$ & $1.00$ & 21.0373 & $ 5.49E+08\pm^{ 1.00E+20 }_{ 5.49E+08 }$ & $ 16.69\pm^{ 0.11 }_{ inf }$ & 1.56\\ 
q1230 & $0.11707$ (\#282)  & 39.83(27) & 39333 & 64 & nan & nan & 51$\pm^{ 20 }_{ 17 }$ & $1.00$ & 21.1796 & $ -5.35\pm^{ 1.11 }_{ 1.02 }$ & $ nan\pm^{ nan }_{ nan }$ & 13.29\\ 
q1230 & $0.11743$ (\#283)  & 34.85(25) & 39333 & 60 & nan & nan & 57$\pm^{ 22 }_{ 19 }$ & $1.00$ & 21.1865 & $ -4.41\pm^{ 0.92 }_{ 0.82 }$ & $ nan\pm^{ nan }_{ nan }$ & 11.53\\ 
q1230 & $0.11781$ (\#284)  & 35.43(25) & 39333 & 60 & nan & nan & 59$\pm^{ 22 }_{ 19 }$ & $1.00$ & 21.1937 & $ -4.31\pm^{ 0.95 }_{ 0.82 }$ & $ nan\pm^{ nan }_{ nan }$ & 10.59\\ 
rbs1892 & $0.15752$ (\#285)  & -- & -- & -- & -- & -- & -- & -- & 21.9466 & -- & -- & --\\ 
rbs1892 & $0.17133$ (\#286)  & 46.32(37) & 4929 & 14 & nan & nan & 312$\pm^{ 101 }_{ 76 }$ & $1.00$ & 22.2084 & $ 2.84E+04\pm^{ 1.00E+20 }_{ 2.85E+04 }$ & $ 16.54\pm^{ 0.25 }_{ nan }$ & 0.45\\ 
rbs1892 & $0.19874$ (\#287)  & 50.02(44) & 4929 & 24 & nan & nan & 332$\pm^{ 100 }_{ 76 }$ & $1.00$ & 22.7281 & $ 65.39\pm^{ 1.00E+20 }_{ 95.39 }$ & $ 16.35\pm^{ 0.45 }_{ nan }$ & 0.16\\ 
rbs542 & $0.10323$ (\#288)  & 48.13(48) & 192804 & 9 & nan & nan & 1054$\pm^{ 22 }_{ 22 }$ & $1.00$ & 20.9172 & $ -0.64\pm^{ 0.80 }_{ 0.54 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.84\\ 
rbs542 & $0.10379$ (\#289)  & 48.09(47) & 192375 & 9 & nan & nan & 1053$\pm^{ 22 }_{ 22 }$ & $1.00$ & 20.9279 & $ -0.52\pm^{ 0.87 }_{ 0.57 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.52\\ 
rxj0439 & $0.11547$ (\#290)  & 38.76(35) & 151442 & 17 & nan & nan & 337$\pm^{ 18 }_{ 18 }$ & $1.00$ & 21.1493 & $ -1.84\pm^{ 0.78 }_{ 0.54 }$ & $ nan\pm^{ nan }_{ nan }$ & 4.30\\ 
rxj0439 & $0.21833$ (\#291)  & 61.09(43) & 145661 & 21 & nan & nan & 419$\pm^{ 22 }_{ 22 }$ & $1.00$ & 23.0995 & $ -2.54\pm^{ 0.83 }_{ 0.62 }$ & $ nan\pm^{ nan }_{ nan }$ & 5.79\\ 
rxj0439 & $0.24235$ (\#292)  & 63.87(47) & 151874 & 19 & 121198 & 15 & 498$\pm^{ 26 }_{ 21 }$ & $1.00$ & 23.5550 & $ 14.62\pm^{ 7.81E+03 }_{ 13.54 }$ & $ 16.28\pm^{ 0.24 }_{ 0.47 }$ & 2.82\\ 
rxj0439 & $0.24258$ (\#293)  & 69.70(49) & 151906 & 19 & 131963 & 21 & 497$\pm^{ 21 }_{ 21 }$ & $1.00$ & 23.5593 & $ 30.90\pm^{ 1.70E+04 }_{ 29.84 }$ & $ 16.31\pm^{ 0.20 }_{ 0.50 }$ & 2.55\\ 
rxj0439 & $0.24313$ (\#294)  & 66.17(48) & 151874 & 18 & 131963 & 22 & 498$\pm^{ 23 }_{ 22 }$ & $1.00$ & 23.5697 & $ 6.96\pm^{ 184.85 }_{ 6.96 }$ & $ 16.18\pm^{ 0.25 }_{ 2.79 }$ & 1.44\\ 
rxj0439 & $0.24387$ (\#295)  & 71.95(50) & 151906 & 18 & 137345 & 21 & 497$\pm^{ 22 }_{ 21 }$ & $1.00$ & 23.5838 & $ 1.28\pm^{ 13.88 }_{ 1.95 }$ & $ 15.85\pm^{ 0.44 }_{ nan }$ & 0.33\\ 
s50716 & $0.23145$ (\#296)  & 57.72(42) & 75697 & 12 & nan & nan & 741$\pm^{ 36 }_{ 35 }$ & $1.00$ & 23.3483 & $ 2.00\pm^{ 3.46E+04 }_{ 3.48 }$ & $ 15.98\pm^{ 0.52 }_{ nan }$ & 0.15\\ 
ton28 & $0.13746$ (\#297)  & -- & -- & -- & -- & -- & -- & -- & 21.5662 & -- & -- & --\\ 
ton28 & $0.13773$ (\#298)  & -- & -- & -- & -- & -- & -- & -- & 21.5714 & -- & -- & --\\ 
ton28 & $0.13781$ (\#299)  & -- & -- & -- & -- & -- & -- & -- & 21.5729 & -- & -- & --\\ 
ton28 & $0.17251$ (\#300)  & 50.74(37) & 81682 & 38 & nan & nan & 131$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.2308 & $ -1.79\pm^{ 3.97 }_{ 1.28 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.60\\ 
ton28 & $0.21259$ (\#301)  & 60.47(42) & 81454 & 35 & nan & nan & 188$\pm^{ 20 }_{ 19 }$ & $1.00$ & 22.9907 & $ 0.13\pm^{ 3.65E+04 }_{ 2.45 }$ & $ 15.01\pm^{ 1.52 }_{ nan }$ & 0.00\\ 
ton28 & $0.24292$ (\#302)  & 30.56(48) & 85563 & 34 & 83705 & 38 & 186$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.5658 & $ 3.06\pm^{ 1.41E+07 }_{ 33.06 }$ & $ 16.07\pm^{ 0.53 }_{ nan }$ & 0.18\\ 
ton28 & $0.24859$ (\#303)  & 52.11(52) & 84503 & 35 & 85711 & 26 & 180$\pm^{ 20 }_{ 19 }$ & $1.00$ & 23.6733 & $ -1.55\pm^{ 5.49 }_{ 1.32 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.42\\ 
ton28 & $0.27338$ (\#304)  & 80.27(77) & 85129 & 37 & 86614 & 30 & 205$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.1433 & $ -1.67\pm^{ 2.16 }_{ 1.04 }$ & $ nan\pm^{ nan }_{ nan }$ & 0.97\\ 
ton28 & $0.33021$ (\#305)  & 107.71(94) & 85874 & 26 & 86028 & 38 & 199$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.2208 & $ -2.21\pm^{ 1.51 }_{ 0.90 }$ & $ nan\pm^{ nan }_{ nan }$ & 2.04\\ 
tons180 & $0.02340$ (\#306)  & 99.08(96) & 177396 & 6 & 194071 & 7 & 901$\pm^{ 18 }_{ 18 }$ & $1.00$ & 19.4037 & $ -0.01\pm^{ 0.89 }_{ 0.46 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.00\\ 
tons180 & $0.04360$ (\#307)  & 69.00(82) & 187350 & 6 & 195496 & 7 & 955$\pm^{ 18 }_{ 18 }$ & $1.00$ & 19.7867 & $ -0.03\pm^{ 0.88 }_{ 0.48 }$ & $ nan\pm^{ nan }_{ nan }$ & -0.01\\ 
tons180 & $0.04560$ (\#308)  & 67.80(80) & 187350 & 6 & 195974 & 7 & 963$\pm^{ 19 }_{ 19 }$ & $1.00$ & 19.8246 & $ 0.49\pm^{ 1.01 }_{ 0.68 }$ & $ 15.54\pm^{ 0.38 }_{ nan }$ & 0.60\\



\hline
\hline
 \end{longtable}
 \end{landscape}

==> Tables/XMM/Latex/xmm_o8_o6_uppers_full.tex <==
\renewcommand{\arraystretch}{.7}
\setlength\LTleft{-.25cm}

%\fontsize{9}{11}
\setlength{\tabcolsep}{3pt}
%\begin{small}
\scriptsize
\begin{landscape}
\begin{longtable}{cc|llllllll|l}
\caption[\xmm\ Data, \oviii\ Upper Limits With \ovi\ Priors Results (Full)]{\oviii\ upper limit measurements with \xmm\ data, at the prior redshift from the \ovi\ lines from Table~\ref{tab:oviPriorsTable}.}
\label{tab:xmmovioviiiuppers}\\
 \hline
 \hline
 \multicolumn{2}{c}{Target line} & cmin & RGS1 & \multicolumn{2}{c}{power--law} & \multicolumn{3}{c}{line component} & $\Delta C$\\
 Name & z & (d.o.f.)& avg exp (s) & \text{norm.} & \text{index} & $\lambda$ (\AA) & $\tau_0$ & $\log N + (\text{cm}^{-2})$ & (d.o.f.)\\
 \hline 
1es1028 & $0.12314$ (\#1)  & 33.31(31) & 146792 & nan & 963$\pm^{ 40 }_{ 26 }$ & $1.00$ & 21.2947 & 2.30 &  16.01 & 0.01\\ 
1es1028 & $0.13706$ (\#2)  & -- & -- & -- & -- & -- & 21.5587 & -- & -- & --\\ 
1es1028 & $0.33735$ (\#3)  & 92.62(96) & 147900 & 144798 & 1196$\pm^{ 31 }_{ 31 }$ & $1.00$ & 25.3562 & 9.35 &  16.25 & 6.58\\ 
1es1553 & $0.18759$ (\#4)  & 29.26(27) & 1729540 & nan & 540$\pm^{ 318 }_{ 194 }$ & $2.55$ & 22.5167 & 0.39 &  15.45 & 1.81\\ 
1es1553 & $0.18775$ (\#5)  & 28.91(27) & 1729540 & nan & 550$\pm^{ 295 }_{ 211 }$ & $2.52$ & 22.5197 & 0.40 &  15.46 & 2.20\\ 
1es1553 & $0.18984$ (\#6)  & 25.62(27) & 1729542 & nan & 406$\pm^{ 219 }_{ 140 }$ & $3.05$ & 22.5594 & 0.54 &  15.56 & 8.20\\ 
1es1553 & $0.21631$ (\#7)  & 33.20(25) & 1723969 & nan & 60$\pm^{ 36 }_{ 21 }$ & $6.19$ & 23.0612 & 0.36 &  15.42 & 0.03\\ 
1es1553 & $0.31130$ (\#8)  & 113.12(91) & 1744157 & 1748313 & 2268$\pm^{ 757 }_{ 440 }$ & $0.67$ & 24.8622 & 0.35 &  15.41 & 17.08\\ 
1es1553 & $0.37868$ (\#9)  & 113.07(88) & 1784762 & 1713272 & 1213$\pm^{ 467 }_{ 336 }$ & $1.52$ & 26.1398 & 0.40 &  15.45 & 15.34\\ 
1es1553 & $0.39497$ (\#10)  & 118.64(92) & 1704141 & 1756581 & 481$\pm^{ 192 }_{ 138 }$ & $2.74$ & 26.4486 & 0.19 &  15.15 & 1.31\\ 
3c249 & $0.24676$ (\#11)  & 41.19(50) & 2644 & 2524 & 373$\pm^{ 135 }_{ 107 }$ & $1.00$ & 23.6386 & 5.00E+19 &  16.80 & 0.10\\ 
3c249 & $0.30788$ (\#12)  & 70.28(91) & 2641 & 2524 & 269$\pm^{ 119 }_{ 90 }$ & $1.00$ & 24.7974 & 5.00E+19 &  16.75 & 0.05\\ 
3c249 & $0.30809$ (\#13)  & 70.31(91) & 2641 & 2524 & 271$\pm^{ 119 }_{ 91 }$ & $1.00$ & 24.8014 & 1.55E+14 &  16.78 & 0.02\\ 
3c249 & $0.31364$ (\#14)  & 73.37(90) & 2640 & 2524 & 377$\pm^{ 139 }_{ 111 }$ & $1.00$ & 24.9066 & 5.00E+19 &  16.80 & 1.07\\ 
3c273 & $0.00337$ (\#15)  & 122.62(82) & 1002935 & 1016589 & 2162$\pm^{ 179 }_{ 168 }$ & $2.23$ & 19.0239 & 0.32 &  15.37 & -0.27\\ 
3c273 & $0.00533$ (\#16)  & 121.19(82) & 1000681 & 1016019 & 2034$\pm^{ 174 }_{ 166 }$ & $2.37$ & 19.0611 & 0.14 &  15.02 & -0.06\\ 
3c273 & $0.00764$ (\#17)  & 119.15(82) & 1000362 & 1015449 & 1895$\pm^{ 175 }_{ 164 }$ & $2.53$ & 19.1049 & 0.14 &  15.03 & 0.70\\ 
3c273 & $0.02947$ (\#18)  & 124.26(90) & 979671 & 1010400 & 2182$\pm^{ 194 }_{ 180 }$ & $2.22$ & 19.5188 & 0.15 &  15.06 & 0.00\\ 
3c273 & $0.04898$ (\#19)  & 97.81(72) & 981682 & 1017674 & 2995$\pm^{ 379 }_{ 339 }$ & $1.54$ & 19.8887 & 0.17 &  15.12 & 0.19\\ 
3c273 & $0.06655$ (\#20)  & 70.47(59) & 1020346 & 1015505 & 3584$\pm^{ 502 }_{ 559 }$ & $1.18$ & 20.2218 & 0.26 &  15.28 & -0.58\\ 
3c273 & $0.09018$ (\#21)  & 39.08(47) & 949280 & nan & 2360$\pm^{ 380 }_{ 338 }$ & $2.03$ & 20.6698 & 0.22 &  15.23 & 1.16\\ 
3c273 & $0.12007$ (\#22)  & 29.12(34) & 930918 & nan & 2926$\pm^{ 1141 }_{ 776 }$ & $1.62$ & 21.2365 & 0.22 &  15.21 & -0.04\\ 
3c273 & $0.14660$ (\#23)  & -- & -- & -- & -- & -- & 21.7395 & -- & -- & --\\ 
3c273 & $0.15784$ (\#24)  & 34.61(25) & 1047179 & nan & 2310$\pm^{ 773 }_{ 593 }$ & $2.01$ & 21.9526 & 0.16 &  15.08 & 12.16\\ 
h1821 & $0.02438$ (\#25)  & 127.18(98) & 30082 & 44303 & 1073$\pm^{ 56 }_{ 55 }$ & $1.00$ & 19.4222 & 1.28 &  15.85 & 0.18\\ 
h1821 & $0.10817$ (\#26)  & 50.54(39) & 33073 & nan & 1206$\pm^{ 79 }_{ 77 }$ & $1.00$ & 21.0109 & 3.07 &  16.07 & 0.13\\ 
h1821 & $0.12133$ (\#27)  & 38.85(28) & 33486 & nan & 1220$\pm^{ 99 }_{ 97 }$ & $1.00$ & 21.2604 & 166.48 &  16.36 & 0.08\\ 
h1821 & $0.12147$ (\#28)  & 38.90(28) & 33486 & nan & 1214$\pm^{ 99 }_{ 97 }$ & $1.00$ & 21.2631 & 33.18 &  16.30 & 0.01\\ 
h1821 & $0.16992$ (\#29)  & 47.55(34) & 32399 & nan & 970$\pm^{ 94 }_{ 91 }$ & $1.00$ & 22.1817 & 4.22E+06 &  16.56 & 0.00\\ 
h1821 & $0.17043$ (\#30)  & 47.37(34) & 32399 & nan & 986$\pm^{ 100 }_{ 91 }$ & $1.00$ & 22.1914 & 3.40E+13 &  16.74 & 0.23\\ 
h1821 & $0.21326$ (\#31)  & 58.03(45) & 29109 & nan & 975$\pm^{ 94 }_{ 92 }$ & $1.00$ & 23.0034 & 2.25 &  16.01 & 0.60\\ 
h1821 & $0.22497$ (\#32)  & 67.04(48) & 29437 & nan & 945$\pm^{ 94 }_{ 91 }$ & $1.00$ & 23.2254 & 1.09 &  15.81 & 1.95\\ 
h1821 & $0.22522$ (\#33)  & 66.78(47) & 29837 & nan & 962$\pm^{ 94 }_{ 90 }$ & $1.00$ & 23.2302 & 1.32 &  15.88 & 1.57\\ 
h1821 & $0.22639$ (\#34)  & 68.85(47) & 29881 & nan & 947$\pm^{ 93 }_{ 89 }$ & $1.00$ & 23.2524 & 1.36 &  15.87 & 1.14\\ 
h1821 & $0.24531$ (\#35)  & 72.51(51) & 31382 & 32028 & 1052$\pm^{ 92 }_{ 86 }$ & $1.00$ & 23.6111 & 3.28E+07 &  16.64 & 0.31\\ 
h1821 & $0.26657$ (\#36)  & 79.55(72) & 31337 & 42756 & 1040$\pm^{ 83 }_{ 81 }$ & $1.00$ & 24.0142 & 1.09 &  15.82 & 1.71\\ 
h1821 & $0.28800$ (\#37)  & 114.20(93) & 27766 & 42046 & 1294$\pm^{ 95 }_{ 91 }$ & $1.00$ & 24.4205 & 50.06 &  16.34 & 0.65\\ 
h1821 & $0.29658$ (\#38)  & 111.33(97) & 27950 & 42972 & 1276$\pm^{ 93 }_{ 91 }$ & $1.00$ & 24.5832 & 0.93 &  15.76 & 1.58\\ 
h1821 & $0.29680$ (\#39)  & 112.27(97) & 27836 & 43008 & 1282$\pm^{ 94 }_{ 91 }$ & $1.00$ & 24.5873 & 1.03 &  15.80 & 1.00\\ 
h2356 & $0.11461$ (\#40)  & 57.52(40) & 476224 & nan & 1072$\pm^{ 17 }_{ 14 }$ & $1.00$ & 21.1330 & 1.17 &  15.84 & 0.03\\ 
h2356 & $0.16512$ (\#41)  & 37.80(32) & 505443 & nan & 1093$\pm^{ 17 }_{ 20 }$ & $1.00$ & 22.0907 & 0.62 &  15.62 & 0.02\\ 
he0056 & $0.16392$ (\#42)  & 27.81(24) & 160091 & nan & 356$\pm^{ 24 }_{ 22 }$ & $1.00$ & 22.0679 & 2.86E+04 &  16.51 & 2.53\\ 
he0056 & $0.16492$ (\#43)  & 28.43(24) & 160091 & nan & 353$\pm^{ 25 }_{ 21 }$ & $1.00$ & 22.0869 & 5.33E+03 &  16.48 & 1.64\\ 
he0226 & $0.01746$ (\#44)  & 124.17(84) & 31711 & 31707 & 157$\pm^{ 20 }_{ 19 }$ & $1.00$ & 19.2910 & 1.85 &  15.97 & 0.93\\ 
he0226 & $0.02679$ (\#45)  & 131.34(93) & 31711 & 31707 & 154$\pm^{ 20 }_{ 18 }$ & $1.00$ & 19.4679 & 290.81 &  16.39 & 0.01\\ 
he0226 & $0.04121$ (\#46)  & 120.74(81) & 31711 & 31707 & 166$\pm^{ 22 }_{ 20 }$ & $1.00$ & 19.7413 & 2.71 &  16.06 & 0.53\\ 
he0226 & $0.04535$ (\#47)  & 113.12(77) & 31711 & 31707 & 161$\pm^{ 22 }_{ 20 }$ & $1.00$ & 19.8198 & 4.95 &  16.16 & 0.29\\ 
he0226 & $0.04609$ (\#48)  & 112.96(76) & 31711 & 31707 & 164$\pm^{ 22 }_{ 20 }$ & $1.00$ & 19.8339 & 55.75 &  16.35 & 0.04\\ 
he0226 & $0.06015$ (\#49)  & 84.08(65) & 31711 & 31707 & 121$\pm^{ 22 }_{ 20 }$ & $1.00$ & 20.1004 & 0.87 &  15.74 & 8.15\\ 
he0226 & $0.06083$ (\#50)  & 83.15(64) & 31711 & 31707 & 129$\pm^{ 22 }_{ 20 }$ & $1.00$ & 20.1133 & 0.88 &  15.73 & 5.31\\ 
he0226 & $0.07023$ (\#51)  & 66.31(54) & 31711 & 31707 & 170$\pm^{ 24 }_{ 23 }$ & $1.00$ & 20.2916 & 7.86E+07 &  16.65 & 0.01\\ 
he0226 & $0.08375$ (\#52)  & 52.16(42) & 31711 & nan & 196$\pm^{ 28 }_{ 23 }$ & $1.00$ & 20.5479 & 5.00E+19 &  16.80 & 2.53\\ 
he0226 & $0.08901$ (\#53)  & 47.97(42) & 31711 & nan & 183$\pm^{ 25 }_{ 23 }$ & $1.00$ & 20.6476 & 1.76 &  15.95 & 1.23\\ 
he0226 & $0.08938$ (\#54)  & 47.78(42) & 31711 & nan & 182$\pm^{ 25 }_{ 23 }$ & $1.00$ & 20.6546 & 1.73 &  15.96 & 1.47\\ 
he0226 & $0.08950$ (\#55)  & 46.05(43) & 31711 & nan & 182$\pm^{ 25 }_{ 23 }$ & $1.00$ & 20.6569 & 1.54 &  15.92 & 1.57\\ 
he0226 & $0.09220$ (\#56)  & 46.95(42) & 31711 & nan & 186$\pm^{ 25 }_{ 23 }$ & $1.00$ & 20.7081 & 2.15 &  16.00 & 0.92\\ 
he0226 & $0.10668$ (\#57)  & 50.29(43) & 31711 & nan & 175$\pm^{ 26 }_{ 24 }$ & $1.00$ & 20.9827 & 1.23 &  15.84 & 2.23\\ 
he0226 & $0.11514$ (\#58)  & 39.66(36) & 31711 & nan & 203$\pm^{ 30 }_{ 27 }$ & $1.00$ & 21.1431 & 2.60E+09 &  16.64 & 0.15\\ 
he0226 & $0.11680$ (\#59)  & 37.43(34) & 31711 & nan & 207$\pm^{ 37 }_{ 25 }$ & $1.00$ & 21.1745 & 5.00E+19 &  16.80 & 1.76\\ 
he0226 & $0.11733$ (\#60)  & 36.95(34) & 31711 & nan & 202$\pm^{ 39 }_{ 25 }$ & $1.00$ & 21.1846 & 5.00E+19 &  16.80 & 2.01\\ 
he0226 & $0.12589$ (\#61)  & 35.52(30) & 31712 & nan & 206$\pm^{ 36 }_{ 27 }$ & $1.00$ & 21.3469 & 5.00E+19 &  16.75 & 2.12\\ 
he0226 & $0.13832$ (\#62)  & -- & -- & -- & -- & -- & 21.5825 & -- & -- & --\\ 
he0226 & $0.15175$ (\#63)  & -- & -- & -- & -- & -- & 21.8372 & -- & -- & --\\ 
he0226 & $0.15549$ (\#64)  & -- & -- & -- & -- & -- & 21.9081 & -- & -- & --\\ 
he0226 & $0.16237$ (\#65)  & 33.50(25) & 31712 & nan & 113$\pm^{ 37 }_{ 33 }$ & $1.00$ & 22.0385 & 1.08 &  15.82 & 15.81\\ 
he0226 & $0.16339$ (\#66)  & 33.20(26) & 31712 & nan & 113$\pm^{ 36 }_{ 32 }$ & $1.00$ & 22.0579 & 1.02 &  15.80 & 16.22\\ 
he0226 & $0.16971$ (\#67)  & 40.73(28) & 31712 & nan & 140$\pm^{ 34 }_{ 30 }$ & $1.00$ & 22.1777 & 4.94E+04 &  16.52 & 0.43\\ 
he0226 & $0.18619$ (\#68)  & 50.47(36) & 31712 & nan & 175$\pm^{ 30 }_{ 27 }$ & $1.00$ & 22.4902 & 5.00E+19 &  16.75 & 1.41\\ 
he0226 & $0.18811$ (\#69)  & 48.87(35) & 31712 & nan & 219$\pm^{ 37 }_{ 30 }$ & $1.00$ & 22.5266 & 5.00E+19 &  16.75 & 1.73\\ 
he0226 & $0.18891$ (\#70)  & 57.62(39) & 31712 & nan & 196$\pm^{ 30 }_{ 28 }$ & $1.00$ & 22.5417 & 5.00E+19 &  16.80 & 2.21\\ 
he0226 & $0.19374$ (\#71)  & 46.89(38) & 31712 & nan & 168$\pm^{ 30 }_{ 28 }$ & $1.00$ & 22.6333 & 5.00E+19 &  16.80 & 2.44\\ 
he0226 & $0.19453$ (\#72)  & 48.32(38) & 31712 & nan & 157$\pm^{ 34 }_{ 26 }$ & $1.00$ & 22.6483 & 5.00E+19 &  16.75 & 0.67\\ 
he0226 & $0.19860$ (\#73)  & 51.59(40) & 31712 & nan & 161$\pm^{ 31 }_{ 28 }$ & $1.00$ & 22.7255 & 5.69E+12 &  16.70 & 0.00\\ 
he0226 & $0.20055$ (\#74)  & 50.95(40) & 31712 & nan & 166$\pm^{ 29 }_{ 27 }$ & $1.00$ & 22.7624 & 5.00E+19 &  16.80 & 0.43\\ 
he0226 & $0.20703$ (\#75)  & 53.97(42) & 31712 & nan & 158$\pm^{ 30 }_{ 27 }$ & $1.00$ & 22.8853 & 2.94E+08 &  16.64 & 0.01\\ 
he0226 & $0.22009$ (\#76)  & 36.18(41) & 31713 & nan & 188$\pm^{ 33 }_{ 30 }$ & $1.00$ & 23.1329 & 4.75E+12 &  16.71 & 0.00\\ 
he0226 & $0.22099$ (\#77)  & 39.39(41) & 31713 & nan & 197$\pm^{ 33 }_{ 30 }$ & $1.00$ & 23.1500 & 1.13E+07 &  16.60 & 0.03\\ 
he0226 & $0.23009$ (\#78)  & 42.36(43) & 31713 & nan & 209$\pm^{ 33 }_{ 28 }$ & $1.00$ & 23.3225 & 5.00E+19 &  16.80 & 1.39\\ 
he0226 & $0.23964$ (\#79)  & 46.29(45) & 31713 & nan & 171$\pm^{ 30 }_{ 27 }$ & $1.00$ & 23.5036 & 5.37E+07 &  16.62 & 0.01\\ 
he0226 & $0.24522$ (\#80)  & 46.47(48) & 31713 & 31705 & 152$\pm^{ 29 }_{ 27 }$ & $1.00$ & 23.6094 & 7.88 &  16.21 & 0.65\\ 
he0226 & $0.25099$ (\#81)  & 54.13(54) & 31713 & 31705 & 163$\pm^{ 30 }_{ 27 }$ & $1.00$ & 23.7188 & 4.10E+05 &  16.60 & 0.00\\ 
he0226 & $0.27155$ (\#82)  & 78.85(73) & 31713 & 31705 & 224$\pm^{ 30 }_{ 28 }$ & $1.00$ & 24.1086 & 5.00E+19 &  16.80 & 1.20\\ 
he0226 & $0.27956$ (\#83)  & 79.52(77) & 31713 & 31705 & 224$\pm^{ 32 }_{ 29 }$ & $1.00$ & 24.2605 & 2.83 &  16.07 & 0.59\\ 
he0226 & $0.28041$ (\#84)  & 78.68(77) & 31713 & 31705 & 234$\pm^{ 33 }_{ 30 }$ & $1.00$ & 24.2766 & 8.93 &  16.24 & 0.27\\ 
he0226 & $0.29134$ (\#85)  & 83.52(84) & 31711 & 31705 & 238$\pm^{ 35 }_{ 32 }$ & $1.00$ & 24.4838 & 1.85 &  15.97 & 1.00\\ 
he0226 & $0.29213$ (\#86)  & 86.12(85) & 31711 & 31705 & 240$\pm^{ 35 }_{ 32 }$ & $1.00$ & 24.4988 & 1.65 &  15.93 & 1.02\\ 
he0226 & $0.30939$ (\#87)  & 97.61(90) & 31709 & 31705 & 246$\pm^{ 33 }_{ 30 }$ & $1.00$ & 24.8260 & 9.52E+05 &  16.61 & 0.27\\ 
he0226 & $0.31833$ (\#88)  & 99.31(91) & 31708 & 31705 & 223$\pm^{ 33 }_{ 30 }$ & $1.00$ & 24.9955 & 4.21E+09 &  16.67 & 0.49\\ 
he0226 & $0.33965$ (\#89)  & 102.15(94) & 31706 & 31705 & 273$\pm^{ 39 }_{ 31 }$ & $1.00$ & 25.3998 & 1.16E+15 &  16.77 & 0.91\\ 
he0226 & $0.34036$ (\#90)  & 108.55(94) & 31706 & 31705 & 273$\pm^{ 40 }_{ 31 }$ & $1.00$ & 25.4132 & 5.00E+19 &  16.80 & 1.70\\ 
he0226 & $0.35493$ (\#91)  & 115.28(93) & 31706 & 31704 & 247$\pm^{ 33 }_{ 30 }$ & $1.00$ & 25.6895 & 1.39 &  15.88 & 1.51\\ 
he0226 & $0.35528$ (\#92)  & 116.14(94) & 31706 & 31704 & 242$\pm^{ 33 }_{ 30 }$ & $1.00$ & 25.6961 & 1.14 &  15.82 & 2.04\\ 
he0226 & $0.37281$ (\#93)  & 117.30(93) & 31706 & 31704 & 305$\pm^{ 42 }_{ 33 }$ & $1.00$ & 26.0285 & 9.19E+12 &  16.71 & 0.86\\ 
he0226 & $0.38420$ (\#94)  & 128.19(92) & 31706 & 31704 & 295$\pm^{ 38 }_{ 36 }$ & $1.00$ & 26.2444 & 5.00E+19 &  16.75 & 2.16\\ 
he0226 & $0.38636$ (\#95)  & 130.09(92) & 31706 & 31704 & 281$\pm^{ 36 }_{ 34 }$ & $1.00$ & 26.2854 & 7.27E+06 &  16.62 & 0.22\\ 
he0226 & $0.39642$ (\#96)  & 139.43(93) & 31706 & 31704 & 262$\pm^{ 37 }_{ 34 }$ & $1.00$ & 26.4761 & 3.22 &  16.09 & 0.35\\ 
he0226 & $0.39692$ (\#97*)  & 137.43(91) & 31706 & 31704 & 261$\pm^{ 37 }_{ 34 }$ & $1.00$ & 26.4856 & 2.52 &  16.05 & 0.52\\ 
he0226 & $0.39890$ (\#98)  & 135.24(93) & 31707 & 31704 & 270$\pm^{ 38 }_{ 35 }$ & $1.00$ & 26.5231 & 2.44 &  16.04 & 0.54\\ 
he0226 & $0.40034$ (\#99)  & 134.81(92) & 31707 & 31704 & 276$\pm^{ 38 }_{ 35 }$ & $1.00$ & 26.5504 & 32.58 &  16.30 & 0.05\\ 
he0226 & $0.40274$ (\#100)  & 137.73(93) & 31707 & 31704 & 295$\pm^{ 39 }_{ 36 }$ & $1.00$ & 26.5960 & 3.94E+08 &  16.62 & 0.26\\ 
he0226 & $0.49225$ (\#101)  & 110.65(88) & 31709 & 31712 & 363$\pm^{ 50 }_{ 46 }$ & $1.00$ & 28.2931 & 6.76E+04 &  16.53 & 0.00\\ 
he0226 & $0.49254$ (\#102)  & 110.33(88) & 31709 & 31712 & 359$\pm^{ 49 }_{ 46 }$ & $1.00$ & 28.2986 & 437.84 &  16.39 & 0.04\\ 
he0226 & $0.49280$ (\#103)  & 110.26(88) & 31709 & 31712 & 357$\pm^{ 50 }_{ 46 }$ & $1.00$ & 28.3035 & 28.12 &  16.29 & 0.12\\ 
he0226 & $0.49309$ (\#104)  & 109.11(87) & 31709 & 31713 & 348$\pm^{ 49 }_{ 46 }$ & $1.00$ & 28.3090 & 5.73 &  16.18 & 0.27\\ 
i22456 & $0.09858$ (\#105)  & 56.99(44) & 79900 & nan & 498$\pm^{ 28 }_{ 27 }$ & $1.00$ & 20.8291 & 5.00E+19 &  16.75 & 4.29\\ 
i22456 & $0.09895$ (\#106)  & 60.07(44) & 79900 & nan & 499$\pm^{ 44 }_{ 27 }$ & $1.00$ & 20.8361 & 5.00E+19 &  16.80 & 3.98\\ 
i22456 & $0.09931$ (\#107)  & 59.72(44) & 79900 & nan & 501$\pm^{ 44 }_{ 27 }$ & $1.00$ & 20.8429 & 5.00E+19 &  16.80 & 4.43\\ 
i22456 & $0.09959$ (\#108)  & 54.85(44) & 79898 & nan & 498$\pm^{ 28 }_{ 27 }$ & $1.00$ & 20.8482 & 5.00E+19 &  16.75 & 4.62\\ 
i22456 & $0.09989$ (\#109)  & 55.11(44) & 79898 & nan & 496$\pm^{ 38 }_{ 27 }$ & $1.00$ & 20.8539 & 5.00E+19 &  16.78 & 4.24\\ 
i22456 & $0.10034$ (\#110)  & 55.73(44) & 79898 & nan & 500$\pm^{ 28 }_{ 27 }$ & $1.00$ & 20.8624 & 5.00E+19 &  16.80 & 4.33\\ 
i22456 & $0.10101$ (\#111)  & 55.60(44) & 79897 & nan & 495$\pm^{ 38 }_{ 27 }$ & $1.00$ & 20.8751 & 5.00E+19 &  16.75 & 3.43\\ 
i22456 & $0.10146$ (\#112)  & 55.42(44) & 79897 & nan & 499$\pm^{ 28 }_{ 28 }$ & $1.00$ & 20.8837 & 1.86E+11 &  16.71 & 3.55\\ 
mr2251 & $0.01070$ (\#113)  & 126.25(97) & 415723 & 451165 & 1562$\pm^{ 16 }_{ 16 }$ & $1.00$ & 19.1629 & 0.20 &  15.19 & 9.49\\ 
mrk421 & $0.01009$ (\#114*)  & 95.39(57) & 1385032 & 1437210 & 27095$\pm^{ 56 }_{ 49 }$ & $1.00$ & 19.1513 & 0.06 &  14.70 & 9.73\\
mrk876 & $0.00311$ (\#115)  & 98.25(96) & 2693 & 2600 & 283$\pm^{ 87 }_{ 69 }$ & $1.00$ & 19.0190 & 5.00E+19 &  16.76 & 0.38\\ 
mrk876 & $0.06248$ (\#116)  & 59.48(66) & 2754 & 2708 & 362$\pm^{ 110 }_{ 83 }$ & $1.00$ & 20.1446 & 5.00E+19 &  16.76 & 1.48\\ 
mrk876 & $0.08579$ (\#117)  & 44.05(43) & 2804 & nan & 444$\pm^{ 126 }_{ 109 }$ & $1.00$ & 20.5866 & 1.80 &  15.95 & 1.79\\ 
mrk876 & $0.11488$ (\#118)  & 52.10(37) & 2790 & nan & 714$\pm^{ 157 }_{ 165 }$ & $1.00$ & 21.1381 & 5.00E+19 &  16.80 & 3.07\\ 
mrk876 & $0.11517$ (\#119)  & 52.51(37) & 2790 & nan & 706$\pm^{ 235 }_{ 159 }$ & $1.00$ & 21.1436 & 5.00E+19 &  16.75 & 2.62\\ 
mrk876 & $0.11588$ (\#120)  & 50.65(36) & 2788 & nan & 705$\pm^{ 157 }_{ 137 }$ & $1.00$ & 21.1571 & 5.00E+19 &  16.80 & 2.97\\ 
ngc7469 & $0.00962$ (\#121)  & 84.33(74) & 631131 & 664074 & 1941$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1424 & 0.77 &  15.70 & 45.84\\ 
ngc7469 & $0.00994$ (\#122)  & 94.79(74) & 630829 & 663435 & 1942$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1485 & 0.95 &  15.77 & 53.76\\ 
ngc7469 & $0.01153$ (\#123)  & 85.80(74) & 622605 & 665535 & 1939$\pm^{ 17 }_{ 17 }$ & $1.00$ & 19.1786 & 1.43 &  15.90 & 53.36\\ 
p1103 & $0.13556$ (\#124)  & -- & -- & -- & -- & -- & 21.5302 & -- & -- & --\\ 
p1103 & $0.13937$ (\#125)  & -- & -- & -- & -- & -- & 21.6025 & -- & -- & --\\ 
p1103 & $0.14099$ (\#126)  & -- & -- & -- & -- & -- & 21.6332 & -- & -- & --\\ 
p1103 & $0.14126$ (\#127)  & -- & -- & -- & -- & -- & 21.6383 & -- & -- & --\\ 
p1103 & $0.17277$ (\#128)  & 44.35(37) & 15674 & nan & 2927$\pm^{ 142 }_{ 138 }$ & $1.00$ & 22.2357 & 3.59E+11 &  16.69 & 6.11\\ 
pg0003 & $0.16521$ (\#129)  & 39.30(31) & 13036 & nan & 287$\pm^{ 72 }_{ 63 }$ & $1.00$ & 22.0924 & 1.49 &  15.91 & 2.77\\ 
pg0003 & $0.20907$ (\#130)  & 38.93(42) & 13036 & nan & 282$\pm^{ 58 }_{ 51 }$ & $1.00$ & 22.9240 & 5.00E+19 &  16.75 & 0.89\\ 
pg0003 & $0.29021$ (\#131)  & 98.06(84) & 13036 & 12941 & 230$\pm^{ 57 }_{ 49 }$ & $1.00$ & 24.4624 & 1.17 &  15.83 & 2.68\\ 
pg0003 & $0.30551$ (\#132)  & 110.03(89) & 13035 & 12941 & 297$\pm^{ 62 }_{ 55 }$ & $1.00$ & 24.7525 & 5.00E+19 &  16.80 & 1.06\\ 
pg0003 & $0.30569$ (\#133)  & 111.09(89) & 13035 & 12941 & 297$\pm^{ 71 }_{ 55 }$ & $1.00$ & 24.7559 & 5.00E+19 &  16.80 & 1.07\\ 
pg0003 & $0.34757$ (\#134)  & 112.83(95) & 13033 & 12938 & 306$\pm^{ 63 }_{ 54 }$ & $1.00$ & 25.5499 & 1.15E+13 &  16.72 & 0.09\\ 
pg0003 & $0.34788$ (\#135)  & 112.95(95) & 13033 & 12938 & 297$\pm^{ 60 }_{ 53 }$ & $1.00$ & 25.5558 & 1.40E+09 &  16.67 & 0.03\\ 
pg0003 & $0.36452$ (\#136)  & 111.56(93) & 13033 & 12904 & 311$\pm^{ 62 }_{ 55 }$ & $1.00$ & 25.8713 & 4.91E+12 &  16.70 & 0.04\\ 
pg0003 & $0.36508$ (\#137)  & 109.85(94) & 13033 & 12903 & 308$\pm^{ 63 }_{ 55 }$ & $1.00$ & 25.8819 & 1.50E+07 &  16.61 & 0.01\\ 
pg0003 & $0.36572$ (\#138)  & 108.78(93) & 13033 & 12902 & 322$\pm^{ 64 }_{ 56 }$ & $1.00$ & 25.8941 & 2.59E+05 &  16.58 & 0.03\\ 
pg0003 & $0.36621$ (\#139)  & 111.21(94) & 13033 & 12901 & 311$\pm^{ 62 }_{ 55 }$ & $1.00$ & 25.9033 & 2.85E+04 &  16.50 & 0.08\\ 
pg0003 & $0.37029$ (\#140)  & 111.68(94) & 13033 & 12891 & 338$\pm^{ 67 }_{ 60 }$ & $1.00$ & 25.9807 & 5.00E+19 &  16.80 & 0.59\\ 
pg0003 & $0.38608$ (\#141)  & 106.87(92) & 13033 & 12857 & 250$\pm^{ 69 }_{ 51 }$ & $1.00$ & 26.2801 & 5.00E+19 &  16.80 & 1.56\\ 
pg0003 & $0.38639$ (\#142)  & 106.91(93) & 13033 & 12857 & 237$\pm^{ 59 }_{ 49 }$ & $1.00$ & 26.2860 & 5.00E+19 &  16.80 & 1.19\\ 
pg0003 & $0.40138$ (\#143)  & 126.94(94) & 13034 & 12830 & 339$\pm^{ 76 }_{ 60 }$ & $1.00$ & 26.5702 & 5.00E+19 &  16.80 & 1.59\\ 
pg0003 & $0.42192$ (\#144)  & 130.53(94) & 13034 & 12830 & 305$\pm^{ 79 }_{ 64 }$ & $1.00$ & 26.9596 & 7.39E+13 &  16.75 & 0.25\\ 
pg0157 & $0.14621$ (\#145)  & -- & -- & -- & -- & -- & 21.7321 & -- & -- & --\\ 
pg0804 & $0.00382$ (\#146)  & 96.91(99) & 28317 & 30000 & 1025$\pm^{ 49 }_{ 47 }$ & $1.00$ & 19.0324 & 0.89 &  15.75 & 1.42\\ 
pg0804 & $0.01851$ (\#147)  & 98.66(99) & 27987 & 30600 & 1068$\pm^{ 52 }_{ 50 }$ & $1.00$ & 19.3109 & 4.80 &  16.15 & 0.46\\ 
pg0804 & $0.10216$ (\#148)  & 59.36(43) & 28660 & nan & 1091$\pm^{ 61 }_{ 59 }$ & $1.00$ & 20.8970 & 5.58 &  16.17 & 0.02\\ 
pg0804 & $0.10230$ (\#149)  & 59.37(43) & 28660 & nan & 1094$\pm^{ 61 }_{ 59 }$ & $1.00$ & 20.8996 & 6.47 &  16.20 & 0.00\\ 
pg0832 & $0.10772$ (\#150)  & 51.86(42) & 20653 & nan & 49$\pm^{ 17 }_{ 14 }$ & $1.00$ & 21.0024 & 5.00E+19 &  16.80 & 0.18\\ 
pg0832 & $0.13230$ (\#151)  & 33.25(28) & 20654 & nan & 37$\pm^{ 21 }_{ 16 }$ & $1.00$ & 21.4684 & 1.24E+04 &  16.49 & 0.59\\ 
pg0832 & $0.15276$ (\#152)  & -- & -- & -- & -- & -- & 21.8563 & -- & -- & --\\ 
pg0832 & $0.23308$ (\#153)  & 50.44(43) & 20655 & nan & 60$\pm^{ 24 }_{ 18 }$ & $1.00$ & 23.3792 & 5.00E+19 &  16.80 & 0.38\\ 
pg0832 & $0.32567$ (\#154)  & 127.93(90) & 20654 & 20637 & 49$\pm^{ 24 }_{ 16 }$ & $1.00$ & 25.1347 & 5.00E+19 &  16.80 & 0.65\\ 
pg0953 & $0.01560$ (\#155)  & 111.24(90) & 12824 & 12310 & 312$\pm^{ 42 }_{ 39 }$ & $1.00$ & 19.2558 & 2.01 &  15.98 & 0.65\\ 
pg0953 & $0.05891$ (\#156)  & 84.64(66) & 12824 & 12310 & 428$\pm^{ 49 }_{ 46 }$ & $1.00$ & 20.0769 & 6.83E+14 &  16.78 & 0.71\\ 
pg0953 & $0.06807$ (\#157)  & 69.63(58) & 12824 & 12310 & 398$\pm^{ 52 }_{ 49 }$ & $1.00$ & 20.2506 & 1.93 &  15.98 & 1.18\\ 
pg0953 & $0.11827$ (\#158)  & 36.08(32) & 12794 & nan & 444$\pm^{ 71 }_{ 65 }$ & $1.00$ & 21.2024 & 5.82E+03 &  16.51 & 0.04\\ 
pg0953 & $0.14236$ (\#159)  & -- & -- & -- & -- & -- & 21.6591 & -- & -- & --\\ 
pg0953 & $0.14263$ (\#160)  & -- & -- & -- & -- & -- & 21.6643 & -- & -- & --\\ 
pg0953 & $0.14307$ (\#161)  & -- & -- & -- & -- & -- & 21.6726 & -- & -- & --\\ 
pg0953 & $0.22967$ (\#162)  & 53.43(43) & 12792 & nan & 475$\pm^{ 71 }_{ 65 }$ & $1.00$ & 23.3145 & 1.98 &  15.98 & 1.08\\ 
pg0953 & $0.23251$ (\#163)  & 49.94(43) & 12792 & nan & 472$\pm^{ 70 }_{ 65 }$ & $1.00$ & 23.3684 & 14.65 &  16.24 & 0.68\\ 
pg0953 & $0.23351$ (\#164)  & 51.78(43) & 12792 & nan & 480$\pm^{ 72 }_{ 67 }$ & $1.00$ & 23.3873 & 8.28 &  16.21 & 0.88\\ 
pg1115 & $0.12285$ (\#165)  & 41.88(32) & 17510 & nan & 304$\pm^{ 54 }_{ 42 }$ & $1.00$ & 21.2892 & 5.00E+19 &  16.80 & 1.56\\ 
pg1115 & $0.12313$ (\#166)  & 41.92(32) & 17510 & nan & 300$\pm^{ 57 }_{ 41 }$ & $1.00$ & 21.2945 & 5.00E+19 &  16.80 & 1.44\\ 
pg1115 & $0.13104$ (\#167*)  & 46.21(29) & 17510 & nan & 319$\pm^{ 61 }_{ 46 }$ & $1.00$ & 21.4445 & 5.00E+19 &  16.80 & 1.03\\ 
pg1115 & $0.15456$ (\#168)  & -- & -- & -- & -- & -- & 21.8905 & -- & -- & --\\ 
pg1115 & $0.15467$ (\#169)  & -- & -- & -- & -- & -- & 21.8925 & -- & -- & --\\ 
pg1116 & $0.05900$ (\#170)  & 85.18(69) & 285035 & 294383 & 469$\pm^{ 12 }_{ 12 }$ & $1.00$ & 20.0786 & 1.13 &  15.82 & 0.00\\ 
pg1116 & $0.05927$ (\#171)  & 85.16(69) & 285035 & 294383 & 470$\pm^{ 12 }_{ 12 }$ & $1.00$ & 20.0838 & 1.30 &  15.87 & 0.03\\ 
pg1116 & $0.11895$ (\#172)  & 37.22(33) & 285607 & nan & 509$\pm^{ 16 }_{ 16 }$ & $1.00$ & 21.2153 & 2.07 &  15.99 & 0.31\\ 
pg1116 & $0.13852$ (\#173)  & -- & -- & -- & -- & -- & 21.5863 & -- & -- & --\\ 
pg1116 & $0.16539$ (\#174)  & 36.23(32) & 288889 & nan & 549$\pm^{ 18 }_{ 18 }$ & $1.00$ & 22.0958 & 2.10 &  16.00 & 0.38\\ 
pg1116 & $0.16554$ (\#175)  & 36.14(32) & 288889 & nan & 549$\pm^{ 19 }_{ 18 }$ & $1.00$ & 22.0986 & 2.40 &  16.02 & 0.48\\ 
pg1116 & $0.16610$ (\#176)  & 37.64(33) & 289091 & nan & 548$\pm^{ 18 }_{ 18 }$ & $1.00$ & 22.1093 & 3.21 &  16.08 & 0.80\\ 
pg1116 & $0.16686$ (\#177)  & 39.71(33) & 289091 & nan & 545$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.1237 & 3.53 &  16.11 & 0.73\\ 
pg1116 & $0.17343$ (\#178)  & 50.92(38) & 289065 & nan & 531$\pm^{ 16 }_{ 16 }$ & $1.00$ & 22.2482 & 0.86 &  15.73 & 0.61\\ 
pg1211 & $0.00711$ (\#179)  & 130.66(97) & 709355 & 767876 & 488$\pm^{ 7 }_{ 7 }$ & $1.00$ & 19.0948 & 0.54 &  15.57 & 1.02\\ 
pg1211 & $0.05117$ (\#180)  & 79.82(69) & 726954 & 778637 & 541$\pm^{ 8 }_{ 8 }$ & $1.00$ & 19.9302 & 0.57 &  15.59 & 0.82\\ 
pg1211 & $0.06449$ (\#181)  & 80.33(55) & 776352 & 776215 & 557$\pm^{ 9 }_{ 9 }$ & $1.00$ & 20.1827 & 0.46 &  15.51 & 1.52\\ 
pg1211 & $0.06491$ (\#182)  & 77.87(55) & 776352 & 776215 & 560$\pm^{ 9 }_{ 9 }$ & $1.00$ & 20.1907 & 0.46 &  15.51 & 1.19\\ 
pg1216 & $0.12362$ (\#183)  & 42.81(30) & 11245 & nan & 225$\pm^{ 51 }_{ 44 }$ & $1.00$ & 21.3038 & 5.00E+19 &  16.80 & 1.17\\ 
pg1216 & $0.12389$ (\#184)  & 42.84(30) & 11245 & nan & 222$\pm^{ 50 }_{ 44 }$ & $1.00$ & 21.3090 & 5.00E+19 &  16.75 & 1.09\\ 
pg1216 & $0.12463$ (\#185)  & 43.15(30) & 11245 & nan & 218$\pm^{ 58 }_{ 44 }$ & $1.00$ & 21.3230 & 5.00E+19 &  16.80 & 0.72\\ 
pg1216 & $0.12485$ (\#186)  & 43.34(30) & 11245 & nan & 216$\pm^{ 58 }_{ 43 }$ & $1.00$ & 21.3272 & 5.00E+19 &  16.75 & 0.50\\ 
pg1216 & $0.13499$ (\#187)  & -- & -- & -- & -- & -- & 21.5194 & -- & -- & --\\ 
pg1216 & $0.26768$ (\#188)  & 88.48(70) & 11245 & 11258 & 157$\pm^{ 56 }_{ 41 }$ & $1.00$ & 24.0352 & 5.00E+19 &  16.80 & 3.23\\ 
pg1216 & $0.28199$ (\#189)  & 109.24(79) & 11245 & 11258 & 184$\pm^{ 46 }_{ 39 }$ & $1.00$ & 24.3065 & 5.00E+19 &  16.80 & 0.71\\ 
pg1216 & $0.28237$ (\#190)  & 109.62(79) & 11245 & 11258 & 184$\pm^{ 46 }_{ 39 }$ & $1.00$ & 24.3137 & 5.00E+19 &  16.80 & 0.31\\ 
pg1259 & $0.00220$ (\#191)  & 124.99(93) & 11480 & 11480 & 106$\pm^{ 26 }_{ 24 }$ & $1.00$ & 19.0017 & 5.00E+19 &  16.80 & 0.30\\ 
pg1259 & $0.00762$ (\#192)  & 122.32(92) & 11480 & 11480 & 112$\pm^{ 30 }_{ 24 }$ & $1.00$ & 19.1045 & 5.00E+19 &  16.75 & 1.94\\ 
pg1259 & $0.02217$ (\#193)  & 129.87(93) & 11480 & 11480 & 99$\pm^{ 27 }_{ 23 }$ & $1.00$ & 19.3803 & 99.18 &  16.39 & 0.24\\ 
pg1259 & $0.04606$ (\#194)  & 94.97(77) & 11479 & 11480 & 122$\pm^{ 32 }_{ 26 }$ & $1.00$ & 19.8333 & 5.00E+19 &  16.75 & 0.40\\ 
pg1259 & $0.04650$ (\#195)  & 92.99(76) & 11479 & 11480 & 123$\pm^{ 30 }_{ 26 }$ & $1.00$ & 19.8416 & 5.00E+19 &  16.79 & 0.84\\ 
pg1259 & $0.19576$ (\#196)  & 53.02(43) & 11485 & nan & 196$\pm^{ 49 }_{ 42 }$ & $1.00$ & 22.6716 & 5.00E+19 &  16.80 & 0.00\\ 
pg1259 & $0.21940$ (\#197)  & 47.70(41) & 11485 & nan & 141$\pm^{ 49 }_{ 41 }$ & $1.00$ & 23.1198 & 1.19 &  15.85 & 6.35\\ 
pg1259 & $0.21953$ (\#198)  & 47.70(41) & 11485 & nan & 141$\pm^{ 48 }_{ 41 }$ & $1.00$ & 23.1223 & 0.99 &  15.77 & 6.32\\ 
pg1259 & $0.22313$ (\#199)  & 51.02(41) & 11485 & nan & 179$\pm^{ 48 }_{ 41 }$ & $1.00$ & 23.1905 & 5.00E+19 &  16.80 & 0.27\\ 
pg1259 & $0.23284$ (\#200)  & 57.87(43) & 11485 & nan & 221$\pm^{ 53 }_{ 47 }$ & $1.00$ & 23.3746 & 5.00E+19 &  16.80 & 0.06\\ 
pg1259 & $0.23956$ (\#201)  & 64.61(45) & 11485 & nan & 204$\pm^{ 49 }_{ 45 }$ & $1.00$ & 23.5021 & 5.00E+19 &  16.80 & 0.07\\ 
pg1259 & $0.25973$ (\#202)  & 74.33(62) & 11485 & 11479 & 204$\pm^{ 59 }_{ 41 }$ & $1.00$ & 23.8845 & 5.00E+19 &  16.75 & 1.08\\
pg1259 & $0.31979$ (\#203)  & 106.65(91) & 11483 & 11479 & 148$\pm^{ 44 }_{ 36 }$ & $1.00$ & 25.0232 & 5.00E+19 &  16.80 & 0.00\\ 
pg1259 & $0.32472$ (\#204)  & 104.67(91) & 11483 & 11479 & 156$\pm^{ 49 }_{ 38 }$ & $1.00$ & 25.1167 & 5.00E+19 &  16.80 & 1.52\\ 
pg1307 & $0.14187$ (\#205)  & -- & -- & -- & -- & -- & 21.6499 & -- & -- & --\\ 
pg1307 & $0.14214$ (\#206)  & -- & -- & -- & -- & -- & 21.6550 & -- & -- & --\\ 
pg1309 & $0.17586$ (\#207)  & 38.46(33) & 27263 & nan & 69$\pm^{ 22 }_{ 21 }$ & $1.00$ & 22.2943 & 5.00E+19 &  16.80 & 0.00\\ 
pg1309 & $0.17745$ (\#208)  & 38.48(35) & 27263 & nan & 68$\pm^{ 23 }_{ 19 }$ & $1.00$ & 22.3245 & 5.00E+19 &  16.75 & 0.01\\ 
pg1309 & $0.17866$ (\#209)  & 39.78(36) & 27263 & nan & 66$\pm^{ 22 }_{ 19 }$ & $1.00$ & 22.3474 & 5.00E+19 &  16.80 & 0.01\\ 
pg1309 & $0.17930$ (\#210)  & 40.20(37) & 27263 & nan & 66$\pm^{ 22 }_{ 19 }$ & $1.00$ & 22.3595 & 5.00E+19 &  16.80 & 0.03\\ 
pg1309 & $0.17979$ (\#211)  & 40.62(37) & 27263 & nan & 65$\pm^{ 21 }_{ 18 }$ & $1.00$ & 22.3688 & 5.00E+19 &  16.80 & 0.03\\ 
pg1309 & $0.18069$ (\#212)  & 43.43(38) & 27263 & nan & 74$\pm^{ 22 }_{ 19 }$ & $1.00$ & 22.3859 & 5.00E+19 &  16.80 & 0.18\\ 
pg1309 & $0.18117$ (\#213)  & 43.39(38) & 27263 & nan & 74$\pm^{ 23 }_{ 19 }$ & $1.00$ & 22.3950 & 5.00E+19 &  16.80 & 0.23\\ 
pg1309 & $0.18139$ (\#214)  & 44.59(39) & 27263 & nan & 79$\pm^{ 21 }_{ 18 }$ & $1.00$ & 22.3992 & 5.00E+19 &  16.75 & 0.42\\ 
pg1309 & $0.18145$ (\#215)  & 44.58(39) & 27263 & nan & 78$\pm^{ 24 }_{ 18 }$ & $1.00$ & 22.4003 & 5.00E+19 &  16.80 & 0.42\\ 
pg1309 & $0.18192$ (\#216)  & 43.04(39) & 27263 & nan & 78$\pm^{ 25 }_{ 18 }$ & $1.00$ & 22.4092 & 5.00E+19 &  16.80 & 0.58\\ 
pg1309 & $0.18698$ (\#217)  & 43.52(37) & 27263 & nan & 79$\pm^{ 24 }_{ 19 }$ & $1.00$ & 22.5051 & 5.00E+19 &  16.80 & 0.52\\ 
pg1444 & $0.22031$ (\#218)  & 50.77(40) & 17630 & nan & 104$\pm^{ 38 }_{ 33 }$ & $1.00$ & 23.1371 & 1.07 &  15.81 & 17.52\\ 
pg1444 & $0.22676$ (\#219)  & 57.73(42) & 17630 & nan & 197$\pm^{ 39 }_{ 35 }$ & $1.00$ & 23.2594 & 5.00E+19 &  16.80 & 0.81\\ 
pg1444 & $0.26690$ (\#220)  & 91.99(69) & 17630 & 17137 & 162$\pm^{ 36 }_{ 32 }$ & $1.00$ & 24.0204 & 1.20E+16 &  16.78 & 0.06\\ 
pg1444 & $0.26728$ (\#221)  & 94.03(70) & 17630 & 17137 & 166$\pm^{ 36 }_{ 32 }$ & $1.00$ & 24.0276 & 4.95E+14 &  16.79 & 0.09\\ 
pg1444 & $0.26738$ (\#222)  & 94.02(70) & 17630 & 17137 & 166$\pm^{ 36 }_{ 32 }$ & $1.00$ & 24.0295 & 1.40E+16 &  16.79 & 0.10\\ 
pg1444 & $0.26747$ (\#223)  & 94.01(70) & 17630 & 17137 & 166$\pm^{ 36 }_{ 32 }$ & $1.00$ & 24.0312 & 5.00E+19 &  16.75 & 0.11\\ 
pg1626 & $0.13075$ (\#224)  & 28.51(25) & 69285 & nan & 214$\pm^{ 44 }_{ 42 }$ & $1.00$ & 21.4390 & 1.16 &  15.84 & 4.65\\ 
phl1811 & $0.07344$ (\#225)  & 64.36(45) & 77298 & 78895 & 51$\pm^{ 0 }_{ 0 }$ & $1.00$ & 20.3524 & 1.00 &  15.79 & 1.51\\ 
phl1811 & $0.07768$ (\#226)  & 59.44(40) & 78263 & 78895 & 51$\pm^{ 12 }_{ 11 }$ & $1.00$ & 20.4328 & 5.00E+19 &  16.75 & 0.08\\ 
phl1811 & $0.08131$ (\#227)  & 49.10(33) & 78178 & nan & 56$\pm^{ 14 }_{ 11 }$ & $1.00$ & 20.5016 & 5.00E+19 &  16.80 & 1.80\\ 
phl1811 & $0.13239$ (\#228)  & -- & -- & -- & -- & -- & 21.4701 & -- & -- & --\\ 
phl1811 & $0.13282$ (\#229)  & -- & -- & -- & -- & -- & 21.4783 & -- & -- & --\\ 
phl1811 & $0.13318$ (\#230)  & -- & -- & -- & -- & -- & 21.4851 & -- & -- & --\\ 
phl1811 & $0.13545$ (\#231)  & -- & -- & -- & -- & -- & 21.5281 & -- & -- & --\\ 
phl1811 & $0.15752$ (\#232)  & -- & -- & -- & -- & -- & 21.9466 & -- & -- & --\\ 
phl1811 & $0.15786$ (\#233)  & -- & -- & -- & -- & -- & 21.9530 & -- & -- & --\\ 
phl1811 & $0.17652$ (\#234)  & -- & -- & -- & -- & -- & 22.3068 & -- & -- & --\\ 
phl1811 & $0.19157$ (\#235)  & -- & -- & -- & -- & -- & 22.5922 & -- & -- & --\\ 
phl1811 & $0.19194$ (\#236)  & -- & -- & -- & -- & -- & 22.5992 & -- & -- & --\\ 
phl1811 & $0.19220$ (\#237)  & -- & -- & -- & -- & -- & 22.6041 & -- & -- & --\\ 
pks0312 & $0.20188$ (\#238)  & 58.64(41) & 23887 & nan & 194$\pm^{ 38 }_{ 35 }$ & $1.00$ & 22.7876 & 3.31E+16 &  16.79 & 0.01\\ 
pks0312 & $0.20275$ (\#239)  & 59.87(41) & 23887 & nan & 181$\pm^{ 37 }_{ 34 }$ & $1.00$ & 22.8041 & 1.94E+10 &  16.70 & 0.14\\ 
pks0405 & $0.09192$ (\#240)  & 40.76(43) & 137149 & nan & 285$\pm^{ 15 }_{ 14 }$ & $1.00$ & 20.7028 & 0.82 &  15.72 & 2.85\\ 
pks0405 & $0.09647$ (\#241)  & 44.12(43) & 137149 & nan & 305$\pm^{ 17 }_{ 20 }$ & $1.00$ & 20.7891 & 1.70E+14 &  16.78 & -0.00\\ 
pks0405 & $0.14808$ (\#242)  & -- & -- & -- & -- & -- & 21.7676 & -- & -- & --\\ 
pks0405 & $0.16566$ (\#243)  & 34.33(32) & 137647 & nan & 322$\pm^{ 21 }_{ 20 }$ & $1.00$ & 22.1009 & 5.20E+03 &  16.48 & 1.05\\ 
pks0405 & $0.16606$ (\#244)  & 35.08(32) & 137647 & nan & 320$\pm^{ 20 }_{ 20 }$ & $1.00$ & 22.1085 & 1.97E+03 &  16.49 & 1.17\\ 
pks0405 & $0.16659$ (\#245)  & 37.18(33) & 137675 & nan & 317$\pm^{ 20 }_{ 20 }$ & $1.00$ & 22.1185 & 2.55E+03 &  16.49 & 0.98\\ 
pks0405 & $0.16688$ (\#246)  & 37.31(33) & 137675 & nan & 316$\pm^{ 19 }_{ 19 }$ & $1.00$ & 22.1240 & 4.59E+03 &  16.48 & 0.80\\ 
pks0405 & $0.16712$ (\#247)  & 37.91(33) & 137675 & nan & 313$\pm^{ 21 }_{ 19 }$ & $1.00$ & 22.1286 & 752.48 &  16.44 & 0.51\\ 
pks0405 & $0.18257$ (\#248)  & 59.45(44) & 136430 & nan & 304$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.4215 & 0.82 &  15.71 & 2.41\\ 
pks0405 & $0.18289$ (\#249)  & 63.38(44) & 136430 & nan & 307$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.4276 & 1.11 &  15.82 & 1.39\\ 
pks0405 & $0.24052$ (\#250)  & 57.03(46) & 137245 & nan & 367$\pm^{ 20 }_{ 19 }$ & $1.00$ & 23.5203 & 4.17E+03 &  16.52 & 1.43\\ 
pks0405 & $0.24094$ (\#251)  & 61.56(45) & 137216 & nan & 377$\pm^{ 21 }_{ 19 }$ & $1.00$ & 23.5282 & 2.45E+06 &  16.56 & 1.85\\ 
pks0405 & $0.24547$ (\#252)  & 66.61(47) & 136481 & 138649 & 361$\pm^{ 19 }_{ 18 }$ & $1.00$ & 23.6141 & 1.37 &  15.88 & 0.52\\ 
pks0405 & $0.29762$ (\#253)  & 85.15(89) & 133010 & 137234 & 392$\pm^{ 21 }_{ 21 }$ & $1.00$ & 24.6029 & 141.00 &  16.42 & 2.58\\ 
pks0405 & $0.34188$ (\#254)  & 114.95(95) & 137986 & 137234 & 365$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.4420 & 1.83 &  15.97 & 0.02\\ 
pks0405 & $0.34225$ (\#255)  & 120.66(97) & 138000 & 137943 & 367$\pm^{ 19 }_{ 19 }$ & $1.00$ & 25.4491 & 1.64 &  15.93 & 0.05\\ 
pks0405 & $0.35092$ (\#256)  & 113.60(95) & 138000 & 136470 & 368$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.6134 & 1.37 &  15.87 & 0.23\\ 
pks0405 & $0.36075$ (\#257)  & 117.15(93) & 137986 & 134948 & 404$\pm^{ 21 }_{ 20 }$ & $1.00$ & 25.7998 & 1.91E+03 &  16.47 & 1.70\\ 
pks0405 & $0.36151$ (\#258)  & 115.63(94) & 138000 & 134948 & 404$\pm^{ 20 }_{ 20 }$ & $1.00$ & 25.8142 & 2.75E+05 &  16.56 & 3.70\\ 
pks0405 & $0.36329$ (\#259)  & 110.13(94) & 138000 & 134948 & 408$\pm^{ 22 }_{ 20 }$ & $1.00$ & 25.8480 & 2.17E+09 &  16.65 & 8.04\\ 
pks0405 & $0.40570$ (\#260)  & 109.37(95) & 137975 & 138647 & 415$\pm^{ 23 }_{ 21 }$ & $1.00$ & 26.6521 & 10.92 &  16.21 & 0.05\\ 
pks0405 & $0.40890$ (\#261)  & 111.06(95) & 137975 & 138647 & 432$\pm^{ 24 }_{ 23 }$ & $1.00$ & 26.7127 & 537.25 &  16.41 & 2.02\\ 
pks0405 & $0.49505$ (\#262)  & 96.58(89) & 136537 & 137118 & 387$\pm^{ 26 }_{ 25 }$ & $1.00$ & 28.3461 & 0.63 &  15.63 & 4.59\\ 
pks0405 & $0.49530$ (\#263)  & 97.66(89) & 136537 & 137118 & 389$\pm^{ 27 }_{ 26 }$ & $1.00$ & 28.3509 & 0.78 &  15.70 & 3.23\\ 
pks0405 & $0.55506$ (\#264)  & 98.30(94) & 138708 & 138714 & 363$\pm^{ 31 }_{ 30 }$ & $1.00$ & 29.4839 & 1.93 &  15.98 & 0.30\\ 
pks2005 & $0.06490$ (\#265)  & 60.15(62) & 54472 & 54641 & 1896$\pm^{ 53 }_{ 53 }$ & $1.00$ & 20.1905 & 0.66 &  15.64 & 1.94\\ 
pks2155 & $0.05405$ (\#266)  & 83.01(59) & 1701313 & 1685268 & 4444$\pm^{ 444 }_{ 409 }$ & $1.55$ & 19.9848 & 0.12 &  14.97 & 0.01\\
pks2155 & $0.05707$ (\#267)  & 76.79(59) & 1701521 & 1685268 & 4316$\pm^{ 448 }_{ 438 }$ & $1.62$ & 20.0420 & 0.17 &  15.11 & 7.35\\
q0045 & $0.11052$ (\#268)  & -- & -- & -- & -- & -- & 21.0555 & -- & -- & --\\ 
q0045 & $0.13521$ (\#269)  & -- & -- & -- & -- & -- & 21.5236 & -- & -- & --\\ 
q1230 & $0.09518$ (\#270)  & 44.14(33) & 39329 & nan & 48$\pm^{ 19 }_{ 18 }$ & $1.00$ & 20.7646 & 5.00E+19 &  16.75 & 1.10\\ 
q1230 & $0.10318$ (\#271)  & 48.14(34) & 39330 & nan & 56$\pm^{ 17 }_{ 15 }$ & $1.00$ & 20.9163 & 39.22 &  16.33 & 0.59\\ 
q1230 & $0.10445$ (\#272)  & 48.96(34) & 39330 & nan & 66$\pm^{ 18 }_{ 14 }$ & $1.00$ & 20.9404 & 5.00E+19 &  16.75 & 0.28\\ 
q1230 & $0.10530$ (\#273)  & 49.30(34) & 39331 & nan & 68$\pm^{ 17 }_{ 15 }$ & $1.00$ & 20.9565 & 5.00E+19 &  16.80 & 0.84\\ 
q1230 & $0.10596$ (\#274)  & 46.27(33) & 39331 & nan & 70$\pm^{ 17 }_{ 15 }$ & $1.00$ & 20.9690 & 5.00E+19 &  16.75 & 1.07\\ 
q1230 & $0.10666$ (\#275)  & 46.39(34) & 39331 & nan & 65$\pm^{ 21 }_{ 15 }$ & $1.00$ & 20.9823 & 5.00E+19 &  16.80 & 0.96\\ 
q1230 & $0.10809$ (\#276)  & 45.09(33) & 39331 & nan & 53$\pm^{ 20 }_{ 14 }$ & $1.00$ & 21.0094 & 5.00E+19 &  16.80 & 1.29\\ 
q1230 & $0.10820$ (\#277)  & 45.09(33) & 39331 & nan & 53$\pm^{ 20 }_{ 14 }$ & $1.00$ & 21.0115 & 5.00E+19 &  16.80 & 1.29\\ 
q1230 & $0.10861$ (\#278)  & 48.14(33) & 39331 & nan & 52$\pm^{ 20 }_{ 14 }$ & $1.00$ & 21.0192 & 5.00E+19 &  16.77 & 1.02\\ 
q1230 & $0.10906$ (\#279)  & 44.60(32) & 39332 & nan & 53$\pm^{ 25 }_{ 15 }$ & $1.00$ & 21.0278 & 5.00E+19 &  16.80 & 1.08\\ 
q1230 & $0.10935$ (\#280)  & 44.06(32) & 39332 & nan & 55$\pm^{ 17 }_{ 14 }$ & $1.00$ & 21.0333 & 5.00E+19 &  16.75 & 1.71\\ 
q1230 & $0.10956$ (\#281)  & 43.57(32) & 39332 & nan & 56$\pm^{ 21 }_{ 15 }$ & $1.00$ & 21.0373 & 5.00E+19 &  16.80 & 1.56\\ 
q1230 & $0.11707$ (\#282)  & 39.83(27) & 39333 & nan & 51$\pm^{ 20 }_{ 17 }$ & $1.00$ & 21.1796 & 1.06 &  15.81 & 13.29\\ 
q1230 & $0.11743$ (\#283)  & 34.85(25) & 39333 & nan & 57$\pm^{ 22 }_{ 19 }$ & $1.00$ & 21.1865 & 0.87 &  15.73 & 11.53\\ 
q1230 & $0.11781$ (\#284)  & 35.43(25) & 39333 & nan & 59$\pm^{ 22 }_{ 19 }$ & $1.00$ & 21.1937 & 0.88 &  15.74 & 10.59\\ 
rbs1892 & $0.15752$ (\#285)  & -- & -- & -- & -- & -- & 21.9466 & -- & -- & --\\ 
rbs1892 & $0.17133$ (\#286)  & 46.32(37) & 4929 & nan & 312$\pm^{ 101 }_{ 76 }$ & $1.00$ & 22.2084 & 5.00E+19 &  16.80 & 0.45\\ 
rbs1892 & $0.19874$ (\#287)  & 50.02(44) & 4929 & nan & 332$\pm^{ 100 }_{ 76 }$ & $1.00$ & 22.7281 & 5.00E+19 &  16.80 & 0.16\\ 
rbs542 & $0.10323$ (\#288)  & 48.13(48) & 192804 & nan & 1054$\pm^{ 22 }_{ 22 }$ & $1.00$ & 20.9172 & 0.67 &  15.64 & 0.84\\ 
rbs542 & $0.10379$ (\#289)  & 48.09(47) & 192375 & nan & 1053$\pm^{ 22 }_{ 22 }$ & $1.00$ & 20.9279 & 0.72 &  15.67 & 0.52\\ 
rxj0439 & $0.11547$ (\#290)  & 38.76(35) & 151442 & nan & 337$\pm^{ 18 }_{ 18 }$ & $1.00$ & 21.1493 & 0.66 &  15.64 & 4.30\\ 
rxj0439 & $0.21833$ (\#291)  & 61.09(43) & 145661 & nan & 419$\pm^{ 22 }_{ 22 }$ & $1.00$ & 23.0995 & 0.73 &  15.68 & 5.79\\ 
rxj0439 & $0.24235$ (\#292)  & 63.87(47) & 151874 & 121198 & 498$\pm^{ 26 }_{ 21 }$ & $1.00$ & 23.5550 & 3.91E+03 &  16.50 & 2.82\\ 
rxj0439 & $0.24258$ (\#293)  & 69.70(49) & 151906 & 131963 & 497$\pm^{ 21 }_{ 21 }$ & $1.00$ & 23.5593 & 8.51E+03 &  16.48 & 2.55\\ 
rxj0439 & $0.24313$ (\#294)  & 66.17(48) & 151874 & 131963 & 498$\pm^{ 23 }_{ 22 }$ & $1.00$ & 23.5697 & 95.90 &  16.40 & 1.44\\ 
rxj0439 & $0.24387$ (\#295)  & 71.95(50) & 151906 & 137345 & 497$\pm^{ 22 }_{ 21 }$ & $1.00$ & 23.5838 & 7.92 &  16.23 & 0.33\\ 
s50716 & $0.23145$ (\#296)  & 57.72(42) & 75697 & nan & 741$\pm^{ 36 }_{ 35 }$ & $1.00$ & 23.3483 & 1.73E+04 &  16.48 & 0.15\\ 
ton28 & $0.13746$ (\#297)  & -- & -- & -- & -- & -- & 21.5662 & -- & -- & --\\ 
ton28 & $0.13773$ (\#298)  & -- & -- & -- & -- & -- & 21.5714 & -- & -- & --\\ 
ton28 & $0.13781$ (\#299)  & -- & -- & -- & -- & -- & 21.5729 & -- & -- & --\\ 
ton28 & $0.17251$ (\#300)  & 50.74(37) & 81682 & nan & 131$\pm^{ 18 }_{ 17 }$ & $1.00$ & 22.2308 & 2.63 &  16.05 & 0.60\\ 
ton28 & $0.21259$ (\#301)  & 60.47(42) & 81454 & nan & 188$\pm^{ 20 }_{ 19 }$ & $1.00$ & 22.9907 & 1.82E+04 &  16.50 & 0.00\\ 
ton28 & $0.24292$ (\#302)  & 30.56(48) & 85563 & 83705 & 186$\pm^{ 19 }_{ 19 }$ & $1.00$ & 23.5658 & 7.04E+06 &  16.58 & 0.18\\ 
ton28 & $0.24859$ (\#303)  & 52.11(52) & 84503 & 85711 & 180$\pm^{ 20 }_{ 19 }$ & $1.00$ & 23.6733 & 3.40 &  16.10 & 0.42\\ 
ton28 & $0.27338$ (\#304)  & 80.27(77) & 85129 & 86614 & 205$\pm^{ 19 }_{ 19 }$ & $1.00$ & 24.1433 & 1.60 &  15.93 & 0.97\\ 
ton28 & $0.33021$ (\#305)  & 107.71(94) & 85874 & 86028 & 199$\pm^{ 20 }_{ 19 }$ & $1.00$ & 25.2208 & 1.21 &  15.85 & 2.04\\ 
tons180 & $0.02340$ (\#306)  & 99.08(96) & 177396 & 194071 & 901$\pm^{ 18 }_{ 18 }$ & $1.00$ & 19.4037 & 0.68 &  15.65 & -0.00\\ 
tons180 & $0.04360$ (\#307)  & 69.00(82) & 187350 & 195496 & 955$\pm^{ 18 }_{ 18 }$ & $1.00$ & 19.7867 & 0.68 &  15.66 & -0.01\\ 
tons180 & $0.04560$ (\#308)  & 67.80(80) & 187350 & 195974 & 963$\pm^{ 19 }_{ 19 }$ & $1.00$ & 19.8246 & 0.84 &  15.74 & 0.60\\




\hline
\hline
\end{longtable}
\end{landscape}

==> deleted.tex <==

\begin{comment}
\section{Upper limits of \ovii\ and \oviii\ absorption lines}
\label{sec:UL}

The results of Sect.~\ref{sec:results} show that the current--generation \xmm\ and \chandra\ 
grating data
do not have sufficient resolution to conclusively detect X--ray absorption lines
even from the most prominent \ovii\ and \oviii\ resonant transitions. Accordingly, we
set out to use this analysis to place upper limits to the non--detection of
X--ray absorption lines at the FUV priors, and to interpret the non--detection
as an upper limit to the cosmological density of baryons in the X--ray WHIM.

\subsection{Determination of upper limits to the ion column density}
\label{sec:ULMethods}

The first task is to determine upper limits to the non--detection of
the $\tau_0$ parameter of 
redshifted absorption lines at the fixed redshifts from the FUV priors.
For this task, we make use of the spectral analysis of Tables~\ref{tab:OVIIOVIXMM} through \ref{tab:OVIIIHIChandra}, 
where the measured values of the parameter are reported. By design, these
parameters are allowed to have either sign, i.e., $\tau_0 \in \mathbb{R}$, although
the physically allowed range for an absorption line is $\tau_0 \geq 0$, with
$\tau_0=0$ representing the null hypothesis that there is no absorption line. The reason for allowing
the parameter to be any real number is so that the $\Delta C$ \gof\ statistic for the 
presence of an absorption can be used for hypothesis testing, as was
discussed in Sect.~\ref{sec:resultsRedshifted}.
The statistical problem at hand is that of making inference on the physical parameter $\theta=\tau_0 \geq$ of each system, making use of measurements that are in the 
form of $\tau_{0,i}=t_i\pm^{\Delta t_i^+}_{\Delta t_i^-}$.

The statistical issues associated with this problem, and the choices
made for this application, are discussed in Appendix~\ref{app:UL}. The method
we chose consists of setting  \emph{average} of the positive and negative
uncertainties in the parameter  as the upper--limit to the value of the parameter.
For example, the best--fit value for the first entry in Table~\ref{tab:OVIIOVIXMM}
is $\tau_0=+0.55\pm^{1.78}_{0.88}$, resulting in an upper limit of $\overline{\tau}_0=1.31$.


The equivalent width $W_{\lambda}$ of a line is
a known function of the measured parameter $\tau_0$, and it is automatically
calculated by \texttt{SPEX} (see e.g. the \texttt{line} model
component definition). In turn, the equivalent width is a linear function 
of the column density of the implied ion, when the line is in the linear part of
its curve of growth,
\begin{equation}
    N= 1.13 \times 10^{20} \dfrac{W_{\lambda}}{\lambda^2 f} \quad (\text{cm}^{-2}),
    \label{eq:EW-N}
\end{equation}
where $\lambda$ is the wavelength and $f$ the oscillator strength of the line, see e.g. \cite{bonamente2016}. Therefore, there is a one--to--one correspondence between the
measured $\tau_0$ parameter and the implied column density. Moreover, the $\tau_0$ parameter, which corresponds to
the optical depth at line center for the assumed Gaussian line profile, is also linearly proportional to the column density, in the same linear regime where \eqref{eq:EW-N} is applicable \citep[e.g.][]{kaastra2008}.
For the practical data analysis task of estimating the upper limit to the column density $N$ of an ion (see Appendix~\ref{app:UL}), we can use this linearity when converting upper limits on $\tau_0$ to upper limits
on $N$.
 

\subsection{Constraints on cosmological density of X--ray WHIM gas}
\label{sec:cosmo}

The large number of sources and the redshift path covered by this sample can be used to 
constrain the cosmological density of baryons implied by the upper limits reported in Sec.~\ref{sec:ULMethods}.
 We refer to this density as \ObX, to imply that it only comprises
the hotter portion of baryons as tracked by \ovii\ and \oviii\ absorption lines. The method makes use of the analysis of \eagle\ simulations to predict
the amount of \ovii\ and \oviii\ column density expected from the detected FUV systems, which was
presented in a previous study \citep{spence2023}. In that paper, we applied the method to the analysis of
one of the sources analyzed in this paper, viz. \es, and found that the non--detection of absorption lines could be interpreted with an upper limit $\ObXbEq \leq 0.90$ for reasonable choices of the temperature and abundance of the 
probed gas, meaning that the X--ray absorbing WHIM is consistent with being the repository of the missing baryons. We outline the method in the following.

The method of analysis starts with the usual relationship
\begin{equation}
 \Omega_{\mathrm{WHIM,ion}} =\Omega_{\ion} \dfrac{\mu_H \, m_H}{m_{\ion}} \dfrac{1}{A \cdot f_{\ion}(T)}
\label{eq:Omega}
\end{equation}
where 
\begin{equation}
    \begin{cases}
        \Omega_{\text{ion}}= \dfrac{\rho_{\text{ion}}}{\rho_c} \text{, and}\\[10pt]
\rho_{\ion} = m_{\ion} \dfrac{N_{\ion}}{D_i},
    \end{cases}
\end{equation}
are the relationships that link the observable column density $N_{\ion}$ to the cosmological density
of baryons, with $D_i$ the distance to the source, $A$ the metal abundance of the gas, $f_{\ion}(T)$
the ionization fraction for the assumed temperature $T$, with all other
constants having the usual meaning (see \citealt{spence2023}). Equation~\ref{eq:Omega} applies to a single source
and a single ion/absorption line. 

The equation can 
 be generalized to multiple sources via
\begin{equation}
\OWHIMX= \dfrac{\mu \, m_H}{\rho_c} \dfrac{{\sum_i} N_{H,i}}{\sum_i D_i}
\label{eq:OmegaWHIMX}
    \end{equation}
    \citep[see, e.g.,][]{schaye2001,nicastro2018}
where the sum extends over all available sources, and the $i$--th source probes
a cosmological distance $D_i$ with a detection of a total WHIM column density $N_{H,i}$, representing
the entire baryonic content of the WHIM. It is clear that care must be exercised in not double--counting absorbers that may
be probing the same $N_{H,i}$ column density (e.g., \ovii\ and \oviii\ that may be originating from the same gas phase); this
issue will be addressed in Sec.~\ref{sec:systematics} below.

In the case of upper limits to the detection of $N_{\ion}$, and therefore of $N_{H,i}$, it is not accurate to just
replace the measurements with upper limits of those quantities in \eqref{eq:Omega} or \eqref{eq:OmegaWHIMX}. 
Rather, in \cite{spence2023} we proposed a method that consists of calculating the \emph{expectation} of the 
column density that is implied by the non--detection, viz. 
\begin{equation}
    \E[\nioni^+]=\sum_{j=1}^{n_i} \E[\nionj^+],
    \label{eq:nionMinus}
\end{equation}
which represents an \emph{average upper limit} to the column density of
the ion that was systematically not detected in a given source, with $n_i$ the number of absorption lines that were probed for
the $i$--th source (note that the index $j$ refers to the $j$--th absorption system for $i$--the source).
The expectation is intended as a probabilistic expectation based on the distribution of values for the 
ion $N_{\ion,j}$ \emph{given} the amount of detected FUV absorption (e.g., either \ovi\ or \hi) as calculated
according to the \eagle\ simulations \citep{wijers2019}. These expectations are a function of the
measured upper limit \NUL, with a higher upper limit naturally corresponding to a larger expectation,
and take into account the measured FUV column density.  A complete description of this method is presented in Sec.~5 of \citep{spence2023}, which we follow in this paper.~\footnote{A more 
appropriate notation for the expectations in the right--hand side of \eqref{eq:nionMinus} would be
$\E[\nionj^+] \coloneq \E[\nionj\ | N_{\mathrm{FUV},j}, \NULeq]$, i.e., the expected ion column \emph{given} the measured value of
the FUV column density, and given the measured upper limit to the non--detection of the X--ray ion.}

In practice, after observational upper limit \NUL\ are obtained for each absorption line system of each source, we 
calculate each expectation $\E[\nionj^+]$, and then sum according to \eqref{eq:nionMinus}. 
That number is used to calculate
the expectation on the column density of the associated hydrogen according to the usual
\begin{equation}
    \E[N_{H,i}]= \dfrac{\mu_H m_H}{m_{\ion} A f_{\ion}(T)}\E[\nioni^+],
\end{equation}
and from this the upper limit on $\OWHIMX$ is obtained from \eqref{eq:OmegaWHIMX}, viz.
\begin{equation}
    \ObXEq \leq  \dfrac{\mu_H \, m_H}{\rho_c\, A\, 
    f_{\ion}} \dfrac{\sum_i\E[\nioni^+]}{\sum_i D_i}.
    \label{eq:OmegaWHIMXUL}
\end{equation}
with the sum at the numerator being the sum of the expected ion column
densities over all sources and all absorption line systems. 
Cosmological results according to \eqref{eq:OmegaWHIMXUL} are presented in Table~\ref{tab:OmegaWHIMXUL}, where $D$ is the sum of all distances, and $\Delta z$
the total redshift path sampled.

\begin{table}
    \centering
    \begin{tabular}{l|ll|ll}
\hline
\hline
Sample & $\log D$ & $\Delta z$ &  $\log \E[\nion^+]$ & \ObXbFrac \\
       & (Mpc) &  & (cm$^{-2}$)  &  \\[3pt]
\hline
 \expandableinput Omegas-ALL.tex
\hline
\hline
    \end{tabular}
    \caption{Cosmological constraints from the upper limits to the systematic non--detection
    of absorption lines. The numerical values of the ratios $\ObXbEq$ are to be rescaled by
    the factor $\left({A}/{0.1 \text{ Solar}}\right)^{-1} \left({\fion}/{\fionref}\right)^{-1}$, where the reference value for the ionization fractions
    was set to $\fionref=1.0$ for \ovii, and to $\fionref=0.1$ for \oviii.}
    \label{tab:OmegaWHIMXUL}
\end{table}

\subsection{Systematics}
\label{sec:systematics}



The cosmological results derived from the upper limits discussed in Sec.~\ref{sec:cosmo}
are affected by a number of sources of systematic error which we proceed to examine.

\subsubsection{Temperature and abundance}
First, the X--ray data we have analyzed do not provide meaningful constraints on the 
temperature and abundance of the absorbers for most of the sources. In the case of the strongest sources,
constraints on the temperature could be obtained by line ratios of ions of the same
elements, similar to what was done in \citep{ahoranta2020} or \cite{ahoranta2021}.
Given the limited resolution of the X--ray data for several of the sources in this sample,
we limit ourselves to parameterize the results as a function of an assumed temperature and abundance. For example, the first entry in Table~\ref{tab:OmegaWHIMXUL} reads
\[
\ObXbFracEq \leq 7.94\, \times \left(\dfrac{A}{0.1 \text{ Solar}}\right)^{-1} \left(\dfrac{\fion} 1\right)^{-1} \quad \text{(XMM OVII/OVI)}
\]
where it was assumed a 10~\% Solar abundances of heavy elements, and a temperature that corresponds to a 100~\% ionization fraction of \ovii, which corresponds to the peak
of the ionization curve in collisional equilibrium around $\log T(K) \simeq 5.8-6$ \citep{mazzotta1998}. Given that \oviii\ reaches at most a $\sim$~20\% peak ionization
near $\log T(K) \simeq 6.3$, entries in Table~\ref{tab:OmegaWHIMXUL} that correspond to \oviii\ were parameterized based on an assumed 10~\% ionization fraction, e.g., the third entry reads
\[
\ObXbFracEq \leq 49.95\, \times \left(\dfrac{A}{0.1 \text{ Solar}}\right)^{-1} \left(\dfrac{\fion} {0.1}\right)^{-1}  \quad \text{(XMM OVIII/OVI)}
\]
It is clear that the order--of--magnitude difference between the two limits is simply
a result of the different $\fion$ used in the calculation.
\begin{figure*}
    \centering
    \includegraphics[width=6.5in]{logN-XMM.pdf}
    \caption{Distributions of: FUV column densities (cyan) from \protect\cite{tilton2012}
    and \protect\cite{danforth2016}; expected column densities        $\E[N^+]$ for all absorption line systems
    that are summed in \eqref{eq:nionMinus}, calculated using the "sensitivity" and the Feldman--Cousins methods (color--coded); and  X--ray upper limits  to the measurable column densities for the two methods (orange and grey), 
    for the \xmm\ data. }
    \label{fig:logN-XMM}
\end{figure*}

\subsubsection{Estimate of $\E[\nion^+]$}

The method used in this paper to calculate \ObX\ is based on the use of \eagle\ simulations
to predict the average amount of \ovii\ and \oviii\ along a given sightline with a prior FUV detection (see Sec.~\ref{sec:cosmo} and Sec.~5 of \citealt{spence2023}).
The key assumptions of this method are that (a) the FUV data has identified all possible
redshifts where associated X--ray absorption can be found; and (b) the $\log N$--$\log N$
scaling relation between the FUV and X--ray column densities are accurate in predicting \ovii\ and \oviii\ column densities associated with the \ovi\ and \hi\ FUV absorbers (these
releationships were identified by \citealt{wijers2019} and were studied in \citealt{spence2023}).
Both of these assumptions are reasonable, but basically untested, given the paucity of X--ray absorption line systems and their limited resolution.

For assumption (a), we point out that X--ray absorbers need not necessarily be associated with
FUV systems. For example, systems with $\log T(K) \gtrsim 6$ would have minimal or no \ovi\ absorption, and therefore they would be missed by a search based on \ovi\ priors, like the present one. Therefore it is possible that our search has missed hotter absorption--line systems at other redshifts.

Regarding assumption (b), the use of \eagle\ scaling relations to estimate upper limits to the column density of \ovii\ and \oviii\ is also a convenient tool, yet one that is also largely untested. In particular, the distributions of Figs.~\ref{fig:logN-XMM}
and \ref{fig:logN-Chandra} show that sightlines with \hi\ priors predict substantially
\emph{lower} X--ray column densities than those with \ovi\ priors, according
to the \cite{wijers2019} analysis of the \eagle\ simulations. This is the reason for substantially tighter constraints on \ObX\ based on the \hi\ FUV priors in Table~\ref{tab:OmegaWHIMXUL}.




Other methods could be used to set an upper limit $\E[\nionj^+]$ to the column density along
a specific sightline. A direct method would be that of using the measured upper limit \NULj\
itself, which would correspond to ignoring the information provided by the column density of the FUV prior, and the predictions based on \eagle. That method would generally give substantially larger upper limits to \ObX, given that the \eagle\ expectations for the unobserved column densities
are substantially lower than the raw X--ray upper limits, see Figs.~\ref{fig:logN-XMM}
and \ref{fig:logN-Chandra}.




Moreover, as already remarked in \cite{spence2023}, our method of FUV priors implies
that we consider \emph{all} absorption line systems and sum the expected column densities
according to \eqref{eq:nionMinus}, as per assumption (a). 
In the absence of FUV priors, one could set the amount of the unobserved column density to
the value of the most stringent upper limit along that sightline. However, that method
would ignore both the observed FUV priors, and the predictions based on \eagle\ simulations.

\subsubsection{Double counting of absorption systems}

Certain sightlines have a large number of \ovi\ and \hi\ FUV absorption line systems, which
we treat as independent for the sake of predicting the associated X--ray column densities, i.e., we make X--ray predictions for each and then we sum them.
It is possible that certain FUV systems are in fact associated with the same absorber,
and therefore it would be appropriate to first add the prior FUV column densities
of all systems that are physically associated, and then predict just one X--ray column density per system, using the summed FUV prior column density. The FUV data used in this paper do not provide an unequivocal way to determine such
association, and therefore we did not attempt it. However, we find that the predicted
$\E[\nionj^+]$ has a positive relationship to the column density of the FUV prior
(see Fig.~8 of \citealt{spence2023}), so that the order
in which to add column densities (adding the FUV priors first, or adding the 
expected X--ray column densities for each FUV system) should not be a major source of
systematic uncertainty.


%{\color{blue} Or do we? If we sum about 10 non-detections with terrible resolution this drives the upper limit too high. There is a prior on the quality of the FUV and the number of lines detected there that must be taken into account.}

\section{Discussion and conclusions}
\label{sec:discussion}


\begin{figure*}
    \centering
    \includegraphics[width=6.5in]{logN-Chandra.pdf}
    \caption{Same as Fig.~\ref{fig:logN-XMM}, for the \chandra\ data.}
    \label{fig:logN-Chandra}
\end{figure*}

\clearpage
\appendix

\section{Determination of upper limits}
\label{app:UL}

The goal of this section is to provide an answer to the following
question, for each fit in Tables~\ref{tab:OVIIOVIXMM} through \ref{tab:OVIIIHIChandra}: \emph{At a given confidence level, what is the largest value allowed for the column density of
an ion along a specific sightline}?
Given the one--to--one correspondence between the $\tau_0$ parameter and the column density $N$, as given by \eqref{eq:EW-N}, it is therefore necessary to use the measurements
of $\tau_0$ to answer the question. We will refer to such column density as the
upper limit $N^+$, which is of course a function of the confidence level chosen for the
probabilistic statement.

The upper limit for each ion and sightline will
then be used to assess an upper limit to the cosmological density of baryons according to
Equations~5 and 11 of \cite{spence2023}, as a sum over all measurements. We are therefore
not interested in a regression of the $N_{\text{ion},i}^+$ measurements to obtain, e.g., their
mean value or other properties. Such methods of regression with upper limits, if interesting
for other applications,
could be performed with the \cite{kaplan1953} estimator, which was
popularized for astronomy by \cite{feigelson1985} as a means to fit data with upper limits.

\subsection{General considerations for confidence intervals on model parameters}
\label{sec:confidenceIntervals}
The task of estimating one or more model parameters $\theta$, in this case the single
parameter $\tau_0$ for the line component, is a central problem in modern statistics.
The point estimate is obtained via the method of \ml, which was pioneered by
R.~A. Fisher \citep[e.g.][]{fisher1925}, and it is the method that 
we follow via the minimization of
the \gof\ \cmin\ statistic. The determination of 
confidence intervals on model parameters in essence consists of 
a devising a suitable method to `invert' probabilities, i.e.,
converting a probability of the observed quantity given an unknown parameter, 
to a probability statement regarding the true model parameters. All the considerations provided in the following apply to the general case of a confidence interval 
with both lower and upper limit, although they are illustrated here for an upper limit, given the case at hand.

Let $x$ be the one of the $i$ observations of the unknown parameter $\theta=\tau_{0}$, i.e.,
one of the entries in Tables~\ref{tab:OVIIOVIXMM} through \ref{tab:OVIIIHIChandra}.
In general, the observations could be of a different \emph{statistic} $x$ that is related to 
the true parameter $\theta$, although in this case it is a measurement of the parameter itself, via the parametric spectral fits described in the paper. 
The (true) parameter $\theta$ is not only unknown, but it is also \emph{fixed}; this is a standard tenet
of the classical statistical approach to parameter estimation  (for example,
see Sec.~12.4 of \citealt{wilks1962} or \citealt{neyman1937}). The statistic or measurement
$x$, on the other hand, is a \emph{random variable} that is assumed to have a known distribution, and
for which it is therefore meaningful to calculate probabilities of occurrence of any
set of values. In the case at hand, for example,
\def\P{\mathrm{P}}
\begin{equation}
\P(x \leq x^u | \theta) = 1-\alpha
\label{eq:PDirect}
\end{equation}
with $\alpha$ a small number, say $\alpha=0.05$ \citep[e.g.][but other choices are also reasonable]{asa2016},
the number $x^u$ would be an upper limit with confidence $1-\alpha$, say 95\%. This means that,
given the distribution of the statistic, 95\% of the observations should yield a value
lower than $x^u$. The notation used for the probability means that one has to assume a
value for the true parameter $\theta$, which is of course unknown.
%, although the distribution itself cannot be
%dependent on that value, if one wants to make certain inferences
%of the true parameter \citep[e.g.][]{wilks1962}, as explained below. 
Often the distribution of a measured
statistic is normal,
and this is the assumption we make in this case; same considerations apply for other distributions.

A \emph{confidence interval} on a parameter, on  the other hand, can be defined
as
\begin{equation}
    \P(\theta \leq \theta^u | \theta) = 1-\alpha
    \label{eq:PInverse}
\end{equation}
which is misleadingly similar in form to \eqref{eq:PDirect}. In fact, what is random
here is the data range $(0, \theta^u)$, and not $\theta$.~\footnote{In general,
when the parameter $\theta$ is a function of different statistic $x$, 
the data range or set $X^u$ (i.e., for $x \in X^u$) corresponds to
a random range $\overline{\theta}(X^u)$ for the parameter such that
\begin{equation}
    \P(\theta \leq \overline{\theta}(X^u) | \theta) = 1-\alpha,
    \label{eq:PInverseGeneral}
\end{equation}
see e.g. \cite{wilks1962}. This notation could be extended also to more than one
parameter $\theta$.} 
Therefore the interpretation of
\eqref{eq:PInverse} is that the data measured range includes the true value $\theta$
in a $1-\alpha$ fraction of cases when such experiment is repeated. 
A clear an concise textbook explanation of this method is provided in Ch.~11 of~\cite{rohatgi1976},
and a more theoretical discussion in Ch.~12 of \cite{wilks1962}, which summarizes
the original \cite{neyman1937} method for confidence interval estimation. 

\subsection{The Feldman--Cousins method}
\label{sec:FC}
For applications in the physical sciences, often an additional complication
arises that is concerned with certain parameter values being `unphysical', for a given application.
Consider as an example one of the measurements from Table~\ref{tab:OVIIOVIXMM},
say $\tau_0=-3.86^{+0.55}_{-0.40}$  in line 17 of the table. A negative
best--fit value means that there is evidence for an \emph{emission line}
feature at that wavelength. This feature is likely caused by a random fluctuation of the
Poisson spectrum at that wavelength, or to the presence of an unrelated emission
phenomenon, or perhaps a combination of both. Either way, a formal confidence interval
on the measured parameter $\tau_0$ would remain negative, which would make it impossible to answer the question at hand.

The seminal contribution by \cite{feldman1997} addresses this exact issue that is
present in our data, whereas our question requires that the true parameter
is non--negative. Their
idea is to consider confidence intervals on the unknown parameter of the 
absorption line process, which we indicate as $\theta$ to distinguish it from the measurement itself, based on the ratio of two probabilities or likelihoods,
\begin{equation}
    R = \dfrac{P(\tau_0|\theta)}{P(\tau_0|\theta_{\mathrm{best}})}
    \label{eq:FC}
\end{equation}
with $\theta_{\mathrm{best}}=\max(0,\tau_0)$. Possible values of the unknown parameter $\theta$ are then chosen among those with the largest
value of $R$, subject to the constraint $\theta \geq 0$, while the measurement $\tau_0$
can in fact be negative. This method, hereafter referred to as the FC method, 
requires the specification of the conditional distributions
in \eqref{eq:FC}, which in this case we assume to be Gaussian, and it returns
a range ($\theta_{min},\theta_{max}$) as a confidence interval at a given level of confidence .~\footnote{
The method is explained in detail in Sec.~IV~B of \cite{feldman1997}. For \texttt{python}, this method
is implemented in the \texttt{gammapy} software version $\leq 0.7$, or from 
the \texttt{FCpy} software \citep{groopman2023}. } 



To implement the FC confidence interval method, we start with the assumption that the
probability distribution $P(\tau_0|\theta)$ is normal. This assumption is somewhat at odds
with the asymmetric errors provided by the $\Delta C=1$ method for several sources, which indicate a more
complex probability model than the Gaussian. In fact, a normal
distribution for the parameter $\tau_0$ would result in a parabolic
log--likelihood function, and therefore symmetric $\Delta C$ intervals 
\citep[see, e.g., Sec.~2.3 of][]{james2006}.
 Nonetheless, we proceed with the Gaussian assumption as an approximation,
and set the standard deviation of the distribution is equal to the average of the
two errors (e.g., we assume $\sigma=0.47$ for the measurement $\tau_0=-3.86^{+0.55}_{-0.40}$)
and is thereafter considered as fixed parameter. 
Our crude method to average the positive and negative error
bars is simply one of convenience, given the size of the sample. We expect that the errors
introduced by this method for a given upper limit would average down when inferences are made
for the entire sample.

Moreover, we also adjust the best--fit value to the midpoint of the range (e.g., $\tau_{0,\mathrm{adj}}=-3.79$); we will 
compare results with and without this adjustment to test the effects on our results.
Upon division by the assumed $\sigma$ parameter, all scaled measurements $x=\tau_{0}/\sigma$ 
are therefore  assumed to be distributed like a Gaussian with unit variance, 
$x \sim N(\theta, 1)$, and to
these scaled values we can then apply the same FC method.

The situation is illustrated in Fig.~\ref{fig:FC}, which reproduces closely the
example provided by Fig.~10 of  \cite{feldman1997} that applies to a Gaussian with unit variance. The band is constructed horizontally for a given value of the mean $\mu=\theta$,
by requiring
\[
\int_{x_L}^{x^U} P(x|\theta) dx = 1- \alpha
\]
with the choice of $\alpha=0.1$, so that a horizontal range contains 90\% of probability.
The FC requires that the limits $x_L$ and $x^U$ are chosen in such a way that they bracket
the maximum of $R$ according to \eqref{eq:FC}, which contains the assumption that the
parent mean must be non--negative.
\begin{figure}
    \centering
    \includegraphics[width=3.2in]{fcUL.pdf}
    \caption{The Feldman--Cousins 90\% confidence band for Gaussian measurements $x$, with unit variance ($\sigma^2=1$) and mean $\mu$. A horizontal line between the two curves at a given value of $\mu$ is a 90\% confidence interval on possible measurements drawn from that distribution. A vertical interval between the two curves at the value of a possible measurement $x$ is a 90\% confidence interval on the possible parent  mean $\mu$.}
    \label{fig:FC}
\end{figure}
For a given standardized measurement $x_i=\tau_{0,i}/\sigma_i$, the upper limit
is the intersection of the vertical line at $x=x_i$ with the red upper limit curve.
Even in those cases with a sufficiently large value of $x_i$, we only consider an upper limit $\theta^U_i$, and ignore the lower limit, as a further conservative measure. The FC method 
therefore yields an upper limit to the line parameter $\tau_{0,i}^U=\theta^U_i \, \sigma_i$,
which is then immediately translated into $N^+_i$.

Notice how the FC method avoids the \emph{empty interval} problem, which would
appear for substantially negative measurements such as the one already considered.
\emph{If} we were to choose the measured value of $\tau_0=-3.86$ as the best--fit estimate 
for the true Gaussian mean, then a 90\% confidence interval would remain negative.
This problem is solved by the use of the likelihood ratio, and was one of the main
motivations behind the method developed by \cite{feldman1997}.






%classical --- i.e., non--Bayesian --- confidence intervals on model parameters requires a 



\subsection{The `sensitivity' method}
\label{sec:ULApproximate}

An alternative method to use the measured $\tau_0$ parameters to set upper limits
on its parent value $\theta$ 
is also considered. The method is based
on the following considerations.
First, the best--fit value itself
(i.e., $\tau_0=-3.86$ for the sample entry) is not interesting, 
since a best--fit value that is positive or negative simply means that the center of the
possible line falls at a position with a number of detected counts that is (randomly) either 
lower or greater than the neighboring points, respectively.
Second, the most useful part of the regression is the measurement of the parameter's uncertainty, which reflects the ability of a given set of data to constrain the model, or its `sensitivity'. In fact, a similar fit to a \texttt{line} model in a neighboring portion
of the spectrum would necessarily have a different best--fit parameter $\tau_0$, but a similar uncertainty, since the data have 
similar number of counts, and the null model (i.e., the power--law) is smooth over the 
$\pm 1$~\AA\ range under consideration. 


The interest is in setting an upper limit to $\theta$, as a means to find the largest value
for the unknown parameter that is allowed by the data, at a given confidence level. This is akin to what is usually done in
source detection with Poisson statistics \citep[e.g.][]{li1983}. In this case, however, 
we assume that the sampling distribution of the parameter $\tau_{0,i}$
for a specific regression is a Gaussian
with unknown mean $\theta \geq 0$, and a variance given by the measured variance $\sigma^2_i$, same as in the previous method. This means that
a measurement is $x_i=\tau_{0,i} \sim N(\theta,\sigma^2_i)$. 

According to this assumption, the one--sided confidence range on $\theta$ with significance
$\alpha$ is set by the condition
\begin{equation}
    P(x>0|\theta) \geq 1-\alpha \quad \text{or} \quad P(x \leq 0| \theta) \leq \alpha
    \label{eq:UL}
\end{equation}
with $\alpha$ the usual small probability, say $\alpha=0.1$ for a 90\% confidence level.
Eqn~\ref{eq:UL} means that one allows (at most) a small residual probability $\alpha$ to measure a negative 
value for the parameter, when the true parameter is $\theta$. In other words, 90\% of the times
a measurement is made from a distribution with such value of $\theta$, the measurement will be positive.
It is immediate to see that, given the normal sampling distribution, \eqref{eq:UL} is satisfied by
\begin{equation}
    \theta \geq 1.65 \sigma,
    \label{eq:CIDirect}
\end{equation}
which can be interpreted as the 90\% C.I. on $\theta$.~\footnote{An equivalent method is used to set
upper limits to the Poisson mean, see e.g. Ch.~7 of \cite{bonamente2023} and \cite{gehrels1986}.}

Let's look at this confidence interval in a different way. Eqn~\eqref{eq:UL} also implies, for the choice 
of $\alpha=0.1$,
\begin{equation}
     P\left(\dfrac{x - \theta}{\sigma} \leq - 1.65\right)=P(\theta\geq x+1.65\, \sigma) \coloneq P(\theta \geq \theta^u) \leq  \alpha,
    \label{eq:UL2}
\end{equation}
with all $\theta$ values satisfying \eqref{eq:UL2} being the values in this confidence 
interval for the parameter $\theta$, and for a given measurement $x \geq 0$. 
This is the type of `classical' confidence 
intervals discussed in Sec.~\ref{sec:confidenceIntervals} in the introduction of this Appendix.~\footnote{ It is clear that $\theta$ is and remains fixed, so the last inequality should be read right--to--left,
i.e., the random interval $(x+1.65\, \sigma, \infty)$ contains the unknown value of $\theta$ 
a fraction $\alpha$ of times that the measurement of $x$ is made. This consideration is mostly
interesting for theoretical purposes, and in practice the data analyst needs not worry about it.}
The one--sided confidence interval with confidence  $\geq 1- \alpha$ is
\begin{equation}
S(x) = (x+1.65\, \sigma, \infty),
\label{eq:CIClassical}
\end{equation}
and it is also referred to as a \emph{fiducial} confidence interval \citep[e.g.][]{fisher1935, wilks1962}.
The `fiducial' qualifier is introduced because
it relates to a statement on a fixed parameter, and not on a traditional random variable (such as the
measurement $x$).~\footnote{Further to the interpretation of fiducial confidence intervals,
\cite{fisher1935} attempted to introduce the concept of \emph{fiducial probability distribution}
on the parameter $\theta$, leveraging the formal similarity between \eqref{eq:UL} and \eqref{eq:UL2}
\citep[see also discussion in Sec. 12.4 of ][]{wilks1962}. Such concept has not gained general acceptance, 
also given certain difficulties with multi--variable problems \citep[see, e.g.][]{tukey1957}.}
The fiducial confidence interval $S(x)$ necessarily depends on the measurement $x$ \citep[see, e.g., textbook examples in ][]{rohatgi1976, bonamente2023}. 



If we take the smallest value allowed, $x=0$,
as speculated at the beginning of the section, then \eqref{eq:CIDirect} and \eqref{eq:CIClassical}
coincide, as one would expect. In general, using $z_{\alpha}$ as the one--sided z--score associated with
a residual probability $\alpha$, $P(z \geq z_{\alpha})=\alpha$ (e.g., for $\alpha=0.1,0.01, 0.001$, 
$z_{\alpha}=1.65, 2.58, 3.29)$, we can generalize these argument and
set the $1-\alpha$ sensitivity upper limit to the Gaussian parameter $\theta$ as
\begin{equation}
    \theta \leq z_{\alpha}\, \sigma.
\end{equation}

It is useful to notice that the classical confidence interval \eqref{eq:CIClassical}
associated with a given measurement $x$ could be used instead, given that all such measurements
are available in the tables. However, as pointed out by \cite{feldman1997}, a measurement
$x \leq z_{\alpha}\, \sigma$, such as the sample entry considered before, would yield a formal confidence interval that remains negative.
Given that only positive values of the $\theta=\tau_0$ parameter are physically meaningful, 
certain measurements give rise to the \emph{empty interval} problem, when the interval is intersected with the physically allowed range. This is in fact one of the reasons for the \cite{feldman1997} method,
which was presented in Sec.~\ref{sec:FC}. The `sensitivity' method can therefore be viewed as
a simplified FC method, where the actual measurement is ignored and replaced by the null--hypothesis value
of zero, and without the enforcement of the likelihood--ratio ordering of likelihoods.

\end{comment}

